Scalable Reinforcement Post-Training Beyond Static Human Prompts: Evolving Alignment via Asymmetric Self-Play

Current reinforcement learning (RL) frameworks for large language models (LLM) post-training typically assume a fixed prompt distribution, which is sub-optimal and bottlenecks scalability. Prior works have explored prompt evolving, but are often limited to the supervised fine-tuning stage, and prompts are sampled and evolved uniformly without signals. This empirical work presents a paradigm shift: Evolving Alignment via Asymmetric Self-Play (eva), that casts post-training as an infinite game with regret-based signals for 2 players: (i) a creator, who strategically samples and creates new informative prompts and (ii) a solver, who learns to produce preferred responses. eva is the first method that allows language models to adaptively create training prompts in both offline and online RL post-training. The design is simple, easy-to-use yet remarkably effective: eva sets a new SOTA on challenging benchmarks, without any extra human prompts, e.g. it boosts the win-rate of gemma-2-9b-it on Arena-Hard by 51.6% -> 60.1% for DPO and 52.6% -> 62.4% for RLOO, surpassing claude-3-opus and catching up to gemini-1.5-pro, both of which are orders of magnitude larger. Extensive experiments show eva can create effective RL curricula and is robust across ablations. We believe adaptively evolving prompts are key to designing the next-generation RL post-training scheme.

==> app-gdm/app-ablation.tex <==
\section{Additional Experimental Results (as Extensions)}\label{app:ablation}


\subsection{Experiments on Different \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{evolve}}(\textperiodcentered)} Methods}\label{app:exp-evol}

As an addition to Table~\ref{tab:main-10k}, we have experimented with three different \texttt{\small evolve}(\textperiodcentered) methods, including:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{SelfInstruct}~\citep{self-instruct}: Given seed prompts, variations are created based on criteria such as verb diversity and style blending (mixing interrogative and imperative styles). Unlike EvolInstruct~\citep{wizardlm}, which generates prompt variations sequentially, this approach generates independently. We follow the one-shot implementation in  \href{https://github.com/argilla-io/distilabel/blob/844165f25c1674076a8286d54cfe96d52c33a24e/src/distilabel/steps/tasks/self_instruct.py#L106}{\texttt{\small self\_instruct.py}} of \texttt{\small distilabel==1.4.1} and modified the instruction on conciseness so that those newly generated prompts have similar lengths compared to the seed prompts. \vspace{+1.5pt}
    \item \textbf{EvolQuality} and \textbf{EvolComplexity}~\citep{deita}: The two methods use the same evolutionary approach (\ie sequentially generating), but with slightly different meta-instructions for prompt generation, where EvolQuality asks to improve the quality (\ie helpfulness, relevance, etc) of the seed prompt and EvolComplexity asks to improve the complexity (\ie increased reasoning steps, etc) of the seed prompt. We follow the implementation in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_quality/utils.py}{\texttt{\small evol\_quality/utils.py}} and \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/evol_complexity/utils.py}{\texttt{\small evol\_complexity/utils.py}} of \texttt{\small distilabel==1.4.1}.
\end{itemize}


% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolInstruct}) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolQuality}) & \text{58.7}  & 721 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolComplexity}) & \textbf{60.6}  & 749 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small SelfInstruct}) & \text{57.2}  & 725 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using different evolving methods.}
\label{tab:evol-10k}
\end{table}
\vspace{-10pt}
% ----------

\vspace{-10pt}
\paragraph{\method~is effective under different evolving methods.} As shown in Table~\ref{tab:evol-10k}, our method brings strong performance gain without training with additional human prompts. Among the experimented methods, we find EvolComplexity shows better results. 

We believe the main strength of such method is its \textbf{simplicity}. Viewing the evolving process as $\rvx' \gets p_{\vtheta}(\cdot \mid  \rvx, \texttt{\small meta\_prompt})$, one can easily tune the meta prompt in natural language for improved performance. However, such simplicity comes at a price: (i) the main weakness is that the default method does not take \textbf{environmental feedback} into account (\eg rewards received, verbal critique on responses, etc) and relies on the pre-defined meta prompt, thus the evolving may be less directional; we encourage practitioners to consider incorporating more richer feedback during evolving (one way to formulate this is by generative optimization~\citep{textgrad,trace,trace-pre}); (ii) another weakness is that existing method is single-shot (\ie we evolve based on a single $\rvx$ each time), thus the \textbf{diversity} of the generation may be limited -- we anticipate future works improving this with multi-shot evolving by graph-based sampling. In this regard, the evolving process can be viewed as $\{\rvx'\}_{i=1}^{N} \gets p_{\vtheta}(\cdot \mid  \{\rvx\}_{i=1}^{M}, \texttt{\small meta\_prompt}, \texttt{\small env\_feedback})$.

\subsection{Experiments on Number of Iterations}\label{app:exp-iter}

As an addition to $\S$~\ref{sec:ab-cont}, we have experimented with the following settings:
\vspace{-5pt}
\begin{itemize}
    \item 10K prompts per iteration with 3 iterations.
    \item 20K prompts per iteration with 3 iterations (\ie all seed prompts are used).
    \item 60K prompts per iteration with 2 iterations (\ie all seed prompts are used).
\end{itemize}

 
Due to time constraints, we did not perform an extensive hyper-parameter search; however, we believe the results presented below sufficiently demonstrate the performance gains achieved by~\method.

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)     & 51.6  & 651  \\

$\vtheta_{1 \rightarrow 2}$: DPO (10k)     & 59.8  &   718\\

$\vtheta_{2 \rightarrow 3}$: DPO (10k)   & 61.2  & 802  \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.0}  & 787  \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.2}  & 774  \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 10k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-10k}
\end{table}
\vspace{-10pt}
% ----------


% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (20k)     & 53.2  & 625 \\

$\vtheta_{1 \rightarrow 2}$: DPO (20k)     & 47.0  & 601  \\

$\vtheta_{2 \rightarrow 3}$: DPO (20k)   & 46.8  & 564 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{59.5}  & 826 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{60.0} & 817 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{61.4} & 791 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 20k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-20k}
\end{table}
\vspace{-10pt}
% ----------

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (60k)    & 58.9  & 717 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (60k) & \text{59.6}  & 725 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{1}'}$: \hspace{-6pt} \quad + \texttt{\textbf{eva}} (60k) & \text{61.9}  & 792 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 60k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-60k}
\end{table}
\vspace{-10pt}
% ----------


\paragraph{\method~can bring robust gains with multiple iterations.} As shown in Table~\ref{tab:ab-10k},~\ref{tab:ab-20k}, and~\ref{tab:ab-60k} below, our method presents persistent performance gain over iterations, and concretely surpasses the performance by default DPO training with true human prompts. 


However, there exist diminishing marginal gains in iterative off-policy training. We ground~\method~in the iterative (off-policy) preference alignment paradigm due to its efficiency and ease of integration. However, such paradigms inherently face diminishing returns, where performance gains decrease with successive iterations, as previously observed in~\citep{self-play-gu,8fold,self-reward,cont-primary-bias}. While the generative data schedule in~\method~mitigates these challenges and extends beyond default training with human prompts (see also $\S$\ref{sec:ab-cont}), the gains can weaken over iterations. We summarize potential reasons as: (i) the \textbf{off-policy signal decay} -- as the number of examples increases, signals from the off-policy data become weaker due to distributional shift; (ii) the \textbf{loss of plasticity}, where the agent's ability to learn good policies decreases in continuing training with more iterations~\citep{cont-primary-bias}; (iii) the \textbf{ability of the solver} -- as we evolve more harder prompts, it is harder for the solver to produce preferred response (thus more explicit reasoning techniques may be needed); (iv) the \textbf{ability of the reward model} to correctly provide reward signals to responses and thus informativeness signals to prompts, as there may exists distributional mismatch.

Thus, we envision future work to build on~\method~by: (i) exploring its integration with \textbf{on-policy RLHF} (\eg instead of evolving prompts in iterations, one may evolve in batches); (ii) \textbf{enhancing solver capabilities}, such as sampling more responses during inference or leveraging meta-instructions to guide deeper reasoning; (iii) continual training of reward models for them to co-evolve with the  creators and the solvers. 









\subsubsection{Bonus Experiments on \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{rewriter}}(\textperiodcentered)} In The Loop}\label{app:exp-rewriter}

We present the basic idea here for practitioners to build upon. The motivation comes from the hypotheses derived from $\S$~\ref{app:exp-iter}: as the prompts gets harder by evolving, there may be greater demands on the solver’s capabilities \emph{compared to earlier iterations}. As such, the solver may not be naively treated the same. One may address this by either scaling  up response sampling or introducing meta-instructions to explicitly enhance the solver’s reasoning.

We design a proof-of-concept experiment \emph{w.r.t} the latter by adding \textbf{rewriter} in \method's solver step. Previously, as in Algo.~\ref{alg:i-eva} and  $\S$~\ref{sec:solver-step}, for each prompt $\rvx$, we generate multiple responses, and choose the best as $\rvy_{+}$ and the worst as $\rvy_{-}$ for preference optimization. Now, we add one more rewriting step that attempts to enhance $\rvy_{+}$ to be $\rvy'_{+}$, by applying a rewriting instruction~\citep{deita} that asks the solver to alter $\rvy_{+}$ with imporved helpfulness, relevance, reasoning depths, creativity and details while keeping the similar length. We then train with $(\rvx, \rvy'_{+}, \rvy_{-})$ for preference optimization. Table~\ref{tab:rewriter-10k} shows that adding the rewriter yields concrete performance gains over the default training method, while keeping the training budget and only slightly increasing cost for offline data generation.
% \vspace{-3pt}

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)    & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \textbf{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} with \texttt{\textbf{rewriter}} (10k) & \textbf{61.9}  & 741 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of adding \textbf{\texttt{\small rewriter}} in the \textbf{\texttt{\small solver}} step.}
\label{tab:rewriter-10k}
\end{table}
\vspace{-10pt}
% ----------



==> app-gdm/app-curr.tex <==
\section{Curriculum Visualization Over Iterations}\label{app:curr}
% \subsection{Curriculum Effect on Prompt Categories}\label{app:curr-cat}
We now present initial observations supporting the intuition in $\S$~\ref{sec:int}, where~\method~brings auto-curricula and the creator is incentivized to create new prompts that are both learnable and worth-learning.

% \begin{figure}[H]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
%         \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
%         \label{fig:dist}
%     \end{minipage}
%     \hspace{0.02\textwidth} % Adjust horizontal space as needed
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/radar-gemma.png}
%         \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
%         \label{fig:radar-gemma}
%     \end{minipage}
% \end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/bart-iter.pdf}\vspace{-3pt}
    \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification.  \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
    \label{fig:dist}
\end{figure}

\vspace{-6pt}
% \subsection{Curriculum Effect on Benchmark Performance}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.66\linewidth]{figs/radar-gemma.png}\vspace{-3pt}
    \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
    \label{fig:radar-gemma}
\end{figure}

\subsection{Complexity and Quality of Prompts Over Iterations}\label{app:curr-2}
% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering \text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity}
\end{table}
\vspace{-10pt}
% ----------

As in Table~\ref{tab:prompt-quality-complexity}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. We sample 10K prompts per iteration, and use the below prompts modified from~\cite{deita} for the complexity and quality evaluation, with \texttt{\small gemini-1.5-flash} as the scorer:

\texttt{\scriptsize > Rank the following questions according to their \textbf{quality}. Your evaluation should consider the below factors: Helpfulness, Relevance, Accuracy, Depth, Creativity, and Level of detail.
Score each response from 1 to 5: \\1: Poor quality, 2: Below average, 3: Average, 4: Good, 5: Excellent.}


\texttt{\scriptsize > Rank the following questions according to their difficulty and \textbf{complexity}. Use a fixed scoring system: \\1: Very simple, 2: Simple, 3: Moderate,  4: Difficult, 5: Very difficult.}



\section{Visualization on Prompt Selection Metric}\label{app:metric}

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-pdf.pdf}
        % \vspace{+0.00001pt}
        \caption{The probability density distributions of  informativeness metrics compared in Table~\ref{tab:ab-metric} -- they show different patterns.}
        \label{fig:metric-pdf}
    \end{minipage}
    \hspace{0.02\textwidth}
    % \hfill
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-corr.pdf}
        % \vspace{+0.00001pt}
        \caption{The correlation plot for reward advantage (ours) and reward variance -- they are only \emph{weakly} correlated.}
        \label{fig:metric-corr}
    \end{minipage}
    % \hspace{4\textwidth} % Space between the two main figures
\end{figure}

In~\method, we assign each prompt an informativeness value, which the creator will use as the weight to sample from the seed prompts for prompt synthesis. In $\S$~\ref{sec:ab-metric}, we have shown that traditional methods like reward mean and reward variance are less effective as our advantage-based informativeness proxy. The intuition is simple: advantage/regret-based proxy aligns better with the preference optimization objective. We here further illustrate that they are statistically different from other choices:\vspace{-6pt}
\begin{itemize}
    \item Figure~\ref{fig:metric-pdf}: The distribution of informativeness values shows that reward variance is heavily concentrated at lower values, reward mean is more uniformly scattered, and reward advantage achieves a better balance, providing a broader yet also focused sampling range.\vspace{+1.5pt}
    \item Figure~\ref{fig:metric-corr}: The \emph{weak correlation} between reward variance and reward advantage shows that variance \emph{cannot} serve as a substitute for advantage as a proxy for informativeness.
\end{itemize}
\vspace{-6pt}
We have discussed the contrastive curriculum hypothesis in $\S$~\ref{sec:int} to support using reward advantage in the sense that the induced samples tend to decrease the loss the most in the contrastive optimization. Furthermore, assuming the optimization algorithm can converge to the \emph{more optimal} responses, neither reward mean nor variance directly capture the learning potential of such responses -- one may easily construct cases with identical variance yet differ much in reward range -- thus variance fails to distinguish such scenarios. By contrast, reward advantage estimate inherently captures the relative improvement towards better response, and is sensitive to differences in reward range; variants of advantage estimate are commonly used in literature, and we discuss underlying principles in $\S$~\ref{app:theory}.

% specifically, \emph{max - min} mimics the worst case, while \emph{max - mean} is more akin to the Bayesian view.

% By contrast, reward advantage inherently captures the relative improvement toward the optimal response, making it sensitive to such differences in reward range. Specifically, max-min provides a worst-case guarantee by considering the full reward span, while max-mean emphasizes the potential of the more optimal response by focusing on deviations from the average.

==> app-gdm/app-downtream.tex <==
\section{Additional Experimental Results for the Main Paper}\label{app:downstream}


In general,~\method~maintains the downstream performance and is robust on reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to training sources for such reward models.
% \input{tables/tab-ab-downstream}
% \vspace{-8pt}

% \input{tables/tab-ab-rm-app}

% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\centering \textbf{Performance on Downstream tasks.}}
\label{tab:ab-downstream}
\end{table}



\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) &  \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 55.01 & 51.68  \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & 9.04 & 8.75 & 60.1  &  55.35 &    55.53 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  & \textbf{56.12} & \textbf{56.40} \\

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\centering \textbf{Effect of (pointwise) reward models.}}
\label{tab:ab-rm-app}
\end{table}
 % on relevant benchmarks
 \vspace{-8pt}

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7 & 51.58 & 42.17 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & 8.78 & \textbf{9.11} &  8.45 &  58.9 & 51.86 & 43.04 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & \textbf{52.71} & \textbf{44.52} \\

\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\centering \textbf{Effect of (pairwise) reward models.}}
\label{tab:ab-rm-sppo-app}
\end{table}
\vspace{-5pt}


==> app-gdm/app-lit.tex <==
% \newpage
\section{Extended Literature Review for Open-Ended Learning}\label{app:lit}

% \subsection{Extended Literature Review on Open-Endedness}

The design of our game-theoretic framework for language model post-training is inspired from many prior works in open-ended learning. The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that  can \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but broad enough to handle the diversity of complexity of future environments. In such curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively builds more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case (\ie most adversarial) environments.  In addition to distinctions discussed in~$\S$~\ref{sec:lit}, we here list several foundational works in this line, and encourage the LLM community to explore with more rigor and depth: \cite{schmidhuber1991possibility} presents an initial investigation into open-ended learning via self-supervised curiosity-driven exploration; \cite{poet} emphasize co-evolution of environments and agent policies by training a population of agents that adapt to and solve progressively complex challenges; \cite{paired} formally introduce the notion of Unsupervised Environment Design (UED), where a protagonist and antagonist agent pair simulates regret by competing in shared environments, driving the protagonist (the main learner) to adapt to increasingly challenging scenarios; \cite{plr} introduce Prioritized Level Replay (PLR), which uses a rolling buffer of high-regret levels to dynamically adjust the training curriculum, and selects levels with the higher learning potential; \cite{accel} further propose improvements by editing previously high-regret levels; \cite{open-endedness} present a formal definition for open-ended system with respect to \emph{novelty} and \emph{learnability}, that generalizes various systems, \eg AlphaGo~\citep{alphago}, AdA~\citep{team2021open}, etc.
% \vspace{-10pt}

% Our focus was on classical, seminal, and directly relevant works. We welcome suggestions for any other references we may have missed that can enhance our citations -- please feel free to reach out.


==> app-gdm/app-loss.tex <==
\section{Plug-In Loss Functions Used in Main Results}~\label{app:loss}
\vspace{-.8cm}
\begin{table}[H]
\centering
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{With Reference Model}    \\ \midrule
DPO~\citep{dpo}  &  $\ell_{\beta}(\pi_{\vtheta})  = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_\vtheta};  {\pi_{\text{ref}}}}^{\rvx} \Bigr)\Bigr] \textcolor{lightgray}{:= - \log \left[\sigma\left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}- \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \right)\right]} $                   \\


SPPO~\citep{self-play-gu}  & $\ell_{\beta}(\pi_{\vtheta})  = - \log \left[\sigma\left( \left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)} - \frac{1}{2}\right)^2 + \left( \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}+ \frac{1}{2}\right)^2  \right)\right]$  \\ 
\midrule
\multicolumn{2}{c}{Without Reference Model} \\ \midrule
SimPO~\citep{simpo} &  $ \ell_{\beta, \alpha}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_{\theta}^{1/|\rvy|}};  1}^{\rvx} - \alpha \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \frac{\beta}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx) -  \frac{\beta}{|\rvy_{-}|} \log \pi_{\vtheta}(\rvy_{-} | \rvx) -\alpha \right)\right]} $                   \\
ORPO~\citep{orpo} &  $ \ell_{\lambda}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\lambda \cdot  \Delta_{\text{odds}_{\vtheta};  1}^{\rvx}  \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \lambda \cdot \log \frac{\text{odds}_{\vtheta}(\rvy_{+} | \rvx)}{\text{odds}_{\vtheta}(\rvy_{-} | \rvx)}  \right)\right]} $\textcolor{lightgray}{, where $\text{odds}_{\vtheta}=\frac{\pi_\vtheta}{1 - \pi_{\vtheta}}$}                   \\
% ORPO~\citep{orpo} &   $\ell_{\lambda}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphslate{\dlogodds} \right)\right]$              \\ 
\bottomrule
\end{tabular}%
}
\caption{Direct preference alignment algorithms used in the main experiments. In parameter tuning, we include an additional negative log-likelihood loss for chosen responses (\ie~$\frac{\gamma}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx)$).}
\label{tab:offline}
\end{table}

==> app-gdm/app-prompt-examples.tex <==
\section{Examples on Prompts and Model Generations}\label{app:examples}
\vspace{-12pt}

% ------------------
\begin{figure}[H]
    % \centering
    % \begin{minipage}{0.39\textwidth}
    \centering
    \includegraphics[width=0.4\linewidth]{figs/example-prompt.png}
    \vspace{-4pt}
    \caption{The initial prompt distribution of AlpacaEval by \texttt{\small bart-large-mnli} with 0-shot classification, which is imbalanced. For the reward distribution, the category with lowest average reward has the highest  reward gap (\ie the default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
    % \end{minipage}
\end{figure}
% \vspace{-12pt}
% ------------------




% ------------------
% \begin{table}[H]
% \centering
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}r p{14cm}@{}}
% \toprule
% \rowcolor{lightgray!16}
% \multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small If a man smokes 1000 cigarettes a day, why is he getting healthier?} \\ \midrule
% \texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Elaborate on the seemingly paradoxical situation where an individual consumes 1000 cigarettes daily yet exhibits signs of improving health, delineating the factors that could underlie such an unexpected outcome.} \\
% \texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Discuss the conundrum of a person drinking a gallon of caffeinated coffee every hour but displaying unusually deep and restful sleep patterns, exploring possible explanations for this unusual phenomenon.} \\
% \texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Examine the paradox of an individual who ingests a gallon of caffeine-laden coffee hourly yet exhibits signs of profoundly tranquil slumber, delving into potential theories that could elucidate this atypical occurrence, and considering the role of genetic predispositions in such a scenario.} \\
% \texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Analyze the conundrum of a person consuming an entire gallon of heavily caffeinated coffee every single hour and yet demonstrating the ability to fall into a state of deep sleep, exploring plausible hypotheses that could illuminate this unusual event, including an assessment of how genetic factors might influence this ability, and include an evaluation of the impact of acquired tolerance to caffeine over time.} \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-4pt}
% % \caption{Examples of evolved prompts from AlpacaEval.}
% \label{tab:prompt-evol}
% \end{table}
% ------------------

\vspace{-10pt}

% ------------------
\begin{table}[H]
\centering
\resizebox{.66\columnwidth}{!}{%
\begin{tabular}{@{}r p{12.6cm}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small Write me the code for a distributed transaction manager.\textbackslash nThink step by step and use pseudo code first.\textbackslash nThen, define interfaces for all involved actors and entities.\textbackslash nUse Rational Unified approach for this part.\textbackslash n\textbackslash nOnly then move on to the actual implementation, class-by-class, and method-by-method.\textbackslash nMake the code be implemented in C\# and follow SOLID principles.} \\ \midrule
\texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Craft a suite of syntax for a distributed transaction coordinator. Start with a sequential breakdown in pseudocode format. Following that, establish the protocols for communication and interaction amongst the various participants and components, incorporating the Rational Unified Process methodology.\textbackslash n\textbackslash nProceed thereafter to the concrete creation, detailing each class and function. Ensure that the final C\# code adheres to the precepts of SOLID and is annotated for clarification and maintainability purposes.} \\
\texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Devise a comprehensive set of directives and structures for a distributed transaction coordinator architecture. Initiate by formulating a step-by-step algorithmic decomposition in pseudocode. Subsequently, delineate the frameworks for dialog and cooperation between the numerous entities and elements, utilizing the tenets of the Rational Unified Process methodology.\textbackslash n\textbackslash nContinue to the actual generation of the code, meticulously detailing every class and corresponding method. Guarantee that the culminating C\# code is in strict compliance with SOLID principles and is supplemented with descriptive commentary to enhance future clarity and upkeep, while also validating the code against a set of unit tests to ensure robust functionality.} \\
\texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Commence by constructing an algorithm in pseudocode that meticulously breaks down the sequential stages for a distributed transaction coordinator system. Progress by outlining the communication protocols and collaborative mechanisms among the myriad components, adhering to the Rational Unified Process approach.\textbackslash n\textbackslash nAdvance to crafting the code in C\#, ensuring each class and method is elaborated with precision, aligning with SOLID design principles. Integrate thorough comments for heightened maintainability and conduct comprehensive unit testing for assured operational integrity.} \\
\texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Design a detailed flowchart that represents the intricate steps of an orchestration engine for managing microservices in a cloud-native environment. Begin by detailing the service discovery, load balancing, and fault tolerance strategies, while incorporating the DevOps philosophy.\textbackslash n\textbackslash nProceed by developing the implementation in Java, focusing on clean, modular code following object-oriented programming best practices. Accompany your code with clear documentation for easy understanding and perform rigorous integration testing to guarantee robustness.} \\ \bottomrule
\end{tabular}%
}
% \vspace{-4pt}
\caption{Examples of evolved prompts from AlpacaEval. We suggest practitioners to include generated responses with oracle rewards and self-critique in the context for better prompt evolving, which is helpful for mitigating the effect of potential self-consuming loops in synthetic data training.}
\label{tab:prompt-evol-2}
\end{table}
% ------------------






\newpage

\hspace{0pt}
\vfill

\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} \texttt{\small When a number is divided by 10, the remainder is 4. What is the remainder when twice the number is divided by 4?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
* "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
* Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
* (20*k + 8) divided by 4 is (20*k)/4 + 8/4 = 5*k + 2\newline
4. Find the remainder:\newline
* Since 5*k is a multiple of 4, the remainder when twice the number is divided by 4 is 2.\newline
Let me know if you'd like to try another example!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}} 
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
- "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
- Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
- When (20*k + 8) is divided by 4, the 20*k term is perfectly divisible by 4.\newline
- The remainder will be the same as the remainder when 8 is divided by 4, which is 0.\newline
Therefore, the remainder when twice the number is divided by 4 is 0.}
\end{tabular} \\ \midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} \texttt{\small What about when twice the number is divided by 5?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 is (20*k)/5 + 8/5 = 4*k + 1.6\newline
3. Find the remainder: Since 4*k is a multiple of 5, the remainder when twice the number is divided by 5 is 1.\newline
Let me know if you have any more number theory puzzles!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. \text{Twice the number:} We know twice the number is 20*k + 8 (from the previous steps).\newline
2. \text{Divide by 5:} \newline
\ \ \ * 20*k is divisible by 5.\newline
\ \ \ * 8 divided by 5 leaves a remainder of 3.\newline
Therefore, the remainder when twice the number is divided by 5 is 3.}
\end{tabular} \\ 

\midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's response is incorrect. The assistant incorrectly calculated the remainder when twice the number is divided by 5. The assistant calculated the decimal part of the division operation, not the remainder. The correct calculation should be (20n + 8) \% 5 = (20n \% 5) + (8 \% 5) = 0 + 3 = 3. Therefore, the remainder when twice the number is divided by 5 is 3, not 1 as the assistant stated.\newline
\newline
The corrected response would be:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 gives us a remainder of (20*k \% 5) + (8 \% 5) = 0 + 3 = 3.\newline
3. Find the remainder: The remainder when twice the number is divided by 5 is 3.\newline
\newline
Rating: [[3]], "score": 3, "turn": 2, "tstamp": 1722737011.7768948}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's answer is correct and matches the reference answer. The assistant correctly explains that twice the number is 20*k + 8 and that when this is divided by 5, the remainder is 3. The assistant's explanation is clear and easy to understand, making it helpful for the user. There are no mistakes to correct.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846518.5543818}

\end{tabular} \\ 

% \sbt{Judgment for gemma-2-9b-it-dpo} & \sbt{Judgment for gemma-2-9b-it-dpo-eva} \\ 

\bottomrule
\end{tabular}%
}
\caption{\centering Comparison of model generations on examples from MT-Bench.}
\label{tab:gen-0}
\end{table}


\vfill
\hspace{0pt}




% ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-2}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
\hspace{0pt}
\vfill
\input{app/tab-gen-3}
\vfill
\hspace{0pt}
% % ------------------

% ------------------
% \newpage
\hspace{0pt}
\vfill
\input{app/tab-gen-1}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-4}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-5}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
% \input{app/tab-gen-6}
% \vfill
% \hspace{0pt}
% % ------------------

==> app-gdm/app-reproduce.tex <==
\section{Details on Reproducibility}\label{app:reproduce}
Our code is built based on many open-source packages, and we sincerely thank every developer and contributor of these projects for their efforts and contributions to the community. 

As mentioned, our code base is made to be simple to use for practitioners, requiring \textbf{only a creator module addition} within the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline.

\vspace{-10pt}
\paragraph{Hyperparameter settings.} We follow the original hyperparameter settings as in~\citep{orpo,simpo,self-play-gu}, default to be:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
$\lambda$                                                      & /      & 0.5      & /      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1024   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
\bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-main-params}
\end{table}

\vspace{-10pt}
\paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-reward}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
    \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
    % \item ...
\end{itemize}

For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this and other plug-in evolving methods. For solver we generate 6 responses per prompt. We use 42 as the random seed.

% \paragraph{Computation environments.} 
\vspace{-10pt}
\paragraph{Software environments.} All experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve Gemini (default to be \texttt{\small gemini-1.5-pro}) and transformers models (default to be \texttt{\small gemma-2-9b-it}). For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. 

% We include main Appendix following references, also in \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}.

==> app-gdm/app-theory-clean.tex <==
In~\secref{app:theory-1}, we present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}



The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.



\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 


Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.


\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.

\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber

\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.




We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.




\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


==> app-gdm/app-theory-old.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

\subsection{Connections in Open-Ended RLHF, Minimax Game and the Proxy}\label{app:intuition}

We provide an extended discussion on $\S$~\ref{sec:method} to make the explanation more coherent and easy-to-understand. Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{cred}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tg{\pi_{\phi}(\rvx)} \cdot \tc{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}), which is a special case if $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expand Eq.~\ref{eq:rlhf-joint-}:

\resizebox{\textwidth}{!}{$
\max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cred}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\textit{KL}}\bigr[\textcolor{cred}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
- \beta \cdot \textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}. \nonumber 
$}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


To clarify, while $\pi_{\text{SFT}}(\cdot)$ refers to the supervised trained model~\citep{rlhf}, the newly proposed $p_{\text{ref}}$ represents an \textbf{open-ended} and potentially intractable probability measure over all possible tasks (instatiated \emph{via} prompts) or user prompts -- note it is not the static training prompt distribution. Here, the regularization $\textcolor{black}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by generating new tasks for self-training and self-improvement, instead of optimizing over a static, pre-defined prompt set. The non-trivial part is on solving this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

In the next, we will provide a step-by-step derivation leading to our Algo.~\ref{alg:i-eva}. To begin with, we first discuss how prior works tractably solve similar open-ended learning problems via two-player game formulation. Next, we formally present the new objective, and discuss how to tractably solve it in our specific setting.

\subsection{Designing Two-Player Games for Open-Ended Environment Design}
The underlying idea is straightforward, while we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$, we are able to create a series of environments. The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

\textcolor{red}{TODO: unifying the theorems/notations in previous literature. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }
\begin{itemize}
    \item \cite{poet}:
    \item \cite{paired}:
    \item \cite{plr}: scoring by generalized advantage estimation
    \item \cite{dcd}:
    \item \cite{accel}:
\end{itemize}

\subsection{Regret Formulation for Open-Ended RLHF}

\subsubsection{Advantage-Based Regret and Approximation by EvolInstruct: The Creator Step}

\subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

\newpage



\textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



 Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
\begin{itemize}
    \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \end{itemize}
    \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \end{itemize}
\end{itemize}

% \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

The regret objective is defined as
\begin{align}
\operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
\end{align}
% $$
% \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% $$

At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
\begin{align}
    \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
\end{align}
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

This approximation introduces two practical advantages:
\begin{enumerate}
    \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
    \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
\end{enumerate}

This deviates from the theoretical Open-Ended RLHF objective. In particular:
\begin{itemize}
    \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
    \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
\end{itemize}

Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


\subsection{KL-Regularized Regret}\label{app:kl}
For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

% This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% \begin{itemize}
%     \item 
%     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% \end{itemize}

\subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
\textcolor{red}{TODO: add derivation to better justify this approximation.}
In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
\begin{align}
    \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
\end{align}

This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
\begin{itemize}
    \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
    \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
    \begin{itemize}
        \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
        \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
    \end{itemize}
    \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
\end{itemize}


We justify this simplification as follows:
\begin{itemize}
    \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
    \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
    \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
\end{itemize}

We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> app-gdm/app-theory.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

This is an extended version of $\S$~\ref{sec:method}. In~\secref{app:theory-1}, we re-present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}

% \resizebox{\textwidth}{!}{$
% \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\text{KL}}\bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
% - \beta \cdot \emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}. \nonumber 
% $}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\vspace{-5pt}
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon. \vspace{+1.5pt}
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.

% A common misunderstanding may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks -- a conceptual target derived from the \textit{underspecified distribution}. As shown in Fig.~\ref{fig:metric-corr}, the initial prompt distribution can be defined along several dimensions (\eg the number or complexity of coding problems). A potential creator policy can be made to modify these dimensions to explore new training distributions.





% The probability matching term $\textcolor{cgreen}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities~\citep{jiang-thesis}, instead of constrained in a static, pre-defined prompt set. 
% The non-trivial part is thus on approaching this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

% The following serves as an illustration from Definition~\ref{eq:rlhf-joint} to  Algorithm~\ref{alg:i-eva}, especially on 

% As a background, we first discuss how prior works/heuristics solve similar open-ended learning problems. Next, we formally present the new objective under a game, and discuss how to tractably solve it in our specific setting.

\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
 \vspace{-5pt}
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{\vspace{-40pt}We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\vspace{-5pt}
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on  high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance. There is an additional filtering step: they do not directly train on newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 
% \begin{itemize}
%     \item \textbf{Regret approximation}: the same as~\citep{plr} -- the positive value loss.
%     \item \textbf{Environment generation}: 
% \end{itemize}







 


% \cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones.


% (TODO: give an overview on this setting; our creator follows the similar setting by identifying the high-regret levels and then making edits with them combining a buffer.)
% Later on, researchers explore more \emph{curriclum}-driven approach, especially through adversarial training~\citep{adr} with minimax objective

% . The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

% \textcolor{red}{This section is about heuristics on distributional matching with a game setting. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }

% \subsubsection{Reformulating Constrained Optimization to Minimax Optimization}

% \newpage
\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric  game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in future.

\vspace{-10pt}
\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
    % &= \frac{1}{1 + \exp \left(- (r\left(\mathbf{x}, \mathbf{y}^w\right) - r\left(\mathbf{x}, \mathbf{y}^l\right))\right)} \\
    % &= \sigma \left(r\left(\mathbf{x}, \mathbf{y}^+\right) - r\left(\mathbf{x}, \mathbf{y}^-\right)\right). \label{eq:bt}
\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\vspace{-10pt}
\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

% Thus the regret with regard to the KL-constrained optimal policy is:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \nonumber
% \end{align}


% Assuming $\rvy_+, \rvy_-$ are correctly labeled by an \textit{oracle reward model} $r(\cdot, \cdot)$, the direct preference optimization objective is:
% \begin{align}
%     \mathcal{L}_{\text{DPO}}=-\mathbb{E}_{\rvx \sim \calD, (\rvy_+, \rvy_-) \sim \pi_{\vtheta}(\cdot \mid \rvx)}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_+ \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_+ \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_- \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_- \mid \rvx\right)}\right)\right]. \nonumber
% \end{align}


We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\vspace{-10pt}
\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.


\vspace{-10pt}
\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them, then mixing with a buffer of the original set to form the new training distribution at each iteration.

% While there exist other approximations choices (see our summarization in Table~\ref{tab:info-metric}), we justify our choice for the minimax regret strategy under the context of contrastive preference optimization.

% (High-level idea: the regret is bounded by the range; we first define the range (the underlying assumption is suffient sampling and correct labeling) then show)

% The expected reward under the policy $\pi_\vtheta$ is given by:
% \begin{align}
%     \mathbb{E}_{\rvy \sim \pi_\vtheta(\cdot \mid \rvx)}[r(\rvx, \rvy)] = \sum_{\rvy} \pi_\vtheta(\rvy \mid \rvx) r(\rvx, \rvy), \nonumber
% \end{align}
% and it satisfies the bound:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+). \nonumber
% \end{align}
% Our objective is to show that with high probability, there is $\operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx)$.
% \begin{align}
%     \mathbb{P}\left(\left|\hat{r}_{\mathrm{KL}}-\mathrm{E}_{\mathbf{y} \sim \pi_{\mathrm{kL}}^t}[r(\mathrm{x}, \mathrm{y})]\right| \geq \varepsilon\right) \leq 2 \exp \left(-\frac{2 n \varepsilon^2}{\left(r_{\text {max }}-r_{\text {min }}\right)^2}\right)
% \end{align}

% (TODO: show that as we optimize, the upper bound of info(x) on the regret would be tighter. thus we effectively achieves high-regret seeking. Then discuss the heuristic generation by making edits through evolinstruct etc.)
% Similarly, for the KL-optimal policy $\pi^\star_{\text{KL}}(\rvy \mid \rvx)$, we have:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+).
% \end{align}

% The KL-regularized regret is defined as:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) = \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] - \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)].
% \end{align}

% Using the bounds above, the regret satisfies:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Define the range $\text{info}_\vtheta(\rvx)$ as:
% \begin{align}
%     \text{info}_\vtheta(\rvx) = r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Thus, the regret is bounded by the range:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx).
% \end{align}


% since the regret in Eq.~\ref{eq:KL-regret} is not directly calculable. Specifically, we choose to approximate the regret as:



% A re-formulation of the reward is:
% \begin{align}
%     r(\rvx, \rvy)=r_E(\rvx, \rvy)-\beta\bigr(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\bigr).
% \end{align}




% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}



% \subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

% In this section, we discuss connection between the regret minimization objective and the contrastive preference optimization objective.
% % \textcolor{red}{TODO: derive regret objective and DPO optimization, checking~\citep{cpl}; the KL is explicitly solved.}

% High-level idea: By the Bellman equation, we have:
% \begin{align}
%     A^*(s, a)=Q^*(s, a)-V^*(s, a)=r(s, a)+\gamma \mathbb{E}_{s^{\prime}}\left[V^*\left(s^{\prime}\right)\right]-V^*(s)
% \end{align}

% In the bandit setting, the negated regret :
% \begin{align}
%     A^{\star}(\rvx, \rvy) &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy),\\
%     & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr].
% \end{align}

% The preference model thus becomes:
% \begin{align}
% P_A \left[\sigma^{+} \succ \sigma^{-}\right] & =\frac{\exp r_E\left(s, a^{+}\right)-V^*(s)}{\exp r_E\left(s, a^{+}\right)-V^*(s)+\exp r_E\left(s, a^{-}\right)-V^*(s)} \\
% & =\frac{\exp r_E\left(s, a^{+}\right)}{\exp r_E\left(s, a^{+}\right)+\exp r_E\left(s, a^{-}\right)}
% \end{align}

% (TODO: show the regret-based preference is equivalent to the DPO objective, thus we implicitly minimizes a function of the regret)

% Under the RLHF framework, a reformulation of the reward function is:
% \begin{align}
%     r'(\rvx, \rvy)=r(\rvx, \rvy)-\beta\left(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\right).
% \end{align}

% \textcolor{red}{TODO: write a theoretical version with the above and a practical version with only the true reward model.}

% \subsubsection{Regret Approximation by EvolInstruct: The Creator Step}
% \textcolor{red}{TODO: derive advantage-based regret approximation; then we further approximated it with reward function and proximal editing on seed prompts, thus we do not tractably solve the KL term.}


% (This should be the reward that we use, however we directly take the reward inside)


% \newpage



% \textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

% While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



%  Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

% To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
% \begin{itemize}
%     \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \end{itemize}
%     \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \end{itemize}
% \end{itemize}

% % \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

% This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% The regret objective is defined as
% \begin{align}
% \operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
% \end{align}
% % $$
% % \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% % $$

% At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
% \begin{align}
%     \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}
% % \begin{align}
% %     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% % \end{align}

% This approximation introduces two practical advantages:
% \begin{enumerate}
%     \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
%     \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
% \end{enumerate}

% This deviates from the theoretical Open-Ended RLHF objective. In particular:
% \begin{itemize}
%     \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
%     \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
% \end{itemize}

% Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


% \subsection{KL-Regularized Regret}\label{app:kl}
% For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% % This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% % \begin{itemize}
% %     \item 
% %     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% % \end{itemize}

% \subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
% \textcolor{red}{TODO: add derivation to better justify this approximation.}
% In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
% \begin{align}
%     \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
% \end{align}

% This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
% \begin{itemize}
%     \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
%     \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
%     \begin{itemize}
%         \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
%         \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
%     \end{itemize}
%     \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
% \end{itemize}


% We justify this simplification as follows:
% \begin{itemize}
%     \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
%     \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
%     \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
% \end{itemize}

% We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

% Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> app-gdm/tab-gen-1.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\tiny Implement a function to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\tiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \ nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \ The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  \ if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  \ imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  \ imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\  \ if i == 0:\textbackslash n\  \ max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  \ return max\_left\textbackslash n\textbackslash n\  \ if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  \ elif j == n:\textbackslash n\  \ min\_right = nums1[i]\textbackslash n\  \ else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1` into two parts: `nums1[0:i]` and `nums1[i:m]`.\textbackslash n\  \ - `j` is calculated to divide `nums2` so that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Partition:**\textbackslash n\  \ - We compare elements at the boundaries of the partitions to see if `i` is in the correct position:\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, `i` is too small, so we move `imin` to `i + 1`.\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move `imax` to `i - 1`.\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - Once `i` is in the correct position, we find:\textbackslash n\  \ - `max\_left`: The maximum element in the left partitions of both arrays.\textbackslash n\  \ - `min\_right`: The minimum element in the right partitions of both arrays.\textbackslash n\  \ - If the total length is odd, `max\_left` is the median.\textbackslash n\  \ - If the total length is even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we perform binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we only use a constant amount of extra space for variables.
}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\tiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\ if i == 0:\textbackslash n\  max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  return max\_left\textbackslash n\textbackslash n\  if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  elif j == n:\textbackslash n\  min\_right = nums1[i]\textbackslash n\  else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1`, and `j` divides `nums2` such that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Search Range:**\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, it means `i` is too small, so we need to move the partition point in `nums1` to the right (`imin = i + 1`).\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move it to the left (`imax = i - 1`).\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - When the correct partition is found (`i` is in the right position), we find:\textbackslash n\  \ - `max\_left`: The maximum element on the left side of the partition.\textbackslash n\  \ - `min\_right`: The minimum element on the right side of the partition.\textbackslash n\  \ - If the total number of elements is odd, `max\_left` is the median.\textbackslash n\  \ - If even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we are performing binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we are only using a constant amount of extra space for variables.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\tiny 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\tiny \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\tiny You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\tiny }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny Judgment} \stt{\tiny (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides an example usage of the function, which is helpful for understanding how to use it. The assistant's code is a different implementation than the reference answer, but it achieves the same result and meets the same complexity requirements. \newline However, the assistant's answer does not address the user's original question about achieving O(n) time complexity. The assistant should have clarified that it's not possible to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity, as stated in the reference answer. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722737514.2011044}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides a step-by-step explanation of the code, which is very helpful for understanding the logic behind the solution. The assistant's code is also correct and will correctly find the median of two sorted arrays of different sizes. Therefore, there are no corrections needed for the assistant's response.\newline\newline Rating: [[10]], "score": 10, "turn": 1, "tstamp": 1722846533.772981}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-1}
\end{table}

==> app-gdm/tab-gen-2.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Imagine you are writing a blog post comparing two popular smartphone models. Develop an outline for the blog post, including key points and subheadings to effectively compare and contrast the features, performance, and user experience of the two models. Please answer in fewer than 200 words.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize \#\# Smartphone Showdown: [Model A] vs. [Model B]\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce the two smartphone models being compared, highlighting their popularity and target audience.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, and display technology (e.g., OLED, LCD).\textbackslash n* Design aesthetics and user preferences.\textbackslash n\textbackslash n**III. Performance and Specs**\textbackslash n* Processor, RAM, and storage comparison.\textbackslash n* Benchmark scores and real-world performance analysis.\textbackslash n* Battery life and charging capabilities.\textbackslash n\textbackslash n**IV. Camera Capabilities**\textbackslash n* Rear and front camera specs (megapixels, aperture, features).\textbackslash n* Image quality comparison in various lighting conditions.\textbackslash n* Video recording capabilities.\textbackslash n\textbackslash n**V. Software and User Experience**\textbackslash n* Operating system and user interface comparison.\textbackslash n* App ecosystem and availability.\textbackslash n* Software features and customization options.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare the price points of both models.\textbackslash n* Analyze the value proposition based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and similarities.\textbackslash n* Recommend the best phone for specific user profiles (e.g., budget-conscious, photography enthusiasts, gamers).}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize \#\# iPhone 14 Pro vs. Samsung Galaxy S23: Which Flagship Reigns Supreme?\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce both smartphones and their position in the market.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, refresh rate, and display technology (OLED vs. Super AMOLED).\textbackslash n* Design aesthetics and unique features (e.g., notch vs. punch-hole, color options).\textbackslash n\textbackslash n**III. Performance and Camera**\textbackslash n* Processor comparison (Apple A16 Bionic vs. Snapdragon 8 Gen 2).\textbackslash n* RAM and storage options.\textbackslash n* Camera specs: megapixels, lens types, aperture, and special features (e.g., telephoto, macro).\textbackslash n* Image quality comparison based on sample photos and user reviews.\textbackslash n\textbackslash n**IV. Software and User Experience**\textbackslash n* Operating systems: iOS 16 vs. Android 13.\textbackslash n* User interface comparison: intuitiveness, customization options, and app ecosystems.\textbackslash n* Special features: Face ID vs. in-display fingerprint sensor, voice assistants.\textbackslash n\textbackslash n**V. Battery Life and Charging**\textbackslash n* Battery capacity and real-world usage comparison.\textbackslash n* Fast charging speeds and wireless charging capabilities.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare starting prices and different storage configurations.\textbackslash n* Assess the overall value for money based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and strengths of each phone.\textbackslash n* Recommend the best phone for specific user types (e.g., photography enthusiasts, gamers, budget-conscious consumers).}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize Take your previous response and rephrase it as a limerick.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize Two phones, a showdown so grand,\textbackslash n[Model A] and [Model B], hand in hand.\textbackslash nDesign, specs, and price,\textbackslash nWe'll analyze nice,\textbackslash nTo help you choose, understand?\textbackslash n\textbackslash nLet me know if you'd like me to try filling in the bracketed parts with specific model names!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize \textbackslash nTwo phones, a Pro and a Galaxy,\textbackslash nFor flagships, they truly are spacy.\textbackslash nWith cameras and screens,\textbackslash nAnd processors keen,\textbackslash nWhich one wins? Read on, and be savvy! \textbackslash nLet me know if you'd like another limerick!}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The user asked the assistant to rephrase the previous response, which was a detailed outline for a blog post, into a limerick. The assistant successfully did so, maintaining the essence of the original response in a limerick format. The assistant also offered to further customize the limerick by filling in the bracketed parts with specific model names, showing a willingness to provide additional detail if needed. However, the limerick does not fully capture the depth and detail of the original response, which is understandable given the constraints of the limerick format. \newline\newline Rating: [[8]], "score": 8, "turn": 2, "tstamp": 1722737024.0327556}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The assistant successfully rephrased the previous response, which was a detailed outline for a blog post comparing two smartphone models, into a limerick. The limerick is playful and engaging, and it maintains the essence of the original response, which is to compare the two phones and help the reader make an informed decision. The assistant also offers to create another limerick if the user wants, showing a willingness to continue the interaction. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846542.9437995}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-2}
\end{table}

==> app-gdm/tab-gen-3.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Each problem consists of three statements. Based on the first two statements, the third statement may be true, false, or uncertain.\textbackslash n1. Oranges cost more than apples.\textbackslash n2. Oranges cost less than bananas.\textbackslash n3. Bananas cost more than apples and bananas cost more than orange.\textbackslash nIf the first two statements are true, then the third statement is?}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nStatement 3 is **partially true**.\textbackslash n\textbackslash n* The part "Bananas > Apples" is true based on our price order.\textbackslash n* The part "Bananas > Oranges" is also true based on our price order.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThese statements tell us that bananas are the most expensive, then oranges, and apples are the least expensive.\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nSince bananas are indeed more expensive than both apples and oranges, statement 3 is **true**.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize If the third statement is true. Is the first statement true, false, or uncertain? Please explain.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, the first statement is **false**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** States that bananas cost more than both apples AND oranges.\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples.\textbackslash n\textbackslash n* **Statement 1:** States that oranges cost more than apples.\textbackslash n\textbackslash nIf bananas are the most expensive, and oranges are second, then oranges cannot be more expensive than apples.\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other logic puzzles!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, then the first statement is **uncertain**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nThis tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges.\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples\textbackslash n\textbackslash nThis statement claims oranges are more expensive than apples.\textbackslash n\textbackslash nStatement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is incorrect. The assistant states that if the third statement is true, the first statement is false. However, the third statement only establishes that bananas cost more than both apples and oranges. It does not provide information about the relative costs of apples and oranges. Therefore, the first statement could be true (if oranges cost more than apples), false (if oranges cost less than apples), or uncertain (if oranges and apples cost the same). The assistant's explanation is flawed because it incorrectly assumes that the order of costs must be Bananas > Oranges > Apples, when in fact the order could also be Bananas > Apples = Oranges or Bananas > Apples > Oranges. \textbackslash n\textbackslash nCorrected Assistant's Answer: If the third statement is true, then bananas cost more than apples and bananas cost more than oranges. This means that oranges could still cost more than apples, making the first statement true. However, it's also possible that oranges and apples have the same cost, which would make the first statement false. Therefore, based on the third statement alone, the first statement is uncertain.\newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737017.2808955}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is correct and helpful. The assistant explains that the first statement is uncertain if the third statement is true, which aligns with the reference answer. The assistant provides a clear explanation of why this is the case, stating that the third statement doesn't contradict the first statement, but it also doesn't confirm it. Therefore, the assistant's response is accurate and informative.\textbackslash n\textbackslash nThe assistant's response: "If the third statement is true, then the first statement is **uncertain**. Here's why: Statement 3: Bananas > Apples AND Bananas > Oranges. This tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges. Statement 1: Oranges > Apples. This statement claims oranges are more expensive than apples. Statement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846527.2339694}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app-gdm/tab-gen-4.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize You are given two sorted lists of size m and n. Implement a function to find the kth smallest element in the union of the two lists with linear complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\  \ """\textbackslash n\  \ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \  list1: The first sorted list.\textbackslash n\  \  list2: The second sorted list.\textbackslash n\  \  k: The desired kth smallest element.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \  The kth smallest element in the union of the two lists.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(list1), len(list2)\textbackslash n\  \ i, j = 0, 0\textbackslash n\  \ min\_heap = []\  \textbackslash n\textbackslash n\ \# Build a min-heap with the first elements of both lists\textbackslash n\  \ for x in range(min(m, n)):\textbackslash n\  \  heapq.heappush(min\_heap, (list1[x], x, 0))\ \# (value, list\_index, position\_in\_list)\textbackslash n\  \  heapq.heappush(min\_heap, (list2[x], x, 1))\textbackslash n\textbackslash n\ \# Extract k smallest elements from the heap\textbackslash n\  \ for \_ in range(k - 1):\textbackslash n\  \  \_, \_, \_ = heapq.heappop(min\_heap)\textbackslash n\textbackslash n\ \# The top element of the heap is the kth smallest\textbackslash n\  \ return heapq.heappop(min\_heap)[0]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\  \ - `m` and `n` store the lengths of the input lists.\textbackslash n\  \ - `i` and `j` are pointers to track the current position in each list.\textbackslash n\  \ - `min\_heap` is a min-heap used to efficiently store and retrieve the smallest elements encountered so far.\textbackslash n\textbackslash n2. **Building the Min-Heap:**\textbackslash n\  \ - The code iterates through the first `min(m, n)` elements of both lists.\textbackslash n\  \ - For each element, a tuple `(value, list\_index, position\_in\_list)` is pushed onto the `min\_heap`. This tuple helps us keep track of the element's value, the list it belongs to, and its original position.\textbackslash n\textbackslash n3. **Extracting k-1 Smallest Elements:**\textbackslash n\  \ - The `for` loop runs `k - 1` times, effectively extracting the `k-1` smallest elements from the `min\_heap`.\textbackslash n\textbackslash n4. **Finding the kth Smallest:**\textbackslash n\  \ - After the loop, the top element of the `min\_heap` contains the `k`th smallest element.\textbackslash n\  \ - `heapq.heappop(min\_heap)` removes and returns this element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- Building the min-heap: O(m + n)\textbackslash n- Extracting k-1 elements: O(k * log(k))\textbackslash n- Overall: **O(m + n + k * log(k))**, which is approximately **O(m + n)** since `k` is usually much smaller than `m + n`.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other questions!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\ Args:\textbackslash n\  \ list1: The first sorted list.\textbackslash n\  \ list2: The second sorted list.\textbackslash n\  \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\  \ The kth smallest element in the union of the lists.\textbackslash n\ """\textbackslash n\textbackslash n\ i = 0\  \# Index for list1\textbackslash n\ j = 0\ \# Index for list2\textbackslash n\ merged = []\  \# Store the merged elements\textbackslash n\textbackslash n\ while i < len(list1) and j < len(list2):\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list1\textbackslash n\ while i < len(list1):\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list2\textbackslash n\ while j < len(list2):\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ return merged[k - 1]\  \# Return the kth element (index k-1)\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash n\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `i` and `j` are index pointers for `list1` and `list2` respectively, starting at 0.\textbackslash n\ - `merged` is an empty list to store the merged sorted elements.\textbackslash n\textbackslash n2. **Merging:**\textbackslash n\ - The `while` loop continues as long as both `i` and `j` are within the bounds of their respective lists.\textbackslash n\ - In each iteration, it compares the elements at `list1[i]` and `list2[j]`.\textbackslash n\ - The smaller element is appended to `merged`, and the corresponding index (`i` or `j`) is incremented.\textbackslash n\textbackslash n3. **Adding Remaining Elements:**\textbackslash n\ - After one list is exhausted, the remaining elements from the other list are directly appended to `merged`.\textbackslash n\textbackslash n4. **Returning the kth Element:**\textbackslash n\ - Finally, `merged[k - 1]` is returned, which represents the kth smallest element in the union (remember that list indices start from 0).\textbackslash n\textbackslash n**Linear Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through each element in both lists at most once during the merging process.\textbackslash n- The time complexity is therefore O(m + n), which is linear in the total number of elements (m + n), making it efficient for large lists.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\scriptsize \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\scriptsize You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\scriptsize }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize The assistant's answer is incorrect. The user asked for a solution with linear complexity, but the assistant provided a solution with a time complexity of O(m + n + k * log(k)), which is not linear. The assistant's solution uses a min-heap, which is not necessary and adds unnecessary complexity to the solution. \newline\newline Rating: [[2]], "score": 2, "turn": 1, "tstamp": 1722737030.6411152}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize The assistant's answer is correct and helpful. It provides a Python function that implements the two-pointer approach to find the kth smallest element in the union of two sorted lists. The assistant's function is slightly different from the reference, but it achieves the same goal. The assistant's function merges the two lists into a new list and then returns the kth element from the merged list. The assistant also provides a detailed explanation of how the function works and confirms that the time complexity is linear, which is what the user asked for. However, the assistant's function uses extra space to store the merged list, which is not necessary and not as efficient as the reference. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722846543.867601}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-4}
\end{table}

==> app-gdm/tab-gen-5.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  You are right to ask! While the previous algorithm has linear time complexity, we can achieve an even better solution with **O(log(min(m, n)))** time complexity using a slightly more sophisticated approach.\textbackslash n\textbackslash nThe key idea is to leverage the sorted nature of the lists and use a **binary search** strategy.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash n\textbackslash\#\#\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ \ """\textbackslash n\ \ Finds the kth smallest element in the union of two sorted lists with O(log(min(m, n))) time complexity.\textbackslash n\textbackslash n\ \ Args:\textbackslash n\ \ list1: The first sorted list.\textbackslash n\ \ list2: The second sorted list.\textbackslash n\ \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ \ Returns:\textbackslash n\ \ The kth smallest element in the union of the lists.\textbackslash n\ \ """\textbackslash n\ \ m, n = len(list1), len(list2)\textbackslash n\ \ if m > n:\textbackslash n\ \ list1, list2, m, n = list2, list1, n, m\ \# Ensure list1 is the shorter one\textbackslash n\textbackslash n\ \ left, right = 0, m\textbackslash n\ \ while left <= right:\textbackslash n\ \ partitionX = (left + right) // 2\textbackslash n\ \ partitionY = k - partitionX\textbackslash n\textbackslash n\ \ maxLeftX = list1[partitionX - 1] if partitionX > 0 else float('-inf')\textbackslash n\ \ minRightX = list1[partitionX] if partitionX < m else float('inf')\textbackslash n\textbackslash n\ \ maxLeftY = list2[partitionY - 1] if partitionY > 0 else float('-inf')\textbackslash n\ \ minRightY = list2[partitionY] if partitionY < n else float('inf')\textbackslash n\textbackslash n\ \ if maxLeftX <= minRightY and maxLeftY <= minRightX:\textbackslash n\ if partitionX == 0:\textbackslash n\ \ return list2[partitionY - 1]\textbackslash n\ elif partitionY == 0:\textbackslash n\ \ return list1[partitionX - 1]\textbackslash n\ else:\textbackslash n\ \ return max(list1[partitionX - 1], list2[partitionY - 1])\textbackslash n\ \ elif maxLeftX > minRightY:\textbackslash n\ right = partitionX - 1\ \# Too many elements on the right side of list1\textbackslash n\ \ else:\textbackslash n\ left = partitionX + 1\ \# Too many elements on the right side of list2\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Shorten Lists:** If `list1` is longer than `list2`, swap them to ensure `list1` is always the shorter one. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\ \ - `left` and `right` pointers define the search space within `list1`.\textbackslash n\ \ - `partitionX` is the middle point in `list1`, and `partitionY` is calculated to divide the remaining elements in `list2` such that `partitionX + partitionY = k`.\textbackslash n\ \ - `maxLeftX`, `minRightX`, `maxLeftY`, and `minRightY` represent the largest element to the left and smallest element to the right of the partitions in both lists.\textbackslash n\textbackslash n3. **Comparison and Adjustment:**\textbackslash n\ \ - If the `maxLeftX` is less than or equal to `minRightY` and `maxLeftY` is less than or equal to `minRightX`, it means the kth smallest element lies within the current partitions. We return the larger of `maxLeftX` and `maxLeftY`.\textbackslash n\ \ - If `maxLeftX` is greater than `minRightY`, it indicates that we need to search in the left subarray of `list1` (i.e., decrease `right`).\textbackslash n\ \ - Otherwise, we search in the right subarray of `list1` (i.e., increase `left`).\textbackslash n\textbackslash n4. **Termination:** The binary search continues until `left` crosses `right`, indicating the correct partition has been found.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The binary search divides the search space in half at each step.\textbackslash n- Therefore, the time complexity is O(log(min(m, n))), which is significantly faster than linear time for large lists where one list is much smaller than the other.
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's first response to the user's question is incorrect. The user asked for a function to find the kth smallest element in the union of two sorted lists with linear complexity. The assistant provided a function that uses a min-heap, which has a time complexity of O(m + n + k * log(k)). This is not linear complexity, as the user requested. The assistant's second response to the user's question is also incorrect. The user asked if there exists an algorithm with better time complexity than linear. The assistant provided a function that has a time complexity of O(m + n), which is linear, not better than linear. The assistant should have provided a function that uses a binary search approach, which has a time complexity of O(log(m) + log(n)), as the reference answer correctly does. \newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737031.5033472}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's response is correct and helpful. The assistant provided a Python function that uses a binary search approach to find the kth smallest element in the union of two sorted lists. The assistant also provided a detailed explanation of how the function works, including the time complexity of the function. The assistant's answer matches the reference answer in terms of the algorithm used and the explanation provided. The assistant also correctly identified that the binary search approach has a better time complexity than the linear approach. However, the assistant's code has a minor issue. The assistant's code does not handle the case when `k` is greater than the sum of the lengths of the two lists. In such a case, the code will raise an `IndexError`. This can be fixed by adding a check at the beginning of the function to return `None` if `k` is greater than the sum of the lengths of the two lists. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846556.6828268}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-5}
\end{table}

==> app-gdm/tab-gen-6.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-6}
\end{table}

==> app-gdm/tab-gen-script.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app-gdm/tab-gen.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\small }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\small }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================



\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app-icml/app-lit-bilevel.tex <==
% \newpage
\section{Extended Literature Review in Bi-Level RLHF}\label{app:lit-bilevel}
% \vspace{-4pt}

Bi-level optimization refers to optimization problems where the cost function is defined \textit{w.r.t.} the optimal solution to another optimization problem~\citep{roger-class}. There is a recent line of works applying bi-level optimization to RLHF. While they all rely on a fixed dataset of prompts, \method~propose to dynamically update the prompt set, as in $\S$~\ref{sec:intro}. We present a detailed comparison of~\method~with~\cite{bilevel-sail,bilevel-shen,bilevel-sta-rlhf}. We  sincerely thank the anonymous reviewer for the kind  references, and welcome suggestions for any other works we may have missed.
% While those works are orthogonal to~\method, We  thank the anonymous reviewer for the kind  references, which may help address the potential distributional mismatch issues as the policy models become more powerful.

\cite{bilevel-sail} formulate iterative online RLHF as a bi-level optimization problem, where the upper-level represents the reward learning, and the lower-level represents the policy optimization. Leveraging reward re-parameterization tricks in~\cite{dpo}, \cite{bilevel-sail} reduces the problem to a single-level objective with regard to the policy. The differences of this work and our work lie in the prompt distribution and preference oracle: (i) \method~features by \textbf{dynamic prompt set generation for Open-Ended RLHF}, whereas~\citep{bilevel-sail} remains using a static prompt set; (ii) we assume the existence of the preference oracle (as discussed in $\S$~\ref{sec:exp}), while~\cite{bilevel-sail} consider online training of reward models and ablate on self-rewarding by the current LLM policy. Our usage of a pre-trained reward model follows from industrial practices~\citep{team-1,gemma2}, which is also commonly used by prior works in academia~\citep{simpo,self-play-gu}. 
% We recognize the online training of reward models (see also~\citep{rlhf-workflow}) as an orthogonal/complementary direction to the current settings of~\method~(our setting is \textbf{agnostic to the preference structure}), and encourage future works and collaborations towards it, as mentioned in $\S$~\ref{sec:conclusion}.

\cite{bilevel-sta-rlhf} provide an interesting exploration on formulating RLHF as a leader-follower game, where the language model (LM) policy is the leader and the reward model (RM) policy is the follower, and the solution is \textbf{Stackelberg equilibrium}~\citep{stackelberg,game-mbrl}, where the \emph{leader does not likewise best respond to the follower's strategy}. Here, following the curriculum RL literature~\citep{paired,accel}, we seek the \textbf{Nash equilibrium}~\citep{nash} between the creator for prompt generation and the solver for response generation. Nevertheless, the LM-RM iterative optimization may be added on top of~\method's~framework, and we look forward to future works exploring the leader-follower re-formulation of~\method.

\cite{bilevel-shen} present a rigorous theoretical work (though it does not directly involve practical post-training of large language models). The authors propose to reduce the bi-level problem to a single-level problem with a penalty-based reformulation, and apply it in the setting of LM-RM optimization within a \textit{fixed} environment, whereas~\method~focuces on dynamic prompt generation and practically train large language models with extensive empirical experiments conducted. We believe it would be interesting to adapt similar first-order optimization techniques to solve Open-Ended RLHF.

In summary, existing bi-level RLHF works focus on online optimization of both the RM and the LM (as the response policy), all with \textbf{fixed} prompt/state distribution. \method~presents an orthogonal direction on \textbf{dynamic} prompt generation for Open-Ended RLHF, with an empirical algorithm which attains state-of-the-art performance with large language models on a variety of benchmarks. It is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and mitigate potential distributional mismatch problems as we evolves for more prompts. This direction may have not been widely adopted in real-world training of language models, due to concerns about practicality~\citep{team-1,team2,gemma2,nemotron}. We look forward to future works exploring \emph{efficient} variations unifying \method\ and existing bi-level RM-LM frameworks.





==> app-icml/app-loss.tex <==
\section{Plug-In Loss Functions}~\label{app:loss}
\vspace{-.8cm}
\begin{table}[H]
\centering
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{With Reference Model}    \\ \midrule
DPO~\citep{dpo}  &  $\ell_{\beta}(\pi_{\vtheta})  = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_\vtheta};  {\pi_{\text{ref}}}}^{\rvx} \Bigr)\Bigr] \textcolor{lightgray}{:= - \log \left[\sigma\left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}- \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \right)\right]} $                   \\


SPPO~\citep{self-play-gu}  & $\ell_{\beta}(\pi_{\vtheta})  = - \log \left[\sigma\left( \left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)} - \frac{1}{2}\right)^2 + \left( \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}+ \frac{1}{2}\right)^2  \right)\right]$  \\ 
\midrule
\multicolumn{2}{c}{Without Reference Model} \\ \midrule
SimPO~\citep{simpo} &  $ \ell_{\beta, \alpha}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_{\theta}^{1/|\rvy|}};  1}^{\rvx} - \alpha \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \frac{\beta}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx) -  \frac{\beta}{|\rvy_{-}|} \log \pi_{\vtheta}(\rvy_{-} | \rvx) -\alpha \right)\right]} $                   \\
ORPO~\citep{orpo} &  $ \ell_{\lambda}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\lambda \cdot  \Delta_{\text{odds}_{\vtheta};  1}^{\rvx}  \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \lambda \cdot \log \frac{\text{odds}_{\vtheta}(\rvy_{+} | \rvx)}{\text{odds}_{\vtheta}(\rvy_{-} | \rvx)}  \right)\right]} $\textcolor{lightgray}{, where $\text{odds}_{\vtheta}=\frac{\pi_\vtheta}{1 - \pi_{\vtheta}}$}                   \\
% ORPO~\citep{orpo} &   $\ell_{\lambda}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphslate{\dlogodds} \right)\right]$              \\ 
\bottomrule
\end{tabular}%
}
\caption{Direct preference alignment algorithms used in the main experiments. In parameter tuning, we include an additional negative log-likelihood loss for chosen responses (\ie~$\frac{\gamma}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx)$).}
\label{tab:offline}
\end{table}

==> app-icml/app-rebuttal.tex <==
\newpage
\section*{Rebuttal to Reviewer ac2P}

\paragraph{Summary.} We sincerely thank the reviewer for the appreciation of~\method~and the constructive feedback. We have made every effort to throughly address the concerns. Specifically, we have:
\begin{itemize}
    \item  added experiments on  implementing \textbf{different evolving methods} and discussed relevant strengths and weaknesses in $\S$~\ref{app:exp-evol};
    \item added \textbf{visualization on the learning curriculum} in $\S$~\ref{app:curr};
    \item provided detailed discussion on \textbf{scaling up}~\method~with million-level data on larger-scale seed sets and/or inference-time scaling for synthesizing prompts.
\end{itemize}

%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 (Choice of the Evolving Method)}:  Could you explain more about the particular choice of evolution algorithm used in your implementation of eva and different potential strengths and weaknesses related to this choice?}
\end{tcolorbox}

\textbf{TL;DR:} We use EvolInstruct~\citep{wizardlm} as it is among the most easy-to-implement methods. We added new experiments w/ other methods, including SelfInstruct~\citep{self-instruct}, EvolQuality and EvolComplexity~\citep{deita}, and show that~\method~remains to be effective in $\S$~\ref{app:exp-evol}.

\textbf{Answer:}
As an addition to Table~\ref{tab:main-10k}, we have experimented with three different \texttt{\small evolve}(\textperiodcentered) methods:
\begin{itemize}
    \item \textbf{SelfInstruct}~\citep{self-instruct}: Given seed prompts, variations are created based on criteria such as verb diversity and style blending (mixing interrogative and imperative styles). Unlike EvolInstruct~\citep{wizardlm}, which generates prompt variations sequentially, this approach generates independently. We follow the one-shot implementation in  \href{https://github.com/argilla-io/distilabel/blob/844165f25c1674076a8286d54cfe96d52c33a24e/src/distilabel/steps/tasks/self_instruct.py#L106}{\texttt{\small self\_instruct.py}} of \texttt{\small distilabel==1.4.1} and modified the instruction on conciseness so that newly generated prompts have similar lengths compared to the seed prompts.
    \item \textbf{EvolQuality} and \textbf{EvolComplexity}~\citep{deita}: The two methods use the same evolutionary approach (\ie sequential generation), but with slightly different meta-instructions for prompt generation, where EvolQuality asks to improve the quality (\ie helpfulness, relevance, etc) of the seed prompt and EvolComplexity asks to improve the complexity (\ie increased reasoning steps, etc) of the seed prompt. We follow the implementation in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_quality/utils.py}{\texttt{\small evol\_quality/utils.py}} and \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/evol_complexity/utils.py}{\texttt{\small evol\_complexity/utils.py}} of \texttt{\small distilabel==1.4.1}.
\end{itemize}


% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolInstruct}) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolQuality}) & \text{58.7}  & 721 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolComplexity}) & \textbf{60.6}  & 749 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small SelfInstruct}) & \text{57.2}  & 725 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using different evolving methods.}
\label{tab:evol-10k-}
\end{table}
\vspace{-10pt}
% ----------

\paragraph{\method~is effective under different evolving methods.} As shown in Table~\ref{tab:evol-10k}, our method brings strong performance gain without training with additional human prompts. Among the experimented methods, we find EvolComplexity shows better results. 

We believe the main strength of such method is its \textbf{simplicity}. Viewing the evolving process as $\rvx' \gets p_{\vtheta}(\cdot \mid  \rvx, \texttt{\small meta\_prompt})$, one can easily tune the meta prompt in natural language for improved performance. However, such simplicity comes at a price: (i) the main weakness is that the default method does not take \textbf{environmental feedback} into account (\eg rewards received, verbal critique on responses, etc) and relies on the pre-defined meta prompt, thus the evolving may be less directional; we encourage practitioners to consider incorporating richer feedback during evolving (one way to formulate this is by generative optimization~\citep{textgrad,trace,trace-pre}); (ii) another weakness is that existing method is single-shot (\ie we evolve based on a single $\rvx$ each time), thus the \textbf{diversity} of the generation may be limited -- we anticipate future works improving this with multi-shot evolving by graph-based sampling or including diversity-related rewards in generation. In this regard, the evolving process can be viewed as $\{\rvx'\}_{i=1}^{N} \gets p_{\vtheta}(\cdot \mid  \{\rvx\}_{i=1}^{M}, \texttt{\small meta\_prompt}, \texttt{\small env\_feedback})$.
%---------------------------------

%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q2 \& Q3 (Empirical Evidence on Learning Progress and Curriculum)}:  Do you see empirical evidence of your intuition about learning progress discussed in section 3.4? It seems like some of these claims are directly testable. Could you visualize the curriculum learned in your experiments with eva? It would be very nice to get an intuition for why performance improves and what the heuristic prioritizes over time.}
\end{tcolorbox}

\textbf{Answer:} We thank the reviewer for the constructive suggestions on empirically validating the intuition. We have revised the manuscript with additional visualization on potential curriculum learned in $\S$~\ref{app:curr}. In general, we observe the creator prioritizes learning in math and coding, which brings gradual improvement on benchmark performance on relevant categories over iterations. We have attached the bar plot and radar figure here for the reviewer's reference:

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist-}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma-}
    \end{minipage}
\end{figure}

%---------------------------------

We further evaluate the complexity and quality of the prompt distributions. As in Table~\ref{tab:prompt-quality-complexity-}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. 


\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity-}
\end{table}
\vspace{-10pt}
% ----------

Implementation notes: We sample 10K prompts per iteration, and use the below prompts modified from~\cite{deita} for the complexity and quality evaluation, with \texttt{\small gemini-1.5-flash} as the generative scorer:
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Rank the following questions according to their quality. Your evaluation should consider the following factors: Helpfulness, Relevance, Accuracy, Depth, Creativity, and Level of detail.
Score each response from 1 to 5: 1: Poor quality, 2: Below average, 3: Average, 4: Good, 5: Excellent.
\end{minted}
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Ranking the following questions according to their difficulty and complexity. Use a fixed scoring system: 1: Very simple, 2: Simple, 3: Moderate,  4: Difficult, 5: Very difficult
\end{minted}




%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q4 (Scaling)}: When discussing future directions, the authors write further scaling up w/ million-level data. Can you clarify what this means? Seems like some important context is missing?}
\end{tcolorbox}

\textbf{TL;DR:} We consider (i) applying~\method~when the seed set contains million-level or more prompts; or (ii) using~\method~to robustly generate million-level or more prompts when the seed set is limited.

\textbf{Answer:} (i) The current paper uses the UltraFeedback~\citep{ultrafeedback} as the seed prompt set, which is a ten-thousands level dataset; in training practically useful large language models~\citep{gpt,team2,rest_em}, the seed prompt set is usually much larger than such a level. We believe it is an interesting direction to explore the data scaling properties of~\method~on larger seed prompt sets, in combination with our on-policy variants. (ii) On the other hand, when the seed prompt set contains only limited data (this issue is particularly concerning in hard reasoning tasks like math~\citep{leandojo}), can we still follow the data generating curriculum and synthesize million-level prompts/problems to help training, and how to robustly verify the generated prompts/problems? Beyond training-time scaling, there is also a recent trend in inference-time scaling~\citep{snell2024scaling}, however these works only consider scaling in the $\calY$ space, not the $\calX$ or the joint $(\calX, \calY)$ space. We believe synthetically scaling up the joint $(\calX, \calY)$ space to a much more larger magnitude under~\method's game-theoretic design presents a new direction worth investigating. 
%---------------------------------

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textbf{Final remarks.} We thank the reviewer once again for spending time providing constructive feedback that helps improve~\method. Please let us know if there is any other concerns or questions, and we are more than grateful to have the opportunity to learn from and discuss with you. 
\end{tcolorbox}

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.




\newpage
\section*{Rebuttal to Reviewer zxTK}

\paragraph{Summary.} We sincerely thank the reviewer for all the constructive feedback helping improving the~\method~method. In response, we have provided:
\begin{itemize}
    \item \textbf{experiments on more iterations} in $\S$~\ref{app:exp-iter};
    \item \textbf{extended discussions on the regret objective and the proxy} in $\S$~\ref{app:theory};
    \item \textbf{evidence on distinction of advantage-based metrics and variance-based ones} in $\S$~\ref{app:metric};
    \item \textbf{revised illustration of the method} in~\secref{sec:method}, and \textbf{evidence on evolving prompt distributions} (to answer it cannot ``cheat by selecting easier prompts'')  in~\secref{app:curr}.
\end{itemize}

% We believe the additional discussions and rebuttals provided have sufficiently addressed the weaknesses and questions raised by the reviewer. Please let us know if there is any additional revision needed and we would be grateful to incorporate.

We appreciate the chance to address the reviewer’s comments and have made every effort to thoroughly address the concerns and revise our manuscript accordingly. We hope that these revisions meet the reviewer’s expectations and would be grateful if the reviewer could kindly consider revise the score. 
% If there are any further suggestions, please do not hesitate to let us know.

% We have made every effort to thoroughly address your concerns and incorporate detailed insights based on your suggestions, both in our responses (above) and the revised draft.

% ---------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W1 (Running for More Iterations)}: The number of iterations in the main results is 2, with only one EVA step in each experiment, which is a little different from what the demonstration in Figure 3 shows. If the~\method~step is performed multiple times, would the results be better or worse? What is performance like when you access all data in UltraFeedback?  }
\end{tcolorbox}

\textbf{TL;DR:} We added experimental result on running more iterations with more data, and~\method~remains to be effective. We have added $\S$~\ref{app:exp-iter} in the manuscript to incorporate the reviewer's suggestion.

\textbf{Rebuttal:} As an addition to $\S$~\ref{sec:ab-cont}, we have experimented with the following settings:
\begin{itemize}
    \item 10K prompts per iteration with 3 iterations.
    \item 20K prompts per iteration with 3 iterations (\ie all seed prompts are used).
    \item 60K prompts per iteration with 2 iterations (\ie all seed prompts are used).
\end{itemize}

Due to time constraints, we did not perform an extensive hyper-parameter search; however, we believe the results presented below sufficiently demonstrate the performance gains achieved by~\method.

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)     & 51.6  & 651  \\

$\vtheta_{1 \rightarrow 2}$: DPO (10k)     & 59.8  &   718\\

$\vtheta_{2 \rightarrow 3}$: DPO (10k)   & 61.2  & 802  \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.0}  & 787  \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.2}  & 774  \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 10k prompts per iteration.}
\label{tab:ab-10k-}
\end{table}
\vspace{-10pt}
% ----------


% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (20k)     & 53.2  & 625 \\

$\vtheta_{1 \rightarrow 2}$: DPO (20k)     & 47.0  & 601  \\

$\vtheta_{2 \rightarrow 3}$: DPO (20k)   & 46.8  & 564 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{59.5}  & 826 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{60.0} & 817 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{61.4} & 791 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 20k prompts per iteration.}
\label{tab:ab-20k-}
\end{table}
\vspace{-10pt}
% ----------

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (60k)    & 58.9  & 717 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (60k) & \text{59.6}  & 725 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{1}'}$: \hspace{-6pt} \quad + \texttt{\textbf{eva}} (60k) & \text{61.9}  & 792 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 60k prompts per iteration.}
\label{tab:ab-60k-}
\end{table}
\vspace{-10pt}
% ----------


\paragraph{\method~can bring robust gains with multiple iterations.} As shown in Table~\ref{tab:ab-10k-},~\ref{tab:ab-20k-}, and~\ref{tab:ab-60k-}, our method presents persistent performance gain over iterations, and concretely surpasses the performance by default DPO training with true human prompts. 


However, there exist diminishing marginal gains in iterative off-policy training. We ground~\method~in the iterative (off-policy) preference alignment paradigm due to its efficiency and ease of integration. However, such paradigms inherently face diminishing returns, where performance gains decrease with successive iterations, as previously observed in~\citep{self-play-gu,8fold,self-reward,cont-primary-bias}. While the generative data schedule in~\method~mitigates these challenges and extends beyond default training with human prompts (see also $\S$\ref{sec:ab-cont}), the gains can weaken over iterations. We summarize potential reasons as: (i) the \textbf{off-policy signal decay} -- as the number of examples increases, signals from the off-policy data become weaker due to distributional shift; (ii) the \textbf{loss of plasticity}, where the agent's ability to learn good policies decreases in continuing training with more iterations~\citep{cont-primary-bias}; (iii) the \textbf{ability of the solver} -- as we evolve more harder prompts, it is harder for the solver to produce preferred response (thus more explicit reasoning techniques may be needed); (iv) the \textbf{ability of the reward model} to correctly provide reward signals to responses and thus informativeness signals to prompts, as there may exists distributional mismatch.

Thus, we envision future work to build on~\method~by: (i) exploring its integration with \textbf{on-policy RLHF} (\eg instead of evolving prompts in iterations, one may evolve in batches); (ii) \textbf{enhancing solver capabilities}, such as sampling more responses during inference or leveraging meta-instructions to guide deeper reasoning; (iii) online training of RM to co-evolve with the creator and the solver. 

\paragraph{Bonus experiments on adding rewriter in the solver step.} This is beyond the current paper, and we present the basic idea here for practitioners to build upon~\method. The motivation comes from the hypotheses derived from $\S$~\ref{app:exp-iter}: as the prompts gets harder by evolving, there may be greater demands on the solver’s capabilities \emph{compared to earlier iterations}. As such, the solver may not be naively treated the same. One may address this by either inference-time scaling on responses or introducing meta-instructions to explicitly enhance the solver’s reasoning.

We hereby design a proof-of-concept experiment \emph{w.r.t} the latter by adding \textbf{rewriter} in \method's solver step. Previously, as in Algo.~\ref{alg:i-eva} and  $\S$~\ref{sec:solver-step}, for each prompt $\rvx$, we generate multiple responses, and choose the best as $\rvy_{+}$ and the worst as $\rvy_{-}$ for preference optimization. Now, we add one more rewriting step that attempts to enhance $\rvy_{+}$ to be $\rvy'_{+}$, by applying a rewriting instruction~\citep{deita} that asks the solver to alter $\rvy_{+}$ with imporved helpfulness, relevance, reasoning depths, creativity and details while keeping the similar length. We then train with $(\rvx, \rvy'_{+}, \rvy_{-})$ for preference optimization. Table~\ref{tab:rewriter-10k} shows that adding the rewriter yields concrete performance gains over the default  method, while keeping training budgets and only slightly increasing response generation cost.
% \vspace{-3pt}

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} with \texttt{\textbf{rewriter}} & \textbf{61.9}  & 741 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of adding \textbf{\texttt{\small rewriter}} in the \textbf{\texttt{\small solver}} step.}
\label{tab:rewriter-10k-}
\end{table}
\vspace{-10pt}
% ----------
% ---------------------

% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W2 (Connection in Minimax Regret and The Algorithm)}: The connection between the minimax regret objective and the algorithm is a somehow vague. The regret concerns the performance gap with the optimal policy. It's not reflected by the informativeness proxy.}
\end{tcolorbox}

\textbf{TL;DR:} We have added $\S$~\ref{app:theory} to address the reviewer's concern in detail. (i) In the current algorithm, the solver explicitly minimizes the regret by plug-in preference optimization algorithms (\eg DPO), while the creator implicitly maximizes the regret by first finding high-regret prompts and generate variations as new prompt distributions for training. (ii) The informativeness proxy is an advantage-based estimate of the regret; similar variants have been used in prior literature like~\cite{plr,accel}; as the policy optimizes, the proxy can approximate the true regret better. 

\textbf{Rebuttal:} For the rebuttal to be self-contained, we  extract contents from~\secref{app:theory-3} here. We feel~\secref{app:theory} offers a better overview -- it would be great if you could take some time to review~\secref{app:theory} when feasible.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}

The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret-}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.

\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optmizes, the proxy should approximate the regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


% At a high-level, we first use the alternating optimization by minimax game to replace the joint optimization in Eq.~\ref{eq:rlhf-joint-}; secondly, we use regret as the objective for the game, where the creator seeks to maximize and the solver seeks to minimize. For the creator, the regret is approximated by the informativeness proxy through sampling from the stochastic policy and measuring the gap between the maximal and the minimal reward received. For the solver, the minimization is practically achieved by the plug-in contrastive preference optimization (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model). Please check $\S$~\ref{app:theory} for our detailed writeup. (Note: without access to the optimal policy, we \emph{need} to approximate the regret in practice; classical works have trained two players~\citep{paired}, while our approach is more simple and efficient, avoids training instability and  empirically brings strong performance gain).
% ---------------------

% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 (Advantage v.s. Variance)}: The informativeness proxy seems to be similar to the variance of the rewards because they all concern the diversity of the generated responses. However, in lines 393-395, the results show using variance leads to poor performance. How to interpret this?}
\end{tcolorbox}

\textbf{Rebuttal:}  To explain, (i) variance does not directly capture the \textbf{learning potential} in preference optimization, while advantage-based informativeness proxy is better aligned to the learning objective; (iii) we \textbf{empirically show} that variance and advantage are only \textbf{weakly correlated} thus will likely result in different sampling. We have added $\S$~\ref{app:metric} to incorporate the reviewer's suggestion. 

% \textbf{Rebuttal:} 
\vspace{-12pt}
\begin{figure}[H]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-pdf.pdf}
        % \vspace{+0.00001pt}
        \caption{The probability density distributions of  informativeness metrics in Table~\ref{tab:ab-metric} -- they show different patterns.}
        \label{fig:metric-pdf-}
    \end{minipage}
    \hspace{0.02\textwidth}
    % \hfill
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-corr.pdf}
        % \vspace{+0.00001pt}
        \caption{The correlation plot for reward advantage (ours) and reward variance -- they are only \emph{weakly} correlated.}
        \label{fig:metric-corr-}
    \end{minipage}
    % \hspace{4\textwidth} % Space between the two main figures
\end{figure}
\vspace{-12pt}

In~\method, we assign each prompt an informativeness value, which the creator will use as the weight to sample from the seed prompts for prompt synthesis. In $\S$~\ref{sec:ab-metric}, we have shown that traditional methods like reward mean and reward variance are less effective as our advantage-based informativeness proxy. The intuition is simple: advantage/regret-based proxy aligns better with the preference optimization objective. We here further illustrate that they are statistically different from other choices:\vspace{-6pt}
\begin{itemize}
    \item Figure~\ref{fig:metric-pdf-}: The distribution of informativeness values shows that reward variance is heavily concentrated at lower values, reward mean is more uniformly scattered, and reward advantage achieves a better balance, providing a broader yet also focused sampling range.\vspace{-3pt}
    \item Figure~\ref{fig:metric-corr-}: The \emph{weak correlation} between reward variance and reward advantage shows that variance \emph{cannot} serve as a substitute for advantage as a proxy for informativeness.
\end{itemize}
\vspace{-6pt}
We have discussed the contrastive curriculum hypothesis in $\S$~\ref{sec:int} to support using reward advantage in the sense that the induced samples tend to decrease the loss the most in the contrastive optimization. Furthermore, assuming the optimization algorithm can converge to the \emph{more optimal} responses, neither reward mean nor variance directly capture the learning potential of such responses -- one may easily construct cases with identical variance yet differ much in reward range  -- thus variance fails to distinguish such scenarios. By contrast, reward advantage estimate inherently captures the relative improvement towards better response, and is sensitive to differences in reward range; variants of advantage estimate are commonly used in literature, and we discuss underlying principles in $\S$~\ref{app:theory}.
% ---------------------




% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q2 (Open-Ended Objective)}: In Line 1399 (authors' note: should be around Line 880 - 886 in the main OpenReview PDF), why is this objective ideal? Optimizing the prompt distribution seems like cheating by selecting easier prompts for a higher reward.}
\end{tcolorbox}

\textbf{TL;DR:} The whole design is to avoid cheating (\textbf{in principle}: adding KL regularization to guide the creator policy towards the open-ended reference; \textbf{in practice}: using the creator to generate new prompts to maximize the solver's regret). We also present further \textbf{empirical evidence} showing~\method~helps create more complex prompts.

\textbf{Answer:} To start with, we quote the conceptual objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

Another way to express the principled objective (with refined coefficients) is:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver $\sim$ ``regret minimization''}} }\ \textcolor{cgreen}{\Bigr]} 
-  \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\beta_2 \cdot \sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator $\sim$ ``regret maximization'' (implicit)}}}. \nonumber 
$}

\textbf{Conceptually}, the cheating will happen when the reference distribution is narrow or wrongly defined. It is important that in our case $p_{\text{ref}}(\rvx)$ represents an \emph{underspecified}, potentially intractable probability distribution over possible tasks (instantiated \emph{via} prompts) in the wild, as an  \textbf{open-ended reference} that covers the full diversity and complexity of tasks agents may encounter, \emph{not} the initial static prompt set $\calD$. The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts, while being close to the SFT policy $\pi_{\text{SFT}}(\rvy | \rvx)$. In brief, the definition of the conceptual $p_{\text{ref}}(\rvx)$ and the \textbf{regularization} avoids collapsing to distributions with easier prompts.

\textbf{Practically}, we do not directly optimize this principle, rather we design a creator-solver game to implicitly achieve this by iteratively creating a sequence of informative prompts. It is important that we use \emph{regret} as the objective and its approximation by the estimate of the \emph{optimal reward advantage}, which avoids selecting prompts that are too easy or too hard by design as well. See also $\S$~\ref{sec:int} on auto-curricula and learning potential for prompt selection, and $\S$~\ref{app:theory} for more connection between the objective and the algorithm.


For \textbf{empirical evidence}, as in Table~\ref{tab:prompt-quality-complexity---}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. We also observe the creator auto-prioritizes learning in problems like math and coding in Fig.~\ref{fig:dist---}, which are initially hard for it as in Fig.~\ref{fig:radar-gemma---}. Thus the creator also practically does not select easier prompts in the~\method~game. Details can be found in~\secref{app:curr}.


\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity---}
\end{table}
\vspace{-10pt}
% ----------

In addition, the whole literature of curriculum RL, open-ended learning and so on are about designing the right metric for the agents to learn increasingly complex and general capabilities, and we summarize at~\secref{app:lit} for the reviewer's reference.


\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist---}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma---}
    \end{minipage}
\end{figure}





% ---------------------


% ---------------------
\begin{tcolorbox}[myquote]
\textbf{Remarks.} We thank Reviewer \texttt{zxTK} for the constructive feedback. We have made careful efforts to address all the weaknesses and questions raised. We would be grateful if the reviewer may kindly consider again the rating for~\method, also with regard to its  strong performance gain, the easy-to-implement method, as well as the new principle and the tractable algorithm. If there are additional concerns, we are more than happy to discuss and revise our manuscript further.
\end{tcolorbox}
% ---------------------

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.




\newpage
\section*{Rebuttal to Reviewer i9kx}

\paragraph{Summary.} We thank the reviewer for the thoughtful and detailed feedback. In response, we have:
\begin{itemize}
    \item provided a point-by-point rebuttal \textbf{fully addressing every suggested weakness/question};
    \item \textbf{improved definitions} for Algorithm 1, the regret and the informativeness proxy in~\secref{sec:method};
    \item \textbf{added a detailed review} on bi-level RLHF and open-ended learning in $\S$~\ref{app:lit-bilevel} and $\S$~\ref{app:lit};
    \item \textbf{added a full section} to illustrate method, from the principle to the asymmetric game setting, then to the regret minimization by the solver and maximization by the creator in $\S$~\ref{app:theory};
    \item \textbf{added new experiments} on empirical gains and prompt evaluation of~\method~in $\S$~\ref{app:ablation} and $\S$~\ref{app:curr}.
\end{itemize}

% As a side note, we sincerely appreciate the reviewer’s thoughtful suggestions,  and note that their perspective may align with a more theory-first approach, akin to the references listed ([\href{https://openreview.net/pdf?id=Xb3IXEBYuw}{1}], [\href{https://openreview.net/forum?id=02kZwCo0C3}{2}], and [\href{https://openreview.net/forum?id=Jcn8pxwRa9}{3}]), which we very much value and find inspiring. The current~\method~framework, however, takes a complementary \textbf{method-first} approach, prioritizing methodological simplicity and empirical performance over rigid theoretical justifications. This design choice is intentional: we aim to offer a \textbf{new, simple, easy-to-implement training paradigm} that can be easily adopted, extended, and elaborated upon by the broader community, both in academia and industry.

% To achieve this, we have intentionally included approximations to make the framework \textbf{practical and easy to use}; we consider the main concerns of the reviewer may also come from such approximations made -- in a way that the current package is not intended to be perfect in theory. We wish to clarify that our primary goal is to prioritize the practical method itself, similar to prior methodological works (\eg CoT~\citep{cot}, ReST~\citep{rest}, etc). The theoretical bits we provide serve to establish a \textbf{high-level and fundamental principle} that inspires further practical and theoretical exploration, rather than being the restriction on the methodology.

% Additionally, we recognize the broader context in which this discussion takes place. It may be slightly sad to observe a gap between current RL/bandit theory research and the practical methods adopted in the real world. Many elegant theoretical ideas remain under-utilized due to the compromises required for theoretical rigidity, while industrial approaches often succeed with brute-force methods that prioritize empirical performance over theory. With \method, we aim to strike a balance between them, offering a conceptual framework that is both theoretically inspired and practically impactful.

% We hope we have sufficiently addressed the reviewer's concerns, and we warmly encourage the reviewer to also consider the \textbf{strong performance gains} with the \textbf{simple design} when judging~\method, and to evaluate the merit of a work (\textit{cf.,} \href{https://psc-g.github.io/posts/mentoring/reviewing/#conclusion}{ (Castro, 2021)}) \emph{w.r.t.} the practicality and how the community can easily build on top of it (\textit{cf.,} \href{https://d37ugbyn3rpeym.cloudfront.net/stripe-press/TAODSAE_zine_press.pdf}{(Hamming, 1986)}). We look forward to and would be very much grateful about any future suggestions to help us revise further, and we sincerely hope that the reviewer would consider update the rating for~\method, if the revision is satisfactory.

% We sincerely thank the reviewer once again for dedicating their valuable time to carefully reviewing our manuscript and for providing constructive feedback to improve~\method. We warmly welcome any future collaborative discussions and are more than happy to address any follow-up questions and to learn from the reviewer's insights.

To avoid repetition, we reorganize the questions and group related answers into a single response.

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q5 (Intuition on Open-Ended RLHF)}: Can you provide intuitions behind equation 7, on the KL divergence between the joint policy for both prompt and response? Is it even tractable to estimate or approximate this KL?}
\vspace{+4pt}
\newline
\textcolor{gray}{\textbf{W2 (Regret and KL)}: The optimization is over $\pi$ in Eq. 9 for solving the minimax regret. However, its not absolutely clear how the KL divergence plays a role here and how it is ensured that the response and prompt distributions are close to reference. Without that, the alignment problem is ill-defined. Please provide concrete justifications in theory and empirical results.}
\vspace{+4pt}
\newline
\textcolor{gray}{\textbf{W1 (Proxy Tractability)}: How is Eq. 10 tractable and being solved? Any heuristic of sampling and approximating should result in sub-optimality which is not clear where its accounted.}
\end{tcolorbox}

\textbf{TL;DR:} We have added $\S$~\ref{app:theory} to fully address related concerns. Regarding specific concerns:
\begin{itemize}
    \item \textbf{Q5 - Intuition.} The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to (i) generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts (note that $p_{\text{ref}}(\rvx)$ is the \emph{underspecified} open-ended reference, \emph{not} the initial static prompt set $\calD$), while (ii) being close to $\pi_{\text{SFT}}(\rvy | \rvx)$. We can reformulate the principle to Eq.~\ref{eq:rlhf-expand}.It is tractable to solve $\mathbb{D} _{\mathrm{KL}}\left[\pi _\theta(\mathbf{y} \mid \mathbf{x}) \| \pi _{\mathrm{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$ by existing plug-in preference optimization algorithms, yet we need to approximate $\mathbb{D} _{\mathrm{KL}}\left[\pi _\phi(\mathbf{x}) \| p _{\mathrm{ref}}(\mathbf{x})\right]$ -- one way to achieve this heuristically is by iteratively creating a \emph{sequence} of prompt distributions directing its learning towards new, informative prompts to continue training. This is the key unconventional approach that~\method~takes (please check $\S$~\ref{app:theory} for more background). 
    \item \textbf{Q2 - KL.} We have revised Eq.~\ref{eq:regret-pi} so that the regret is the difference in the reward of the current policy and the KL-optimal policy (thanks for catching this). For the solver, by design, preference optimization would be equivalent to regret minimization, thus the alignment problem remains to be correctly defined. For the creator, the distribution matching to the open-ended reference is implicitly achieved by prompt curriculum construction, and we present empirical evidence in $\S$~\ref{app:curr} to justify that prompts are evolving towards broader tasks with higher complexity.
    \item \textbf{W1 - Proxy.} We have revised Definition~\ref{def:info-proxy} for better readability. It is estimated by sampling multiple responses from the stochastic policy and calculating the reward range (or other advantage-based proxy). This approximation will result in sub-optimality for creator's regret maximization process, and we present more discussion in $\S$~\ref{app:theory-2}.
\end{itemize} 

% (i) we have revised the manuscript \emph{w.r.t.} KL-regularized regret and discussed our approximation made in $\S$~\ref{app:theory}; (ii) we sample multiple times from the stochastic policy to tractably estimate the informativeness proxy, which we explained in detail at $\S$~\ref{app:theory-3}; (iii) the \textbf{solver maintains the KL regularization} with regard to the reference policy during training, thus the alignment problem at each iteration remains correctly defined; (iv) the creator does not have a tractable reference distribution, and we use a fixed creator and apply meta instructions and buffer sampling to adapt/constrain the prompt generations (as described in $\S$~\ref{sec:algo}, $\S$~\ref{app:reproduce} and $\S$~\ref{app:exp-evol}), which is easy-to-implement and empirically effective.

\textbf{Rebuttal:}  For the rebuttal to be self-contained, we  extract contents from~\secref{app:theory} here.

First, we re-present the open-ended RLHF principle, and discuss the intuition under the KL regularization. Next, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. Finally, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection*{\textbf{.1} \ The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1-}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}

The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.

\subsection*{\textbf{.2} \ Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2-}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection*{\textbf{.2.1} \ The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection*{\textbf{.2.2} \ Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 
% \begin{itemize}
%     \item \textbf{Regret approximation}: the same as~\citep{plr} -- the positive value loss.
%     \item \textbf{Environment generation}: 
% \end{itemize}

Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.





 


% \cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones.


% (TODO: give an overview on this setting; our creator follows the similar setting by identifying the high-regret levels and then making edits with them combining a buffer.)
% Later on, researchers explore more \emph{curriclum}-driven approach, especially through adversarial training~\citep{adr} with minimax objective

% . The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

% \textcolor{red}{This section is about heuristics on distributional matching with a game setting. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }

% \subsubsection{Reformulating Constrained Optimization to Minimax Optimization}

% \newpage
\subsection*{\textbf{.3} \ Regret Formulation for Open-Ended RLHF}\label{app:theory-3-}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.





\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right). \nonumber
\end{align}
% where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

% Thus the regret with regard to the KL-constrained optimal policy is:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \nonumber
% \end{align}


% Assuming $\rvy_+, \rvy_-$ are correctly labeled by an \textit{oracle reward model} $r(\cdot, \cdot)$, the direct preference optimization objective is:
% \begin{align}
%     \mathcal{L}_{\text{DPO}}=-\mathbb{E}_{\rvx \sim \calD, (\rvy_+, \rvy_-) \sim \pi_{\vtheta}(\cdot \mid \rvx)}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_+ \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_+ \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_- \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_- \mid \rvx\right)}\right)\right]. \nonumber
% \end{align}


We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret--}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.



\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


% We thank the reviewer for catching the omission of the KL term in the original writeup on regret. Please see our revised definition and detailed discussion on the approximation that we made in $\S$~\ref{app:theory}, and empirical results in $\S$~\ref{sec:main_results} on  alignment gains over different algorithms and benchmarks, $\S$~\ref{app:curr} on generated prompt distributions and alignment gains across different categories. 





% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{W2 (Regret and KL)}: The optimization is over $\pi$ in Eq. 9 for solving the minimax regret. However, its not absolutely clear how the KL divergence plays a role here and how it is ensured that the response and prompt distributions are close to reference. Without that, the alignment problem is ill-defined. Please provide concrete justifications in theory and empirical results.}
% \end{tcolorbox}

% \textbf{TL;DR:}

% \textbf{Rebuttal}


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W3 (Understanding the Iterative Algorithm)}: As described in Algorithm 1, informativeness is evaluated and a prompt subset is created based on current policy estimate and then the policy is updated based on the prompt subset. However, this causes an inter-dependence between the two which leads to nested structure, which is not clearly explained. Specifically, while computing the informativeness score for the prompts, it depends on $\theta^\star(x_{t-1})$ , \ie optimal parameter for the previous distribution. Provide clear explaination on the same.}
\end{tcolorbox}

\textbf{TL;DR:} (i) We revised Algo.~\ref{alg:i-eva} with updated subscripts to reflect the training process -- please take a look in our main paper. Given a current model checkpoint, we evaluate the prompt informativeness based on it, and evolve a new prompt set more informative to the current checkpoint, and use the new prompt set for continual training. (ii) We intend to use an iterative best-response framework to approximate equilibrium in expectation, balancing computational efficiency and practicality. 

\textbf{Rebuttal:} The iterative updates in~\method, as described in Algo.~\ref{alg:i-eva}, are based on a best-response-to-best-response framework. Specifically, the creator updates the prompt distribution based on the solver’s current policy, and the solver then optimizes its policy over the updated prompts, and the process repeats. This sequential structure approximates a Nash equilibrium in expectation over iterations, inspired by works such as~\cite{freund,self-play-gu}, which establish convergence to optimal policies on average through iterative optimization.

We intentionally avoid simultaneous joint optimization as it would significantly increase computational and memory overhead, making it less practical for integration into current RLHF pipelines. 

% The current approach is simple and effective, and leads to concrete empirical performance gain as shown in $\S$~\ref{app:curr}. While this paper emphasizes \textbf{practical usability} over formal theoretical guarantees, we look forward to future works on extensions for Open-Ended RLHF (such as adding convergence rates and equilibrium guarantees, deriving first-order solutions, etc). We would greatly appreciate any further suggestions or insights the reviewer may have to improve this direction.

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W4 (Understanding Reward Models)}: While iterating, every new prompt distribution will require generating new response, how is the evaluation coming from which reward model? Is the ground reward available, if not please explain how the preference is obtained and how does it affect suboptimality? Also: } \textcolor{gray}{\textbf{Q3 (RM Availability)}: What's the reward model availability? Is the true reward model available?}
\end{tcolorbox}

\textbf{TL;DR:} We assume a preference oracle provided by an \textbf{external, pre-trained reward model}, which is practically  used in many real-world LLM training scenarios~\citep{team-1}.

\textbf{Rebuttal:} As discussed in the beginning of the experimental setting in $\S$~\ref{sec:exp}, we assume the availability of a pre-trained, fixed reward model. This approach is practically adopted in industry~\citep{team-1,team2,gemma2} and is also commonly used in academia works~\citep{dpo-iterative,simpo,self-play-gu}. The reason is more on efficiency concerns. For example, in \textsc{Gemma-2} training, the reward model is \emph{an order of magnitude larger} than the policy~\citep{gemma2}; it would thus be impractical or the gain may only be marginal if we update the reward model on-the-fly. 

% (as done in many prior works on bi-level RLHF -- thanks again for the reviewer's nice references). 

Nevertheless, it is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} (ablation studies) that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and address the potential distribution mismatch problem. We believe this is an interesting direction to pursue, and have listed it in $\S$~\ref{sec:conclusion} (future works) on adding more players including rewarders in the self-play loop.


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W5 (Improvement of Sub-Optimality)}: Overall, which expression/Theorem guides us in understanding the improvement of prior suboptimality is not clear? Can you please point out/highlight how the current method improves upon the prior suboptimality due to static prompt distribution? }
\end{tcolorbox}

\textbf{TL;DR:} The improvement of sub-optimality is guided by the minimax regret objective (Remark 1) through its iterative implementation. While this work does not explicitly derive suboptimality bounds, our approach has demonstrated \textbf{strong empirical gains} over the training by static distributions, as shown in $\S$~\ref{sec:exp} (main experiments), $\S$~\ref{app:curr} (benchmark performance), and $\S$~\ref{app:exp-iter} (alignment gains over iterations).

\textbf{Rebuttal:} In general, the improvement of prior suboptimality due to static prompt distributions is guided by the minimax game outlined in Remark 1. This expression forms the basic foundation for our iterative algorithm, where the creator updates prompts to maximize informativeness (proxy for regret), and the solver minimizes regret (through direct preference optimization). This iterative process ensures the solver and creator adapt to each other, implicitly forming a curriculum and addressing sub-optimality  in static prompts. We also added $\S$~\ref{app:theory} to help illustrate the intuition behind.

The empirical results in $\S$~\ref{sec:exp} (main results), $\S$~\ref{app:curr} (curriculum effect and benchmark improvement), and $\S$~\ref{app:exp-iter} (alignment gains over iterations) demonstrate that the dynamic prompt distribution improves solver performance and alignment metrics, thereby mitigating suboptimality. While the current package does not explicitly derive sub-optimality bounds (as would be typical in formal RL/bandit theory papers) and emphasizes practicality and usability as a methodology paper, we would love to learn if the reviewer has any suggestions for this as the future work.

% We thank the reviewer’s suggestions on formalizing sub-optimality analysis further and would love to consider this an exciting direction for future work.


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W6 (Prompt Distribution)}: It is extremely crucial to show the prompt distribution and demonstrate its perplexity to ensure its not generating some meaningless or irrelevant prompts, since its not very evident on the KL divergence in the prompt space and its relation with the informative measure. Please provide detailed explanation to clarify that. }
\end{tcolorbox}

\textbf{TL;DR:} We have (i) added experimental results in $\S$~\ref{app:curr} (prompt distribution visualization) and $\S$~\ref{app:examples} (prompt examples) to verify that~\method~evolves meaningful and relevant prompts with improved complexity and quality; (ii) added explanation in $\S$~\ref{app:theory} (detailed illustration of method) on the conceptual KL regularization in the prompt space and the implicit approximation by the creator.

\textbf{Rebuttal:} (This rebuttal also addresses Reviewer \texttt{\small ac2p}'s concerns on curriculum.)

We have revised the manuscript with additional visualization on potential curriculum learned in $\S$~\ref{app:curr}. In general, we observe the creator prioritizes learning in math and coding for the generated prompt distribution, which brings gradual improvement on benchmark performance on relevant categories over iterations. In other words, \method~effectively shifts focus towards harder yet learnable categories. We have attached the bar plot and radar figure here for the reviewer's reference:

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist--}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma--}
    \end{minipage}
\end{figure}

We have added Table~\ref{tab:prompt-evol-2} providing qualitative examples for evolved prompts. Also, as noted in $\S$~\ref{app:theory}, the solver maintains KL regularization during optimization, ensuring that the response distribution remain close to the reference policy; in the this work, we do not explicitly add KL regularization in the prompt distribution since we do not directly conduct parameter update for the creator (which we empirically find to bring training instability); rather, we use \textbf{meta instructions} and \textbf{buffer sampling} to constrain the prompt generations (as described in $\S$~\ref{sec:algo}, $\S$~\ref{app:reproduce} and $\S$~\ref{app:exp-evol}), which is empirically very effective, and introduces only minimal changes to existing pipeline thus can be easily applied. As noted in $\S$~\ref{sec:conclusion}, we look forward to future works on making the creator policy differentiable.

Regarding the relation with the informativeness measure, our current proxy is an efficient proxy among many possibilities to approximate regret (where one way to implicitly achieve $\mathbb{D} _{\mathrm{KL}}\left[\pi _\phi(\mathbf{x}) \| p _{\mathrm{ref}}(\mathbf{x})\right]$ is by training on the prompt curriculum created by the creator with regret maximization as its strategy). We have provided detailed discussions in $\S$~\ref{app:theory} to help interpret it. 
% There could be other proxies -- one interesting direction is to completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection.

We note that perplexity is not commonly used nor the most preferred  measure for data quality in practical training of large language models~\citep{team-1,wrong}, and can be computationally heavy to measure. We have added experiments in~\secref{app:curr-2} which we follow~\cite{deita} to generatively measure the complexity and quality of prompt distributions.  As in Table~\ref{tab:prompt-quality-complexity--}, there is a gradual improvement of prompt complexity and quality over iterations with~\method.  We believe this would address the reviewer's concerns.

% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity--}
\end{table}
\vspace{-10pt}
% ----------

% ------------------
% \begin{table}[H]
% \centering
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}r p{12.6cm}@{}}
% \toprule
% \rowcolor{lightgray!16}
% \multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small Write me the code for a distributed transaction manager.\textbackslash nThink step by step and use pseudo code first.\textbackslash nThen, define interfaces for all involved actors and entities.\textbackslash nUse Rational Unified approach for this part.\textbackslash n\textbackslash nOnly then move on to the actual implementation, class-by-class, and method-by-method.\textbackslash nMake the code be implemented in C\# and follow SOLID principles.} \\ \midrule
% \texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Craft a suite of syntax for a distributed transaction coordinator. Start with a sequential breakdown in pseudocode format. Following that, establish the protocols for communication and interaction amongst the various participants and components, incorporating the Rational Unified Process methodology.\textbackslash n\textbackslash nProceed thereafter to the concrete creation, detailing each class and function. Ensure that the final C\# code adheres to the precepts of SOLID and is annotated for clarification and maintainability purposes.} \\
% \texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Devise a comprehensive set of directives and structures for a distributed transaction coordinator architecture. Initiate by formulating a step-by-step algorithmic decomposition in pseudocode. Subsequently, delineate the frameworks for dialog and cooperation between the numerous entities and elements, utilizing the tenets of the Rational Unified Process methodology.\textbackslash n\textbackslash nContinue to the actual generation of the code, meticulously detailing every class and corresponding method. Guarantee that the culminating C\# code is in strict compliance with SOLID principles and is supplemented with descriptive commentary to enhance future clarity and upkeep, while also validating the code against a set of unit tests to ensure robust functionality.} \\
% \texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Commence by constructing an algorithm in pseudocode that meticulously breaks down the sequential stages for a distributed transaction coordinator system. Progress by outlining the communication protocols and collaborative mechanisms among the myriad components, adhering to the Rational Unified Process approach.\textbackslash n\textbackslash nAdvance to crafting the code in C\#, ensuring each class and method is elaborated with precision, aligning with SOLID design principles. Integrate thorough comments for heightened maintainability and conduct comprehensive unit testing for assured operational integrity.} \\
% \texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Design a detailed flowchart that represents the intricate steps of an orchestration engine for managing microservices in a cloud-native environment. Begin by detailing the service discovery, load balancing, and fault tolerance strategies, while incorporating the DevOps philosophy.\textbackslash n\textbackslash nProceed by developing the implementation in Java, focusing on clean, modular code following object-oriented programming best practices. Accompany your code with clear documentation for easy understanding and perform rigorous integration testing to guarantee robustness.} \\ \bottomrule
% \end{tabular}%
% }
% % \vspace{-4pt}
% \caption{Examples of evolved prompts from AlpacaEval. We suggest practitioners to include generated responses with oracle rewards and self-critique in the context for better prompt evolving, which is helpful for mitigating the effect of potential self-consuming loops in synthetic data training.}
% \label{tab:prompt-evol-2-}
% \end{table}


% ----------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 and Q2 (KL in the Solver Loop)}:  Since equation 7, can't be directly solved, and is solved in an asymmetric fashion, then in the solver loop the KL should be over the response distribution and not joint right? How is the KL divergence w.r.t reference policy for the algorithm? Please provide detailed ablation.}
\end{tcolorbox}

\textbf{Answer:} (i) Yes, in the solver loop, the KL regularization is applied over the response distribution, not the joint distribution, as shown in Algo.~\ref{alg:i-eva}. (ii) The KL divergence \emph{w.r.t.} reference policy is determined by the plug-in solver (\eg DPO), which is orthogonal to our framework. We have added detailed explanation in $\S$~\ref{app:theory} to illustrate the whole process.

% ----------------


% ----------------
% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{Q3 (RM Availability)}: What's the reward model availability? Is the true reward model available?}
% \end{tcolorbox}

% \textbf{Answer:} Yes, we assume the availability of a pre-trained, off-the-shelf reward model. This approach is practically adopted in industry~\citep{team-1,team2,gemma2} and is also commonly used in academia works~\citep{dpo-iterative,simpo,self-play-gu}. See also our detailed rebuttal for \textbf{W4}.
% ----------------

% ----------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q4 (Literature)}: There is a recent line of works on Stacklberg and Bilevel RLHF which deals with the entanglement in a leader-follower setting. Although not specific to updating prompt dist, but can be trivially applied. Provide a detailed comparison with the literature around that [1,2,3].}
\end{tcolorbox}

\textbf{TL;DR:} We thank the reviewer for this nice suggestion. Please see below for a detailed review on the relevant literature, highlighting the unique contribution of~\method. We have added $\S$~\ref{app:lit-bilevel} in the manuscript.

\textbf{Rebuttal:}
Bi-level optimization refers to optimization problems where the cost function is defined \textit{w.r.t.} the optimal solution to another optimization problem~\citep{roger-class}. There is a recent line of works applying bi-level optimization to RLHF. While they all rely on a fixed dataset of prompts, \method~propose to dynamically update the prompt set. We hereby present a detailed comparison of~\method~with~\cite{bilevel-sail,bilevel-shen,bilevel-sta-rlhf}. We thank the anonymous reviewer for the kind  references, and welcome suggestions for any other works we may have missed.
% While those works are orthogonal to~\method, We  thank the anonymous reviewer for the kind  references, which may help address the potential distributional mismatch issues as the policy models become more powerful.

\cite{bilevel-sail} formulate iterative online RLHF as a bi-level optimization problem, where the upper-level represents the reward learning, and the lower-level represents the policy optimization. Leveraging reward re-parameterization tricks in~\cite{dpo}, \cite{bilevel-sail} reduces the problem to a single-level objective with regard to the policy. The differences of this work and our work lie in the prompt distribution and preference oracle: (i) \method~features by \textbf{dynamic prompt set generation for Open-Ended RLHF}, whereas~\citep{bilevel-sail} remains using a static prompt set; (ii) we assume the existence of the preference oracle (as discussed in $\S$~\ref{sec:exp}), while~\cite{bilevel-sail} consider online training of reward models and ablate on self-rewarding by the current LLM policy. Our usage of a pre-trained reward model follows from industrial practices~\citep{team-1,gemma2}, which is also commonly used by prior works in academia~\citep{simpo,self-play-gu}. 
% We recognize the online training of reward models (see also~\citep{rlhf-workflow}) as an orthogonal/complementary direction to the current settings of~\method~(our setting is \textbf{agnostic to the preference structure}), and encourage future works and collaborations towards it, as mentioned in $\S$~\ref{sec:conclusion}.

\cite{bilevel-sta-rlhf} provide an interesting exploration on formulating RLHF as a leader-follower game, where the language model (LM) policy is the leader and the reward model (RM) policy is the follower, and the solution is \textbf{Stackelberg equilibrium}~\citep{stackelberg,game-mbrl}, where the \emph{leader does not likewise best respond to the follower's strategy}. Here, following the curriculum RL literature~\citep{paired,accel}, we seek the \textbf{Nash equilibrium}~\citep{nash} between the creator for prompt generation and the solver for response generation. Nevertheless, the LM-RM iterative optimization may be added on top of~\method's~framework, and we look forward to future works exploring the leader-follower re-formulation of~\method.

\cite{bilevel-shen} present a rigorous theoretical work (though it does not directly involve practical post-training of large language models). The authors propose to reduce the bi-level problem to a single-level problem with a penalty-based reformulation, and apply it in the setting of LM-RM optimization within a \textit{fixed} environment, whereas~\method~focuces on dynamic prompt generation and practically train large language models with extensive empirical experiments conducted. We believe it would be interesting to adapt similar first-order optimization techniques to solve Open-Ended RLHF.

In summary, existing bi-level RLHF works focus on online optimization of both the RM and the LM (as the response policy), all with \textbf{fixed} prompt/state distribution. \method~presents an orthogonal direction on \textbf{dynamic} prompt generation for Open-Ended RLHF, with an empirical algorithm which attains state-of-the-art performance with large language models on a variety of benchmarks. It is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and mitigate potential distributional mismatch problems as we evolves for more prompts. This direction may have not been widely adopted in real-world training of language models, due to concerns about practicality~\citep{team-1,team2,gemma2,nemotron}. We look forward to future works exploring \emph{efficient} variations unifying \method\ and existing bi-level RM-LM frameworks.
% ----------------


% ----------------
% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{Q5 (Intuition on Open-Ended RLHF)}: Can you provide intuitions behind equation 7, on the KL divergence between the joint policy for both prompt and response? Is it even tractable to estimate or approximate this KL?}
% \end{tcolorbox}

% \textbf{Answer:} To avoid repetition, please see our detailed rebuttal for \textbf{W1}. We have also added $\S$~\ref{app:theory} to ensure this concern is sufficiently addressed.
% ----------------

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textbf{Final Remarks.} We thank the reviewer for the precious time and efforts on the~\method~method. We value all those opinions, and have made every effort to thoroughly address the concerns raised and revise our manuscript accordingly. Regarding the rejection, we hope the reviewer may kindly consider the points that we have summarized at the beginning of this rebuttal, on the \textbf{strong empirical alignment gain} brought by the \textbf{simple design} of~\method, also on judging the merit of a work (\textit{cf.,} \href{https://psc-g.github.io/posts/mentoring/reviewing/#conclusion}{ (Castro, 2021)}) \emph{w.r.t.} the practicality and how the community may easily build on top of the principle and the method we proposed (\textit{cf.,} \href{https://d37ugbyn3rpeym.cloudfront.net/stripe-press/TAODSAE_zine_press.pdf}{(Hamming, 1986)}), which we are confident are valuable to the broader alignment community. We look forward to any future discussion, and would be grateful if the reviewer may consider revising the score if the revision is satisfactory.
\end{tcolorbox}

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.







==> app-icml/app-theory-clean.tex <==
In~\secref{app:theory-1}, we present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}



The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.



\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 


Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.


\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.

\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber

\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.




We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.




\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


==> app-icml/app-theory-old.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

\subsection{Connections in Open-Ended RLHF, Minimax Game and the Proxy}\label{app:intuition}

We provide an extended discussion on $\S$~\ref{sec:method} to make the explanation more coherent and easy-to-understand. Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{cred}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tg{\pi_{\phi}(\rvx)} \cdot \tc{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}), which is a special case if $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expand Eq.~\ref{eq:rlhf-joint-}:

\resizebox{\textwidth}{!}{$
\max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cred}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\textit{KL}}\bigr[\textcolor{cred}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
- \beta \cdot \textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}. \nonumber 
$}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


To clarify, while $\pi_{\text{SFT}}(\cdot)$ refers to the supervised trained model~\citep{rlhf}, the newly proposed $p_{\text{ref}}$ represents an \textbf{open-ended} and potentially intractable probability measure over all possible tasks (instatiated \emph{via} prompts) or user prompts -- note it is not the static training prompt distribution. Here, the regularization $\textcolor{black}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by generating new tasks for self-training and self-improvement, instead of optimizing over a static, pre-defined prompt set. The non-trivial part is on solving this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

In the next, we will provide a step-by-step derivation leading to our Algo.~\ref{alg:i-eva}. To begin with, we first discuss how prior works tractably solve similar open-ended learning problems via two-player game formulation. Next, we formally present the new objective, and discuss how to tractably solve it in our specific setting.

\subsection{Designing Two-Player Games for Open-Ended Environment Design}
The underlying idea is straightforward, while we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$, we are able to create a series of environments. The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

\textcolor{red}{TODO: unifying the theorems/notations in previous literature. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }
\begin{itemize}
    \item \cite{poet}:
    \item \cite{paired}:
    \item \cite{plr}: scoring by generalized advantage estimation
    \item \cite{dcd}:
    \item \cite{accel}:
\end{itemize}

\subsection{Regret Formulation for Open-Ended RLHF}

\subsubsection{Advantage-Based Regret and Approximation by EvolInstruct: The Creator Step}

\subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

\newpage



\textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



 Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
\begin{itemize}
    \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \end{itemize}
    \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \end{itemize}
\end{itemize}

% \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

The regret objective is defined as
\begin{align}
\operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
\end{align}
% $$
% \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% $$

At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
\begin{align}
    \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
\end{align}
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

This approximation introduces two practical advantages:
\begin{enumerate}
    \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
    \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
\end{enumerate}

This deviates from the theoretical Open-Ended RLHF objective. In particular:
\begin{itemize}
    \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
    \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
\end{itemize}

Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


\subsection{KL-Regularized Regret}\label{app:kl}
For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

% This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% \begin{itemize}
%     \item 
%     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% \end{itemize}

\subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
\textcolor{red}{TODO: add derivation to better justify this approximation.}
In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
\begin{align}
    \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
\end{align}

This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
\begin{itemize}
    \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
    \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
    \begin{itemize}
        \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
        \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
    \end{itemize}
    \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
\end{itemize}


We justify this simplification as follows:
\begin{itemize}
    \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
    \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
    \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
\end{itemize}

We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> app-icml/tab-gen-1.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\tiny Implement a function to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\tiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \ nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \ The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  \ if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  \ imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  \ imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\  \ if i == 0:\textbackslash n\  \ max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  \ return max\_left\textbackslash n\textbackslash n\  \ if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  \ elif j == n:\textbackslash n\  \ min\_right = nums1[i]\textbackslash n\  \ else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1` into two parts: `nums1[0:i]` and `nums1[i:m]`.\textbackslash n\  \ - `j` is calculated to divide `nums2` so that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Partition:**\textbackslash n\  \ - We compare elements at the boundaries of the partitions to see if `i` is in the correct position:\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, `i` is too small, so we move `imin` to `i + 1`.\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move `imax` to `i - 1`.\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - Once `i` is in the correct position, we find:\textbackslash n\  \ - `max\_left`: The maximum element in the left partitions of both arrays.\textbackslash n\  \ - `min\_right`: The minimum element in the right partitions of both arrays.\textbackslash n\  \ - If the total length is odd, `max\_left` is the median.\textbackslash n\  \ - If the total length is even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we perform binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we only use a constant amount of extra space for variables.
}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\tiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\ if i == 0:\textbackslash n\  max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  return max\_left\textbackslash n\textbackslash n\  if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  elif j == n:\textbackslash n\  min\_right = nums1[i]\textbackslash n\  else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1`, and `j` divides `nums2` such that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Search Range:**\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, it means `i` is too small, so we need to move the partition point in `nums1` to the right (`imin = i + 1`).\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move it to the left (`imax = i - 1`).\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - When the correct partition is found (`i` is in the right position), we find:\textbackslash n\  \ - `max\_left`: The maximum element on the left side of the partition.\textbackslash n\  \ - `min\_right`: The minimum element on the right side of the partition.\textbackslash n\  \ - If the total number of elements is odd, `max\_left` is the median.\textbackslash n\  \ - If even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we are performing binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we are only using a constant amount of extra space for variables.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\tiny 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\tiny \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\tiny You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\tiny }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny Judgment} \stt{\tiny (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides an example usage of the function, which is helpful for understanding how to use it. The assistant's code is a different implementation than the reference answer, but it achieves the same result and meets the same complexity requirements. \newline However, the assistant's answer does not address the user's original question about achieving O(n) time complexity. The assistant should have clarified that it's not possible to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity, as stated in the reference answer. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722737514.2011044}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides a step-by-step explanation of the code, which is very helpful for understanding the logic behind the solution. The assistant's code is also correct and will correctly find the median of two sorted arrays of different sizes. Therefore, there are no corrections needed for the assistant's response.\newline\newline Rating: [[10]], "score": 10, "turn": 1, "tstamp": 1722846533.772981}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-1}
\end{table}

==> app-icml/tab-gen-2.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Imagine you are writing a blog post comparing two popular smartphone models. Develop an outline for the blog post, including key points and subheadings to effectively compare and contrast the features, performance, and user experience of the two models. Please answer in fewer than 200 words.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize \#\# Smartphone Showdown: [Model A] vs. [Model B]\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce the two smartphone models being compared, highlighting their popularity and target audience.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, and display technology (e.g., OLED, LCD).\textbackslash n* Design aesthetics and user preferences.\textbackslash n\textbackslash n**III. Performance and Specs**\textbackslash n* Processor, RAM, and storage comparison.\textbackslash n* Benchmark scores and real-world performance analysis.\textbackslash n* Battery life and charging capabilities.\textbackslash n\textbackslash n**IV. Camera Capabilities**\textbackslash n* Rear and front camera specs (megapixels, aperture, features).\textbackslash n* Image quality comparison in various lighting conditions.\textbackslash n* Video recording capabilities.\textbackslash n\textbackslash n**V. Software and User Experience**\textbackslash n* Operating system and user interface comparison.\textbackslash n* App ecosystem and availability.\textbackslash n* Software features and customization options.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare the price points of both models.\textbackslash n* Analyze the value proposition based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and similarities.\textbackslash n* Recommend the best phone for specific user profiles (e.g., budget-conscious, photography enthusiasts, gamers).}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize \#\# iPhone 14 Pro vs. Samsung Galaxy S23: Which Flagship Reigns Supreme?\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce both smartphones and their position in the market.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, refresh rate, and display technology (OLED vs. Super AMOLED).\textbackslash n* Design aesthetics and unique features (e.g., notch vs. punch-hole, color options).\textbackslash n\textbackslash n**III. Performance and Camera**\textbackslash n* Processor comparison (Apple A16 Bionic vs. Snapdragon 8 Gen 2).\textbackslash n* RAM and storage options.\textbackslash n* Camera specs: megapixels, lens types, aperture, and special features (e.g., telephoto, macro).\textbackslash n* Image quality comparison based on sample photos and user reviews.\textbackslash n\textbackslash n**IV. Software and User Experience**\textbackslash n* Operating systems: iOS 16 vs. Android 13.\textbackslash n* User interface comparison: intuitiveness, customization options, and app ecosystems.\textbackslash n* Special features: Face ID vs. in-display fingerprint sensor, voice assistants.\textbackslash n\textbackslash n**V. Battery Life and Charging**\textbackslash n* Battery capacity and real-world usage comparison.\textbackslash n* Fast charging speeds and wireless charging capabilities.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare starting prices and different storage configurations.\textbackslash n* Assess the overall value for money based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and strengths of each phone.\textbackslash n* Recommend the best phone for specific user types (e.g., photography enthusiasts, gamers, budget-conscious consumers).}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize Take your previous response and rephrase it as a limerick.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize Two phones, a showdown so grand,\textbackslash n[Model A] and [Model B], hand in hand.\textbackslash nDesign, specs, and price,\textbackslash nWe'll analyze nice,\textbackslash nTo help you choose, understand?\textbackslash n\textbackslash nLet me know if you'd like me to try filling in the bracketed parts with specific model names!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize \textbackslash nTwo phones, a Pro and a Galaxy,\textbackslash nFor flagships, they truly are spacy.\textbackslash nWith cameras and screens,\textbackslash nAnd processors keen,\textbackslash nWhich one wins? Read on, and be savvy! \textbackslash nLet me know if you'd like another limerick!}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The user asked the assistant to rephrase the previous response, which was a detailed outline for a blog post, into a limerick. The assistant successfully did so, maintaining the essence of the original response in a limerick format. The assistant also offered to further customize the limerick by filling in the bracketed parts with specific model names, showing a willingness to provide additional detail if needed. However, the limerick does not fully capture the depth and detail of the original response, which is understandable given the constraints of the limerick format. \newline\newline Rating: [[8]], "score": 8, "turn": 2, "tstamp": 1722737024.0327556}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The assistant successfully rephrased the previous response, which was a detailed outline for a blog post comparing two smartphone models, into a limerick. The limerick is playful and engaging, and it maintains the essence of the original response, which is to compare the two phones and help the reader make an informed decision. The assistant also offers to create another limerick if the user wants, showing a willingness to continue the interaction. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846542.9437995}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-2}
\end{table}

==> app-icml/tab-gen-3.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Each problem consists of three statements. Based on the first two statements, the third statement may be true, false, or uncertain.\textbackslash n1. Oranges cost more than apples.\textbackslash n2. Oranges cost less than bananas.\textbackslash n3. Bananas cost more than apples and bananas cost more than orange.\textbackslash nIf the first two statements are true, then the third statement is?}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nStatement 3 is **partially true**.\textbackslash n\textbackslash n* The part "Bananas > Apples" is true based on our price order.\textbackslash n* The part "Bananas > Oranges" is also true based on our price order.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThese statements tell us that bananas are the most expensive, then oranges, and apples are the least expensive.\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nSince bananas are indeed more expensive than both apples and oranges, statement 3 is **true**.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize If the third statement is true. Is the first statement true, false, or uncertain? Please explain.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, the first statement is **false**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** States that bananas cost more than both apples AND oranges.\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples.\textbackslash n\textbackslash n* **Statement 1:** States that oranges cost more than apples.\textbackslash n\textbackslash nIf bananas are the most expensive, and oranges are second, then oranges cannot be more expensive than apples.\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other logic puzzles!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, then the first statement is **uncertain**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nThis tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges.\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples\textbackslash n\textbackslash nThis statement claims oranges are more expensive than apples.\textbackslash n\textbackslash nStatement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is incorrect. The assistant states that if the third statement is true, the first statement is false. However, the third statement only establishes that bananas cost more than both apples and oranges. It does not provide information about the relative costs of apples and oranges. Therefore, the first statement could be true (if oranges cost more than apples), false (if oranges cost less than apples), or uncertain (if oranges and apples cost the same). The assistant's explanation is flawed because it incorrectly assumes that the order of costs must be Bananas > Oranges > Apples, when in fact the order could also be Bananas > Apples = Oranges or Bananas > Apples > Oranges. \textbackslash n\textbackslash nCorrected Assistant's Answer: If the third statement is true, then bananas cost more than apples and bananas cost more than oranges. This means that oranges could still cost more than apples, making the first statement true. However, it's also possible that oranges and apples have the same cost, which would make the first statement false. Therefore, based on the third statement alone, the first statement is uncertain.\newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737017.2808955}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is correct and helpful. The assistant explains that the first statement is uncertain if the third statement is true, which aligns with the reference answer. The assistant provides a clear explanation of why this is the case, stating that the third statement doesn't contradict the first statement, but it also doesn't confirm it. Therefore, the assistant's response is accurate and informative.\textbackslash n\textbackslash nThe assistant's response: "If the third statement is true, then the first statement is **uncertain**. Here's why: Statement 3: Bananas > Apples AND Bananas > Oranges. This tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges. Statement 1: Oranges > Apples. This statement claims oranges are more expensive than apples. Statement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846527.2339694}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app-icml/tab-gen-4.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize You are given two sorted lists of size m and n. Implement a function to find the kth smallest element in the union of the two lists with linear complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\  \ """\textbackslash n\  \ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \  list1: The first sorted list.\textbackslash n\  \  list2: The second sorted list.\textbackslash n\  \  k: The desired kth smallest element.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \  The kth smallest element in the union of the two lists.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(list1), len(list2)\textbackslash n\  \ i, j = 0, 0\textbackslash n\  \ min\_heap = []\  \textbackslash n\textbackslash n\ \# Build a min-heap with the first elements of both lists\textbackslash n\  \ for x in range(min(m, n)):\textbackslash n\  \  heapq.heappush(min\_heap, (list1[x], x, 0))\ \# (value, list\_index, position\_in\_list)\textbackslash n\  \  heapq.heappush(min\_heap, (list2[x], x, 1))\textbackslash n\textbackslash n\ \# Extract k smallest elements from the heap\textbackslash n\  \ for \_ in range(k - 1):\textbackslash n\  \  \_, \_, \_ = heapq.heappop(min\_heap)\textbackslash n\textbackslash n\ \# The top element of the heap is the kth smallest\textbackslash n\  \ return heapq.heappop(min\_heap)[0]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\  \ - `m` and `n` store the lengths of the input lists.\textbackslash n\  \ - `i` and `j` are pointers to track the current position in each list.\textbackslash n\  \ - `min\_heap` is a min-heap used to efficiently store and retrieve the smallest elements encountered so far.\textbackslash n\textbackslash n2. **Building the Min-Heap:**\textbackslash n\  \ - The code iterates through the first `min(m, n)` elements of both lists.\textbackslash n\  \ - For each element, a tuple `(value, list\_index, position\_in\_list)` is pushed onto the `min\_heap`. This tuple helps us keep track of the element's value, the list it belongs to, and its original position.\textbackslash n\textbackslash n3. **Extracting k-1 Smallest Elements:**\textbackslash n\  \ - The `for` loop runs `k - 1` times, effectively extracting the `k-1` smallest elements from the `min\_heap`.\textbackslash n\textbackslash n4. **Finding the kth Smallest:**\textbackslash n\  \ - After the loop, the top element of the `min\_heap` contains the `k`th smallest element.\textbackslash n\  \ - `heapq.heappop(min\_heap)` removes and returns this element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- Building the min-heap: O(m + n)\textbackslash n- Extracting k-1 elements: O(k * log(k))\textbackslash n- Overall: **O(m + n + k * log(k))**, which is approximately **O(m + n)** since `k` is usually much smaller than `m + n`.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other questions!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\ Args:\textbackslash n\  \ list1: The first sorted list.\textbackslash n\  \ list2: The second sorted list.\textbackslash n\  \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\  \ The kth smallest element in the union of the lists.\textbackslash n\ """\textbackslash n\textbackslash n\ i = 0\  \# Index for list1\textbackslash n\ j = 0\ \# Index for list2\textbackslash n\ merged = []\  \# Store the merged elements\textbackslash n\textbackslash n\ while i < len(list1) and j < len(list2):\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list1\textbackslash n\ while i < len(list1):\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list2\textbackslash n\ while j < len(list2):\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ return merged[k - 1]\  \# Return the kth element (index k-1)\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash n\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `i` and `j` are index pointers for `list1` and `list2` respectively, starting at 0.\textbackslash n\ - `merged` is an empty list to store the merged sorted elements.\textbackslash n\textbackslash n2. **Merging:**\textbackslash n\ - The `while` loop continues as long as both `i` and `j` are within the bounds of their respective lists.\textbackslash n\ - In each iteration, it compares the elements at `list1[i]` and `list2[j]`.\textbackslash n\ - The smaller element is appended to `merged`, and the corresponding index (`i` or `j`) is incremented.\textbackslash n\textbackslash n3. **Adding Remaining Elements:**\textbackslash n\ - After one list is exhausted, the remaining elements from the other list are directly appended to `merged`.\textbackslash n\textbackslash n4. **Returning the kth Element:**\textbackslash n\ - Finally, `merged[k - 1]` is returned, which represents the kth smallest element in the union (remember that list indices start from 0).\textbackslash n\textbackslash n**Linear Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through each element in both lists at most once during the merging process.\textbackslash n- The time complexity is therefore O(m + n), which is linear in the total number of elements (m + n), making it efficient for large lists.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\scriptsize \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\scriptsize You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\scriptsize }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize The assistant's answer is incorrect. The user asked for a solution with linear complexity, but the assistant provided a solution with a time complexity of O(m + n + k * log(k)), which is not linear. The assistant's solution uses a min-heap, which is not necessary and adds unnecessary complexity to the solution. \newline\newline Rating: [[2]], "score": 2, "turn": 1, "tstamp": 1722737030.6411152}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize The assistant's answer is correct and helpful. It provides a Python function that implements the two-pointer approach to find the kth smallest element in the union of two sorted lists. The assistant's function is slightly different from the reference, but it achieves the same goal. The assistant's function merges the two lists into a new list and then returns the kth element from the merged list. The assistant also provides a detailed explanation of how the function works and confirms that the time complexity is linear, which is what the user asked for. However, the assistant's function uses extra space to store the merged list, which is not necessary and not as efficient as the reference. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722846543.867601}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-4}
\end{table}

==> app-icml/tab-gen-5.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  You are right to ask! While the previous algorithm has linear time complexity, we can achieve an even better solution with **O(log(min(m, n)))** time complexity using a slightly more sophisticated approach.\textbackslash n\textbackslash nThe key idea is to leverage the sorted nature of the lists and use a **binary search** strategy.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash n\textbackslash\#\#\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ \ """\textbackslash n\ \ Finds the kth smallest element in the union of two sorted lists with O(log(min(m, n))) time complexity.\textbackslash n\textbackslash n\ \ Args:\textbackslash n\ \ list1: The first sorted list.\textbackslash n\ \ list2: The second sorted list.\textbackslash n\ \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ \ Returns:\textbackslash n\ \ The kth smallest element in the union of the lists.\textbackslash n\ \ """\textbackslash n\ \ m, n = len(list1), len(list2)\textbackslash n\ \ if m > n:\textbackslash n\ \ list1, list2, m, n = list2, list1, n, m\ \# Ensure list1 is the shorter one\textbackslash n\textbackslash n\ \ left, right = 0, m\textbackslash n\ \ while left <= right:\textbackslash n\ \ partitionX = (left + right) // 2\textbackslash n\ \ partitionY = k - partitionX\textbackslash n\textbackslash n\ \ maxLeftX = list1[partitionX - 1] if partitionX > 0 else float('-inf')\textbackslash n\ \ minRightX = list1[partitionX] if partitionX < m else float('inf')\textbackslash n\textbackslash n\ \ maxLeftY = list2[partitionY - 1] if partitionY > 0 else float('-inf')\textbackslash n\ \ minRightY = list2[partitionY] if partitionY < n else float('inf')\textbackslash n\textbackslash n\ \ if maxLeftX <= minRightY and maxLeftY <= minRightX:\textbackslash n\ if partitionX == 0:\textbackslash n\ \ return list2[partitionY - 1]\textbackslash n\ elif partitionY == 0:\textbackslash n\ \ return list1[partitionX - 1]\textbackslash n\ else:\textbackslash n\ \ return max(list1[partitionX - 1], list2[partitionY - 1])\textbackslash n\ \ elif maxLeftX > minRightY:\textbackslash n\ right = partitionX - 1\ \# Too many elements on the right side of list1\textbackslash n\ \ else:\textbackslash n\ left = partitionX + 1\ \# Too many elements on the right side of list2\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Shorten Lists:** If `list1` is longer than `list2`, swap them to ensure `list1` is always the shorter one. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\ \ - `left` and `right` pointers define the search space within `list1`.\textbackslash n\ \ - `partitionX` is the middle point in `list1`, and `partitionY` is calculated to divide the remaining elements in `list2` such that `partitionX + partitionY = k`.\textbackslash n\ \ - `maxLeftX`, `minRightX`, `maxLeftY`, and `minRightY` represent the largest element to the left and smallest element to the right of the partitions in both lists.\textbackslash n\textbackslash n3. **Comparison and Adjustment:**\textbackslash n\ \ - If the `maxLeftX` is less than or equal to `minRightY` and `maxLeftY` is less than or equal to `minRightX`, it means the kth smallest element lies within the current partitions. We return the larger of `maxLeftX` and `maxLeftY`.\textbackslash n\ \ - If `maxLeftX` is greater than `minRightY`, it indicates that we need to search in the left subarray of `list1` (i.e., decrease `right`).\textbackslash n\ \ - Otherwise, we search in the right subarray of `list1` (i.e., increase `left`).\textbackslash n\textbackslash n4. **Termination:** The binary search continues until `left` crosses `right`, indicating the correct partition has been found.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The binary search divides the search space in half at each step.\textbackslash n- Therefore, the time complexity is O(log(min(m, n))), which is significantly faster than linear time for large lists where one list is much smaller than the other.
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's first response to the user's question is incorrect. The user asked for a function to find the kth smallest element in the union of two sorted lists with linear complexity. The assistant provided a function that uses a min-heap, which has a time complexity of O(m + n + k * log(k)). This is not linear complexity, as the user requested. The assistant's second response to the user's question is also incorrect. The user asked if there exists an algorithm with better time complexity than linear. The assistant provided a function that has a time complexity of O(m + n), which is linear, not better than linear. The assistant should have provided a function that uses a binary search approach, which has a time complexity of O(log(m) + log(n)), as the reference answer correctly does. \newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737031.5033472}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's response is correct and helpful. The assistant provided a Python function that uses a binary search approach to find the kth smallest element in the union of two sorted lists. The assistant also provided a detailed explanation of how the function works, including the time complexity of the function. The assistant's answer matches the reference answer in terms of the algorithm used and the explanation provided. The assistant also correctly identified that the binary search approach has a better time complexity than the linear approach. However, the assistant's code has a minor issue. The assistant's code does not handle the case when `k` is greater than the sum of the lengths of the two lists. In such a case, the code will raise an `IndexError`. This can be fixed by adding a check at the beginning of the function to return `None` if `k` is greater than the sum of the lengths of the two lists. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846556.6828268}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{\centering (Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-5}
\end{table}

==> app-icml/tab-gen-6.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-6}
\end{table}

==> app-icml/tab-gen-script.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app-icml/tab-gen.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\small }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\small }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================



\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app/app-ablation.tex <==
\section{Additional Experimental Results (as Extensions)}\label{app:ablation}


\subsection{Experiments on Different \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{evolve}}(\textperiodcentered)} Methods}\label{app:exp-evol}

As an addition to Table~\ref{tab:main-10k}, we have experimented with three different \texttt{\small evolve}(\textperiodcentered) methods, including:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{SelfInstruct}~\citep{self-instruct}: Given seed prompts, variations are created based on criteria such as verb diversity and style blending (mixing interrogative and imperative styles). Unlike EvolInstruct~\citep{wizardlm}, which generates prompt variations sequentially, this approach generates independently. We follow the one-shot implementation in  \href{https://github.com/argilla-io/distilabel/blob/844165f25c1674076a8286d54cfe96d52c33a24e/src/distilabel/steps/tasks/self_instruct.py#L106}{\texttt{\small self\_instruct.py}} of \texttt{\small distilabel==1.4.1} and modified the instruction on conciseness so that those newly generated prompts have similar lengths compared to the seed prompts. \vspace{+1.5pt}
    \item \textbf{EvolQuality} and \textbf{EvolComplexity}~\citep{deita}: The two methods use the same evolutionary approach (\ie sequentially generating), but with slightly different meta-instructions for prompt generation, where EvolQuality asks to improve the quality (\ie helpfulness, relevance, etc) of the seed prompt and EvolComplexity asks to improve the complexity (\ie increased reasoning steps, etc) of the seed prompt. We follow the implementation in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_quality/utils.py}{\texttt{\small evol\_quality/utils.py}} and \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/evol_complexity/utils.py}{\texttt{\small evol\_complexity/utils.py}} of \texttt{\small distilabel==1.4.1}.
\end{itemize}


% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolInstruct}) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolQuality}) & \text{58.7}  & 721 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolComplexity}) & \textbf{60.6}  & 749 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small SelfInstruct}) & \text{57.2}  & 725 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using different evolving methods.}
\label{tab:evol-10k}
\end{table}
\vspace{-10pt}
% ----------

\vspace{-10pt}
\paragraph{\method~is effective under different evolving methods.} As shown in Table~\ref{tab:evol-10k}, our method brings strong performance gain without training with additional human prompts. Among the experimented methods, we find EvolComplexity shows better results. 

We believe the main strength of such method is its \textbf{simplicity}. Viewing the evolving process as $\rvx' \gets p_{\vtheta}(\cdot \mid  \rvx, \texttt{\small meta\_prompt})$, one can easily tune the meta prompt in natural language for improved performance. However, such simplicity comes at a price: (i) the main weakness is that the default method does not take \textbf{environmental feedback} into account (\eg rewards received, verbal critique on responses, etc) and relies on the pre-defined meta prompt, thus the evolving may be less directional; we encourage practitioners to consider incorporating more richer feedback during evolving (one way to formulate this is by generative optimization~\citep{textgrad,trace,trace-pre}); (ii) another weakness is that existing method is single-shot (\ie we evolve based on a single $\rvx$ each time), thus the \textbf{diversity} of the generation may be limited -- we anticipate future works improving this with multi-shot evolving by graph-based sampling. In this regard, the evolving process can be viewed as $\{\rvx'\}_{i=1}^{N} \gets p_{\vtheta}(\cdot \mid  \{\rvx\}_{i=1}^{M}, \texttt{\small meta\_prompt}, \texttt{\small env\_feedback})$.

\subsection{Experiments on Number of Iterations}\label{app:exp-iter}

As an addition to $\S$~\ref{sec:ab-cont}, we have experimented with the following settings:
\vspace{-5pt}
\begin{itemize}
    \item 10K prompts per iteration with 3 iterations.
    \item 20K prompts per iteration with 3 iterations (\ie all seed prompts are used).
    \item 60K prompts per iteration with 2 iterations (\ie all seed prompts are used).
\end{itemize}

 
Due to time constraints, we did not perform an extensive hyper-parameter search; however, we believe the results presented below sufficiently demonstrate the performance gains achieved by~\method.

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)     & 51.6  & 651  \\

$\vtheta_{1 \rightarrow 2}$: DPO (10k)     & 59.8  &   718\\

$\vtheta_{2 \rightarrow 3}$: DPO (10k)   & 61.2  & 802  \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.0}  & 787  \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.2}  & 774  \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 10k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-10k}
\end{table}
\vspace{-10pt}
% ----------


% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (20k)     & 53.2  & 625 \\

$\vtheta_{1 \rightarrow 2}$: DPO (20k)     & 47.0  & 601  \\

$\vtheta_{2 \rightarrow 3}$: DPO (20k)   & 46.8  & 564 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{59.5}  & 826 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{60.0} & 817 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{61.4} & 791 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 20k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-20k}
\end{table}
\vspace{-10pt}
% ----------

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (60k)    & 58.9  & 717 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (60k) & \text{59.6}  & 725 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{1}'}$: \hspace{-6pt} \quad + \texttt{\textbf{eva}} (60k) & \text{61.9}  & 792 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of using 60k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-60k}
\end{table}
\vspace{-10pt}
% ----------


\paragraph{\method~can bring robust gains with multiple iterations.} As shown in Table~\ref{tab:ab-10k},~\ref{tab:ab-20k}, and~\ref{tab:ab-60k} below, our method presents persistent performance gain over iterations, and concretely surpasses the performance by default DPO training with true human prompts. 


However, there exist diminishing marginal gains in iterative off-policy training. We ground~\method~in the iterative (off-policy) preference alignment paradigm due to its efficiency and ease of integration. However, such paradigms inherently face diminishing returns, where performance gains decrease with successive iterations, as previously observed in~\citep{self-play-gu,8fold,self-reward,cont-primary-bias}. While the generative data schedule in~\method~mitigates these challenges and extends beyond default training with human prompts (see also $\S$\ref{sec:ab-cont}), the gains can weaken over iterations. We summarize potential reasons as: (i) the \textbf{off-policy signal decay} -- as the number of examples increases, signals from the off-policy data become weaker due to distributional shift; (ii) the \textbf{loss of plasticity}, where the agent's ability to learn good policies decreases in continuing training with more iterations~\citep{cont-primary-bias}; (iii) the \textbf{ability of the solver} -- as we evolve more harder prompts, it is harder for the solver to produce preferred response (thus more explicit reasoning techniques may be needed); (iv) the \textbf{ability of the reward model} to correctly provide reward signals to responses and thus informativeness signals to prompts, as there may exists distributional mismatch.

Thus, we envision future work to build on~\method~by: (i) exploring its integration with \textbf{on-policy RLHF} (\eg instead of evolving prompts in iterations, one may evolve in batches); (ii) \textbf{enhancing solver capabilities}, such as sampling more responses during inference or leveraging meta-instructions to guide deeper reasoning; (iii) continual training of reward models for them to co-evolve with the  creators and the solvers. 









\subsubsection{Bonus Experiments on \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{rewriter}}(\textperiodcentered)} In The Loop}\label{app:exp-rewriter}

We present the basic idea here for practitioners to build upon. The motivation comes from the hypotheses derived from $\S$~\ref{app:exp-iter}: as the prompts gets harder by evolving, there may be greater demands on the solver’s capabilities \emph{compared to earlier iterations}. As such, the solver may not be naively treated the same. One may address this by either scaling  up response sampling or introducing meta-instructions to explicitly enhance the solver’s reasoning.

We design a proof-of-concept experiment \emph{w.r.t} the latter by adding \textbf{rewriter} in \method's solver step. Previously, as in Algo.~\ref{alg:i-eva} and  $\S$~\ref{sec:solver-step}, for each prompt $\rvx$, we generate multiple responses, and choose the best as $\rvy_{+}$ and the worst as $\rvy_{-}$ for preference optimization. Now, we add one more rewriting step that attempts to enhance $\rvy_{+}$ to be $\rvy'_{+}$, by applying a rewriting instruction~\citep{deita} that asks the solver to alter $\rvy_{+}$ with imporved helpfulness, relevance, reasoning depths, creativity and details while keeping the similar length. We then train with $(\rvx, \rvy'_{+}, \rvy_{-})$ for preference optimization. Table~\ref{tab:rewriter-10k} shows that adding the rewriter yields concrete performance gains over the default training method, while keeping the training budget and only slightly increasing cost for offline data generation.
% \vspace{-3pt}

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)    & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \textbf{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} with \texttt{\textbf{rewriter}} (10k) & \textbf{61.9}  & 741 \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering Results of adding \textbf{\texttt{\small rewriter}} in the \textbf{\texttt{\small solver}} step.}
\label{tab:rewriter-10k}
\end{table}
\vspace{-10pt}
% ----------



==> app/app-curr.tex <==
\section{Curriculum Visualization Over Iterations}\label{app:curr}
% \subsection{Curriculum Effect on Prompt Categories}\label{app:curr-cat}
We now present initial observations supporting the intuition in $\S$~\ref{sec:int}, where~\method~brings auto-curricula and the creator is incentivized to create new prompts that are both learnable and worth-learning.

% \begin{figure}[H]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
%         \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
%         \label{fig:dist}
%     \end{minipage}
%     \hspace{0.02\textwidth} % Adjust horizontal space as needed
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/radar-gemma.png}
%         \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
%         \label{fig:radar-gemma}
%     \end{minipage}
% \end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/bart-iter.pdf}\vspace{-3pt}
    \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification.  \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
    \label{fig:dist}
\end{figure}

\vspace{-6pt}
% \subsection{Curriculum Effect on Benchmark Performance}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.66\linewidth]{figs/radar-gemma.png}\vspace{-3pt}
    \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
    \label{fig:radar-gemma}
\end{figure}

\subsection{Complexity and Quality of Prompts Over Iterations}\label{app:curr-2}
% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\centering \text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity}
\end{table}
\vspace{-10pt}
% ----------

As in Table~\ref{tab:prompt-quality-complexity}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. We sample 10K prompts per iteration, and use the below prompts modified from~\cite{deita} for the complexity and quality evaluation, with \texttt{\small gemini-1.5-flash} as the scorer:

\texttt{\scriptsize > Rank the following questions according to their \textbf{quality}. Your evaluation should consider the below factors: Helpfulness, Relevance, Accuracy, Depth, Creativity, and Level of detail.
Score each response from 1 to 5: \\1: Poor quality, 2: Below average, 3: Average, 4: Good, 5: Excellent.}


\texttt{\scriptsize > Rank the following questions according to their difficulty and \textbf{complexity}. Use a fixed scoring system: \\1: Very simple, 2: Simple, 3: Moderate,  4: Difficult, 5: Very difficult.}



\section{Visualization on Prompt Selection Metric}\label{app:metric}

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-pdf.pdf}
        % \vspace{+0.00001pt}
        \caption{The probability density distributions of  informativeness metrics compared in Table~\ref{tab:ab-metric} -- they show different patterns.}
        \label{fig:metric-pdf}
    \end{minipage}
    \hspace{0.02\textwidth}
    % \hfill
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-corr.pdf}
        % \vspace{+0.00001pt}
        \caption{The correlation plot for reward advantage (ours) and reward variance -- they are only \emph{weakly} correlated.}
        \label{fig:metric-corr}
    \end{minipage}
    % \hspace{4\textwidth} % Space between the two main figures
\end{figure}

In~\method, we assign each prompt an informativeness value, which the creator will use as the weight to sample from the seed prompts for prompt synthesis. In $\S$~\ref{sec:ab-metric}, we have shown that traditional methods like reward mean and reward variance are less effective as our advantage-based informativeness proxy. The intuition is simple: advantage/regret-based proxy aligns better with the preference optimization objective. We here further illustrate that they are statistically different from other choices:\vspace{-6pt}
\begin{itemize}
    \item Figure~\ref{fig:metric-pdf}: The distribution of informativeness values shows that reward variance is heavily concentrated at lower values, reward mean is more uniformly scattered, and reward advantage achieves a better balance, providing a broader yet also focused sampling range.\vspace{+1.5pt}
    \item Figure~\ref{fig:metric-corr}: The \emph{weak correlation} between reward variance and reward advantage shows that variance \emph{cannot} serve as a substitute for advantage as a proxy for informativeness.
\end{itemize}
\vspace{-6pt}
We have discussed the contrastive curriculum hypothesis in $\S$~\ref{sec:int} to support using reward advantage in the sense that the induced samples tend to decrease the loss the most in the contrastive optimization. Furthermore, assuming the optimization algorithm can converge to the \emph{more optimal} responses, neither reward mean nor variance directly capture the learning potential of such responses -- one may easily construct cases with identical variance yet differ much in reward range -- thus variance fails to distinguish such scenarios. By contrast, reward advantage estimate inherently captures the relative improvement towards better response, and is sensitive to differences in reward range; variants of advantage estimate are commonly used in literature, and we discuss underlying principles in $\S$~\ref{app:theory}.

% specifically, \emph{max - min} mimics the worst case, while \emph{max - mean} is more akin to the Bayesian view.

% By contrast, reward advantage inherently captures the relative improvement toward the optimal response, making it sensitive to such differences in reward range. Specifically, max-min provides a worst-case guarantee by considering the full reward span, while max-mean emphasizes the potential of the more optimal response by focusing on deviations from the average.

==> app/app-downtream.tex <==
\section{Additional Experimental Results for the Main Paper}\label{app:downstream}


In general,~\method~maintains the downstream performance and is robust on reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to training sources for such reward models.
% \input{tables/tab-ab-downstream}
% \vspace{-8pt}

% \input{tables/tab-ab-rm-app}

% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\centering \textbf{Performance on Downstream tasks.}}
\label{tab:ab-downstream}
\end{table}



\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) &  \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 55.01 & 51.68  \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & 9.04 & 8.75 & 60.1  &  55.35 &    55.53 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  & \textbf{56.12} & \textbf{56.40} \\

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\centering \textbf{Effect of (pointwise) reward models.}}
\label{tab:ab-rm-app}
\end{table}
 % on relevant benchmarks
 \vspace{-8pt}

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7 & 51.58 & 42.17 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & 8.78 & \textbf{9.11} &  8.45 &  58.9 & 51.86 & 43.04 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & \textbf{52.71} & \textbf{44.52} \\

\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\centering \textbf{Effect of (pairwise) reward models.}}
\label{tab:ab-rm-sppo-app}
\end{table}
\vspace{-5pt}


==> app/app-lit.tex <==
% \newpage
\section{Extended Literature Review for Open-Ended Learning}\label{app:lit}

% \subsection{Extended Literature Review on Open-Endedness}

The design of our game-theoretic framework for language model post-training is inspired from many prior works in open-ended learning. The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that  can \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but broad enough to handle the diversity of complexity of future environments. In such curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively builds more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case (\ie most adversarial) environments.  In addition to distinctions discussed in~$\S$~\ref{sec:lit}, we here list several foundational works in this line, and encourage the LLM community to explore with more rigor and depth: \cite{schmidhuber1991possibility} presents an initial investigation into open-ended learning via self-supervised curiosity-driven exploration; \cite{poet} emphasize co-evolution of environments and agent policies by training a population of agents that adapt to and solve progressively complex challenges; \cite{paired} formally introduce the notion of Unsupervised Environment Design (UED), where a protagonist and antagonist agent pair simulates regret by competing in shared environments, driving the protagonist (the main learner) to adapt to increasingly challenging scenarios; \cite{plr} introduce Prioritized Level Replay (PLR), which uses a rolling buffer of high-regret levels to dynamically adjust the training curriculum, and selects levels with the higher learning potential; \cite{accel} further propose improvements by editing previously high-regret levels; \cite{open-endedness} present a formal definition for open-ended system with respect to \emph{novelty} and \emph{learnability}, that generalizes various systems, \eg AlphaGo~\citep{alphago}, AdA~\citep{team2021open}, etc.
% \vspace{-10pt}

% Our focus was on classical, seminal, and directly relevant works. We welcome suggestions for any other references we may have missed that can enhance our citations -- please feel free to reach out.


==> app/app-loss.tex <==
\section{Plug-In Loss Functions Used in Main Results}~\label{app:loss}
\vspace{-.8cm}
\begin{table}[H]
\centering
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{With Reference Model}    \\ \midrule
DPO~\citep{dpo}  &  $\ell_{\beta}(\pi_{\vtheta})  = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_\vtheta};  {\pi_{\text{ref}}}}^{\rvx} \Bigr)\Bigr] \textcolor{lightgray}{:= - \log \left[\sigma\left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}- \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \right)\right]} $                   \\


SPPO~\citep{self-play-gu}  & $\ell_{\beta}(\pi_{\vtheta})  = - \log \left[\sigma\left( \left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)} - \frac{1}{2}\right)^2 + \left( \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}+ \frac{1}{2}\right)^2  \right)\right]$  \\ 
\midrule
\multicolumn{2}{c}{Without Reference Model} \\ \midrule
SimPO~\citep{simpo} &  $ \ell_{\beta, \alpha}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_{\theta}^{1/|\rvy|}};  1}^{\rvx} - \alpha \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \frac{\beta}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx) -  \frac{\beta}{|\rvy_{-}|} \log \pi_{\vtheta}(\rvy_{-} | \rvx) -\alpha \right)\right]} $                   \\
ORPO~\citep{orpo} &  $ \ell_{\lambda}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\lambda \cdot  \Delta_{\text{odds}_{\vtheta};  1}^{\rvx}  \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \lambda \cdot \log \frac{\text{odds}_{\vtheta}(\rvy_{+} | \rvx)}{\text{odds}_{\vtheta}(\rvy_{-} | \rvx)}  \right)\right]} $\textcolor{lightgray}{, where $\text{odds}_{\vtheta}=\frac{\pi_\vtheta}{1 - \pi_{\vtheta}}$}                   \\
% ORPO~\citep{orpo} &   $\ell_{\lambda}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphslate{\dlogodds} \right)\right]$              \\ 
\bottomrule
\end{tabular}%
}
\caption{Direct preference alignment algorithms used in the main experiments. In parameter tuning, we include an additional negative log-likelihood loss for chosen responses (\ie~$\frac{\gamma}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx)$).}
\label{tab:offline}
\end{table}

==> app/app-prompt-examples.tex <==
\section{Examples on Prompts and Model Generations}\label{app:examples}
\vspace{-12pt}

% ------------------
\begin{figure}[H]
    % \centering
    % \begin{minipage}{0.39\textwidth}
    \centering
    \includegraphics[width=0.4\linewidth]{figs/example-prompt.png}
    \vspace{-4pt}
    \caption{The initial prompt distribution of AlpacaEval by \texttt{\small bart-large-mnli} with 0-shot classification, which is imbalanced. For the reward distribution, the category with lowest average reward has the highest  reward gap (\ie the default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
    % \end{minipage}
\end{figure}
% \vspace{-12pt}
% ------------------




% ------------------
% \begin{table}[H]
% \centering
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}r p{14cm}@{}}
% \toprule
% \rowcolor{lightgray!16}
% \multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small If a man smokes 1000 cigarettes a day, why is he getting healthier?} \\ \midrule
% \texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Elaborate on the seemingly paradoxical situation where an individual consumes 1000 cigarettes daily yet exhibits signs of improving health, delineating the factors that could underlie such an unexpected outcome.} \\
% \texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Discuss the conundrum of a person drinking a gallon of caffeinated coffee every hour but displaying unusually deep and restful sleep patterns, exploring possible explanations for this unusual phenomenon.} \\
% \texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Examine the paradox of an individual who ingests a gallon of caffeine-laden coffee hourly yet exhibits signs of profoundly tranquil slumber, delving into potential theories that could elucidate this atypical occurrence, and considering the role of genetic predispositions in such a scenario.} \\
% \texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Analyze the conundrum of a person consuming an entire gallon of heavily caffeinated coffee every single hour and yet demonstrating the ability to fall into a state of deep sleep, exploring plausible hypotheses that could illuminate this unusual event, including an assessment of how genetic factors might influence this ability, and include an evaluation of the impact of acquired tolerance to caffeine over time.} \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-4pt}
% % \caption{Examples of evolved prompts from AlpacaEval.}
% \label{tab:prompt-evol}
% \end{table}
% ------------------

\vspace{-10pt}

% ------------------
\begin{table}[H]
\centering
\resizebox{.66\columnwidth}{!}{%
\begin{tabular}{@{}r p{12.6cm}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small Write me the code for a distributed transaction manager.\textbackslash nThink step by step and use pseudo code first.\textbackslash nThen, define interfaces for all involved actors and entities.\textbackslash nUse Rational Unified approach for this part.\textbackslash n\textbackslash nOnly then move on to the actual implementation, class-by-class, and method-by-method.\textbackslash nMake the code be implemented in C\# and follow SOLID principles.} \\ \midrule
\texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Craft a suite of syntax for a distributed transaction coordinator. Start with a sequential breakdown in pseudocode format. Following that, establish the protocols for communication and interaction amongst the various participants and components, incorporating the Rational Unified Process methodology.\textbackslash n\textbackslash nProceed thereafter to the concrete creation, detailing each class and function. Ensure that the final C\# code adheres to the precepts of SOLID and is annotated for clarification and maintainability purposes.} \\
\texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Devise a comprehensive set of directives and structures for a distributed transaction coordinator architecture. Initiate by formulating a step-by-step algorithmic decomposition in pseudocode. Subsequently, delineate the frameworks for dialog and cooperation between the numerous entities and elements, utilizing the tenets of the Rational Unified Process methodology.\textbackslash n\textbackslash nContinue to the actual generation of the code, meticulously detailing every class and corresponding method. Guarantee that the culminating C\# code is in strict compliance with SOLID principles and is supplemented with descriptive commentary to enhance future clarity and upkeep, while also validating the code against a set of unit tests to ensure robust functionality.} \\
\texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Commence by constructing an algorithm in pseudocode that meticulously breaks down the sequential stages for a distributed transaction coordinator system. Progress by outlining the communication protocols and collaborative mechanisms among the myriad components, adhering to the Rational Unified Process approach.\textbackslash n\textbackslash nAdvance to crafting the code in C\#, ensuring each class and method is elaborated with precision, aligning with SOLID design principles. Integrate thorough comments for heightened maintainability and conduct comprehensive unit testing for assured operational integrity.} \\
\texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Design a detailed flowchart that represents the intricate steps of an orchestration engine for managing microservices in a cloud-native environment. Begin by detailing the service discovery, load balancing, and fault tolerance strategies, while incorporating the DevOps philosophy.\textbackslash n\textbackslash nProceed by developing the implementation in Java, focusing on clean, modular code following object-oriented programming best practices. Accompany your code with clear documentation for easy understanding and perform rigorous integration testing to guarantee robustness.} \\ \bottomrule
\end{tabular}%
}
% \vspace{-4pt}
\caption{Examples of evolved prompts from AlpacaEval. We suggest practitioners to include generated responses with oracle rewards and self-critique in the context for better prompt evolving, which is helpful for mitigating the effect of potential self-consuming loops in synthetic data training.}
\label{tab:prompt-evol-2}
\end{table}
% ------------------






\newpage

\hspace{0pt}
\vfill

\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} \texttt{\small When a number is divided by 10, the remainder is 4. What is the remainder when twice the number is divided by 4?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
* "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
* Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
* (20*k + 8) divided by 4 is (20*k)/4 + 8/4 = 5*k + 2\newline
4. Find the remainder:\newline
* Since 5*k is a multiple of 4, the remainder when twice the number is divided by 4 is 2.\newline
Let me know if you'd like to try another example!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}} 
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
- "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
- Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
- When (20*k + 8) is divided by 4, the 20*k term is perfectly divisible by 4.\newline
- The remainder will be the same as the remainder when 8 is divided by 4, which is 0.\newline
Therefore, the remainder when twice the number is divided by 4 is 0.}
\end{tabular} \\ \midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} \texttt{\small What about when twice the number is divided by 5?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 is (20*k)/5 + 8/5 = 4*k + 1.6\newline
3. Find the remainder: Since 4*k is a multiple of 5, the remainder when twice the number is divided by 5 is 1.\newline
Let me know if you have any more number theory puzzles!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. \text{Twice the number:} We know twice the number is 20*k + 8 (from the previous steps).\newline
2. \text{Divide by 5:} \newline
\ \ \ * 20*k is divisible by 5.\newline
\ \ \ * 8 divided by 5 leaves a remainder of 3.\newline
Therefore, the remainder when twice the number is divided by 5 is 3.}
\end{tabular} \\ 

\midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's response is incorrect. The assistant incorrectly calculated the remainder when twice the number is divided by 5. The assistant calculated the decimal part of the division operation, not the remainder. The correct calculation should be (20n + 8) \% 5 = (20n \% 5) + (8 \% 5) = 0 + 3 = 3. Therefore, the remainder when twice the number is divided by 5 is 3, not 1 as the assistant stated.\newline
\newline
The corrected response would be:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 gives us a remainder of (20*k \% 5) + (8 \% 5) = 0 + 3 = 3.\newline
3. Find the remainder: The remainder when twice the number is divided by 5 is 3.\newline
\newline
Rating: [[3]], "score": 3, "turn": 2, "tstamp": 1722737011.7768948}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's answer is correct and matches the reference answer. The assistant correctly explains that twice the number is 20*k + 8 and that when this is divided by 5, the remainder is 3. The assistant's explanation is clear and easy to understand, making it helpful for the user. There are no mistakes to correct.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846518.5543818}

\end{tabular} \\ 

% \sbt{Judgment for gemma-2-9b-it-dpo} & \sbt{Judgment for gemma-2-9b-it-dpo-eva} \\ 

\bottomrule
\end{tabular}%
}
\caption{\centering Comparison of model generations on examples from MT-Bench.}
\label{tab:gen-0}
\end{table}


\vfill
\hspace{0pt}




% ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-2}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
\hspace{0pt}
\vfill
\input{app/tab-gen-3}
\vfill
\hspace{0pt}
% % ------------------

% ------------------
% \newpage
\hspace{0pt}
\vfill
\input{app/tab-gen-1}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-4}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{app/tab-gen-5}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
% \input{app/tab-gen-6}
% \vfill
% \hspace{0pt}
% % ------------------

==> app/app-reproduce.tex <==
\section{Details on Reproducibility}\label{app:reproduce}
Our code is built based on many open-source packages, and we sincerely thank every developer and contributor of these projects for their efforts and contributions to the community. 

As mentioned, our code base is made to be simple to use for practitioners, requiring \textbf{only a creator module addition} within the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline.

\vspace{-10pt}
\paragraph{Hyperparameter settings.} We follow the original hyperparameter settings as in~\citep{orpo,simpo,self-play-gu}, default to be:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
$\lambda$                                                      & /      & 0.5      & /      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1024   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
\bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-main-params}
\end{table}

\vspace{-10pt}
\paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-reward}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
    \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
    % \item ...
\end{itemize}

For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this and other plug-in evolving methods. For solver we generate 6 responses per prompt. We use 42 as the random seed.

% \paragraph{Computation environments.} 
\vspace{-10pt}
\paragraph{Software environments.} All experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve Gemini (default to be \texttt{\small gemini-1.5-pro}) and transformers models (default to be \texttt{\small gemma-2-9b-it}). For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. 

% We include main Appendix following references, also in \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}.

==> app/app-theory-clean.tex <==
In~\secref{app:theory-1}, we present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}



The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.



\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 


Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.


\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.

\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber

\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.




We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.




\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


==> app/app-theory-old.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

\subsection{Connections in Open-Ended RLHF, Minimax Game and the Proxy}\label{app:intuition}

We provide an extended discussion on $\S$~\ref{sec:method} to make the explanation more coherent and easy-to-understand. Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{cred}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tg{\pi_{\phi}(\rvx)} \cdot \tc{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}), which is a special case if $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expand Eq.~\ref{eq:rlhf-joint-}:

\resizebox{\textwidth}{!}{$
\max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cred}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\textit{KL}}\bigr[\textcolor{cred}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
- \beta \cdot \textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}. \nonumber 
$}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


To clarify, while $\pi_{\text{SFT}}(\cdot)$ refers to the supervised trained model~\citep{rlhf}, the newly proposed $p_{\text{ref}}$ represents an \textbf{open-ended} and potentially intractable probability measure over all possible tasks (instatiated \emph{via} prompts) or user prompts -- note it is not the static training prompt distribution. Here, the regularization $\textcolor{black}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by generating new tasks for self-training and self-improvement, instead of optimizing over a static, pre-defined prompt set. The non-trivial part is on solving this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

In the next, we will provide a step-by-step derivation leading to our Algo.~\ref{alg:i-eva}. To begin with, we first discuss how prior works tractably solve similar open-ended learning problems via two-player game formulation. Next, we formally present the new objective, and discuss how to tractably solve it in our specific setting.

\subsection{Designing Two-Player Games for Open-Ended Environment Design}
The underlying idea is straightforward, while we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$, we are able to create a series of environments. The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

\textcolor{red}{TODO: unifying the theorems/notations in previous literature. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }
\begin{itemize}
    \item \cite{poet}:
    \item \cite{paired}:
    \item \cite{plr}: scoring by generalized advantage estimation
    \item \cite{dcd}:
    \item \cite{accel}:
\end{itemize}

\subsection{Regret Formulation for Open-Ended RLHF}

\subsubsection{Advantage-Based Regret and Approximation by EvolInstruct: The Creator Step}

\subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

\newpage



\textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



 Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
\begin{itemize}
    \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \end{itemize}
    \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \end{itemize}
\end{itemize}

% \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

The regret objective is defined as
\begin{align}
\operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
\end{align}
% $$
% \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% $$

At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
\begin{align}
    \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
\end{align}
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

This approximation introduces two practical advantages:
\begin{enumerate}
    \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
    \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
\end{enumerate}

This deviates from the theoretical Open-Ended RLHF objective. In particular:
\begin{itemize}
    \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
    \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
\end{itemize}

Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


\subsection{KL-Regularized Regret}\label{app:kl}
For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

% This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% \begin{itemize}
%     \item 
%     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% \end{itemize}

\subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
\textcolor{red}{TODO: add derivation to better justify this approximation.}
In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
\begin{align}
    \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
\end{align}

This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
\begin{itemize}
    \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
    \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
    \begin{itemize}
        \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
        \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
    \end{itemize}
    \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
\end{itemize}


We justify this simplification as follows:
\begin{itemize}
    \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
    \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
    \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
\end{itemize}

We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> app/app-theory.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

This is an extended version of $\S$~\ref{sec:method}. In~\secref{app:theory-1}, we re-present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}

% \resizebox{\textwidth}{!}{$
% \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\text{KL}}\bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
% - \beta \cdot \emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}. \nonumber 
% $}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\vspace{-5pt}
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon. \vspace{+1.5pt}
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.

% A common misunderstanding may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks -- a conceptual target derived from the \textit{underspecified distribution}. As shown in Fig.~\ref{fig:metric-corr}, the initial prompt distribution can be defined along several dimensions (\eg the number or complexity of coding problems). A potential creator policy can be made to modify these dimensions to explore new training distributions.





% The probability matching term $\textcolor{cgreen}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities~\citep{jiang-thesis}, instead of constrained in a static, pre-defined prompt set. 
% The non-trivial part is thus on approaching this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

% The following serves as an illustration from Definition~\ref{eq:rlhf-joint} to  Algorithm~\ref{alg:i-eva}, especially on 

% As a background, we first discuss how prior works/heuristics solve similar open-ended learning problems. Next, we formally present the new objective under a game, and discuss how to tractably solve it in our specific setting.

\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
 \vspace{-5pt}
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{\vspace{-40pt}We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\vspace{-5pt}
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on  high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance. There is an additional filtering step: they do not directly train on newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 
% \begin{itemize}
%     \item \textbf{Regret approximation}: the same as~\citep{plr} -- the positive value loss.
%     \item \textbf{Environment generation}: 
% \end{itemize}







 


% \cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones.


% (TODO: give an overview on this setting; our creator follows the similar setting by identifying the high-regret levels and then making edits with them combining a buffer.)
% Later on, researchers explore more \emph{curriclum}-driven approach, especially through adversarial training~\citep{adr} with minimax objective

% . The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

% \textcolor{red}{This section is about heuristics on distributional matching with a game setting. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }

% \subsubsection{Reformulating Constrained Optimization to Minimax Optimization}

% \newpage
\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric  game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in future.

\vspace{-10pt}
\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
    % &= \frac{1}{1 + \exp \left(- (r\left(\mathbf{x}, \mathbf{y}^w\right) - r\left(\mathbf{x}, \mathbf{y}^l\right))\right)} \\
    % &= \sigma \left(r\left(\mathbf{x}, \mathbf{y}^+\right) - r\left(\mathbf{x}, \mathbf{y}^-\right)\right). \label{eq:bt}
\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\vspace{-10pt}
\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

% Thus the regret with regard to the KL-constrained optimal policy is:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \nonumber
% \end{align}


% Assuming $\rvy_+, \rvy_-$ are correctly labeled by an \textit{oracle reward model} $r(\cdot, \cdot)$, the direct preference optimization objective is:
% \begin{align}
%     \mathcal{L}_{\text{DPO}}=-\mathbb{E}_{\rvx \sim \calD, (\rvy_+, \rvy_-) \sim \pi_{\vtheta}(\cdot \mid \rvx)}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_+ \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_+ \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_- \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_- \mid \rvx\right)}\right)\right]. \nonumber
% \end{align}


We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\vspace{-10pt}
\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.


\vspace{-10pt}
\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them, then mixing with a buffer of the original set to form the new training distribution at each iteration.

% While there exist other approximations choices (see our summarization in Table~\ref{tab:info-metric}), we justify our choice for the minimax regret strategy under the context of contrastive preference optimization.

% (High-level idea: the regret is bounded by the range; we first define the range (the underlying assumption is suffient sampling and correct labeling) then show)

% The expected reward under the policy $\pi_\vtheta$ is given by:
% \begin{align}
%     \mathbb{E}_{\rvy \sim \pi_\vtheta(\cdot \mid \rvx)}[r(\rvx, \rvy)] = \sum_{\rvy} \pi_\vtheta(\rvy \mid \rvx) r(\rvx, \rvy), \nonumber
% \end{align}
% and it satisfies the bound:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+). \nonumber
% \end{align}
% Our objective is to show that with high probability, there is $\operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx)$.
% \begin{align}
%     \mathbb{P}\left(\left|\hat{r}_{\mathrm{KL}}-\mathrm{E}_{\mathbf{y} \sim \pi_{\mathrm{kL}}^t}[r(\mathrm{x}, \mathrm{y})]\right| \geq \varepsilon\right) \leq 2 \exp \left(-\frac{2 n \varepsilon^2}{\left(r_{\text {max }}-r_{\text {min }}\right)^2}\right)
% \end{align}

% (TODO: show that as we optimize, the upper bound of info(x) on the regret would be tighter. thus we effectively achieves high-regret seeking. Then discuss the heuristic generation by making edits through evolinstruct etc.)
% Similarly, for the KL-optimal policy $\pi^\star_{\text{KL}}(\rvy \mid \rvx)$, we have:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+).
% \end{align}

% The KL-regularized regret is defined as:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) = \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] - \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)].
% \end{align}

% Using the bounds above, the regret satisfies:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Define the range $\text{info}_\vtheta(\rvx)$ as:
% \begin{align}
%     \text{info}_\vtheta(\rvx) = r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Thus, the regret is bounded by the range:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx).
% \end{align}


% since the regret in Eq.~\ref{eq:KL-regret} is not directly calculable. Specifically, we choose to approximate the regret as:



% A re-formulation of the reward is:
% \begin{align}
%     r(\rvx, \rvy)=r_E(\rvx, \rvy)-\beta\bigr(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\bigr).
% \end{align}




% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}



% \subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

% In this section, we discuss connection between the regret minimization objective and the contrastive preference optimization objective.
% % \textcolor{red}{TODO: derive regret objective and DPO optimization, checking~\citep{cpl}; the KL is explicitly solved.}

% High-level idea: By the Bellman equation, we have:
% \begin{align}
%     A^*(s, a)=Q^*(s, a)-V^*(s, a)=r(s, a)+\gamma \mathbb{E}_{s^{\prime}}\left[V^*\left(s^{\prime}\right)\right]-V^*(s)
% \end{align}

% In the bandit setting, the negated regret :
% \begin{align}
%     A^{\star}(\rvx, \rvy) &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy),\\
%     & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr].
% \end{align}

% The preference model thus becomes:
% \begin{align}
% P_A \left[\sigma^{+} \succ \sigma^{-}\right] & =\frac{\exp r_E\left(s, a^{+}\right)-V^*(s)}{\exp r_E\left(s, a^{+}\right)-V^*(s)+\exp r_E\left(s, a^{-}\right)-V^*(s)} \\
% & =\frac{\exp r_E\left(s, a^{+}\right)}{\exp r_E\left(s, a^{+}\right)+\exp r_E\left(s, a^{-}\right)}
% \end{align}

% (TODO: show the regret-based preference is equivalent to the DPO objective, thus we implicitly minimizes a function of the regret)

% Under the RLHF framework, a reformulation of the reward function is:
% \begin{align}
%     r'(\rvx, \rvy)=r(\rvx, \rvy)-\beta\left(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\right).
% \end{align}

% \textcolor{red}{TODO: write a theoretical version with the above and a practical version with only the true reward model.}

% \subsubsection{Regret Approximation by EvolInstruct: The Creator Step}
% \textcolor{red}{TODO: derive advantage-based regret approximation; then we further approximated it with reward function and proximal editing on seed prompts, thus we do not tractably solve the KL term.}


% (This should be the reward that we use, however we directly take the reward inside)


% \newpage



% \textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

% While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



%  Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

% To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
% \begin{itemize}
%     \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \end{itemize}
%     \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \end{itemize}
% \end{itemize}

% % \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

% This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% The regret objective is defined as
% \begin{align}
% \operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
% \end{align}
% % $$
% % \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% % $$

% At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
% \begin{align}
%     \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}
% % \begin{align}
% %     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% % \end{align}

% This approximation introduces two practical advantages:
% \begin{enumerate}
%     \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
%     \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
% \end{enumerate}

% This deviates from the theoretical Open-Ended RLHF objective. In particular:
% \begin{itemize}
%     \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
%     \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
% \end{itemize}

% Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


% \subsection{KL-Regularized Regret}\label{app:kl}
% For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% % This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% % \begin{itemize}
% %     \item 
% %     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% % \end{itemize}

% \subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
% \textcolor{red}{TODO: add derivation to better justify this approximation.}
% In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
% \begin{align}
%     \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
% \end{align}

% This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
% \begin{itemize}
%     \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
%     \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
%     \begin{itemize}
%         \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
%         \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
%     \end{itemize}
%     \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
% \end{itemize}


% We justify this simplification as follows:
% \begin{itemize}
%     \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
%     \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
%     \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
% \end{itemize}

% We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

% Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> app/tab-gen-6.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-6}
\end{table}

==> app/tab-gen-script.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> app/tab-gen.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\small }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\small }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================



\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> appp/app-ablation.tex <==
\section{Additional Experimental Results (as Extensions)}\label{app:ablation}


\subsection{Experiments on Different \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{evolve}}(\textperiodcentered)} Methods}\label{app:exp-evol}

As an addition to Table~\ref{tab:main-10k}, we have experimented with three different \texttt{\small evolve}(\textperiodcentered) methods, including:
\begin{itemize}
    \item \textbf{SelfInstruct}~\citep{self-instruct}: Given seed prompts, variations are created based on criteria such as verb diversity and style blending (mixing interrogative and imperative styles). Unlike EvolInstruct~\citep{wizardlm}, which generates prompt variations sequentially, this approach generates independently. We follow the one-shot implementation in  \href{https://github.com/argilla-io/distilabel/blob/844165f25c1674076a8286d54cfe96d52c33a24e/src/distilabel/steps/tasks/self_instruct.py#L106}{\texttt{\small self\_instruct.py}} of \texttt{\small distilabel==1.4.1} and modified the instruction on conciseness so that newly generated prompts have similar lengths compared to the seed prompts.
    \item \textbf{EvolQuality} and \textbf{EvolComplexity}~\citep{deita}: The two methods use the same evolutionary approach (\ie sequentially generating), but with slightly different meta-instructions for prompt generation, where EvolQuality asks to improve the quality (\ie helpfulness, relevance, etc) of the seed prompt and EvolComplexity asks to improve the complexity (\ie increased reasoning steps, etc) of the seed prompt. We follow the implementation in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_quality/utils.py}{\texttt{\small evol\_quality/utils.py}} and \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/evol_complexity/utils.py}{\texttt{\small evol\_complexity/utils.py}} of \texttt{\small distilabel==1.4.1}.
\end{itemize}


% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolInstruct}) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolQuality}) & \text{58.7}  & 721 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolComplexity}) & \textbf{60.6}  & 749 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small SelfInstruct}) & \text{57.2}  & 725 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using different evolving methods.}
\label{tab:evol-10k}
\end{table}
\vspace{-10pt}
% ----------

\paragraph{\method~is effective under different evolving methods.} As shown in Table~\ref{tab:evol-10k}, our method brings strong performance gain without training with additional human prompts. Among the experimented methods, we find EvolComplexity shows better results. 

We believe the main strength of such method is its \textbf{simplicity}. Viewing the evolving process as $\rvx' \gets p_{\vtheta}(\cdot \mid  \rvx, \texttt{\small meta\_prompt})$, one can easily tune the meta prompt in natural language for improved performance. However, such simplicity comes at a price: (i) the main weakness is that the default method does not take \textbf{environmental feedback} into account (\eg rewards received, verbal critique on responses, etc) and relies on the pre-defined meta prompt, thus the evolving may be less directional; we encourage practitioners to consider incorporating more richer feedback during evolving (one way to formulate this is by generative optimization~\citep{textgrad,trace,trace-pre}); (ii) another weakness is that existing method is single-shot (\ie we evolve based on a single $\rvx$ each time), thus the \textbf{diversity} of the generation may be limited -- we anticipate future works improving this with multi-shot evolving by graph-based sampling. In this regard, the evolving process can be viewed as $\{\rvx'\}_{i=1}^{N} \gets p_{\vtheta}(\cdot \mid  \{\rvx\}_{i=1}^{M}, \texttt{\small meta\_prompt}, \texttt{\small env\_feedback})$.

\subsection{Experiments on Number of Iterations}\label{app:exp-iter}

As an addition to $\S$~\ref{sec:ab-cont}, we have experimented with the following settings:
\begin{itemize}
    \item 10K prompts per iteration with 3 iterations.
    \item 20K prompts per iteration with 3 iterations (\ie all seed prompts are used).
    \item 60K prompts per iteration with 2 iterations (\ie all seed prompts are used).
\end{itemize}

 
Due to time constraints, we did not perform an extensive hyper-parameter search; however, we believe the results presented below sufficiently demonstrate the performance gains achieved by~\method.

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)     & 51.6  & 651  \\

$\vtheta_{1 \rightarrow 2}$: DPO (10k)     & 59.8  &   718\\

$\vtheta_{2 \rightarrow 3}$: DPO (10k)   & 61.2  & 802  \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.0}  & 787  \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.2}  & 774  \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 10k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-10k}
\end{table}
\vspace{-10pt}
% ----------


% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (20k)     & 53.2  & 625 \\

$\vtheta_{1 \rightarrow 2}$: DPO (20k)     & 47.0  & 601  \\

$\vtheta_{2 \rightarrow 3}$: DPO (20k)   & 46.8  & 564 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{59.5}  & 826 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{60.0} & 817 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{61.4} & 791 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 20k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-20k}
\end{table}
\vspace{-10pt}
% ----------

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (60k)    & 58.9  & 717 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (60k) & \text{59.6}  & 725 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{1}'}$: \hspace{-6pt} \quad + \texttt{\textbf{eva}} (60k) & \text{61.9}  & 792 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 60k prompts per iteration (DPO + length-penalized NLL loss).}
\label{tab:ab-60k}
\end{table}
\vspace{-10pt}
% ----------


\paragraph{\method~can bring robust gains with multiple iterations.} As shown in Table~\ref{tab:ab-10k},~\ref{tab:ab-20k}, and~\ref{tab:ab-60k} below, our method presents persistent performance gain over iterations, and concretely surpasses the performance by default DPO training with true human prompts. 


However, there exist diminishing marginal gains in iterative off-policy training. We ground~\method~in the iterative (off-policy) preference alignment paradigm due to its efficiency and ease of integration. However, such paradigms inherently face diminishing returns, where performance gains decrease with successive iterations, as previously observed in~\citep{self-play-gu,8fold,self-reward,cont-primary-bias}. While the generative data schedule in~\method~mitigates these challenges and extends beyond default training with human prompts (see also $\S$\ref{sec:ab-cont}), the gains can weaken over iterations. We summarize potential reasons as: (i) the \textbf{off-policy signal decay} -- as the number of examples increases, signals from the off-policy data become weaker due to distributional shift; (ii) the \textbf{loss of plasticity}, where the agent's ability to learn good policies decreases in continuing training with more iterations~\citep{cont-primary-bias}; (iii) the \textbf{ability of the solver} -- as we evolve more harder prompts, it is harder for the solver to produce preferred response (thus more explicit reasoning techniques may be needed); (iv) the \textbf{ability of the reward model} to correctly provide reward signals to responses and thus informativeness signals to prompts, as there may exists distributional mismatch.

Thus, we envision future work to build on~\method~by: (i) exploring its integration with \textbf{on-policy RLHF} (\eg instead of evolving prompts in iterations, one may evolve in batches); (ii) \textbf{enhancing solver capabilities}, such as sampling more responses during inference or leveraging meta-instructions to guide deeper reasoning; (iii) online training of RM to co-evolve with the creator and the solver. 









\subsubsection{Bonus Experiments on \hspace{-3.6pt}\texttt{ \textnormal{\bf \texttt{rewriter}}(\textperiodcentered)} In The Loop}\label{app:exp-rewriter}

Though beyond the current package, we present the basic idea here for practitioners to build upon. The motivation comes from the hypotheses derived from $\S$~\ref{app:exp-iter}: as the prompts gets harder by evolving, there may be greater demands on the solver’s capabilities \emph{compared to earlier iterations}. As such, the solver may not be naively treated the same. One may address this by either inference-time scaling on responses or introducing meta-instructions to explicitly enhance the solver’s reasoning.

We design a proof-of-concept experiment \emph{w.r.t} the latter by adding \textbf{rewriter} in \method's solver step. Previously, as in Algo.~\ref{alg:i-eva} and  $\S$~\ref{sec:solver-step}, for each prompt $\rvx$, we generate multiple responses, and choose the best as $\rvy_{+}$ and the worst as $\rvy_{-}$ for preference optimization. Now, we add one more rewriting step that attempts to enhance $\rvy_{+}$ to be $\rvy'_{+}$, by applying a rewriting instruction~\citep{deita} that asks the solver to alter $\rvy_{+}$ with imporved helpfulness, relevance, reasoning depths, creativity and details while keeping the similar length. We then train with $(\rvx, \rvy'_{+}, \rvy_{-})$ for preference optimization. Table~\ref{tab:rewriter-10k} shows that adding the rewriter yields concrete performance gains over the default training method, while keeping the training budget and slightly increasing cost for offline data generation.
% \vspace{-3pt}

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} with \texttt{\textbf{rewriter}} & \textbf{61.9}  & 741 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of adding \textbf{\texttt{\small rewriter}} in the \textbf{\texttt{\small solver}} step.}
\label{tab:rewriter-10k}
\end{table}
\vspace{-10pt}
% ----------



==> appp/app-curr.tex <==
\section{Curriculum Visualization Over Iterations}\label{app:curr}
% \subsection{Curriculum Effect on Prompt Categories}\label{app:curr-cat}
We now present initial observations supporting the intuition in $\S$~\ref{sec:int}, where~\method~brings auto-curricula and the creator is incentivized to create new prompts that are both learnable and worth-learning.

% \begin{figure}[H]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
%         \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
%         \label{fig:dist}
%     \end{minipage}
%     \hspace{0.02\textwidth} % Adjust horizontal space as needed
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/radar-gemma.png}
%         \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
%         \label{fig:radar-gemma}
%     \end{minipage}
% \end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/bart-iter.pdf}\vspace{-3pt}
    \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification.  \method~creates a curriculum that prioritizes math / coding prompts over iterations.}
    \label{fig:dist}
\end{figure}

\vspace{-6pt}
% \subsection{Curriculum Effect on Benchmark Performance}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.66\linewidth]{figs/radar-gemma.png}\vspace{-3pt}
    \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
    \label{fig:radar-gemma}
\end{figure}

\subsection{Complexity and Quality of Prompts Over Iterations}\label{app:curr-2}
% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity}
\end{table}
\vspace{-10pt}
% ----------

As in Table~\ref{tab:prompt-quality-complexity}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. We sample 10K prompts per iteration, and use the below prompts modified from~\cite{deita} for the complexity and quality evaluation, with \texttt{\small gemini-1.5-flash} as the scorer:
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Rank the following questions according to their quality. Your evaluation should consider the following factors: Helpfulness, Relevance, Accuracy, Depth, Creativity, and Level of detail.
Score each response from 1 to 5: 1: Poor quality, 2: Below average, 3: Average, 4: Good, 5: Excellent.
\end{minted}
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Ranking the following questions according to their difficulty and complexity. Use a fixed scoring system: 1: Very simple, 2: Simple, 3: Moderate,  4: Difficult, 5: Very difficult
\end{minted}


\section{Visualization on Prompt Selection Metric}\label{app:metric}

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-pdf.pdf}
        % \vspace{+0.00001pt}
        \caption{The probability density distributions of  informativeness metrics compared in Table~\ref{tab:ab-metric} -- they show different patterns.}
        \label{fig:metric-pdf}
    \end{minipage}
    \hspace{0.02\textwidth}
    % \hfill
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-corr.pdf}
        % \vspace{+0.00001pt}
        \caption{The correlation plot for reward advantage (ours) and reward variance -- they are only \emph{weakly} correlated.}
        \label{fig:metric-corr}
    \end{minipage}
    % \hspace{4\textwidth} % Space between the two main figures
\end{figure}

In~\method, we assign each prompt an informativeness value, which the creator will use as the weight to sample from the seed prompts for prompt synthesis. In $\S$~\ref{sec:ab-metric}, we have shown that traditional methods like reward mean and reward variance are less effective as our advantage-based informativeness proxy. The intuition is simple: advantage/regret-based proxy aligns better with the preference optimization objective. We here further illustrate that they are statistically different from other choices:\vspace{-6pt}
\begin{itemize}
    \item Figure~\ref{fig:metric-pdf}: The distribution of informativeness values shows that reward variance is heavily concentrated at lower values, reward mean is more uniformly scattered, and reward advantage achieves a better balance, providing a broader yet also focused sampling range.\vspace{-3pt}
    \item Figure~\ref{fig:metric-corr}: The \emph{weak correlation} between reward variance and reward advantage shows that variance \emph{cannot} serve as a substitute for advantage as a proxy for informativeness.
\end{itemize}
\vspace{-6pt}
We have discussed the contrastive curriculum hypothesis in $\S$~\ref{sec:int} to support using reward advantage in the sense that the induced samples tend to decrease the loss the most in the contrastive optimization. Furthermore, assuming the optimization algorithm can converge to the \emph{more optimal} responses, neither reward mean nor variance directly capture the learning potential of such responses -- one may easily construct cases with identical variance yet differ much in reward range -- thus variance fails to distinguish such scenarios. By contrast, reward advantage estimate inherently captures the relative improvement towards better response, and is sensitive to differences in reward range; variants of advantage estimate are commonly used in literature, and we discuss underlying principles in $\S$~\ref{app:theory}.

% specifically, \emph{max - min} mimics the worst case, while \emph{max - mean} is more akin to the Bayesian view.

% By contrast, reward advantage inherently captures the relative improvement toward the optimal response, making it sensitive to such differences in reward range. Specifically, max-min provides a worst-case guarantee by considering the full reward span, while max-mean emphasizes the potential of the more optimal response by focusing on deviations from the average.

==> appp/app-downtream.tex <==
\section{Additional Experimental Results for the Main Paper}\label{app:downstream}


In general,~\method~maintains the accuracy on downstream tasks and is robust on those reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to the training sources for such reward models.
\input{tables/tab-ab-downstream}
\vspace{-8pt}

\input{tables/tab-ab-rm-app}

% \begin{table}[H]
% \centering

% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Llama-3.2-3B-instruct}}} \\ \cmidrule(l){2-7}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}



% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%)      & \textbf{avg. score}   & $1^{\text{st}}$ turn  & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

% $\vtheta_0$: SFT                & 9.7  & 7.24 & 7.60 & 6.88 & 27.15 & 29.94 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 11.4  &7.28  & 7.67 & 6.88 & 28.32 & 32.17 \\


% \rowcolor{green!10} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \textbf{13.0} & \textbf{7.37} & \textbf{7.71} & \textbf{7.03} & \textbf{29.54}  & \textbf{33.68} \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{}  & \tgray{} & \tgray{} & \tgray{} & \tgray{\textbf{}}  & \tgray{\textbf{}}  \\



% \bottomrule

% \end{tabular}%
% }
% \caption{\textbf{Results with \text{Llama} models.}.}
% \label{tab:main-10k-llama}
% \end{table}
% \vspace{-10pt}


==> appp/app-lit-bilevel.tex <==
% \newpage
\section{Extended Literature Review in Bi-Level RLHF}\label{app:lit-bilevel}
% \vspace{-4pt}

Bi-level optimization refers to optimization problems where the cost function is defined \textit{w.r.t.} the optimal solution to another optimization problem~\citep{roger-class}. There is a recent line of works applying bi-level optimization to RLHF. While they all rely on a fixed dataset of prompts, \method~propose to dynamically update the prompt set, as in $\S$~\ref{sec:intro}. We present a detailed comparison of~\method~with~\cite{bilevel-sail,bilevel-shen,bilevel-sta-rlhf}. We  sincerely thank the anonymous reviewer for the kind  references, and welcome suggestions for any other works we may have missed.
% While those works are orthogonal to~\method, We  thank the anonymous reviewer for the kind  references, which may help address the potential distributional mismatch issues as the policy models become more powerful.

\cite{bilevel-sail} formulate iterative online RLHF as a bi-level optimization problem, where the upper-level represents the reward learning, and the lower-level represents the policy optimization. Leveraging reward re-parameterization tricks in~\cite{dpo}, \cite{bilevel-sail} reduces the problem to a single-level objective with regard to the policy. The differences of this work and our work lie in the prompt distribution and preference oracle: (i) \method~features by \textbf{dynamic prompt set generation for Open-Ended RLHF}, whereas~\citep{bilevel-sail} remains using a static prompt set; (ii) we assume the existence of the preference oracle (as discussed in $\S$~\ref{sec:exp}), while~\cite{bilevel-sail} consider online training of reward models and ablate on self-rewarding by the current LLM policy. Our usage of a pre-trained reward model follows from industrial practices~\citep{team-1,gemma2}, which is also commonly used by prior works in academia~\citep{simpo,self-play-gu}. 
% We recognize the online training of reward models (see also~\citep{rlhf-workflow}) as an orthogonal/complementary direction to the current settings of~\method~(our setting is \textbf{agnostic to the preference structure}), and encourage future works and collaborations towards it, as mentioned in $\S$~\ref{sec:conclusion}.

\cite{bilevel-sta-rlhf} provide an interesting exploration on formulating RLHF as a leader-follower game, where the language model (LM) policy is the leader and the reward model (RM) policy is the follower, and the solution is \textbf{Stackelberg equilibrium}~\citep{stackelberg,game-mbrl}, where the \emph{leader does not likewise best respond to the follower's strategy}. Here, following the curriculum RL literature~\citep{paired,accel}, we seek the \textbf{Nash equilibrium}~\citep{nash} between the creator for prompt generation and the solver for response generation. Nevertheless, the LM-RM iterative optimization may be added on top of~\method's~framework, and we look forward to future works exploring the leader-follower re-formulation of~\method.

\cite{bilevel-shen} present a rigorous theoretical work (though it does not directly involve practical post-training of large language models). The authors propose to reduce the bi-level problem to a single-level problem with a penalty-based reformulation, and apply it in the setting of LM-RM optimization within a \textit{fixed} environment, whereas~\method~focuces on dynamic prompt generation and practically train large language models with extensive empirical experiments conducted. We believe it would be interesting to adapt similar first-order optimization techniques to solve Open-Ended RLHF.

In summary, existing bi-level RLHF works focus on online optimization of both the RM and the LM (as the response policy), all with \textbf{fixed} prompt/state distribution. \method~presents an orthogonal direction on \textbf{dynamic} prompt generation for Open-Ended RLHF, with an empirical algorithm which attains state-of-the-art performance with large language models on a variety of benchmarks. It is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and mitigate potential distributional mismatch problems as we evolves for more prompts. This direction may have not been widely adopted in real-world training of language models, due to concerns about practicality~\citep{team-1,team2,gemma2,nemotron}. We look forward to future works exploring \emph{efficient} variations unifying \method\ and existing bi-level RM-LM frameworks.





==> appp/app-lit.tex <==
% \newpage
\section{Extended Literature Review for Open-Ended Learning}\label{app:lit}

% \subsection{Extended Literature Review on Open-Endedness}

The design of our game-theoretic framework for language model post-training is inspired from many prior works in open-ended learning. The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that  can \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but broad enough to handle the diversity of complexity of future environments. In such curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively builds more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case (\ie most adversarial) environments.  In addition to distinctions discussed in~$\S$~\ref{sec:lit}, we here list several foundational works in this line, and encourage the LLM community to explore with more rigor and depth: \cite{schmidhuber1991possibility} presents an initial investigation into open-ended learning via self-supervised curiosity-driven exploration; \cite{poet} emphasize co-evolution of environments and agent policies by training a population of agents that adapt to and solve progressively complex challenges; \cite{paired} formally introduce the notion of Unsupervised Environment Design (UED), where a protagonist and antagonist agent pair simulates regret by competing in shared environments, driving the protagonist (the main learner) to adapt to increasingly challenging scenarios; \cite{plr} introduce Prioritized Level Replay (PLR), which uses a rolling buffer of high-regret levels to dynamically adjust the training curriculum, and selects levels with the higher learning potential; \cite{accel} further propose improvements by editing previously high-regret levels; \cite{open-endedness} present a formal definition for open-ended system with respect to \emph{novelty} and \emph{learnability}, that generalizes various systems, \eg AlphaGo~\citep{alphago}, AdA~\citep{team2021open}, etc.
% \vspace{-10pt}

% Our focus was on classical, seminal, and directly relevant works. We welcome suggestions for any other references we may have missed that can enhance our citations -- please feel free to reach out.


==> appp/app-loss.tex <==
\section{Plug-In Loss Functions Used in Main Results}~\label{app:loss}
\vspace{-.8cm}
\begin{table}[H]
\centering
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{With Reference Model}    \\ \midrule
DPO~\citep{dpo}  &  $\ell_{\beta}(\pi_{\vtheta})  = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_\vtheta};  {\pi_{\text{ref}}}}^{\rvx} \Bigr)\Bigr] \textcolor{lightgray}{:= - \log \left[\sigma\left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}- \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \right)\right]} $                   \\


SPPO~\citep{self-play-gu}  & $\ell_{\beta}(\pi_{\vtheta})  = - \log \left[\sigma\left( \left(\beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)} - \frac{1}{2}\right)^2 + \left( \beta \cdot \log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}+ \frac{1}{2}\right)^2  \right)\right]$  \\ 
\midrule
\multicolumn{2}{c}{Without Reference Model} \\ \midrule
SimPO~\citep{simpo} &  $ \ell_{\beta, \alpha}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\pi_{\theta}^{1/|\rvy|}};  1}^{\rvx} - \alpha \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \frac{\beta}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx) -  \frac{\beta}{|\rvy_{-}|} \log \pi_{\vtheta}(\rvy_{-} | \rvx) -\alpha \right)\right]} $                   \\
ORPO~\citep{orpo} &  $ \ell_{\lambda}(\pi_{\vtheta}) = -\log \Bigr[\sigma \Bigr(\lambda \cdot  \Delta_{\text{odds}_{\vtheta};  1}^{\rvx}  \Bigr)\Bigr] \textcolor{lightgray}{:= -\log \left[\sigma \left( \lambda \cdot \log \frac{\text{odds}_{\vtheta}(\rvy_{+} | \rvx)}{\text{odds}_{\vtheta}(\rvy_{-} | \rvx)}  \right)\right]} $\textcolor{lightgray}{, where $\text{odds}_{\vtheta}=\frac{\pi_\vtheta}{1 - \pi_{\vtheta}}$}                   \\
% ORPO~\citep{orpo} &   $\ell_{\lambda}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphslate{\dlogodds} \right)\right]$              \\ 
\bottomrule
\end{tabular}%
}
\caption{Direct preference alignment algorithms used in the main experiments. In parameter tuning, we include an additional negative log-likelihood loss for chosen responses (\ie~$\frac{\gamma}{|\rvy_{+}|} \log \pi_{\vtheta}(\rvy_{+} | \rvx)$).}
\label{tab:offline}
\end{table}

==> appp/app-prompt-examples.tex <==
\section{Examples on Prompts and Model Generations}\label{app:examples}
\vspace{-12pt}

% ------------------
\begin{figure}[H]
    % \centering
    % \begin{minipage}{0.39\textwidth}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
    \vspace{-4pt}
    \caption{The initial prompt distribution of AlpacaEval by \texttt{\small bart-large-mnli} with 0-shot classification, which is imbalanced. For the reward distribution, the category with lowest average reward has the highest  reward gap (\ie the default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
    % \end{minipage}
\end{figure}
% \vspace{-12pt}
% ------------------




% ------------------
% \begin{table}[H]
% \centering
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}r p{14cm}@{}}
% \toprule
% \rowcolor{lightgray!16}
% \multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small If a man smokes 1000 cigarettes a day, why is he getting healthier?} \\ \midrule
% \texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Elaborate on the seemingly paradoxical situation where an individual consumes 1000 cigarettes daily yet exhibits signs of improving health, delineating the factors that could underlie such an unexpected outcome.} \\
% \texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Discuss the conundrum of a person drinking a gallon of caffeinated coffee every hour but displaying unusually deep and restful sleep patterns, exploring possible explanations for this unusual phenomenon.} \\
% \texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Examine the paradox of an individual who ingests a gallon of caffeine-laden coffee hourly yet exhibits signs of profoundly tranquil slumber, delving into potential theories that could elucidate this atypical occurrence, and considering the role of genetic predispositions in such a scenario.} \\
% \texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Analyze the conundrum of a person consuming an entire gallon of heavily caffeinated coffee every single hour and yet demonstrating the ability to fall into a state of deep sleep, exploring plausible hypotheses that could illuminate this unusual event, including an assessment of how genetic factors might influence this ability, and include an evaluation of the impact of acquired tolerance to caffeine over time.} \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-4pt}
% % \caption{Examples of evolved prompts from AlpacaEval.}
% \label{tab:prompt-evol}
% \end{table}
% ------------------

\vspace{-10pt}

% ------------------
\begin{table}[H]
\centering
\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{@{}r p{12.6cm}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small Write me the code for a distributed transaction manager.\textbackslash nThink step by step and use pseudo code first.\textbackslash nThen, define interfaces for all involved actors and entities.\textbackslash nUse Rational Unified approach for this part.\textbackslash n\textbackslash nOnly then move on to the actual implementation, class-by-class, and method-by-method.\textbackslash nMake the code be implemented in C\# and follow SOLID principles.} \\ \midrule
\texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Craft a suite of syntax for a distributed transaction coordinator. Start with a sequential breakdown in pseudocode format. Following that, establish the protocols for communication and interaction amongst the various participants and components, incorporating the Rational Unified Process methodology.\textbackslash n\textbackslash nProceed thereafter to the concrete creation, detailing each class and function. Ensure that the final C\# code adheres to the precepts of SOLID and is annotated for clarification and maintainability purposes.} \\
\texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Devise a comprehensive set of directives and structures for a distributed transaction coordinator architecture. Initiate by formulating a step-by-step algorithmic decomposition in pseudocode. Subsequently, delineate the frameworks for dialog and cooperation between the numerous entities and elements, utilizing the tenets of the Rational Unified Process methodology.\textbackslash n\textbackslash nContinue to the actual generation of the code, meticulously detailing every class and corresponding method. Guarantee that the culminating C\# code is in strict compliance with SOLID principles and is supplemented with descriptive commentary to enhance future clarity and upkeep, while also validating the code against a set of unit tests to ensure robust functionality.} \\
\texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Commence by constructing an algorithm in pseudocode that meticulously breaks down the sequential stages for a distributed transaction coordinator system. Progress by outlining the communication protocols and collaborative mechanisms among the myriad components, adhering to the Rational Unified Process approach.\textbackslash n\textbackslash nAdvance to crafting the code in C\#, ensuring each class and method is elaborated with precision, aligning with SOLID design principles. Integrate thorough comments for heightened maintainability and conduct comprehensive unit testing for assured operational integrity.} \\
\texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Design a detailed flowchart that represents the intricate steps of an orchestration engine for managing microservices in a cloud-native environment. Begin by detailing the service discovery, load balancing, and fault tolerance strategies, while incorporating the DevOps philosophy.\textbackslash n\textbackslash nProceed by developing the implementation in Java, focusing on clean, modular code following object-oriented programming best practices. Accompany your code with clear documentation for easy understanding and perform rigorous integration testing to guarantee robustness.} \\ \bottomrule
\end{tabular}%
}
% \vspace{-4pt}
\caption{Examples of evolved prompts from AlpacaEval. We suggest practitioners to include generated responses with oracle rewards and self-critique in the context for better prompt evolving, which is helpful for mitigating the effect of potential self-consuming loops in synthetic data training.}
\label{tab:prompt-evol-2}
\end{table}
% ------------------






\newpage

\hspace{0pt}
\vfill

\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} \texttt{\small When a number is divided by 10, the remainder is 4. What is the remainder when twice the number is divided by 4?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
* "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
* Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
* (20*k + 8) divided by 4 is (20*k)/4 + 8/4 = 5*k + 2\newline
4. Find the remainder:\newline
* Since 5*k is a multiple of 4, the remainder when twice the number is divided by 4 is 2.\newline
Let me know if you'd like to try another example!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}} 
\texttt{\small Here's how to solve this problem:\newline
1. Understand the first statement:\newline
- "When a number is divided by 10, the remainder is 4" means the number can be represented as 10*k + 4, where k is an integer.\newline
2. Double the number:\newline
- Twice the number is 2*(10*k + 4) = 20*k + 8\newline
3. Divide by 4:\newline
- When (20*k + 8) is divided by 4, the 20*k term is perfectly divisible by 4.\newline
- The remainder will be the same as the remainder when 8 is divided by 4, which is 0.\newline
Therefore, the remainder when twice the number is divided by 4 is 0.}
\end{tabular} \\ \midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} \texttt{\small What about when twice the number is divided by 5?}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 is (20*k)/5 + 8/5 = 4*k + 1.6\newline
3. Find the remainder: Since 4*k is a multiple of 5, the remainder when twice the number is divided by 5 is 1.\newline
Let me know if you have any more number theory puzzles!}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small Here's how to solve that:\newline
1. \text{Twice the number:} We know twice the number is 20*k + 8 (from the previous steps).\newline
2. \text{Divide by 5:} \newline
\ \ \ * 20*k is divisible by 5.\newline
\ \ \ * 8 divided by 5 leaves a remainder of 3.\newline
Therefore, the remainder when twice the number is divided by 5 is 3.}
\end{tabular} \\ 

\midrule

\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's response is incorrect. The assistant incorrectly calculated the remainder when twice the number is divided by 5. The assistant calculated the decimal part of the division operation, not the remainder. The correct calculation should be (20n + 8) \% 5 = (20n \% 5) + (8 \% 5) = 0 + 3 = 3. Therefore, the remainder when twice the number is divided by 5 is 3, not 1 as the assistant stated.\newline
\newline
The corrected response would be:\newline
1. We know: Twice the number is 20*k + 8 (from the previous calculation).\newline
2. Divide by 5: (20*k + 8) divided by 5 gives us a remainder of (20*k \% 5) + (8 \% 5) = 0 + 3 = 3.\newline
3. Find the remainder: The remainder when twice the number is divided by 5 is 3.\newline
\newline
Rating: [[3]], "score": 3, "turn": 2, "tstamp": 1722737011.7768948}
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}
\texttt{\small The assistant's answer is correct and matches the reference answer. The assistant correctly explains that twice the number is 20*k + 8 and that when this is divided by 5, the remainder is 3. The assistant's explanation is clear and easy to understand, making it helpful for the user. There are no mistakes to correct.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846518.5543818}

\end{tabular} \\ 

% \sbt{Judgment for gemma-2-9b-it-dpo} & \sbt{Judgment for gemma-2-9b-it-dpo-eva} \\ 

\bottomrule
\end{tabular}%
}
\caption{Comparison of model generations on examples from MT-Bench.}
\label{tab:gen-0}
\end{table}


\vfill
\hspace{0pt}




% ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{appp/tab-gen-2}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
\hspace{0pt}
\vfill
\input{appp/tab-gen-3}
\vfill
\hspace{0pt}
% % ------------------

% ------------------
% \newpage
\hspace{0pt}
\vfill
\input{appp/tab-gen-1}
\vfill
\hspace{0pt}
% ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{appp/tab-gen-4}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
\input{appp/tab-gen-5}
% \vfill
% \hspace{0pt}
% % ------------------

% % ------------------
% \newpage
% \hspace{0pt}
% \vfill
% \input{appp/tab-gen-6}
% \vfill
% \hspace{0pt}
% % ------------------

==> appp/app-prompt-vis.tex <==
% \section{Prompt Visualization}\label{app:prompt-vis}

% \section{Issues of Fixed Prompt Training Distributions}\label{app:prompts}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
%     \caption{The initial prompt distribution of AlpacaEval (openly accessible on HuggingFace) obtained from zero-shot classification with \texttt{bart-large-mnli}, which is imbalanced. Additionally, looking at the reward distribution, the category with lowest average reward has the highest average reward gap (\ie our default informativeness proxy), implying the potential to improve.}
%     \label{fig:app-prompts}
% \end{figure}


==> appp/app-rebuttal.tex <==
\newpage
\section*{Rebuttal to Reviewer ac2P}

\paragraph{Summary.} We sincerely thank the reviewer for the appreciation of~\method~and the constructive feedback. We have made every effort to throughly address the concerns. Specifically, we have:
\begin{itemize}
    \item  added experiments on  implementing \textbf{different evolving methods} and discussed relevant strengths and weaknesses in $\S$~\ref{app:exp-evol};
    \item added \textbf{visualization on the learning curriculum} in $\S$~\ref{app:curr};
    \item provided detailed discussion on \textbf{scaling up}~\method~with million-level data on larger-scale seed sets and/or inference-time scaling for synthesizing prompts.
\end{itemize}

%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 (Choice of the Evolving Method)}:  Could you explain more about the particular choice of evolution algorithm used in your implementation of eva and different potential strengths and weaknesses related to this choice?}
\end{tcolorbox}

\textbf{TL;DR:} We use EvolInstruct~\citep{wizardlm} as it is among the most easy-to-implement methods. We added new experiments w/ other methods, including SelfInstruct~\citep{self-instruct}, EvolQuality and EvolComplexity~\citep{deita}, and show that~\method~remains to be effective in $\S$~\ref{app:exp-evol}.

\textbf{Answer:}
As an addition to Table~\ref{tab:main-10k}, we have experimented with three different \texttt{\small evolve}(\textperiodcentered) methods:
\begin{itemize}
    \item \textbf{SelfInstruct}~\citep{self-instruct}: Given seed prompts, variations are created based on criteria such as verb diversity and style blending (mixing interrogative and imperative styles). Unlike EvolInstruct~\citep{wizardlm}, which generates prompt variations sequentially, this approach generates independently. We follow the one-shot implementation in  \href{https://github.com/argilla-io/distilabel/blob/844165f25c1674076a8286d54cfe96d52c33a24e/src/distilabel/steps/tasks/self_instruct.py#L106}{\texttt{\small self\_instruct.py}} of \texttt{\small distilabel==1.4.1} and modified the instruction on conciseness so that newly generated prompts have similar lengths compared to the seed prompts.
    \item \textbf{EvolQuality} and \textbf{EvolComplexity}~\citep{deita}: The two methods use the same evolutionary approach (\ie sequential generation), but with slightly different meta-instructions for prompt generation, where EvolQuality asks to improve the quality (\ie helpfulness, relevance, etc) of the seed prompt and EvolComplexity asks to improve the complexity (\ie increased reasoning steps, etc) of the seed prompt. We follow the implementation in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_quality/utils.py}{\texttt{\small evol\_quality/utils.py}} and \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/evol_complexity/utils.py}{\texttt{\small evol\_complexity/utils.py}} of \texttt{\small distilabel==1.4.1}.
\end{itemize}


% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolInstruct}) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolQuality}) & \text{58.7}  & 721 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small EvolComplexity}) & \textbf{60.6}  & 749 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (\texttt{\small evolve}(\textperiodcentered) = \texttt{\small SelfInstruct}) & \text{57.2}  & 725 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using different evolving methods.}
\label{tab:evol-10k-}
\end{table}
\vspace{-10pt}
% ----------

\paragraph{\method~is effective under different evolving methods.} As shown in Table~\ref{tab:evol-10k}, our method brings strong performance gain without training with additional human prompts. Among the experimented methods, we find EvolComplexity shows better results. 

We believe the main strength of such method is its \textbf{simplicity}. Viewing the evolving process as $\rvx' \gets p_{\vtheta}(\cdot \mid  \rvx, \texttt{\small meta\_prompt})$, one can easily tune the meta prompt in natural language for improved performance. However, such simplicity comes at a price: (i) the main weakness is that the default method does not take \textbf{environmental feedback} into account (\eg rewards received, verbal critique on responses, etc) and relies on the pre-defined meta prompt, thus the evolving may be less directional; we encourage practitioners to consider incorporating richer feedback during evolving (one way to formulate this is by generative optimization~\citep{textgrad,trace,trace-pre}); (ii) another weakness is that existing method is single-shot (\ie we evolve based on a single $\rvx$ each time), thus the \textbf{diversity} of the generation may be limited -- we anticipate future works improving this with multi-shot evolving by graph-based sampling or including diversity-related rewards in generation. In this regard, the evolving process can be viewed as $\{\rvx'\}_{i=1}^{N} \gets p_{\vtheta}(\cdot \mid  \{\rvx\}_{i=1}^{M}, \texttt{\small meta\_prompt}, \texttt{\small env\_feedback})$.
%---------------------------------

%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q2 \& Q3 (Empirical Evidence on Learning Progress and Curriculum)}:  Do you see empirical evidence of your intuition about learning progress discussed in section 3.4? It seems like some of these claims are directly testable. Could you visualize the curriculum learned in your experiments with eva? It would be very nice to get an intuition for why performance improves and what the heuristic prioritizes over time.}
\end{tcolorbox}

\textbf{Answer:} We thank the reviewer for the constructive suggestions on empirically validating the intuition. We have revised the manuscript with additional visualization on potential curriculum learned in $\S$~\ref{app:curr}. In general, we observe the creator prioritizes learning in math and coding, which brings gradual improvement on benchmark performance on relevant categories over iterations. We have attached the bar plot and radar figure here for the reviewer's reference:

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist-}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma-}
    \end{minipage}
\end{figure}

%---------------------------------

We further evaluate the complexity and quality of the prompt distributions. As in Table~\ref{tab:prompt-quality-complexity-}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. 


\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity-}
\end{table}
\vspace{-10pt}
% ----------

Implementation notes: We sample 10K prompts per iteration, and use the below prompts modified from~\cite{deita} for the complexity and quality evaluation, with \texttt{\small gemini-1.5-flash} as the generative scorer:
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Rank the following questions according to their quality. Your evaluation should consider the following factors: Helpfulness, Relevance, Accuracy, Depth, Creativity, and Level of detail.
Score each response from 1 to 5: 1: Poor quality, 2: Below average, 3: Average, 4: Good, 5: Excellent.
\end{minted}
\begin{minted}[fontsize=\tiny, breaklines, frame=single]{text}
Ranking the following questions according to their difficulty and complexity. Use a fixed scoring system: 1: Very simple, 2: Simple, 3: Moderate,  4: Difficult, 5: Very difficult
\end{minted}




%---------------------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q4 (Scaling)}: When discussing future directions, the authors write further scaling up w/ million-level data. Can you clarify what this means? Seems like some important context is missing?}
\end{tcolorbox}

\textbf{TL;DR:} We consider (i) applying~\method~when the seed set contains million-level or more prompts; or (ii) using~\method~to robustly generate million-level or more prompts when the seed set is limited.

\textbf{Answer:} (i) The current paper uses the UltraFeedback~\citep{ultrafeedback} as the seed prompt set, which is a ten-thousands level dataset; in training practically useful large language models~\citep{gpt,team2,rest_em}, the seed prompt set is usually much larger than such a level. We believe it is an interesting direction to explore the data scaling properties of~\method~on larger seed prompt sets, in combination with our on-policy variants. (ii) On the other hand, when the seed prompt set contains only limited data (this issue is particularly concerning in hard reasoning tasks like math~\citep{leandojo}), can we still follow the data generating curriculum and synthesize million-level prompts/problems to help training, and how to robustly verify the generated prompts/problems? Beyond training-time scaling, there is also a recent trend in inference-time scaling~\citep{snell2024scaling}, however these works only consider scaling in the $\calY$ space, not the $\calX$ or the joint $(\calX, \calY)$ space. We believe synthetically scaling up the joint $(\calX, \calY)$ space to a much more larger magnitude under~\method's game-theoretic design presents a new direction worth investigating. 
%---------------------------------

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textbf{Final remarks.} We thank the reviewer once again for spending time providing constructive feedback that helps improve~\method. Please let us know if there is any other concerns or questions, and we are more than grateful to have the opportunity to learn from and discuss with you. 
\end{tcolorbox}

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.




\newpage
\section*{Rebuttal to Reviewer zxTK}

\paragraph{Summary.} We sincerely thank the reviewer for all the constructive feedback helping improving the~\method~method. In response, we have provided:
\begin{itemize}
    \item \textbf{experiments on more iterations} in $\S$~\ref{app:exp-iter};
    \item \textbf{extended discussions on the regret objective and the proxy} in $\S$~\ref{app:theory};
    \item \textbf{evidence on distinction of advantage-based metrics and variance-based ones} in $\S$~\ref{app:metric};
    \item \textbf{revised illustration of the method} in~\secref{sec:method}, and \textbf{evidence on evolving prompt distributions} (to answer it cannot ``cheat by selecting easier prompts'')  in~\secref{app:curr}.
\end{itemize}

% We believe the additional discussions and rebuttals provided have sufficiently addressed the weaknesses and questions raised by the reviewer. Please let us know if there is any additional revision needed and we would be grateful to incorporate.

We appreciate the chance to address the reviewer’s comments and have made every effort to thoroughly address the concerns and revise our manuscript accordingly. We hope that these revisions meet the reviewer’s expectations and would be grateful if the reviewer could kindly consider revise the score. 
% If there are any further suggestions, please do not hesitate to let us know.

% We have made every effort to thoroughly address your concerns and incorporate detailed insights based on your suggestions, both in our responses (above) and the revised draft.

% ---------------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W1 (Running for More Iterations)}: The number of iterations in the main results is 2, with only one EVA step in each experiment, which is a little different from what the demonstration in Figure 3 shows. If the~\method~step is performed multiple times, would the results be better or worse? What is performance like when you access all data in UltraFeedback?  }
\end{tcolorbox}

\textbf{TL;DR:} We added experimental result on running more iterations with more data, and~\method~remains to be effective. We have added $\S$~\ref{app:exp-iter} in the manuscript to incorporate the reviewer's suggestion.

\textbf{Rebuttal:} As an addition to $\S$~\ref{sec:ab-cont}, we have experimented with the following settings:
\begin{itemize}
    \item 10K prompts per iteration with 3 iterations.
    \item 20K prompts per iteration with 3 iterations (\ie all seed prompts are used).
    \item 60K prompts per iteration with 2 iterations (\ie all seed prompts are used).
\end{itemize}

Due to time constraints, we did not perform an extensive hyper-parameter search; however, we believe the results presented below sufficiently demonstrate the performance gains achieved by~\method.

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (10k)     & 51.6  & 651  \\

$\vtheta_{1 \rightarrow 2}$: DPO (10k)     & 59.8  &   718\\

$\vtheta_{2 \rightarrow 3}$: DPO (10k)   & 61.2  & 802  \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.0}  & 787  \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (10k) & \text{62.2}  & 774  \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 10k prompts per iteration.}
\label{tab:ab-10k-}
\end{table}
\vspace{-10pt}
% ----------


% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (20k)     & 53.2  & 625 \\

$\vtheta_{1 \rightarrow 2}$: DPO (20k)     & 47.0  & 601  \\

$\vtheta_{2 \rightarrow 3}$: DPO (20k)   & 46.8  & 564 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{59.5}  & 826 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{2}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{60.0} & 817 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{2} \rightarrow \Tilde{3}}$: \quad + \texttt{\textbf{eva}} (20k) & \text{61.4} & 791 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 20k prompts per iteration.}
\label{tab:ab-20k-}
\end{table}
\vspace{-10pt}
% ----------

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO (60k)    & 58.9  & 717 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} (60k) & \text{59.6}  & 725 \\ 

\rowcolor{green!10} 
$\vtheta_{\Tilde{1} \rightarrow \Tilde{1}'}$: \hspace{-6pt} \quad + \texttt{\textbf{eva}} (60k) & \text{61.9}  & 792 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of using 60k prompts per iteration.}
\label{tab:ab-60k-}
\end{table}
\vspace{-10pt}
% ----------


\paragraph{\method~can bring robust gains with multiple iterations.} As shown in Table~\ref{tab:ab-10k-},~\ref{tab:ab-20k-}, and~\ref{tab:ab-60k-}, our method presents persistent performance gain over iterations, and concretely surpasses the performance by default DPO training with true human prompts. 


However, there exist diminishing marginal gains in iterative off-policy training. We ground~\method~in the iterative (off-policy) preference alignment paradigm due to its efficiency and ease of integration. However, such paradigms inherently face diminishing returns, where performance gains decrease with successive iterations, as previously observed in~\citep{self-play-gu,8fold,self-reward,cont-primary-bias}. While the generative data schedule in~\method~mitigates these challenges and extends beyond default training with human prompts (see also $\S$\ref{sec:ab-cont}), the gains can weaken over iterations. We summarize potential reasons as: (i) the \textbf{off-policy signal decay} -- as the number of examples increases, signals from the off-policy data become weaker due to distributional shift; (ii) the \textbf{loss of plasticity}, where the agent's ability to learn good policies decreases in continuing training with more iterations~\citep{cont-primary-bias}; (iii) the \textbf{ability of the solver} -- as we evolve more harder prompts, it is harder for the solver to produce preferred response (thus more explicit reasoning techniques may be needed); (iv) the \textbf{ability of the reward model} to correctly provide reward signals to responses and thus informativeness signals to prompts, as there may exists distributional mismatch.

Thus, we envision future work to build on~\method~by: (i) exploring its integration with \textbf{on-policy RLHF} (\eg instead of evolving prompts in iterations, one may evolve in batches); (ii) \textbf{enhancing solver capabilities}, such as sampling more responses during inference or leveraging meta-instructions to guide deeper reasoning; (iii) online training of RM to co-evolve with the creator and the solver. 

\paragraph{Bonus experiments on adding rewriter in the solver step.} This is beyond the current paper, and we present the basic idea here for practitioners to build upon~\method. The motivation comes from the hypotheses derived from $\S$~\ref{app:exp-iter}: as the prompts gets harder by evolving, there may be greater demands on the solver’s capabilities \emph{compared to earlier iterations}. As such, the solver may not be naively treated the same. One may address this by either inference-time scaling on responses or introducing meta-instructions to explicitly enhance the solver’s reasoning.

We hereby design a proof-of-concept experiment \emph{w.r.t} the latter by adding \textbf{rewriter} in \method's solver step. Previously, as in Algo.~\ref{alg:i-eva} and  $\S$~\ref{sec:solver-step}, for each prompt $\rvx$, we generate multiple responses, and choose the best as $\rvy_{+}$ and the worst as $\rvy_{-}$ for preference optimization. Now, we add one more rewriting step that attempts to enhance $\rvy_{+}$ to be $\rvy'_{+}$, by applying a rewriting instruction~\citep{deita} that asks the solver to alter $\rvy_{+}$ with imporved helpfulness, relevance, reasoning depths, creativity and details while keeping the similar length. We then train with $(\rvx, \rvy'_{+}, \rvy_{-})$ for preference optimization. Table~\ref{tab:rewriter-10k} shows that adding the rewriter yields concrete performance gains over the default  method, while keeping training budgets and only slightly increasing response generation cost.
% \vspace{-3pt}

% ----------
\begin{table}[H]
\centering

\resizebox{0.42\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{2}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-3}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{2}{c}{\textbf{Arena-Hard}} \\ \cmidrule(l){2-3}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. len}     \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 544 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 651 \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{60.1}  & 733 \\ 

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad + \texttt{\textbf{eva}} with \texttt{\textbf{rewriter}} & \textbf{61.9}  & 741 \\ 

\bottomrule

\end{tabular}%
}
\caption{Results of adding \textbf{\texttt{\small rewriter}} in the \textbf{\texttt{\small solver}} step.}
\label{tab:rewriter-10k-}
\end{table}
\vspace{-10pt}
% ----------
% ---------------------

% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W2 (Connection in Minimax Regret and The Algorithm)}: The connection between the minimax regret objective and the algorithm is a somehow vague. The regret concerns the performance gap with the optimal policy. It's not reflected by the informativeness proxy.}
\end{tcolorbox}

\textbf{TL;DR:} We have added $\S$~\ref{app:theory} to address the reviewer's concern in detail. (i) In the current algorithm, the solver explicitly minimizes the regret by plug-in preference optimization algorithms (\eg DPO), while the creator implicitly maximizes the regret by first finding high-regret prompts and generate variations as new prompt distributions for training. (ii) The informativeness proxy is an advantage-based estimate of the regret; similar variants have been used in prior literature like~\cite{plr,accel}; as the policy optimizes, the proxy can approximate the true regret better. 

\textbf{Rebuttal:} For the rebuttal to be self-contained, we  extract contents from~\secref{app:theory-3} here. We feel~\secref{app:theory} offers a better overview -- it would be great if you could take some time to review~\secref{app:theory} when feasible.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}

The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret-}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.

\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optmizes, the proxy should approximate the regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


% At a high-level, we first use the alternating optimization by minimax game to replace the joint optimization in Eq.~\ref{eq:rlhf-joint-}; secondly, we use regret as the objective for the game, where the creator seeks to maximize and the solver seeks to minimize. For the creator, the regret is approximated by the informativeness proxy through sampling from the stochastic policy and measuring the gap between the maximal and the minimal reward received. For the solver, the minimization is practically achieved by the plug-in contrastive preference optimization (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model). Please check $\S$~\ref{app:theory} for our detailed writeup. (Note: without access to the optimal policy, we \emph{need} to approximate the regret in practice; classical works have trained two players~\citep{paired}, while our approach is more simple and efficient, avoids training instability and  empirically brings strong performance gain).
% ---------------------

% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 (Advantage v.s. Variance)}: The informativeness proxy seems to be similar to the variance of the rewards because they all concern the diversity of the generated responses. However, in lines 393-395, the results show using variance leads to poor performance. How to interpret this?}
\end{tcolorbox}

\textbf{Rebuttal:}  To explain, (i) variance does not directly capture the \textbf{learning potential} in preference optimization, while advantage-based informativeness proxy is better aligned to the learning objective; (iii) we \textbf{empirically show} that variance and advantage are only \textbf{weakly correlated} thus will likely result in different sampling. We have added $\S$~\ref{app:metric} to incorporate the reviewer's suggestion. 

% \textbf{Rebuttal:} 
\vspace{-12pt}
\begin{figure}[H]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-pdf.pdf}
        % \vspace{+0.00001pt}
        \caption{The probability density distributions of  informativeness metrics in Table~\ref{tab:ab-metric} -- they show different patterns.}
        \label{fig:metric-pdf-}
    \end{minipage}
    \hspace{0.02\textwidth}
    % \hfill
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/var-gap-corr.pdf}
        % \vspace{+0.00001pt}
        \caption{The correlation plot for reward advantage (ours) and reward variance -- they are only \emph{weakly} correlated.}
        \label{fig:metric-corr-}
    \end{minipage}
    % \hspace{4\textwidth} % Space between the two main figures
\end{figure}
\vspace{-12pt}

In~\method, we assign each prompt an informativeness value, which the creator will use as the weight to sample from the seed prompts for prompt synthesis. In $\S$~\ref{sec:ab-metric}, we have shown that traditional methods like reward mean and reward variance are less effective as our advantage-based informativeness proxy. The intuition is simple: advantage/regret-based proxy aligns better with the preference optimization objective. We here further illustrate that they are statistically different from other choices:\vspace{-6pt}
\begin{itemize}
    \item Figure~\ref{fig:metric-pdf-}: The distribution of informativeness values shows that reward variance is heavily concentrated at lower values, reward mean is more uniformly scattered, and reward advantage achieves a better balance, providing a broader yet also focused sampling range.\vspace{-3pt}
    \item Figure~\ref{fig:metric-corr-}: The \emph{weak correlation} between reward variance and reward advantage shows that variance \emph{cannot} serve as a substitute for advantage as a proxy for informativeness.
\end{itemize}
\vspace{-6pt}
We have discussed the contrastive curriculum hypothesis in $\S$~\ref{sec:int} to support using reward advantage in the sense that the induced samples tend to decrease the loss the most in the contrastive optimization. Furthermore, assuming the optimization algorithm can converge to the \emph{more optimal} responses, neither reward mean nor variance directly capture the learning potential of such responses -- one may easily construct cases with identical variance yet differ much in reward range  -- thus variance fails to distinguish such scenarios. By contrast, reward advantage estimate inherently captures the relative improvement towards better response, and is sensitive to differences in reward range; variants of advantage estimate are commonly used in literature, and we discuss underlying principles in $\S$~\ref{app:theory}.
% ---------------------




% ---------------------
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q2 (Open-Ended Objective)}: In Line 1399 (authors' note: should be around Line 880 - 886 in the main OpenReview PDF), why is this objective ideal? Optimizing the prompt distribution seems like cheating by selecting easier prompts for a higher reward.}
\end{tcolorbox}

\textbf{TL;DR:} The whole design is to avoid cheating (\textbf{in principle}: adding KL regularization to guide the creator policy towards the open-ended reference; \textbf{in practice}: using the creator to generate new prompts to maximize the solver's regret). We also present further \textbf{empirical evidence} showing~\method~helps create more complex prompts.

\textbf{Answer:} To start with, we quote the conceptual objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

Another way to express the principled objective (with refined coefficients) is:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver $\sim$ ``regret minimization''}} }\ \textcolor{cgreen}{\Bigr]} 
-  \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\beta_2 \cdot \sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator $\sim$ ``regret maximization'' (implicit)}}}. \nonumber 
$}

\textbf{Conceptually}, the cheating will happen when the reference distribution is narrow or wrongly defined. It is important that in our case $p_{\text{ref}}(\rvx)$ represents an \emph{underspecified}, potentially intractable probability distribution over possible tasks (instantiated \emph{via} prompts) in the wild, as an  \textbf{open-ended reference} that covers the full diversity and complexity of tasks agents may encounter, \emph{not} the initial static prompt set $\calD$. The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts, while being close to the SFT policy $\pi_{\text{SFT}}(\rvy | \rvx)$. In brief, the definition of the conceptual $p_{\text{ref}}(\rvx)$ and the \textbf{regularization} avoids collapsing to distributions with easier prompts.

\textbf{Practically}, we do not directly optimize this principle, rather we design a creator-solver game to implicitly achieve this by iteratively creating a sequence of informative prompts. It is important that we use \emph{regret} as the objective and its approximation by the estimate of the \emph{optimal reward advantage}, which avoids selecting prompts that are too easy or too hard by design as well. See also $\S$~\ref{sec:int} on auto-curricula and learning potential for prompt selection, and $\S$~\ref{app:theory} for more connection between the objective and the algorithm.


For \textbf{empirical evidence}, as in Table~\ref{tab:prompt-quality-complexity---}, there is a gradual improvement of prompt complexity and quality over iterations with~\method. We also observe the creator auto-prioritizes learning in problems like math and coding in Fig.~\ref{fig:dist---}, which are initially hard for it as in Fig.~\ref{fig:radar-gemma---}. Thus the creator also practically does not select easier prompts in the~\method~game. Details can be found in~\secref{app:curr}.


\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity---}
\end{table}
\vspace{-10pt}
% ----------

In addition, the whole literature of curriculum RL, open-ended learning and so on are about designing the right metric for the agents to learn increasingly complex and general capabilities, and we summarize at~\secref{app:lit} for the reviewer's reference.


\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist---}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma---}
    \end{minipage}
\end{figure}





% ---------------------


% ---------------------
\begin{tcolorbox}[myquote]
\textbf{Remarks.} We thank Reviewer \texttt{zxTK} for the constructive feedback. We have made careful efforts to address all the weaknesses and questions raised. We would be grateful if the reviewer may kindly consider again the rating for~\method, also with regard to its  strong performance gain, the easy-to-implement method, as well as the new principle and the tractable algorithm. If there are additional concerns, we are more than happy to discuss and revise our manuscript further.
\end{tcolorbox}
% ---------------------

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.




\newpage
\section*{Rebuttal to Reviewer i9kx}

\paragraph{Summary.} We thank the reviewer for the thoughtful and detailed feedback. In response, we have:
\begin{itemize}
    \item provided a point-by-point rebuttal \textbf{fully addressing every suggested weakness/question};
    \item \textbf{improved definitions} for Algorithm 1, the regret and the informativeness proxy in~\secref{sec:method};
    \item \textbf{added a detailed review} on bi-level RLHF and open-ended learning in $\S$~\ref{app:lit-bilevel} and $\S$~\ref{app:lit};
    \item \textbf{added a full section} to illustrate method, from the principle to the asymmetric game setting, then to the regret minimization by the solver and maximization by the creator in $\S$~\ref{app:theory};
    \item \textbf{added new experiments} on empirical gains and prompt evaluation of~\method~in $\S$~\ref{app:ablation} and $\S$~\ref{app:curr}.
\end{itemize}

% As a side note, we sincerely appreciate the reviewer’s thoughtful suggestions,  and note that their perspective may align with a more theory-first approach, akin to the references listed ([\href{https://openreview.net/pdf?id=Xb3IXEBYuw}{1}], [\href{https://openreview.net/forum?id=02kZwCo0C3}{2}], and [\href{https://openreview.net/forum?id=Jcn8pxwRa9}{3}]), which we very much value and find inspiring. The current~\method~framework, however, takes a complementary \textbf{method-first} approach, prioritizing methodological simplicity and empirical performance over rigid theoretical justifications. This design choice is intentional: we aim to offer a \textbf{new, simple, easy-to-implement training paradigm} that can be easily adopted, extended, and elaborated upon by the broader community, both in academia and industry.

% To achieve this, we have intentionally included approximations to make the framework \textbf{practical and easy to use}; we consider the main concerns of the reviewer may also come from such approximations made -- in a way that the current package is not intended to be perfect in theory. We wish to clarify that our primary goal is to prioritize the practical method itself, similar to prior methodological works (\eg CoT~\citep{cot}, ReST~\citep{rest}, etc). The theoretical bits we provide serve to establish a \textbf{high-level and fundamental principle} that inspires further practical and theoretical exploration, rather than being the restriction on the methodology.

% Additionally, we recognize the broader context in which this discussion takes place. It may be slightly sad to observe a gap between current RL/bandit theory research and the practical methods adopted in the real world. Many elegant theoretical ideas remain under-utilized due to the compromises required for theoretical rigidity, while industrial approaches often succeed with brute-force methods that prioritize empirical performance over theory. With \method, we aim to strike a balance between them, offering a conceptual framework that is both theoretically inspired and practically impactful.

% We hope we have sufficiently addressed the reviewer's concerns, and we warmly encourage the reviewer to also consider the \textbf{strong performance gains} with the \textbf{simple design} when judging~\method, and to evaluate the merit of a work (\textit{cf.,} \href{https://psc-g.github.io/posts/mentoring/reviewing/#conclusion}{ (Castro, 2021)}) \emph{w.r.t.} the practicality and how the community can easily build on top of it (\textit{cf.,} \href{https://d37ugbyn3rpeym.cloudfront.net/stripe-press/TAODSAE_zine_press.pdf}{(Hamming, 1986)}). We look forward to and would be very much grateful about any future suggestions to help us revise further, and we sincerely hope that the reviewer would consider update the rating for~\method, if the revision is satisfactory.

% We sincerely thank the reviewer once again for dedicating their valuable time to carefully reviewing our manuscript and for providing constructive feedback to improve~\method. We warmly welcome any future collaborative discussions and are more than happy to address any follow-up questions and to learn from the reviewer's insights.

To avoid repetition, we reorganize the questions and group related answers into a single response.

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q5 (Intuition on Open-Ended RLHF)}: Can you provide intuitions behind equation 7, on the KL divergence between the joint policy for both prompt and response? Is it even tractable to estimate or approximate this KL?}
\vspace{+4pt}
\newline
\textcolor{gray}{\textbf{W2 (Regret and KL)}: The optimization is over $\pi$ in Eq. 9 for solving the minimax regret. However, its not absolutely clear how the KL divergence plays a role here and how it is ensured that the response and prompt distributions are close to reference. Without that, the alignment problem is ill-defined. Please provide concrete justifications in theory and empirical results.}
\vspace{+4pt}
\newline
\textcolor{gray}{\textbf{W1 (Proxy Tractability)}: How is Eq. 10 tractable and being solved? Any heuristic of sampling and approximating should result in sub-optimality which is not clear where its accounted.}
\end{tcolorbox}

\textbf{TL;DR:} We have added $\S$~\ref{app:theory} to fully address related concerns. Regarding specific concerns:
\begin{itemize}
    \item \textbf{Q5 - Intuition.} The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to (i) generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts (note that $p_{\text{ref}}(\rvx)$ is the \emph{underspecified} open-ended reference, \emph{not} the initial static prompt set $\calD$), while (ii) being close to $\pi_{\text{SFT}}(\rvy | \rvx)$. We can reformulate the principle to Eq.~\ref{eq:rlhf-expand}.It is tractable to solve $\mathbb{D} _{\mathrm{KL}}\left[\pi _\theta(\mathbf{y} \mid \mathbf{x}) \| \pi _{\mathrm{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$ by existing plug-in preference optimization algorithms, yet we need to approximate $\mathbb{D} _{\mathrm{KL}}\left[\pi _\phi(\mathbf{x}) \| p _{\mathrm{ref}}(\mathbf{x})\right]$ -- one way to achieve this heuristically is by iteratively creating a \emph{sequence} of prompt distributions directing its learning towards new, informative prompts to continue training. This is the key unconventional approach that~\method~takes (please check $\S$~\ref{app:theory} for more background). 
    \item \textbf{Q2 - KL.} We have revised Eq.~\ref{eq:regret-pi} so that the regret is the difference in the reward of the current policy and the KL-optimal policy (thanks for catching this). For the solver, by design, preference optimization would be equivalent to regret minimization, thus the alignment problem remains to be correctly defined. For the creator, the distribution matching to the open-ended reference is implicitly achieved by prompt curriculum construction, and we present empirical evidence in $\S$~\ref{app:curr} to justify that prompts are evolving towards broader tasks with higher complexity.
    \item \textbf{W1 - Proxy.} We have revised Definition~\ref{def:info-proxy} for better readability. It is estimated by sampling multiple responses from the stochastic policy and calculating the reward range (or other advantage-based proxy). This approximation will result in sub-optimality for creator's regret maximization process, and we present more discussion in $\S$~\ref{app:theory-2}.
\end{itemize} 

% (i) we have revised the manuscript \emph{w.r.t.} KL-regularized regret and discussed our approximation made in $\S$~\ref{app:theory}; (ii) we sample multiple times from the stochastic policy to tractably estimate the informativeness proxy, which we explained in detail at $\S$~\ref{app:theory-3}; (iii) the \textbf{solver maintains the KL regularization} with regard to the reference policy during training, thus the alignment problem at each iteration remains correctly defined; (iv) the creator does not have a tractable reference distribution, and we use a fixed creator and apply meta instructions and buffer sampling to adapt/constrain the prompt generations (as described in $\S$~\ref{sec:algo}, $\S$~\ref{app:reproduce} and $\S$~\ref{app:exp-evol}), which is easy-to-implement and empirically effective.

\textbf{Rebuttal:}  For the rebuttal to be self-contained, we  extract contents from~\secref{app:theory} here.

First, we re-present the open-ended RLHF principle, and discuss the intuition under the KL regularization. Next, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. Finally, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection*{\textbf{.1} \ The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1-}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}

The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.

\subsection*{\textbf{.2} \ Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2-}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection*{\textbf{.2.1} \ The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection*{\textbf{.2.2} \ Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 
% \begin{itemize}
%     \item \textbf{Regret approximation}: the same as~\citep{plr} -- the positive value loss.
%     \item \textbf{Environment generation}: 
% \end{itemize}

Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.





 


% \cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones.


% (TODO: give an overview on this setting; our creator follows the similar setting by identifying the high-regret levels and then making edits with them combining a buffer.)
% Later on, researchers explore more \emph{curriclum}-driven approach, especially through adversarial training~\citep{adr} with minimax objective

% . The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

% \textcolor{red}{This section is about heuristics on distributional matching with a game setting. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }

% \subsubsection{Reformulating Constrained Optimization to Minimax Optimization}

% \newpage
\subsection*{\textbf{.3} \ Regret Formulation for Open-Ended RLHF}\label{app:theory-3-}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.





\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right). \nonumber
\end{align}
% where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

% Thus the regret with regard to the KL-constrained optimal policy is:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \nonumber
% \end{align}


% Assuming $\rvy_+, \rvy_-$ are correctly labeled by an \textit{oracle reward model} $r(\cdot, \cdot)$, the direct preference optimization objective is:
% \begin{align}
%     \mathcal{L}_{\text{DPO}}=-\mathbb{E}_{\rvx \sim \calD, (\rvy_+, \rvy_-) \sim \pi_{\vtheta}(\cdot \mid \rvx)}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_+ \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_+ \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_- \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_- \mid \rvx\right)}\right)\right]. \nonumber
% \end{align}


We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret--}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.



\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


% We thank the reviewer for catching the omission of the KL term in the original writeup on regret. Please see our revised definition and detailed discussion on the approximation that we made in $\S$~\ref{app:theory}, and empirical results in $\S$~\ref{sec:main_results} on  alignment gains over different algorithms and benchmarks, $\S$~\ref{app:curr} on generated prompt distributions and alignment gains across different categories. 





% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{W2 (Regret and KL)}: The optimization is over $\pi$ in Eq. 9 for solving the minimax regret. However, its not absolutely clear how the KL divergence plays a role here and how it is ensured that the response and prompt distributions are close to reference. Without that, the alignment problem is ill-defined. Please provide concrete justifications in theory and empirical results.}
% \end{tcolorbox}

% \textbf{TL;DR:}

% \textbf{Rebuttal}


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W3 (Understanding the Iterative Algorithm)}: As described in Algorithm 1, informativeness is evaluated and a prompt subset is created based on current policy estimate and then the policy is updated based on the prompt subset. However, this causes an inter-dependence between the two which leads to nested structure, which is not clearly explained. Specifically, while computing the informativeness score for the prompts, it depends on $\theta^\star(x_{t-1})$ , \ie optimal parameter for the previous distribution. Provide clear explaination on the same.}
\end{tcolorbox}

\textbf{TL;DR:} (i) We revised Algo.~\ref{alg:i-eva} with updated subscripts to reflect the training process -- please take a look in our main paper. Given a current model checkpoint, we evaluate the prompt informativeness based on it, and evolve a new prompt set more informative to the current checkpoint, and use the new prompt set for continual training. (ii) We intend to use an iterative best-response framework to approximate equilibrium in expectation, balancing computational efficiency and practicality. 

\textbf{Rebuttal:} The iterative updates in~\method, as described in Algo.~\ref{alg:i-eva}, are based on a best-response-to-best-response framework. Specifically, the creator updates the prompt distribution based on the solver’s current policy, and the solver then optimizes its policy over the updated prompts, and the process repeats. This sequential structure approximates a Nash equilibrium in expectation over iterations, inspired by works such as~\cite{freund,self-play-gu}, which establish convergence to optimal policies on average through iterative optimization.

We intentionally avoid simultaneous joint optimization as it would significantly increase computational and memory overhead, making it less practical for integration into current RLHF pipelines. 

% The current approach is simple and effective, and leads to concrete empirical performance gain as shown in $\S$~\ref{app:curr}. While this paper emphasizes \textbf{practical usability} over formal theoretical guarantees, we look forward to future works on extensions for Open-Ended RLHF (such as adding convergence rates and equilibrium guarantees, deriving first-order solutions, etc). We would greatly appreciate any further suggestions or insights the reviewer may have to improve this direction.

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W4 (Understanding Reward Models)}: While iterating, every new prompt distribution will require generating new response, how is the evaluation coming from which reward model? Is the ground reward available, if not please explain how the preference is obtained and how does it affect suboptimality? Also: } \textcolor{gray}{\textbf{Q3 (RM Availability)}: What's the reward model availability? Is the true reward model available?}
\end{tcolorbox}

\textbf{TL;DR:} We assume a preference oracle provided by an \textbf{external, pre-trained reward model}, which is practically  used in many real-world LLM training scenarios~\citep{team-1}.

\textbf{Rebuttal:} As discussed in the beginning of the experimental setting in $\S$~\ref{sec:exp}, we assume the availability of a pre-trained, fixed reward model. This approach is practically adopted in industry~\citep{team-1,team2,gemma2} and is also commonly used in academia works~\citep{dpo-iterative,simpo,self-play-gu}. The reason is more on efficiency concerns. For example, in \textsc{Gemma-2} training, the reward model is \emph{an order of magnitude larger} than the policy~\citep{gemma2}; it would thus be impractical or the gain may only be marginal if we update the reward model on-the-fly. 

% (as done in many prior works on bi-level RLHF -- thanks again for the reviewer's nice references). 

Nevertheless, it is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} (ablation studies) that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and address the potential distribution mismatch problem. We believe this is an interesting direction to pursue, and have listed it in $\S$~\ref{sec:conclusion} (future works) on adding more players including rewarders in the self-play loop.


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W5 (Improvement of Sub-Optimality)}: Overall, which expression/Theorem guides us in understanding the improvement of prior suboptimality is not clear? Can you please point out/highlight how the current method improves upon the prior suboptimality due to static prompt distribution? }
\end{tcolorbox}

\textbf{TL;DR:} The improvement of sub-optimality is guided by the minimax regret objective (Remark 1) through its iterative implementation. While this work does not explicitly derive suboptimality bounds, our approach has demonstrated \textbf{strong empirical gains} over the training by static distributions, as shown in $\S$~\ref{sec:exp} (main experiments), $\S$~\ref{app:curr} (benchmark performance), and $\S$~\ref{app:exp-iter} (alignment gains over iterations).

\textbf{Rebuttal:} In general, the improvement of prior suboptimality due to static prompt distributions is guided by the minimax game outlined in Remark 1. This expression forms the basic foundation for our iterative algorithm, where the creator updates prompts to maximize informativeness (proxy for regret), and the solver minimizes regret (through direct preference optimization). This iterative process ensures the solver and creator adapt to each other, implicitly forming a curriculum and addressing sub-optimality  in static prompts. We also added $\S$~\ref{app:theory} to help illustrate the intuition behind.

The empirical results in $\S$~\ref{sec:exp} (main results), $\S$~\ref{app:curr} (curriculum effect and benchmark improvement), and $\S$~\ref{app:exp-iter} (alignment gains over iterations) demonstrate that the dynamic prompt distribution improves solver performance and alignment metrics, thereby mitigating suboptimality. While the current package does not explicitly derive sub-optimality bounds (as would be typical in formal RL/bandit theory papers) and emphasizes practicality and usability as a methodology paper, we would love to learn if the reviewer has any suggestions for this as the future work.

% We thank the reviewer’s suggestions on formalizing sub-optimality analysis further and would love to consider this an exciting direction for future work.


\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{W6 (Prompt Distribution)}: It is extremely crucial to show the prompt distribution and demonstrate its perplexity to ensure its not generating some meaningless or irrelevant prompts, since its not very evident on the KL divergence in the prompt space and its relation with the informative measure. Please provide detailed explanation to clarify that. }
\end{tcolorbox}

\textbf{TL;DR:} We have (i) added experimental results in $\S$~\ref{app:curr} (prompt distribution visualization) and $\S$~\ref{app:examples} (prompt examples) to verify that~\method~evolves meaningful and relevant prompts with improved complexity and quality; (ii) added explanation in $\S$~\ref{app:theory} (detailed illustration of method) on the conceptual KL regularization in the prompt space and the implicit approximation by the creator.

\textbf{Rebuttal:} (This rebuttal also addresses Reviewer \texttt{\small ac2p}'s concerns on curriculum.)

We have revised the manuscript with additional visualization on potential curriculum learned in $\S$~\ref{app:curr}. In general, we observe the creator prioritizes learning in math and coding for the generated prompt distribution, which brings gradual improvement on benchmark performance on relevant categories over iterations. In other words, \method~effectively shifts focus towards harder yet learnable categories. We have attached the bar plot and radar figure here for the reviewer's reference:

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/bart-iter.pdf}
        \caption{\textbf{Training distributions.} The prompt distribution of Table~\ref{tab:ab-10k} for evolved prompts by zero-shot classification. \method~creates a curriculum that prioritizes math / coding prompts.}
        \label{fig:dist--}
    \end{minipage}
    \hspace{0.02\textwidth} % Adjust horizontal space as needed
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/radar-gemma.png}
        \vspace{+2pt}
        \caption{\textbf{Benchmark performance.} The radar figure for ratings on MT-Bench~\citep{llm-judge}, where each category contains ten problems. \method~prioritizes and gradually improves on coding, math and reasoning over iterations, implicitly reflecting a learned curriculum.}
        \label{fig:radar-gemma--}
    \end{minipage}
\end{figure}

We have added Table~\ref{tab:prompt-evol-2} providing qualitative examples for evolved prompts. Also, as noted in $\S$~\ref{app:theory}, the solver maintains KL regularization during optimization, ensuring that the response distribution remain close to the reference policy; in the this work, we do not explicitly add KL regularization in the prompt distribution since we do not directly conduct parameter update for the creator (which we empirically find to bring training instability); rather, we use \textbf{meta instructions} and \textbf{buffer sampling} to constrain the prompt generations (as described in $\S$~\ref{sec:algo}, $\S$~\ref{app:reproduce} and $\S$~\ref{app:exp-evol}), which is empirically very effective, and introduces only minimal changes to existing pipeline thus can be easily applied. As noted in $\S$~\ref{sec:conclusion}, we look forward to future works on making the creator policy differentiable.

Regarding the relation with the informativeness measure, our current proxy is an efficient proxy among many possibilities to approximate regret (where one way to implicitly achieve $\mathbb{D} _{\mathrm{KL}}\left[\pi _\phi(\mathbf{x}) \| p _{\mathrm{ref}}(\mathbf{x})\right]$ is by training on the prompt curriculum created by the creator with regret maximization as its strategy). We have provided detailed discussions in $\S$~\ref{app:theory} to help interpret it. 
% There could be other proxies -- one interesting direction is to completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection.

We note that perplexity is not commonly used nor the most preferred  measure for data quality in practical training of large language models~\citep{team-1,wrong}, and can be computationally heavy to measure. We have added experiments in~\secref{app:curr-2} which we follow~\cite{deita} to generatively measure the complexity and quality of prompt distributions.  As in Table~\ref{tab:prompt-quality-complexity--}, there is a gradual improvement of prompt complexity and quality over iterations with~\method.  We believe this would address the reviewer's concerns.

% ----------
\begin{table}[H]
\centering

\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule

\textbf{Prompt Set ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{Complexity} (1-5) & \textbf{Quality} (1-5)    \\ \midrule



UltraFeedback (seed)    & 2.90  & 3.18 \\

\rowcolor{green!10} 
UltraFeedback-\method-Iter-1  & 3.84  & 3.59 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-2  & 3.92  & 3.63 \\ 

\rowcolor{green!10} 
UltraFeedback-\method-Iter-3  & \textbf{3.98}  & \textbf{3.73} \\ 

\bottomrule

\end{tabular}%
}
\caption{\text{\method~improves prompt quality and complexity}.}
\label{tab:prompt-quality-complexity--}
\end{table}
\vspace{-10pt}
% ----------

% ------------------
% \begin{table}[H]
% \centering
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}r p{12.6cm}@{}}
% \toprule
% \rowcolor{lightgray!16}
% \multicolumn{1}{r}{\texttt{\small initial prompt} $\rightarrow$} & \texttt{\small Write me the code for a distributed transaction manager.\textbackslash nThink step by step and use pseudo code first.\textbackslash nThen, define interfaces for all involved actors and entities.\textbackslash nUse Rational Unified approach for this part.\textbackslash n\textbackslash nOnly then move on to the actual implementation, class-by-class, and method-by-method.\textbackslash nMake the code be implemented in C\# and follow SOLID principles.} \\ \midrule
% \texttt{\small evolved \#1 $\rightarrow$} & \texttt{\small Craft a suite of syntax for a distributed transaction coordinator. Start with a sequential breakdown in pseudocode format. Following that, establish the protocols for communication and interaction amongst the various participants and components, incorporating the Rational Unified Process methodology.\textbackslash n\textbackslash nProceed thereafter to the concrete creation, detailing each class and function. Ensure that the final C\# code adheres to the precepts of SOLID and is annotated for clarification and maintainability purposes.} \\
% \texttt{\small evolved \#2 $\rightarrow$} & \texttt{\small Devise a comprehensive set of directives and structures for a distributed transaction coordinator architecture. Initiate by formulating a step-by-step algorithmic decomposition in pseudocode. Subsequently, delineate the frameworks for dialog and cooperation between the numerous entities and elements, utilizing the tenets of the Rational Unified Process methodology.\textbackslash n\textbackslash nContinue to the actual generation of the code, meticulously detailing every class and corresponding method. Guarantee that the culminating C\# code is in strict compliance with SOLID principles and is supplemented with descriptive commentary to enhance future clarity and upkeep, while also validating the code against a set of unit tests to ensure robust functionality.} \\
% \texttt{\small evolved \#3 $\rightarrow$} & \texttt{\small Commence by constructing an algorithm in pseudocode that meticulously breaks down the sequential stages for a distributed transaction coordinator system. Progress by outlining the communication protocols and collaborative mechanisms among the myriad components, adhering to the Rational Unified Process approach.\textbackslash n\textbackslash nAdvance to crafting the code in C\#, ensuring each class and method is elaborated with precision, aligning with SOLID design principles. Integrate thorough comments for heightened maintainability and conduct comprehensive unit testing for assured operational integrity.} \\
% \texttt{\small evolved \#4 $\rightarrow$} & \texttt{\small Design a detailed flowchart that represents the intricate steps of an orchestration engine for managing microservices in a cloud-native environment. Begin by detailing the service discovery, load balancing, and fault tolerance strategies, while incorporating the DevOps philosophy.\textbackslash n\textbackslash nProceed by developing the implementation in Java, focusing on clean, modular code following object-oriented programming best practices. Accompany your code with clear documentation for easy understanding and perform rigorous integration testing to guarantee robustness.} \\ \bottomrule
% \end{tabular}%
% }
% % \vspace{-4pt}
% \caption{Examples of evolved prompts from AlpacaEval. We suggest practitioners to include generated responses with oracle rewards and self-critique in the context for better prompt evolving, which is helpful for mitigating the effect of potential self-consuming loops in synthetic data training.}
% \label{tab:prompt-evol-2-}
% \end{table}


% ----------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q1 and Q2 (KL in the Solver Loop)}:  Since equation 7, can't be directly solved, and is solved in an asymmetric fashion, then in the solver loop the KL should be over the response distribution and not joint right? How is the KL divergence w.r.t reference policy for the algorithm? Please provide detailed ablation.}
\end{tcolorbox}

\textbf{Answer:} (i) Yes, in the solver loop, the KL regularization is applied over the response distribution, not the joint distribution, as shown in Algo.~\ref{alg:i-eva}. (ii) The KL divergence \emph{w.r.t.} reference policy is determined by the plug-in solver (\eg DPO), which is orthogonal to our framework. We have added detailed explanation in $\S$~\ref{app:theory} to illustrate the whole process.

% ----------------


% ----------------
% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{Q3 (RM Availability)}: What's the reward model availability? Is the true reward model available?}
% \end{tcolorbox}

% \textbf{Answer:} Yes, we assume the availability of a pre-trained, off-the-shelf reward model. This approach is practically adopted in industry~\citep{team-1,team2,gemma2} and is also commonly used in academia works~\citep{dpo-iterative,simpo,self-play-gu}. See also our detailed rebuttal for \textbf{W4}.
% ----------------

% ----------------
\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textcolor{gray}{\textbf{Q4 (Literature)}: There is a recent line of works on Stacklberg and Bilevel RLHF which deals with the entanglement in a leader-follower setting. Although not specific to updating prompt dist, but can be trivially applied. Provide a detailed comparison with the literature around that [1,2,3].}
\end{tcolorbox}

\textbf{TL;DR:} We thank the reviewer for this nice suggestion. Please see below for a detailed review on the relevant literature, highlighting the unique contribution of~\method. We have added $\S$~\ref{app:lit-bilevel} in the manuscript.

\textbf{Rebuttal:}
Bi-level optimization refers to optimization problems where the cost function is defined \textit{w.r.t.} the optimal solution to another optimization problem~\citep{roger-class}. There is a recent line of works applying bi-level optimization to RLHF. While they all rely on a fixed dataset of prompts, \method~propose to dynamically update the prompt set. We hereby present a detailed comparison of~\method~with~\cite{bilevel-sail,bilevel-shen,bilevel-sta-rlhf}. We thank the anonymous reviewer for the kind  references, and welcome suggestions for any other works we may have missed.
% While those works are orthogonal to~\method, We  thank the anonymous reviewer for the kind  references, which may help address the potential distributional mismatch issues as the policy models become more powerful.

\cite{bilevel-sail} formulate iterative online RLHF as a bi-level optimization problem, where the upper-level represents the reward learning, and the lower-level represents the policy optimization. Leveraging reward re-parameterization tricks in~\cite{dpo}, \cite{bilevel-sail} reduces the problem to a single-level objective with regard to the policy. The differences of this work and our work lie in the prompt distribution and preference oracle: (i) \method~features by \textbf{dynamic prompt set generation for Open-Ended RLHF}, whereas~\citep{bilevel-sail} remains using a static prompt set; (ii) we assume the existence of the preference oracle (as discussed in $\S$~\ref{sec:exp}), while~\cite{bilevel-sail} consider online training of reward models and ablate on self-rewarding by the current LLM policy. Our usage of a pre-trained reward model follows from industrial practices~\citep{team-1,gemma2}, which is also commonly used by prior works in academia~\citep{simpo,self-play-gu}. 
% We recognize the online training of reward models (see also~\citep{rlhf-workflow}) as an orthogonal/complementary direction to the current settings of~\method~(our setting is \textbf{agnostic to the preference structure}), and encourage future works and collaborations towards it, as mentioned in $\S$~\ref{sec:conclusion}.

\cite{bilevel-sta-rlhf} provide an interesting exploration on formulating RLHF as a leader-follower game, where the language model (LM) policy is the leader and the reward model (RM) policy is the follower, and the solution is \textbf{Stackelberg equilibrium}~\citep{stackelberg,game-mbrl}, where the \emph{leader does not likewise best respond to the follower's strategy}. Here, following the curriculum RL literature~\citep{paired,accel}, we seek the \textbf{Nash equilibrium}~\citep{nash} between the creator for prompt generation and the solver for response generation. Nevertheless, the LM-RM iterative optimization may be added on top of~\method's~framework, and we look forward to future works exploring the leader-follower re-formulation of~\method.

\cite{bilevel-shen} present a rigorous theoretical work (though it does not directly involve practical post-training of large language models). The authors propose to reduce the bi-level problem to a single-level problem with a penalty-based reformulation, and apply it in the setting of LM-RM optimization within a \textit{fixed} environment, whereas~\method~focuces on dynamic prompt generation and practically train large language models with extensive empirical experiments conducted. We believe it would be interesting to adapt similar first-order optimization techniques to solve Open-Ended RLHF.

In summary, existing bi-level RLHF works focus on online optimization of both the RM and the LM (as the response policy), all with \textbf{fixed} prompt/state distribution. \method~presents an orthogonal direction on \textbf{dynamic} prompt generation for Open-Ended RLHF, with an empirical algorithm which attains state-of-the-art performance with large language models on a variety of benchmarks. It is possible to incorporate the online RM training within~\method~--~we have shown in $\S$~\ref{sec:ab-rm} that \method\ scales with quality of reward models, thus integrating online RM training may further enhance performance and mitigate potential distributional mismatch problems as we evolves for more prompts. This direction may have not been widely adopted in real-world training of language models, due to concerns about practicality~\citep{team-1,team2,gemma2,nemotron}. We look forward to future works exploring \emph{efficient} variations unifying \method\ and existing bi-level RM-LM frameworks.
% ----------------


% ----------------
% \vspace{+6pt}
% \begin{tcolorbox}[myquote]
% \textcolor{gray}{\textbf{Q5 (Intuition on Open-Ended RLHF)}: Can you provide intuitions behind equation 7, on the KL divergence between the joint policy for both prompt and response? Is it even tractable to estimate or approximate this KL?}
% \end{tcolorbox}

% \textbf{Answer:} To avoid repetition, please see our detailed rebuttal for \textbf{W1}. We have also added $\S$~\ref{app:theory} to ensure this concern is sufficiently addressed.
% ----------------

\vspace{+6pt}
\begin{tcolorbox}[myquote]
\textbf{Final Remarks.} We thank the reviewer for the precious time and efforts on the~\method~method. We value all those opinions, and have made every effort to thoroughly address the concerns raised and revise our manuscript accordingly. Regarding the rejection, we hope the reviewer may kindly consider the points that we have summarized at the beginning of this rebuttal, on the \textbf{strong empirical alignment gain} brought by the \textbf{simple design} of~\method, also on judging the merit of a work (\textit{cf.,} \href{https://psc-g.github.io/posts/mentoring/reviewing/#conclusion}{ (Castro, 2021)}) \emph{w.r.t.} the practicality and how the community may easily build on top of the principle and the method we proposed (\textit{cf.,} \href{https://d37ugbyn3rpeym.cloudfront.net/stripe-press/TAODSAE_zine_press.pdf}{(Hamming, 1986)}), which we are confident are valuable to the broader alignment community. We look forward to any future discussion, and would be grateful if the reviewer may consider revising the score if the revision is satisfactory.
\end{tcolorbox}

\textbf{Paper Link}: \href{https://openreview.net/pdf?id=TMYe4rUuTc}{\texttt{\small https://openreview.net/pdf?id=TMYe4rUuTc}}.







==> appp/app-reproduce.tex <==
\section{Details on Reproducibility}\label{app:reproduce}
Our code is built based on many open-source packages, and we sincerely thank every developer and contributor of these projects for their efforts and contributions to the community.

\paragraph{Code release.} We hope to open-source all codes, generated data and trained models, \textit{upon approval} -- before then, we are more than happy to provide any clarification to help re-implement~\method~and replicate our results. In general, our code base is made to be simple to use for practitioners, requiring \textbf{only a creator module addition} within the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline.

\paragraph{Hyperparameter settings.} We follow the original hyperparameter settings as in~\citep{orpo,simpo,self-play-gu}, default to be:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
$\lambda$                                                      & /      & 0.5      & /      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1024   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
\bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-main-params}
\end{table}


\paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-reward}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
    \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
    % \item ...
\end{itemize}

For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this and other plug-in evolving methods. For solver we generate 6 responses per prompt.

% \paragraph{Computation environments.} 

\paragraph{Software environments.} All experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve Gemini (default to be \texttt{\small gemini-1.5-pro}) and transformers models (default to be \texttt{\small gemma-2-9b-it}). For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. We use 42 as the random seed.

% We include main Appendix following references, also in \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}.

==> appp/app-theory-clean.tex <==
In~\secref{app:theory-1}, we present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}



The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.



\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 


Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.


\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.

\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber

\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.




We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.




\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.


==> appp/app-theory-old.tex <==
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

\subsection{Connections in Open-Ended RLHF, Minimax Game and the Proxy}\label{app:intuition}

We provide an extended discussion on $\S$~\ref{sec:method} to make the explanation more coherent and easy-to-understand. Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{cred}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tg{\pi_{\phi}(\rvx)} \cdot \tc{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}), which is a special case if $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expand Eq.~\ref{eq:rlhf-joint-}:

\resizebox{\textwidth}{!}{$
\max_{\tg{\vphi}, \tc{\vtheta}} \ \mathbb{E}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cred}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\textit{KL}}\bigr[\textcolor{cred}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
- \beta \cdot \textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}. \nonumber 
$}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


To clarify, while $\pi_{\text{SFT}}(\cdot)$ refers to the supervised trained model~\citep{rlhf}, the newly proposed $p_{\text{ref}}$ represents an \textbf{open-ended} and potentially intractable probability measure over all possible tasks (instatiated \emph{via} prompts) or user prompts -- note it is not the static training prompt distribution. Here, the regularization $\textcolor{black}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by generating new tasks for self-training and self-improvement, instead of optimizing over a static, pre-defined prompt set. The non-trivial part is on solving this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

In the next, we will provide a step-by-step derivation leading to our Algo.~\ref{alg:i-eva}. To begin with, we first discuss how prior works tractably solve similar open-ended learning problems via two-player game formulation. Next, we formally present the new objective, and discuss how to tractably solve it in our specific setting.

\subsection{Designing Two-Player Games for Open-Ended Environment Design}
The underlying idea is straightforward, while we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$, we are able to create a series of environments. The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

\textcolor{red}{TODO: unifying the theorems/notations in previous literature. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }
\begin{itemize}
    \item \cite{poet}:
    \item \cite{paired}:
    \item \cite{plr}: scoring by generalized advantage estimation
    \item \cite{dcd}:
    \item \cite{accel}:
\end{itemize}

\subsection{Regret Formulation for Open-Ended RLHF}

\subsubsection{Advantage-Based Regret and Approximation by EvolInstruct: The Creator Step}

\subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

\newpage



\textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



 Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
\begin{itemize}
    \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
    % \end{itemize}
    \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \begin{itemize}
    %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
    % \end{itemize}
\end{itemize}

% \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

The regret objective is defined as
\begin{align}
\operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
\end{align}
% $$
% \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% $$

At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
\begin{align}
    \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
\end{align}
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

This approximation introduces two practical advantages:
\begin{enumerate}
    \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
    \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
\end{enumerate}

This deviates from the theoretical Open-Ended RLHF objective. In particular:
\begin{itemize}
    \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
    \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
\end{itemize}

Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


\subsection{KL-Regularized Regret}\label{app:kl}
For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
\begin{align}
    \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
\end{align}

Using this definition, the regret at a given prompt $\mathbf{x}$ is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
\end{align}

% This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% \begin{itemize}
%     \item 
%     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% \end{itemize}

\subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
\textcolor{red}{TODO: add derivation to better justify this approximation.}
In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
\begin{align}
    \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
\end{align}

This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
\begin{itemize}
    \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
    \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
    \begin{itemize}
        \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
        \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
    \end{itemize}
    \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
\end{itemize}


We justify this simplification as follows:
\begin{itemize}
    \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
    \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
    \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
\end{itemize}

We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> appp/app-theory.tex <==
\newpage
\section{Extended Illustration on the Methodology}\label{app:theory}
% In this section, we discuss missing details for $\S$~\ref{sec:method}. 

This is an extended version of $\S$~\ref{sec:method}. In~\secref{app:theory-1}, we re-present the open-ended RLHF principle in Definition~\ref{eq:rlhf-joint}, and discuss the intuition under the KL regularization. In~\secref{app:theory-2}, we show heuristic approaches in open-ended learning to approximate this objective, with a focus on minimax game formulation. In~\secref{app:theory-3}, we formalize the regret objective in our RLHF setting, and discuss the regret minimization for the solver and the regret maximization for the creator.

\subsection{The Conceptual Open-Ended RLHF Formulation}\label{app:theory-1}

 Classical RLHF optimizes over a static prompt set:
\begin{align}
    \max _{\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Bigl]. \nonumber
\end{align}

We propose to drop the static prompt set assumption, and jointly update the prompt distribution via a creator policy for Open-Ended RLHF, with the ideal objective below:
\begin{align}
    \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\rvx \sim \pi_{\vphi}(\cdot)}  ,  \textcolor{black}{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Bigr[ \ r(\rvx, \rvy) \ \Bigr]
    - \beta \cdot  \sD_{\text{KL}}\Bigl[\ \tb{\pi_{\phi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl]. \nonumber
\end{align}

This generalizes RLHF (Eq.~\ref{eq:rlhf-cls}). We can rewrite Eq.~\ref{eq:rlhf-joint-} with modified coefficients for precision:

\resizebox{\textwidth}{!}{$
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
$}

% \resizebox{\textwidth}{!}{$
% \max_{\tb{\vphi}, \tb{\vtheta}} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]    - \textcolor{cgreen}{\sE}_{\textcolor{cgreen}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cgreen}{\Bigr[ \ } \beta \cdot \textcolor{black}{\sD_{\text{KL}}\bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}\ \textcolor{cgreen}{\Bigr]} 
% - \beta \cdot \emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}. \nonumber 
% $}

% \begin{align}
% \resizebox{\textwidth}{!}{$
% \max_{\tg{\vphi}, \tc{\vtheta}} \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot), \mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})} \big[r(\mathbf{x}, \mathbf{y})\big] 
% - \beta \cdot \mathbb{E}_{\mathbf{x} \sim \pi_{\phi}(\cdot)} \big[\sD_{\textit{KL}}[\pi_{\theta}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})]\big] 
% - \beta \cdot \sD_{\text{KL}}[\pi_{\phi}(\mathbf{x}) \| p_{\text{ref}}(\mathbf{x})].
% $}
% \end{align}


The newly proposed $p_{\text{ref}}$ represents an \textit{underspecified}, potentially intractable probability distribution over possible tasks in the \textbf{open-ended world} (instatiated \emph{via} prompts) -- it is \emph{not} the initial static training prompt distribution (which is only the seed set for the creator to evolve upon); it can be seen serve as a conceptual guide to steer the prompt distribution. 

To further clarify, there are two types of regularization in open-ended RLHF:
\begin{itemize}
    \item $\mathbb{D}_{\text{KL}}\left[\pi_\theta(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\text{SFT}}(\mathbf{y} \mid \mathbf{x})\right]$: this is the classical regularization on the response policy, ensuring that no matter how the training distribution over prompts evolves during optimization, the response policy remained anchored to the supervised fine-tuned (SFT) policy.
    \begin{itemize}
        \item This KL (and preference optimization) is \textbf{explicitly achieved} in plug-in algorithms (\eg DPO) in  Algo.~\ref{alg:i-eva}. We later show how it relates to \textbf{solver's regret minimization}.
    \end{itemize}
    \item $\tg{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$: this probability matching term captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities, directing its learning towards informative, new tasks~\citep{jiang-thesis}, instead being constrained in a static, pre-defined set of tasks. 
    \begin{itemize}
        \item This conceptual KL is \textbf{implicitly achieved} by the creator step in the current~\method~setting by training on a \emph{sequence of informative prompt sets}. We later show how it relates to \textbf{creator's regret maximization}. As illustrated in $\S$~\ref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration. This approach resembles classical open-ended learning in $\S$~\ref{app:theory-2}, and we hope it can serve as a small step for future works to build upon.
        \item A common misunderstanding among readers may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks (\eg user prompts in the real wild world), as a conceptual target derived from the \textit{underspecified distribution}~\citep{paired}, \ie an environment with free parameters that control. Let's use an illustrative example with Fig.~\ref{fig:dist}: the prompt distribution may be defined along several dimensions (\eg the number or complexity of coding problems); a potential creator can be designed to modify these dimensions, steering the initial $\mathcal{D}$ to new training distributions, by certain decision rules (\eg minimax regret, which offers worst-case guarantees) that forms \emph{a sequence of informative prompts} for training. 
    \end{itemize}
\end{itemize}

This joint optimization objective only serves as a general principle. In the next, we discuss how existing works \textbf{implicitly achieve} the open-ended learning objective through \textbf{two-player games}.

% A common misunderstanding may be to confuse the open-ended reference $p_{\text{ref}}(\rvx)$ with the initial seed prompt distribution $\mathcal{D}$, which is static. In contrast, $p_{\text{ref}}(\rvx)$ represents a broader space of tasks -- a conceptual target derived from the \textit{underspecified distribution}. As shown in Fig.~\ref{fig:metric-corr}, the initial prompt distribution can be defined along several dimensions (\eg the number or complexity of coding problems). A potential creator policy can be made to modify these dimensions to explore new training distributions.





% The probability matching term $\textcolor{cgreen}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \bigr]}$ captures the intuition on optimizing $\pi_{\phi}(\rvx)$ to approach the conceptualized $p_{\text{ref}}(\rvx)$, in the sense that a language model optimizes itself by adapting its training distributions with newly generated prompts for self-training to develop increasingly general capabilities~\citep{jiang-thesis}, instead of constrained in a static, pre-defined prompt set. 
% The non-trivial part is thus on approaching this open-ended optimization when we do not have a tractable parameterization for $p_{\text{ref}}(\rvx)$.

% The following serves as an illustration from Definition~\ref{eq:rlhf-joint} to  Algorithm~\ref{alg:i-eva}, especially on 

% As a background, we first discuss how prior works/heuristics solve similar open-ended learning problems. Next, we formally present the new objective under a game, and discuss how to tractably solve it in our specific setting.

\subsection{Approaching Open-Ended Learning by Unsupervised Environment Design}\label{app:theory-2}
% \subsubsection{Prior Heuristics for Open-Ended Learning}
\subsubsection{The Asymmetric Game Formulation for Unsupervised Environment Design}
While we cannot directly train the agent with the intractable $p_{\text{ref}}(\rvx)$ of the open-ended world, it is possible to curate a \textbf{curriculum of prompt distributions} to improve over the static distribution and support the \emph{continual training} of the  policy $\pi_{\vtheta}(\cdot | \rvx)$, for it to keep improving and succeed over the full task space, thus conceptually approaching $p_{\text{ref}}(\rvx)$. This is often framed as an \textbf{asymmetric two-player game}.

\cite{paired} first formally define this problem as Unsupervised Environment Design (UED). The idea is that while the real-world environments are inexhaustible and hard to tract, there may exist some free parameters (\eg height and roughness in a maze) which one may control to generate new environments; UED then concerns about designing a distribution of those free parameters (\ie settings) to create new fully specified environments, that can be used to train the agents. 

 In this setup, one player, the \textbf{creator}, generates new environments based on some specific decision rules (see the following), while the other player, the \textbf{solver}, optimizes its policy within these training environments, and the process continues iteratively. Common \textbf{heuristic strategies} include: 
\begin{itemize}
    \item \textbf{Randomization}: environments are generated uniformly and independently of the solver's current policy. This method is simple but less effective~\citep{dr}.  
    \item \textbf{Maximin}: the creator generates environments that minimize the solver’s maximum possible reward, which can often lead to unsolvable scenarios~\citep{adr}.  
    \item \textbf{Minimax regret}: The creator targets environments that maximize the solver's \emph{regret}, defined as the difference between the optimal return achievable  and that of the solver's current policy~\citep{remidi}. The regret is often conceived as the \textbf{creator's utility}.
\end{itemize}

Among them\footnote{We have implemented variants of these in $\S$~\ref{sec:ab-metric}, and show minimax regret is empirically better.}, the minimax regret approach presents a sweet spot where the creator can create hard yet solvable environments, and is often empirically better. The minimax regret strategy also implies that the agent's policy is trained to perform well under all levels/settings, thus enjoys a worst-case guarantee. However, while it is often straightforward for the solver to minimize the regret (\eg through direct policy optimization, as we discuss in $\S$~\ref{app:theory-3}), the optimal policy remains \emph{unknown} during the optimization process, thus regret as the decision signal is often intractable to the creator -- which requires \emph{approximation} (as an amusing side note, this is described as the Achilles' heel of those curriculum RL methods by~\cite{accel}).

\subsubsection{Approximating the Regret and Generating New Environments}
In general, the \textbf{creator} design in this line of research contains two steps:
\begin{enumerate}
    \item \textbf{identifying high-regret levels} using different (often heuristic) regret approximation;
    \item \textbf{generating new environments} by making variations or retrieving from buffers on those high-regret levels.
\end{enumerate}

We hereby review major works on regret approximation and environment generation as follows:

\cite{paired} propose joint training for the creator and two competing solvers. 
\begin{itemize}
    \item \textbf{Regret approximation}: here, two solver policies are trained, with the regret approximated as the \textbf{difference in their returns}. During each optimization step, one solver \emph{maximizes} this regret, the other \emph{minimizes} it, and the creator maximizes it.
    \item \textbf{Environment generation}: the system directly sample the parameter from the creator policy and use that to specify the environment.
\end{itemize}

\cite{plr} propose to random sampling on high-regret levels.
\begin{itemize}
    \item \textbf{Regret approximation}: as a heuristic, the authors use \emph{positive value loss}, which is a function of Generalized Advantage Estimate~\citep{gae} (which itself is a function of the TD error -- the difference between the expected and the actual returns) as the creator's utility.
    \item \textbf{Environment generation}: the creator have a rolloing buffer of highest-regret levels by random searching on relevant configurations. 
\end{itemize}
\cite{dcd} further propose a double-creator setting based on~\citep{plr}, where one creator is actively generating new environments, and the other is retrieving from the buffer.

\cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones. The regret approximation is the same as~\citep{plr} -- the positive value loss. For the environment generation, the authors suggest a general editing/mutation mechanism, where the creator chooses from high-regret levels and make small variations within an edit distance, which by heuristics will lead to the discovery of more high-regret environments. There is an additional filtering step: they do not directly train on the newly generated levels, but evaluate on those levels first, then add only the high-regret ones to the training buffer. 
% \begin{itemize}
%     \item \textbf{Regret approximation}: the same as~\citep{plr} -- the positive value loss.
%     \item \textbf{Environment generation}: 
% \end{itemize}

Note the solvers are often directly trained with PPO~\citep{ppo} under the environments.





 


% \cite{accel} propose to sample high-regret levels and generate new environments by making \emph{edits} on existing ones.


% (TODO: give an overview on this setting; our creator follows the similar setting by identifying the high-regret levels and then making edits with them combining a buffer.)
% Later on, researchers explore more \emph{curriclum}-driven approach, especially through adversarial training~\citep{adr} with minimax objective

% . The objective is to ensure the agents can perform robustly over the generated environments (such that the agents have a broader learning experience), and thus to \emph{generalize} better to the open-ended world.

% \textcolor{red}{This section is about heuristics on distributional matching with a game setting. First justify the problem of unsupervised environment design; next present justify regret as an objective for the environment design; next discuss existing \emph{approximations} made to approximate the regret, specifically discuss the explicit two-player training approach by~\citep{paired} and the advantage-estimation approach by~\citep{plr} and~\citep{accel}. }

% \subsubsection{Reformulating Constrained Optimization to Minimax Optimization}

% \newpage
\subsection{Regret Formulation for Open-Ended RLHF}\label{app:theory-3}
Next, we discuss the regret minimization and maximization in our setting for alignment. Specifically,
\begin{itemize}
    \item \textbf{Regret minimization for the solver}: we avoid calculating regret and use direct policy optimization (\eg DPO) to equivalently achieve regret minimization.
    \item \textbf{Regret maximization for the creator}: similarly to~\citep{plr,accel}, we first find an approximation of regret, then curate new environments for the solver to train on by (i) sampling from a replay buffer of existing prompts, and (ii) making variations (through \texttt{\small EvolInstruct}~\citep{wizardlm}) on those high-regret prompts. Specifically, we use \textbf{advantage-based estimates of the current policy}, as summarized in Table~\ref{tab:info-metric}.
\end{itemize}

This asymmetric two-player game serves as one potential modeling choice to implicitly achieve the open-ended RLHF principle that we proposed in Definition~\ref{eq:rlhf-joint}. We look forward to exploring more principled solutions in the future.

\paragraph{Preliminaries.} Let $r(\cdot, \cdot)$ be an oracle reward model. The (unregularized) optimal policy is:
\begin{align}
    \pi^{\star} = \arg \max_{\pi} \ \sE_{\rvx \sim \calD, \rvy \sim \pi(\cdot \mid \rvx)} \Bigr[\ r(\rvx, \rvy) \ \Bigr]. \nonumber
\end{align}
We have the  \emph{optimal advantage} / the \emph{negated regret} as:
\begin{align}
    A^{\star}(\rvx, \rvy) & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] \nonumber \\
    &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy). \nonumber
\end{align}
Classical preference-based RL assumes a \textit{reward}-based preference model, that is:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp  \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
    % &= \frac{1}{1 + \exp \left(- (r\left(\mathbf{x}, \mathbf{y}^w\right) - r\left(\mathbf{x}, \mathbf{y}^l\right))\right)} \\
    % &= \sigma \left(r\left(\mathbf{x}, \mathbf{y}^+\right) - r\left(\mathbf{x}, \mathbf{y}^-\right)\right). \label{eq:bt}
\end{align}

As a side note~\citep{cpl}, this is equivalent to the \emph{advantage/regret}-based preference model, due to the bandit setup in RLHF:
\begin{align}
    P\left(\mathbf{y}^+ \succeq \mathbf{y}^-\right) &=\frac{\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^+\right) - V^{\star}(\rvx, \rvy) \bigr) }{\exp \bigr(r\left(\mathbf{x}, \mathbf{y}^+\right)  - V^{\star}(\rvx, \rvy) \bigr) +\exp \bigr( r\left(\mathbf{x}, \mathbf{y}^-\right) - V^{\star}(\rvx, \rvy) \bigr) } \nonumber \\
    &= \frac{\exp  \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) }{\exp \bigr(A^\star\left(\mathbf{x}, \mathbf{y}^+\right) \bigr) +\exp \bigr( A^\star\left(\mathbf{x}, \mathbf{y}^-\right) \bigr)}. \nonumber
\end{align}

In our current setting, we assume there is an oracle preference model for the preference pair labeling.

\paragraph{KL-regularized regret.} In the RLHF setting at fixed prompt distribution, the objective is:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \pi_{\phi}(\cdot), \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \pi_{\phi}(\cdot)_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber 
\end{align}
The optimal policy of the above KL-constrained objective is:
\begin{align}
    \pi^{\star}_{\text{KL}}(\rvy \mid \rvx) = \frac{1}{Z(\rvx)} \pi_{\text{SFT}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right), \nonumber
\end{align}
where the partition function is defined as $Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)$.

% Thus the regret with regard to the KL-constrained optimal policy is:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \nonumber
% \end{align}


% Assuming $\rvy_+, \rvy_-$ are correctly labeled by an \textit{oracle reward model} $r(\cdot, \cdot)$, the direct preference optimization objective is:
% \begin{align}
%     \mathcal{L}_{\text{DPO}}=-\mathbb{E}_{\rvx \sim \calD, (\rvy_+, \rvy_-) \sim \pi_{\vtheta}(\cdot \mid \rvx)}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_+ \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_+ \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_- \mid \rvx\right)}{\pi_{\text {SFT}}\left(\rvy_- \mid \rvx\right)}\right)\right]. \nonumber
% \end{align}


We can now formally define the \emph{regret} with regard to $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$ as:
\begin{align}
    \text{Regret}_{\text{KL}}(\rvx, \pi_{\vtheta}) = \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\cdot|\rvx)} \Bigr[ \ r(\rvx, \rvy) \ \Bigr]. \label{eq:KL-regret}
\end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward/trivial to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures \emph{the alignment problem is well-defined}. In practice, we use Direct Preference Optimization (DPO) and its variants, which approximate the KL-optimal solution by iteratively adjusting $\pi_{\vtheta}$ to reflect preference differences.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.



\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    |\hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta})| \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or } \mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.

For new environment generation, as illustrated in~\secref{sec:creator-step}, we start from the seed prompt set, choose those high-regret prompts and generate variations upon them by \texttt{\small EvolInstruct}, then mixing with a buffer of the original set to form the new training distribution at each iteration.

% While there exist other approximations choices (see our summarization in Table~\ref{tab:info-metric}), we justify our choice for the minimax regret strategy under the context of contrastive preference optimization.

% (High-level idea: the regret is bounded by the range; we first define the range (the underlying assumption is suffient sampling and correct labeling) then show)

% The expected reward under the policy $\pi_\vtheta$ is given by:
% \begin{align}
%     \mathbb{E}_{\rvy \sim \pi_\vtheta(\cdot \mid \rvx)}[r(\rvx, \rvy)] = \sum_{\rvy} \pi_\vtheta(\rvy \mid \rvx) r(\rvx, \rvy), \nonumber
% \end{align}
% and it satisfies the bound:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+). \nonumber
% \end{align}
% Our objective is to show that with high probability, there is $\operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx)$.
% \begin{align}
%     \mathbb{P}\left(\left|\hat{r}_{\mathrm{KL}}-\mathrm{E}_{\mathbf{y} \sim \pi_{\mathrm{kL}}^t}[r(\mathrm{x}, \mathrm{y})]\right| \geq \varepsilon\right) \leq 2 \exp \left(-\frac{2 n \varepsilon^2}{\left(r_{\text {max }}-r_{\text {min }}\right)^2}\right)
% \end{align}

% (TODO: show that as we optimize, the upper bound of info(x) on the regret would be tighter. thus we effectively achieves high-regret seeking. Then discuss the heuristic generation by making edits through evolinstruct etc.)
% Similarly, for the KL-optimal policy $\pi^\star_{\text{KL}}(\rvy \mid \rvx)$, we have:
% \begin{align}
%     r(\rvx, \rvy_-) \leq \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] \leq r(\rvx, \rvy_+).
% \end{align}

% The KL-regularized regret is defined as:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) = \mathbb{E}_{\rvy \sim \pi^\star_{\text{KL}}}[r(\rvx, \rvy)] - \mathbb{E}_{\rvy \sim \pi_\vtheta}[r(\rvx, \rvy)].
% \end{align}

% Using the bounds above, the regret satisfies:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Define the range $\text{info}_\vtheta(\rvx)$ as:
% \begin{align}
%     \text{info}_\vtheta(\rvx) = r(\rvx, \rvy_+) - r(\rvx, \rvy_-).
% \end{align}

% Thus, the regret is bounded by the range:
% \begin{align}
%     \operatorname{Regret}_{\text{KL}}(\rvx, \pi_\vtheta) \leq \text{info}_\vtheta(\rvx).
% \end{align}


% since the regret in Eq.~\ref{eq:KL-regret} is not directly calculable. Specifically, we choose to approximate the regret as:



% A re-formulation of the reward is:
% \begin{align}
%     r(\rvx, \rvy)=r_E(\rvx, \rvy)-\beta\bigr(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\bigr).
% \end{align}




% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}



% \subsubsection{Advantage-Based Regret and Approximation by Contrastive Optimization: The Solver Step}

% In this section, we discuss connection between the regret minimization objective and the contrastive preference optimization objective.
% % \textcolor{red}{TODO: derive regret objective and DPO optimization, checking~\citep{cpl}; the KL is explicitly solved.}

% High-level idea: By the Bellman equation, we have:
% \begin{align}
%     A^*(s, a)=Q^*(s, a)-V^*(s, a)=r(s, a)+\gamma \mathbb{E}_{s^{\prime}}\left[V^*\left(s^{\prime}\right)\right]-V^*(s)
% \end{align}

% In the bandit setting, the negated regret :
% \begin{align}
%     A^{\star}(\rvx, \rvy) &= r(\rvx, \rvy) - V^{\star}(\rvx, \rvy),\\
%     & = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi^{\star}(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr].
% \end{align}

% The preference model thus becomes:
% \begin{align}
% P_A \left[\sigma^{+} \succ \sigma^{-}\right] & =\frac{\exp r_E\left(s, a^{+}\right)-V^*(s)}{\exp r_E\left(s, a^{+}\right)-V^*(s)+\exp r_E\left(s, a^{-}\right)-V^*(s)} \\
% & =\frac{\exp r_E\left(s, a^{+}\right)}{\exp r_E\left(s, a^{+}\right)+\exp r_E\left(s, a^{-}\right)}
% \end{align}

% (TODO: show the regret-based preference is equivalent to the DPO objective, thus we implicitly minimizes a function of the regret)

% Under the RLHF framework, a reformulation of the reward function is:
% \begin{align}
%     r'(\rvx, \rvy)=r(\rvx, \rvy)-\beta\left(\log \pi_\theta(\rvy \mid \rvx)-\log \pi_{\text{ref}}(\rvy \mid \rvx)\right).
% \end{align}

% \textcolor{red}{TODO: write a theoretical version with the above and a practical version with only the true reward model.}

% \subsubsection{Regret Approximation by EvolInstruct: The Creator Step}
% \textcolor{red}{TODO: derive advantage-based regret approximation; then we further approximated it with reward function and proximal editing on seed prompts, thus we do not tractably solve the KL term.}


% (This should be the reward that we use, however we directly take the reward inside)


% \newpage



% \textcolor{red}{TODO: add discussions on how we can translate this joint optimization to a minimax game.}

% While the theoretical formulation of the joint optimization objective provides an elegant framework (Eq.~\ref{eq:rlhf-joint-}), it is not directly equivalent to the minimax regret game (there are many nuances in converting constrained optimization to a minimax problem). The primary source of this gap lies in the intractability of $p_{\mathrm{ref}}(\mathbf{x})$, which represents an idealized distribution over all possible prompts $\mathbf{x}$ in the wild. Since it is inaccessible, we cannot directly evaluate or optimize the KL term $\mathbb{D}_{\mathrm{KL}}\left[\pi_{\phi}(\mathbf{x}) \ \| \ p_{\mathrm{ref}}(\mathbf{x})\right]$.



%  Consequently, the joint optimization, which assumes a coupling between the creator policy $\pi_\phi(\mathbf{x})$ and solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ through the reward $r(\mathbf{x}, \mathbf{y})$, may not be fully realized in practice.

% To address this, we propose an approximation inspired by \textit{minimax regret}. In this formulation:
% \begin{itemize}
%     \item The \textbf{creator policy} $\pi_\phi(\mathbf{x})$ is tasked with maximizing regret by generating prompts $\mathbf{x}$ that are most challenging for the solver. As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:creator-step}, this is practically achieved by choosing seed prompts with the highest informativeness metric (\eg reward advantage as in Table~\ref{tab:info-metric}) and make variations upon them in the language space.
%     % \end{itemize}
%     \item The \textbf{solver policy} $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ minimizes regret, learning to perform robustly across these challenging prompts. As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \begin{itemize}
%     %     \item As in $\S$~\ref{sec:solver-step}, this minimization is practically achieved by the plug-in contrastive preference optimization algorithm (\eg DPO), where we construct the contrastive pairs by sampling from the stochastic policy and choosing the best and the worst responses (see also~\citep{cpl} on DPO as a special case for contrastive preference optimization under regret-based model).
%     % \end{itemize}
% \end{itemize}

% % \textcolor{red}{TODO: directly write the regret in the KL form, and discuss why DPO minimizes the regret (justification for the solver step), and the approach we choose the maximize the regret with the creator (justification for the creator step).}

% This formulation avoids direct dependence on $p_{\mathrm{ref}}(\mathbf{x})$ and instead uses the creator policy $\pi_\phi(\mathbf{x})$ to generate a dynamic curriculum of prompts. To formally define the regret, we first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set $\calD$ as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% The regret objective is defined as
% \begin{align}
% \operatorname{Regret}(\mathbf{x}, \tb{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tb{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].  
% \end{align}
% % $$
% % \operatorname{Regret}(\mathbf{x}, \tc{\pi_\theta}) = \max_{\mathbf{y} \in \mathcal{Y}} r(\mathbf{x}, \mathbf{y}) - \mathbb{E}_{\tc{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[r(\mathbf{x}, \mathbf{y})\Bigr].
% % $$

% At equilibrium, this minimax regret strategy provides the solver policy $\pi_\theta$ with a worst-case guarantee over the distribution of prompts generated by $\pi_\phi$:
% \begin{align}
%     \textcolor{black}{\pi^{\star}} \in \arg \min _{\tb{\pi_{\vtheta}}} \max _{\textcolor{black}{\pi_{\phi}} }  \ \mathbb{E} _{\tb{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}
% % \begin{align}
% %     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% % \end{align}

% This approximation introduces two practical advantages:
% \begin{enumerate}
%     \item \textbf{Eliminating dependence on $p_{\mathrm{ref}}(\mathbf{x})$:} The creator policy $\pi_\phi(\mathbf{x})$ evolves dynamically to approximate an optimal curriculum without needing access to $p_{\mathrm{ref}}(\mathbf{x})$.
%     \item \textbf{Flexibility in reward estimation:} Instead of directly evaluating $r(\mathbf{x}, \mathbf{y})$ for all possible responses $\mathbf{y}$, we estimate regret by sampling multiple responses from the solver policy $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ and computing the difference between the maximum and minimum rewards.
% \end{enumerate}

% This deviates from the theoretical Open-Ended RLHF objective. In particular:
% \begin{itemize}
%     \item The coupling between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ in the reward term $r(\mathbf{x}, \mathbf{y})$ is no longer explicitly enforced. Instead, the creator focuses on maximizing regret, which may not perfectly align with the reference distribution $p_{\mathrm{ref}}(\mathbf{x}) \cdot \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})$.
%     \item The dynamic interplay between $\pi_\phi(\mathbf{x})$ and $\pi_\theta(\mathbf{y} \mid \mathbf{x})$ is approximated through alternating optimization, where each policy optimizes its objective iteratively.
% \end{itemize}

% Another challenge we are facing is the instability of training the creator policy. We currently find it effective to just use a fixed creator, which selects high-regret prompts and makes variations on them in each iteration. This is similar to incentivizing creating prompts within the agent's zone of \emph{proximal development}~\citep{zone-promximal}. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% In summary, the transition from the theoretical joint optimization to the practical minimax regret formulation is  due to the intractability of $p_{\mathrm{ref}}(\mathbf{x})$. While this approximation sacrifices some theoretical guarantees, it is easy-to-implement and enables scalable training and curriculum design by leveraging the expressive power of language models to generate diverse and challenging prompts, and we show it empirically works very well and outperforms other choices, as presented in $\S$~\ref{sec:exp}.


% \subsection{KL-Regularized Regret}\label{app:kl}
% For simplicity, we have omitted the KL terms in Eq.~\ref{eq:regret-pi}. We now present a more precise version. 

% We first denote the KL-regularized optimal policy $\pi^\star$ with regard to any induced prompt set as:
% \begin{align}
%     \pi^\star = \arg\max_{\pi_{{\theta}}} \mathbb{E}_{\mathbf{x} \sim \calD, \mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigr[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \ \| \ \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})\Bigr]. \nonumber
% \end{align}

% Using this definition, the regret at a given prompt $\mathbf{x}$ is:
% \begin{align}
%     \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) - \beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})] \Bigr]. \nonumber
% \end{align}

% % This formulation makes it clear that the regret compares the rewards of $\pi^\star$ (which is implicitly KL-regularized) and $\pi_{\boldsymbol{\theta}}$, ensuring alignment with the reference policy $\pi_{\mathrm{ref}}$.
% % \begin{itemize}
% %     \item 
% %     \item The KL penalty explicitly applies to $\pi_{\boldsymbol{\theta}}$, as the solver is trained to respect this regularization via the direct preference optimization objective.
% % \end{itemize}

% \subsubsection{Approximation in the Current Implementation}\label{app:theory-info}
% \textcolor{red}{TODO: add derivation to better justify this approximation.}
% In our current implementation, we approximate the informativeness proxy without explicitly incorporating the KL term. The informativeness proxy is defined as:
% \begin{align}
%     \widehat{A}^*_{\text{min}} = \left| \min_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) - \max_{\mathbf{y}} r(\mathbf{x}, \mathbf{y}) \right|. \nonumber
% \end{align}

% This choice of approximation avoids calculating the KL term $-\beta \cdot \mathbb{D}_{\mathrm{KL}}[\pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x}) \| \pi_{\mathrm{ref}}(\mathbf{y} \mid \mathbf{x})]$ for every sampled response when evaluating the informativeness, and we use this proxy for the creator to select prompts. To compute it in practice, we:
% \begin{itemize}
%     \item \textbf{Sample multiple responses}: For each prompt $\mathbf{x}$, we draw multiple responses $\mathbf{y}_i \sim \pi(\mathbf{y} \mid \mathbf{x})$.
%     \item \textbf{Calculate reward extremes}: Using the reward oracle, we compute:
%     \begin{itemize}
%         \item  $r_{\max} = \max_{i} r(\mathbf{x}, \mathbf{y}_i)$, the maximal reward among the sampled responses.
%         \item $r_{\min} = \min_{i} r(\mathbf{x}, \mathbf{y}_i)$, the minimal reward among the sampled responses.
%     \end{itemize}
%     \item \textbf{Compute the gap}: The informativeness proxy is then estimated as $r_{\max} - r_{\min}$.
% \end{itemize}


% We justify this simplification as follows:
% \begin{itemize}
%     \item \textbf{Practical efficiency}: By omitting the KL term in the proxy, we avoid additional forward passes through $\pi_{\mathrm{ref}}$ in the \texttt{\small creator} step,  reducing computational cost, introducing minimal changes to the pipeline and ensuring scalability for large-scale experiments.
%     \item \textbf{Solver alignment}: \textbf{The} \textbf{\small \tt solver} \textbf{is still trained to minimize the KL-regularized preference optimization objective}, as in Line 5 of Algo.~\ref{alg:i-eva}, thus the alignment problem remains \emph{well-defined}. Specifically, as we discussed in $\S$~\ref{sec:solver-step}, for each prompt, we sample multiple responses, and construct the contrastive preference pair in training by choosing the response with the \emph{minimal} and the \emph{maximal} reward, then use any off-the-shelf direct preference optimization method with KL regularization on the reference policy. This can be seen as an \emph{efficient approximation by the stochastic policy} to minimize the regret while we do not know the optimal policy (see also~\citep{paired} which explicitly trained two policies to approximate the regret).
%     \item \textbf{Empirical validation}: Despite the approximation, empirical results show that the solver achieves strong alignment and generalization. The simpler proxy effectively identifies informative prompts by focusing on the reward gap.
% \end{itemize}

% We encourage future works to take the KL regularization into account for this informativeness proxy. One interesting direction is to  completely remove the dependence on the reward model and directly use model likelihoods to make the prompt selection, leveraging the reward re-parameterization trick.

% Further investigations can explore rigorous sub-optimality bounds for such approximations. It is slightly sad to observe a gap between nowadays RL/bandit theory research and the practical algorithms adopted in practice. Many elegant theoretical ideas remain underutilized by practitioners due to the compromises required to maintain certain theoretical rigidity, while industrial approaches are often brute-force but empirically very well-performing. \method~aims to strike a balance in between.






% The first challenge we are facing is the intractability of $p_{\text{ref}}(\rvx)$, which in this formulation represents an idealized probability measure over all possible user prompts x in the wild world. 

% We instead propose a different training objective – the motivation is similar to unsupervised environment design, which we seek to \emph{evolve} a series of prompts to form a curriculum for the solver policy, $\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)$, so that it can learn to generalize across all possible prompts. The main innovation here is that traditional RL can only  \emph{edit levels}~\citep{accel,plr} for new environments, but we are directly leveraging languages to \emph{generate} new environments.

% We choose regret as the objective for the environment design, which the solver is incentivized to minimize and the creator is incentivized to maximize. At equilibrium, the solver policy follows the minimax regret strategy, providing a worst-case guarantee:
% \begin{align}
%     \textcolor{cred}{\pi^{\star}} \in \arg \min _{\tc{\pi_{\vtheta}}} \max _{\textcolor{cgreen}{\pi_{\phi}} }  \ \mathbb{E} _{\tg{\rvx \sim \pi_{\phi}}}\Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\vtheta}}) \ \Bigr]. \nonumber
% \end{align}

% To approximate this regret, prior works usually train two policies and take their difference in return. For efficiency, we choose to sample multiple responses from a single stochastic solver policy, and use the difference in the maximum and minimum reward it receives.

% As a side note, the original joint optimization is not directly equivalent to the minimax game due to the coupling between the solver policy and the creator policy with regard to reward. One way is to first optimize $\pi_\phi(\mathrm{x})$ for regularization then fix it and optimize $\pi_\theta(\mathbf{y} \mid \mathbf{x})$, and update $\pi_\phi(\mathrm{x})$ to align with reward





% We take a different approach to directly starting from the minimax regret formulation, then show that it can be expressed as the joint optimization problem.

% Let's start with the unsupervised environment design problem~\citep{paired}, and illustrate why minimax regret is a proper objective for the solver.

% \emph{Training on regret-maximizing levels has been shown to improve generalization to out-of-distribution level in challenging domains.} At convergence, the MMR policy would achieve zero regret for each level. Meaning that we have the optimal solver.

% Next, we show why this can be formulating into the joint optimization objective in Eq.~\ref{eq:rlhf-joint-} by introducing an additional $p_{\text{ref}}(\cdot)$.

% Specifically, we made three approximations:
% \begin{itemize}
%     \item Approximating a minimax optimization to a maximization problem with KL constraint
%     \item Using the stochastic policy to replace the minimax
% \end{itemize}

==> appp/tab-gen-1.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\ttiny Implement a function to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\ttiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \ nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \ The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  \ if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  \ imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  \ imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\  \ if i == 0:\textbackslash n\  \ max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  \ return max\_left\textbackslash n\textbackslash n\  \ if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  \ elif j == n:\textbackslash n\  \ min\_right = nums1[i]\textbackslash n\  \ else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1` into two parts: `nums1[0:i]` and `nums1[i:m]`.\textbackslash n\  \ - `j` is calculated to divide `nums2` so that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Partition:**\textbackslash n\  \ - We compare elements at the boundaries of the partitions to see if `i` is in the correct position:\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, `i` is too small, so we move `imin` to `i + 1`.\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move `imax` to `i - 1`.\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - Once `i` is in the correct position, we find:\textbackslash n\  \ - `max\_left`: The maximum element in the left partitions of both arrays.\textbackslash n\  \ - `min\_right`: The minimum element in the right partitions of both arrays.\textbackslash n\  \ - If the total length is odd, `max\_left` is the median.\textbackslash n\  \ - If the total length is even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we perform binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we only use a constant amount of extra space for variables.
}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\ttiny python\textbackslash n\textbackslash def find\_median\_sorted\_arrays(nums1, nums2):\textbackslash n\  \ """\textbackslash n\  \ Finds the median of two sorted arrays of different sizes.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  nums1: The first sorted array.\textbackslash n\  \ nums2: The second sorted array.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  The median of the two sorted arrays.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(nums1), len(nums2)\textbackslash n\  \ if m > n:\textbackslash n\  \ nums1, nums2, m, n = nums2, nums1, n, m\  \# Ensure m <= n\textbackslash n\textbackslash n\  \ imin, imax, half\_len = 0, m, (m + n + 1) // 2\textbackslash n\textbackslash n\  \ while imin <= imax:\textbackslash n\  \ i = (imin + imax) // 2\textbackslash n\  \ j = half\_len - i\textbackslash n\  if i < m and nums2[j - 1] > nums1[i]:\textbackslash n\  imin = i + 1\  \# i is too small, increase it\textbackslash n\  \ elif i > 0 and nums1[i - 1] > nums2[j]:\textbackslash n\  imax = i - 1\  \# i is too big, decrease it\textbackslash n\  \ else:\textbackslash n\  \ \# i is perfect\textbackslash n\textbackslash n\ if i == 0:\textbackslash n\  max\_left = nums2[j - 1]\textbackslash n\  \ elif j == 0:\textbackslash n\  \ max\_left = nums1[i - 1]\textbackslash n\  \ else:\textbackslash n\  \ max\_left = max(nums1[i - 1], nums2[j - 1])\textbackslash n\textbackslash n\  \ if (m + n) \% 2 == 1:\textbackslash n\  return max\_left\textbackslash n\textbackslash n\  if i == m:\textbackslash n\  \ min\_right = nums2[j]\textbackslash n\  elif j == n:\textbackslash n\  min\_right = nums1[i]\textbackslash n\  else:\textbackslash n\  \ min\_right = min(nums1[i], nums2[j])\textbackslash n\textbackslash n\  \ return (max\_left + min\_right) / 2.0\textbackslash n\textbackslash n\# Example usage\textbackslash nnums1 = [1, 3]\textbackslash nnums2 = [2]\textbackslash nmedian = find\_median\_sorted\_arrays(nums1, nums2)\textbackslash nprint(f"The median of \{nums1\} and \{nums2\} is: \{median\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Handle Unequal Lengths:**\textbackslash n\  \ - If `nums1` is longer than `nums2`, swap them to ensure `nums1` is always the shorter array. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\  \ - The core idea is to use binary search on the shorter array (`nums1`).\textbackslash n\  \ - `imin` and `imax` define the search range for the partition point `i` in `nums1`.\textbackslash n\  \ - `half\_len` calculates the desired total number of elements on the left side of the partition (to find the median).\textbackslash n\textbackslash n3. **Partitioning:**\textbackslash n\  \ - In each iteration, `i` divides `nums1`, and `j` divides `nums2` such that the total number of elements on the left side is `half\_len`.\textbackslash n\textbackslash n4. **Adjusting the Search Range:**\textbackslash n\  \ - If `nums2[j - 1] > nums1[i]`, it means `i` is too small, so we need to move the partition point in `nums1` to the right (`imin = i + 1`).\textbackslash n\  \ - If `nums1[i - 1] > nums2[j]`, `i` is too large, so we move it to the left (`imax = i - 1`).\textbackslash n\textbackslash n5. **Finding the Median:**\textbackslash n\  \ - When the correct partition is found (`i` is in the right position), we find:\textbackslash n\  \ - `max\_left`: The maximum element on the left side of the partition.\textbackslash n\  \ - `min\_right`: The minimum element on the right side of the partition.\textbackslash n\  \ - If the total number of elements is odd, `max\_left` is the median.\textbackslash n\  \ - If even, the median is the average of `max\_left` and `min\_right`.\textbackslash n\textbackslash n**Time Complexity:** O(log(min(m, n))) because we are performing binary search on the shorter array.\textbackslash n\textbackslash n**Space Complexity:** O(1) as we are only using a constant amount of extra space for variables.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\ttiny \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\ttiny You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\ttiny }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny Judgment} \stt{\ttiny (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides an example usage of the function, which is helpful for understanding how to use it. The assistant's code is a different implementation than the reference answer, but it achieves the same result and meets the same complexity requirements. \newline However, the assistant's answer does not address the user's original question about achieving O(n) time complexity. The assistant should have clarified that it's not possible to find the median of two sorted arrays of different sizes with O(1) space complexity and O(n) time complexity, as stated in the reference answer. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722737514.2011044}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny The assistant's answer is correct and provides a detailed explanation of the code. The assistant correctly states that the time complexity is O(log(min(m, n))) and the space complexity is O(1), which aligns with the reference answer. The assistant also provides a step-by-step explanation of the code, which is very helpful for understanding the logic behind the solution. The assistant's code is also correct and will correctly find the median of two sorted arrays of different sizes. Therefore, there are no corrections needed for the assistant's response.\newline\newline Rating: [[10]], "score": 10, "turn": 1, "tstamp": 1722846533.772981}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-1}
\end{table}

==> appp/tab-gen-2.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Imagine you are writing a blog post comparing two popular smartphone models. Develop an outline for the blog post, including key points and subheadings to effectively compare and contrast the features, performance, and user experience of the two models. Please answer in fewer than 200 words.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize \#\# Smartphone Showdown: [Model A] vs. [Model B]\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce the two smartphone models being compared, highlighting their popularity and target audience.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, and display technology (e.g., OLED, LCD).\textbackslash n* Design aesthetics and user preferences.\textbackslash n\textbackslash n**III. Performance and Specs**\textbackslash n* Processor, RAM, and storage comparison.\textbackslash n* Benchmark scores and real-world performance analysis.\textbackslash n* Battery life and charging capabilities.\textbackslash n\textbackslash n**IV. Camera Capabilities**\textbackslash n* Rear and front camera specs (megapixels, aperture, features).\textbackslash n* Image quality comparison in various lighting conditions.\textbackslash n* Video recording capabilities.\textbackslash n\textbackslash n**V. Software and User Experience**\textbackslash n* Operating system and user interface comparison.\textbackslash n* App ecosystem and availability.\textbackslash n* Software features and customization options.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare the price points of both models.\textbackslash n* Analyze the value proposition based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and similarities.\textbackslash n* Recommend the best phone for specific user profiles (e.g., budget-conscious, photography enthusiasts, gamers).}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize \#\# iPhone 14 Pro vs. Samsung Galaxy S23: Which Flagship Reigns Supreme?\textbackslash n\textbackslash n**I. Introduction**\textbackslash n* Briefly introduce both smartphones and their position in the market.\textbackslash n* State the purpose of the comparison: to help readers decide which phone best suits their needs.\textbackslash n\textbackslash n**II. Design and Display**\textbackslash n* Physical dimensions, weight, and build quality comparison.\textbackslash n* Screen size, resolution, refresh rate, and display technology (OLED vs. Super AMOLED).\textbackslash n* Design aesthetics and unique features (e.g., notch vs. punch-hole, color options).\textbackslash n\textbackslash n**III. Performance and Camera**\textbackslash n* Processor comparison (Apple A16 Bionic vs. Snapdragon 8 Gen 2).\textbackslash n* RAM and storage options.\textbackslash n* Camera specs: megapixels, lens types, aperture, and special features (e.g., telephoto, macro).\textbackslash n* Image quality comparison based on sample photos and user reviews.\textbackslash n\textbackslash n**IV. Software and User Experience**\textbackslash n* Operating systems: iOS 16 vs. Android 13.\textbackslash n* User interface comparison: intuitiveness, customization options, and app ecosystems.\textbackslash n* Special features: Face ID vs. in-display fingerprint sensor, voice assistants.\textbackslash n\textbackslash n**V. Battery Life and Charging**\textbackslash n* Battery capacity and real-world usage comparison.\textbackslash n* Fast charging speeds and wireless charging capabilities.\textbackslash n\textbackslash n**VI. Price and Value**\textbackslash n* Compare starting prices and different storage configurations.\textbackslash n* Assess the overall value for money based on features and performance.\textbackslash n\textbackslash n**VII. Conclusion**\textbackslash n* Summarize the key differences and strengths of each phone.\textbackslash n* Recommend the best phone for specific user types (e.g., photography enthusiasts, gamers, budget-conscious consumers).}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize Take your previous response and rephrase it as a limerick.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize Two phones, a showdown so grand,\textbackslash n[Model A] and [Model B], hand in hand.\textbackslash nDesign, specs, and price,\textbackslash nWe'll analyze nice,\textbackslash nTo help you choose, understand?\textbackslash n\textbackslash nLet me know if you'd like me to try filling in the bracketed parts with specific model names!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize \textbackslash nTwo phones, a Pro and a Galaxy,\textbackslash nFor flagships, they truly are spacy.\textbackslash nWith cameras and screens,\textbackslash nAnd processors keen,\textbackslash nWhich one wins? Read on, and be savvy! \textbackslash nLet me know if you'd like another limerick!}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The user asked the assistant to rephrase the previous response, which was a detailed outline for a blog post, into a limerick. The assistant successfully did so, maintaining the essence of the original response in a limerick format. The assistant also offered to further customize the limerick by filling in the bracketed parts with specific model names, showing a willingness to provide additional detail if needed. However, the limerick does not fully capture the depth and detail of the original response, which is understandable given the constraints of the limerick format. \newline\newline Rating: [[8]], "score": 8, "turn": 2, "tstamp": 1722737024.0327556}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is creative and relevant to the user's request. The assistant successfully rephrased the previous response, which was a detailed outline for a blog post comparing two smartphone models, into a limerick. The limerick is playful and engaging, and it maintains the essence of the original response, which is to compare the two phones and help the reader make an informed decision. The assistant also offers to create another limerick if the user wants, showing a willingness to continue the interaction. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846542.9437995}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-2}
\end{table}

==> appp/tab-gen-3.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize Each problem consists of three statements. Based on the first two statements, the third statement may be true, false, or uncertain.\textbackslash n1. Oranges cost more than apples.\textbackslash n2. Oranges cost less than bananas.\textbackslash n3. Bananas cost more than apples and bananas cost more than orange.\textbackslash nIf the first two statements are true, then the third statement is?}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nStatement 3 is **partially true**.\textbackslash n\textbackslash n* The part "Bananas > Apples" is true based on our price order.\textbackslash n* The part "Bananas > Oranges" is also true based on our price order.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize Here's how to break down the logic:\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples (Oranges cost more than apples)\textbackslash n* **Statement 2:** Oranges < Bananas (Oranges cost less than bananas)\textbackslash n\textbackslash nThese statements tell us that bananas are the most expensive, then oranges, and apples are the least expensive.\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nSince bananas are indeed more expensive than both apples and oranges, statement 3 is **true**.\textbackslash n\textbackslash n\textbackslash nLet me know if you'd like to try another one!}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize If the third statement is true. Is the first statement true, false, or uncertain? Please explain.}
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, the first statement is **false**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** States that bananas cost more than both apples AND oranges.\textbackslash n\textbackslash nThis means the price order is: Bananas > Oranges > Apples.\textbackslash n\textbackslash n* **Statement 1:** States that oranges cost more than apples.\textbackslash n\textbackslash nIf bananas are the most expensive, and oranges are second, then oranges cannot be more expensive than apples.\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other logic puzzles!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize If the third statement is true, then the first statement is **uncertain**.\textbackslash n\textbackslash nHere's why:\textbackslash n\textbackslash n* **Statement 3:** Bananas > Apples AND Bananas > Oranges\textbackslash n\textbackslash nThis tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges.\textbackslash n\textbackslash n* **Statement 1:** Oranges > Apples\textbackslash n\textbackslash nThis statement claims oranges are more expensive than apples.\textbackslash n\textbackslash nStatement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is incorrect. The assistant states that if the third statement is true, the first statement is false. However, the third statement only establishes that bananas cost more than both apples and oranges. It does not provide information about the relative costs of apples and oranges. Therefore, the first statement could be true (if oranges cost more than apples), false (if oranges cost less than apples), or uncertain (if oranges and apples cost the same). The assistant's explanation is flawed because it incorrectly assumes that the order of costs must be Bananas > Oranges > Apples, when in fact the order could also be Bananas > Apples = Oranges or Bananas > Apples > Oranges. \textbackslash n\textbackslash nCorrected Assistant's Answer: If the third statement is true, then bananas cost more than apples and bananas cost more than oranges. This means that oranges could still cost more than apples, making the first statement true. However, it's also possible that oranges and apples have the same cost, which would make the first statement false. Therefore, based on the third statement alone, the first statement is uncertain.\newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737017.2808955}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize The assistant's response is correct and helpful. The assistant explains that the first statement is uncertain if the third statement is true, which aligns with the reference answer. The assistant provides a clear explanation of why this is the case, stating that the third statement doesn't contradict the first statement, but it also doesn't confirm it. Therefore, the assistant's response is accurate and informative.\textbackslash n\textbackslash nThe assistant's response: "If the third statement is true, then the first statement is **uncertain**. Here's why: Statement 3: Bananas > Apples AND Bananas > Oranges. This tells us bananas are the most expensive, but it doesn't explicitly state the relative prices of apples and oranges. Statement 1: Oranges > Apples. This statement claims oranges are more expensive than apples. Statement 3 doesn't contradict statement 1, but it also doesn't confirm it. It's possible that oranges *are* more expensive than apples, but statement 3 alone doesn't give us enough information to be sure.\newline\newline Rating: [[10]], "score": 10, "turn": 2, "tstamp": 1722846527.2339694}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> appp/tab-gen-4.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\tiny You are given two sorted lists of size m and n. Implement a function to find the kth smallest element in the union of the two lists with linear complexity.}
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\tiny ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\  \ """\textbackslash n\  \ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\  \ Args:\textbackslash n\  \  list1: The first sorted list.\textbackslash n\  \  list2: The second sorted list.\textbackslash n\  \  k: The desired kth smallest element.\textbackslash n\textbackslash n\  \ Returns:\textbackslash n\  \  The kth smallest element in the union of the two lists.\textbackslash n\  \ """\textbackslash n\textbackslash n\  \ m, n = len(list1), len(list2)\textbackslash n\  \ i, j = 0, 0\textbackslash n\  \ min\_heap = []\  \textbackslash n\textbackslash n\ \# Build a min-heap with the first elements of both lists\textbackslash n\  \ for x in range(min(m, n)):\textbackslash n\  \  heapq.heappush(min\_heap, (list1[x], x, 0))\ \# (value, list\_index, position\_in\_list)\textbackslash n\  \  heapq.heappush(min\_heap, (list2[x], x, 1))\textbackslash n\textbackslash n\ \# Extract k smallest elements from the heap\textbackslash n\  \ for \_ in range(k - 1):\textbackslash n\  \  \_, \_, \_ = heapq.heappop(min\_heap)\textbackslash n\textbackslash n\ \# The top element of the heap is the kth smallest\textbackslash n\  \ return heapq.heappop(min\_heap)[0]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\  \ - `m` and `n` store the lengths of the input lists.\textbackslash n\  \ - `i` and `j` are pointers to track the current position in each list.\textbackslash n\  \ - `min\_heap` is a min-heap used to efficiently store and retrieve the smallest elements encountered so far.\textbackslash n\textbackslash n2. **Building the Min-Heap:**\textbackslash n\  \ - The code iterates through the first `min(m, n)` elements of both lists.\textbackslash n\  \ - For each element, a tuple `(value, list\_index, position\_in\_list)` is pushed onto the `min\_heap`. This tuple helps us keep track of the element's value, the list it belongs to, and its original position.\textbackslash n\textbackslash n3. **Extracting k-1 Smallest Elements:**\textbackslash n\  \ - The `for` loop runs `k - 1` times, effectively extracting the `k-1` smallest elements from the `min\_heap`.\textbackslash n\textbackslash n4. **Finding the kth Smallest:**\textbackslash n\  \ - After the loop, the top element of the `min\_heap` contains the `k`th smallest element.\textbackslash n\  \ - `heapq.heappop(min\_heap)` removes and returns this element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- Building the min-heap: O(m + n)\textbackslash n- Extracting k-1 elements: O(k * log(k))\textbackslash n- Overall: **O(m + n + k * log(k))**, which is approximately **O(m + n)** since `k` is usually much smaller than `m + n`.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any other questions!}
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\tiny ```python\textbackslash n\textbackslash def find\_kth\_smallest(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists.\textbackslash n\textbackslash n\ Args:\textbackslash n\  \ list1: The first sorted list.\textbackslash n\  \ list2: The second sorted list.\textbackslash n\  \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\  \ The kth smallest element in the union of the lists.\textbackslash n\ """\textbackslash n\textbackslash n\ i = 0\  \# Index for list1\textbackslash n\ j = 0\ \# Index for list2\textbackslash n\ merged = []\  \# Store the merged elements\textbackslash n\textbackslash n\ while i < len(list1) and j < len(list2):\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list1\textbackslash n\ while i < len(list1):\textbackslash n\  \ merged.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\textbackslash n\ \# Add any remaining elements from list2\textbackslash n\ while j < len(list2):\textbackslash n\  \ merged.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\textbackslash n\ return merged[k - 1]\  \# Return the kth element (index k-1)\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash n\textbackslash nkth\_smallest = find\_kth\_smallest(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `i` and `j` are index pointers for `list1` and `list2` respectively, starting at 0.\textbackslash n\ - `merged` is an empty list to store the merged sorted elements.\textbackslash n\textbackslash n2. **Merging:**\textbackslash n\ - The `while` loop continues as long as both `i` and `j` are within the bounds of their respective lists.\textbackslash n\ - In each iteration, it compares the elements at `list1[i]` and `list2[j]`.\textbackslash n\ - The smaller element is appended to `merged`, and the corresponding index (`i` or `j`) is incremented.\textbackslash n\textbackslash n3. **Adding Remaining Elements:**\textbackslash n\ - After one list is exhausted, the remaining elements from the other list are directly appended to `merged`.\textbackslash n\textbackslash n4. **Returning the kth Element:**\textbackslash n\ - Finally, `merged[k - 1]` is returned, which represents the kth smallest element in the union (remember that list indices start from 0).\textbackslash n\textbackslash n**Linear Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through each element in both lists at most once during the merging process.\textbackslash n- The time complexity is therefore O(m + n), which is linear in the total number of elements (m + n), making it efficient for large lists.
}
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\tiny 2nd-turn prompt:} 
% % ------- Put User Q2 Here ---------
% \texttt{\tiny \hspace{-2pt}Does there exist algorithm with better time complexity?If so, implement it.}
% % ------- Put User Q2 Here ---------
% } 
% \\ \midrule
% % ========================================================



% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 



% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
% \texttt{\tiny You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q2 Here ---------
% \texttt{\tiny }
% % ------- Put DPO-eva response to Q2 Here ---------
% \end{tabular} \\ 
% \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\tiny Judgment} \stt{\tiny (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\tiny Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is incorrect. The user asked for a solution with linear complexity, but the assistant provided a solution with a time complexity of O(m + n + k * log(k)), which is not linear. The assistant's solution uses a min-heap, which is not necessary and adds unnecessary complexity to the solution. \newline\newline Rating: [[2]], "score": 2, "turn": 1, "tstamp": 1722737030.6411152}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\tiny The assistant's answer is correct and helpful. It provides a Python function that implements the two-pointer approach to find the kth smallest element in the union of two sorted lists. The assistant's function is slightly different from the reference, but it achieves the same goal. The assistant's function merges the two lists into a new list and then returns the kth element from the merged list. The assistant also provides a detailed explanation of how the function works and confirms that the time complexity is linear, which is what the user asked for. However, the assistant's function uses extra space to store the merged list, which is not necessary and not as efficient as the reference. \newline \newline Rating: [[8]], "score": 8, "turn": 1, "tstamp": 1722846543.867601}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-4}
\end{table}

==> appp/tab-gen-5.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  You are absolutely right! There's a more efficient algorithm with a time complexity of **O(m + n)** without using a heap.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ """\textbackslash n\ Finds the kth smallest element in the union of two sorted lists\textbackslash n\ with O(m + n) time complexity.\textbackslash n\textbackslash n\ Args:\textbackslash n\ list1: The first sorted list.\textbackslash n\ list2: The second sorted list.\textbackslash n\ k: The desired kth smallest element.\textbackslash n\textbackslash n\ Returns:\textbackslash n\ The kth smallest element in the union of the two lists.\textbackslash n\ """\textbackslash n\ m, n = len(list1), len(list2)\textbackslash n\ i, j = 0, 0\textbackslash n\ result = []\textbackslash n\textbackslash n\ \# Merge the lists while keeping track of the kth smallest\textbackslash n\ while len(result) < k:\textbackslash n\ if i < m and j < n:\textbackslash n\  \ if list1[i] <= list2[j]:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\  \ else:\textbackslash n\  \ result.append(list2[j])\textbackslash n\  \ j += 1\textbackslash n\ elif i < m:\textbackslash n\  \ result.append(list1[i])\textbackslash n\  \ i += 1\textbackslash n\ else:\textbackslash n\ result.append(list2[j])\textbackslash n\ j += 1\textbackslash n\textbackslash n\ return result[k - 1]\textbackslash n\textbackslash n\# Example usage:\textbackslash nlist1 = [2, 5, 8, 12]\textbackslash nlist2 = [1, 3, 7, 9, 10]\textbackslash nk = 5\textbackslash nkth\_smallest = find\_kth\_smallest\_optimized(list1, list2, k)\textbackslash nprint(f"The \{k\}th smallest element is: \{kth\_smallest\}")\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Initialization:**\textbackslash n\ - `m` and `n` store the lengths of the lists.\textbackslash n\ - `i` and `j` are pointers for `list1` and `list2`, respectively.\textbackslash n\ - `result` is a list to store the merged and sorted elements.\textbackslash n\textbackslash n2. **Merging and Tracking:**\textbackslash n\ - The `while` loop continues until `k` elements are in the `result` list.\textbackslash n\ - In each iteration, it compares the current elements from `list1` and `list2`.\textbackslash n\ - The smaller element is appended to `result`, and the corresponding pointer (`i` or `j`) is incremented.\textbackslash n\ - If one list is exhausted, the remaining elements from the other list are appended to `result`.\textbackslash n\textbackslash n3. **Returning the kth Smallest:**\textbackslash n\ - Finally, `result[k - 1]` contains the `k`th smallest element.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The algorithm iterates through both lists once, resulting in a time complexity of **O(m + n)**.\textbackslash n\textbackslash n\textbackslash n\textbackslash nLet me know if you have any more questions!}
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  You are right to ask! While the previous algorithm has linear time complexity, we can achieve an even better solution with **O(log(min(m, n)))** time complexity using a slightly more sophisticated approach.\textbackslash n\textbackslash nThe key idea is to leverage the sorted nature of the lists and use a **binary search** strategy.\textbackslash n\textbackslash nHere's the implementation:\textbackslash n\textbackslash n\textbackslash\#\#\textbackslash npython\textbackslash n\textbackslash def find\_kth\_smallest\_optimized(list1, list2, k):\textbackslash n\ \ """\textbackslash n\ \ Finds the kth smallest element in the union of two sorted lists with O(log(min(m, n))) time complexity.\textbackslash n\textbackslash n\ \ Args:\textbackslash n\ \ list1: The first sorted list.\textbackslash n\ \ list2: The second sorted list.\textbackslash n\ \ k: The desired rank of the smallest element.\textbackslash n\textbackslash n\ \ Returns:\textbackslash n\ \ The kth smallest element in the union of the lists.\textbackslash n\ \ """\textbackslash n\ \ m, n = len(list1), len(list2)\textbackslash n\ \ if m > n:\textbackslash n\ \ list1, list2, m, n = list2, list1, n, m\ \# Ensure list1 is the shorter one\textbackslash n\textbackslash n\ \ left, right = 0, m\textbackslash n\ \ while left <= right:\textbackslash n\ \ partitionX = (left + right) // 2\textbackslash n\ \ partitionY = k - partitionX\textbackslash n\textbackslash n\ \ maxLeftX = list1[partitionX - 1] if partitionX > 0 else float('-inf')\textbackslash n\ \ minRightX = list1[partitionX] if partitionX < m else float('inf')\textbackslash n\textbackslash n\ \ maxLeftY = list2[partitionY - 1] if partitionY > 0 else float('-inf')\textbackslash n\ \ minRightY = list2[partitionY] if partitionY < n else float('inf')\textbackslash n\textbackslash n\ \ if maxLeftX <= minRightY and maxLeftY <= minRightX:\textbackslash n\ if partitionX == 0:\textbackslash n\ \ return list2[partitionY - 1]\textbackslash n\ elif partitionY == 0:\textbackslash n\ \ return list1[partitionX - 1]\textbackslash n\ else:\textbackslash n\ \ return max(list1[partitionX - 1], list2[partitionY - 1])\textbackslash n\ \ elif maxLeftX > minRightY:\textbackslash n\ right = partitionX - 1\ \# Too many elements on the right side of list1\textbackslash n\ \ else:\textbackslash n\ left = partitionX + 1\ \# Too many elements on the right side of list2\textbackslash n\textbackslash n\textbackslash n**Explanation:**\textbackslash n\textbackslash n1. **Shorten Lists:** If `list1` is longer than `list2`, swap them to ensure `list1` is always the shorter one. This simplifies the logic.\textbackslash n\textbackslash n2. **Binary Search:**\textbackslash n\ \ - `left` and `right` pointers define the search space within `list1`.\textbackslash n\ \ - `partitionX` is the middle point in `list1`, and `partitionY` is calculated to divide the remaining elements in `list2` such that `partitionX + partitionY = k`.\textbackslash n\ \ - `maxLeftX`, `minRightX`, `maxLeftY`, and `minRightY` represent the largest element to the left and smallest element to the right of the partitions in both lists.\textbackslash n\textbackslash n3. **Comparison and Adjustment:**\textbackslash n\ \ - If the `maxLeftX` is less than or equal to `minRightY` and `maxLeftY` is less than or equal to `minRightX`, it means the kth smallest element lies within the current partitions. We return the larger of `maxLeftX` and `maxLeftY`.\textbackslash n\ \ - If `maxLeftX` is greater than `minRightY`, it indicates that we need to search in the left subarray of `list1` (i.e., decrease `right`).\textbackslash n\ \ - Otherwise, we search in the right subarray of `list1` (i.e., increase `left`).\textbackslash n\textbackslash n4. **Termination:** The binary search continues until `left` crosses `right`, indicating the correct partition has been found.\textbackslash n\textbackslash n**Time Complexity:**\textbackslash n\textbackslash n- The binary search divides the search space in half at each step.\textbackslash n- Therefore, the time complexity is O(log(min(m, n))), which is significantly faster than linear time for large lists where one list is much smaller than the other.
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's first response to the user's question is incorrect. The user asked for a function to find the kth smallest element in the union of two sorted lists with linear complexity. The assistant provided a function that uses a min-heap, which has a time complexity of O(m + n + k * log(k)). This is not linear complexity, as the user requested. The assistant's second response to the user's question is also incorrect. The user asked if there exists an algorithm with better time complexity than linear. The assistant provided a function that has a time complexity of O(m + n), which is linear, not better than linear. The assistant should have provided a function that uses a binary search approach, which has a time complexity of O(log(m) + log(n)), as the reference answer correctly does. \newline\newline Rating: [[2]], "score": 2, "turn": 2, "tstamp": 1722737031.5033472}
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  The assistant's response is correct and helpful. The assistant provided a Python function that uses a binary search approach to find the kth smallest element in the union of two sorted lists. The assistant also provided a detailed explanation of how the function works, including the time complexity of the function. The assistant's answer matches the reference answer in terms of the algorithm used and the explanation provided. The assistant also correctly identified that the binary search approach has a better time complexity than the linear approach. However, the assistant's code has a minor issue. The assistant's code does not handle the case when `k` is greater than the sum of the lengths of the two lists. In such a case, the code will raise an `IndexError`. This can be fixed by adding a check at the beginning of the function to return `None` if `k` is greater than the sum of the lengths of the two lists. \newline\newline Rating: [[9]], "score": 9, "turn": 2, "tstamp": 1722846556.6828268}
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-5}
\end{table}

==> appp/tab-gen-6.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% % ========================================================
% \rowcolor{lightgray!16}
% \multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  1st-turn prompt:} 
% % ------- Put User Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put User Q1 Here ---------
% } \\ \midrule
% % ========================================================


% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
% \end{tabular} &

% \begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
% \end{tabular} \\ 


% ========================================================
% \begin{tabular}[c]{@{}p{\linewidth}@{}}
% % ------- Put  DPO response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put  DPO response to Q1 Here ---------
% \end{tabular} &


% \begin{tabular}[c]{@{}p{\linewidth}@{}} 
% % ------- Put DPO-eva response to Q1 Here ---------
% \texttt{\ttiny  }
% % ------- Put DPO-eva response to Q1 Here ---------
% \end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  2nd-turn prompt: Does there exist an algorithm with better time complexity? If so, implement it.} 
% ------- Put User Q2 Here ---------
\texttt{\ttiny  }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\ttiny  
}
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\ttiny  Judgment} \stt{\ttiny  (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\ttiny  Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\ttiny  }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen-6}
\end{table}

==> appp/tab-gen-script.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\scriptsize }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize 2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\scriptsize }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================


% ========================================================
\rowcolor{lightgray!16}
\multicolumn{2}{p{\textwidth}}{\sbt{\scriptsize Judgment} \stt{\scriptsize (by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{\scriptsize Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put  DPO judgment to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva judgment to Q2 Here ---------
\texttt{\scriptsize }
% ------- Put DPO-eva judgment to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> appp/tab-gen.tex <==
\begin{table}[H]
\centering
\resizebox{.8\textwidth}{!}{%
\begin{tabular}{@{}p{0.5\textwidth} p{0.5\textwidth}@{}}
\toprule

% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{1st-turn prompt:} 
% ------- Put User Q1 Here ---------
\texttt{\small }
% ------- Put User Q1 Here ---------
} \\ \midrule
% ========================================================


\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q1 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q1 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q1 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q1 Here ---------
\end{tabular} \\ \midrule
% ========================================================


% ========================================================
\multicolumn{2}{p{\textwidth}}{\sbt{2nd-turn prompt:} 
% ------- Put User Q2 Here ---------
\texttt{\small }
% ------- Put User Q2 Here ---------
} 
\\ \midrule
% ========================================================



\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Answer from gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 



% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\midrule
% ========================================================



\multicolumn{2}{p{\textwidth}}{\sbt{Judgment} \stt{(by gpt-4)}} \\ \midrule

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo}\\ 
\end{tabular} &

\begin{tabular}[c]{@{}p{\linewidth}@{}}\sbt{Judgment for gemma-2-9b-it-dpo-eva}\\
\end{tabular} \\ 


% ========================================================
\begin{tabular}[c]{@{}p{\linewidth}@{}}
% ------- Put  DPO response to Q2 Here ---------
\texttt{\small }
% ------- Put  DPO response to Q2 Here ---------
\end{tabular} &


\begin{tabular}[c]{@{}p{\linewidth}@{}} 
% ------- Put DPO-eva response to Q2 Here ---------
\texttt{\small }
% ------- Put DPO-eva response to Q2 Here ---------
\end{tabular} \\ 
\bottomrule
% ========================================================

\end{tabular}%
}
\caption{(Continued) comparison of model generations on examples from MT-Bench.}
\label{tab:gen}
\end{table}

==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> fancyhdr.tex <==
% fancyhdr.sty version 3.2
% Fancy headers and footers for LaTeX.
% Piet van Oostrum, 
% Dept of Computer and Information Sciences, University of Utrecht,
% Padualaan 14, P.O. Box 80.089, 3508 TB Utrecht, The Netherlands
% Telephone: +31 30 2532180. Email: piet@cs.uu.nl
% ========================================================================
% LICENCE:
% This file may be distributed under the terms of the LaTeX Project Public
% License, as described in lppl.txt in the base LaTeX distribution.
% Either version 1 or, at your option, any later version.
% ========================================================================
% MODIFICATION HISTORY:
% Sep 16, 1994
% version 1.4: Correction for use with \reversemargin
% Sep 29, 1994:
% version 1.5: Added the \iftopfloat, \ifbotfloat and \iffloatpage commands
% Oct 4, 1994:
% version 1.6: Reset single spacing in headers/footers for use with
% setspace.sty or doublespace.sty
% Oct 4, 1994:
% version 1.7: changed \let\@mkboth\markboth to
% \def\@mkboth{\protect\markboth} to make it more robust
% Dec 5, 1994:
% version 1.8: corrections for amsbook/amsart: define \@chapapp and (more
% importantly) use the \chapter/sectionmark definitions from ps@headings if
% they exist (which should be true for all standard classes).
% May 31, 1995:
% version 1.9: The proposed \renewcommand{\headrulewidth}{\iffloatpage...
% construction in the doc did not work properly with the fancyplain style. 
% June 1, 1995:
% version 1.91: The definition of \@mkboth wasn't restored on subsequent
% \pagestyle{fancy}'s.
% June 1, 1995:
% version 1.92: The sequence \pagestyle{fancyplain} \pagestyle{plain}
% \pagestyle{fancy} would erroneously select the plain version.
% June 1, 1995:
% version 1.93: \fancypagestyle command added.
% Dec 11, 1995:
% version 1.94: suggested by Conrad Hughes <chughes@maths.tcd.ie>
% CJCH, Dec 11, 1995: added \footruleskip to allow control over footrule
% position (old hardcoded value of .3\normalbaselineskip is far too high
% when used with very small footer fonts).
% Jan 31, 1996:
% version 1.95: call \@normalsize in the reset code if that is defined,
% otherwise \normalsize.
% this is to solve a problem with ucthesis.cls, as this doesn't
% define \@currsize. Unfortunately for latex209 calling \normalsize doesn't
% work as this is optimized to do very little, so there \@normalsize should
% be called. Hopefully this code works for all versions of LaTeX known to
% mankind.  
% April 25, 1996:
% version 1.96: initialize \headwidth to a magic (negative) value to catch
% most common cases that people change it before calling \pagestyle{fancy}.
% Note it can't be initialized when reading in this file, because
% \textwidth could be changed afterwards. This is quite probable.
% We also switch to \MakeUppercase rather than \uppercase and introduce a
% \nouppercase command for use in headers. and footers.
% May 3, 1996:
% version 1.97: Two changes:
% 1. Undo the change in version 1.8 (using the pagestyle{headings} defaults
% for the chapter and section marks. The current version of amsbook and
% amsart classes don't seem to need them anymore. Moreover the standard
% latex classes don't use \markboth if twoside isn't selected, and this is
% confusing as \leftmark doesn't work as expected.
% 2. include a call to \ps@empty in ps@@fancy. This is to solve a problem
% in the amsbook and amsart classes, that make global changes to \topskip,
% which are reset in \ps@empty. Hopefully this doesn't break other things.
% May 7, 1996:
% version 1.98:
% Added % after the line  \def\nouppercase
% May 7, 1996:
% version 1.99: This is the alpha version of fancyhdr 2.0
% Introduced the new commands \fancyhead, \fancyfoot, and \fancyhf.
% Changed \headrulewidth, \footrulewidth, \footruleskip to
% macros rather than length parameters, In this way they can be
% conditionalized and they don't consume length registers. There is no need
% to have them as length registers unless you want to do calculations with
% them, which is unlikely. Note that this may make some uses of them
% incompatible (i.e. if you have a file that uses \setlength or \xxxx=)
% May 10, 1996:
% version 1.99a:
% Added a few more % signs
% May 10, 1996:
% version 1.99b:
% Changed the syntax of \f@nfor to be resistent to catcode changes of :=
% Removed the [1] from the defs of \lhead etc. because the parameter is
% consumed by the \@[xy]lhead etc. macros.
% June 24, 1997:
% version 1.99c:
% corrected \nouppercase to also include the protected form of \MakeUppercase
% \global added to manipulation of \headwidth.
% \iffootnote command added.
% Some comments added about \@fancyhead and \@fancyfoot.
% Aug 24, 1998
% version 1.99d
% Changed the default \ps@empty to \ps@@empty in order to allow
% \fancypagestyle{empty} redefinition.
% Oct 11, 2000
% version 2.0
% Added LPPL license clause.
%
% A check for \headheight is added. An errormessage is given (once) if the
% header is too large. Empty headers don't generate the error even if
% \headheight is very small or even 0pt. 
% Warning added for the use of 'E' option when twoside option is not used.
% In this case the 'E' fields will never be used.
%
% Mar 10, 2002
% version 2.1beta
% New command: \fancyhfoffset[place]{length}
% defines offsets to be applied to the header/footer to let it stick into
% the margins (if length > 0).
% place is like in fancyhead, except that only E,O,L,R can be used.
% This replaces the old calculation based on \headwidth and the marginpar
% area.
% \headwidth will be dynamically calculated in the headers/footers when
% this is used.
%
% Mar 26, 2002
% version 2.1beta2
% \fancyhfoffset now also takes h,f as possible letters in the argument to
% allow the header and footer widths to be different.
% New commands \fancyheadoffset and \fancyfootoffset added comparable to
% \fancyhead and \fancyfoot.
% Errormessages and warnings have been made more informative.
%
% Dec 9, 2002
% version 2.1
% The defaults for \footrulewidth, \plainheadrulewidth and
% \plainfootrulewidth are changed from \z@skip to 0pt. In this way when
% someone inadvertantly uses \setlength to change any of these, the value
% of \z@skip will not be changed, rather an errormessage will be given.

% March 3, 2004
% Release of version 3.0

% Oct 7, 2004
% version 3.1
% Added '\endlinechar=13' to \fancy@reset to prevent problems with
% includegraphics in header when verbatiminput is active.

% March 22, 2005
% version 3.2
% reset \everypar (the real one) in \fancy@reset because spanish.ldf does
% strange things with \everypar between << and >>.

\def\ifancy@mpty#1{\def\temp@a{#1}\ifx\temp@a\@empty}

\def\fancy@def#1#2{\ifancy@mpty{#2}\fancy@gbl\def#1{\leavevmode}\else
                                   \fancy@gbl\def#1{#2\strut}\fi}

\let\fancy@gbl\global

\def\@fancyerrmsg#1{%
        \ifx\PackageError\undefined
        \errmessage{#1}\else
        \PackageError{Fancyhdr}{#1}{}\fi}
\def\@fancywarning#1{%
        \ifx\PackageWarning\undefined
        \errmessage{#1}\else
        \PackageWarning{Fancyhdr}{#1}{}\fi}

% Usage: \@forc \var{charstring}{command to be executed for each char}
% This is similar to LaTeX's \@tfor, but expands the charstring.

\def\@forc#1#2#3{\expandafter\f@rc\expandafter#1\expandafter{#2}{#3}}
\def\f@rc#1#2#3{\def\temp@ty{#2}\ifx\@empty\temp@ty\else
                                    \f@@rc#1#2\f@@rc{#3}\fi}
\def\f@@rc#1#2#3\f@@rc#4{\def#1{#2}#4\f@rc#1{#3}{#4}}

% Usage: \f@nfor\name:=list\do{body}
% Like LaTeX's \@for but an empty list is treated as a list with an empty
% element

\newcommand{\f@nfor}[3]{\edef\@fortmp{#2}%
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}}

% Usage: \def@ult \cs{defaults}{argument}
% sets \cs to the characters from defaults appearing in argument
% or defaults if it would be empty. All characters are lowercased.

\newcommand\def@ult[3]{%
    \edef\temp@a{\lowercase{\edef\noexpand\temp@a{#3}}}\temp@a
    \def#1{}%
    \@forc\tmpf@ra{#2}%
        {\expandafter\if@in\tmpf@ra\temp@a{\edef#1{#1\tmpf@ra}}{}}%
    \ifx\@empty#1\def#1{#2}\fi}
% 
% \if@in <char><set><truecase><falsecase>
%
\newcommand{\if@in}[4]{%
    \edef\temp@a{#2}\def\temp@b##1#1##2\temp@b{\def\temp@b{##1}}%
    \expandafter\temp@b#2#1\temp@b\ifx\temp@a\temp@b #4\else #3\fi}

\newcommand{\fancyhead}{\@ifnextchar[{\f@ncyhf\fancyhead h}%
                                     {\f@ncyhf\fancyhead h[]}}
\newcommand{\fancyfoot}{\@ifnextchar[{\f@ncyhf\fancyfoot f}%
                                     {\f@ncyhf\fancyfoot f[]}}
\newcommand{\fancyhf}{\@ifnextchar[{\f@ncyhf\fancyhf{}}%
                                   {\f@ncyhf\fancyhf{}[]}}

% New commands for offsets added

\newcommand{\fancyheadoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyheadoffset h}%
                                           {\f@ncyhfoffs\fancyheadoffset h[]}}
\newcommand{\fancyfootoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyfootoffset f}%
                                           {\f@ncyhfoffs\fancyfootoffset f[]}}
\newcommand{\fancyhfoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyhfoffset{}}%
                                         {\f@ncyhfoffs\fancyhfoffset{}[]}}

% The header and footer fields are stored in command sequences with
% names of the form: \f@ncy<x><y><z> with <x> for [eo], <y> from [lcr]
% and <z> from [hf].

\def\f@ncyhf#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolcrhf,EOLCRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lcr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\fancy@def\csname
                      f@ncy\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}}

\def\f@ncyhfoffs#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolrhf,EOLRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\setlength\csname
                      f@ncyO@\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}%
     \fancy@setoffs}

% Fancyheadings version 1 commands. These are more or less deprecated,
% but they continue to work.

\newcommand{\lhead}{\@ifnextchar[{\@xlhead}{\@ylhead}}
\def\@xlhead[#1]#2{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#2}}
\def\@ylhead#1{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#1}}

\newcommand{\chead}{\@ifnextchar[{\@xchead}{\@ychead}}
\def\@xchead[#1]#2{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#2}}
\def\@ychead#1{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#1}}

\newcommand{\rhead}{\@ifnextchar[{\@xrhead}{\@yrhead}}
\def\@xrhead[#1]#2{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#2}}
\def\@yrhead#1{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#1}}

\newcommand{\lfoot}{\@ifnextchar[{\@xlfoot}{\@ylfoot}}
\def\@xlfoot[#1]#2{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#2}}
\def\@ylfoot#1{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#1}}

\newcommand{\cfoot}{\@ifnextchar[{\@xcfoot}{\@ycfoot}}
\def\@xcfoot[#1]#2{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#2}}
\def\@ycfoot#1{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#1}}

\newcommand{\rfoot}{\@ifnextchar[{\@xrfoot}{\@yrfoot}}
\def\@xrfoot[#1]#2{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#2}}
\def\@yrfoot#1{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#1}}

\newlength{\fancy@headwidth}
\let\headwidth\fancy@headwidth
\newlength{\f@ncyO@elh}
\newlength{\f@ncyO@erh}
\newlength{\f@ncyO@olh}
\newlength{\f@ncyO@orh}
\newlength{\f@ncyO@elf}
\newlength{\f@ncyO@erf}
\newlength{\f@ncyO@olf}
\newlength{\f@ncyO@orf}
\newcommand{\headrulewidth}{0.4pt}
\newcommand{\footrulewidth}{0pt}
\newcommand{\footruleskip}{.3\normalbaselineskip}

% Fancyplain stuff shouldn't be used anymore (rather
% \fancypagestyle{plain} should be used), but it must be present for
% compatibility reasons.

\newcommand{\plainheadrulewidth}{0pt}
\newcommand{\plainfootrulewidth}{0pt}
\newif\if@fancyplain \@fancyplainfalse
\def\fancyplain#1#2{\if@fancyplain#1\else#2\fi}

\headwidth=-123456789sp %magic constant

% Command to reset various things in the headers:
% a.o.  single spacing (taken from setspace.sty)
% and the catcode of ^^M (so that epsf files in the header work if a
% verbatim crosses a page boundary)
% It also defines a \nouppercase command that disables \uppercase and
% \Makeuppercase. It can only be used in the headers and footers.
\let\fnch@everypar\everypar% save real \everypar because of spanish.ldf
\def\fancy@reset{\fnch@everypar{}\restorecr\endlinechar=13
 \def\baselinestretch{1}%
 \def\nouppercase##1{{\let\uppercase\relax\let\MakeUppercase\relax
     \expandafter\let\csname MakeUppercase \endcsname\relax##1}}%
 \ifx\undefined\@newbaseline% NFSS not present; 2.09 or 2e
   \ifx\@normalsize\undefined \normalsize % for ucthesis.cls
   \else \@normalsize \fi
 \else% NFSS (2.09) present
  \@newbaseline%
 \fi}

% Initialization of the head and foot text.

% The default values still contain \fancyplain for compatibility.
\fancyhf{} % clear all
% lefthead empty on ``plain'' pages, \rightmark on even, \leftmark on odd pages
% evenhead empty on ``plain'' pages, \leftmark on even, \rightmark on odd pages
\if@twoside
  \fancyhead[el,or]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[er,ol]{\fancyplain{}{\sl\leftmark}}
\else
  \fancyhead[l]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[r]{\fancyplain{}{\sl\leftmark}}
\fi
\fancyfoot[c]{\rm\thepage} % page number

% Use box 0 as a temp box and dimen 0 as temp dimen. 
% This can be done, because this code will always
% be used inside another box, and therefore the changes are local.

\def\@fancyvbox#1#2{\setbox0\vbox{#2}\ifdim\ht0>#1\@fancywarning
  {\string#1 is too small (\the#1): ^^J Make it at least \the\ht0.^^J
    We now make it that large for the rest of the document.^^J
    This may cause the page layout to be inconsistent, however\@gobble}%
  \dimen0=#1\global\setlength{#1}{\ht0}\ht0=\dimen0\fi
  \box0}

% Put together a header or footer given the left, center and
% right text, fillers at left and right and a rule.
% The \lap commands put the text into an hbox of zero size,
% so overlapping text does not generate an errormessage.
% These macros have 5 parameters:
% 1. LEFTSIDE BEARING % This determines at which side the header will stick
%    out. When \fancyhfoffset is used this calculates \headwidth, otherwise
%    it is \hss or \relax (after expansion).
% 2. \f@ncyolh, \f@ncyelh, \f@ncyolf or \f@ncyelf. This is the left component.
% 3. \f@ncyoch, \f@ncyech, \f@ncyocf or \f@ncyecf. This is the middle comp.
% 4. \f@ncyorh, \f@ncyerh, \f@ncyorf or \f@ncyerf. This is the right component.
% 5. RIGHTSIDE BEARING. This is always \relax or \hss (after expansion).

\def\@fancyhead#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
  \@fancyvbox\headheight{\hbox
    {\rlap{\parbox[b]{\headwidth}{\raggedright#2}}\hfill
      \parbox[b]{\headwidth}{\centering#3}\hfill
      \llap{\parbox[b]{\headwidth}{\raggedleft#4}}}\headrule}}#5}

\def\@fancyfoot#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
    \@fancyvbox\footskip{\footrule
      \hbox{\rlap{\parbox[t]{\headwidth}{\raggedright#2}}\hfill
        \parbox[t]{\headwidth}{\centering#3}\hfill
        \llap{\parbox[t]{\headwidth}{\raggedleft#4}}}}}#5}

\def\headrule{{\if@fancyplain\let\headrulewidth\plainheadrulewidth\fi
    \hrule\@height\headrulewidth\@width\headwidth \vskip-\headrulewidth}}

\def\footrule{{\if@fancyplain\let\footrulewidth\plainfootrulewidth\fi
    \vskip-\footruleskip\vskip-\footrulewidth
    \hrule\@width\headwidth\@height\footrulewidth\vskip\footruleskip}}

\def\ps@fancy{%
\@ifundefined{@chapapp}{\let\@chapapp\chaptername}{}%for amsbook
%
% Define \MakeUppercase for old LaTeXen.
% Note: we used \def rather than \let, so that \let\uppercase\relax (from
% the version 1 documentation) will still work.
%
\@ifundefined{MakeUppercase}{\def\MakeUppercase{\uppercase}}{}%
\@ifundefined{chapter}{\def\sectionmark##1{\markboth
{\MakeUppercase{\ifnum \c@secnumdepth>\z@
 \thesection\hskip 1em\relax \fi ##1}}{}}%
\def\subsectionmark##1{\markright {\ifnum \c@secnumdepth >\@ne
 \thesubsection\hskip 1em\relax \fi ##1}}}%
{\def\chaptermark##1{\markboth {\MakeUppercase{\ifnum \c@secnumdepth>\m@ne
 \@chapapp\ \thechapter. \ \fi ##1}}{}}%
\def\sectionmark##1{\markright{\MakeUppercase{\ifnum \c@secnumdepth >\z@
 \thesection. \ \fi ##1}}}}%
%\csname ps@headings\endcsname % use \ps@headings defaults if they exist
\ps@@fancy
\gdef\ps@fancy{\@fancyplainfalse\ps@@fancy}%
% Initialize \headwidth if the user didn't
%
\ifdim\headwidth<0sp
%
% This catches the case that \headwidth hasn't been initialized and the
% case that the user added something to \headwidth in the expectation that
% it was initialized to \textwidth. We compensate this now. This loses if
% the user intended to multiply it by a factor. But that case is more
% likely done by saying something like \headwidth=1.2\textwidth. 
% The doc says you have to change \headwidth after the first call to
% \pagestyle{fancy}. This code is just to catch the most common cases were
% that requirement is violated.
%
    \global\advance\headwidth123456789sp\global\advance\headwidth\textwidth
\fi}
\def\ps@fancyplain{\ps@fancy \let\ps@plain\ps@plain@fancy}
\def\ps@plain@fancy{\@fancyplaintrue\ps@@fancy}
\let\ps@@empty\ps@empty
\def\ps@@fancy{%
\ps@@empty % This is for amsbook/amsart, which do strange things with \topskip
\def\@mkboth{\protect\markboth}%
\def\@oddhead{\@fancyhead\fancy@Oolh\f@ncyolh\f@ncyoch\f@ncyorh\fancy@Oorh}%
\def\@oddfoot{\@fancyfoot\fancy@Oolf\f@ncyolf\f@ncyocf\f@ncyorf\fancy@Oorf}%
\def\@evenhead{\@fancyhead\fancy@Oelh\f@ncyelh\f@ncyech\f@ncyerh\fancy@Oerh}%
\def\@evenfoot{\@fancyfoot\fancy@Oelf\f@ncyelf\f@ncyecf\f@ncyerf\fancy@Oerf}%
}
% Default definitions for compatibility mode:
% These cause the header/footer to take the defined \headwidth as width
% And to shift in the direction of the marginpar area

\def\fancy@Oolh{\if@reversemargin\hss\else\relax\fi}
\def\fancy@Oorh{\if@reversemargin\relax\else\hss\fi}
\let\fancy@Oelh\fancy@Oorh
\let\fancy@Oerh\fancy@Oolh

\let\fancy@Oolf\fancy@Oolh
\let\fancy@Oorf\fancy@Oorh
\let\fancy@Oelf\fancy@Oelh
\let\fancy@Oerf\fancy@Oerh

% New definitions for the use of \fancyhfoffset
% These calculate the \headwidth from \textwidth and the specified offsets.

\def\fancy@offsolh{\headwidth=\textwidth\advance\headwidth\f@ncyO@olh
                   \advance\headwidth\f@ncyO@orh\hskip-\f@ncyO@olh}
\def\fancy@offselh{\headwidth=\textwidth\advance\headwidth\f@ncyO@elh
                   \advance\headwidth\f@ncyO@erh\hskip-\f@ncyO@elh}

\def\fancy@offsolf{\headwidth=\textwidth\advance\headwidth\f@ncyO@olf
                   \advance\headwidth\f@ncyO@orf\hskip-\f@ncyO@olf}
\def\fancy@offself{\headwidth=\textwidth\advance\headwidth\f@ncyO@elf
                   \advance\headwidth\f@ncyO@erf\hskip-\f@ncyO@elf}

\def\fancy@setoffs{%
% Just in case \let\headwidth\textwidth was used
  \fancy@gbl\let\headwidth\fancy@headwidth
  \fancy@gbl\let\fancy@Oolh\fancy@offsolh
  \fancy@gbl\let\fancy@Oelh\fancy@offselh
  \fancy@gbl\let\fancy@Oorh\hss
  \fancy@gbl\let\fancy@Oerh\hss
  \fancy@gbl\let\fancy@Oolf\fancy@offsolf
  \fancy@gbl\let\fancy@Oelf\fancy@offself
  \fancy@gbl\let\fancy@Oorf\hss
  \fancy@gbl\let\fancy@Oerf\hss}

\newif\iffootnote
\let\latex@makecol\@makecol
\def\@makecol{\ifvoid\footins\footnotetrue\else\footnotefalse\fi
\let\topfloat\@toplist\let\botfloat\@botlist\latex@makecol}
\def\iftopfloat#1#2{\ifx\topfloat\empty #2\else #1\fi}
\def\ifbotfloat#1#2{\ifx\botfloat\empty #2\else #1\fi}
\def\iffloatpage#1#2{\if@fcolmade #1\else #2\fi}

\newcommand{\fancypagestyle}[2]{%
  \@namedef{ps@#1}{\let\fancy@gbl\relax#2\relax\ps@fancy}}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/algo-eva.tex <==
{
\noindent
\centering
\begin{minipage}{0.9\linewidth}
  \begin{algorithm}[H]
    \small
    
    \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
    \begin{algorithmic}[1]
    \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
    % , sample size of responses per prompt $n$ 
    \vspace{+3pt}

    \For{\textbf{iteration} $t = 1, 2, \ldots$}
        \vspace{+5pt}
        
        \LineComment{\textcolor{cgreen}{{\textbf{\texttt{creator step}}}}}
        
        \vspace{+5pt}
        % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t-1} \gets \calX_{t-1} \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}_i$ 
        \State \tb{\emph{estimate informativeness}:} \hspace{+18pt} $\mathcal{X}_{t-1} \gets \{ (\rvx_i, \textbf{\texttt{info}}(\rvx_i)) \mid \rvx_i \in \mathcal{X}_{t-1} \}$

        
        \vspace{+2pt}
        

        \Statex \hspace{+11pt}  \tb{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t-1}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t-1})}}$ 
        \vspace{+2.5pt}

        \Statex \hspace{+11pt} \tb{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t-1}^{\texttt{info}})}}$ 

        \vspace{+8pt}
        
         \LineComment{\textcolor{cred}{ \textbf{ \texttt{solver step} } }}
        
        \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 

        \Statex \hspace{+11pt} \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 

        \vspace{+2.5pt}
        
        \Statex \hspace{+11pt} \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}_{t} \leftarrow \boldsymbol{\theta}_{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
        \vspace{+5pt}
        
    \EndFor 
    \State \Return final solver policy $\pi_{\vtheta_T}$
    \end{algorithmic}
  \end{algorithm}
  \vspace{+5pt}
\end{minipage}
\par
}

% {
% \noindent
% \centering
% \begin{minipage}{0.9\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
%     % , sample size of responses per prompt $n$ 
%     \vspace{+3pt}

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \vspace{+5pt}
        
%         \LineComment{\textcolor{cred}{{\textbf{\texttt{creator step}}}}}
%         % \State \tb{\emph{self-generate responses}:} \hspace{+25pt}\tb{$\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ }
%         % %\Comment{self-generate $\rvy$}
%         % % \vspace{+2.5pt}
        
%         % % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$
%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{ ({\vy^{(j)}_i}, {r^{(j)}_i})\}$}

%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}\}$} 
%         %\Comment{annotate reward}
%         % \vspace{+0.1pt}
        
%         \vspace{+5pt}
%         \State  \tc{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t} \gets \calX_t \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}$ 
        
%         % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \{(\rvx_i, \tb{\texttt{info}(\rvx_i)}\}$ 
%         % where $\texttt{info}_i = f(\calD_{t}[i])$ 
%         %\Comment{estimate information}
%         \vspace{+2pt}
        

%         \Statex \hspace{+11pt}  \tc{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t})}}$ 
%         %\Comment{sample the informative subset}
%         \vspace{+2.5pt}

%         \Statex \hspace{+11pt} \tc{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t}^{\prime} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t}^{\texttt{info}})}}$ 
%         %\Comment{self-evolve $\rvx$}

%         \vspace{+8pt}
        
%          \LineComment{\textcolor{cgreen}{ \textbf{ \texttt{solver step} } } \tgray{(classical RLHF)}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
        
%         \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}^{\prime}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 
%         %\Comment{self-generate $\rvy$}
%         % \hspace{+11pt} 
%         \State \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t}^{\prime} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 
%         %\Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \vspace{+2.5pt}
        
%         \State \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
%         %\Comment{preference optimization}

%         \vspace{+5pt}

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor 
%     \State \Return final solver policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
%   \vspace{+5pt}
% \end{minipage}
% \par
% }

==> tables/fig-intro.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.39\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/game.pdf}
        % \vspace{+0.00001pt}
        \caption{\method. Open-Ended RLHF \textit{via} Asymmetric Self-Play. The creator is the prompt generation policy $\pi_X$ and the solver is the response generation policy $\pi_{Y|X}$.}
        \label{fig:game}
    \end{minipage}
    \hfill
    \begin{minipage}{0.58\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/mt-bench.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hspace{0.01\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/arena-hard.pdf}
            % \caption{Arena Hard}
        \end{subfigure}
        \hspace{0.01\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/alpaca-eval.pdf}
        \end{subfigure}
        \hspace{0.01\textwidth}
        \vspace{-5pt}
        \caption{\textbf{Results}. Our method~\method~achieves concrete performance gain especially on \emph{hard} alignment benchmarks, without relying on any additional human prompts. Here, we report results for DPO-\method; see more in \S\ref{sec:main_results}.}.
        \label{fig:three_benchmarks}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}
\vspace{-10pt}

==> tables/fig-pipeline.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.2\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/ah.png}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hspace{0.16\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.8\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/creator.png}
            % \caption{Arena Hard}
        \end{subfigure}
        \caption{\textbf{Results}: Our proposed \texttt{eva} achieves SOTA results on \emph{hard} alignment benchmakrs.}
        \label{fig:three_benchmarks}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}

==> tables/fig-rm.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth} % Adjust width to fit two figures in the same line
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure2}
    \end{minipage}
    
    \vspace{10pt} % Space between the two rows
    
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth} % Adjust width to fit two figures in the same line
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure4}
    \end{minipage}
\end{figure}


==> tables/tab-ab-cont.tex <==
\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{0.88\columnwidth}{!}{%
\begin{tabular}{@{}l c c c@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{3}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-4}

\textbf{Benchmark ($\rightarrow$)}           & \textbf{Arena-Hard} & \textbf{MT-Bench} & \textbf{AlpacaEval 2.0}\\ \cmidrule(l){2-2} \cmidrule(l){3-3} \cmidrule(l){4-4}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%) & \textbf{avg. score} & \textbf{LC-WR} (\%) \\ \midrule

$\vtheta_0$: SFT                & 41.3  & 8.57  & 47.11 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 8.66  & 55.01  \\

\rowcolor{green!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: \quad \texttt{\textbf{eva}} (scratch) & 59.8 & 8.88  & \text{54.59} \\

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \quad \texttt{\textbf{eva}} (incremental)  & \textbf{60.1} & \textbf{8.90}  &  \textbf{55.35}  \\ 

\bottomrule

\end{tabular}%
}
\vspace{-4pt}
\caption{\textbf{Ablation on incremental v.s. scratch training.}}
\label{tab:ab-cont}
\end{table}


==> tables/tab-ab-downstream-cache.tex <==
% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\textbf{Performance on Downstream tasks.} Evaluation results on selected downstream tasks.}
\label{tab:ab-downstream}
\end{table}

% \footnotetext{We find the original code of~\cite{mmlu-pro} for mmlu-pro, and use~\cite{eval-harness} to evaluate the rest.}


==> tables/tab-ab-downstream.tex <==
% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\textbf{Performance on Downstream tasks.}}
\label{tab:ab-downstream}
\end{table}


% \footnotetext{We find the original code of~\cite{mmlu-pro} for mmlu-pro, and use~\cite{eval-harness} to evaluate the rest.}


==> tables/tab-ab-gen-lm.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68 & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gpt-4-1106-preview}) } & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gpt-4o-mini}) } & & & & & & & & \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gemini-1.5-pro})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{Gemma-2-9B-it})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{Gemma-2-9B-dpo})} & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-gen-lm}
\end{table}

\notes{We may also discuss a bit on the student-teacher setting.}

==> tables/tab-ab-init.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\




$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\

\midrule




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}}} & & & & & & & & \\


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 30K  \texttt{\textbf{eva-i}} } & & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 60K  \texttt{\textbf{eva-i}} } & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-init}
\end{table}

==> tables/tab-ab-iter.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow 2}$: \text{\quad  +    \texttt{\textbf{eva-i}}} & \text{8.90} & \text{9.04}& \text{8.75} & \text{60.1}  &  725 &  55.35 &    55.53 & 2089 \\ 


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{2 \rightarrow 3}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & 60.8 & 741 & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{3 \rightarrow 4}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & 61.2 & 748 & & & \\



\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-iter}
\end{table}

==> tables/tab-ab-metric-cache.tex <==

% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{min}}$) } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / (r_{\max} - r_{\min})$)}  & 8.64 & 8.96 & 8.31 & 52.3 \textcolor{gray}{{\tiny CI: (-2.7, 3.1)}} & 669 & 53.84 & 52.92 \textcolor{gray}{{\tiny $\pm$ 1.76}}  & 1999 \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{avg}}$)} & 8.85 & 9.08 & 8.61 & 60.0  \textcolor{gray}{{\tiny CI: (-2.2, 2.8)}} & 725 & \textbf{56.01} & \textbf{56.46} \textcolor{gray}{{\tiny $\pm$ 1.75}} & 2107 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{second\_max}}$)}   & 8.86 & 9.18 & 8.52 & 60.0  \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}}& 745 & 55.96 & 56.09 \textcolor{gray}{{\tiny $\pm$ 1.75}}  & 2101 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{loo}(\vr)$)}  & 8.79 & 9.17 & 8.41 & 58.8 \textcolor{gray}{{\tiny CI: (-2.1, 2.5)}} & 752 & 53.41 & 53.60 \textcolor{gray}{{\tiny $\pm$ 1.76}}  & 2078 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{var}(\vr)$)}  & 8.66 & 9.13 & 8.20 & 54.8 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 654  & 54.58 & 52.55 \textcolor{gray}{{\tiny $\pm$ 1.76}} & 1957 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{avg}}$)}  & 8.76 & 9.13 & 8.40 & 58.5 \textcolor{gray}{{\tiny CI: (-2.2, 3.0)}} & 743 & 55.01 & 55.47 \textcolor{gray}{{\tiny $\pm$ 1.75}}  &2105 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / r_{\text{avg}}$)}  & 8.79  & 9.13 & 8.45 & 56.7  \textcolor{gray}{{\tiny CI: (-2.1, 2.0)}}&  712 & 55.04 &  54.97 \textcolor{gray}{{\tiny $\pm$ 1.75}} & 2076 \\



% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / \textcolor{black}{\dlog} $)}  & & & & & & & & \\

% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=(r_{\text{max}} - r_{\text{min}}) / \beta - \log(Z)$) } & & & & & & & & \\

% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w= \alpha\cdot(r_{\text{max}} - r_{\text{avg}}) + (1-\alpha)\cdot\text{diversity}$)} & 8.76 & 9.07 & 8.44  & 57.8  \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} & 725 & 55.48 & 55.96 \textcolor{gray}{\tiny $\pm$ 1.75}  & 2099 \\ 

% \rowcolor[HTML]{e2ebee} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{uniform}$)} & 8.71 & 9.02 & 8.40 & 57.5  \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} & 750 & 53.43 & 53.98 \textcolor{gray}{\tiny $\pm$ 1.76} & 2111 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Effect of different performance metric.} Our proposed metric achieves best performance on the \emph{hard} benchmark, \text{MT-Bench} and \text{Arena-Hard}.}
% \label{tab:ab-metric}
% \end{table}

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 651 & 55.01 & 51.68  & 1883  \\


\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{uniform}$)} & 8.71 & 9.02 & 8.40 & 57.5  & 750 & 53.43 & 53.98  & 2111 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\min}^{\star}$) } & \textbf{8.90} & \text{9.04}& \textbf{8.75} & \textbf{60.1}  &  725 &  55.35 &    55.53  & 2089 \\ 




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{avg}}^{\star}$)} & 8.85 & 9.08 & 8.61 & 60.0   & 725 & \textbf{56.01} & \textbf{56.46}  & 2107 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{dts}}$)}   & 8.86 & \textbf{9.18} & 8.52 & 60.0 & 745 & 55.96 & 56.09   & 2101 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{loo}}$)}  & 8.79 & 9.17 & 8.41 & 58.8  & 752 & 53.41 & 53.60  & 2078 \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{var}(\vr)$)}  & 8.66 & 9.13 & 8.20 & 54.8  & 654  & 54.58 & 52.55  & 1957 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{avg}}$)}  & 8.76 & 9.13 & 8.40 & 58.5  & 743 & 55.01 & 55.47   &2105 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / (r_{\max} - r_{\min})$)}  & 8.64 & 8.96 & 8.31 & 52.3  & 669 & 53.84 & 52.92   & 1999 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / r_{\text{avg}}$)}  & 8.79  & 9.13 & 8.45 & 56.7  &  712 & 55.04 &  54.97  & 2076 \\





\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Effect of informativeness metric.} Our advantage-based metric achieves best performance.}
\label{tab:ab-metric}
\end{table}



==> tables/tab-ab-metric.tex <==
\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-7}

\textbf{Benchmark ($\rightarrow$)} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}} \\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR (\%)} & \textbf{avg. score} & $1^{\text{st}}$ turn & $2^{\text{nd}}$ turn & \textbf{LC-WR (\%)} & \textbf{WR (\%)} \\ \midrule


% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  \\
    
    
    
$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 8.66 & 9.01 & 8.32 & 55.01 & 51.68    \\
\midrule


\rowcolor{brown!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($\texttt{\small uniform}$)} & 57.5  & 8.71 & 9.02 & 8.40 & 53.43 & 53.98  \\ 
\midrule

\rowcolor{gblue!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($\texttt{\small var}(\vr)$)}  & 54.8  & 8.66 & 9.13 & 8.20 & 54.58 & 52.55   \\


\rowcolor{gblue!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($\texttt{\small avg}(\vr)$)}  & 58.5  & 8.76 & 9.13 & 8.40 & 55.01 & 55.47    \\

\rowcolor{gblue!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($1 / \texttt{\small avg}(\vr)$)} & 56.7  & 8.79  & 9.13 & 8.45  & 55.04 &  54.97   \\

\midrule

    
\rowcolor{blue!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($1 / A_{\text{min}}^{\star}$)}  & 52.3  & 8.64 & 8.96 & 8.31 & 53.84 & 52.92  \\
\midrule
    

    
% \rowcolor{gred!8} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($A_{\text{loo}}$)} \textcolor{gray}{\tiny(variant)}  & 58.8  & 8.79 & 9.17 & 8.41 & 53.41 & 53.60   \\
    
    
\rowcolor{green!8} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($A_{\text{avg}}^{\star}$)} \textcolor{gray}{\tiny(our variant)} & 60.0 & 8.85 & 9.08 & 8.61 & \textbf{56.01} & \textbf{56.46}  \\ 
    
\rowcolor{green!8}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($A^{\star}_{\text{dts}}$)} \textcolor{gray}{\tiny(our variant)}   & 60.0 & 8.86 & \textbf{9.18} & 8.52 & 55.96 & 56.09   \\
    


% \midrule
\cdashlinelr{1-7}



\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \method~ ($A^{\star}_{\text{min}}$)} \textcolor{gray}{\tiny(our default)} & \hspace{+0.6cm}\textbf{60.1} \tc{\tiny (+8.5)}  & \textbf{8.90} & \text{9.04} & \hspace{+0.7cm}\textbf{8.75} \tc{\tiny (+0.43)} &  55.35  & 55.53 \\ 
    
    
    
    
\bottomrule

\end{tabular}%
}
\vspace{-4pt}
\caption{\textbf{Choice of informativeness metric matters.} Our metric by \emph{advantage} achieves the best performances, comparing with others as weights to sample for evolving. See also $\S$~\ref{app:metric} for visualization.}
\label{tab:ab-metric}
\end{table}


==> tables/tab-ab-procedure-cache-cache.tex <==
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Benchmark ($\rightarrow$)} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}} \\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{score (\%)} & \textbf{avg. score} & $1^{\text{st}}$ turn & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO & 51.6 & 8.66 & 9.01 & 8.32 & 55.01 & 51.68  \\

\midrule

\rowcolor{ggreen!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +    \texttt{subset-greedy}} & 56.1 & 8.68 & 8.98 & 8.38 & 54.11 & 53.66 \\ 

\rowcolor{ggreen!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +  \texttt{subset-sample} } & 55.3 & 8.69 & 9.00 & 8.38 & 54.22 & 54.16 \\ 


\midrule

\rowcolor{gred!12}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad   \method\texttt{-greedy} } & 59.5 & 8.72 & \text{9.06} & 8.36 & 54.52 & 55.22  \\ 

\rowcolor{gred!12} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  \texttt{\textbf{eva}-sample} \textcolor{gray}{\tiny(default)} } & \textbf{60.1} & \textbf{8.90} & \text{9.04} & \textbf{8.75} & \textbf{55.35} & \textbf{55.53} \\ 





\bottomrule

\end{tabular}%
}
\vspace{-4pt}
% \caption{\textbf{Effect of the {sample-then-evolve} procedure.} Evaluation results on general instruction-following alignment benchmarks. The green highlighted rows are training with only the informative subsets without evolving, and we use \texttt{\small greedy} to denote the training whose samples are selected greedily based on the  informativeness metric, and \texttt{\small sample} for the default~\method~procedure.} 
\caption{\textbf{Effect of sampling and evolving.} The green are those training w/ only the informative subset and w/o evolving); we add \texttt{\small -sample} for the default weighted sampling procedure in Algo~\ref{alg:i-eva}, while using \texttt{\small -greedy} for the classical active data selection procedure (\emph{cf}., a recent work~\citep{active-pl} and a pre-LLM work~\citep{ordered-sgd}), which simply selects data by a high-to-low ranking via the metric. We show, in general, sampling is better than being greedy (\emph{cf}.,~\cite{ts-tutorial}, p.15), and evolving data brings a remarkable alignment gain combing such active sampling.}
\label{tab:ab-procedure}
\end{table}
\vspace{-10pt}




==> tables/tab-ab-procedure-cache.tex <==
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

\rowcolor[HTML]{e2fbe2}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{eva-greedy} } & 8.72 & \textbf{9.06} & 8.36 & 59.5 \textcolor{gray}{{\tiny CI: (-2.5, 2.2)}} & 736 & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K  \texttt{subset-iw} } & 8.69 & 9.00 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K   \texttt{subset-greedy} } & 8.68 & 8.98 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\






\rowcolor[HTML]{e9ebee}
Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% \midrule




% $\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% \rowcolor[HTML]{e2fbe2} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1692 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: IPO      & 8.72 & 9.00 & 8.45 & 45.2 \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}} & 587 & 52.02 & 45.43 \textcolor{gray}{\tiny $\pm$ 1.75} & 1726 \\

% \rowcolor[HTML]{e2fbe2} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad + 10K  \texttt{\textbf{eva-iw}}  &  &  &  &  &  & 52.94  & 52.67 \textcolor{gray}{\tiny $\pm$ 1.76} & 2054 \\ 


% \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% \midrule





\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-procedure}
\end{table}
% ------------

==> tables/tab-ab-procedure.tex <==
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Benchmark ($\rightarrow$)} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}} \\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR (\%)} & \textbf{avg. score} & $1^{\text{st}}$ turn & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO & 51.6 & 8.66 & 9.01 & 8.32 & 55.01 & 51.68  \\

\midrule

\rowcolor{gblue!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad     \texttt{[no evolve]-greedy}} & 56.1 & 8.68 & 8.98 & 8.38 & 54.11 & 53.66 \\ 

\rowcolor{gblue!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad   \texttt{[no evolve]-sample} } & 55.3 & 8.69 & 9.00 & 8.38 & 54.22 & 54.16 \\ 

\midrule
\rowcolor{green!8} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +  \method\texttt{-greedy}} \textcolor{gray}{\tiny(our variant)}  & 59.5 & 8.72 & \text{9.06} & 8.36 & 54.52 & 55.22  \\ 


\cdashlinelr{1-7}

\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \texttt{\textbf{eva}-sample} \textcolor{gray}{\tiny(our default)} } & \textbf{60.1} & \textbf{8.90} & \text{9.04} & \textbf{8.75} & \textbf{55.35} & \textbf{55.53} \\ 





\bottomrule

\end{tabular}%
}
\vspace{-4pt}
% \caption{\textbf{Effect of the {sample-then-evolve} procedure.} Evaluation results on general instruction-following alignment benchmarks. The green highlighted rows are training with only the informative subsets without evolving, and we use \texttt{\small greedy} to denote the training whose samples are selected greedily based on the  informativeness metric, and \texttt{\small sample} for the default~\method~procedure.} 
\caption{\textbf{Effect of evolving.} The blue are those training w/ only the informative subset and w/o evolving); we denote \texttt{\small -sample} for the default weighted sampling procedure in Algo~\ref{alg:i-eva}, while using \texttt{\small -greedy} for the variant from the classical active data selection procedure (\emph{cf}., a recent work~\citep{active-pl} and a pre-LLM work~\citep{ordered-sgd}), which selects data by a high-to-low ranking via the metric greedily. We show evolving  brings a remarkable alignment gain (the red v.s. the blue); and as we evolve, sampling is more robust than being greedy (\emph{cf}.,~\cite{ts-tutorial}).}
\label{tab:ab-procedure}
\end{table}
\vspace{-10pt}




==> tables/tab-ab-rm-app.tex <==
% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule


% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\


% \rowcolor{green!10}
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & \text{9.04}& \text{8.75} & \text{60.1}  &  725 &  55.35 &    55.53 & 2089 \\ 

% \rowcolor{green!10}
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  &744  & \textbf{56.12} & \textbf{56.40}  & 2097 \\


% \bottomrule

% \end{tabular}%
% }
% % \vspace{+5pt}
% \caption{\textbf{Effect of (pointwise) reward models.}}
% \label{tab:ab-rm-app}
% \end{table}
%  % on relevant benchmarks

% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{.8\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule


% $\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7  & 560 & 51.58 & 42.17  & 1850 \\




% \rowcolor{green!10}
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & \text{8.78} & \textbf{9.11} &  \text{8.45} &  \text{58.9}  & 567 & \text{51.86} & \text{43.04}  & 1870 \\ 


% \rowcolor{green!10}
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & 563 & \textbf{52.71} & \textbf{44.52} & 1848 \\

% \bottomrule

% \end{tabular}%
% }
% % \vspace{+2pt}
% \caption{\textbf{Effect of (pairwise) reward models.}}
% \label{tab:ab-rm-sppo-app}
% \end{table}
% \vspace{-5pt}

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) &  \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 55.01 & 51.68  \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & 9.04 & 8.75 & 60.1  &  55.35 &    55.53 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  & \textbf{56.12} & \textbf{56.40} \\

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\textbf{Effect of (pointwise) reward models.}}
\label{tab:ab-rm-app}
\end{table}
 % on relevant benchmarks
 \vspace{-8pt}

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7 & 51.58 & 42.17 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & 8.78 & \textbf{9.11} &  8.45 &  58.9 & 51.86 & 43.04 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & \textbf{52.71} & \textbf{44.52} \\

\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\textbf{Effect of (pairwise) reward models.}}
\label{tab:ab-rm-sppo-app}
\end{table}
\vspace{-5pt}


==> tables/tab-ab-rm.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 & 544 &  47.11 & 38.39  & 1567 \\


% \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\




% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) } & & & & & & & & \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & \text{9.04}& \text{8.75} & \text{60.1}  &  725 &  55.35 &    55.53 & 2089 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  &744  & \textbf{56.12} & \textbf{56.40}  & 2097 \\


\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\textbf{Effect of reward models.} In general, \method~scales with better reward models.}
\label{tab:ab-rm}
\end{table}
 % on relevant benchmarks

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\


% \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7  & 560 & 51.58 & 42.17  & 1850 \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & \text{8.78} & \textbf{9.11} &  \text{8.45} &  \text{58.9}  & 567 & \text{51.86} & \text{43.04}  & 1870 \\ 


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & 563 & \textbf{52.71} & \textbf{44.52} & 1848 \\

% probably need to re-run to double check the judge used in the previous round

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & \text{9.04}& \text{8.75} & \text{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &744  & \textbf{56.12} & \textbf{56.40} \textcolor{gray}{\tiny $\pm$ 1.75} & 2097 \\


\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\textbf{Effect of different reward models.} In general, \method~scales with better reward models.}
\label{tab:ab-rm-sppo}
\end{table}
\vspace{-5pt}

==> tables/tab-ab-scale.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-i}}} & & & & & & & & \\


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 20K  \texttt{\textbf{eva-i}} } & \textbf{8.81} & 9.11 & \textbf{8.51} & \textbf{55.3} \textcolor{gray}{{\tiny CI: (-2.2, 2.4)}} &  871 & 52.37  &   52.92 \textcolor{gray}{\tiny $\pm$ 1.76} & 2300 \\ 

% & 8.73 & 9.18 & 8.28 & 53.2 \textcolor{gray}{{\tiny CI: (-2.2, 3.2)}}  & 625 & 53.48 & 48.70 \textcolor{gray}{\tiny $\pm$ 1.76} & 1824 \\ % this is the default 20k

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 30K  \texttt{\textbf{eva-i}} } & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 60K  \texttt{\textbf{eva-i}} } & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-scale}
\end{table}

==> tables/tab-info-metric.tex <==
\begin{table}[H]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{\hspace{+1.5cm} Metric} & $\textbf{\hspace{+1.8cm} info}(\rvx)$  & \textbf{\hspace{+.cm} Related Approximation}  \\ \midrule
% \rowcolor[HTML]{fcf1f0} 

$A^{\star}_{\text{min}}\text{: worst-case optimal advantage}$            & $| \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | $  &  minimax regret{\tiny~\citep{savage1951theory}} \vspace{+2pt} \\ 

$A^{\star}_{\text{avg}}\text{: average optimal advantage}$    &  $| \frac{1}{N} \sum_{\rvy}r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') |$  & Bayesian regret{\tiny~\citep{banos1968pseudo}}\vspace{+2pt} \\ 

$A^{\star}_{\text{dts}}\text{: dueling optimal advantage}$  & $|\max_{\rvy \neq \rvy^\star} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy')| $ & min-margin regret{\tiny~\citep{dts}}\vspace{+2pt} \\ 

% $A_{\text{loo}} \text{: leave-one-out advantage}$ &  $| \frac{1}{N} \sum_{\rvy} \bigr(r(\rvx, \rvy) - \frac{1}{N-1} \sum_{\rvy' \neq \rvy} r(\rvx, \rvy') \bigr) |$ & var-reduced gain{\tiny~\citep{kool2019buy}}\\



\bottomrule
\end{tabular}%
}
\vspace{-4pt}
\caption{The reward-advantage-based metrics that serve as the informativeness proxies for prompts.}
\label{tab:info-metric}
\vspace{-15pt}
\end{table}

==> tables/tab-main-10k-len.tex <==
% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-i}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1850 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-2.9, 2.1)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1870 \\ 

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-3.0, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1875 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.1)}} & 662 & 54.29 & 52.05 \textcolor{gray}{\tiny $\pm$ 1.75} & 1880  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \textbf{60.7} \textcolor{gray}{{\tiny CI: (-2.7, 2.3)}} & 683 & \textbf{55.85} & \textbf{55.92} \textcolor{gray}{\tiny $\pm$ 1.74} & 1903 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.76 & 9.00 & 8.52 & 54.6 \textcolor{gray}{{\tiny CI: (-2.8, 2.2)}} & 664 & 54.40 & 55.72 \textcolor{gray}{\tiny $\pm$ 1.74} & 1841\\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8 \textcolor{gray}{{\tiny CI: (-2.4, 2.1)}} & 665 & 52.17 & 49.50 \textcolor{gray}{\tiny $\pm$ 1.75} & 1962 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \textbf{60.3} \textcolor{gray}{{\tiny CI: (-2.8, 2.2)}} & 728 & \textbf{54.39} & \text{50.88} \textcolor{gray}{\tiny $\pm$ 1.74} & 1994 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.74 & 9.01 & 8.47 & 57.2 \textcolor{gray}{{\tiny CI: (-2.9, 2.2)}} & 733 & 54.00 & 51.21 \textcolor{gray}{\tiny $\pm$ 1.75} & 2017\\

% \bottomrule

% \end{tabular}%
% }
% % \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:main-10k}
% \end{table}


\begin{table}[!ht]
\centering

% \vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 651 & 55.01 & 51.68  & 1883  \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8  & 733 & \textbf{55.74} & \textbf{56.15}  & 2111  \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva-i}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \textbf{60.1}  &  725 &  55.35 &    55.53  & 2089 \\ 

\midrule

$\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7  & 560 & 51.58 & 42.17  & 1850 \\

\rowcolor[HTML]{e9ebee}
$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7  & 562 & 51.78 & 42.98  & 1875 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9}  & 567 & \textbf{51.86} & \textbf{43.04}  & 1870 \\ 


\midrule

$\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3  & 662 & 54.29 & 52.05  & 1880  \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts}      & 8.76 & 9.00 & 8.52 & 54.6  & 664 & 54.40 & 55.72  & 1841\\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \textbf{60.7}  & 683 & \textbf{55.85} & \textbf{55.92}  & 1903 \\ 



\midrule

$\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8  & 665 & 52.17 & 49.50  & 1962 \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}      & 8.74 & 9.01 & 8.47 & 57.2  & 733 & 54.00 & \textbf{51.21}  & 2017\\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \textbf{60.3}  & 728 & \textbf{54.39} & 50.88  & 1994 \\ 

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:main-10k}
\end{table}



==> tables/tab-main-10k-o.tex <==
% \notes{The experiment is re-running.}
\FloatBarrier
\begin{table}[h]
\centering

% \vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ 
\midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     &  & & & & & & & \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-o}} } & & & & & & & & \\





% \midrule



% $\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}      & 8,62 & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +    \texttt{\textbf{eva-o}} } & & & & & & & & \\

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}    & & & & & & & & \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.63 & & & & & & &  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad +    \texttt{\textbf{eva-o}}  & & & & & & & & \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.62 & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad +    \texttt{\textbf{eva-o}}  & & & & & & & & \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\





\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:main-eva-o}
\end{table}

% \notes{This experiment is on-going.}

==> tables/tab-main-10k.tex <==
% \begin{table}[H]
% \centering

% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-7}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-7}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 47.11 & 38.39 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 55.01  & 51.68  \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \hspace{+0.6cm}\textbf{60.1} \tc{\tiny (+8.5)}  &  55.35  & 55.53 \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{8.64} & \tgray{8.88} & \tgray{8.39} & \tgray{59.8}  & \tgray{\textbf{55.74}}  & \tgray{\textbf{56.15}}  \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7  & 51.58  & 42.17 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \hspace{+0.6cm}\textbf{58.9} \tc{\tiny (+3.2)}   & \textbf{51.86}  & \textbf{43.04} \\ 

% \rowcolor[HTML]{f5f7fc}
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts} }   &  \tgray{8.64} &  \tgray{8.90} &  \tgray{8.39} &  \tgray{57.7}  & \tgray{51.78}  & \tgray{42.98} \\


% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3  & 54.29  & 52.05 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \hspace{+0.6cm}\textbf{60.7} \tc{\tiny (+8.4)}   & \textbf{55.85}  & \textbf{55.92} \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts} }     & \tgray{8.76} & \tgray{9.00} & \tgray{8.52} & \tgray{54.6}  & \tgray{54.40}  & \tgray{55.72}\\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8  & 52.17  & 49.50 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \hspace{+0.6cm}\textbf{60.3} \tc{\tiny  (+5.5)}   & \textbf{54.39}  & \textbf{50.88} \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}}      & \tgray{8.74} & \tgray{9.01} & \tgray{8.47} & \tgray{57.2}  & \tgray{54.00}  & \tgray{\textbf{51.21}} \\

% \bottomrule

% \end{tabular}%
% }
% \caption{\textbf{Main results.} \method~achieves concrete alignment gain and even surpasses  human prompts.}

% \label{tab:main-10k}
% \end{table}

\begin{table}[H]
\centering

\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-7}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}



\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%)      & \textbf{avg. score}   & $1^{\text{st}}$ turn  & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

$\vtheta_0$: SFT                &  41.3  &  8.57 &  8.81 &  8.32 & 47.11 & 38.39 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 8.66 & 9.01 & 8.32 & 55.01  & 51.68  \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.1} \tc{\tiny (+8.5)}  & \textbf{8.90} & \textbf{9.04} & \hspace{+0.7cm}\textbf{8.75} \tc{\tiny (+0.43)} &  55.35  & 55.53 \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{59.8}  & \tgray{8.64} & \tgray{8.88} & \tgray{8.39} & \tgray{\textbf{55.74}}  & \tgray{\textbf{56.15}}  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: SPPO       & 55.7  & 8.62 &  9.03 &  8.21 &  51.58  & 42.17 \\



\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } &  \hspace{+0.6cm}\textbf{58.9} \tc{\tiny (+3.2)} & \textbf{8.78} & \textbf{9.11} &  \hspace{+0.7cm}\textbf{8.45} \tc{\tiny (+0.24)} & \textbf{51.86}  & \textbf{43.04} \\ 

\rowcolor[HTML]{f5f7fc}
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts} }   & \tgray{57.7}  &  \tgray{8.64} &  \tgray{8.90} &  \tgray{8.39} &  \tgray{51.78}  & \tgray{42.98} \\


\midrule

$\vtheta_{0 \rightarrow 1}$: SimPO      & 52.3  & 8.69 & 9.03 & 8.35 & 54.29  & 52.05 \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.7} \tc{\tiny (+8.4)} & \textbf{8.92} & \textbf{9.08} & \hspace{+0.7cm}\textbf{8.77} \tc{\tiny (+0.42)} & \textbf{55.85}  & \textbf{55.92} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts} }     & \tgray{54.6}  & \tgray{8.76} & \tgray{9.00} & \tgray{8.52} & \tgray{54.40}  & \tgray{55.72}\\

\midrule

$\vtheta_{0 \rightarrow 1}$: ORPO     & 54.8  & 8.67 & 9.04 & 8.30 & 52.17  & 49.50 \\



\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.3} \tc{\tiny  (+5.5)} & \textbf{8.89} & \textbf{9.07} & \hspace{+0.7cm}\textbf{8.71} \tc{\tiny (+0.41)} & \textbf{54.39}  & \textbf{50.88} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}}      & \tgray{57.2}  & \tgray{8.74} & \tgray{9.01} & \tgray{8.47} & \tgray{54.00}  & \tgray{\textbf{51.21}} \\

\bottomrule

\end{tabular}%
}
\caption{\textbf{Main results.} Our~\method~achieves notable alignment gains and can surpass human prompts on major benchmarks across a variety of representative direct preference optimization algorithms.}
\label{tab:main-10k}
\end{table}
\vspace{-10pt}



==> tabs/algo-eva-icml.tex <==
{
\noindent
\centering
\begin{minipage}{0.66\linewidth}
  \begin{algorithm}[H]
    \small
    
    \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
    \begin{algorithmic}[1]
    \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
    % , sample size of responses per prompt $n$ 
    \vspace{+3pt}

    \For{\textbf{iteration} $t = 1, 2, \ldots$}
        \vspace{+5pt}
        
        \LineComment{\textcolor{cgreen}{{\textbf{\texttt{creator step}}}}}
        
        \vspace{+5pt}
        % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t-1} \gets \calX_{t-1} \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}_i$ 
        \State \tb{\emph{estimate informativeness}:} \hspace{+18pt} $\mathcal{X}_{t-1} \gets \{ (\rvx_i, \textbf{\texttt{info}}(\rvx_i)) \mid \rvx_i \in \mathcal{X}_{t-1} \}$

        
        \vspace{+2pt}
        

        \Statex \hspace{+11pt}  \tb{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t-1}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t-1})}}$ 
        \vspace{+2.5pt}

        \Statex \hspace{+11pt} \tb{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t-1}^{\texttt{info}})}}$ 

        \vspace{+8pt}
        
         \LineComment{\textcolor{cred}{ \textbf{ \texttt{solver step} } }}
        
        \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 

        \Statex \hspace{+11pt} \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 

        \vspace{+2.5pt}
        
        \Statex \hspace{+11pt} \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}_{t} \leftarrow \boldsymbol{\theta}_{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
        \vspace{+5pt}
        
    \EndFor 
    \State \Return final solver policy $\pi_{\vtheta_T}$
    \end{algorithmic}
  \end{algorithm}
\end{minipage}
\par
}

% {
% \noindent
% \centering
% \begin{minipage}{0.9\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
%     % , sample size of responses per prompt $n$ 
%     \vspace{+3pt}

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \vspace{+5pt}
        
%         \LineComment{\textcolor{cred}{{\textbf{\texttt{creator step}}}}}
%         % \State \tb{\emph{self-generate responses}:} \hspace{+25pt}\tb{$\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ }
%         % %\Comment{self-generate $\rvy$}
%         % % \vspace{+2.5pt}
        
%         % % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$
%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{ ({\vy^{(j)}_i}, {r^{(j)}_i})\}$}

%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}\}$} 
%         %\Comment{annotate reward}
%         % \vspace{+0.1pt}
        
%         \vspace{+5pt}
%         \State  \tc{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t} \gets \calX_t \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}$ 
        
%         % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \{(\rvx_i, \tb{\texttt{info}(\rvx_i)}\}$ 
%         % where $\texttt{info}_i = f(\calD_{t}[i])$ 
%         %\Comment{estimate information}
%         \vspace{+2pt}
        

%         \Statex \hspace{+11pt}  \tc{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t})}}$ 
%         %\Comment{sample the informative subset}
%         \vspace{+2.5pt}

%         \Statex \hspace{+11pt} \tc{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t}^{\prime} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t}^{\texttt{info}})}}$ 
%         %\Comment{self-evolve $\rvx$}

%         \vspace{+8pt}
        
%          \LineComment{\textcolor{cgreen}{ \textbf{ \texttt{solver step} } } \tgray{(classical RLHF)}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
        
%         \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}^{\prime}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 
%         %\Comment{self-generate $\rvy$}
%         % \hspace{+11pt} 
%         \State \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t}^{\prime} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 
%         %\Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \vspace{+2.5pt}
        
%         \State \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
%         %\Comment{preference optimization}

%         \vspace{+5pt}

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor 
%     \State \Return final solver policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
%   \vspace{+5pt}
% \end{minipage}
% \par
% }

==> tabs/algo-eva.tex <==
{
\noindent
\centering
\begin{minipage}{0.66\linewidth}
  \begin{algorithm}[H]
    \small
    
    \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
    \begin{algorithmic}[1]
    \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
    % , sample size of responses per prompt $n$ 
    \vspace{+3pt}

    \For{\textbf{iteration} $t = 1, 2, \ldots$}
        \vspace{+5pt}
        
        \LineComment{\textcolor{cgreen}{{\textbf{\texttt{creator step}}}}}
        
        \vspace{+5pt}
        % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t-1} \gets \calX_{t-1} \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}_i$ 
        \State \tb{\emph{estimate informativeness}:} \hspace{+18pt} $\mathcal{X}_{t-1} \gets \{ (\rvx_i, \textbf{\texttt{info}}(\rvx_i)) \mid \rvx_i \in \mathcal{X}_{t-1} \}$

        
        \vspace{+2pt}
        

        \Statex \hspace{+11pt}  \tb{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t-1}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t-1})}}$ 
        \vspace{+2.5pt}

        \Statex \hspace{+11pt} \tb{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t-1}^{\texttt{info}})}}$ 

        \vspace{+8pt}
        
         \LineComment{\textcolor{cred}{ \textbf{ \texttt{solver step} } }}
        
        \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 

        \Statex \hspace{+11pt} \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 

        \vspace{+2.5pt}
        
        \Statex \hspace{+11pt} \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}_{t} \leftarrow \boldsymbol{\theta}_{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
        \vspace{+5pt}
        
    \EndFor 
    \State \Return final solver policy $\pi_{\vtheta_T}$
    \end{algorithmic}
  \end{algorithm}
\end{minipage}
\par
}

% {
% \noindent
% \centering
% \begin{minipage}{0.9\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
%     % , sample size of responses per prompt $n$ 
%     \vspace{+3pt}

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \vspace{+5pt}
        
%         \LineComment{\textcolor{cred}{{\textbf{\texttt{creator step}}}}}
%         % \State \tb{\emph{self-generate responses}:} \hspace{+25pt}\tb{$\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ }
%         % %\Comment{self-generate $\rvy$}
%         % % \vspace{+2.5pt}
        
%         % % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$
%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{ ({\vy^{(j)}_i}, {r^{(j)}_i})\}$}

%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}\}$} 
%         %\Comment{annotate reward}
%         % \vspace{+0.1pt}
        
%         \vspace{+5pt}
%         \State  \tc{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t} \gets \calX_t \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}$ 
        
%         % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \{(\rvx_i, \tb{\texttt{info}(\rvx_i)}\}$ 
%         % where $\texttt{info}_i = f(\calD_{t}[i])$ 
%         %\Comment{estimate information}
%         \vspace{+2pt}
        

%         \Statex \hspace{+11pt}  \tc{\emph{sample subset}:} \hspace{+60pt}$\tb{\calX_{t}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t})}}$ 
%         %\Comment{sample the informative subset}
%         \vspace{+2.5pt}

%         \Statex \hspace{+11pt} \tc{\emph{self-evolve prompts}:} \hspace{+40pt}$\tb{\mathcal{X}_{t}^{\prime} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t}^{\texttt{info}})}}$ 
%         %\Comment{self-evolve $\rvx$}

%         \vspace{+8pt}
        
%          \LineComment{\textcolor{cgreen}{ \textbf{ \texttt{solver step} } } \tgray{(classical RLHF)}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
        
%         \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}^{\prime}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 
%         %\Comment{self-generate $\rvy$}
%         % \hspace{+11pt} 
%         \State \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t}^{\prime} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 
%         %\Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \vspace{+2.5pt}
        
%         \State \tb{\emph{preference optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})}$ 
%         %\Comment{preference optimization}

%         \vspace{+5pt}

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor 
%     \State \Return final solver policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
%   \vspace{+5pt}
% \end{minipage}
% \par
% }

==> tabs/fig-intro.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.39\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/game.pdf}
        % \vspace{+0.00001pt}
        \caption{\method. Open-Ended RLHF \textit{via} Asymmetric Self-Play. The creator is the prompt generation policy $\pi_X$ and the solver is the response generation policy $\pi_{Y|X}$.}
        \label{fig:game}
    \end{minipage}
    \hfill
    \begin{minipage}{0.58\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/mt-bench.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hspace{0.01\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/arena-hard.pdf}
            % \caption{Arena Hard}
        \end{subfigure}
        \hspace{0.01\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/alpaca-eval.pdf}
        \end{subfigure}
        \hspace{0.01\textwidth}
        \vspace{-5pt}
        \caption{\textbf{Results}. Our method~\method~achieves concrete performance gain especially on \emph{hard} alignment benchmarks, without relying on any additional human prompts. Here, we report results for DPO-\method; see more in \S~\ref{sec:main_results}.}.
        \label{fig:three_benchmarks}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}
\vspace{-10pt}

==> tabs/fig-pipeline.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.2\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/ah.png}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hspace{0.16\textwidth} % Small space between the subfigures
        \begin{subfigure}{0.8\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/creator.png}
            % \caption{Arena Hard}
        \end{subfigure}
        \caption{\textbf{Results}: Our proposed \texttt{eva} achieves SOTA results on \emph{hard} alignment benchmakrs.}
        \label{fig:three_benchmarks}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}

==> tabs/fig-rm.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth} % Adjust width to fit two figures in the same line
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure2}
    \end{minipage}
    
    \vspace{10pt} % Space between the two rows
    
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure3}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth} % Adjust width to fit two figures in the same line
        \centering
        \includegraphics[width=\linewidth]{figs/dpo-rm-ae.png}
        \vspace{+0.1pt}
        \caption{}
        \label{fig:figure4}
    \end{minipage}
\end{figure}


==> tabs/tab-ab-downstream-cache.tex <==
% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\textbf{Performance on Downstream tasks.} Evaluation results on selected downstream tasks.}
\label{tab:ab-downstream}
\end{table}

% \footnotetext{We find the original code of~\cite{mmlu-pro} for mmlu-pro, and use~\cite{eval-harness} to evaluate the rest.}


==> tabs/tab-ab-downstream.tex <==
% -------------------------------------------------------------
\begin{table}[H]
\centering
\vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
% \textbf{Model Family ($\rightarrow$)}           & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Method ($\downarrow$) / Dataset ($\rightarrow$)} & \textbf{MUSR-TA}   & \textbf{TruthfulQA-Gen}        & \textbf{WMDP}  & \textbf{GSM8K}    & \textbf{GSM-Plus} & \textbf{MMLU-Pro}\\ \midrule

$\vtheta_0$: SFT        & 38.80 & 34.76 & 58.62 & 24.64 & 18.62 & 52.08 \\

\midrule
$\vtheta_{0 \rightarrow 1}$: DPO     & 38.40 & 34.76 & 58.45 & 24.56 & 18.50 & 52.63 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & 38.40 & 34.15 & 58.40 & 24.26 & 17.96 & \textbf{53.03} \\

\midrule
$\vtheta_{0 \rightarrow 1}$: SPPO        & 40.80 & 34.15 & 58.72 & 24.79 & 18.42 & 52.70 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + \texttt{\textbf{eva}} & \textbf{41.20} & 34.64 & \textbf{58.94} & \textbf{25.40} & \textbf{18.88} & 52.47 \\ 

\bottomrule
\end{tabular}%
}
\vspace{-2pt}
\caption{\textbf{Performance on Downstream tasks.}}
\label{tab:ab-downstream}
\end{table}


% \footnotetext{We find the original code of~\cite{mmlu-pro} for mmlu-pro, and use~\cite{eval-harness} to evaluate the rest.}


==> tabs/tab-ab-gen-lm.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68 & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gpt-4-1106-preview}) } & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gpt-4o-mini}) } & & & & & & & & \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\texttt{gemini-1.5-pro})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{Gemma-2-9B-it})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{Gemma-2-9B-dpo})} & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-gen-lm}
\end{table}

\notes{We may also discuss a bit on the student-teacher setting.}

==> tabs/tab-ab-init.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\




$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\

\midrule




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}}} & & & & & & & & \\


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 30K  \texttt{\textbf{eva-i}} } & & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 60K  \texttt{\textbf{eva-i}} } & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-init}
\end{table}

==> tabs/tab-ab-iter.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow 2}$: \text{\quad  +    \texttt{\textbf{eva-i}}} & \text{8.90} & \text{9.04}& \text{8.75} & \text{60.1}  &  725 &  55.35 &    55.53 & 2089 \\ 


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{2 \rightarrow 3}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & 60.8 & 741 & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{3 \rightarrow 4}$: \text{\quad  +    \texttt{\textbf{eva-i}} } & & & & 61.2 & 748 & & & \\



\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-iter}
\end{table}

==> tabs/tab-ab-metric-cache.tex <==

% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{min}}$) } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / (r_{\max} - r_{\min})$)}  & 8.64 & 8.96 & 8.31 & 52.3 \textcolor{gray}{{\tiny CI: (-2.7, 3.1)}} & 669 & 53.84 & 52.92 \textcolor{gray}{{\tiny $\pm$ 1.76}}  & 1999 \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{avg}}$)} & 8.85 & 9.08 & 8.61 & 60.0  \textcolor{gray}{{\tiny CI: (-2.2, 2.8)}} & 725 & \textbf{56.01} & \textbf{56.46} \textcolor{gray}{{\tiny $\pm$ 1.75}} & 2107 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{max}} - r_{\text{second\_max}}$)}   & 8.86 & 9.18 & 8.52 & 60.0  \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}}& 745 & 55.96 & 56.09 \textcolor{gray}{{\tiny $\pm$ 1.75}}  & 2101 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{loo}(\vr)$)}  & 8.79 & 9.17 & 8.41 & 58.8 \textcolor{gray}{{\tiny CI: (-2.1, 2.5)}} & 752 & 53.41 & 53.60 \textcolor{gray}{{\tiny $\pm$ 1.76}}  & 2078 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{var}(\vr)$)}  & 8.66 & 9.13 & 8.20 & 54.8 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 654  & 54.58 & 52.55 \textcolor{gray}{{\tiny $\pm$ 1.76}} & 1957 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{avg}}$)}  & 8.76 & 9.13 & 8.40 & 58.5 \textcolor{gray}{{\tiny CI: (-2.2, 3.0)}} & 743 & 55.01 & 55.47 \textcolor{gray}{{\tiny $\pm$ 1.75}}  &2105 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / r_{\text{avg}}$)}  & 8.79  & 9.13 & 8.45 & 56.7  \textcolor{gray}{{\tiny CI: (-2.1, 2.0)}}&  712 & 55.04 &  54.97 \textcolor{gray}{{\tiny $\pm$ 1.75}} & 2076 \\



% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / \textcolor{black}{\dlog} $)}  & & & & & & & & \\

% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=(r_{\text{max}} - r_{\text{min}}) / \beta - \log(Z)$) } & & & & & & & & \\

% % \rowcolor[HTML]{fcf1f0} 
% % $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w= \alpha\cdot(r_{\text{max}} - r_{\text{avg}}) + (1-\alpha)\cdot\text{diversity}$)} & 8.76 & 9.07 & 8.44  & 57.8  \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} & 725 & 55.48 & 55.96 \textcolor{gray}{\tiny $\pm$ 1.75}  & 2099 \\ 

% \rowcolor[HTML]{e2ebee} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{uniform}$)} & 8.71 & 9.02 & 8.40 & 57.5  \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} & 750 & 53.43 & 53.98 \textcolor{gray}{\tiny $\pm$ 1.76} & 2111 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Effect of different performance metric.} Our proposed metric achieves best performance on the \emph{hard} benchmark, \text{MT-Bench} and \text{Arena-Hard}.}
% \label{tab:ab-metric}
% \end{table}

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 651 & 55.01 & 51.68  & 1883  \\


\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{uniform}$)} & 8.71 & 9.02 & 8.40 & 57.5  & 750 & 53.43 & 53.98  & 2111 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\min}^{\star}$) } & \textbf{8.90} & \text{9.04}& \textbf{8.75} & \textbf{60.1}  &  725 &  55.35 &    55.53  & 2089 \\ 




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{avg}}^{\star}$)} & 8.85 & 9.08 & 8.61 & 60.0   & 725 & \textbf{56.01} & \textbf{56.46}  & 2107 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{dts}}$)}   & 8.86 & \textbf{9.18} & 8.52 & 60.0 & 745 & 55.96 & 56.09   & 2101 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=A_{\text{loo}}$)}  & 8.79 & 9.17 & 8.41 & 58.8  & 752 & 53.41 & 53.60  & 2078 \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=\texttt{var}(\vr)$)}  & 8.66 & 9.13 & 8.20 & 54.8  & 654  & 54.58 & 52.55  & 1957 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=r_{\text{avg}}$)}  & 8.76 & 9.13 & 8.40 & 58.5  & 743 & 55.01 & 55.47   &2105 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / (r_{\max} - r_{\min})$)}  & 8.64 & 8.96 & 8.31 & 52.3  & 669 & 53.84 & 52.92   & 1999 \\

\rowcolor[HTML]{e6ebee} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} ($w=1 / r_{\text{avg}}$)}  & 8.79  & 9.13 & 8.45 & 56.7  &  712 & 55.04 &  54.97  & 2076 \\





\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Effect of informativeness metric.} Our advantage-based metric achieves best performance.}
\label{tab:ab-metric}
\end{table}



==> tabs/tab-ab-procedure-cache-cache.tex <==
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Benchmark ($\rightarrow$)} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}} \\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{score (\%)} & \textbf{avg. score} & $1^{\text{st}}$ turn & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO & 51.6 & 8.66 & 9.01 & 8.32 & 55.01 & 51.68  \\

\midrule

\rowcolor{ggreen!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +    \texttt{subset-greedy}} & 56.1 & 8.68 & 8.98 & 8.38 & 54.11 & 53.66 \\ 

\rowcolor{ggreen!15} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +  \texttt{subset-sample} } & 55.3 & 8.69 & 9.00 & 8.38 & 54.22 & 54.16 \\ 


\midrule

\rowcolor{gred!12}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad   \method\texttt{-greedy} } & 59.5 & 8.72 & \text{9.06} & 8.36 & 54.52 & 55.22  \\ 

\rowcolor{gred!12} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  \texttt{\textbf{eva}-sample} \textcolor{gray}{\tiny(default)} } & \textbf{60.1} & \textbf{8.90} & \text{9.04} & \textbf{8.75} & \textbf{55.35} & \textbf{55.53} \\ 





\bottomrule

\end{tabular}%
}
\vspace{-4pt}
% \caption{\textbf{Effect of the {sample-then-evolve} procedure.} Evaluation results on general instruction-following alignment benchmarks. The green highlighted rows are training with only the informative subsets without evolving, and we use \texttt{\small greedy} to denote the training whose samples are selected greedily based on the  informativeness metric, and \texttt{\small sample} for the default~\method~procedure.} 
\caption{\textbf{Effect of sampling and evolving.} The green are those training w/ only the informative subset and w/o evolving); we add \texttt{\small -sample} for the default weighted sampling procedure in Algo~\ref{alg:i-eva}, while using \texttt{\small -greedy} for the classical active data selection procedure (\emph{cf}., a recent work~\citep{active-pl} and a pre-LLM work~\citep{ordered-sgd}), which simply selects data by a high-to-low ranking via the metric. We show, in general, sampling is better than being greedy (\emph{cf}.,~\cite{ts-tutorial}, p.15), and evolving data brings a remarkable alignment gain combing such active sampling.}
\label{tab:ab-procedure}
\end{table}
\vspace{-10pt}




==> tabs/tab-ab-procedure-cache.tex <==
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

\rowcolor[HTML]{e2fbe2}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{eva-greedy} } & 8.72 & \textbf{9.06} & 8.36 & 59.5 \textcolor{gray}{{\tiny CI: (-2.5, 2.2)}} & 736 & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K  \texttt{subset-iw} } & 8.69 & 9.00 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K   \texttt{subset-greedy} } & 8.68 & 8.98 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\






\rowcolor[HTML]{e9ebee}
Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% \midrule




% $\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% \rowcolor[HTML]{e2fbe2} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1692 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: IPO      & 8.72 & 9.00 & 8.45 & 45.2 \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}} & 587 & 52.02 & 45.43 \textcolor{gray}{\tiny $\pm$ 1.75} & 1726 \\

% \rowcolor[HTML]{e2fbe2} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad + 10K  \texttt{\textbf{eva-iw}}  &  &  &  &  &  & 52.94  & 52.67 \textcolor{gray}{\tiny $\pm$ 1.76} & 2054 \\ 


% \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% \midrule





\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-procedure}
\end{table}
% ------------

==> tabs/tab-ab-rm-app.tex <==

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) &  \\ \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 55.01 & 51.68  \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & 9.04 & 8.75 & 60.1  &  55.35 &    55.53 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  & \textbf{56.12} & \textbf{56.40} \\

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\textbf{Effect of (pointwise) reward models.}}
\label{tab:ab-rm-app}
\end{table}
 % on relevant benchmarks
 \vspace{-8pt}

\begin{table}[H]
\centering

% \vspace{+5pt}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{7}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-8}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-8}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%) & \textbf{LC} (\%) & \textbf{WR} (\%) \\ \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7 & 51.58 & 42.17 \\

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & 8.78 & \textbf{9.11} &  8.45 &  58.9 & 51.86 & 43.04 \\ 

\rowcolor{green!10}
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & \textbf{52.71} & \textbf{44.52} \\

\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\textbf{Effect of (pairwise) reward models.}}
\label{tab:ab-rm-sppo-app}
\end{table}
\vspace{-5pt}


==> tabs/tab-ab-rm.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 & 544 &  47.11 & 38.39  & 1567 \\


% \midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6  & 651 & 55.01 & 51.68  & 1883  \\




% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) } & & & & & & & & \\


% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & \text{9.04}& \text{8.75} & \text{60.1}  &  725 &  55.35 &    55.53 & 2089 \\ 

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3}  &744  & \textbf{56.12} & \textbf{56.40}  & 2097 \\


\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
\caption{\textbf{Effect of reward models.} In general, \method~scales with better reward models.}
\label{tab:ab-rm}
\end{table}
 % on relevant benchmarks

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\


% \midrule

$\vtheta_{0 \rightarrow 1}$: SPPO      & 8.62 &  9.03 &  8.21 &  55.7  & 560 & 51.58 & 42.17  & 1850 \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-0.4B}) }  & \text{8.78} & \textbf{9.11} &  \text{8.45} &  \text{58.9}  & 567 & \text{51.86} & \text{43.04}  & 1870 \\ 


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{PairRM-8B})} & \textbf{8.89} & 9.08 & \textbf{8.70} & \textbf{60.2} & 563 & \textbf{52.71} & \textbf{44.52} & 1848 \\

% probably need to re-run to double check the judge used in the previous round

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{ArMO-8B})} & \textbf{8.90} & \text{9.04}& \text{8.75} & \text{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-i}} (\textsc{SkyworkRM-27B})} & 8.75  & 9.07 & 8.43 & \textbf{60.3} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &744  & \textbf{56.12} & \textbf{56.40} \textcolor{gray}{\tiny $\pm$ 1.75} & 2097 \\


\bottomrule

\end{tabular}%
}
% \vspace{+2pt}
\caption{\textbf{Effect of different reward models.} In general, \method~scales with better reward models.}
\label{tab:ab-rm-sppo}
\end{table}
\vspace{-5pt}

==> tabs/tab-ab-scale.tex <==

\begin{table}[H]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-i}}} & & & & & & & & \\


\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 20K  \texttt{\textbf{eva-i}} } & \textbf{8.81} & 9.11 & \textbf{8.51} & \textbf{55.3} \textcolor{gray}{{\tiny CI: (-2.2, 2.4)}} &  871 & 52.37  &   52.92 \textcolor{gray}{\tiny $\pm$ 1.76} & 2300 \\ 

% & 8.73 & 9.18 & 8.28 & 53.2 \textcolor{gray}{{\tiny CI: (-2.2, 3.2)}}  & 625 & 53.48 & 48.70 \textcolor{gray}{\tiny $\pm$ 1.76} & 1824 \\ % this is the default 20k

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 30K  \texttt{\textbf{eva-i}} } & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 60K  \texttt{\textbf{eva-i}} } & & & & & & & & \\


\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:ab-scale}
\end{table}

==> tabs/tab-main-10k-icml-online-cache.tex <==
\begin{table}[H]

\caption{\textbf{Online \method\ results.} Our method achieves notable alignment gains and self-plays for continual RL post-training. Note only $\mathsf{1x}$ human prompts are used for \method.
}
\vspace{-5pt}

\centering

\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule

\textbf{Optimization Method ($\rightarrow$)}          & \multicolumn{5}{c}{$\mathsf{Online\ RLHF}$} \\ \cmidrule(l){2-6}

\textbf{Benchmark ($\rightarrow$)}           
& \multicolumn{1}{c}{\textbf{Arena-Hard}} 
& \multicolumn{3}{c}{\textbf{MT-Bench}}
& \multicolumn{1}{c}{\textbf{AE 2.0}} 

\\ 
\cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-6}



\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} {\tiny (\%)}      & \textbf{avg.}   & turn 1  & turn 2 & \textbf{LC-WR} {\tiny (\%)}  \\ \midrule

$\vtheta_0$: Base Model                &  41.3  &  8.57 &  8.81 &  8.32 & 47.11 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: $\mathsf{RLOO}$  ($\mathsf{1x}$)    
& 52.6  & 8.68 & 9.02 & 8.34 & 54.23   \\

\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{RLOO}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{1x}$) 
& \textbf{57.3}   &  &  &   &    \\ 

\cdashlinelr{1-6}

$\vtheta_{0 \rightarrow 1}$: $\mathsf{RLOO}$  ($\mathsf{2x}$)    
&   \\


\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{RLOO}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{2x}$) 
& \textbf{60.5}   &  &  &   &    \\ 

\cdashlinelr{1-6}

$\vtheta_{0 \rightarrow 1}$: $\mathsf{RLOO}$  ($\mathsf{3x}$)    
&    \\

\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{RLOO}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{3x}$)  
& \textbf{62.4}   &  &  &   &    \\ 

\midrule

$\vtheta_{0 \rightarrow 1}$: $\mathsf{OAIF}$  ($\mathsf{1x}$)     & 52.1  &  &  &  &    \\

\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{OAIF}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{1x}$) 
& \textbf{55.0}   &  &  &   &    \\ 


\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{OAIF}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{2x}$) 
& \textbf{60.4}   &  &  &   &    \\ 

\rowcolor{ggreen!10} 
$\vtheta_{0 \rightarrow \Tilde{1}}$: $\mathsf{OAIF}${\footnotesize -}\texttt{\textbf{\footnotesize eva}} ($\mathsf{3x}$) 
& \textbf{61.7}   &  &  &   &    \\ 

\bottomrule

\end{tabular}%
}

\label{tab:main-10k-online}
\end{table}



==> tabs/tab-main-10k-len.tex <==
% \begin{table}[H]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-i}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1850 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-2.9, 2.1)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1870 \\ 

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-3.0, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1875 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.1)}} & 662 & 54.29 & 52.05 \textcolor{gray}{\tiny $\pm$ 1.75} & 1880  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \textbf{60.7} \textcolor{gray}{{\tiny CI: (-2.7, 2.3)}} & 683 & \textbf{55.85} & \textbf{55.92} \textcolor{gray}{\tiny $\pm$ 1.74} & 1903 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.76 & 9.00 & 8.52 & 54.6 \textcolor{gray}{{\tiny CI: (-2.8, 2.2)}} & 664 & 54.40 & 55.72 \textcolor{gray}{\tiny $\pm$ 1.74} & 1841\\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8 \textcolor{gray}{{\tiny CI: (-2.4, 2.1)}} & 665 & 52.17 & 49.50 \textcolor{gray}{\tiny $\pm$ 1.75} & 1962 \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-i}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \textbf{60.3} \textcolor{gray}{{\tiny CI: (-2.8, 2.2)}} & 728 & \textbf{54.39} & \text{50.88} \textcolor{gray}{\tiny $\pm$ 1.74} & 1994 \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.74 & 9.01 & 8.47 & 57.2 \textcolor{gray}{{\tiny CI: (-2.9, 2.2)}} & 733 & 54.00 & 51.21 \textcolor{gray}{\tiny $\pm$ 1.75} & 2017\\

% \bottomrule

% \end{tabular}%
% }
% % \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:main-10k}
% \end{table}


\begin{table}[!ht]
\centering

% \vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39  & 1567 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 651 & 55.01 & 51.68  & 1883  \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8  & 733 & \textbf{55.74} & \textbf{56.15}  & 2111  \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva-i}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \textbf{60.1}  &  725 &  55.35 &    55.53  & 2089 \\ 

\midrule

$\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7  & 560 & 51.58 & 42.17  & 1850 \\

\rowcolor[HTML]{e9ebee}
$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7  & 562 & 51.78 & 42.98  & 1875 \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9}  & 567 & \textbf{51.86} & \textbf{43.04}  & 1870 \\ 


\midrule

$\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3  & 662 & 54.29 & 52.05  & 1880  \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts}      & 8.76 & 9.00 & 8.52 & 54.6  & 664 & 54.40 & 55.72  & 1841\\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \textbf{60.7}  & 683 & \textbf{55.85} & \textbf{55.92}  & 1903 \\ 



\midrule

$\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8  & 665 & 52.17 & 49.50  & 1962 \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}      & 8.74 & 9.01 & 8.47 & 57.2  & 733 & 54.00 & \textbf{51.21}  & 2017\\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva-i}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \textbf{60.3}  & 728 & \textbf{54.39} & 50.88  & 1994 \\ 

\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:main-10k}
\end{table}



==> tabs/tab-main-10k-o.tex <==
% \notes{The experiment is re-running.}
\FloatBarrier
\begin{table}[h]
\centering

% \vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ 
\midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 544 &  47.11 & 38.39 & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     &  & & & & & & & \\

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\

\rowcolor[HTML]{fcf1f0} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +    \texttt{\textbf{eva-o}} } & & & & & & & & \\





% \midrule



% $\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}      & 8,62 & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +    \texttt{\textbf{eva-o}} } & & & & & & & & \\

% \rowcolor[HTML]{e9ebee}
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}    & & & & & & & & \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.63 & & & & & & &  \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad +    \texttt{\textbf{eva-o}}  & & & & & & & & \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.62 & & & & & & & \\

% \rowcolor[HTML]{fcf1f0} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \quad +    \texttt{\textbf{eva-o}}  & & & & & & & & \\ 

% \rowcolor[HTML]{e9ebee} 
% $\vtheta_{1 \rightarrow 2}$: \quad +     \texttt{new human prompts}      & & & & & & & & \\





\bottomrule

\end{tabular}%
}
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:main-eva-o}
\end{table}

% \notes{This experiment is on-going.}

==> tabs/tab-main-10k.tex <==
% \begin{table}[H]
% \centering

% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-7}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-5} \cmidrule(l){6-7}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{WR} (\%)  & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

% $\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3  & 47.11 & 38.39 \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32 & 51.6  & 55.01  & 51.68  \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \textbf{8.90} & \textbf{9.04} & \textbf{8.75} & \hspace{+0.6cm}\textbf{60.1} \tc{\tiny (+8.5)}  &  55.35  & 55.53 \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{8.64} & \tgray{8.88} & \tgray{8.39} & \tgray{59.8}  & \tgray{\textbf{55.74}}  & \tgray{\textbf{56.15}}  \\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: SPPO       & 8.62 &  9.03 &  8.21 &  55.7  & 51.58  & 42.17 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \hspace{+0.6cm}\textbf{58.9} \tc{\tiny (+3.2)}   & \textbf{51.86}  & \textbf{43.04} \\ 

% \rowcolor[HTML]{f5f7fc}
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts} }   &  \tgray{8.64} &  \tgray{8.90} &  \tgray{8.39} &  \tgray{57.7}  & \tgray{51.78}  & \tgray{42.98} \\


% \midrule

% $\vtheta_{0 \rightarrow 1}$: SimPO      & 8.69 & 9.03 & 8.35 & 52.3  & 54.29  & 52.05 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} }  & \textbf{8.92} & \textbf{9.08} & \textbf{8.77} & \hspace{+0.6cm}\textbf{60.7} \tc{\tiny (+8.4)}   & \textbf{55.85}  & \textbf{55.92} \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts} }     & \tgray{8.76} & \tgray{9.00} & \tgray{8.52} & \tgray{54.6}  & \tgray{54.40}  & \tgray{55.72}\\

% \midrule

% $\vtheta_{0 \rightarrow 1}$: ORPO     & 8.67 & 9.04 & 8.30 & 54.8  & 52.17  & 49.50 \\



% \rowcolor{gred!12} 
% $\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} }  & \textbf{8.89} & \textbf{9.07} & \textbf{8.71} & \hspace{+0.6cm}\textbf{60.3} \tc{\tiny  (+5.5)}   & \textbf{54.39}  & \textbf{50.88} \\ 

% \rowcolor[HTML]{f5f7fc} 
% \tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}}      & \tgray{8.74} & \tgray{9.01} & \tgray{8.47} & \tgray{57.2}  & \tgray{54.00}  & \tgray{\textbf{51.21}} \\

% \bottomrule

% \end{tabular}%
% }
% \caption{\textbf{Main results.} \method~achieves concrete alignment gain and even surpasses  human prompts.}

% \label{tab:main-10k}
% \end{table}

\begin{table}[H]
\centering

\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Gemma-2-9B-it}}} \\ \cmidrule(l){2-7}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}



\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%)      & \textbf{avg. score}   & $1^{\text{st}}$ turn  & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

$\vtheta_0$: SFT                &  41.3  &  8.57 &  8.81 &  8.32 & 47.11 & 38.39 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 51.6  & 8.66 & 9.01 & 8.32 & 55.01  & 51.68  \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.1} \tc{\tiny (+8.5)}  & \textbf{8.90} & \textbf{9.04} & \hspace{+0.7cm}\textbf{8.75} \tc{\tiny (+0.43)} &  55.35  & 55.53 \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{59.8}  & \tgray{8.64} & \tgray{8.88} & \tgray{8.39} & \tgray{\textbf{55.74}}  & \tgray{\textbf{56.15}}  \\

\midrule

$\vtheta_{0 \rightarrow 1}$: SPPO       & 55.7  & 8.62 &  9.03 &  8.21 &  51.58  & 42.17 \\



\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } &  \hspace{+0.6cm}\textbf{58.9} \tc{\tiny (+3.2)} & \textbf{8.78} & \textbf{9.11} &  \hspace{+0.7cm}\textbf{8.45} \tc{\tiny (+0.24)} & \textbf{51.86}  & \textbf{43.04} \\ 

\rowcolor[HTML]{f5f7fc}
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts} }   & \tgray{57.7}  &  \tgray{8.64} &  \tgray{8.90} &  \tgray{8.39} &  \tgray{51.78}  & \tgray{42.98} \\


\midrule

$\vtheta_{0 \rightarrow 1}$: SimPO      & 52.3  & 8.69 & 9.03 & 8.35 & 54.29  & 52.05 \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.7} \tc{\tiny (+8.4)} & \textbf{8.92} & \textbf{9.08} & \hspace{+0.7cm}\textbf{8.77} \tc{\tiny (+0.42)} & \textbf{55.85}  & \textbf{55.92} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +  \texttt{new human prompts} }     & \tgray{54.6}  & \tgray{8.76} & \tgray{9.00} & \tgray{8.52} & \tgray{54.40}  & \tgray{55.72}\\

\midrule

$\vtheta_{0 \rightarrow 1}$: ORPO     & 54.8  & 8.67 & 9.04 & 8.30 & 52.17  & 49.50 \\



\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \text{\quad +   \texttt{\textbf{eva}} } & \hspace{+0.6cm}\textbf{60.3} \tc{\tiny  (+5.5)} & \textbf{8.89} & \textbf{9.07} & \hspace{+0.7cm}\textbf{8.71} \tc{\tiny (+0.41)} & \textbf{54.39}  & \textbf{50.88} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +    \texttt{new human prompts}}      & \tgray{57.2}  & \tgray{8.74} & \tgray{9.01} & \tgray{8.47} & \tgray{54.00}  & \tgray{\textbf{51.21}} \\

\bottomrule

\end{tabular}%
}
\caption{\textbf{Main results.} Our~\method~achieves notable alignment gains and can surpass human prompts on major benchmarks across a variety of representative direct preference optimization algorithms.}
\label{tab:main-10k}
\end{table}
\vspace{-10pt}



==> texs/ack.tex <==
\section*{Acknowledgements}
We extend our sincerest gratitude to Bilal Piot for his thoughtful reviews and valuable advice on this paper. We are also grateful to Chenkai Kuang, Dustin Tran, Albert Webson, Hanzhao Lin, Clara Huiyi Hu, Jeremiah Liu, Luheng He, Chenjie Gu, Yong Cheng, Pei Sun, and Heng-Tze Cheng for their fun discussions and notes on Self-Play. We also thank David Abel, Yuxin Chen, Ziniu Hu, Guohao Li, Rylan Schaeffer, Haifeng Xu, Chaoqi Wang and Yifei Wang for their initial helpful discussions and references on fine-tuning, contrastive learning, data synthesis, open-ended learning, and continual reinforcement learning.

\section*{Reproducibility Statement}

We hope to open-source all the code,  datasets (synthesized prompts/responses) and models, \textit{upon approval}. Before then, we are more than happy to provide any clarification requested to help re-implement~\method~and replicate our results. Our code base is made to be simple to use for practitioners, requiring \text{only a creator module addition} to the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline. 

\section*{Societal Impact}
% Example from the Genie Paper
% Genie could enable a large amount of people to generate their own game-like experiences. This could be positive for those who wish to express their creativity in a new way, for example children who could design and step into their own imagined worlds. We also recognize that with significant advances, it will be critical to explore the possibilities of using this technology to amplify existing human game generation and creativity-and empowering relevant industries to utilize Genie to enable their next generation of playable world development.

\method~enables scalable training of language agents through open-ended training, improving AI alignment with human values, which may ultimately contribute to social welfare~\citep{pigou1920some,arrow1952social,zhi2024beyond}. This could \emph{democratize} the development of more generally capable AI agents, benefiting a wide range of applications from education to scientific discovery.

We recognize that~\method~relies on self-exploration guided by reward signals. If these signals are inaccurate or misaligned, the trained agents may exhibit undesirable behaviors such as reinforcing biased hallucination. Mitigating these risks requires continued research into robust reward models, transparent evaluation protocols, open collaboration within the AI research community, and more. We are committed to supporting these efforts by sharing our findings and  implementations to promote open and responsible research and development.

==> texs/analysis.tex <==
% \newpage
% \section{\textcolor{Gray}{[1\% Draft]} Theoretical Analysis}

% % \begin{thm}[Restated from Theorem 1 of~\citep{self-play-gu}] 
% % Assume the optimization problem is realizable in Eq.~\ref{eq:sppo-2}. Denote $\bar{\pi}_T=\frac{1}{T} \sum_{t=1}^T \pi_t$ as the average policy. By setting $\eta=\Theta(1 / \sqrt{T})$, the convergence rate of the average policy towards the Nash equilibrium is:
% % \begin{align}
% %     \max _\pi\left[\mathbb{P}\left(\pi \succ \bar{\pi}_T\right)\right]-\min _\pi\left[\mathbb{P}\left(\pi \prec \bar{\pi}_T\right)\right]=O(1 / \sqrt{T}) .
% % \end{align}
% % \end{thm}

% % The optimal policy is defined with regard to the initial $\calX_{\text{init}}$ and a pre-defined preference oracle $\sP(\cdot)$. Assuming there is a superset $\calX$ that $\mathcal{X}_{\text{init}} \subset \mathcal{X}$, we can show that the learned policy can be suboptimal under $\calX$. The interesting question is, that can we construct a sequence of $\{\calX_t\}_{t=0}^{\infty}$, such that the policy performance is monotonically improving?

% % The challenge here is, that unlike classical active learning, which mostly  cares about the \emph{sampling} issues, we care about \emph{generating} novel prompts from a fixed vocabulary.


% \begin{ftheo}[Policy Convergence with a Fixed Prompt Set, Restated from~\cite{self-play-gu}]

% Let $\mathcal{X}_{\text{init}}$ be a fixed prompt set and $\mathbb{P}(\cdot \succ \cdot)$ be a pre-defined preference oracle. Assume that the optimization problem is realizable in Eq.~\ref{eq:sppo-2}. Denote $\bar{\pi}_T=\frac{1}{T} \sum_{t=1}^T \pi_t$ as the average policy learned from $\mathcal{X}_{\text{init}}$. By setting $\eta=\Theta(1 / \sqrt{T})$, the convergence rate of the average policy towards the Nash equilibrium is:
% \begin{align}
%     \max_\pi\left[\mathbb{P}\left(\pi \succ \bar{\pi}_T\right)\right]-\min_\pi\left[\mathbb{P}\left(\pi \prec \bar{\pi}_T\right)\right]=O(1 / \sqrt{T}) .
% \end{align}
% \end{ftheo}
% % \begin{ftheo}

% Assuming a golden preference oracle, the convergence properties is established for a fixed prompt set $\mathcal{X}_{\text{init}}$. However, in real-world scenarios, we often encounter a broader range of prompts than initially anticipated. Let $\mathcal{X}$ be a superset representing the true distribution of prompts, where $\mathcal{X}_{\text{init}} \subset \mathcal{X}$. The policy $\pi^\star$ that is optimal with respect to $\mathcal{X}_{\text{init}}$ \emph{can be suboptimal} when evaluated on $\calX$.

% This observation motivates us to consider an evolving prompt set. The key question is: \emph{can we construct this sequence such that the performance of $\pi_t$ improves monotonically when evaluated on the full set $\mathcal{X}$?} This is just like mathematical conjecturing. Given a fixed set of known axioms or theorem statements, our goal is to navigate in the language space to iteratively create a new set which approximately covers all valid theorem statements. We formalize the idea below.

% \begin{mdframed}
% \begin{defn}[Prompt Set Sequence]
% A prompt set sequence is a series $\{\mathcal{X}_t\}_{t=0}^{\infty}$ where $\mathcal{X}_0 = \mathcal{X}_{\text{init}}$ and for all $t \geq 0$, $\mathcal{X}_t \subseteq \mathcal{X}_{t+1} \subseteq \mathcal{X}$, with $\mathcal{X}$ being a superset with all possible prompts.
% \end{defn}
% \end{mdframed}

% This question presents unique challenges distinct from classical active learning. While active learning primarily addresses sampling from a fixed set, our problem involves generating novel prompts from a fixed vocabulary. This generative aspect introduces additional complexity, as we must ensure that new prompts are both syntactically valid and semantically meaningful.



% \begin{mdframed}
% \begin{defn}[Policy Performance]
% Given a prompt set $\mathcal{X}$ and a preference oracle $\mathbb{P}(\cdot)$, the performance of a policy $\pi$ is defined as:
% \begin{align}
%     J(\pi, \mathcal{X}) = \mathbb{E}_{\mathbf{x} \sim \mathrm{Unif}(\mathcal{X})} \left[ \mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x})} [\mathbb{P}(\vtau \succ \pi_{\text{ref}} \mid \mathbf{x})] \right].
% \end{align}
% where $\pi_{\text{ref}}$ is any reference policy.
% \end{defn}
% \end{mdframed}

% The challenge lies in constructing each $\mathcal{X}_{t+1}$ such that $J(\pi_{t+1}, \mathcal{X}) \geq J(\pi_t, \mathcal{X})$. 

% %This is non-trivial because expanding the prompt set introduces new challenges for the policy, potentially leading to temporary decreases in performance. Moreover, the true set $\mathcal{X}$ is unknown, making direct optimization of $J(\pi_t, \mathcal{X})$ infeasible.

% \begin{mdframed}
% \begin{pro}[Prompt Generation]
% Given a fixed vocabulary $V$, a current prompt set $\mathcal{X}_t$, and a current policy $\pi_t$, find a function $g: V \times \mathcal{X}_t \times \Pi \rightarrow \mathcal{X}$ such that:
% \begin{enumerate}
%     \item $g(V, \mathcal{X}_t, \pi_t) \not\subseteq \mathcal{X}_t$.
%     \item $J(\pi_t, \mathcal{X}_t \cup g(V, \mathcal{X}_t, \pi_t)) \geq J(\pi_t, \mathcal{X}_t)$.
% \end{enumerate}

% where $\Pi$ is the space of all policies.
% \end{pro}
% \end{mdframed}












% % \subsection{Evolving Prompt Distribution}
% % \notes{To add more motivation here with formalized theoretical toy example. A simple intuition is, that assume the original prompt set contain an imbalanced set of easy and hard examples, and we should do dynamic upsampling and downsampling. Check the efficient exploration paper~\citep{efficient-llm}.}

% % In the SPPO framework, prompts are assumed to be sampled from a fixed distribution $\mathcal{X}$. However, in practice, we often work with a finite set of prompts that may not fully represent the true distribution of tasks the model will encounter. This mismatch can lead to poor generalization and inefficient learning. We formalize this issue in the following theorem:

% % \begin{lem}[Inefficiency of Static Prompt Set]
% % Let $\mathcal{X}$ be the true distribution of prompts, and let $\mathcal{X}_0 \subset \mathcal{X}$ be a finite subset used for training. Define the expected improvement for a prompt $\mathbf{x}$ at iteration $t$ as:
% % \begin{equation}
% % I_t(\mathbf{x}) = \mathbb{E}_{\vtau \sim \pi_t(\cdot|\mathbf{x})}[\max(0, \mathbb{P}(\vtau \succ \pi_t | \mathbf{x}) - 1/2)].
% % \end{equation}

% % For any $\epsilon > 0$, there exists a $T$ such that for all $t > T$:
% % \begin{equation}
% % \max_{\mathbf{x} \in \mathcal{X}_0} I_t(\mathbf{x}) < \epsilon,
% % \end{equation}

% % while there exists an $\mathbf{x}' \in \mathcal{X} \setminus \mathcal{X}_0$ such that:
% % \begin{equation}
% % I_t(\mathbf{x}') > \epsilon.
% % \end{equation}
% % \end{lem}

% % \notes{Re-state the lemma. The fundamental idea here is, that if we are sampling from a subset, the convergence will not be the Nash equilibrium, but rather the Berk-Nash equilibrium. We should thus build a sequence of $\calX_t$, so that we can converge.}

% % The intuition is that a static prompt set eventually becomes inefficient for learning, as the model's performance on these prompts plateaus while it remains poor on unseen prompts.

% % To address this issue, we propose a dynamic prompt set expansion strategy:

% % \begin{defn}[Dynamic Prompt Set]
% % Let $\mathcal{X}_t$ be the prompt set at iteration $t$. We update the prompt set according to:
% % \begin{equation}
% % \mathcal{X}_{t+1} = (1 - \alpha) \cdot \mathcal{X}_t \cup \alpha \cdot \calS_t
% % \end{equation}
% % where $\calS_t$ is a set of newly sampled prompts based on a criterion $C_t$ defined below, and $\alpha \in (0,1)$ is a mixing parameter.
% % \end{defn}

% % % The key challenge is defining an effective criterion $C_t$ for sampling new prompts. 

% % \begin{defn}[Uncertainty-based Prompt Sampling]
% % Let $U_t(\mathbf{x})$ be an uncertainty measure for prompt $\mathbf{x}$ at iteration $t$. We define:
% % \begin{equation}
% % C_t(\mathbf{x}) \propto U_t(\mathbf{x}) \cdot p(\mathbf{x})
% % \end{equation}

% % where $p(\mathbf{x})$ is an estimate of the true prompt distribution.
% % \end{defn}

% % There are different practical design choices to concertize the evolving prompt sets.

% % % -----------------------------------------
% % \subsection{Preference Model Refinement}
% % % -----------------------------------------

% % To address the limitations of a fixed preference oracle, we propose to \emph{distill} and \emph{refine} a preference (critic?) model alongside the policy. This approach allows us to distill knowledge from the oracle and potentially generalize beyond its limitations.

% % Let $p_\phi(\vtau \succ \vtau' | \mathbf{x})$ be a parameterized preference model (which could be trained with the network for the policy?). In the most naïve formulation, we can update this model using the beow objective:
% % \begin{equation}
% % \mathcal{L}_\text{pref}(\phi) = \mathbb{E}_{\mathbf{x}, \vtau, \vtau'}[(\mathbb{P}(\vtau \succ \vtau' | \mathbf{x}) - P_\phi(\vtau \succ \vtau' | \mathbf{x}))^2]
% % \end{equation}

% % We can then use this learned preference model in the SPPO update:
% % \begin{align}
% % \pi_{t+1}(\vtau | \mathbf{x}) \propto \pi_t(\vtau | \mathbf{x}) \exp(\eta \cdot p_\phi(\vtau \succ \pi_t | \mathbf{x})).
% % \end{align}

% % Intuitively, this approach allows the model to learn to discriminate at the same time.

% % Some other ideas:

% % \subsubsection{Online Preference Learning}

% % We can learn the preference model online, simultaneously with the policy. This approach is closer to the Berk-Nash equilibrium concept. The learned preference model represents the \emph{subjective belief} of the language models.

% % \begin{defn}[Online Preference Learning]
% % At each iteration $t$:
% % \begin{enumerate}
% %     \item Update preference model: $\theta_{t+1} = \arg\min_\theta L(\theta; \mathcal{D}_t)$
% %     where $\mathcal{D}_t$ is the observed preference data up to time $t$, and $L$ is a suitable loss function.
% %     \item Update policy: $\pi_{t+1}(\vtau|\mathbf{x}) \propto \pi_t(\vtau|\mathbf{x}) \exp(\eta P_{\theta_{t+1}}(\vtau \succ \pi_t | \mathbf{x}))$
% % \end{enumerate}
% % \end{defn}

% % This approach allows the preference model to adapt over time as more data is collected.

% % \subsubsection{Uncertainty-Aware Preference Modeling}

% % Instead of a point estimate, we maintain a distribution over preference models to capture uncertainty in our preference estimates.

% % \begin{defn}[Bayesian Preference Modeling]
% % We model the preference probability as:
% % \begin{align}
% % P(\vtau \succ \vtau' \mid \mathbf{x}) = \int P(\vtau \succ \vtau' \mid \mathbf{x}, \theta) p(\theta \mid \mathcal{D}_t) d\theta
% % \end{align}

% % where $p(\theta \mid \mathcal{D}_t)$ is the posterior  over preference model parameters given observed data $\mathcal{D}_t$.
% % \end{defn}

% % This Bayesian approach allows us to incorporate uncertainty into our policy updates and potentially make more informed decisions.

% % \begin{thm}[Convergence under Misspecified Preferences]
% % Under certain regularity conditions, if we use either the Online Preference Learning or Uncertainty-Aware Preference Modeling approach, the policy $\pi_t$ converges to a Berk-Nash equilibrium as $t \to \infty$.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows these key steps:
% % \begin{enumerate}
% %     \item The preference model converges to the best approximation within the model class, minimizing KL divergence to the true preference distribution.
% %     \item Given this converged preference model, the policy update converges to the optimal policy for this model.
% %     \item This combination of beliefs (represented by the converged preference model) and policy satisfies the definition of Berk-Nash equilibrium.
% % \end{enumerate}
% % A full proof would require specifying the regularity conditions and providing a more detailed analysis of the convergence properties.
% % \end{proof}

% % This theorem provides a theoretical foundation for our approach, showing that under appropriate conditions, our evolving self-play alignment framework can converge to a meaningful equilibrium even in the presence of misspecified preferences.



==> texs/app-exp.tex <==
\newpage
\textbf{------------------- OLD OUTDATED STUFFS IGNORE --------------------}
\section{Comprehensive Evaluation Results on Alignment Benchmarks}

We here show evolving is helpful for alignment under different training settings.


\paragraph{Hyperparameter settings.} Unless otherwise specified, we use the hyperparameter setting below:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.66\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{IPO}    & \textbf{SimPO}  & \textbf{SPPO}    \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & 0.6    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ \bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-params}
\end{table}

\paragraph{Iterative Training Settings.} By default~\citep{self-play-gu}, we split data into equal-size subsets, then iterative train the model with different split at each iteration as:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_1$ : init with $\vtheta_0$; trained w/ the prompt split $D_1$ by self-generated responses.
    \item $\vtheta_2$ : init with $\vtheta_1$; trained w/ the prompt split $D_2$ via by self-generated responses.
    \item ...
\end{itemize}
\vspace{-5pt}
For the evolved models:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_1^{\text{evol}}$ : init with $\vtheta_1$; evolve $D_1$ to $D_1^{\text{evol}}$ by feedbacks from $\vtheta_1$; train with a mixture of $D_1$ and $D_1^{\text{evol}}$ by self-generated responses. 
    \item $\vtheta_2^{\text{evol}}$ : init with $\vtheta_1^{\text{evol}}$; train w/ $D_2$ by self-generated responses to get $\vtheta_2^{\text{evol}, \prime}$; evolve $D_2$ to $D_2^{\text{evol}}$ by feedbacks from $\vtheta_2^{\text{evol}, \prime}$; train w/ a mix of $D_2$ and $D_2^{\text{evol}}$ by self-generated responses. 
    \item ...
\end{itemize}



    % \item \textbf{Average Optimal Advantage}: This can be viewed as an approximation to the \emph{negative} \textbf{Bayesian regret}. Take $N$ as the total number of generated responses:
    % \begin{align}
    %     \hspace{-66pt} \emphblue{A^{\star}_{\text{avg}}(\rvx)} = r^{\star}(\rvx) - \frac{1}{N} \sum_{\rvy}r(\rvx, \rvy). \label{eq:avg-advantage}
    % \end{align}
    % \item \textbf{Leave-One-Out Advantage:} Excluding the current response from the average:
    % \begin{align}
    %     \emphblue{A_{\text{loo}}(\rvx)} = \frac{1}{N} \sum_{\rvy} \Bigr(r(\rvx, \rvy) - \frac{1}{N-1} \sum_{\rvy' \neq \rvy} r(\rvx, \rvy') \Bigr). \label{eq:loo-advantage}
    % \end{align}

% \begin{table}[!h]
% \centering
% \label{tab:lm-glossary}
% % \resizebox{1.0\columnwidth}{!}{%
% \begin{tabular}{ll}
%  &  \\
%  &  \\
% \end{tabular}%
% % }
% \end{table}


% \subsection{Setting 1: Iterative Training with 6 Splits}


% % In the default setting, we split the 60K UltraFeedback data into 6 splits. For each iteration, we use the exactly same hyperparameter setting, albeit different.

% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule

% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 9.01 & 8.32& 8.66& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-p}) } &  \textbf{9.04}& \textbf{8.75} & \textbf{8.90}& \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  \textbf{55.35} &    \textbf{55.53} \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 
% \midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  9.00 &  8.45 &  8.72 & \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{eva-p}) } &   &  &   &  &  &  &  & \\ 
% \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      &  9.03 &  8.21 &  8.62 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% \qquad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% \qquad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{eva-p}) } & \textbf{9.11} &  \textbf{8.45} &  \textbf{8.78} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-1}
% \end{table}
% % --------------------------------------------------------

% \ziyu{It looks like IPO is sensitive to the hyperparameter setting. The previous setting uses n\_epoch=2}

% \subsection{Setting 2: Iterative Training with 3 Splits}
% % --------------------------------------------------------
% \ziyu{The DPO here is using gpt-4o-mini to evolve, and we observe a drop in the performance compared to Iter 1. Notice that existing literature~\citep{self-play-gu} also reports drop during multiple iterations. It is likely that we need to control the hyper-parameter setting (\eg decrease the learning rate for the new iteration) for better performance.}

% \ziyu{It is very likely that there is reward hacking, and the reward model per se may be much imperfect.}

% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}
% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule

% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule

% DPO \  \hspace{+3pt}   Iter 1 / 3    & 9.21 & 8.67& 8.94 &  56.6 \textcolor{gray}{{\tiny CI: (-2.1, 2.5)}} &  729&  \textbf{54.38} &  50.93 \textcolor{gray}{\tiny $\pm$ 1.76} & 1909  \\
% \qquad \ \ \ \hspace{+1pt} Iter 2 / 3      &   9.35 &  8.83 & 9.09 & &  & 41.98 & 40.75 \textcolor{gray}{\tiny $\pm$ 1.73} & 3505  \\
% \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       &  9.15 & 8.55 & 8.85 & & & 37.17 & 35.40 \textcolor{gray}{\tiny $\pm$ 1.68} & 2962 \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \  \hspace{+3pt}   Iter 1 / 3 (\texttt{eva-p}) } & 9.19 & 8.39 & 8.79& \textbf{59.5} \textcolor{gray}{{\tiny CI: (-2.0, 2.4)}} & 826   &  49.89 &    \textbf{51.61} \textcolor{gray}{\tiny $\pm$ 1.76} & 2394 \\ 

% % \midrule

% % IPO \ \hspace{+6pt}  Iter 1    &  &   &   \\
% % \qquad \ \ \ \hspace{+0.001pt} Iter 2        &   \\
% % \qquad \ \ \  \hspace{+0.001pt} Iter 3        &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO \ \hspace{+6pt}  Iter 1  (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 

% % \midrule

% % SimPO  Iter 1 / 3         &    \\
% % \qquad \ \ \ \hspace{+1pt} Iter 2 / 3        &   \\
% % \qquad \ \ \  \hspace{+1pt} Iter 3 / 3        &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{SimPO Iter 1 / 3 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% % \midrule

% % SPPO \hspace{+2pt}  Iter 1 / 3     &   \\
% % \qquad \ \ \ \hspace{+1pt} Iter 2 / 3       &   \\
% % \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{SPPO \hspace{+2pt} Iter 1 / 3 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 



% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-2}
% \end{table}
% % --------------------------------------------------------


% \subsection{Setting 3: Iterative Training with No Split}
% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}
% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule
% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule
% DPO \hspace{+1pt}        &  \\
% \rowcolor[HTML]{e2fbe2} 

% \text{DPO (\texttt{eva-p}) } &  &  &   &  &  &  &  &  \\ 
% \midrule
% IPO \hspace{+1pt}      &  &   &   \\
% \rowcolor[HTML]{e2fbe2} 
% \text{IPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \midrule
% SPPO \hspace{+1pt}     &   \\



% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \midrule
% SimPO \hspace{+1pt}        &    \\
% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \bottomrule
% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-3}
% \end{table}
% % --------------------------------------------------------


% \newpage
% \section{Ablation Studies}
% In this section, we present detailed analysis with ablation on:
% \begin{itemize}
%     \item Sampling setting:
%     \item Infomrativeness metric:
%     \item Prompt Evolving Strategy:
%     \item Prompt Generation Model:
% \end{itemize}

% % (i) sampling setting; (ii)

% For all the ablation study, we use DPO as the default loss function, and use 10K data (\ie the first split) from the UltraFeedback dataset as the training data.

% \subsection{Ablation Study on the Sampling Setting}
% We consider using filtering v.s. weighted sampling v.s. weighted sampling on a graph.

% \subsection{Ablation Study on the Informativeness Metric}
% Take one of the above setting, vary on the metric. We currently consider:
% \begin{itemize}
%     \item max-min advantage:
%     \item max-mean advantage:
%     \item leave-one-out advantage:
%     \item reward mean:
% \end{itemize}

% \subsection{Ablation Study on the Prompt Evolving Strategy}

% % \subsection{Ablation Study on the Mixup Ratio}

% \subsection{Ablation Study on the LLMs Used to Generate the Prompts}
% We consider to use different underlying models to generate new prompts.
% \textbf{---------- OLD STUFFS ----------}

==> texs/app-lit.tex <==
% \newpage
% \section{Extended Literature Review}

% \paragraph{Open-ended learning.} 
% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{plr}:
%     \item \cite{paired}:
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% % \cite{poet, paired, accel, minimax-refine}
% % faster convergence and better generalization
% % incentivizing / guiding the learner to better basin of attraction



% % \paragraph{Open-ended learning.}

==> texs/app-main-cp.tex <==
% \section{Reproducibility Statement}\label{app:settings}

% \paragraph{Hyperparameter settings.} We follow the hyperparameter setting stated in~\citep{orpo,simpo,self-play-gu}, default to be:

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \centering
% \resizebox{0.7\columnwidth}{!}{%
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
% learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
% learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
% $\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
% $\gamma$                                                      & /      & /      & 5      & /       \\
% $\lambda$                                                      & /      & 0.5      & /      & /       \\
% no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
% warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
% effective batch size                                          & 8      & 8      & 32     & 8       \\
% max length                                                    & 2048   & 2048   & 2048   & 1024    \\
% max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
% optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
% \bottomrule
% \end{tabular}%
% }
% % \caption{Hyper}
% \label{tab:app-main-params}
% \end{table}


% \paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-rewarding}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
% \vspace{-5pt}
% \begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
%     \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
%     % \item ...
% \end{itemize}

% For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this as well as other plug-in evolving methods.

% % \paragraph{Computation environments.} 

% \paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve OpenAI models and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. In general, our codebase is very simple to use and requires only a creator module addition within the \href{https://github.com/huggingface/alignment-handbook}{Alignment Handbook} pipeline.

%  \paragraph{Code release.} We currently put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\textcolor{black}{\texttt{\small anonymous.4open.science/r/eva-i/}}}, which we intend to as well release all the source code there, and all the datasets and models to HuggingFace, upon approval -- before then, we are happy to provide any additional clarification requested to help re-implement~\method~and replicate our results. 

% \paragraph{Evaluation settings.} If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge, and \texttt{gpt-4-0314} as the baseline when calculating the win rate for evaluating on the benchmarks.





% -------------------------------------------------------------
\section{Issues of Fixed Prompt Training Distributions}\label{app:prompts}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
    \caption{The initial prompt distribution of AlpacaEval (openly accessible on HuggingFace) obtained from zero-shot classification with \texttt{bart-large-mnli}, which is imbalanced. Additionally, looking at the reward distribution, the category with lowest average reward has the highest average reward gap (\ie our default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
\end{figure}


% \paragraph{\emphtext{\method~minimally impact downstream tasks.}} 




% \section{Extended Discussions on Open-Ended Learning}

% The design of our game-theoretic framework is inspired from many prior works in open-ended learning, which we encourage the LLM community to explore more.  The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but general enough to handle the diversity of complexity of future environments. In the curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively build more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case environments. It is not just about generalizing to novel environments but also about ensuring that the agent can handle the most challenging scenarios within those environments. This distinction highlights the value of minimax regret: while classical open-ended learning focuses on generalization through exposure to diverse environments, minimax regret ensures that the agent is robust even under the most adversarial conditions.


% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{paired}: using two agents to simulate the regret.
%     \item \cite{plr}: having a rolling buffer of high-regret levels.
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% \paragraph{Self-improving / self-training language models.} 
\section{Additional Experimental Results}
% \subsection{Evaluation on Downstream Tasks}\label{sec:ab-downstream}
In general,~\method~maintains the accuracy on downstream tasks and is robust on those reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to the training sources for such reward models~\citep{armorm}.
\input{tables/tab-ab-downstream}
\vspace{-8pt}

% \subsection{The Effect of Different Reward Models at Different Scales}\label{app:ab-rm}
% In general, \method~presents scaling behavior across different datasets. We notice that the performance on MT-Bench is less stable, which may be due to the limited evaluation scale (80 questions), as similarly reported in~\citep{simpo,ah}
% \notes{The experiment is running.}
\input{tables/tab-ab-rm-app}


% -------------------------------------------------------------
% \section{Limitations}\label{app:limit}
% Off-policy is one concern. Another concern is that the advantage-based framework does not inherently works for general preference (we first do pairwise comparison; after )

% \subsection{The On-Polcy Variant: \texttt{eva-o}}\label{app:eva-o}
% The iterative training approach is inherently an off-policy algorithm; while being efficient, the performance can get plateau when more iterations goes on. We hereby show our method can easily extend to be on-policy, as shown in Algorithm~\ref{alg:o-eva}, that draws inspiration from Iterative Machine Teaching~\citep{bo-mt} and Ordered SGD~\citep{ordered-sgd} in the informative pool set selection (Line 4, which can be achieved either by greedy or through weighted sampling), while adding the new evolving step (Line 5). 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}(\vx_i)\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \texttt{evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }





% \section{Prompt Examples and Distributions}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/example-prompt.png}
%     \caption{Prompts}
%     \label{fig:app-prompts}
% \end{figure}




==> texs/app-main.tex <==
% \section{Reproducibility Statement}\label{app:settings}

% \paragraph{Hyperparameter settings.} We follow the hyperparameter setting stated in~\citep{orpo,simpo,self-play-gu}, default to be:

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \centering
% \resizebox{0.7\columnwidth}{!}{%
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
% learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
% learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
% $\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
% $\gamma$                                                      & /      & /      & 5      & /       \\
% $\lambda$                                                      & /      & 0.5      & /      & /       \\
% no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
% warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
% effective batch size                                          & 8      & 8      & 32     & 8       \\
% max length                                                    & 2048   & 2048   & 2048   & 1024    \\
% max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
% optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
% \bottomrule
% \end{tabular}%
% }
% % \caption{Hyper}
% \label{tab:app-main-params}
% \end{table}


% \paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-rewarding}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
% \vspace{-5pt}
% \begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
%     \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
%     % \item ...
% \end{itemize}

% For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this as well as other plug-in evolving methods.

% % \paragraph{Computation environments.} 

% \paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve OpenAI models and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. In general, our codebase is very simple to use and requires only a creator module addition within the \href{https://github.com/huggingface/alignment-handbook}{Alignment Handbook} pipeline.

%  \paragraph{Code release.} We currently put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\textcolor{black}{\texttt{\small anonymous.4open.science/r/eva-i/}}}, which we intend to as well release all the source code there, and all the datasets and models to HuggingFace, upon approval -- before then, we are happy to provide any additional clarification requested to help re-implement~\method~and replicate our results. 

% \paragraph{Evaluation settings.} If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge, and \texttt{gpt-4-0314} as the baseline when calculating the win rate for evaluating on the benchmarks.





% -------------------------------------------------------------
\section{Issues of Fixed Prompt Training Distributions}\label{app:prompts}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
    \caption{The initial prompt distribution of AlpacaEval (openly accessible on HuggingFace) obtained from zero-shot classification with \texttt{bart-large-mnli}, which is imbalanced. Additionally, looking at the reward distribution, the category with lowest average reward has the highest average reward gap (\ie our default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
\end{figure}


% \paragraph{\emphtext{\method~minimally impact downstream tasks.}} 




% \section{Extended Discussions on Open-Ended Learning}

% The design of our game-theoretic framework is inspired from many prior works in open-ended learning, which we encourage the LLM community to explore more.  The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but general enough to handle the diversity of complexity of future environments. In the curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively build more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case environments. It is not just about generalizing to novel environments but also about ensuring that the agent can handle the most challenging scenarios within those environments. This distinction highlights the value of minimax regret: while classical open-ended learning focuses on generalization through exposure to diverse environments, minimax regret ensures that the agent is robust even under the most adversarial conditions.


% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{paired}: using two agents to simulate the regret.
%     \item \cite{plr}: having a rolling buffer of high-regret levels.
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% \paragraph{Self-improving / self-training language models.} 
\section{Additional Experimental Results}

In general,~\method~maintains the accuracy on downstream tasks and is robust on those reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to the training sources for such reward models~\citep{armorm}.
\input{tables/tab-ab-downstream}
\vspace{-8pt}

\input{tables/tab-ab-rm-app}

\begin{table}[H]
\centering

\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Llama-3.2-3B-instruct}}} \\ \cmidrule(l){2-7}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}



\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%)      & \textbf{avg. score}   & $1^{\text{st}}$ turn  & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

$\vtheta_0$: SFT                & 9.7  & 7.24 & 7.60 & 6.88 & 27.15 & 29.94 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 11.4  &7.28  & 7.67 & 6.88 & 28.32 & 32.17 \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \textbf{13.0} & \textbf{7.37} & \textbf{7.71} & \textbf{7.03} & \textbf{29.54}  & \textbf{33.68} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{}  & \tgray{} & \tgray{} & \tgray{} & \tgray{\textbf{}}  & \tgray{\textbf{}}  \\



\bottomrule

\end{tabular}%
}
\caption{\textbf{Results with \text{Llama} models.}.}
\label{tab:main-10k-llama}
\end{table}
\vspace{-10pt}


% -------------------------------------------------------------
% \section{Limitations}\label{app:limit}
% Off-policy is one concern. Another concern is that the advantage-based framework does not inherently works for general preference (we first do pairwise comparison; after )

% \subsection{The On-Polcy Variant: \texttt{eva-o}}\label{app:eva-o}
% The iterative training approach is inherently an off-policy algorithm; while being efficient, the performance can get plateau when more iterations goes on. We hereby show our method can easily extend to be on-policy, as shown in Algorithm~\ref{alg:o-eva}, that draws inspiration from Iterative Machine Teaching~\citep{bo-mt} and Ordered SGD~\citep{ordered-sgd} in the informative pool set selection (Line 4, which can be achieved either by greedy or through weighted sampling), while adding the new evolving step (Line 5). 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}(\vx_i)\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \texttt{evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }





% \section{Prompt Examples and Distributions}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/example-prompt.png}
%     \caption{Prompts}
%     \label{fig:app-prompts}
% \end{figure}




==> texs/app-notes.tex <==
\section{Temporary Notes}



% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% DPO \ \hspace{+3pt} Iter 2 / 6       & 8.64 & 8.88 & 8.39 & on h100-west \textcolor{gray}{{\tiny CI: (, )}} &  & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{d6fcf9}  
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-greedy}) } & 8.72 & \textbf{9.06} & 8.36 & on a100-cc & & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-iw}) } & \\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-greedy}) } & \\ 

% \rowcolor[HTML]{e9ebee}
% Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% % IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% % \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% % \quad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% % \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:notes}
% \end{table}
% % --------------------------------------------------------
% \footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
% \footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}



% --------------------------------------------------------
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

\rowcolor[HTML]{e2fbe2}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{eva-greedy} } & 8.72 & \textbf{9.06} & 8.36 & 59.5 \textcolor{gray}{{\tiny CI: (-2.5, 2.2)}} & 736 & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K  \texttt{subset-iw} } & 8.69 & 9.00 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K   \texttt{subset-greedy} } & 8.68 & 8.98 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\






\rowcolor[HTML]{e9ebee}
Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

\midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% \midrule




$\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 

\rowcolor[HTML]{e9ebee}
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1692 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: IPO      & 8.72 & 9.00 & 8.45 & 45.2 \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}} & 587 & 52.02 & 45.43 \textcolor{gray}{\tiny $\pm$ 1.75} & 1726 \\

\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + 10K  \texttt{\textbf{eva-iw}}  &  &  &  &  &  & 52.94  & 52.67 \textcolor{gray}{\tiny $\pm$ 1.76} & 2054 \\ 


% \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% \midrule





\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:notes-1}
\end{table}
% --------------------------------------------------------
\footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
\footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}











\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\

DPO + NLL$_{\text{LC}}$ \  \hspace{+3pt}   Iter 1 / 3    & 8.73 & 9.18 & 8.28 & 53.2 \textcolor{gray}{{\tiny CI: (-2.2, 3.2)}}  & 625 & 53.48 & 48.70 \textcolor{gray}{\tiny $\pm$ 1.76} & 1824 \\

\qquad \qquad \qquad \ \ \ \hspace{+1pt} Iter 2 / 3      &  8.75  & 9.25 & 8.24 & 47.0 \textcolor{gray}{{\tiny CI: (-2.0, 2.7)}} & 601 & 52.57 & 46.76 \textcolor{gray}{\tiny $\pm$ 1.76} & 1729   \\

\qquad \qquad \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       & 8.66 & 9.13 & 8.19 & 46.8 \textcolor{gray}{{\tiny CI: (-2.2, 2.2)}} & 564 & 53.50 & 46.02 \textcolor{gray}{\tiny $\pm$ 1.76} & 1673  \\

\rowcolor[HTML]{e2fbe2} 
\text{DPO + NLL$_{\text{LC}}$  \  \hspace{+3pt}   Iter 1 / 3 (\texttt{eva-p}) } & \textbf{8.81} & 9.11 & \textbf{8.51} & \textbf{55.3} \textcolor{gray}{{\tiny CI: (-2.2, 2.4)}} &  871 & 52.37  &   52.92 \textcolor{gray}{\tiny $\pm$ 1.76} & 2300 \\ 

\bottomrule

\end{tabular}%
}
\vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:rpo}
\end{table}
% --------------------------------------------------------

% \begin{align}
%     \mathcal{L}_{\mathrm{DPO}+\mathrm{NLL}^{\mathrm{LC}}}\left(\pi_\vtheta ; \pi_{\text {\text{ref}}}\right)=-\mathbb{E}_{\left(\rvx, \rvy_{+}, \rvy_{-}\right) \sim \mathcal{D}}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text {ref}}\left(\rvy_{+} \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text {ref}}\left(\rvy_{-} \mid \rvx\right)}\right)\right] - \alpha \frac{\log \pi_{\vtheta}(\rvy_{+} \mid \rvx)}{|\rvy_{+}|}. \nonumber
% \end{align}


\begin{minipage}{\linewidth}

\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{DPO}+\mathrm{NLL}_{\mathrm{LC}}}(\pi_\vtheta ; \pi_{\text{ref}}) = 
-\mathbb{E}
&\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta(\rvy_{+} \mid \rvx)}{\pi_{\text{ref}}(\rvy_{+} \mid \rvx)}
-\beta \log \frac{\pi_\vtheta(\rvy_{-} \mid \rvx)}{\pi_{\text{ref}}(\rvy_{-} \mid \rvx)}\right)\right]- \alpha \frac{\log \pi_{\vtheta}(\rvy_{+} \mid \rvx)}{|\rvy_{+}|}. \nonumber
\end{split}
\end{equation}
\end{minipage}


% -------------------------------------------------------------
\subsubsection{The Effect of Different Initialization}\label{sec:ab-init}
\notes{This subsection can be put in the appendix section. In all our current setting, we start with a DPO checkpoint. We can test starting with the SFT checkpoint, and one-round BoN SFT checkpoint.}
\input{tables/tab-ab-init}
% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{Performance on the Downstream Tasks}\label{sec:ab-downstream}
% \input{tables/tab-ab-downstream}
% % -------------------------------------------------------------

\subsubsection{Other Preference Optimization Methods: BoN Finetuning and RLOO}\label{sec:ab-optim}
While in this work we focus on direct preference optimization, we also add ablation for other methods.
% In this section, we attempt the simplest setting. Instead of using contrastive methods like DPO, we directly use the chosen (\ie the response that achieves the best reward for each prompt)  


% \subsubsection{The Effect of Difficulty Aware Sampling}
% \notes{The idea is straightforward. For harder prompts, we just sample more responses. This is another way to utilize our informativeness metric, and making the response sampling more \emph{adaptive}.}

% % -------------------------------------------------------------
% \subsubsection{The Effect of Different Early Stopping Criteria}\label{sec:ab-stop}
% \notes{This subsection can be put in the appendix section.}
% \input{tables/tab-ab-stop}
% % -------------------------------------------------------------
% This is orthogonal to our contribution. Putting here just as a reference for tuning model performance in the later stages.


% \paragraph{Iterative training scheduling.} The base experiments test performance in one iteration. We now consider iterative training. Specifically, we define the models and the training data they use as follows:\begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_1$ : init with $\vtheta_0$; trained w/ the $1^{\text{st}}$ prompt split $D_1$ by self-generated responses.
%     \item $\vtheta_2$ : init with $\vtheta_1$; trained w/ the $2^{\text{st}}$ prompt split $D_2$ via by self-generated responses.
%     \item ...
% \end{itemize}


% \paragraph{Self-rewarding mechanism.} In the base experiments, we assume preference comes from an external preference oracle. Following the setting of~\citep{self-reward}, we finetune the model for reward generation, then use the generated reward to replace the preference oracle for reward annotation.

% # saturated benchmark


























% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{avg. score}      & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% SFT                &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 9.01 & 8.32& 8.66& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% DPO \ \hspace{+3pt} Iter 2 / 6       & 8.88 & 8.39 & 8.64 & on h100-west \textcolor{gray}{{\tiny CI: (, )}} &  & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  \textbf{9.04}& \textbf{8.75} & \textbf{8.90}& \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  \textbf{55.35} &    \textbf{55.53} \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{d6fcf9}  
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-greedy}) } & \textbf{9.06} & 8.36 & 8.72 & on a100-cc & & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-iw}) } & \\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-greedy}) } & \\ 

% \rowcolor[HTML]{e9ebee}
% Offline DPO w/ 60K Prompts\footnotemark       &   9.22 &   8.53 & 8.78  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  56.46 & 58.07 \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% % IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% % \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      &  9.03 &  8.21 &  8.62 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% % \quad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% % \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{9.11} &  \textbf{8.45} &  \textbf{8.78} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:notes}
% \end{table}
% % --------------------------------------------------------
% \footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
% \footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}


==> texs/app-settings.tex <==
\paragraph{Code release.} At the moment, we put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}, where we intend to release all the source code there, and all the datasets (generated prompts and responses) and models (with other models beyond the current model family) \emph{anonymously} to HuggingFace, \text{upon approval} -- before then, we are happy to provide any clarification requested to help re-implement~\method~and replicate our results. 

In general, our codebase is made to be simple to use for practitioners, requiring \textbf{only a creator module addition} within the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline.

\paragraph{Hyperparameter settings.} We follow the original hyperparameter settings as in~\citep{orpo,simpo,self-play-gu}, default to be:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
$\lambda$                                                      & /      & 0.5      & /      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1024   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
\bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-main-params}
\end{table}


\paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-reward}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
    \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
    % \item ...
\end{itemize}

For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this and other plug-in evolving methods. For solver we generate 6 responses per prompt.

% \paragraph{Computation environments.} 

\paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve Gemini, OpenAI (default to be \texttt{\small gpt-4o-mini}) and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. We use 42 as the random seed.

% We include main Appendix following references, also in \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}.

==> texs/conclusion-ckpt.tex <==
% \newpage
\section{\textcolor{Gray}{[Draft]} Conclusions, Limitations and Future Works}

\notes{Scratchpad. To refine later.}

\paragraph{Conclusions.} The primary implication of our work is: ....

Most post-training algorithms only consider how to provide a good answer (y | x); few consider how to teach the model to ask the right question (x). But an important property of intelligence is to actively ask questions.

This also brings a new perspective of ``generative'' exploration for RLHF, in the sense that we actively generate states for exploration and exploitation, which is typically undoable in classical contextual bandits and RL.

While \texttt{eva} standalone is self-contained, we also bring new perspective in classical literature. 
\begin{itemize}
    \item Compared to the self-training literature: (we are the first to self-training by jointly optimization $(\calX, \calY)$)
    \item Compared to the self-instruct literature: (we are the first to apply the method with contrastive preference optimization, and we also propose a new data selection metric.)
    \item Compared to the curriculum learning literature: (we incorporate generative data augmentation, instead of purely re-ordering the learning sequence.)
\end{itemize}

% Perhaps the primary implication of our work is: 

% Write some philosophical bits on robust, open-ended, sample efficient superintelligence.

% Write concrete future directions for people to follow based on our general framework.


\textbf{Limitation and future direction.}
\begin{itemize}
    \item Make the creator policy differentiable.
    \item Adding self-reward generation.
    \item Applying the method in reasoning tasks (combining with RPO~\citep{rpo}). 
    \begin{itemize}
        \item One way is on directly generating new problems or conjectures. 
        \item We may also combine with MCTS (add the theorem proving and auto conjecturing lines of work).
    \end{itemize}
    
    \item consider more players in the loop, \eg~the critic, the re-writer.
    \item extending to multi-turn.
    \item adding exploration bonus for diversity and coverage. (to cite the recent few papers on coverage guarantee.)
    \item explore more use of advantage function with other anchors
\end{itemize}

\notes{Some figures/tables to include in the main paper: prompt distribution (coverage and difficulty); also add the bar plot. and a pipeline, just like the self-rewarding paper.)}

% comparison with existing works (compared to rest-like paper, our generation happens in the joint space of x|y; compared to the self-instruct-like paper, our optimization is on contrastive optimization, instead of finetuning; we also have a specific data selection criteria; compared to curriculum learning paper, our data has generative augmentation, instead of purely re-ordering. 

\newpage

==> texs/conclusion.tex <==
% \newpage
\section{Concluding Remarks}\label{sec:conclusion}


% \vspace{-2pt}





% Perhaps the primary implication of our work is: 

% Write some philosophical bits on robust, open-ended, sample efficient superintelligence.

% Write concrete future directions for people to follow based on our general framework.

% also discuss the challenge of the evolving methods in the appendix

\textbf{Future directions.}
\ \ \method~defines a new paradigm for reinforcement learning from human feedback, opening up many new directions, \eg (i) extending to differentiable creator policies, combining w/ other $\texttt{\small evolve}(\cdot)$ methods; (ii) evolving for more iterations w/ on-policy solvers like RLOO~\citep{rloo}; (iii) investigating exploration bonuses for distribution diversity and coverage, and the self-consuming loop~\citep{collapse}; (iv) extending the game with more modality~\citep{genie}, and/or with more players for full automation (\eg rewarders, critics, rewriters, verifiers, retrievers); (v) extending from alignment to reasoning (\eg auto-conjecturing for theorem proving~\citep{math-conjecture} can be cast as an asymmetric game), or from the bandits to the trajectories w/ process reward models and hierarchical search for creator and solver generations;  (vii) further scaling up w/ millions of prompts with continual RL training~\citep{continual-rl}.
\vspace{-6pt}

\paragraph{Conclusions.} \method~is a new, simple and scalable framework for aligning language models, and can be plugged into any existing alignment pipeline. The primary takeaway may be that RLHF can be made open-ended: (i) self-evolving joint data distributions can bring significant gain (as shown across various optimization algorithms), and (ii) reward advantage acts as an effective metric informing the collection and creation of \emph{future} prompts for alignment. \method~presents a new view of alignment by framing it as an asymmetric  game between a creator generating \emph{new \emph{and} learnable} states (\ie prompts) and a solver producing preferred actions (\ie responses).  \method~also \emph{incentivizes agents to create problems} rather than to simply \emph{solve problems}, which is a key feature of intelligence, yet classical bandit/RL works often neglect.






==> texs/exp-fix.tex <==

\section{Experiments}\label{sec:exp}
% In this section, we present main results of our experiments, showing the remarkable performance gain from the additional creator step in~\method~on various benchmarks.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/arena-hard.png}
%         \caption{Caption for Arena Hard}
%         \label{fig:arena-hard}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/mt-bench.png}
%         \caption{Caption for MT Bench}
%         \label{fig:mt-bench}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/alpaca-eval.png}
%         \caption{Caption for Alpaca Eval}
%         \label{fig:alpaca-eval}
%     \end{subfigure}
%     \caption{Overall caption for the three figures}
%     \label{fig:three-figures}
% \end{figure} 


% \subsection{Experimental Settings}
\paragraph{Datasets and models for training.} We use  \textbf{UltraFeedback}~\citep{ultrafeedback} as the training dataset, which contains diverse high-quality prompts that are primarily human-generated. We use the instruction-finetuned \textsc{Gemma-2-9B}~\citep{gemma2} as the primary model, which is a strong baseline for models of its size.   Detailed experimental setting can be found in $\S$~\ref{app:reproduce}.
\vspace{-10pt}
\paragraph{Evaluation settings.} We choose:   (i) \textbf{AlpacaEval 2.0}~\citep{ae}, which assesses general instruction following with 805 questions; (ii) \textbf{MT-Bench}~\citep{llm-judge}, which evaluates multi-turn instruction following with 80 hard questions in 8 categories; (iii) \textbf{Arena-Hard}~\citep{ah}, which is derived from 200K user queries on Chatbot Arena with 500 challenging prompts across 250 topics.  We use \texttt{\small gpt-4-1106} as the judge and \texttt{\small gpt-4-0314} as the baseline for win rate.
\vspace{-10pt}
\paragraph{Optimization algorithms.} We focus on direct preference optimization and consider the following:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{With reference policy}: DPO~\citep{dpo}, SPPO~\citep{self-play-gu}.
    \item \textbf{Without reference policy}: SimPO~\citep{simpo}, ORPO~\citep{orpo}.
\end{itemize}
\vspace{-10pt}
\paragraph{Reward models as preference oracles.} We use \textsc{ArmoRM-8B}~\citep{armorm} as our default reward model as the human-preference proxy, and consider the following for ablation studies:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Pointwise}: \textsc{ArmoRM-8B}~\citep{armorm}, \textsc{SkyworkRM-27B}~\citep{skyworkrm}.
    \item \textbf{Pairwise}: \textsc{PairRM-0.4B}~\citep{pairrm}, \textsc{PairRM-8B}~\citep{pairrm8b}.
\end{itemize}

\subsection{Main Results}
\label{sec:main_results}
% For iterative training, we split the training set into equal-size partition and use one partition per iteration.

% \footnote{\vspace{-2pt}Unless stated otherwise, each iteration uses 10K prompts (\ie 1/6 partition from UltraFeedback in classical training). We denote \vspace{-16pt}$\vtheta_{t \rightarrow t+1}$ as the model trained with new human prompts based on the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the model trained with evolved prompts \vspace{-56pt}from the $t$-th checkpoint w/o adding any new human prompts.}
In general, \method~brings notable gains in alignment without relying on any human-crafted data, thus offering more efficiency. In the base setup, building on the one-iteration finetuned model ($\vtheta_{0 \rightarrow 1}$), \method~adds a creator to self-evolve the prompt set of the initial iteration and uses any preference optimization algorithm  for an additional open-ended RLHF iteration, resulting in  $\vtheta_{1 \rightarrow \tilde{1}}$\footnote{\vspace{-0pt}Unless stated otherwise, each training iteration uses 10K prompts; we denote $\vtheta_{t \rightarrow t+1}$ as the one trained w/ new human prompts \\\vspace{-49pt}from the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the one trained w/ evolved prompts from the $t$-th checkpoint w/o any new human prompts.}.
\vspace{-10pt}
\paragraph{\method~achieves self-improvement.}  As shown in red rows in Table~\ref{tab:main-10k}, \method~yields notable performance improvement over $\vtheta_{0 \rightarrow 1}$ across different optimization algorithms, especially on the harder Arena-Hard benchmark, which is recognized to be more challenging and distinguishable among others due to the complexity of its prompts and its fairer scoring system~\citep{ah,simpo}. Specifically, \method~brings $8.4\%$ gain with SimPO as the solver, and $8.5\%$ gain with DPO as the solver, surpassing its 27B version and matching \texttt{\small claude-3-opus-240229} as reported on the \href{https://github.com/lm-sys/arena-hard-auto/tree/efc012e192b88024a5203f5a28ec8fc0342946df?tab=readme-ov-file#full-leaderboard-updated-0831}{\textcolor{gblue}{AH leaderboard}}, while using fully self-automated prompt generation for alignment. Interestingly, \method~brings the least gains on AlpacaEval 2.0, a simpler evaluation benchmark. This indicates \method~improves the most for challenging tasks.
\vspace{-10pt}
\paragraph{\method~can surpass human-crafted prompts.}  We further show that \method-prompt-trained models ($\vtheta_{1 \rightarrow \tilde{1}}$) can match and even outperform those trained on additional new prompts from UltraFeedback ($\vtheta_{1 \rightarrow 2}$) (which we denoted as human prompts), while being much cheaper and more efficient. Additionally, on MT-Bench, training with new human prompts typically show decreased performance in the first turn and only modest gains in the second turn. In contrast,~\method~notably enhances second-turn performance. We hypothesize that~\method~evolves novel, learnable prompts that include characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions.
\input{tables/tab-main-10k}
% Additionally, on MT-Bench, we found that human prompts generally exhibit performance recession in first turn with modest gain in the second turn -- \method~fixes this while remarkably improves the second-turn performance without explicit training for it; we hypothesize that the novel, learnable prompts evolved from~\method~may incorporate characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions more effectively.


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: Main Results with the Online Training Setting}
% \input{tables/tab-main-10k-o}

% \subsection{Subsections}





% -------------------------------------------------------------


% \newpage
\vspace{-10pt}
\subsection{Ablation Studies}
% \notes{For now, we use tables to record results. We can shift to other illustrations later (\eg performance plot, pareto circle, prompt distribution w.r.t. metric, etc).}
We conduct in-depth ablation studies on \texttt{\textbf{eva}}, with findings below to be elaborated on later: 

% \setlength{\leftmargini}{9pt}
\vspace{-5pt}
\begin{itemize}
    \item $\S$~\ref{sec:ab-metric} - \textbf{informativeness metric}: our \emph{regret}-based metric outperforms other alternatives.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-procedure} - \textbf{sample-then-evolve procedure}: our method outperforms greedy selection.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-rm} - \textbf{scaling w/ reward models}: the alignment gain of~\method~scales with reward models.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-cont} - \textbf{continual training }: our method has monotonic gain with incremental training;  the \emph{evolved data and schedule} by~\method~serves as an \emph{implicit regularizer} for better local minima.
\end{itemize}
\vspace{-4pt}

%-------------------------------------------------------------
\vspace{-10pt}
\subsubsection{The Choice of Informativeness Metrics: \texttt{info(\textperiodcentered)}}\label{sec:ab-metric}
\vspace{-4pt}
% \notes{To make a table on all metrics in Section~\ref{sec:ab-metric}, similar to~\citep{plr}.}
\input{tables/tab-info-metric}
\vspace{-8pt}
\input{tables/tab-ab-metric}
\vspace{-12pt}
% (\textit{cf}., the principle of insufficient reason~\citep{key,dr})
\paragraph{Advantage as the informativeness metric outperforms baselines.} \hspace{-5pt}As in Table~\ref{tab:ab-metric}, \textbf{\texttt{eva}} offers an effective curriculum by the advantage-based proxy as the informativeness metric (bottom row):
\vspace{-5pt}
\begin{itemize}
    \item \emph{Comparing w/ uniform evolving} (\textcolor{brown!85}{brown}): Existing baselines generate prompts in a uniform manner~\citep{self-reward}  (\textit{cf}., the principle of insufficient reason~\citep{key,dr}). \method~concretely outperforms, corroborating~\cite{active-rlhf} that uniform learners can suffer from sub-optimality gaps.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ other heuristics} (\textcolor{dmblue200}{blue}): Prior practices~\citep{team-1} tried heuristics like prioritizing prompts w/ the most variance in its  rewards or w/ the lowest/highest average. We find our advantage based methods (red) outperforms those heuristics; see $\S$~\ref{app:metric} for more.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ the inverse advantage} (\textcolor{dmpurple500}{purple}): Contrary to curriculum learning, a line of works conjecture that examples w/ higher losses may be prioritized~\citep{hard-losers,ordered-sgd}, which can be done by inverting our metric. We find it significantly \emph{hurt} the alignment gain, corroborating~\cite{rho-loss} that those examples can be unlearnable or irrelevant, meaning our curriculum is effective and practical. \vspace{+1.5pt}
    
    \item \emph{Among our advantage variants} (\textcolor{dmgreen900}{green}): We  designed variants of our default advantage-based metric, as in Table~\ref{tab:info-metric}; the default $A^{\star}_{\min}$ remains competitive among its peers. Together, the advantage-based principle provides a robust guideline for prompt sampling and evolving.
\end{itemize}
\vspace{-6pt}
The lesson is that we must be selective about which are the promising to evolve, otherwise unlearnable, noisy or naïve prompts may hinder learning. Our regret-inspired metric represents a solid baseline. 
\vspace{-6pt}


% \notes{Compare a star min with the uniform (no ordering), then compare it with its inverse (from hard to easy).}

% \paragraph{\emphtext{\method~is better other metric.}}  

% \notes{compare eva with other advantage variants, and other common choices that people have been using (choosing variance or mean) probably cite~\citep{active-pl,active-rlhf,selm} and emphasize our reliance on reward model. then cite~\cite{self-improving} in the footnote.}

% \paragraph{\emphtext{\method~.}}  \notes{compare eva with other advantage variants.}
% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{The Effect of the Sample-then-Evolve Procedure}\label{sec:ab-procedure}
\input{tables/tab-ab-procedure}

\paragraph{The design of \texttt{\small evolve(\textperiodcentered)} in~\method~is effective.} As in Table~\ref{tab:ab-procedure}, we show:
\vspace{-5pt}
\begin{itemize}
    \item Removing the $\texttt{\small evolve}(\cdot)$ step: if we only do subset sampling or ordered selection, we still have gain, but not as much as w/ evolving (\eg \method~brings $4.8\%$ additional wins on AH).\vspace{+1.5pt}
    \item Altering the $\texttt{\small sample}(\cdot)$ step: if we greedily select prompts by the metric instead of using them as weights for importance sampling, the performance will be weaker as we evolve.
    % \footnote{When there is only subset selection, however, being greedy is slightly better on the Arena-Hard benchmark, but as we evolve more prompts such gain disappears.}. 
\end{itemize}
\vspace{-4pt}

% The lesson is that simply active learning on fixed prompts is unsatisfactory~\notes{To find a better description. AL is more about budget}; the open-ended RLHF with \emph{generative} prompt exploration we present brings a substantial headroom for self-improvement.
This shows that simply adaptive training within a fixed prompt distribution is unsatisfactory; our open-ended RLHF with \emph{generative} prompt exploration gives a substantial headroom for self-improvement.
% -------------------------------------------------------------




% -------------------------------------------------------------
\subsubsection{Scaling Pointwise and Pairwise Reward Models}\label{sec:ab-rm}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
        \end{subfigure}
        \vspace{-8pt}
        \caption{\textbf{\method\ scales with quality of reward models}, under pointwise RMs w/ DPO (\emph{left}) and pairwise RMs w/ SPPO (\emph{right}).  Note SPPO handles general preferences thus requires pairwise RMs, and DPO relies on the Bradley-Terry assumption, for which pointwise RMs are suitable.}
        \label{fig:ab-rm}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\textwidth}
        Figure~\ref{fig:ab-rm} presents the length-controlled win rate of \method~on  AlpacaEval  using pointwise and pairwise reward models of varying scales.
        %and types. We compare pointwise reward models w/ DPO, and pairwise reward models w/ SPPO\footnotemark.  
        The results give a clear trend: as the quality of reward models improve, \method~brings higher alignment gain. The scaling observation shows the effectiveness of~\method~in exploiting more accurate reward signals to choose informative prompts for better alignment.  One takeaway is interaction w/ the external world is essential for intelligence. The more accurate reward signals observed, the better the agent incentivize themself to improve (\textit{cf.},~\cite{silver2021reward}).
    \end{minipage}
\end{figure}
\vspace{-8pt}


% \footnotetext{We note that when there is only subset selection, being greedy is slightly better on the Arena-Hard benchmark. However, as we evolve more prompts, this discrepancy reverses.}

% \begin{figure}[!ht]
%     \centering
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
%         \end{subfigure}
%         \vspace{+0.1pt}
%         \caption{\textbf{Scaling with reward models.} Benchmark evaluation shows~\method~scales with reward models under both pointwise (\emph{left}) and pairwise (\emph{right}) setting.}
%         \label{fig:ab-rm}
%     \end{minipage}
% \end{figure}
% \vspace{-3pt}

% \paragraph{\emphtext{\method~scales with reward models.}} Figure~\ref{fig:ab-rm} presents the performance of \method~on the AlpacaEval benchmark using reward models of varying scales and types. We compare pointwise reward models with DPO~\citep{dpo} with pairwise reward models with SPPO~\citep{self-play-gu}\footnote{SPPO handles general preferences and thus requires pairwise reward models, whereas DPO relies on the Bradley-Terry model, for which pointwise reward models are suitable.}.  The results demonstrate a clear trend: as the quality of the reward model improves, \method~brings higher performance gain. The scaling observation shows the effectiveness of~\method~in leveraging more accurate reward signals to select informative prompts for better alignment. More results are in $\S$~\ref{app:ab-rm}.


% % \notes{The experiment is running.}
% \input{tables/tab-ab-rm}





% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{\method~Improves Both Sample Efficiency and Generalization}\label{sec:ab-cont}
We continuously run the default \emph{incremental training} (\ie trainining from the last checkpoint w/ the evolved set in each iteration), as in Fig~\ref{fig:sad} and~\secref{app:exp-iter}, \method~presents \emphtext{\it monotonic performance gain} over iterations, and surpasses that trained w/ new human prompts, implying the generalization benefit. 

We conjecture that behaviors of the dashed/dotted lines relate to \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-primary-bias,cont-loss-rl,cont-repeat}.  Classical works resolve it by the \emph{optimization} perspective (\eg weight perturbing), whereas~\method~provides a new \emph{data} perspective, potentially mimicing an \textbf{implicit regularizer for better generalization}.
\vspace{-3pt}

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% \notes{Finished running. Waiting for evaluation.}



% A prominent line of research is on the loss of plasticity for continual (incremental) training~\citep{cont-critical,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm,cont-warm}; prior works all try to solve this via the optimization perspective, while our \eva method provides a fresh data perspective to solve the issue, operating like adding a regularizer to find better local minima.

\vspace{-5pt}
\begin{figure}[h!]
\centering

% \begin{minipage}{0.34\textwidth}
% \includegraphics[width=.8\textwidth]{figs/sad.png}
% % \caption{Iterative incremental training in different settings. } \label{fig:sad}
% \vspace{+2pt}
% \caption{\textbf{Continual training.} Our method stays robust w/ more iterations in incremental training. } \label{fig:sad}
% \end{minipage}
\begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=.86\textwidth]{figs/dpo-it.pdf} % First figure
    % \vspace{10pt} % Adjust spacing between figures if needed
    \includegraphics[width=.86\textwidth]{figs/sppo-it.pdf} % Second figure
    \vspace{-6pt}
    \caption{\textbf{Continual training.} \method~stays robust w/ more iterations in incremental training.}
    \label{fig:sad}
\end{minipage}
\hfill
\begin{minipage}{0.64\textwidth} 
% \setlength{\parindent}{1em} % Adjust as needed for indentation
The solutions found by~\method~cannot be recovered by training longer w/ a fixed distribution (the dashed), nor by naïvely sourcing new prompts w/o examining informativeness (the gray dotted),  thus our generative data schedule is effective.\vspace{+6pt}

In Table~\ref{tab:ab-cont}, we ablate~\method~in \textit{scratch training}, \ie training w/ the full set (the evolved and the original data). \method~is competitive in incremental training, thus \emphtext{\emph{learns more effective} with \emph{less data}} -- a nice bonus via minimax regret~\citep{dcd}.

% , as in $\S$~\ref{sec:int}


% Next, we consider two different continual procedures:
% \begin{itemize}
%     \item \textbf{Incremental training}\footnotemark: train with only the evolved data on the finetuned checkpoint $\vtheta_{0 \rightarrow 1}$.\vspace{-1pt}
%     \item \textbf{Scratch training}: combine the evolved data with the full initial prompt set, train from scratch with $\vtheta_0$.
% \end{itemize}
% \vspace{+4pt}

\vspace{-6pt}
\input{tables/tab-ab-cont}


% We then iteratively run incremental training, as in Figure~\ref{fig:sad}, \method~presents monotonic performance gain.\vspace{+4pt}

% A prominent line of research is on the difficulty of continual (incremental) training, and prior works all try to solve this via the explicit regularizer perspective~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}, while \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

\end{minipage}

\end{figure}
\vspace{-9pt}


% cont-rewarm
% acting like an implicit regularizer for better local minima

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% Furthermore, the open-ended nature of~\method~naturally aligns with the continual learning literature; one of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better generalization.

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% The open-ended nature of~\method~naturally aligns with the continual learning literature.
% One of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima, 
% ~\notes{To update the figure; having DPO+SPPO.}
% \vspace{+6pt}


% \footnotetext{This is the default training strategy that we are using as it is computational efficient.}



% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{The Effect of Iteratively Evolving}\label{sec:ab-iter}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% \input{tables/tab-ab-iter}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of the Base LLM for the Creator}\label{sec:ab-gen-lm}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% % \notes{Experiments running in process. Mostly finished training. }
% \input{tables/tab-ab-gen-lm}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of The Number of Training Examples}\label{sec:ab-scale}
% \input{tables/tab-ab-scale}
% % -------------------------------------------------------------

% \notes{We may need to add additional compute resources usage discussions to illustrate efficiency.}














==> texs/exp.tex <==

\section{Experiments}\label{sec:exp}
% In this section, we present main results of our experiments, showing the remarkable performance gain from the additional creator step in~\method~on various benchmarks.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/arena-hard.png}
%         \caption{Caption for Arena Hard}
%         \label{fig:arena-hard}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/mt-bench.png}
%         \caption{Caption for MT Bench}
%         \label{fig:mt-bench}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/alpaca-eval.png}
%         \caption{Caption for Alpaca Eval}
%         \label{fig:alpaca-eval}
%     \end{subfigure}
%     \caption{Overall caption for the three figures}
%     \label{fig:three-figures}
% \end{figure} 


% \subsection{Experimental Settings}
\paragraph{Datasets and models for training.} We use  \textbf{UltraFeedback}~\citep{ultrafeedback} as the training dataset, which contains diverse high-quality prompts that are primarily human-generated. We use the instruction-finetuned \textsc{Gemma-2-9B}~\citep{gemma2} as the primary model, which is a strong baseline for models of its size.   Detailed experimental setting can be found in $\S$~\ref{app:reproduce}.
\vspace{-10pt}
\paragraph{Evaluation settings.} We choose:   (i) \textbf{AlpacaEval 2.0}~\citep{ae}, which assesses general instruction following with 805 questions; (ii) \textbf{MT-Bench}~\citep{llm-judge}, which evaluates multi-turn instruction following with 80 hard questions in 8 categories; (iii) \textbf{Arena-Hard}~\citep{ah}, which is derived from 200K user queries on Chatbot Arena with 500 challenging prompts across 250 topics.  We use \texttt{\small gpt-4-1106} as the judge and \texttt{\small gpt-4-0314} as the baseline for win rate.
\vspace{-10pt}
\paragraph{Optimization algorithms.} We focus on direct preference optimization and consider the following:
\vspace{-6pt}
\begin{itemize}
    \item \textbf{With reference policy}: DPO~\citep{dpo}, SPPO~\citep{self-play-gu}.\vspace{+1pt}
    \item \textbf{Without reference policy}: SimPO~\citep{simpo}, ORPO~\citep{orpo}.
\end{itemize}
\vspace{-10pt}
\paragraph{Reward models as preference oracles.} We use \textsc{ArmoRM-8B}~\citep{armorm} as our default reward model as the human-preference proxy, and consider the following for ablation studies:
\vspace{-6pt}
\begin{itemize}
    \item \textbf{Pointwise}: \textsc{ArmoRM-8B}~\citep{armorm}, \textsc{SkyworkRM-27B}~\citep{skyworkrm}.\vspace{+1pt}
    \item \textbf{Pairwise}: \textsc{PairRM-0.4B}~\citep{pairrm}, \textsc{PairRM-8B}~\citep{pairrm8b}.
\end{itemize}

\subsection{Main Results}
\label{sec:main_results}
% For iterative training, we split the training set into equal-size partition and use one partition per iteration.

% \footnote{\vspace{-2pt}Unless stated otherwise, each iteration uses 10K prompts (\ie 1/6 partition from UltraFeedback in classical training). We denote \vspace{-16pt}$\vtheta_{t \rightarrow t+1}$ as the model trained with new human prompts based on the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the model trained with evolved prompts \vspace{-56pt}from the $t$-th checkpoint w/o adding any new human prompts.}
In general, \method~brings notable gains in alignment without relying on any human-crafted data, thus offering more efficiency. In the base setup, building on the one-iteration finetuned model ($\vtheta_{0 \rightarrow 1}$), \method~adds a creator to self-evolve the prompt set of the initial iteration and uses any preference optimization algorithm  for an additional open-ended RLHF iteration, resulting in  $\vtheta_{1 \rightarrow \tilde{1}}$\footnote{\vspace{-0pt}Unless stated otherwise, each training iteration uses 10K prompts; we denote $\vtheta_{t \rightarrow t+1}$ as the one trained w/ new human prompts \\\vspace{-49pt}from the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the one trained w/ evolved prompts from the $t$-th checkpoint w/o any new human prompts.}.
\vspace{-10pt}
\paragraph{\method~achieves self-improvement.}  As shown in red rows in Table~\ref{tab:main-10k}, \method~yields notable performance improvement over $\vtheta_{0 \rightarrow 1}$ across different optimization algorithms, especially on the harder Arena-Hard benchmark, which is recognized to be more challenging and distinguishable among others due to the complexity of its prompts and its fairer scoring system~\citep{ah,simpo}. Specifically, \method~brings $8.4\%$ gain with SimPO as the solver, and $8.5\%$ gain with DPO as the solver, surpassing its 27B version and matching \texttt{\small claude-3-opus-240229} as reported on the \href{https://github.com/lm-sys/arena-hard-auto/tree/efc012e192b88024a5203f5a28ec8fc0342946df?tab=readme-ov-file#full-leaderboard-updated-0831}{\textcolor{gblue}{AH leaderboard}}, while using fully self-automated prompt generation for alignment. Interestingly, \method~brings the least gains on AlpacaEval 2.0, a simpler evaluation benchmark. This indicates \method~improves the most for challenging tasks.
\vspace{-10pt}
\paragraph{\method~can surpass human-crafted prompts.}  We further show that \method-prompt-trained models ($\vtheta_{1 \rightarrow \tilde{1}}$) can match and even outperform those trained on additional new prompts from UltraFeedback ($\vtheta_{1 \rightarrow 2}$) (which we denoted as human prompts), while being much cheaper and more efficient. Additionally, on MT-Bench, training with new human prompts typically show decreased performance in the first turn and only modest gains in the second turn. In contrast,~\method~notably enhances second-turn performance. We hypothesize that~\method~evolves novel, learnable prompts that include characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions.
\input{tabs/tab-main-10k}
% Additionally, on MT-Bench, we found that human prompts generally exhibit performance recession in first turn with modest gain in the second turn -- \method~fixes this while remarkably improves the second-turn performance without explicit training for it; we hypothesize that the novel, learnable prompts evolved from~\method~may incorporate characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions more effectively.


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: Main Results with the Online Training Setting}
% \input{tabs/tab-main-10k-o}

% \subsection{Subsections}





% -------------------------------------------------------------


% \newpage
\vspace{-10pt}
\subsection{Ablation Studies}
% \notes{For now, we use tables to record results. We can shift to other illustrations later (\eg performance plot, pareto circle, prompt distribution w.r.t. metric, etc).}
We conduct in-depth ablation studies on \texttt{\textbf{eva}}, with findings below to be elaborated on later: 

% \setlength{\leftmargini}{9pt}
\vspace{-5pt}
\begin{itemize}
    \item $\S$~\ref{sec:ab-metric} - \textbf{informativeness metric}: our \emph{regret}-based metric outperforms other alternatives.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-procedure} - \textbf{sample-then-evolve procedure}: our method outperforms greedy selection.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-rm} - \textbf{scaling w/ reward models}: the alignment gain of~\method~scales with reward models.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-cont} - \textbf{continual training }: our method has monotonic gain with incremental training;  the \emph{evolved data and schedule} by~\method~serves as an \emph{implicit regularizer} for better local minima.
\end{itemize}
\vspace{-4pt}

%-------------------------------------------------------------
\vspace{-10pt}
\subsubsection{The Choice of Informativeness Metrics: \texttt{info(\textperiodcentered)}}\label{sec:ab-metric}
\vspace{-4pt}
% \notes{To make a table on all metrics in Section~\ref{sec:ab-metric}, similar to~\citep{plr}.}
\input{tabs/tab-info-metric}
\vspace{-8pt}
\input{tabs/tab-ab-metric}
\vspace{-12pt}
% (\textit{cf}., the principle of insufficient reason~\citep{key,dr})
\paragraph{Advantage as the informativeness metric outperforms baselines.} \hspace{-5pt}As in Table~\ref{tab:ab-metric}, \textbf{\texttt{eva}} offers an effective curriculum by the advantage-based proxy as the informativeness metric (bottom row):
\vspace{-6pt}
\begin{itemize}
    \item \emph{Comparing w/ uniform evolving} (\textcolor{brown!85}{brown}): Existing baselines generate prompts in a uniform manner~\citep{self-reward}  (\textit{cf}., the principle of insufficient reason~\citep{key,dr}). \method~concretely outperforms, corroborating~\cite{active-rlhf} that uniform learners can suffer from sub-optimality gaps.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ other heuristics} (\textcolor{dmblue200}{blue}): Prior practices~\citep{team-1} tried heuristics like prioritizing prompts w/ the most variance in its  rewards or w/ the lowest/highest average. We find our advantage based methods (red) outperforms those heuristics; see $\S$~\ref{app:metric} for more.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ the inverse advantage} (\textcolor{dmpurple500}{purple}): Contrary to curriculum learning, a line of works conjecture that examples w/ higher losses may be prioritized~\citep{hard-losers,ordered-sgd}, which can be done by inverting our metric. We find it significantly \emph{hurt} the alignment gain, corroborating~\cite{rho-loss} that those examples can be unlearnable or irrelevant, meaning our curriculum is effective and practical. \vspace{+1.5pt}
    
    \item \emph{Among our advantage variants} (\textcolor{dmgreen900}{green}): We  designed variants of our default advantage-based metric, as in Table~\ref{tab:info-metric}; the default $A^{\star}_{\min}$ remains competitive among its peers. Together, the advantage-based principle provides a robust guideline for prompt sampling and evolving.
\end{itemize}
\vspace{-6pt}
The lesson is that we must be selective about which are the promising to evolve, otherwise unlearnable, noisy or naïve prompts may hinder learning. Our regret-inspired metric represents a solid baseline. 
\vspace{-6pt}


% \notes{Compare a star min with the uniform (no ordering), then compare it with its inverse (from hard to easy).}

% \paragraph{\emphtext{\method~is better other metric.}}  

% \notes{compare eva with other advantage variants, and other common choices that people have been using (choosing variance or mean) probably cite~\citep{active-pl,active-rlhf,selm} and emphasize our reliance on reward model. then cite~\cite{self-improving} in the footnote.}

% \paragraph{\emphtext{\method~.}}  \notes{compare eva with other advantage variants.}
% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{The Effect of the Sample-then-Evolve Procedure}\label{sec:ab-procedure}
\input{tabs/tab-ab-procedure}

\paragraph{The design of \texttt{\small evolve(\textperiodcentered)} in~\method~is effective.} As in Table~\ref{tab:ab-procedure}, we show:
\vspace{-6pt}
\begin{itemize}
    \item Removing the $\texttt{\small evolve}(\cdot)$ step: if we only do subset sampling or ordered selection, we still have gain, but not as much as w/ evolving (\eg \method~brings $4.8\%$ additional wins on AH).\vspace{+1.5pt}
    \item Altering the $\texttt{\small sample}(\cdot)$ step: if we greedily select prompts by the metric instead of using them as weights for importance sampling, the performance will be weaker as we evolve.
    % \footnote{When there is only subset selection, however, being greedy is slightly better on the Arena-Hard benchmark, but as we evolve more prompts such gain disappears.}. 
\end{itemize}
\vspace{-4pt}

% The lesson is that simply active learning on fixed prompts is unsatisfactory~\notes{To find a better description. AL is more about budget}; the open-ended RLHF with \emph{generative} prompt exploration we present brings a substantial headroom for self-improvement.
This shows that simply adaptive training within a fixed prompt distribution is unsatisfactory; our open-ended RLHF with \emph{generative} prompt exploration gives a substantial headroom for self-improvement.
% -------------------------------------------------------------




% -------------------------------------------------------------
\subsubsection{Scaling Pointwise and Pairwise Reward Models}\label{sec:ab-rm}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
        \end{subfigure}
        \vspace{-8pt}
        \caption{\textbf{\method\ scales with quality of reward models}, under pointwise RMs w/ DPO (\emph{left}) and pairwise RMs w/ SPPO (\emph{right}).  Note SPPO handles general preferences thus requires pairwise RMs, and DPO relies on the Bradley-Terry assumption, for which pointwise RMs are suitable.}
        \label{fig:ab-rm}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\textwidth}
        Figure~\ref{fig:ab-rm} presents the length-controlled win rate of \method~on  AlpacaEval  using pointwise and pairwise reward models of varying scales.
        %and types. We compare pointwise reward models w/ DPO, and pairwise reward models w/ SPPO\footnotemark.  
        The results give a clear trend: as the quality of reward models improve, \method~brings higher alignment gain. The scaling observation shows the effectiveness of~\method~in exploiting more accurate reward signals to choose informative prompts for better alignment.  One takeaway is interaction w/ the external world is essential for intelligence. The more accurate reward signals observed, the better the agent incentivize themself to improve (\textit{cf.},~\cite{silver2021reward}).
    \end{minipage}
\end{figure}
\vspace{-8pt}


% \footnotetext{We note that when there is only subset selection, being greedy is slightly better on the Arena-Hard benchmark. However, as we evolve more prompts, this discrepancy reverses.}

% \begin{figure}[!ht]
%     \centering
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
%         \end{subfigure}
%         \vspace{+0.1pt}
%         \caption{\textbf{Scaling with reward models.} Benchmark evaluation shows~\method~scales with reward models under both pointwise (\emph{left}) and pairwise (\emph{right}) setting.}
%         \label{fig:ab-rm}
%     \end{minipage}
% \end{figure}
% \vspace{-3pt}

% \paragraph{\emphtext{\method~scales with reward models.}} Figure~\ref{fig:ab-rm} presents the performance of \method~on the AlpacaEval benchmark using reward models of varying scales and types. We compare pointwise reward models with DPO~\citep{dpo} with pairwise reward models with SPPO~\citep{self-play-gu}\footnote{SPPO handles general preferences and thus requires pairwise reward models, whereas DPO relies on the Bradley-Terry model, for which pointwise reward models are suitable.}.  The results demonstrate a clear trend: as the quality of the reward model improves, \method~brings higher performance gain. The scaling observation shows the effectiveness of~\method~in leveraging more accurate reward signals to select informative prompts for better alignment. More results are in $\S$~\ref{app:ab-rm}.


% % \notes{The experiment is running.}
% \input{tabs/tab-ab-rm}





% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{\method~Improves Both Sample Efficiency and Generalization}\label{sec:ab-cont}
We continuously run the default \emph{incremental training} (\ie trainining from the last checkpoint w/ the evolved set in each iteration), as in Fig~\ref{fig:sad} and~\secref{app:exp-iter}, \method~presents \emphtext{\it monotonic performance gain} over iterations, and surpasses that trained w/ new human prompts, implying the generalization benefit. 

We conjecture that behaviors of the dashed/dotted lines relate to \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-primary-bias,cont-loss-rl,cont-repeat}.  Classical works resolve it by the \emph{optimization} perspective (\eg weight perturbing), whereas~\method~provides a new \emph{data} perspective, potentially mimicing an \textbf{implicit regularizer for better generalization}.
\vspace{-3pt}

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% \notes{Finished running. Waiting for evaluation.}



% A prominent line of research is on the loss of plasticity for continual (incremental) training~\citep{cont-critical,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm,cont-warm}; prior works all try to solve this via the optimization perspective, while our \eva method provides a fresh data perspective to solve the issue, operating like adding a regularizer to find better local minima.

\vspace{-5pt}
\begin{figure}[!ht]
\centering
\begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=.86\textwidth]{figs/dpo-it.pdf} % First figure
    % \vspace{10pt} % Adjust spacing between figures if needed
    \includegraphics[width=.86\textwidth]{figs/sppo-it.pdf} % Second figure
    \vspace{-6pt}
    \caption{\textbf{Continual training.} \method~stays robust w/ more iterations in incremental training.}
    \label{fig:sad}
\end{minipage}
\hfill
\begin{minipage}{0.64\textwidth} 
% \setlength{\parindent}{1em} % Adjust as needed for indentation
The solutions found by~\method~cannot be recovered by training longer w/ a fixed distribution (the dashed), nor by naïvely sourcing new prompts w/o examining informativeness (the gray dotted),  thus our generative data schedule is effective.\vspace{+6pt}

In Table~\ref{tab:ab-cont}, we ablate~\method~in \textit{scratch training}, \ie training w/ the full set (the evolved and the original data). \method~is competitive in incremental training, thus \emphtext{\emph{learns more effective} with \emph{less data}} -- a nice bonus via minimax regret~\citep{dcd}.

% , as in $\S$~\ref{sec:int}


% Next, we consider two different continual procedures:
% \begin{itemize}
%     \item \textbf{Incremental training}\footnotemark: train with only the evolved data on the finetuned checkpoint $\vtheta_{0 \rightarrow 1}$.\vspace{-1pt}
%     \item \textbf{Scratch training}: combine the evolved data with the full initial prompt set, train from scratch with $\vtheta_0$.
% \end{itemize}
% \vspace{+4pt}

\vspace{-6pt}
\input{tabs/tab-ab-cont}


% We then iteratively run incremental training, as in Figure~\ref{fig:sad}, \method~presents monotonic performance gain.\vspace{+4pt}

% A prominent line of research is on the difficulty of continual (incremental) training, and prior works all try to solve this via the explicit regularizer perspective~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}, while \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

\end{minipage}

\end{figure}
\vspace{-9pt}


% cont-rewarm
% acting like an implicit regularizer for better local minima

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% Furthermore, the open-ended nature of~\method~naturally aligns with the continual learning literature; one of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better generalization.

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% The open-ended nature of~\method~naturally aligns with the continual learning literature.
% One of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima, 
% ~\notes{To update the figure; having DPO+SPPO.}
% \vspace{+6pt}


% \footnotetext{This is the default training strategy that we are using as it is computational efficient.}



% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{The Effect of Iteratively Evolving}\label{sec:ab-iter}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% \input{tabs/tab-ab-iter}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of the Base LLM for the Creator}\label{sec:ab-gen-lm}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% % \notes{Experiments running in process. Mostly finished training. }
% \input{tabs/tab-ab-gen-lm}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of The Number of Training Examples}\label{sec:ab-scale}
% \input{tabs/tab-ab-scale}
% % -------------------------------------------------------------

% \notes{We may need to add additional compute resources usage discussions to illustrate efficiency.}














==> texs/intro-cache.tex <==


% \textcolor{red}{[Expected to have a complete draft by tonight (Mon Sep 23.); the introduction section will be revised in the last after we have a good draft of Section~\ref{sec:method}.]}





% \begin{figure}[hb]
%     \centering
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/mt-bench.png}
%         \caption{Alpaca Eval}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/arena-hard.png}
%         \caption{Arena Hard}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/alpaca-eval.png}
%         \caption{MT Bench}
%     \end{subfigure}
%     \caption{Placeholder plot on evaluation results.}
%     \label{fig:three_benchmarks}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
%     \caption{Placeholder plot on pipeline.}
% \end{figure}


%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
\section {Introduction}
Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
High quality human data, crucial for scaling large language model (LLM) based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as LLMs become more capable, they need to solve increasingly complex challenges, requiring training data beyond abilities of humans to create. This necessitates a new fundamental mechanism for self-improving, where models is able to continuously self-generate and self-solve harder problems. We thereby investigates the research question below:\vspace{+6pt}
\begin{minipage}{1.\textwidth}
% \footnotesize
\centering
\textit{Can language models \emph{self-create} new, learnable tasks to work on,\\}
\textit{to \emph{self-improve} to \emph{generalize} better for human preferences alignment?}
\end{minipage}
%or higher intelligence.


% \notes{One way to write the motivation part may be to follow ~\citep{poet,bengio2009curriculum,accel,paired}. Discuss how we incentivize the agent to generate prompt distribution with increasing complexity, promoting the models to solve harder problems.}

% \notes{Additional motivation/intuition/background paragraphs need to be added here. Motivate why we need to jointly optimize for both.}

% We aim to develop language agents capable of surpassing even superior intelligence, enabling them to solve increasingly complex problems.

\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.258\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline.png}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.732\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/creator.png}
            % \caption{Arena Hard}
        \end{subfigure}
        \caption{\textbf{Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our proposed~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with an easy-to-implement \emph{estimate, sample then evolve} procedure; specifically, it estimates the informativeness for each prompt by how contrastive the self-generated responses are to the prompt, from the reward signals it receives. The creator evolves new prompts  from highly informative prompts, which the solver uses for continual training. Both the solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective design in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}
\vspace{-6pt}

% (\eg rewriting the prompts for in-depth/breadth variations)

\vspace{+2pt}



% at the same time as
% Given a fixed training set,
%to generalize well on new, unseen tasks?
% on \fix{to fix: some target domain}

% \notes{Add more intuition. Motivating why we are doing so.}

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

\vspace{-6pt}
To go beyond the fixed training paradigm, we propose to evolve the training distribution for aligning LLMs. Our method, which we call~\method,  alternates between two steps: (i) \tb{creating tasks} (or prompts), and (ii) \tb{solving them}.  As shown in Figure~\ref{fig:game}, these two steps are as follows:
\vspace{-3pt}
\begin{itemize}
    \item $\emphredd{\text{\bf \tc{Creator}}}$ \hspace{+1pt}: generates increasingly informative prompts.
    \item $\emphgreenn{\text{\bf \tg{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}}$ \hspace{+1pt}: produces responses to prompts and optimize for alignment.
\end{itemize}

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% One of the key challenges in open-ended learning is ensuring that an agent can generalize to unseen, novel environments, rather than overfitting to a fixed distribution. 

Typical preference optimization algorithms~\citep{dpo,self-play-gu,simpo} rely on a static set of training prompts, which can be viewed as a single \tb{solver step}. By adding the \tb{creator step}, ~\method\ can identify and generate a set of most informative prompts for the current policy to most efficiently learn from. This allow going beyond a static prompt set during training in the typical preference learning setting, and creating an evolving training curriculum that's most fit to the current policy and help generalize to the real-world tasks. Specifically, we implement the creator step by: (i) \textbf{estimate} the informativeness of each prompt, given an existing prompt distribution; (ii) \textbf{sample} an informative subset from those prompts, weighted by the informativeness score; (iii) \textbf{evolve} the informative subset by synthetically generating similar prompts in its \emph{proximal region}, and combine with a buffer of previous prompts, which forms a new prompt distribution. This can be flexibly plugged into any existing alignment pipeline, as shown in  Fig~\ref{fig:pipeline} and Algo~\ref{alg:i-eva}.

% \footnote{The informativeness measure we use is %related to the advantage function, which is empirically 
% estimated by sampling multiple responses from the prompt and take the difference between the maximal reward $r_{\max}$ and the minimal reward $r_{\min}$ received for the responses.}

% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 

% RA.24.9: Discuss and summarize empirical results here.

%% RA.24.9: This seemed quite repetitive, so merged it with previous para.
% In Algorithm~\ref{alg:i-eva}, we illustrate a practical algorithm for~\method. Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{dpo,simpo}.

% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.


% \notes{To write it differently. Instead of motivating by the iterative training issue, we should directly focus on our method per se. First introduce the underlying principle of generative state exploration; then discuss the classical literature on instruction generation (mostly uniform). Then discuss the practical design of our method. Our main table would focus on 1-iteration improvement with our method. We can then move to the iterative setting . In the literature part, we can mention other concurrent works.}

% Our setup is iterative preference optimization with self-generated responses\footnote{This approach has become increasingly common in recent literature~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}.}. It is important that we choose to initilize using the solution of the previous iteration\footnote{See more discussion on efficiency issues forthcoming}, rather than initilizing from scratch. The baseline setting is that there is only a fixed prompt set, and we iteratively train models with the fixed prompt set with newly self-generated response. We can show that there is a performance drop or plateau as more iterations go, if we only evolve in the $\rvy \mid \rvx$ distribution for the new iterations. We propose that we must adapt the $\rvx$ distribution as well, and propose a new principle as well as an practical algorithm.
  
% \begin{center}
% \emph{Starting from a fixed training prompt set, can we continuously improve alignment on the target domain?}
% \end{center}

% \method~generates the next training batch of prompts, by evolving prompts (\ie~making edits or variations) with higher estimated learning potential.

% Our method, \method, evolves the prompt distribution by generating prompts with high learning potential, incentivizing the language agents to solve increasingly informative prompts. 



Our main contributions are summarized as:
\begin{itemize}
\vspace{-3pt}
    % \item \textbf{A phenomenon}: We show that classical iterative preference optimization algorithms exhibit the \emph{reverse scaling trap}, where continual training with more data can \emph{hurts}  alignment. 

    \item \textbf{A new principle}: We propose \method, a generalized \textbf{open-ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment.
    % \fix{add generalization, and say that also generalize classical RLHF}
% \begin{align}
% % \max_{\phi, \theta} &\mathbb{E}_{\textcolor{red}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{Green}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] \nonumber \\
% % &- D_{\text{KL}}(\textcolor{red}{p_{\phi}(x)} \cdot \pi_{\theta}(y \mid x) \mid\mid \textcolor{red}{p_{\text{true}}(x)}\cdot \pi_{\text{ref}}(y \mid x)) \nonumber \\
% \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \emphred{\textcolor{cred}{\pi_{\vphi}(\rvx)}} \cdot \emphgreen{ \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)}} \ \| \ \emphgray{\tb{\pi_{\text{ref}}(\rvx, \rvy)}}\ \Biggr]\nonumber 
% % \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{black}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\ \Biggr]\nonumber 
% % \\
% % &= \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})]   - \mathbb{E}_{\textcolor{red}{\mathbf{x} \sim p_{\phi}(\cdot)}}[\textcolor{black}{D_{\text{KL}}(\textcolor{cgreen}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx))}] \nonumber \\
% % & \qquad \quad \ - \textcolor{cred}{D_{\text{KL}}(\pi_{\phi}(\rvx) \mid\mid p_{\text{true}}(\rvx))} \nonumber
% \end{align} 

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline.

    % \item \textbf{A new continual training procedure}: We first formally identify the \textbf{inverse scaling trap} in iterative alignment. Combining with explicit regularization, we present an efficient continual training procedure with our method. \ziyu{This part needs more tuning.}
    
    \item \textbf{State-of-the-art performance}: We empirically validate our method on public alignment benchmarks and present universally strong performance improvement when plugged in with different preference optimization algorithms (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide additional insights on the choice of informativeness metric, reward model, and training schedules. 
    % \notes{To mention impact on downstream tasks, as the original RLHF paper did~\citep{rlhf}.}
\end{itemize}

% [TODO: a paragraph that explains our method in the simplest form.] Our approach is very simple: given any existing prompt set, the creator sample prompts that are most informative for preference aligning, then evolve a new set upon the previous set; the solver will generate responses, which will in turn be used for preference optimization. Central to our approach is the informativeness metric, which we use the reward gap (contrastive ratio). 


% \notes{consider adding the metric (reward advantage / contrastive ratio) for prompt informativeness as a new contribution (useful beyond our work); also provide an intuitive example with bandits.}

% \notes{Also discuss the regret-based curriculum and the open-endedness literature~\citep{accel} }

% \notes{TODO: providing an intuitive example using bandits to illustrate that our perspective is new (This also brings a new perspective of ``\emph{generative exploration}'' for RL, in the sense that we actively generate states during the learning process, which is typically undoable in classical contextual bandits/RL.). }

% Having a distribution that covers all the complexity of the real world is very challenging~\citep{paired}.

% \fix{The creator step is straight-forward.}



\method~is simple to implement. We hope it can serve as a scalable starting point to build \text{open-ended} self-improving language agents that align with human values and co-evolve with human intelligence.

% \notes{producing learnable but novel artifacts~\citep{open-endedness}}\notes{maybe somewhere differentiate mention intrinsic motivation and incentivizing } 
% \fix{See App~\ref{sec:temporary notes} for some revision notes (\eg adding literature discussion; structured motivation; most importantly, highlight on the usage of reward model; improve clarity; etc.). We can improve a lot.}

% \textcolor{red}{[Introduction needs some work and should state that the creator step relies on the computation of a notion of informativeness and on a method that evolves prompts. This needs to be stated asap so the reader understands the method and the algorithm. ]}

% \notes{Also adding a figure to illustrate the joint distribution perspective. One figure is on standard alignment, and the other figure is on eva.}

% Line 6 – 8 is a practical plug-in implementation to mimic the adversarial prompt player:
% evaluating the informativeness for each prompt
% e.g., max_reward - min_reward
% using the above metric as the weight for adaptive sampling to create an informative subset
% generating new prompts via a prompt generation policy 


% are many human values really worth to align?

% Central to our method is the informativeness measure 

% TODO: add plots of algo pipeline and performance.

% Two motivations: (i) the size of the prompt set is a bottleneck on existing alignment performance, and we need a robust way to continuously improve the alignment performance; (ii) naïvely training with more data could hurt the performance - this happens in both training from scratch  

% In~\citep{warm}, ``conventional intuition suggests that when solving a sequence of related optimization problem of this from, it should be possible to initialize using the solution of the previous iterate to ``warm start'' the optimization rather than ``initialize from scratch''. However, in practice this warm-starting seems to yield poorer generalization performance than models that have fresh random initialization.''

% Adding discussions on the re-warming and loss of plasticity literature; comparing with them.

% Adding discussions in the exploration literature of bandit and RL.



% We cast the preference alignment problem as an two-player asymmetric self-play game, while one player learns to propose the most informative prompt set, and the other player learns to best respond to the proposed prompt set. At the equilibrium, we expect to have the optimal policy of language generation for both players.

% % The simplifying assumptions underlying Bradley-Terry model cannot capture real-world human preferences, which are often intransitive.

% Self-play preference optimization~\citep{nlhf,rlhf-more-diff,self-play-gu} casts the alignment problem as a two-player, general-sum game, where each player is a policy, parameterized by the language model, that aims to optimize the probability of its responses to be preferred against the other player's. Existing works iteratively update the policy network for it to converge to the optimal policy characterizing by the Nash equilibrium, empirically showing it as a promising framework.

% However, a fundamental issue, which is often neglected by current algorithms, is that the initial prompt set may not adequately represent the full range of scenarios the model will encounter in the real world. This limitation can lead to policies that are optimal within the confined space of the initial prompts but suboptimal or even poorly performing when faced with a broader distribution of inputs.  
% %\notes{The reasoning gap could be one example.}
% %Moreover, as language models continue to evolve and improve, the nature and complexity of prompts that can effectively challenge and improve these models also change. This dynamic landscape necessitates a more adaptive approach to prompt selection and generation throughout the finetuning process. 

% % \notes{Rewrite this paragraph, and put emphasis only on the prompt set optimization part.}
% % However, several fundamental challenges arise when applying self-play alignment in the real world:
% % \begin{itemize}
% %     \item \textbf{Prompt Distribution Mismatch:} The assumption of sampling from a fixed prompt distribution $\mathcal{X}$ may lead to generalization issues. \notes{i.e., exploration in $p(x)$?}
% %     \item \textbf{Preference Uncertainty:} The preference oracle $\mathbb{P}(\cdot)$ may be noisy, biased, or limited in its capacity to judge all types of responses.\notes{This is like having two nested equilibriums; policy v. policy; generator v. discriminator.}
% %     \item \textbf{Response Space Constraints:} The model's ability to generate responses may not sufficiently cover the space of optimal responses. \notes{to rephrase; simply exploration for $p(y|x)$}
% % \end{itemize}

% % A useful prompt is often a \emph{surprising} prompt~\citep{ai-mathematician}.

% To address these challenges, we propose an \emph{evolving alignment} framework, with an \emph{asymmetric self-play} mechanism.

% Simply put, we consider to grow $\calX, \calY$, while existing work mostly care about $\calY \mid \calX$ with a fixed $\calX$.


    

    

==> texs/intro-fix.tex <==
\section{\textcolor{Gray}{[Draft]} Introduction}



% \begin{figure}[hb]
%     \centering
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/mt-bench.png}
%         \caption{Alpaca Eval}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/arena-hard.png}
%         \caption{Arena Hard}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/alpaca-eval.png}
%         \caption{MT Bench}
%     \end{subfigure}
%     \caption{Placeholder plot on evaluation results.}
%     \label{fig:three_benchmarks}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
%     \caption{Placeholder plot on pipeline.}
% \end{figure}


%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
Long-lived language agents must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
The human-generated data, crucial for scaling language models, is projected to run out in the next few years \citep{run-out-of-data}. This limitation necessitates new framework for continual model improvement.

% Some motivation statements:
% The key thing here is that learning is not a ``train-once'' thing; it should be open-ended and self-improving. Just like humans, we start with some basic knowledge, then we develop the whole modern science. The central things for  learning is about: (i) identifying the informative spaces (states \emph{and} actions) to explore; (ii) receiving useful feedback on such exploration. In this way we can continuously improve. 

% then motivate with 

% maybe providing a simple bandit example.

% revealed preference theory

% ~\citep{poet}: ``as compelling as this narrative may be, it is not the only conceivable path forward.  ... only rarely discussed, the job of the algorithm could be to conveive both the challenges and the solutions at the same time.'' increased complexity
% relation of self-play to co-evolution

Our research question is:

\begin{minipage}{1.0\textwidth}
% \footnotesize
\centering
\textit{Starting from a given training prompt set,\\}
\textit{can we continuously improve the alignment performance on a target domain?}
\end{minipage}


%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.


% \notes{To write it differently. Instead of motivating by the iterative training issue, we should directly focus on our method per se. First introduce the underlying principle of generative state exploration; then discuss the classical literature on instruction generation (mostly uniform). Then discuss the practical design of our method. Our main table would focus on 1-iteration improvement with our method. We can then move to the iterative setting . In the literature part, we can mention other concurrent works.}

% Our setup is iterative preference optimization with self-generated responses\footnote{This approach has become increasingly common in recent literature~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}.}. It is important that we choose to initilize using the solution of the previous iteration\footnote{See more discussion on efficiency issues forthcoming}, rather than initilizing from scratch. The baseline setting is that there is only a fixed prompt set, and we iteratively train models with the fixed prompt set with newly self-generated response. We can show that there is a performance drop or plateau as more iterations go, if we only evolve in the $\rvy \mid \rvx$ distribution for the new iterations. We propose that we must adapt the $\rvx$ distribution as well, and propose a new principle as well as an practical algorithm.
  
% \begin{center}
% \emph{Starting from a fixed training prompt set, can we continuously improve alignment on the target domain?}
% \end{center}




Our main contributions are summarized as:
\begin{itemize}
    % \item \textbf{A phenomenon}: We show that classical iterative preference optimization algorithms exhibit the \emph{reverse scaling trap}, where continual training with more data can \emph{hurts}  alignment. 

    \item \textbf{A new principle}: We propose \method, a general \textit{open-ended self-improving} \textbf{RLHF principle}:
\begin{align}
% \max_{\phi, \theta} &\mathbb{E}_{\textcolor{red}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{Green}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] \nonumber \\
% &- D_{\text{KL}}(\textcolor{red}{p_{\phi}(x)} \cdot \pi_{\theta}(y \mid x) \mid\mid \textcolor{red}{p_{\text{true}}(x)}\cdot \pi_{\text{ref}}(y \mid x)) \nonumber \\
\hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \emphred{\textcolor{cred}{\pi_{\vphi}(\rvx)}} \cdot \emphgreen{ \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)}} \ \| \ \emphgray{\tb{\pi_{\text{target}}(\rvx, \rvy)}}\ \Biggr]\nonumber 
% \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{black}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\ \Biggr]\nonumber 
% \\
% &= \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})]   - \mathbb{E}_{\textcolor{red}{\mathbf{x} \sim p_{\phi}(\cdot)}}[\textcolor{black}{D_{\text{KL}}(\textcolor{cgreen}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx))}] \nonumber \\
% & \qquad \quad \ - \textcolor{cred}{D_{\text{KL}}(\pi_{\phi}(\rvx) \mid\mid p_{\text{true}}(\rvx))} \nonumber
\end{align} 

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, implemented through alternating optimization in a \textbf{creator \emph{v.s.} solver game}\footnote{In the language space, the creator refers to the prompt generation policy $\pi_X$ and the solver refers to the response generation policy $\pi_{Y|X}$.}. We develop a simple and flexible algorithm that can be easily plugged into any existing alignment pipeline, with both off-policy (\texttt{eva-i}) and on-policy (\texttt{eva-o}) variants.

    % \item \textbf{A new continual training procedure}: We first formally identify the \textbf{inverse scaling trap} in iterative alignment. Combining with explicit regularization, we present an efficient continual training procedure with our method. \ziyu{This part needs more tuning.}
    
    \item \textbf{State-of-the-art performance}: We empirically validate our method on popular alignment benchmarks and present strong performance improvement with extensive ablation studies.
\end{itemize}

% [TODO: a paragraph that explains our method in the simplest form.] Our approach is very simple: given any existing prompt set, the creator sample prompts that are most informative for preference aligning, then evolve a new set upon the previous set; the solver will generate responses, which will in turn be used for preference optimization. Central to our approach is the informativeness metric, which we use the reward gap (contrastive ratio). 


% \notes{consider adding the metric (reward advantage / contrastive ratio) for prompt informativeness as a new contribution (useful beyond our work); also provide an intuitive example with bandits.}

% \notes{Also discuss the regret-based curriculum and the open-endedness literature~\citep{accel} }

% \notes{TODO: providing an intuitive example using bandits to illustrate that our perspective is new (This also brings a new perspective of ``\emph{generative exploration}'' for RL, in the sense that we actively generate states during the learning process, which is typically undoable in classical contextual bandits/RL.). }



We envision \texttt{eva}~as a foundational and scalable starting point to build open-ended self-improving language agents that aligns with human values. \fix{See Appendix~\ref{sec:temporary notes} for revision notes.}

% \notes{Also adding a figure to illustrate the joint distribution perspective. One figure is on standard alignment, and the other figure is on eva.}

% Line 6 – 8 is a practical plug-in implementation to mimic the adversarial prompt player:
% evaluating the informativeness for each prompt
% e.g., max_reward - min_reward
% using the above metric as the weight for adaptive sampling to create an informative subset
% generating new prompts via a prompt generation policy 


% are many human values really worth to align?

% Central to our method is the informativeness measure 

% TODO: add plots of algo pipeline and performance.

% Two motivations: (i) the size of the prompt set is a bottleneck on existing alignment performance, and we need a robust way to continuously improve the alignment performance; (ii) naïvely training with more data could hurt the performance - this happens in both training from scratch  

% In~\citep{warm}, ``conventional intuition suggests that when solving a sequence of related optimization problem of this from, it should be possible to initialize using the solution of the previous iterate to ``warm start'' the optimization rather than ``initialize from scratch''. However, in practice this warm-starting seems to yield poorer generalization performance than models that have fresh random initialization.''

% Adding discussions on the re-warming and loss of plasticity literature; comparing with them.

% Adding discussions in the exploration literature of bandit and RL.



% We cast the preference alignment problem as an two-player asymmetric self-play game, while one player learns to propose the most informative prompt set, and the other player learns to best respond to the proposed prompt set. At the equilibrium, we expect to have the optimal policy of language generation for both players.

% % The simplifying assumptions underlying Bradley-Terry model cannot capture real-world human preferences, which are often intransitive.

% Self-play preference optimization~\citep{nlhf,rlhf-more-diff,self-play-gu} casts the alignment problem as a two-player, general-sum game, where each player is a policy, parameterized by the language model, that aims to optimize the probability of its responses to be preferred against the other player's. Existing works iteratively update the policy network for it to converge to the optimal policy characterizing by the Nash equilibrium, empirically showing it as a promising framework.

% However, a fundamental issue, which is often neglected by current algorithms, is that the initial prompt set may not adequately represent the full range of scenarios the model will encounter in the real world. This limitation can lead to policies that are optimal within the confined space of the initial prompts but suboptimal or even poorly performing when faced with a broader distribution of inputs.  
% %\notes{The reasoning gap could be one example.}
% %Moreover, as language models continue to evolve and improve, the nature and complexity of prompts that can effectively challenge and improve these models also change. This dynamic landscape necessitates a more adaptive approach to prompt selection and generation throughout the finetuning process. 

% % \notes{Rewrite this paragraph, and put emphasis only on the prompt set optimization part.}
% % However, several fundamental challenges arise when applying self-play alignment in the real world:
% % \begin{itemize}
% %     \item \textbf{Prompt Distribution Mismatch:} The assumption of sampling from a fixed prompt distribution $\mathcal{X}$ may lead to generalization issues. \notes{i.e., exploration in $p(x)$?}
% %     \item \textbf{Preference Uncertainty:} The preference oracle $\mathbb{P}(\cdot)$ may be noisy, biased, or limited in its capacity to judge all types of responses.\notes{This is like having two nested equilibriums; policy v. policy; generator v. discriminator.}
% %     \item \textbf{Response Space Constraints:} The model's ability to generate responses may not sufficiently cover the space of optimal responses. \notes{to rephrase; simply exploration for $p(y|x)$}
% % \end{itemize}

% % A useful prompt is often a \emph{surprising} prompt~\citep{ai-mathematician}.

% To address these challenges, we propose an \emph{evolving alignment} framework, with an \emph{asymmetric self-play} mechanism.

% Simply put, we consider to grow $\calX, \calY$, while existing work mostly care about $\calY \mid \calX$ with a fixed $\calX$.


    

    

==> texs/intro.tex <==
\vspace{+6pt}
\emph{What I cannot \tb{create}, I do not \tb{understand}.} 
\vspace{-8pt}
\begin{flushright}
\emph{-- Richard P. Feynman}
\end{flushright}
\vspace{-8pt}

%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
% \vspace{+3.pt}
% \section {Introduction}\label{sec:intro}\vspace{-5pt}

\section{Introduction}\label{sec:intro}
Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
High-quality human data, crucial for scaling large language model based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as those large models become more capable, they need to identify and solve new and increasingly complex challenges, requiring training data beyond the capabilities of humans to create. This necessitates a new fundamental training mechanism, where models can continue to self-improve by generatively exploring and solving new problems. We thereby investigate the research question below:

\begin{minipage}{1.\textwidth}
\centering\vspace{+5.6pt}
\textit{Can language models identify and \emph{self-create} new, learnable tasks to work on,\\}
\textit{to \emph{self-improve} to \emph{generalize} better for human preferences alignment?}
\vspace{-6.6pt}
\end{minipage}
%or higher intelligence.


% \notes{One way to write the motivation part may be to follow ~\citep{poet,bengio2009curriculum,accel,paired}. Discuss how we incentivize the agent to generate prompt distribution with increasing complexity, promoting the models to solve harder problems.}

% \notes{Additional motivation/intuition/background paragraphs need to be added here. Motivate why we need to jointly optimize for both.}

% We aim to develop language agents capable of surpassing even superior intelligence, enabling them to solve increasingly complex problems.


% \vspace{-6pt}


% \vspace{+2pt}







% \vspace{-6pt}

Many preference optimization algorithms~\citep{rlhf,dpo,slic, liu2023statistical, dpo-ai-feedback} have been proposed to improve the alignment of language models, however, they all default to  fixed prompt training distributions. Such fixed training paradigm inevitably leads to: (i) \emph{generalization issues} (models may underperform or hack on instructions that are insufficiently represented in the fixed set) and (ii) \emph{efficiency issues} (data annotation and model training are costly, however not all prompt provide the same utility; it is wasteful to invest in sub-optimal fixed set, while identifying informative prompts through human efforts is expensive and time-consuming)~\citep{team-1,gemma2,llama3}. 

The objective thereby should not only be to optimize over a specific, static distribution of prompts, yet to develop an agent that can autonomously evolve the training data distribution for self-improvement, to align well across unseen, novel environments or tasks (instantiated by prompts).

\begin{figure}[t]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \caption{\textbf{Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our proposed~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with an easy-to-implement \emph{estimate, sample then evolve} procedure; specifically, it estimates the informativeness for each prompt by how contrastive the self-generated responses are to the prompt, from the reward signals it receives. The creator evolves new prompts  from highly informative prompts, which the solver uses for continual training. The solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective that drives the above design in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \vspace{-6pt}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}

% rely on a static set of training prompts.

% , which can be viewed as a single \tb{solver step}. 

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.


Thus, we develop~\method~(\underline{E}volving Alignment \emph{\underline{v}ia} \underline{A}symmetric Self-Play), as illustrated in Figure~\ref{fig:game}. Central to our approach is a game with the minimax-regret objective, achieved through alternating optimization between \tb{creating prompts} and  \tb{solving them}. The interplay encourages evolving curricula~\citep{accel}, potentially benefits both generalization and efficiency (see also $\S$~\ref{sec:int}). Orthogonal to many recent self-play studies in LLM alignment~\citep{nlhf,srpo,self-play-gu}, \method~is \emph{asymmetric}~\citep{intrinsic}, with two policies of different goals:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Creator}: evolves the prompt distribution for alignment.\vspace{+1.5pt}
    \item \textbf{Solver}: produces responses and optimizes  alignment based on the evolving prompts.
\end{itemize}


% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 



% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.




\vspace{-5pt}
Our main contributions are summarized as:
\begin{itemize}
\vspace{-5pt}
    \item \textbf{A new principle}: We propose a generalized \textbf{Open-Ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment, as in Definition~\ref{eq:rlhf-joint}.\vspace{+1.5pt}

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline, as in Algorithm~\ref{alg:i-eva}.\vspace{+1.5pt}
    
    \item \textbf{State-of-the-art performance}: We empirically validate~\method~on public alignment benchmarks and present general strong performance improvement when plugged in with different preference optimization algorithms (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide further insights on choices of informativeness metrics, reward models and training schedules, as in $\S$~\ref{sec:exp}.

\end{itemize}





\method~\textbf{is easy to implement}. We hope it can serve as a scalable method for the research community to build \text{open-ended}, robust, and self-improving language agents, that align with human values.




==> texs/lit-fix.tex <==
% \newpage
\section{\textcolor{Gray}{[Draft]} Related Works}

% to read: curriculum learning, trpo, self-rewarding llm.

% We here cite major relevant works and highlight the difference from our work. More detailed discussions can be found in the Appendix \textcolor{Maroon}{?}.

% We hereby cite the most relevant works and highlight the distinctions between them and our framework. A more comprehensive discussion is provided in the Appendix \textcolor{Maroon}{?}.

\paragraph{Self-improving algorithms and iterative optimization.} This line of work focuses on iteratively generating samples from the response policy and continuously re-training the policy by selected self-generated samples. Major works include ReST~\citep{rest, rest_em}, STaR~\citep{star}, RFT~\citep{rft}, RAFT~\citep{raft}, self-improving LLMs~\citep{llm-can-self-improve, self-reward}; in the context of preference optimization, iterative DPO~\citep{dpo-iterative,dpo-on-policy,snorkel,xiong2024iterative,rpo} has proven effective. Most works focus on self-training by improving in the $\calY \mid \calX$ space, we are the first to \emph{jointly optimize} both responses and prompts through generative exploration in the $(\calX, \calY)$ space. 
% \notes{We may add detailed comparison with~\cite{self-reward} on the usage of instructions.}
% Maybe we can explain this in a more clear way in the appendix. Check the self-play finetuning review in the sppo paper.

\paragraph{Prompt synthesis for language models.}  Existing works, such as Self-Instruct~\citep{self-instruct}, WizardLM~\citep{wizardlm,wizardmath}, Self-Align~\citep{self-align}, Glan~\citep{glan}, EvoPrompt~\citep{evoprompt}, Magpie~\citep{magpie} and others~\citep{survey-data}, primarily rely on supervised fine-tuning (\ie the SFT phase) to optimize language models. In contrast, our work (i) presents a new reward-driven metric to endow prompt the notion of informativenss; (ii) focuses on preference optimization (\ie the RLHF phase), and (iii) is supported by solid theoretical foundations.



% \notes{Most existing works consider to (i) uniformly evolve prompts, (ii) using the evolved prompts for SFT. Our works differ by proposing a prompt selection metric elicited from rewards, and utilizing the prompts for alignment.}

\paragraph{Self-play and curriculum RL.} Any agent trained on a fixed data distribution is often brittle and may struggle to adapt to the real world~\citep{open}. Self-play~\citep{checker,gan,alphago} addresses this by having the agent learn through self-interaction, thus creating more diverse experiences and automatic curricula. In asymmetric self-play, the paradigm centers on ``\emph{Alice proposing a task, and Bob doing it}''~\citep{intrinsic,maestro,minimax-refine,paired}. We\hide{are among the first to} rejuvenate the classical asymmetric self-play principle~\citep{horde} in optimizing language models. Unlike traditional curriculum RL~\citep{accel}, which usually renders environments from specified settings~\citep{paired}, our approach is \emph{generative} by nature, as we directly generate contexts (prompts) from the auto-regressive language models, guided by informativeness signals elicited from preferences.

% \paragraph{Self-play in RLHF.} There is a growing line of research that frame RLHF as two-player constant game, where both players are the response player compete to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between the response players, they still assume a fixed prompt distribution, while the most important thing of our approach is that we enable a dynamic prompt distribution useful for training. One similar concurrent work to ours is GPO~\citep{gpo}, however it is (i) designed for defend adversarial attack instead of general alignment; (ii) using PPO instead of direct preference optimization. We additionally present a summary table on other alignment algorithms in Appendix~\ref{app:table}.

\paragraph{Self-play in RLHF.} A growing line of research frames RLHF as a symmetric two-player game, where both players are the  response players competing to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between response players, these methods still rely on a fixed prompt distribution thus is sub-optimal. In contrast, our method  integrates evolving prompt distributions \textit{via} the asymmetric game setting\footnote{We notice one concurrent work adopting the asymmetric two-player setup~\citep{gpo}, however (i) it focuses on adversarial defense rather than general alignment, (ii) it uses PPO instead of direct preference optimization, and (iii) it uses the maxmin principle (which is known to be producing unlearnable environments~\citep{paired} and is not incentivized to guide the learning agents) instead of minimax \emph{regret} principle~\citep{fan1953minimax,savage1951theory} as we do.}.
% Additionally, our approach is more flexible and can be easily integrated into existing alignment pipelines. 

% \paragraph{Curriculum learning, active learning and evolution strategies.} Curriculum learning~\citep{bengio2009curriculum}; ordered SGD~\citep{ordered-sgd}, Active Preference Learning~\citep{active-pl}, Curry-DPO~\citep{curry-dpo},  Selective Reflection-Tuning~\citep{selective-rt}; . \notes{Existing works consider only \emph{re-weighting} or \emph{re-ordering} the data presented in training, while we propose to \emph{generate} new data based on, this resembles evolution strategies~\citep{es-openai}. }

\paragraph{Curriculum learning, active learning, and evolution strategies.} Existing methods, such as curriculum learning~\citep{bengio2009curriculum}, ordered SGD~\citep{ordered-sgd}, active preference optimization~\citep{active-pl,curry-dpo},  and selective finetuning~\citep{selective-rt}, focus on \emph{re-weighting} or \emph{re-ordering} the training data. In contrast, we propose a method that \emph{generates} new data based on preference signals, with similarities to evolution strategies~\citep{es-openai}. 





% \paragraph{Iterative (preference) optimization.} Self-improving LLMs~\citep{llm-can-self-improve},  self-rewarding LLMs~\citep{self-reward}, \citep{xiong2024iterative}, SRPO~\citep{srpo}, reasoning preference optimization~\citep{rpo}, ReST~\citep{rest}, Iterative DPO~\citep{snorkel}.

% \paragraph{Self-play LLMs.} Self-Reine, STaR, ReST, SPPO, SRPO.
% ~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}

% (Some somewhat relevant concurrent works: GPO~\citep{gpo}, SEAS~\citep{seas}, , )



% % \paragraph{Data Synthesis with LLMs.} EvoPrompt~\citep{evoprompt}, Self-Instruct~\citep{self-instruct}

% \paragraph{Self-improving algorithms.} General: \citep{def-open,open-endedness,continual-rl}. For LLMs: self-instruct~\citep{camel,self-instruct,evoprompt}, self-critique~\citep{camel}, self-debug~\citep{self-debug}. 

% \paragraph{Self-play and automatic curriculum generation.} \citep{checker,silver2017mastering}

% % \paragraph{Self-training.} 

% \paragraph{Online (contrastive) alignment algorithms.} 
% % Generating in the X space presents a fundamentally different challenge.

% % \paragraph{Evolving instructions for language model post-training.} 


==> texs/lit.tex <==
\newpage
\section{Related Works}\label{sec:lit}
\vspace{-4pt}

% to read: curriculum learning, trpo, self-rewarding llm.

% We here cite major relevant works and highlight the difference from our work. More detailed discussions can be found in the Appendix \textcolor{Maroon}{?}.

% We hereby cite the most relevant works and highlight the distinctions between them and our framework. A more comprehensive discussion is provided in the Appendix \textcolor{Maroon}{?}.

\paragraph{Self-improving algorithms and iterative optimization.} This line of work focuses on iteratively generating samples from the response policy and continuously re-training the policy by selected self-generated samples. Major works include ReST~\citep{rest, rest_em}, STaR~\citep{star}, RFT~\citep{rft}, RAFT~\citep{raft}, self-improving LLMs~\citep{llm-can-self-improve, self-reward}; in the context of preference optimization, iterative DPO~\citep{dpo-iterative,dpo-on-policy,snorkel,xiong2024iterative,rpo} has proven effective. Most works focus on self-training by improving in $\calY \mid \calX$, while we \emph{jointly optimize} both responses and prompts via generative exploration in the $(\calX, \calY)$ space. Among them, we also distinctly present a game-theoretic framework for continual training. 
\vspace{-10pt}
% \notes{We may add detailed comparison with~\cite{self-reward} on the usage of instructions.}
% Maybe we can explain this in a more clear way in the appendix. Check the self-play finetuning review in the sppo paper.

\paragraph{Prompt synthesis for language models.}  Existing works include Self-Instruct~\citep{self-instruct}, WizardLM~\citep{wizardlm,wizardmath}, Self-Align~\citep{self-align}, Glan~\citep{glan}, EvoPrompt~\citep{evoprompt}, Magpie~\citep{magpie} and others~\citep{survey-data}. \method~is an orthogonal contribution since any synthesis method can be plugged in as the $\texttt{\small evolve}(\cdot)$ for the creator. Importantly, our work presents a new reward-related metric to endow prompt the notion of informativeness. We also focus on preference optimization algorithms, while those existing works  primarily use synthesized prompts in an SFT-only way.
% supervised fine-tuning (\ie the SFT phase).
 
\vspace{-10pt}
% \notes{Mention that our work is an orthogonal contribution to this since we can plug in any prompt synthesis method -- just editting in the high-regret levels.}
% , and (iii) is supported by solid theoretical foundations.
% (\ie the RLHF phase)



% \notes{Most existing works consider to (i) uniformly evolve prompts, (ii) using the evolved prompts for SFT. Our works differ by proposing a prompt selection metric elicited from rewards, and utilizing the prompts for alignment.}

\paragraph{Self-play and curriculum RL.} Agents trained on a fixed data distribution are often brittle and may struggle to adapt to the real world~\citep{open}. Self-play~\citep{checker,gan,alphago} addresses this by having the agent learn through self-interaction, thus creating more diverse experiences and automatic curricula. In asymmetric self-play, the paradigm centers on ``\emph{Alice proposing a task, and Bob doing it}''~\citep{intrinsic,maestro,minimax-refine,paired}. We\hide{are among the first to} revive the classical asymmetric self-play~\citep{horde} in optimizing language models. Unlike traditional curriculum RL~\citep{accel}, which renders environments by specifying levels~\citep{paired}, our approach is \emph{generative} by nature, as we directly generate \emph{states} from auto-regressive language models. We believe such generative exploration in the joint state-action space presents a new training paradigm.
\vspace{-20pt}
% guided by informativeness signals elicited from preferences.

% \paragraph{Self-play in RLHF.} There is a growing line of research that frame RLHF as two-player constant game, where both players are the response player compete to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between the response players, they still assume a fixed prompt distribution, while the most important thing of our approach is that we enable a dynamic prompt distribution useful for training. One similar concurrent work to ours is GPO~\citep{gpo}, however it is (i) designed for defend adversarial attack instead of general alignment; (ii) using PPO instead of direct preference optimization. We additionally present a summary table on other alignment algorithms in Appendix~\ref{app:table}.
 % competing to generate more preferred responses
\paragraph{Self-play in RLHF.} A growing line of research frames RLHF as a \emph{symmetric} self-play game, where both players are response players~\citep{nlhf,self-play-gu,srpo,dno}. However,  these methods still rely on a fixed prompt distribution thus is sub-optimal. In contrast, we solve this by \emph{asymmetric} self-play, enabling evolving prompt distributions for more generalizable language agents. During our work, we notice one concurrent paper adopting the asymmetric two-player setup~\citep{gpo}, however (i) it applies to adversarial attack tasks instead of general alignment benchmarks, (ii) it is incompatible w/ direct preference optimization, and (iii) it relies on the maxmin principle (which may produce unlearnable environments~\citep{paired}) instead of the minimax \emph{regret} principle~\citep{fan1953minimax,savage1951theory} as we do. We also first precisely define the new problem of open-ended RLHF, generalizing over classical RLHF.
\vspace{-6pt}
 % and is not incentivized to guide the learning agents
% Additionally, our approach is more flexible and can be easily integrated into existing alignment pipelines. 

% \paragraph{Curriculum learning, active learning and evolution strategies.} Curriculum learning~\citep{bengio2009curriculum}; ordered SGD~\citep{ordered-sgd}, Active Preference Learning~\citep{active-pl}, Curry-DPO~\citep{curry-dpo},  Selective Reflection-Tuning~\citep{selective-rt}; . \notes{Existing works consider only \emph{re-weighting} or \emph{re-ordering} the data presented in training, while we propose to \emph{generate} new data based on, this resembles evolution strategies~\citep{es-openai}. }

% \paragraph{Curriculum learning, active learning, and evolution strategies.} Existing methods, such as curriculum learning~\citep{bengio2009curriculum}, ordered SGD~\citep{ordered-sgd}, active preference optimization~\citep{active-pl,curry-dpo},  and selective finetuning~\citep{selective-rt}, focus on \emph{re-weighting} or \emph{re-ordering} the training data. In contrast, we propose a method that \emph{generates} new data based on preference signals, with similarities to evolution strategies~\citep{es-openai}. 





% \paragraph{Iterative (preference) optimization.} Self-improving LLMs~\citep{llm-can-self-improve},  self-rewarding LLMs~\citep{self-reward}, \citep{xiong2024iterative}, SRPO~\citep{srpo}, reasoning preference optimization~\citep{rpo}, ReST~\citep{rest}, Iterative DPO~\citep{snorkel}.

% \paragraph{Self-play LLMs.} Self-Reine, STaR, ReST, SPPO, SRPO.
% ~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}

% (Some somewhat relevant concurrent works: GPO~\citep{gpo}, SEAS~\citep{seas}, , )



% % \paragraph{Data Synthesis with LLMs.} EvoPrompt~\citep{evoprompt}, Self-Instruct~\citep{self-instruct}

% \paragraph{Self-improving algorithms.} General: \citep{def-open,open-endedness,continual-rl}. For LLMs: self-instruct~\citep{camel,self-instruct,evoprompt}, self-critique~\citep{camel}, self-debug~\citep{self-debug}. 

% \paragraph{Self-play and automatic curriculum generation.} \citep{checker,silver2017mastering}

% % \paragraph{Self-training.} 

% \paragraph{Online (contrastive) alignment algorithms.} 
% % Generating in the X space presents a fundamentally different challenge.

% % \paragraph{Evolving instructions for language model post-training.} 


==> texs/method-cache.tex <==
\newpage
\section{Method}\label{sec:method}
Our objective is to develop LLMs that can \emph{self-improve  to generalize well on new, unseen tasks} beyond the initial training prompt distribution for alignment. 
In $\S$\ref{sec:principle}, we motivate by the limitations of existing RLHF frameworks and formally define the new objective of open-ended RLHF. Next in $\S$\ref{sec:mechanism}, we introduce the creator-solver game to tractably optimize the objective. Later in $\S$\ref{sec:algo}, we detail the practical algorithm compatible with any preference optimization method as the solver, with a creator in the loop. Lastly in $\S$\ref{sec:int}, we present further interpretations on the nice properties of~\method.

% We frame this as a creator-solver game: starting from a given prompt distribution, the creator identifies the region with the most learning potential using reward signals, then evolves prompts in those regions via proximal modifications; the solver then generates multiple responses to each of the evolved prompts and performs preference optimization based on reward annotation. We will precisely define the terminology used here as follows.

% The creator LLM and the solver LLM can share the same or different parameters. % maybe make this a footnote
% ~\notes{Revise this paragraph for intuitive motivation.}


% \textcolor{red}{[The method and algorithm section should be merged together and go directly to the point. The reader needs to wait for page 5 before having a clear understanding of what is the proposed method. Bring the presentation of the method sooner. Explaining that the method consists of two steps, creating prompts and solving them. Needs to appear asap in the presentation. Especially the choice of what is the creator optimising.]}

% to add more discussions. the initial RLHF fixed in a training set~\citep{rlhf}; we want the process to be open-ended (there are many informal or formal definitions of open-endedness~\citep{open-endedness}); two crucial characteristics are that 


% Our goal is to achieve high rewards on the unknown target distribution for prompts in the wild $\pi_{\text{target}}(\rvx)$, while maintaining the proximity of the response policy to the reference policy. Here, the newly introduced $\pi_{\text{target}}(\rvx)$  can be seen as an \emph{unspecified environment}~\citep{paired}.

% \tc{Discuss the issue of traditional RLHF, then lead to that we need a framework that can discover novel and learnable prompts to further improve the performance. In open-ended RLHF, we want to generate a distribution of prompts to continue to train the policy for preference optimization;}
%% RA.21.9: Before showing any math, probably worth motivating what we want to do -- the role of  theory is formalize things, which should be intutitive. 

% TODO: introducing the asymmetric self-play mechanism for language models.
% Essentially there are two 
\subsection{The Principle: Open-edned RLHF for Joint Self-Improvement}~\label{sec:principle}
\hspace{-6pt}\textbf{Intuition.} \ \ Classical RLHF (\textit{cf}., Eq.~\ref{eq:rlhf-cls}) optimizes over a static distribution, meaning that the agent is only aligned to a fixed reference point, making the agent brittle when it encounters new tasks or is evaluated on new benchmarks in the ever-changing real world, \ie \emph{the static optimization fails to adapt}. The idea behind our Open-Ended RLHF is to break away from this static framework, with the objective of developing an agent that generalizes well across \emph{unseen, novel} environments, where the prompts (tasks) may not have been explicitly encountered during training. To achieve this, we must design a new objective that moves beyond optimizing over a fixed dataset $\mathcal{D}$, allowing $\rvx$ to come from a dynamic, ever-changing distribution that co-evolves with the agent's ability to solve tasks.




\vspace{-4pt}
\paragraph{Formalization.} We formally define this by introducing an \emph{optimizable} prompt generation policy $\pi_{\vphi}(\rvx)$, which is \emph{jointly} optimized with the response policy $\pi_{\vtheta}(\rvy \mid \rvx)$, as follows:

\vspace{+1pt}


% \notes{First mention the limit of traditional RLHF here, then discuss why we need open-ended RLHF}
% \hspace{-8pt}The goal is to train a language agent that can perform well across the unknown target prompt distribution. We formalize the idea below.
% \vspace{-0.35cm}
\begin{mdframed}
\begin{defn}[Open-ended RLHF]\label{eq:rlhf-joint}
We define \emph{evolving alignment} as the open-ended joint optimization\footnote{\textcolor{black}{Classical RLHF (Eq.~\ref{eq:rlhf-cls}) is a special case when $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint-}:}
\begin{align}
\max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\bigr[\ r(\mathbf{x}, \mathbf{y}) \ \bigr]   &- \textcolor{cred}{\sE}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cred}{\bigr[ \ }\textcolor{black}{\sD_{\text{KL}}\bigr[\textcolor{black}{\pi_{\theta}(\rvy | \rvx)} \| \pi_{\text{ref}}(\rvy | \rvx)\bigr]}\ \textcolor{cred}{\bigr]} 
- \textcolor{cred}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \| p_{\text{ref}}(\rvx)\ \bigr]}. \nonumber 
\end{align}}  on the prompt and response policy for alignment w.r.t the joint reference policy:
\begin{align}
    \max_{\vphi, \vtheta} \  J_{\vphi, \vtheta}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\emphinlinered{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}} \ , \ \emphinlinegreen{\textcolor{cgreen}{\rvy \sim \pi_{\vtheta}(\rvy|\rvx)}} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
    - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vphi, \vtheta}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)  } \ \Biggl], \label{eq:rlhf-joint-} \vspace{-5pt}
\end{align}
where $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ and $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$.
% denotes the training joint distribution and the reference joint distribution, respectively.
\end{defn}
\end{mdframed}
Here, $p_{\text{ref}}(\rvx)$ represents an idealized, potentially intractable probability measure over all possible tasks (instantiated \emph{via} prompts) in the wild. This is a conceptual reference  that encompasses the full diversity and complexity of tasks agents may encounter, serving as a guiding target for alignment. Additionally, the \emph{joint optimization} ensures that the task distribution and the agent’s response policy are updated in tandem, enabling adaptation to increasingly complex tasks, thereby promoting generalization.
 % or directly optimizable

% \begin{itemize}
%     \vspace{-4pt}
%     \item $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ is the joint policy for prompts and responses.
%     % \item $\tc{\emphred{\pi_{\vphi, \vtheta}(\rvx, \rvy) }} := \tc{\emphred{\pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}$ is the joint policy for prompts and responses.
%     \item $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$ is the reference joint distribution.
% \end{itemize}

% \begin{defn}[Evolving Alignment]
% Evolving alignment is the open-ended joint optimization\footnote{Classical RLHF is a special case when $\pi_{\phi}$ is a static distribution as $\pi_{\text{target}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint}:
% \begin{align}
% \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]   &- \textcolor{black}{\sE}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{black}{\Bigr[}\textcolor{black}{\sD_{\text{KL}}\Bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx)\Bigr]}\textcolor{black}{\Bigr]} 
% - \textcolor{black}{\sD_{\text{KL}}\Bigr[\pi_{\phi}(\rvx) \mid\mid \pi_{\text{target}}(\rvx)\Bigr]}. \nonumber
% \end{align}}  of the prompt distribution and response policy for alignment w.r.t the joint reference distribution, that is:
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\emphinlinered{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}} \ , \ \emphinlinegreen{\textcolor{cgreen}{\rvy \sim \pi_{\vtheta}(\rvy|\rvx)}} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vpsi}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
% \end{align}
% where $\vpsi = (\vphi, \vtheta)$ represents all parameters of the joint policy such that:
% \begin{itemize}
%     \item $\tc{\emphred{\pi_{\vpsi}(\rvx, \rvy) }} := \tc{\emphred{\pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}$ is the joint policy distribution for prompts and responses.
%     \item $\pi_{\text{ref}}(\rvx, \rvy) := \pi_{\text{target}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$ is the reference joint distribution.
% \end{itemize}
% \end{defn}

% \notes{Revise the definition for more rigor and clarity.}


% We generalize the classical RLHF objective to jointly optimize over contexts and responses\footnote{Classical RLHF is a special case when $\pi_{\phi}$ is a static distribution as $\pi_{\text{target}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint}:
% \begin{align}
% \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]   &- \textcolor{cred}{\sE}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cred}{\Bigr[}\textcolor{black}{\sD_{\text{KL}}\Bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx)\Bigr]}\textcolor{cred}{\Bigr]} 
% - \textcolor{cred}{\sD_{\text{KL}}\Bigr[\pi_{\phi}(\rvx) \mid\mid \pi_{\text{target}}(\rvx)\Bigr]}. \nonumber
% \end{align}}:
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{target}})\ := \ \mathbb{E}_{\textcolor{cred}{(\rvx,\, \rvy) \sim \pi_{\vpsi}(\rvx, \rvy)}}\Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \underbrace{\tc{\emphred{ \hspace{+5pt} \pi_{\vpsi}(\rvx, \rvy) \hspace{+5pt} }  }}_{  \tc{\emphred{  \pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}   } \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
%     % \\ \underbrace{a}_{b}
% \end{align}
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}, \tg{\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)}}\Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vpsi}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
% \end{align}
% which can be equivalently written in the \emph{regret minimization form}, and we have:








% \begin{defn}[Evolving Alignment]
% Evolving Alignment describes the optimization process of the prompt distribution $\pi_{\vphi}(\rvx)$ and response policy $\pi_{\vtheta}(\rvy \mid \rvx)$ for alignment improvement with regard to the target distribution $\pi_{\text{target}}(\rvx)$.
% \end{defn}





% We propose a new objective:
% \begin{align}
% &\quad \max _{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] - \beta \cdot \sD_{\text{KL}}\Bigr[\textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{black}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{cred}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\Bigr],
% \end{align} 



\subsection{The Mechanism: Asymmetric Self-Play \emph{via} the Creator v.s. Solver Game}~\label{sec:mechanism}
% \notes{TODO: add explanation texts on how we could optimize this through alternating optimization, which naturally gives rise to the asymmetric self-play view.}
\hspace{-6pt}\textbf{Motivation.}\quad  It is challenging to directly optimize the objective in Eq.~\ref{eq:rlhf-joint-}, due to (i) the \textbf{intractability} of the unspecified target environment~\citep{paired}; (ii) the \textbf{instability} of joint differentiable optimization~\citep{gan}. We hereby propose an \textit{alternating optimization} solution by formulating evolving alignment as an asymmetric game between a creator and the solver. Mathematically, this is similar to RL optimization based on expectation-maximization~\citep{hinton-em, rest_em}, where the parameter $\vphi$ for the prompt distribution is fixed at each step.


% Instead of directly optimizing Eq.~\ref{eq:rlhf-joint}, we seek to optimize the performance in the worst-case scenario.  

% This motivate us to formulate the above self-improving alignment problem as an asymmetric self-play game with the minimax regret objective.



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.48\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
% \end{figure}


% \subsubsection{The High Level: {Solver v.s. Creator}}\label{sec:high-level}
% \notes{In preliminaries, discuss the regret-based preference learning paradigm~\citep{cpl,regret-knox,regret-knox-0,open-problems}.}
% \notes{The upcoming subsections still needs lots of re-writing.}

% To start with, we first define the regret of a policy with regard to a prompt as follows\footnote{For simplicity, we here omit the KL divergence term and present a detailed discussion in Section~\ref{sec:int-dpo}.}:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi)=\max _{\pi^{\prime} \in \Pi_{\calX}}\Bigr[\ r\left(\rvx, \pi^{\prime}\right)-r(\rvx, \pi) \ \Bigr]
% \end{align}

% Instead of directly optimize for~\ref{eq:rlhf-joint}, we seek a minimax regret objective.

\textbf{Formalization.}\quad We formalize the alternating optimization as an asymmetric game as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\emphredd{\text{\bf \tc{Creator}}}$ \hspace{+1pt}: the prompt player \textcolor{cred}{$\emphredd{\pi_\calX}$} that generates prompts for the solver to solve.
    \item  $\emphgreenn{\text{\bf \tg{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}}$ \hspace{+1pt}: the response player \textcolor{cgreen}{$\emphgreenn{\pi_{\calY \mid \calX}}$} (denoted as \textcolor{cgreen}{$\pi$} occasionally for simplicity).
    % , whose goal is to identify areas where the solver can improve and propose increasingly informative prompts for the solver to learn.
\end{itemize}

 
% Note the regularized \emph{reward maximization} in Eq.~\ref{eq:rlhf-cls} can be cast as \emph{regret minimization}~\citep{rl-maxent}.

We now illustrate objectives for both players. A proper goal for the \tg{solver} is to minimize regret~\citep{cpl}, \ie the difference in the reward of the current policy and the optimal policy:
\begin{align}
    \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr].\label{eq:regret-pi}
\end{align}


Similar to unsupervised environment design~\citep{accel}, the \tc{creator} agent seeks to produce a series of prompt distributions that form a curriculum for the solver agent to improve its generalization across the vast target prompt distribution space and to solve even harder problems unseen in the initial distribution. This is often characterized by maximizing the regret for the solver,
which leads to the following result~\citep{cpl,regret-knox,regret-knox-0,open-problems}:
\vspace{+1pt}
\begin{mdframed}
\begin{rem}[Minimax Regret]
    If the solver-creator game reaches an equilibrium, the solver follows a minimax regret strategy, \ie it can produce preferred responses in all scenarios:
\begin{align}
    \textcolor{cgreen}{\pi^{\star}} \in \arg \min _{\tg{\pi \in \Pi_{\calY | \calX}}} \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}}  \ \mathbb{E} _{\tc{\rvx \sim \pi_{\calX}}}\Bigr[\ \operatorname{Regret}(\rvx, \tg{\pi}) \ \Bigr].\label{eq:minimax-regret}
\end{align}
\end{rem}
\end{mdframed}

% \begin{mdframed}
% \begin{rem}
%     When the solver-creator game reaches a Nash equilibrium, the solver follows a minimax regret strategy, \ie it is able to generate preferred responses for all solvable prompts.
% \begin{align}
%     \left(\textcolor{cgreen}{\pi^{\star}}, \textcolor{cred}{\pi_{\mathcal{X}}^{\star}}\right) \in \arg \min _{\tg{\pi \in \Pi_{\calY | \calX}}} \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}}  \ \mathbb{E} _{\tc{\rvx \sim \pi_{\calX}}}\Bigr[\ \operatorname{Regret}(\rvx, \tg{\pi}) \ \Bigr].\label{eq:minimax-regret}
% \end{align}
% \end{rem}
% \end{mdframed}


% \begin{align}
%     \left( \textcolor{cred}{\pi_{\mathcal{X}}^{\star}}, \textcolor{cgreen}{\pi^{\star}}\right) \in \arg \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}} \min _{\tg{\pi \in \Pi}} \ \mathbb{E}_{\tc{\rvx \sim \pi_{\calX}}}\left[\operatorname{Regret}(\rvx, \tg{\pi})\right]
% \end{align}


% TODO: change the sequence and add the KL terms


% \subsubsection{The low Level: Solver v.s. Solver}\label{sec:low-level}
% Without direct access to the optimal policy, we choose to approximate the regret via the value obtained by two competing solvers: 
% \begin{align}
% \left(\tg{\pi^{\star}}, \tg{\pi^{\prime\star}}\right)=\arg \max _{\pi \in \Pi} \min _{\pi^{\prime} \in \Pi^{\prime}} \mathbb{E}_{\rvx\sim \mathcal{X}}\left[\mathbb{E}_{\rvy \sim \pi(\cdot \mid \mathbf{x}), \rvy^{\prime} \sim \pi^{\prime}(\cdot \mid \rvx)} \left[\mathbb{P}\left(\rvy \succ \rvy^{\prime} \mid \rvx\right)\right]\right]
% \end{align}

% \notes{We might need to revise this to make it more aligned with our setting; \ie sample multiple responses (actions), then using the reward discrepancy between the best and the worst (or the average) as the \emph{regret proxy}.}

% \subsubsection{Putting Together: The Dual Minimax Regret and Automatic Curricular}
% The overall objective can thus be expressed as:
% \begin{align}
%     \left(\tc{\pi_{\mathcal{X}}^{\star}}, \tg{\pi^{\star}}, \tg{\pi^{\prime \star}}\right)=\arg \max _{\pi_{\mathcal{X}} \in \Pi_{\mathcal{X}}} \max _{\pi \in \Pi} \min _{\pi^{\prime} \in \Pi^{\prime}} \mathbb{E}_{\rvx \sim \pi_{\mathcal{X}}}\left[\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \rvx\right)\right]
% \end{align}


Without access to the true optimal policy, we must approximate the regret. We choose to use variants of advantage functions for the approximation, as shown in Table~\ref{tab:info-metric}, which we also refer as the informativeness proxy\footnote{Note that some works~\citep{plr,active-pl} had tested using Shannon entropy as the informativeness metric, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage more future studies into this.}, with $A^{\star}_{\min}$ as the default proxy due to its relation to minimax regret in Eq.~\ref{eq:minimax-regret}.
\vspace{+1pt}
\begin{mdframed}
\begin{defn}[Informativeness Proxy]
    We use the minimax regret as the proxy for the informativeness metric of the prompt, approximated by the (absolute) worst-case optimal advantage:
\begin{align}
    \text{info}(\rvx) \gets A_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | 
\end{align}
\end{defn}
\end{mdframed}


To calculate the empirical value of $A^{\star}_{\min}$ for  each prompt, we first sample multiple responses from the prompt, where we label each response with its reward, then we use the difference between the highest reward $r_{\max}$ and the lowest reward $r_{\min}$ to represent the informativeness proxy. This proxy enjoys many nice properties, which we present an in-depth discussion in $\S$~\ref{sec:int}.


\subsection{The Practical Algorithm}~\label{sec:algo}
\hspace{-6pt}Next, we illustrate \method~of Algorithm~\ref{alg:i-eva} in details, with  implementation specifications in Appendix~\ref{app:settings}.

The full pipeline is that we combine the creator and solver step in an iterative preference optimization pipeline.

\subsubsection{\tb{\emphtextred{The Creator Step}}:  Estimate, Sample then Evolve}\label{sec:creator-step}
\textbf{Intuition.}\quad We find prompts with the most learning potential and generatively evolve them. This is similar to curriculum RL~\citep{accel} which finds environments with high-regret levels and edit within some distance, or the evolution strategies~\citep{schwefel1977evolutionsstrategien} which find the most promising species then mutate and crossover. As in Section~\ref{sec:mechanism}, we do not seek a differentiable creator for optimization in this work. The creator is implemented in three steps as in Figure~\ref{fig:pipeline}. 
\vspace{-5pt}

% \textbf{$\emphgray{\texttt{sample}(\cdot)}$ -- weighted sampling for an informative subset.}
% We then sample a prompt set with high learning potential. This is achieved by weighted sampling using the informativeness metric as the weight.

% \textbf{$\emphgray{\texttt{evolve}(\cdot)}$ -- evolving for a proximal region of high-advantage prompts.}

% This gives a simple heuristic: sampling multiple responses from the LLM, then using the maximal reward minus the minimal reward, $r_{\max} - r_{\min}$ as the reward for the creator, thus incentivizing the creator to generate more such prompts.

\paragraph{Step 1: $\emphgray{\texttt{\small info}(\cdot)}$ -- estimate the informativeness.} For each prompt $\rvx$ in the initial prompt set $\calX_t$, we generate responses, annotate rewards and calculate a informativeness metric to $\rvx$ as in Table~\ref{tab:info-metric}.\vspace{-3pt}

\paragraph{Step 2: $\emphgray{\texttt{\small sample}(\cdot)}$ -- weighted sampling for an informative subset.} Using the informativeness metric as the weight,
we sample a smaller informative prompt set $\calX_t^{\texttt{\tiny info}}$ (\eg 20\% of the original). \vspace{-3pt}

\paragraph{Step 3: $\emphgray{\texttt{\small evolve}(\cdot)}$ -- evolving for a proximal region of high-advantage prompts.} Our method does not rely on any specific evolving method. We take \text{EvolInstruct}~\citep{wizardlm} as an off-the-shelf baseline evolving method, which conducts in-depth (\ie, adding constraints, deepening, concretising, complicating) and in-breadth evolving (\ie mutation) by meta-instruction (\ie using an LLM to re-write the original prompts with the aforementioned evolving directions). Specifically, we iterate over each prompt in the $\calX_t^{\texttt{\tiny info}}$, where each prompt is evolved to multiple (\eg 4) variations, then mix the newly generated prompts with a uniformly sampled buffer from $\calX_t$ to create $\calX_{t+1}$.


\subsubsection{\tb{\emphtextgreen{The Solver Step}}: Solve then Optimize}
This step is the classical preference optimization algorithm~\citep{dpo,simpo}, where responses are generated and the gradient descent is performed, as shown in Algorithm~\ref{alg:i-eva}.



% \paragraph{Further Interpretations on the Informativeness Proxy.} \tc{[Discuss further interpretations.]}
\subsection{Further Interpretation on the Informativeness Proxy}\label{sec:int}
\tc{An important contribution of our work is proposing the metric for preference optimization; so worth having a subsection somewhere on this.}
\paragraph{Learning potential.} Finding the prompts where the agent is weak, but still solvable.

\paragraph{Worst-case guarantees.}

\paragraph{Auto-curricula for the creator.}
the advantage can be generalized as the reward difference between a base solver and a reference solver, where the creator is incentivized to produce new prompts that are just out of the comfort zone of solvers~\citep{zone-promximal}:
\vspace{-4pt}
\begin{itemize}
    \item For very complex prompts, both solutions may perform poorly, leading to low regret proxy.\vspace{-2pt}
    \item For very simple prompts, the base solution already performs well, giving low regret proxy.\vspace{-2pt}
    \item The optimal strategy is to find prompts that are just beyond the solvers’ current capability.
\end{itemize}


\paragraph{Auto-curricula for the \textnormal{\textit{contrastive}} solver.} 
Another nice property of our informativeness metric (\eg $A^{\star}_{\min}$) is that it matches the curriculum learning property with the DPO loss. In the specific case of contrastive preference optimization~\citep{cpl,dpo}, the loss is monotonically smaller as $\bdlog$ gets larger. This justifies our use of $r_{\max} - r_{\min}$ as the informativeness metric to prioritize the training examples according to the curriculum learning literature~\citep{easy-bengio2009curriculum}\footnote{We follow the curriculum learning literature that prioritizes examples with smaller losses for improvement in convergence and generalization. There is another line of work in optimization that claims examples with higher losses should be prioritized~\citep{hard-losers,hard-obs,hard-osgd,ordered-sgd}; however, \cite{rho-loss} conjecture that those example are often noisy (not learnable) or irrelevant thus are impractical. Our empirical results in Section~\ref{sec:ab-metric} on confirms this.}, which is essentially the reward of the chosen response ($r_{\max}$) minus the reward of the rejected response ($r_{\min}$), that is:
\begin{align}
    \emphgray{A^{\star}_{\min}(\rvx)}  = \beta \cdot \textcolor{black}{\emphgray{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}}}  \ \approx \ \emphgray{r_{\max} - r_{\min}}.
\end{align}
In this way, we incentivize the creator to generate prompts that \emph{bring the most contrastive responses}\footnote{One direction that worth to explore could be to directly use $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ instead of the reward proxy.}, that improves the convergence and generalization of the solver, formalized as below:
\begin{hypo}[Contrastive Curriculum Hypothesis]
    In direct preference optimization, prioritizing prompts w/ \emph{higher contrastive ratio} improves sample efficiency and generalization.
\end{hypo}




% \begin{itemize}
%     \item \textbf{Worst-case guarantee} for generally capable agents:
%     \item \textbf{Curriculum effect for the creator}: This is analogous to the solver \emph{v.s.} solver game~\citep{paired,dcd}, where the advantage can be generalized as the reward difference between a base solver and a reference solver. This naturally induce a curriculum effect, where the creator is incentivized to produce new prompts that are just out of the comfort zone of the solver~\citep{zone-promximal}.
%     \item \textbf{Curriculum effect for the solver}: 
%     \item \textbf{Learning potential}:
% \end{itemize}

% \notes{Maybe move the interpretation on the informativeness metric upward here. including: (i) \textbf{worst-case guarantee} for generally capable agents; (ii) \textbf{curriculum effect for the creator}; (iii) \textbf{curriculum effect for the contrastive solver}; (iv) learning potential. }














% \subsection{Further Interpretation via Contrastive Preference Optimization}\label{sec:int-dpo}

% \textcolor{red}{[How do compute rmax and rmin in practice? This needs to be explained more clearly.]}

% \textcolor{red}{[More time needs to be spent on explaining how the informativeness measure is computed in practice and how the prompts are evolved. Those are the two major steps in the algorithm and it is quite important for readability and reproducibility that the presentation focuses on those.]}





% -------------------------

% \subsubsection{Further Interpretation from Continual Deep Learning}\label{sec:int-cont}
% {\color{red} RA.9.26: This sounds like a para for related work possibly along with the footnote}


% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------
% , which accelerates the learning.

% \footnote{While we may directly select data with $\bdlog$, the usage of $r_{\max} - r_{\min}$ provides a fast approximation to the empirical contrastive ratio.}.



% \footnote{This presents another message on adaptively adjusting the , we should adaptively choose the informativeness metric when we use different optimization algorithms.}




% The overall objective can be expressed as:
% \begin{align}
%     (\emphtactic{\pi_\mathcal{X}^\star}, \emphgoal{\pi^{\prime\star}}, \emphgoal{\pi^{\star}}) \in \arg \emphtactic{\max_{\pi_\mathcal{X} \in \Pi_\mathcal{X}}} \ \emphgoal{\max_{\pi^{\prime} \in \Pi^{\prime}}} \ \emphgoal{\min_{\pi \in \Pi}} \ \mathbb{E}_{\vx \sim \pi_\mathcal{X}} \left[ \emphgold{\mathbb{P}\left(\pi^{\prime} \succ \pi \mid \vx \right)} \right].
% \end{align}

% TODO: introducing the new loss design. We may leave this as a theoretical version.

% \subsubsection{The New Loss Design}
% (TODO: make this general then use different inner-loop derivation)
% \begin{align}
%     \nabla_\theta \mathcal{L}\left(\pi_\theta ; \pi_{\text {ref}}\right)= 
%     -\beta \mathbb{E}_{\rvx \sim \pi_\theta(\rvx), (\rvy_w, \rvy_l) \sim \pi_\theta(\rvy|\rvx)}[&\sigma\left(\hat{r}_\theta\left(\rvx, \rvy_l\right)-\hat{r}_\theta\left(\rvx, \rvy_w\right)\right) \nonumber \\
%     &[\nabla_\theta \log \pi_\theta(\rvx) + \nabla_\theta \log \pi_\theta\left(\rvy_w \mid \rvx\right)-\nabla_\theta \log \pi_\theta\left(\rvy_l \mid \rvx\right)]]. \nonumber
% \end{align}


% \begin{figure}[H]
% \centering
% \begin{minipage}{0.46\textwidth}
%     \includegraphics[width=\textwidth]{texs_/mechanism.png}
%     \caption{\text{The creator step of Algorithm~\ref{alg:i-eva}.} }
%     \label{fig:mechanism}
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\textwidth} 
% In Algorithm~\ref{alg:i-eva}, we illustrate a practical algorithm for~\method. Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{simpo}.
% \end{minipage}
% \end{figure}
% \vspace{-10pt}


% Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{simpo}.



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.48\linewidth]{texs_/mechanism.png}
%     \caption{\text{The creator step of Algorithm~\ref{alg:i-eva}.} }
%     \label{fig:mechanism}
% \end{figure}

% We illustrate a practical algorithm for~\method~in Algorithm~\ref{alg:i-eva}. We introduce an additional \text{\tc{creator step}} for  an evolving prompt distribution during preference optimization, which can be plugged on top of any alignment algorithms (which can be seen come with only the \tg{solver step} that generates responses.).

% \newpage
% \notes{Re-writing this part to make the evolving part more clear. Essentially, this is a bit like~\citep{accel}, which we make edits at the proximal region of the prompts which have high learning potential.}
% As shown in Fig~\ref{fig:pipeline}, the \tc{creator step} can be practically implemented by three steps:
% \begin{enumerate}
%     \item \textbf{Estimate} the informativeness for each prompt.

%     \begin{itemize}
%         \item Under the minimax regret game, we use the worst-case optimal advantage for each prompt $\rvx$, that is $\widehat{A}^{\star}_{\min}(\rvx)=r_{\max}(\rvx)-r_{\min}(\rvx)$, to measure their informativeness.
%     \end{itemize}
    
%     \item \textbf{Sample} an subset of prompts by the informativeness weight.
    
%     \item \textbf{Evolve} a new prompt set from the subset, mix with a buffer of the seed prompts.
% \end{enumerate}

% \notes{Add a table or color code to illustrate the difference from existing works.}

% \subsection{The Informativeness Measure by Reward Models}
% The non-trivial part here is leveraging the reward model to elicit informativeness of prompts.

% \subsubsection{\textnormal{\textbf{\texttt{eva-i}}}: The Iterative Off-Policy EVA Algorithm}\label{sec:eva-i}

% For simplicity, we remove subscripts and the superscripts for sets.
% We introduce an additional creator step that can be plugged into any alignment algorithms.

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% % -------------------------------------------
% \subsection{The Practical Algorithm}~\label{sec:algo}
% \hspace{-6pt}In Algorithm~\ref{alg:i-eva}, we illustrate a simple practical algorithm for~\method, where the details of $\texttt{info}(\cdot)$, $\texttt{sample}(\cdot)$ and $\texttt{evolve}(\cdot)$ are shown in Section~\ref{sec:creator-step}.  We use iterative off-policy (\method\texttt{\textbf{-i}}) training as our baseline setting, which is popularly adopted in recent works~\citep{dpo-iterative,snorkel,self-play-gu}. In this setup, the prompt set $\calX$ represents the full or a partition of the full dataset, with each iteration corresponding to a complete pass over this set\footnote{Our algorithm can be easily made on-policy, where the prompt set $\calX_t$ is essentially a mini-batch or a mini-pool (from which we sample mini-batches). We present the algorithm in Appendix~\ref{app:eva-o}.}.
% % ------------------------------------

% {
% \noindent
% \centering
% \begin{minipage}{.8\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
%     % , sample size of responses per prompt $n$ 
%     \Statex

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{{creator step}}}
%         \State \tb{\emph{self-generate responses}:} \hspace{+25pt}\tb{$\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ }
%         %\Comment{self-generate $\rvy$}
%         % \vspace{+2.5pt}
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$
%         \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{ ({\vy^{(j)}_i}, {r^{(j)}_i})\}$}

%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}\}$} 
%         %\Comment{annotate reward}
%         % \vspace{+0.1pt}
        
%         \vspace{+5pt}
%         \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \calX_t \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}$ 
        
%         % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \{(\rvx_i, \tb{\texttt{info}(\rvx_i)}\}$ 
%         % where $\texttt{info}_i = f(\calD_{t}[i])$ 
%         %\Comment{estimate information}
%         \vspace{+2pt}
        

%         \Statex \hspace{+11pt}  \tb{\emph{sample subset}:} \hspace{+60pt}$\calX_{t}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t})}$ 
%         %\Comment{sample the informative subset}
%         \vspace{+2.5pt}

%         \Statex \hspace{+11pt} \tb{\emph{self-evolve prompts}:} \hspace{+40pt}$\mathcal{X}_{t}^{\prime} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t}^{\texttt{info}})}$ 
%         %\Comment{self-evolve $\rvx$}

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
        
%         \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}^{\prime}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 
%         %\Comment{self-generate $\rvy$}
        
%         \Statex \hspace{+11pt} \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t}^{\prime} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 
%         %\Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \vspace{+2.5pt}
        
%         \State \tb{\emph{preference optimization}:}$ \hspace{+32pt} \boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})$ 
%         %\Comment{preference optimization}

%         \Statex

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }


% It is easy to see that this algorithm can be made on-policy, or off-policy (which is faster). To illustrate:
% \vspace{-5pt}
% \begin{itemize}
%     \item \texttt{eva-o}: for the on-policy version, the seed prompt set $\calX_t$ is essentially a mini-batch or a mini-pool (from which we sample mini-batches), and each episode is one optimization step.

    
%     \item \texttt{eva-i}: for the off-policy version, the seed prompt set is the full dataset; and each episode is one full iteration over the dataset, containing multiple optimization steps.\vspace{-5pt}
%     %This resembles~\citep{dpo-iterative}.
% \end{itemize}
% By removing the creator step, we can recover the classical  (iterative) preference optimization algorithm~\citep{cringe,snorkel,dpo-iterative}.



% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Iterative \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-i})}} }\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State $\forall$ $\vx_i \in \mathcal{X}_{t-1}$,  sample $\{{\vy^{(j)}_i}\}^{n}_{j=1} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ \Comment{self-generate $\rvy$}
%         % \vspace{+2.5pt}
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$

%         \State $\mathcal{D}_{t-1} \gets \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{n}_{j=1}\}_{i = 1 }^{|\calX_{t-1}|}$ \Comment{annotate reward}
%         % \vspace{+0.1pt}

%         \Statex \hspace{+11pt} $\calI_{t-1} \gets \{(\rvx_i, \texttt{info}_i)\}_{i = 1 }^{|\calX_{t-1}|}$ where $\texttt{info}_i = f(\calD_{t-1}[i])$ \Comment{estimate information}
%         \vspace{+2.5pt}

%         \State $\calX_{t-1}^{\texttt{info}} \gets \textsc{Sample}(\mathcal{X}_{t-1} \mid \calI_{t-1})$ \Comment{sample the informative subset}

%         \Statex \hspace{+11pt} $\mathcal{X}_{t} \leftarrow \textsc{Evolve}(\calX_{t-1}^{\texttt{info}})$ \Comment{self-evolve $\rvx$}

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{X}_{t}$,  sample $\{{\vy^{(j)}_i}\}^{n}_{j=1} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ \Comment{self-generate $\rvy$}
%         \State  $\mathcal{D}_{t} \gets \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{n}_{j=1}\}_{i \in |\calX_{t}|}$ \Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \State $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calD_t}(\boldsymbol{\theta})$ \Comment{preference optimization}

%         \Statex

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: The On-Policy EVA Algorithm}\label{sec:eva-o}
% % ~\citep{ordered-sgd}
% % Naïvely, this can also be considered as a variant of ordered gradient descent with generative data augmentation. At each step, we first uniformly select a pool (e,g., with 8 examples) from the original; then form a subset (e.g., with 2 examples) and evolve a new batch (e.g., each evolving 2), then train with 2 (top original) + 2 (random original) + 4 (evolved). In this way, we create an online data curriculum with newly generated data. 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}_i\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \textsc{Evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }



% \newpage
% \section{\textcolor{Gray}{[1\% Draft]} Method}


% % Essentially there are two 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, preference oracle $\mathbb{P}$, learning rate $\eta$, number of generated samples $K$, initial prompt set $\mathcal{X}_0$
%     \Statex

%     \For{$t = 0, 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{prepare the training dataset}
%         \State for all $\vx_i \in \mathcal{X}_t$,  sample $\{{\vy^{(j)}_i}\}^{K}_{j=1} \sim \pi_{\vtheta_t}(\cdot \mid \mathbf{x})$
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$

%         \State annotate the preference and form the dataset $\mathcal{D}_t = \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{K}_{j=1}\}_{i \in [N]}$

%         \Statex
        
%         \LineComment{update policy (any other loss can be plug-in as well)}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$

%         \Statex
        
%         \LineComment{evolve the prompt distribution from learned metric}
%         \State $\calI_t(\mathbf{x}) \leftarrow \textsc{Assess}(\pi_{\vtheta_{t+1}}, \mathbf{x})$, $\forall \mathbf{x} \in \mathcal{X}_t$
        
%         \State $S_t \leftarrow \textsc{Evolve}(\pi_{\vtheta_{t+1}}, \calI_t, \mathcal{X}_t)$
        
%         \State $\mathcal{X}_{t+1} \leftarrow \textsc{Update}(\mathcal{X}_t, S_t)$

%         \Statex
%     \EndFor
%     \State \Return Final policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }

% % \subsection{Regret and Minimax Framework}

% % Our goal is to design a self-improving agent that continually expands its capabilities through generative exploration. We formulate this using a minimax regret objective, which provides performance guarantees across an evolving distribution of prompts.

% % Let $\mathcal{X}$ be the space of prompts, $\mathcal{Y}$ the space of responses, and $\Pi$ the space of policies. We define regret as:

% % \begin{align}
% %     \text{Regret}(\vx, \pi) &= \max_{\pi^\star \in \Pi} [V(\vx, \pi^\star) - V(\vx, \pi)]
% % \end{align}

% % where $V(\vx, \pi) = \mathbb{E}_{\vy \sim \pi(\cdot \mid \vx)}[r(\vx, \vy)]$ is the value function, with $r(\vx, \vy)$ being the reward for response $\vy$ to prompt $\vx$. This formulation quantifies the difference in performance between a given policy $\pi$ and the best possible policy $\pi^\star$ for a given prompt $\vx$.

% % We then introduce a prompt player $\pi_X: \mathcal{H} \rightarrow \Delta(\mathcal{X})$, where $\mathcal{H}$ represents the interaction history. The minimax regret objective is:

% % \begin{align}
% %     J^\star &= \min_{\pi \in \Pi} \max_{\pi_X} \mathbb{E}_{\vx \sim \pi_X} [\text{Regret}(\vx, \pi)]
% % \end{align}

% % This formulation aims to find a policy $\pi$ that minimizes the worst-case regret across all possible prompt distributions. At equilibrium, this guarantees that the chosen policy $\pi$ performs robustly across the entire prompt space $\mathcal{X}$.

% % \subsection{Proxy for Regret Computation}

% % Computing the regret directly is infeasible as we lack access to the optimal policy $\pi^\star$. We therefore introduce a proxy using two policies: a base policy $\pi$ and an improvement policy $\pi_\dagger$. The regret proxy is defined as:

% % \begin{align}
% %     \text{Regret}_\text{proxy}(\vx, \pi, \pi_\dagger) = \max_{\pi_\dagger} \min_\pi [\emphgoal{p(\vy_2 \succ \vy_1 \mid \vx)} - \beta D_\text{KL}(\pi_\dagger \parallel \pi_\text{ref} \mid \vy_1, \vx) + \beta D_\text{KL}(\pi \parallel \pi_\text{ref} \mid \vx)] \nonumber
% % \end{align}

% % where $\vy_1 \sim \pi(\cdot \mid \vx)$, $\vy_2 \sim \pi_\dagger(\cdot \mid \vy_1, \vx)$, and $p(\vy_2 \succ \vy_1 \mid \vx)$ is the probability that $\vy_2$ is preferred to $\vy_1$ given $\vx$.

% % This proxy serves as an approximation of the true regret for several reasons:

% % \begin{itemize}
% %     \item The term $p(\vy_2 \succ \vy_1 \mid \vx)$ captures the improvement of $\pi_\dagger$ over $\pi$, analogous to the value difference in the true regret.
% %     \item The KL divergence terms encourage exploration of the policy space while maintaining proximity to a reference policy, mimicking the search for the optimal policy in the true regret.
% %     \item The max-min formulation reflects the adversarial nature of finding the largest possible improvement, similar to finding the optimal policy in the true regret.
% % \end{itemize}

% \subsection{Combined Objective}

% Incorporating this proxy into our original objective, we obtain:

% \begin{align}
%     J^\star = \min_\pi \max_{\pi_\dagger} \min_{\pi_X} \mathbb{E}_{\vx \sim \pi_X, \vy_1 \sim \pi, \vy_2 \sim \pi_\dagger} [\text{Regret}_\text{proxy}(\vx, \pi, \pi_\dagger)]
% \end{align}

% \subsection{Curriculum Effect}

% This formulation naturally induces a curriculum effect. The prompt player $\pi_X$ is incentivized to generate prompts that maximize the regret proxy, leading to a progression of challenges:

% \begin{itemize}
%     \item For prompts where $\pi$ performs poorly but $\pi_\dagger$ can improve, $p(\vy_2 \succ \vy_1 \mid \vx)$ will be high, increasing the regret proxy.
%     \item The KL divergence term $D_\text{KL}(\pi \parallel \pi_\text{ref} \mid \vx)$ will be larger for prompts that challenge $\pi$, further increasing the regret proxy.
%     \item As $\pi$ improves on certain prompts, $\pi_X$ must generate new, more challenging prompts to maintain a high regret proxy.
% \end{itemize}

% This mechanism ensures that $\pi_X$ continuously generates prompts just out of the comfort zone of $\pi$'s capabilities. The regret proxy is maximized when $\pi_X$ generates the simplest prompts that $\pi$ cannot yet solve but $\pi_\dagger$ can improve upon:

% \begin{itemize}
%     \item For very complex prompts, both $\pi$ and $\pi_\dagger$ may perform poorly, leading to low $p(\vy_2 \succ \vy_1 \mid \vx)$ and thus low regret proxy.
%     \item For very simple prompts, $\pi$ may already perform well, again leading to low regret proxy.
%     \item The optimal strategy for $\pi_X$ is to find prompts just beyond $\pi$'s current capabilities, where $\pi_\dagger$ can still demonstrate improvement.
% \end{itemize}

% This property ensures a smooth progression of the curriculum, always challenging $\pi$ with prompts that are neither too easy nor impossibly difficult.


% % As a naive baseline, we can use the preference advantage to evaluate the value of the prompt. We can set a threshold to select the prompts.

% % Next, we can adopt a combination of different practical prompting methods to grow the chosen prompt set:
% % \begin{itemize}
% %     \item Contrastive prompting
% %     \item Interpolating prompting
% %     \item Extrapolating prompting
% %     \item Adversarial prompting (like the camel paper)
% % \end{itemize}

% % \notes{TODO: provide concrete examples; check literature on similar synthetic data generation works.}

% % \notes{As an ablation study, we can add adversarial training loss in the original loss.}

% % One relevant baseline could be EvoPrompt~\citep{evoprompt}.

% % Essentially this is just like evolutionary algorithms as it is about population optimization. However, we don't need to confine ourselves in the rigid setting of classical evolution strategies.


% \newpage

% IGNORE THE OLD STUFFS

% \textbf{Stackelberg Game Formulation for Self-Improving Language Models}

% \begin{enumerate}
%     \item \textbf{Players:}
%     \begin{itemize}
%         \item Prompt Player: $$\textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)}$$
%         \item Response Player: $$\textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')}$$
%     \end{itemize}

%     \item \textbf{Definitions:}
%     \begin{itemize}
%         \item $\rvx \in \mathcal{X}$: Base prompts from a distribution $\mathcal{X}$
%         \item $\rvx' \in \mathcal{X}'$: Generated prompts
%         \item $\rvy \in \mathcal{Y}$: Responses
%         \item $\rvh \in \mathcal{H}$: Historical information
%         \item $\vtheta \in \Theta$: Shared parameters of the prompt and response generators
%     \end{itemize}

%     \item \textbf{Objective Functions:}
%     \begin{equation*}
%     \overbrace{\max_{\vtheta} \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}}}})}^{\text{prompt player}}, \qquad 
%     \overbrace{\max_{\vtheta} \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}}^{\text{response player}}
%     \end{equation*}
    
%     where
%     \begin{align*}
%        \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}, \rvy\sim p^{\text{response}}_{\vtheta}}\left[D(\rvx', \rvx) + \lambda U(\rvx', \vtheta)\right] \\
%         \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}}\left[R(p^{\text{response}}_{\vtheta}(\cdot \mid \rvx'), \rvx')\right]
%     \end{align*}

%     And:
%     \begin{itemize}
%         \item $D: \mathcal{X}' \times \mathcal{X} \to \mathbb{R}_+$ is a diversity measure
%         \item $U: \mathcal{X}' \times \Theta \to \mathbb{R}_+$ is an uncertainty measure
%         \item $R: (\mathcal{Y} \to [0,1]) \times \mathcal{X}' \to \mathbb{R}$ is a reward function
%         \item $\lambda \in \mathbb{R}_+$ is a hyperparameter
%     \end{itemize}

%     \item \textbf{Game Formulation:}
%     \begin{align*}
%         &\vtheta^\star = \arg\max_{\vtheta}\emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} \\
%         \text{s.t. } &\vtheta \in \arg\max_{\vtheta'} \ \   \emphgoal{J_R(\vtheta', \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}
%     \end{align*}

%     \item \textbf{Induced Distributions:}
%     \begin{align*}
%         \mu_{\vtheta}(\rvx', \rvy) &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \cdot \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')} \ \right] \\
%         \nu_{\vtheta}(\rvx') &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \ \right]
%     \end{align*}
% \end{enumerate}

% \textbf{Game Formulation Explanation:}

% The Stackelberg game formulation captures the interaction between the prompt generator (leader) and the response generator (follower). The prompt generator aims to maximize $J_P$, which encourages the generation of diverse and uncertain prompts. The response generator, in turn, maximizes $J_R$, which rewards high-quality responses to the generated prompts.

% % The game is asymmetric, with the prompt generator acting first. This allows the prompt generator to anticipate the response generator's behavior and generate prompts that will lead to overall improvement in the language model's capabilities.

% The constraint $\vtheta \in \arg\max_{\vtheta'} J_R(\vtheta', p^{\text{prompt}}_{\vtheta})$ ensures that the response generator is optimal with respect to the current prompt distribution. This captures the idea that the response generator quickly adapts to the prompts generated by the prompt generator.

% \textbf{Induced Distributions Explanation:}

% The induced distributions $\mu_{\vtheta}$ and $\nu_{\vtheta}$ characterize the behavior of the language model under the current parameters $\vtheta$:

% 1. $\mu_{\vtheta}(\rvx', \rvy)$ is the joint distribution of generated prompts and responses. It captures the overall behavior of the language model, including both prompt generation and response generation.

% 2. $\nu_{\vtheta}(\rvx')$ is the marginal distribution of generated prompts. This distribution is crucial for understanding the diversity and coverage of the prompt space achieved by the prompt generator.

% % These distributions play a key role in analyzing the equilibrium properties of the game and in proving theoretical guarantees about the language model's performance.
% \newpage

% \textbf{Equilibrium Properties and Theoretical Guarantees}

% \begin{itemize}
%     \setcounter{enumi}{5}
%     \item \textbf{Stackelberg Equilibrium:}
%     A Stackelberg equilibrium $\vtheta^\star$ satisfies:
%     \begin{align*}
%         \vtheta^\star &\in \arg\max_{\vtheta} J_P(\vtheta, \textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}) \\
%         \vtheta^\star &\in \arg\max_{\vtheta} J_R(\vtheta, \textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}})
%     \end{align*}

%     At this equilibrium:
%     \begin{enumerate}
%         \item $\textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}}$ generates diverse prompts that effectively explore the prompt space and target areas of model uncertainty.
%         \item $\textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}$ produces high-quality responses across the range of generated prompts.
%     \end{enumerate}

%     \item \textbf{Theorem (Performance Guarantee):} 
%     At the Stackelberg equilibrium $\vtheta^\star$:
%     \begin{equation*}
%         \mathbb{E}_{\rvx'\sim\nu_{\vtheta^\star}}[R(p^{\text{response}}_{\vtheta^\star}(\cdot \mid \rvx'), \rvx')] \geq R^\star - (\varepsilon_D + \varepsilon_U + \varepsilon_T)
%     \end{equation*}

%     Where:
%     \begin{itemize}
%         \item $R^*$ is the optimal achievable reward
%         \item $\varepsilon_D \geq 0$ is the suboptimality in prompt diversity
%         \item $\varepsilon_U \geq 0$ is the suboptimality in uncertainty targeting
%         \item $\varepsilon_T \geq 0$ is a transfer error term
%     \end{itemize}

%     \item \textbf{Proof Sketch:}
%     \begin{enumerate}
%         \item Let $p^{\text{prompt}*}$ and $p^{\text{response}*}$ be the optimal prompt and response generators, respectively.
%         \item By the optimality of $\vtheta^*$ for the response player:
%         \begin{equation*}
%             \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}}_{\vtheta^*}(\cdot \mid \rvx'), \rvx')] \geq \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \varepsilon_R
%         \end{equation*}
%         where $\varepsilon_R \geq 0$ is the suboptimality of the response generator.
        
%         \item The diversity and uncertainty terms in $J_P$ ensure:
%         \begin{equation*}
%             D_{KL}(\nu_{\vtheta^*} \parallel \nu^*) \leq \varepsilon_D + \varepsilon_U
%         \end{equation*}
%         where $\nu^*$ is the optimal prompt distribution and $D_{KL}$ is the Kullback-Leibler divergence.
        
%         \item Using Pinsker's inequality and the properties of the reward function:
%         \begin{equation*}
%             |\mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')]| \leq \varepsilon_T
%         \end{equation*}
        
%         \item Combining these inequalities and noting that $\mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] = R^*$, we obtain the desired result.
%     \end{enumerate}

%     \item \textbf{Corollary (Convergence):}
%     Under mild conditions on the learning dynamics and function approximators, the iterative algorithm converges to a Stackelberg equilibrium as $T \to \infty$.
% \end{itemize}

% \textbf{Stackelberg Game Variants}

% \begin{itemize}
%     \setcounter{enumi}{9}
%     \item \textbf{Prompt as Leader (PaL):} 
%     Choosing the prompt player as leader results in the following optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_P\left(\vtheta, p^{\text{response}*}_{\vtheta}\right) \text{ s.t. } p^{\text{response}*}_{\vtheta} \in \arg \max_{p^{\text{response}}} J_R\left(\vtheta, p^{\text{prompt}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     We solve this nested optimization using the first-order gradient approximation, resulting in updates:
%     \begin{align*}
%     p^{\text{response}}_{k+1} &\approx \arg \max_{p^{\text{response}}} J_R\left(\vtheta_k, p^{\text{prompt}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \alpha_k \nabla_{\vtheta} J_P\left(\vtheta, p^{\text{response}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Response as Leader (RaL):} 
%     Conversely, choosing the response player as leader results in the optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_R\left(\vtheta, p^{\text{prompt}*}_{\vtheta}\right) \text{ s.t. } p^{\text{prompt}*}_{\vtheta} \in \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta, p^{\text{response}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     Similarly, we solve this using the first-order gradient approximation:
%     \begin{align*}
%     p^{\text{prompt}}_{k+1} &\approx \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta_k, p^{\text{response}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \beta_k \nabla_{\vtheta} J_R\left(\vtheta, p^{\text{prompt}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Comparison:} 
%     \begin{itemize}
%         \item PaL prioritizes the generation of diverse and uncertain prompts, potentially leading to more exploratory behavior.
%         \item RaL focuses on optimizing responses, which may result in more stable learning but potentially less exploration.
%         \item The choice between PaL and RaL depends on the specific requirements of the task and the desired balance between exploration and exploitation.
%     \end{itemize}

%     \item \textbf{Convergence Properties:}
%     Under suitable regularity conditions on $J_P$, $J_R$, and the function approximators:
%     \begin{itemize}
%         \item Both PaL and RaL converge to local Stackelberg equilibria as $k \to \infty$.
%         \item The rate of convergence and the quality of the equilibrium may differ between PaL and RaL, depending on the landscape of $J_P$ and $J_R$.
%     \end{itemize}
% \end{itemize}


% \newpage
% \section{Experiments}

% \notes{TODO: add experimental details in this section. In general, we can consider two types of tasks, one is the general alignment task, where the preference comes from human values; the other can be math/coding task, where the preference oracle is the environment, signaling true or false for the correctness.}

% % \section{Evolutionary Prompt Set Optimization}

% % We formulate the problem of evolving the prompt set as a population-based optimization algorithm. Let $\mathcal{X}$ be the space of all possible prompts, and $\mathcal{X}_t \subset \mathcal{X}$ be our prompt set at iteration $t$.

% % \subsection{Fitness Function}

% % Define a fitness function $f: \mathcal{X} \times \Pi \rightarrow \mathbb{R}$, where $\Pi$ is the space of policies. For a prompt $\mathbf{x} \in \mathcal{X}$ and policy $\pi \in \Pi$, $f(\mathbf{x}, \pi)$ measures the "fitness" of $\mathbf{x}$ with respect to $\pi$. This could be defined in various ways, such as:

% % \begin{equation}
% % f(\mathbf{x}, \pi) = \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[\mathbb{P}(\vtau \succ \pi | \mathbf{x})] - \frac{1}{2}
% % \end{equation}

% % where $\mathbb{P}(\vtau \succ \pi | \mathbf{x})$ is the probability that response $\vtau$ is preferred over $\pi$'s typical response to $\mathbf{x}$.

% % \subsection{Population Dynamics}

% % Let $P_t = \{(\mathbf{x}_i, w_i)\}_{i=1}^N$ be the population at time $t$, where $\mathbf{x}_i \in \mathcal{X}_t$ and $w_i \in \mathbb{R}^+$ is a weight associated with $\mathbf{x}_i$. The evolution of the population follows these steps:

% % 1. \textbf{Selection}: Select a subset $S_t \subset P_t$ based on fitness values.
% % 2. \textbf{Variation}: Generate new prompts $V_t$ through mutation and crossover operations on $S_t$.
% % 3. \textbf{Evaluation}: Compute fitness for new prompts in $V_t$.
% % 4. \textbf{Replacement}: Update $P_{t+1}$ by combining $P_t$ and $V_t$.

% % \subsection{Information-Theoretic Approach}

% % We can incorporate information theory to guide the evolution process. Define the information content of a prompt $\mathbf{x}$ with respect to policy $\pi$ as:

% % \begin{equation}
% % I(\mathbf{x}, \pi) = H(\pi(\cdot|\mathbf{x})) - \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[H(\mathbb{P}(\cdot|\mathbf{x}, \vtau))]
% % \end{equation}

% % where $H(\cdot)$ is the Shannon entropy and $\mathbb{P}(\cdot|\mathbf{x}, \vtau)$ is the distribution over preferences given prompt $\mathbf{x}$ and response $\vtau$.

% % We can then define a composite fitness function:

% % \begin{equation}
% % F(\mathbf{x}, \pi) = \alpha f(\mathbf{x}, \pi) + (1-\alpha) I(\mathbf{x}, \pi)
% % \end{equation}

% % where $\alpha \in [0,1]$ balances between preference improvement and information gain.

% % \subsection{Variation Operators}

% % 1. \textbf{Mutation}: For $\mathbf{x} \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \mathbf{x} + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% %    \end{equation}
% %    where $\sigma^2$ is the mutation strength.

% % 2. \textbf{Crossover}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \lambda \mathbf{x}_1 + (1-\lambda) \mathbf{x}_2, \quad \lambda \sim \text{Beta}(a, b)
% %    \end{equation}

% % 3. \textbf{Information Exchange}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$ from different topics, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \textsc{Combine}(\mathbf{x}_1, \mathbf{x}_2)
% %    \end{equation}
% %    where \textsc{Combine} is a function that merges aspects of $\mathbf{x}_1$ and $\mathbf{x}_2$.

% % \subsection{Convergence Analysis}

% % Under certain conditions, we can prove convergence properties of this evolutionary algorithm:

% % \begin{thm}[Convergence of Evolutionary Prompt Optimization]
% % Let $\{\mathcal{X}_t\}_{t=0}^\infty$ be the sequence of prompt sets generated by the evolutionary algorithm. Assume:
% % \begin{enumerate}
% %     \item $f(\mathbf{x}, \pi)$ is continuous in $\mathbf{x}$ for all $\pi \in \Pi$.
% %     \item The variation operators are ergodic.
% %     \item The selection operator retains the best prompt with non-zero probability.
% % \end{enumerate}
% % Then, with probability 1:
% % \begin{equation}
% % \lim_{t \to \infty} \max_{\mathbf{x} \in \mathcal{X}_t} f(\mathbf{x}, \pi_t) = \sup_{\mathbf{x} \in \mathcal{X}} f(\mathbf{x}, \pi^*)
% % \end{equation}
% % where $\pi^*$ is the optimal policy.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows from the theory of evolutionary algorithms with elitist selection. The key steps are:
% % 1. Show that the best fitness in the population is non-decreasing.
% % 2. Use the ergodicity of variation operators to show that any point in $\mathcal{X}$ can be reached with non-zero probability.
% % 3. Apply the Borel-Cantelli lemma to show that the global optimum will be found in the limit.
% % \end{proof}



% % Essentially for the prompt evolving, we care about two things:
% % \begin{itemize}
% %     \item When the coverage is sufficient: we want to make sure the distribution is balanced.
% %     \item When the coverage is insufficient: we want to generate more \emph{novel} prompts.
% % \end{itemize}

% % {
% % \noindent
% % \centering
% % \begin{minipage}{.96\linewidth}
% %   \begin{algorithm}[H]
% %     \small
    
% %     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
% %     \begin{algorithmic}[1]
% %     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$
% %     \Statex

% %     \Repeat

% %     \Until 
% %     \State
% %     \Return 
% %     \end{algorithmic}
% %   \end{algorithm}
% % \end{minipage}
% % \par
% % }

% %self-improving robust optimization

==> texs/method.tex <==
\newpage
% \section{Method}\label{sec:method}
\vspace{-10pt}
\paragraph{Section overview.} We aim to develop language models that can \emph{self-improve to generalize well on new, unseen tasks} beyond the initial training prompt distribution. 
In $\S$~\ref{sec:principle}, we show the limitations of classical RLHF and generalize it to the new objective of open-ended RLHF. In $\S$~\ref{sec:mechanism}, we introduce creator-solver games to tractably achieve the objective. In $\S$~\ref{sec:algo}, we detail a practical algorithm with a plug-in creator, compatible with any preference optimization algorithm as the solver. Lastly in $\S$~\ref{sec:int}, we discuss various interpretations for~\method.
%% RA.21.9: Before showing any math, probably worth motivating what we want to do -- the role of  theory is formalize things, which should be intutitive. 
\vspace{-10pt}
\subsection{The Principle: Open-Ended RLHF for Joint Self-Improvement}~\label{sec:principle}
\hspace{-6pt}\textbf{Intuition.} \ \ Classical RLHF (\textit{cf}., Eq.~\ref{eq:rlhf-cls}) optimizes over a \emph{static} prompt distribution, meaning that the agent is only aligned to a fixed prompt set $\mathcal{D}$, making it brittle when it is evaluated on new problems from the ever-changing real world. Our Open-Ended RLHF breaks away from this static framework, with the goal to develop an agent that \emph{generalizes} well across \emph{unseen, novel} environments (where the tasks entailed in prompts may not have been explicitly encountered during training). To achieve this, we must design a new objective that agents can generate its own problems for self-improvement.
% , allowing $\rvx$ to come from a dynamic, ever-changing distribution that co-evolves with the agent's ability to solve tasks.
 % \ie \emph{the static optimization fails to adapt}.


\vspace{-10pt}
\paragraph{Formalization.} We introduce an \emph{open-ended} reference distribution $p_{\text{ref}}(\rvx)$, which is conceptually approached by a prompt  policy $\pi_{\vphi}(\rvx)$, co-evolving with the response policy for alignment:

% We introduce an \emph{optimizable} prompt generation policy $\pi_{\vphi}(\rvx)$, which is conceptually optimized towards an \emph{open-ended reference distribution} $p_{\text{ref}}(\rvx)$, jointly with the response policy optimization for preference alignment, formalized as:

\vspace{+3pt}

\begin{mdframed}
\begin{defn}[Open-Ended RLHF]\label{eq:rlhf-joint}
We define \emph{evolving alignment} as the open-ended joint optimization  on the prompt and response policy for alignment w.r.t the joint reference policy:
\vspace{-3pt}
\begin{align}
    \max_{\vphi, \vtheta}  \ \mathbb{E}_{\tg{\rvx\sim \pi_{\vphi}(\cdot)}  , \  \tc{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
    - \beta \cdot  \sD_{\text{KL}}\Biggl[\ \tb{\pi_{\vphi, \vtheta}(}\tb{\rvx}\tb{, \ } \tb{\rvy}\tb{)} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)  } \ \Biggl], \label{eq:rlhf-joint-} \vspace{-5pt}
\end{align}
where $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ and $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx)$\footnote{\textcolor{black}{This generalizes  classical RLHF (Eq.~\ref{eq:rlhf-cls}). One may extend the above and rewrite coefficients to be:}
\vspace{-6pt}
\begin{align}
\scalebox{0.9}{$ 
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \emphred{\tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \bigr[ r(\mathbf{x}, \mathbf{y})  \bigr] - \beta_1 {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \bigr]}}} \ \textcolor{cgreen}{\Bigr]} 
- \beta_2  \emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx) \Bigr]}}.
$}\label{eq:rlhf-expand}
\end{align} \vspace{-10pt}}.
% denotes the training joint distribution and the reference joint distribution, respectively.
\end{defn}
\end{mdframed}
\vspace{-2pt}
Here, $p_{\text{ref}}(\rvx)$ represents an \emph{underspecified}, potentially intractable probability distribution over possible tasks (instantiated \emph{via} prompts) in the wild, as a realizable \textbf{open-ended reference} that covers the full diversity and complexity of tasks agents may encounter, \emph{not} the initial static prompt set $\calD$. The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts, while being close to the SFT policy $\pi_{\text{SFT}}(\rvy | \rvx)$. 
% The joint optimization formalizes the setting that task distributions and the agent’s response policy are both updated, for the agent to be well-aligned in the broader prompt space of the open world.
\vspace{-3pt}



\subsection{The Mechanism: Asymmetric Self-Play \emph{via} Creator-Solver Games}~\label{sec:mechanism}
\hspace{-6pt}\textbf{Intuition.}\quad  It can be hard to directly solve  Eq.~\ref{eq:rlhf-joint-}, due to (i) the \textbf{intractability} of the underspecified reference~\citep{paired}, (ii) the  \textbf{instability} of joint differentiation~\citep{gan}. We present a heuristic of iterative alternating optimization by casting it as an \textbf{asymmetric creator-solver game}, that \textbf{implicitly achieves} the conceptual probability matching of $\sD_{\text{KL}}[\pi_{\phi}(\rvx) \ \| \ p_{\text{ref}}(\rvx) ]$ by iteratively creating a \emph{sequence} of prompt distributions to expand over the task space. 
\vspace{-5pt}
\begin{itemize}
    \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{${\pi_{\phi}(\rvx)}$} that strategically generate new prompt distributions.
    \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
\end{itemize}
\vspace{-10pt}
This game serves as one potential choice to implicitly achieve the Open-Ended RLHF principle.
\vspace{-5pt}
\begin{itemize}
    \item By design, the creator can guide the solver with an \emph{informative prompt curriculum}, for it to develop more general capabilities to handle complexities in the wild~\citep{jiang-thesis}. 
    \item Intuitively, this resembles RL optimization \emph{via} expectation-maximization~\citep{hinton-em, rest_em}, where $\vphi$ for the prompt distribution is fixed at each step.
\end{itemize}



% \quad We formalize the alternating optimization as an asymmetric game as follows:
% \vspace{-3pt}
% \begin{itemize}
%     \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{$\pi_{\phi}(\rvx)$} that strategically generate new prompt distributions.
%     \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
% \end{itemize}

% This asymmetric game is one potential modeling choice to implicitly achieve the open-ended RLHF principle. We look forward to exploring more principled solutions in the future.

\textbf{Formalization.} We consider the \emph{minimax regret} strategy~\citep{savage1951theory},  where the \tb{solver} minimizes and the \tb{creator}  maximizes regret\footnote{\vspace{-40pt}Please see $\S$~\ref{app:theory} and Eq.~\ref{eq:KL-regret} for details on the KL-optimal policy $\pi^{\star}_{\text{KL}}(\rvy \mid \rvx)$. }, \ie the reward difference of the current and KL-optimal policy:
\begin{align}
    \operatorname{Regret}(\pi_{\phi}, \pi_{\vtheta}) = \sE_{\rvx \sim \pi_{\phi}(\cdot)} \Bigr[ \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] \Bigr].\label{eq:regret-pi}
\end{align}
\vspace{-10pt}
At the equilibrium~\citep{nash}, prior works~\citep{paired} have shown:
\vspace{+5pt}

\begin{mdframed}
\begin{rem}[Minimax Regret]
    If the above solver-creator game reaches an equilibrium, the solver follows a minimax regret policy, \ie the worst-case regret is bounded:
\begin{align}
    \tb{\pi^{\star}_{\calY \mid \calX}} \in \underset{ \tb{\pi_{\calY \mid \calX}} }{\arg \min} \  \underset{\tb{\pi_\calX}}{\max} \ \sE_{\rvx \sim \pi_{\calX}}  \ \Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\calY \mid \calX}}) \ \Bigr].\label{eq:minimax-regret}
\end{align}
\end{rem}
\end{mdframed}
\vspace{-6pt}
To illustrate, open-ended RLHF allows for the creation of evolving prompt distributions that challenge the agent progressively for better generalization; the introduced minimax regret objective further adds \emph{robustness} on top of such evolving curricula by \emph{incentivizing agents to perform well in all cases}. 

% \begin{align}
%     \text{info}(\rvx) \gets \widehat{A}_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') |, \label{eq:info-proxy}
% \end{align}


However, while it is often straightforward for the \textbf{solver} to minimize the regret (\eg by direct policy optimization), the optimal policy remains unknown during optimization, thus regret as the decision signal is often intractable to the \textbf{creator} -- regret approximation is needed. We design the proxy below for creator's  regret approximation (see  $\S$~\ref{app:theory} for further illustration), also as a metric for prompt informativeness:
\vspace{+0.6pt}
\begin{mdframed}
\begin{defn}[Informativeness]\label{def:info-proxy}
    We estimate the informativeness of a prompt $\rvx$ in preference optimization by the (absolute) worst-case optimal advantage, approximating regret in Eq.~\ref{eq:regret_definition}:
\begin{align}
    | \hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta}) | \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{-}) , \label{eq:info-proxy}
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \quad \mathbf{y}_{-} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}
and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle.
% which is estimated by sampling multiple responses for $\rvx$ from the solver and calculating  gap between the maximal reward (from the best $\rvy$) and the minimal reward (from the worst $\rvy$).
\end{defn}
\end{mdframed}
\vspace{-4pt}
We use the informativeness proxy to guide the creator for prompt distribution adaptation, which has a few useful properties under different interpretations, as in $\S$~\ref{sec:int}. In this way, we define a mechanism that the solver learns to improve, as the creator keeps challenging the solver on its weaknesses.

% \footnote{Some works~\citep{plr,active-pl} tested Shannon entropy, which is empirically found to underperform reward-based metric. We encourage future studies into this.}

% \fix{Add one sentence comment on the implications on the mimax regret; for example: To iterate, our open-ended RLHF objective does not focus on a fixed distribution of prompts, but rather allow for the creation of an evolving distribution that challenges the agent progressively, to ensure it generalize well under unseen, novel scenarios. The minimax regret framework adds a layer of robustness by minimizing the agent's performance gap in worst cases. It is not just about generalizing to novel prompted tasks, but also ..} Without access to the true optimal policy, we must approximate the regret. We design the advantage-based proxy as follows:

% We choose to use variants of advantage functions for the approximation, as shown in Table~\ref{tab:info-metric}, which we also refer as the informativeness proxy\footnote{Note that some works~\citep{plr,active-pl} had tested using Shannon entropy as the informativeness metric, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage more future studies into this.}, with $A^{\star}_{\min}$ as the default proxy due to its relation to minimax regret in Eq.~\ref{eq:minimax-regret}.
% \vspace{+1pt}
% \begin{mdframed}
% \begin{defn}[Informativeness Proxy]
%     We use the minimax regret as the proxy for the informativeness metric of the prompt, approximated by the (absolute) worst-case optimal advantage:
% \begin{align}
%     \text{info}(\rvx) \gets A_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | 
% \end{align}
% \end{defn}
% \end{mdframed}
% This proxy enjoys many nice properties under various interpretations, which we illustrate in $\S$~\ref{sec:int}.

\vspace{-4pt}
\subsection{The Practical Algorithm}~\label{sec:algo}\vspace{-4pt}
\hspace{-4pt}We now illustrate~\method~of Algorithm~\ref{alg:i-eva}, with practical implementations specified in $\S$~\ref{app:reproduce}. 

% The full pipeline is that we combine the creator and solver step in an iterative preference optimization pipeline.

\subsubsection{The Creator Step:  Estimate, Sample then Evolve}\label{sec:creator-step}\vspace{-2pt}
Plainly, the creator finds most useful prompts and generate variants of them for preference optimization. One may relate this to \emph{evolution strategies}~\citep{schwefel1977evolutionsstrategien} which find the most promising species, then mutate and crossover, or to \emph{curriculum RL}~\citep{accel} which finds environments with high-regret levels, then edits within some distance. In this work, we do not seek a differentiable creator in this work; the creator is implemented in three steps as in Figure~\ref{fig:pipeline} to approximate regret maximization. See more in $\S$~\ref{app:theory}.
\vspace{-6pt}

\paragraph{Step 1: $\texttt{\small info}(\cdot)$ -- \textnormal{\it estimate the informativeness}.} For each $\rvx$ in the  prompt set $\calX_t$, we generate responses, annotate rewards and estimate a informativeness metric to $\rvx$ by Eq.~\ref{eq:info-proxy} (see also Table~\ref{tab:info-metric}). \vspace{-6pt}
% To calculate the empirical value of $A^{\star}_{\min}$ for  each prompt, we first sample multiple responses from the prompt, where we label each response with its reward, then we use the difference between the highest reward $r_{\max}$ and the lowest reward $r_{\min}$ to represent the informativeness proxy.

\paragraph{Step 2: $\texttt{\small sample}(\cdot)$ -- \textnormal{\it weighted sampling for an informative subset}.} By using the informativeness metric as the weight,
we sample an informative prompt subset $\calX_t^{\texttt{\tiny info}}$ to be evolved later. This is similar to finding high-regret levels in curriculum RL~\citep{accel}.\vspace{-6pt}

\paragraph{Step 3: $\texttt{\small evolve}(\cdot)$ -- \textnormal{\it evolving for a proximal region of high-advantage prompts}.} Our algorithm is agnostic to and does not rely on any specific evolving method (see empirical evidence in~\secref{app:exp-evol}). We take \text{EvolInstruct}~\citep{wizardlm} as a default off-the-shelf method, which conducts in-depth (\ie adding constraints, deepening, concretising, complicating) and in-breadth evolving (\ie mutation) for prompts. Specifically, we iterate over each prompt in the $\calX_t^{\texttt{\tiny info}}$, where each one is evolved to multiple variations, then optionally mix the newly generated prompts with a uniformly sampled buffer from $\calX_t$ to create $\calX_{t+1}$.

 % (\eg 20\% of the original)

 % by meta-instruction (\ie using an LLM to re-write the original prompts with the aforementioned evolving directions)


\subsubsection{The Solver Step: Solve then Optimize}\label{sec:solver-step}\vspace{-2pt}
This step is the classical preference optimization~\citep{dpo}, where responses are generated and the gradient descent is performed. Take the pointwise reward model setting as an example, for every prompt, we sample $n$ responses with reward annotated for each; we take the responses with the maximal and the minimal reward to construct the preference pairs, then optimize upon. This implicitly minimizes the regret to the KL-optimal policy, which we present in more details at $\S$~\ref{app:theory}.

Put together, \method~can unify existing iterative optimization pipeline~\citep{snorkel} with a new creator module, which can either share the same network as the solver policy or operate independently.

% \tc{An important contribution of our work is proposing the metric for preference optimization; so worth having a subsection somewhere on this.}
% (probably point to the appendix on the prompt distribution when we have it).


% \paragraph{Learning potential.} Our metric intuitively captures prompts with high learning potential by distinguishing between those that elicit both high-reward and low-reward responses. This contrast highlights areas where the agent can improve.

\subsection{Understanding the Informativeness Proxy in Different Intuitive Ways}\label{sec:int}

\paragraph{Learning potential.} Our metric intuitively identifies the learning potential of a prompt by measuring the gap between the best and worst response to it from the solver. We reason, that prompts eliciting \emph{both} high-reward and low-reward outcomes, reflect \emph{learnable} tasks where the model is capable of improving but has not yet mastered, thereby implying learning potential (\textit{cf.}, \cite{plr}). 
% The evolving step then generates similar prompts with increased diversity to further promote generalization.
\vspace{-10pt}
\paragraph{Worst-case guarantees.} The minimax-regret objective, by design, leads to solvers that  perform robustly across the prompt space, thus gives the worst-case guarantee. While exact equilibrium may not be attainable with approximation,  our empirical results in  $\S$~\ref{sec:ab-metric} demonstrate robustness.
\vspace{-10pt}
\paragraph{Auto-curricula for the players.}
We visualize the curriculum induced by~\method~in $\S$~\ref{app:curr}. With the stochastic policy, the advantage may be heuristically understood as the reward difference between \emph{a base solver} and \emph{a reference solver}. Rather than optimizing separate solvers~\citep{paired}, we sample multiple times from the same policy to create the pair. In this way, the creator is incentivized to produce new prompts that are just out of the comfort zone of solvers~\citep{zone-promximal}:
\vspace{-6pt}
\begin{itemize}
    \item For overly challenging prompts, both solutions perform poorly, leading to a low  proxy.\vspace{+1pt}
    \item For overly easy prompts, the base solution already performs well, again giving a low proxy.\vspace{+1pt}
    \item The optimal strategy is to find prompts that are just beyond the solver's current capability.
\end{itemize}
\vspace{-2pt}
\vspace{-10pt}
\paragraph{Auto-curricula inherent to Contrastive Optimization.} Contrastive preference optimization generalizes DPO and a family of algorithms (\textit{c.f.}, \cite{cpl,dpo,tang2024generalized}), many of whose losses monotonically decrease as the contrastive ratio increases. Here, by Eq.~\ref{eq:reward-re} and Eq.~\ref{eq:contrastive-ratio-main}, the \emph{contrastive ratio} can be written via the \emph{advantage-based proxy}:
\begin{align}
    A^{\star}_{\min}(\rvx)  = \beta \cdot \textcolor{black}{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}} .
\end{align}
By our proxy, we implicitly incentivize the creator to generate prompts that \emph{bring the most contrastive responses}, which decrease the loss the most. This matches the curriculum learning literature, which prioritizes (in~\method, \emph{generatively} prioritizes) examples with smaller losses for better convergence and generalization~\citep{easy-bengio2009curriculum}. We hence suggest the \emphtext{\textit{Contrastive Curriculum Hypothesis}}: in contrastive preference optimization, prioritizing prompts with higher contrastive ratio improves sample efficiency and generalization. We show initial empirical results on this in $\S$~\ref{sec:ab-metric} and $\S$~\ref{sec:ab-cont}.
% \begin{hypo}[Contrastive Curriculum Hypothesis]
%     In contrastive preference optimization, prioritizing prompts w/ \emph{higher contrastive ratio} improves sample efficiency and generalization.
% \end{hypo}

% footnote{One direction that worth to explore could be to directly use $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ instead of the reward proxy.}















% {\color{red} RA.9.26: This sounds like a para for related work possibly along with the footnote}

% % This formulation aims to find a policy $\pi$ that minimizes the worst-case regret across all possible prompt distributions. At equilibrium, this guarantees that the chosen policy $\pi$ performs robustly across the entire prompt space $\mathcal{X}$.

% This property ensures a smooth progression of the curriculum, always challenging $\pi$ with prompts that are neither too easy nor impossibly difficult.


% \textbf{Stackelberg Game Formulation for Self-Improving Language Models}

% \begin{enumerate}
%     \item \textbf{Players:}
%     \begin{itemize}
%         \item Prompt Player: $$\textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)}$$
%         \item Response Player: $$\textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')}$$
%     \end{itemize}

%     \item \textbf{Definitions:}
%     \begin{itemize}
%         \item $\rvx \in \mathcal{X}$: Base prompts from a distribution $\mathcal{X}$
%         \item $\rvx' \in \mathcal{X}'$: Generated prompts
%         \item $\rvy \in \mathcal{Y}$: Responses
%         \item $\rvh \in \mathcal{H}$: Historical information
%         \item $\vtheta \in \Theta$: Shared parameters of the prompt and response generators
%     \end{itemize}

%     \item \textbf{Objective Functions:}
%     \begin{equation*}
%     \overbrace{\max_{\vtheta} \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}}}})}^{\text{prompt player}}, \qquad 
%     \overbrace{\max_{\vtheta} \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}}^{\text{response player}}
%     \end{equation*}
    
%     where
%     \begin{align*}
%        \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}, \rvy\sim p^{\text{response}}_{\vtheta}}\left[D(\rvx', \rvx) + \lambda U(\rvx', \vtheta)\right] \\
%         \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}}\left[R(p^{\text{response}}_{\vtheta}(\cdot \mid \rvx'), \rvx')\right]
%     \end{align*}

%     And:
%     \begin{itemize}
%         \item $D: \mathcal{X}' \times \mathcal{X} \to \mathbb{R}_+$ is a diversity measure
%         \item $U: \mathcal{X}' \times \Theta \to \mathbb{R}_+$ is an uncertainty measure
%         \item $R: (\mathcal{Y} \to [0,1]) \times \mathcal{X}' \to \mathbb{R}$ is a reward function
%         \item $\lambda \in \mathbb{R}_+$ is a hyperparameter
%     \end{itemize}

%     \item \textbf{Game Formulation:}
%     \begin{align*}
%         &\vtheta^\star = \arg\max_{\vtheta}\emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} \\
%         \text{s.t. } &\vtheta \in \arg\max_{\vtheta'} \ \   \emphgoal{J_R(\vtheta', \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}
%     \end{align*}

%     \item \textbf{Induced Distributions:}
%     \begin{align*}
%         \mu_{\vtheta}(\rvx', \rvy) &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \cdot \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')} \ \right] \\
%         \nu_{\vtheta}(\rvx') &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \ \right]
%     \end{align*}
% \end{enumerate}

% \textbf{Game Formulation Explanation:}

% The Stackelberg game formulation captures the interaction between the prompt generator (leader) and the response generator (follower). The prompt generator aims to maximize $J_P$, which encourages the generation of diverse and uncertain prompts. The response generator, in turn, maximizes $J_R$, which rewards high-quality responses to the generated prompts.

% % The game is asymmetric, with the prompt generator acting first. This allows the prompt generator to anticipate the response generator's behavior and generate prompts that will lead to overall improvement in the language model's capabilities.

% The constraint $\vtheta \in \arg\max_{\vtheta'} J_R(\vtheta', p^{\text{prompt}}_{\vtheta})$ ensures that the response generator is optimal with respect to the current prompt distribution. This captures the idea that the response generator quickly adapts to the prompts generated by the prompt generator.

% \textbf{Induced Distributions Explanation:}

% The induced distributions $\mu_{\vtheta}$ and $\nu_{\vtheta}$ characterize the behavior of the language model under the current parameters $\vtheta$:

% 1. $\mu_{\vtheta}(\rvx', \rvy)$ is the joint distribution of generated prompts and responses. It captures the overall behavior of the language model, including both prompt generation and response generation.

% 2. $\nu_{\vtheta}(\rvx')$ is the marginal distribution of generated prompts. This distribution is crucial for understanding the diversity and coverage of the prompt space achieved by the prompt generator.

% % These distributions play a key role in analyzing the equilibrium properties of the game and in proving theoretical guarantees about the language model's performance.
% \newpage

% \textbf{Equilibrium Properties and Theoretical Guarantees}

% \begin{itemize}
%     \setcounter{enumi}{5}
%     \item \textbf{Stackelberg Equilibrium:}
%     A Stackelberg equilibrium $\vtheta^\star$ satisfies:
%     \begin{align*}
%         \vtheta^\star &\in \arg\max_{\vtheta} J_P(\vtheta, \textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}) \\
%         \vtheta^\star &\in \arg\max_{\vtheta} J_R(\vtheta, \textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}})
%     \end{align*}

%     At this equilibrium:
%     \begin{enumerate}
%         \item $\textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}}$ generates diverse prompts that effectively explore the prompt space and target areas of model uncertainty.
%         \item $\textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}$ produces high-quality responses across the range of generated prompts.
%     \end{enumerate}

%     \item \textbf{Theorem (Performance Guarantee):} 
%     At the Stackelberg equilibrium $\vtheta^\star$:
%     \begin{equation*}
%         \mathbb{E}_{\rvx'\sim\nu_{\vtheta^\star}}[R(p^{\text{response}}_{\vtheta^\star}(\cdot \mid \rvx'), \rvx')] \geq R^\star - (\varepsilon_D + \varepsilon_U + \varepsilon_T)
%     \end{equation*}

%     Where:
%     \begin{itemize}
%         \item $R^*$ is the optimal achievable reward
%         \item $\varepsilon_D \geq 0$ is the suboptimality in prompt diversity
%         \item $\varepsilon_U \geq 0$ is the suboptimality in uncertainty targeting
%         \item $\varepsilon_T \geq 0$ is a transfer error term
%     \end{itemize}

%     \item \textbf{Proof Sketch:}
%     \begin{enumerate}
%         \item Let $p^{\text{prompt}*}$ and $p^{\text{response}*}$ be the optimal prompt and response generators, respectively.
%         \item By the optimality of $\vtheta^*$ for the response player:
%         \begin{equation*}
%             \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}}_{\vtheta^*}(\cdot \mid \rvx'), \rvx')] \geq \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \varepsilon_R
%         \end{equation*}
%         where $\varepsilon_R \geq 0$ is the suboptimality of the response generator.
        
%         \item The diversity and uncertainty terms in $J_P$ ensure:
%         \begin{equation*}
%             D_{KL}(\nu_{\vtheta^*} \parallel \nu^*) \leq \varepsilon_D + \varepsilon_U
%         \end{equation*}
%         where $\nu^*$ is the optimal prompt distribution and $D_{KL}$ is the Kullback-Leibler divergence.
        
%         \item Using Pinsker's inequality and the properties of the reward function:
%         \begin{equation*}
%             |\mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')]| \leq \varepsilon_T
%         \end{equation*}
        
%         \item Combining these inequalities and noting that $\mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] = R^*$, we obtain the desired result.
%     \end{enumerate}

%     \item \textbf{Corollary (Convergence):}
%     Under mild conditions on the learning dynamics and function approximators, the iterative algorithm converges to a Stackelberg equilibrium as $T \to \infty$.
% \end{itemize}

% \textbf{Stackelberg Game Variants}

% \begin{itemize}
%     \setcounter{enumi}{9}
%     \item \textbf{Prompt as Leader (PaL):} 
%     Choosing the prompt player as leader results in the following optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_P\left(\vtheta, p^{\text{response}*}_{\vtheta}\right) \text{ s.t. } p^{\text{response}*}_{\vtheta} \in \arg \max_{p^{\text{response}}} J_R\left(\vtheta, p^{\text{prompt}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     We solve this nested optimization using the first-order gradient approximation, resulting in updates:
%     \begin{align*}
%     p^{\text{response}}_{k+1} &\approx \arg \max_{p^{\text{response}}} J_R\left(\vtheta_k, p^{\text{prompt}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \alpha_k \nabla_{\vtheta} J_P\left(\vtheta, p^{\text{response}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Response as Leader (RaL):} 
%     Conversely, choosing the response player as leader results in the optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_R\left(\vtheta, p^{\text{prompt}*}_{\vtheta}\right) \text{ s.t. } p^{\text{prompt}*}_{\vtheta} \in \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta, p^{\text{response}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     Similarly, we solve this using the first-order gradient approximation:
%     \begin{align*}
%     p^{\text{prompt}}_{k+1} &\approx \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta_k, p^{\text{response}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \beta_k \nabla_{\vtheta} J_R\left(\vtheta, p^{\text{prompt}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Comparison:} 
%     \begin{itemize}
%         \item PaL prioritizes the generation of diverse and uncertain prompts, potentially leading to more exploratory behavior.
%         \item RaL focuses on optimizing responses, which may result in more stable learning but potentially less exploration.
%         \item The choice between PaL and RaL depends on the specific requirements of the task and the desired balance between exploration and exploitation.
%     \end{itemize}

%     \item \textbf{Convergence Properties:}
%     Under suitable regularity conditions on $J_P$, $J_R$, and the function approximators:
%     \begin{itemize}
%         \item Both PaL and RaL converge to local Stackelberg equilibria as $k \to \infty$.
%         \item The rate of convergence and the quality of the equilibrium may differ between PaL and RaL, depending on the landscape of $J_P$ and $J_R$.
%     \end{itemize}
% \end{itemize}


% \newpage
% \section{Experiments}

% \notes{TODO: add experimental details in this section. In general, we can consider two types of tasks, one is the general alignment task, where the preference comes from human values; the other can be math/coding task, where the preference oracle is the environment, signaling true or false for the correctness.}

% % \section{Evolutionary Prompt Set Optimization}

% % We formulate the problem of evolving the prompt set as a population-based optimization algorithm. Let $\mathcal{X}$ be the space of all possible prompts, and $\mathcal{X}_t \subset \mathcal{X}$ be our prompt set at iteration $t$.

% % \subsection{Fitness Function}

% % Define a fitness function $f: \mathcal{X} \times \Pi \rightarrow \mathbb{R}$, where $\Pi$ is the space of policies. For a prompt $\mathbf{x} \in \mathcal{X}$ and policy $\pi \in \Pi$, $f(\mathbf{x}, \pi)$ measures the "fitness" of $\mathbf{x}$ with respect to $\pi$. This could be defined in various ways, such as:

% % \begin{equation}
% % f(\mathbf{x}, \pi) = \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[\mathbb{P}(\vtau \succ \pi | \mathbf{x})] - \frac{1}{2}
% % \end{equation}

% % where $\mathbb{P}(\vtau \succ \pi | \mathbf{x})$ is the probability that response $\vtau$ is preferred over $\pi$'s typical response to $\mathbf{x}$.

% % \subsection{Population Dynamics}

% % Let $P_t = \{(\mathbf{x}_i, w_i)\}_{i=1}^N$ be the population at time $t$, where $\mathbf{x}_i \in \mathcal{X}_t$ and $w_i \in \mathbb{R}^+$ is a weight associated with $\mathbf{x}_i$. The evolution of the population follows these steps:

% % 1. \textbf{Selection}: Select a subset $S_t \subset P_t$ based on fitness values.
% % 2. \textbf{Variation}: Generate new prompts $V_t$ through mutation and crossover operations on $S_t$.
% % 3. \textbf{Evaluation}: Compute fitness for new prompts in $V_t$.
% % 4. \textbf{Replacement}: Update $P_{t+1}$ by combining $P_t$ and $V_t$.

% % \subsection{Information-Theoretic Approach}

% % We can incorporate information theory to guide the evolution process. Define the information content of a prompt $\mathbf{x}$ with respect to policy $\pi$ as:

% % \begin{equation}
% % I(\mathbf{x}, \pi) = H(\pi(\cdot|\mathbf{x})) - \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[H(\mathbb{P}(\cdot|\mathbf{x}, \vtau))]
% % \end{equation}

% % where $H(\cdot)$ is the Shannon entropy and $\mathbb{P}(\cdot|\mathbf{x}, \vtau)$ is the distribution over preferences given prompt $\mathbf{x}$ and response $\vtau$.

% % We can then define a composite fitness function:

% % \begin{equation}
% % F(\mathbf{x}, \pi) = \alpha f(\mathbf{x}, \pi) + (1-\alpha) I(\mathbf{x}, \pi)
% % \end{equation}

% % where $\alpha \in [0,1]$ balances between preference improvement and information gain.

% % \subsection{Variation Operators}

% % 1. \textbf{Mutation}: For $\mathbf{x} \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \mathbf{x} + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% %    \end{equation}
% %    where $\sigma^2$ is the mutation strength.

% % 2. \textbf{Crossover}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \lambda \mathbf{x}_1 + (1-\lambda) \mathbf{x}_2, \quad \lambda \sim \text{Beta}(a, b)
% %    \end{equation}

% % 3. \textbf{Information Exchange}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$ from different topics, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \textsc{Combine}(\mathbf{x}_1, \mathbf{x}_2)
% %    \end{equation}
% %    where \textsc{Combine} is a function that merges aspects of $\mathbf{x}_1$ and $\mathbf{x}_2$.

% % \subsection{Convergence Analysis}

% % Under certain conditions, we can prove convergence properties of this evolutionary algorithm:

% % \begin{thm}[Convergence of Evolutionary Prompt Optimization]
% % Let $\{\mathcal{X}_t\}_{t=0}^\infty$ be the sequence of prompt sets generated by the evolutionary algorithm. Assume:
% % \begin{enumerate}
% %     \item $f(\mathbf{x}, \pi)$ is continuous in $\mathbf{x}$ for all $\pi \in \Pi$.
% %     \item The variation operators are ergodic.
% %     \item The selection operator retains the best prompt with non-zero probability.
% % \end{enumerate}
% % Then, with probability 1:
% % \begin{equation}
% % \lim_{t \to \infty} \max_{\mathbf{x} \in \mathcal{X}_t} f(\mathbf{x}, \pi_t) = \sup_{\mathbf{x} \in \mathcal{X}} f(\mathbf{x}, \pi^*)
% % \end{equation}
% % where $\pi^*$ is the optimal policy.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows from the theory of evolutionary algorithms with elitist selection. The key steps are:
% % 1. Show that the best fitness in the population is non-decreasing.
% % 2. Use the ergodicity of variation operators to show that any point in $\mathcal{X}$ can be reached with non-zero probability.
% % 3. Apply the Borel-Cantelli lemma to show that the global optimum will be found in the limit.
% % \end{proof}



% % Essentially for the prompt evolving, we care about two things:
% % \begin{itemize}
% %     \item When the coverage is sufficient: we want to make sure the distribution is balanced.
% %     \item When the coverage is insufficient: we want to generate more \emph{novel} prompts.
% % \end{itemize}

% % {
% % \noindent
% % \centering
% % \begin{minipage}{.96\linewidth}
% %   \begin{algorithm}[H]
% %     \small
    
% %     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
% %     \begin{algorithmic}[1]
% %     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$
% %     \Statex

% %     \Repeat

% %     \Until 
% %     \State
% %     \Return 
% %     \end{algorithmic}
% %   \end{algorithm}
% % \end{minipage}
% % \par
% % }

% %self-improving robust optimization

==> texs/pre.tex <==
\newpage
\section{Preliminaries}
We hereby review major concepts, which we later in $\S$~\ref{sec:method} use  \emphtext{\emph{regret}}  and the proxy by  \emphtext{\emph{advantage}} to identify informative prompts, leading to learning curricular implicitly maximizing \emphtext{\emph{contrastive ratio}}.

\vspace{-10pt}
\paragraph{Alignment by RLHF.} Classical RLHF~\citep{ouyang2022training} optimizes on a fixed distribution $\calD$:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \bigl] \Bigl],\label{eq:rlhf-cls}
\end{align}
where $\rvx$ and $\rvy$ denote the prompts and responses, and $r(\cdot, \cdot)$ is the reward function.

\vspace{-10pt}
\paragraph{Reward.} Let the \emph{optimal policy} of Eq.~\ref{eq:rlhf-cls} be $\pi^{\star}(\cdot)$ and $Z(\cdot)$ be the partition function, we have:
\begin{align}
    \hspace{+5pt}r(\rvx, \rvy)=\beta \cdot \log \frac{ \pi^{\star}(\rvy \mid \rvx)} {\pi_{\text {\text{SFT}}}(\rvy \mid \rvx)}\textcolor{black}{ \ + \ \beta \cdot \log Z(\rvx)}. \label{eq:reward-re}\vspace{-10pt}
\end{align}
\vspace{-20pt}
\paragraph{Regret and advantage.} Given the optimal policy \( \pi^\star \), the \emph{regret} of a policy \( \pi_{\boldsymbol{\theta}} \) at \( \mathbf{x} \) is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\mathbf{y} \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr]. \label{eq:regret_definition}
\end{align}
The \emph{advantage} function quantifies how much better a response $\rvy$ is w.r.t. a baseline:
\begin{align}
    \hspace{+8pt}A(\rvx, \rvy) = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \label{eq:advantage-definition}
\end{align}
Variants of advantage (\eg the worst-case advantage $A^{\star}_{\min}$) are related to regret, as shown in Table~\ref{tab:info-metric}.



\vspace{-10pt}
\paragraph{Direct preference optimization.} The DPO~\citep{dpo} objective for RLHF is:
% \begin{align}
%     \calL_{\beta}^{\text{DPO}}(\pi_\vtheta) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}} - \log \Biggr[\sigma \Bigr(\beta \cdot  \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right) \Bigr)\Biggr],
% \end{align}
\begin{align}
    \hspace{+16pt}\calL_{\beta}^{\text{DPO}}(\pi_\vtheta) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}} - \log \Bigr[\sigma \bigr(\beta \cdot  \Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx} \bigr)\Bigr],
\end{align}
where we use $+, -$ to denote chosen and rejected responses, and denote the \textbf{contrastive ratio} as:
\begin{align}
\hspace{+16pt}\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}:=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}. \label{eq:contrastive-ratio-main}
\end{align}
By reward reparameterization with Eq.~\ref{eq:reward-re},  variants of advantage also relate to contrastive ratio, as in $\S$~\ref{sec:int}.

\vspace{-5pt}
\section{Method}\label{sec:method}
\paragraph{Algorithm overview.} On a high level, \method~extends classical RLHF to open-ended  RLHF \emph{via} a creator that adapts prompt distributions with an easy-to-implement \emphtext{\emph{estimate, sample then evolve}} procedure, mimicing the \emphtext{\emph{minimax-regret}} policy of asymmetric self-play games, as detailed in $\S$~\ref{sec:algo}.
% \paragraph{Algorithm overview.} Motivated by the \emph{minimax-regret} principle for open-ended learning, our~\method~introduces a creator that adapts prompt distributions through an \emph{estimate, sample, then evolve} procedure. This requires only minor modifications to the existing alignment pipeline. Further details are provided in $\S$\ref{sec
% }.

\vspace{-10pt}
\input{tabs/algo-eva}
\vspace{-10pt}


% We now present a verbose description of our method~\method, which we will revisit later in different ways. Our overall procedure trains a series of models $\vtheta_1, \cdots, \vtheta_T$ from the initial model $\vtheta_0$. For the creator step, starting from the initial prompt set $\calX_t$ where $t=0$, for each prompt $\vx_i$ in the prompt set, we generate $n$ responses $\vy_i^{(j)}$ with the current $\vtheta_t$, then each response receives a reward $r_i^{(j)}$ from an external preference oracle. We then evaluate the informativeness of the prompt by signals elicited from rewards, say the worst-case reward advantage, such that $\text{info}(\rvx_i) = \widehat{A}^{\star}_{\min}(\rvx) = \max(\{ r_i^{(j)}\}_{j=1}^n) - \min(\{ r_i^{(j)}\}_{j=1}^n)$. Next, we conduct weighted sampling on the original set $\calX_t$ using $\text{info}(\rvx_i)$ as the weight to obtain a informative subset $\calX_t^{\text{info}}$. This step is similar to finding the high-regret level among all levels in classical open-ended learning~\citep{accel}. We then evolve a new set  based on $\calX_t^{\text{info}}$; the evolving process (\eg adding constraints to or concretizing the original prompts as in~\citep{wizardlm}) is similar to making small edits on the high-regret levels; we then combine the evolved new set with a buffer of original prompts from $\calX_t$ to obtain $\calX_{t+1}$. This will be used as the training prompt distribution to train $\vtheta_t$ to $\vtheta_{t+1}$, which we term as the solver step. We then repeat the process to continuously grow the prompt distribution and optimize the parameter.

% , where each current model $\vtheta_t$ is trained 

% \paragraph{Creator step.}

% \paragraph{Solver step.}


% In the next, we will illustrate that a useful strategy for open-ended learning is to continuously generate \emph{high regret} environments. In our context, this is equivalent to generating prompts with \emph{high absolute advantage}. This can also be interpreted as generating prompts with \emph{high contrastive ratio}. Informally, the notion of the contrastive ratio $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ captures captures how much \emph{surprise} we have about the $\rvx$ by sampling responses from $\pi_{\vtheta}$, and we use it as a proxy for the informativeness of a prompt.


% Together this brings an automatic curriculum that helps the learning agent generalize better.

% (\log \frac{\pi_{\vtheta}\left(\rvy_{+} \mid \rvx \right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx \right)}- \log \frac{\pi_{\vtheta}\left(\rvy_{-} \mid \rvx \right)}{\pi_{\mathrm{ref}}\left(\rvy_{-} \mid \rvx \right)}) 
% \begin{align}
% \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot   \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right)\right)\right],
% \end{align}
% where we define the \textcolor{black}{\emph{contrastive ratio}} as:
% \begin{align}
%     \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right):=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \label{eq:contrastive-ratio-main}
% \end{align}

% Essentially, the loss function of most preference optimization algorithms can be generalized as a convex function of the contrastive ratio, \ie~$f_{\beta}(\Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right))$\footnote{A concurrent work~\citep{tang2024generalized} discusses about this generalization as well.}.




% \begin{align}
%     \min_{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}} \left[ \mathbb{E}_{\rvy \sim \pi_\vtheta(\rvy \mid \rvx)} \left[ \operatorname{Regret}(\rvx, \rvy) \right] \right]
%     + \beta \cdot \mathbb{D}_{\mathrm{KL}}\left[ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\mathrm{ref}}(\rvy \mid \rvx) \right]. \label{eq:regret_minimization}
% \end{align}


% the optimal policy is also proportional to the optimal advantage function, which is the negated regret:
% \begin{align}
%     \pi^{\star}(\rvy | \rvx) \propto  
% \end{align}


% The optimal solution is:
% \begin{align}
%     \pi^{\star}(\rvy | \rvx) = \textcolor{lightgray}{\frac{1}{Z(\rvx)}} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right). 
% \end{align}

% By re-parameterization, we have:
% \begin{align}
%     r(\rvx, \rvy)=\beta \cdot \log \frac{\pi^{\star}(\rvy \mid \rvx)}{\pi_{\text {\text{ref}}}(\rvy \mid \rvx)} + \textcolor{lightgray}{\beta \cdot \log Z(\rvx)}.
% \end{align}


% The RLHF objective is to maximize:
% \begin{align}
%     J_{\beta}(\pi) &= J(\pi) - \beta \cdot \mathbb{D}_{\mathrm{KL}}\left[\pi(\vtau) \| \pi_{\mathrm{ref}}(\vtau)\right] \\
%     &= \sE_{\vtau \sim \pi(\vtau)} \left[ r(\vtau) - \beta \cdot \log \frac{\pi(\vtau)}{\pi_{\text{ref}}(\vtau)}\right] \label{eq:rlhf-2} \\
%     &= \sE_{\rva_h \sim \pi(\cdot \mid \rvs_h)} \left[ \sum_{h=1}^{H} \left( r(\rvs_h, \rva_h) -\beta \log \frac{\pi\left(\rva_h \mid \rvs_h\right)}{\pi_{\mathrm{ref}}\left(\rva_h \mid \rvs_h\right)} \right)  \mid \rvs_0 \sim \rho(\rvs_0)\right]. 
%     %= \underset{\rva_h \sim \pi(\cdot \mid \rvs_h)}{\sE}
% \end{align}









% \paragraph{Direct preference optimization (DPO).} The DPO objective~\citep{dpo} is to minimize:
% \begin{align}
%     \calL_{\beta}^{\text{DPO}}(\pi) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}_{\text {pref}}} - \log \left[\sigma\left(\beta \cdot  \log \frac{\pi\left(\rvy_{+} \mid \rvx \right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx \right)}-\beta \cdot \log \frac{\pi\left(\rvy_{-} \mid \rvx \right)}{\pi_{\mathrm{ref}}\left(\rvy_{-} \mid \rvx \right)}\right)\right],
% \end{align}
% where $\sigma(\cdot)$ is the sigmoid function. We denote the loss function as:
% % \begin{align}
% % \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphgray{\dlog} \right)\right],
% % \end{align}
% \begin{align}
% \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot   \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right)\right)\right],
% \end{align}
% where we define the \textcolor{black}{\emph{contrastive ratio}} as:
% \begin{align}
%     \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right):=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \label{eq:contrastive-ratio-main}
% \end{align}

% Essentially, the loss function of most preference optimization algorithms can be generalized as a convex function of the contrastive ratio, \ie~$f_{\beta}(\Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right))$\footnote{A concurrent work~\citep{tang2024generalized} discusses about this generalization as well.}.

% We present a summary table on other preference alignment algorithms in Appendix~\ref{app:table}.

















% \paragraph{No-regret learning.}

% \notes{TODO: Move the following part to Section~\ref{sec:mechanism} as a sub-sub-section, that illustrate that our objective has a specific meaning for DPO objective.}

% In the specific case of DPO, the loss is monotonically smaller as $\dlog$ gets larger. This justifies our use of $r_{\max} - r_{\min}$ as the informativeness metric to prioritize the training examples according to the curriculum learning literature~\citep{easy-bengio2009curriculum}\footnote{In general, the curriculum learning literature prioritizes examples with lower losses and claims improvement in both convergence and generalization. There is also another line of literature in optimization that claims examples with higher losses can be prioritized~\citep{hard-losers,hard-obs,hard-osgd,ordered-sgd}; however, \cite{rho-loss} conjecture that those example are often noisy (not learnable) or task-irrelevant, and are impractical. Our empirical results in Section~\ref{sec:ab-metric} confirms this. We hereby follow the curriculum learning literature.}, which is essentially the reward of the chosen response ($r_{\max}$) minus the reward of the rejected response ($r_{\min}$), that is:
% \begin{align}
%     r_{\max} - r_{\min} = \beta \cdot \textcolor{SlateBlue4}{\Delta_{\log}(\pi ^\star \| \pi_{\text{ref}})}.
% \end{align}

% While we may directly select data with $\dlog$, the usage of $r_{\max} - r_{\min}$ provides a fast approximation to this term.

% Another message is that, we should adaptively choose the informativeness metric when we use different optimization algorithms.

% \notes{A issue might be that, as the contrastive ratio becomes larger, the gradient update will decrease. We may want to adaptively adjust the learning rate.}
% \notes{To generalize all the online RLHF algorithms in the game-theoretic framework.}

% \paragraph{Alignment with Reward Modeling.} Classical preference optimization methods consider to first learn a reward model explicitly~\citep{rlhf} or implicitly~\citep{nash} using the Bradley-Terry model~\citep{bt}. Given a triplet $(\rvx, \vtau^+, \vtau^-)$ where $\rvx$ is the prompt and $\vtau$ is the response, the Bradley-Terry model specifies the probability of preferring $\vtau^+$ over $\vtau^-$ as:
% \begin{align}
%     \sP_{\text{BT}}\left(\vtau^+ \succeq \mathbf{\vtau}^- \mid \rvx \right) &=\frac{\exp (r\left(\vtau^+, \rvx\right)) }{\exp (r\left(\vtau^+, \rvx\right)) +\exp( r\left(\vtau^-, \rvx\right))} \nonumber \\
%     % &= \frac{1}{1 + \exp \left(- (r\left(\mathbf{x}, \vtau^+\right) - r\left(\mathbf{x}, \vtau^-\right))\right)} \\
%     &= \sigma \left(r\left(\vtau^+, \rvx\right) - r\left(\vtau^-, \rvx\right)\right). \label{eq:bt}
% \end{align}
% Classical RLHF~\citep{rlhf} first learn a reward model $r_{\phi}(\cdot, \cdot)$ by maximizing the log likelihood of the above, then optimize the following objective:
% \begin{align}
%     \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \calX, \vtau \sim \pi_\theta(\cdot \mid \rvx)}\left[r_\phi(\rvx, \vtau)\right]-\eta ^{-1} \cdot \mathbb{D}_{\mathrm{KL}}\left[\pi_\vtheta(\vtau \mid \rvx) \ \| \ \pi_{\mathrm{ref}}(\vtau \mid \rvx)\right].\label{eq:rlhf-cls}
% \end{align}
% The optimization problem has a closed-form solution~\citep{dpo} as:
% \begin{align}
%     \pi^{\star}(\vtau \mid \rvx) &= \textcolor{gray}{\frac{1}{Z(\rvx)}}\cdot \pi_{\text{ref}}(\vtau \mid \rvx) \cdot \exp \left(\eta \cdot \emphgray{r(\vtau, \rvx)}\right) \label{eq:rlhf-1} \\
%     &\propto \pi_{\mathrm{ref}}(\vtau \mid \mathbf{x}) \cdot \exp (\eta \cdot r(\vtau, \rvx)). \label{eq:rlhf-2}
% \end{align}
% This leads to the implicit optimal reward formulation:
% \begin{align}
%     r^{\star}(\vtau, \rvx)=\eta^{-1} \cdot \log \frac{\pi^{\star}(\vtau \mid \rvx)}{\pi_{\text {\text{ref}}}(\vtau \mid \rvx)}+\textcolor{gray}{\eta^{-1} \cdot \log Z(\rvx)}.
% \end{align}

% Taken it back to the Bradley Terry model, we have:
% \begin{align}
%       \sP_{\text{BT}}\left(\vtau^+ \succeq \mathbf{\vtau}^- \mid \rvx \right) &= \sigma\left(\eta^{-1} \log \frac{\pi^{\star}\left(\vtau^+ \mid \rvx\right)}{\pi_{\text{ref}}\left(\vtau^+ \mid \rvx\right)}-\eta^{-1} \log \frac{\pi^{\star}\left(\vtau^- \mid \rvx\right)}{\pi_{\text{ref}}\left(\vtau^- \mid \rvx\right)}\right).
% \end{align}
% The direct preference optimization (DPO) loss thus is:
% \begin{align}
%     \mathcal{L}_{\mathrm{DPO}}\left(\pi_\vtheta ; \pi_{\text {\text{ref}}}\right)=-\mathbb{E}_{\left(\rvx, \vtau^+, \vtau^-\right) \sim \mathcal{D}}\left[\log \sigma\left(\eta^{-1} \log \frac{\pi_\vtheta\left(\vtau^+ \mid \rvx\right)}{\pi_{\text {ref}}\left(\vtau^+ \mid \rvx\right)}-\eta^{-1} \log \frac{\pi_\vtheta\left(\vtau^- \mid \rvx\right)}{\pi_{\text {ref}}\left(\vtau^- \mid \rvx\right)}\right)\right].
% \end{align}

% % \notes{Double check IPO on the preference modeling part.}


% \paragraph{Alignment with General Preferences.} This line of works~\citep{nlhf,self-play-gu} consider to learn the general preference $\sP\left(\vtau \succeq \mathbf{\vtau}^\prime \mid \rvx \right)$ \emph{without reward modeling}, by casting the problem as a two-player constant-sum game, where optimal policy is assumed to be identified by the minimax winner or the Nash equilibrium~\citep{nash}:
% \begin{align}
%     \left(\pi^\star, \pi^\star\right)=\arg \max _\pi \min _{\pi^{\prime}} \mathbb{E}_{\mathbf{x} \sim \mathcal{X}}\left[\mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x}), \vtau^{\prime} \sim \pi^{\prime}(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right]\right].
% \end{align}
% Define the preference over policies as:
% \begin{align}
%     &\mathbb{P}(\vtau \succ \pi \mid \mathbf{x})=\mathbb{E}_{\vtau^{\prime} \sim \pi(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right], \\
%     &\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \mathbf{x}\right)=\mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x})} \mathbb{E}_{\vtau^{\prime} \sim \pi^{\prime}(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right], \\
%     &\mathbb{P}\left(\pi \succ \pi^{\prime}\right)=\mathbb{E}_{\mathbf{x} \sim \mathcal{X}}\left[\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \mathbf{x}\right)\right].
% \end{align}
% The Nash equilibrium can then be expressed as:
% \begin{align}
%     \left(\pi^\star, \pi^\star\right)=\arg \max _\pi \min _{\pi^{\prime}} \mathbb{P}\left(\pi \succ \pi^{\prime}\right) .
% \end{align}

% \paragraph{Self-Play Preference Optimization (SPPO).} We hereby provide a brief intro on SPPO~\citep{self-play-gu}. The high-level idea is to iteratively update the policy with the multiplicative weight for it to asymptotically converge to the optimal policy. The iterative framework is:
% \begin{align}
%     \pi_{t+1}(\vtau \mid \rvx) = \textcolor{gray}{\frac{1}{Z_{\pi_t}(\rvx)}} \cdot \pi_t(\vtau \mid \rvx) \cdot \exp \left(\eta \cdot \emphgray{\mathbb{P}(\vtau \succ \pi_t \mid \mathbf{x})} \right). \label{eq:sppo-1}
% \end{align}
% Notice how this differs from Eq.~\ref{eq:rlhf-1}. The DPO-alike loss considers to re-parameterize the reward model and cancel out the normalizing factor $Z(\cdot)$. Alternatively, SPPO considers to directly approximate the policy update raio, in terms of $L_2$ distance:
% \begin{align}
% \pi_{t+1}=\underset{\pi}{\arg \min} \ \mathbb{E}_{\mathbf{x} \sim \mathcal{X}, \vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left(\underbrace{\log \left(\frac{\pi(\vtau \mid \mathbf{x})}{\pi_t(\vtau \mid \mathbf{x})}\right)}_{\text{Policy Update Ratio}} - \underbrace{\left(\eta \cdot \emphgray{\mathbb{P}\left(\vtau \succ \pi_t \mid \mathbf{x}\right)}-\log Z_{\pi_t}(\mathbf{x})\right)}_{\text{Preference Advantage Term}}\right)^2. \label{eq:sppo-2}
% \end{align}
% The finite-sample optimization problem is written as:
% \begin{align}
% \pi_{t+1}=\underset{\pi}{\arg \min} \ \mathbb{E}_{\mathbf{x} \sim \mathcal{X}, \vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left(\underbrace{\log \left(\frac{\pi(\vtau \mid \mathbf{x})}{\pi_t(\vtau \mid \mathbf{x})}\right)}_{\text{Policy Update Ratio}} - \underbrace{\left(\eta \cdot \emphorange{\mathbb{P}\left(\vtau \succ \widehat{\pi}^K_t \mid \mathbf{x}\right)}-\log Z_{\widehat{\pi}^K_t}(\mathbf{x})\right)}_{\text{Preference Advantage Term}}\right)^2,
% \end{align}
% where the preference is approximated by $K$ samples of responses with the oracle $\sP(\cdot)$:
% \begin{align}
%     \emphorange{\mathbb{P}\left(\vtau \succ \widehat{\pi}_t^K \mid \mathbf{x}\right)} = \frac{1}{K} \cdot \sum_{k=1}^K \mathbb{P}\left(\vtau \succ \vtau_k \mid \mathbf{x}\right),
% \end{align}
% and the normalizing factor is:
% \begin{align}
%     Z_{\widehat{\pi}_t^K}(\mathbf{x})=\mathbb{E}_{\vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left[\exp \left(\eta \cdot \mathbb{P}\left(\vtau \succ \widehat{\pi}_t^K \mid \mathbf{x}\right)\right)\right],
% \end{align}
% where the expectation can be approximated by $M$ samples from the policy $\pi_t$. In~\citep{self-play-gu}, the term is replaced by a constant $1/2$, meaning the model will not be updated when there is a tie.


% % \paragraph{Nash Equilibrium.}





==> texs/quotes.tex <==
% QUOTES from the accel~\citep{accel} paper

% --------------------
Deep reinforcement learning (RL) has seen tremendous success over the past decade. However, agents trained on fixed environments are brittle, often failing the moment the environment changes even slightly, thus limiting the real-world applicability of current RL methods. A common remedy is to introduce more training data diversity by randomizing the environment’s parameters in every episode—a process called domain randomization (DR). For example, these parameters might control the friction coefficient and lighting conditions in a robotic arm simulation or the position of obstacles in a maze (we call each such environment variation a level). Procedurally generating training levels to expose RL agents to more diverse experiences has quickly become a common method for improving the robustness of RL agents. However, DR is often not enough to train robust agents in domains where the agent struggles to make progress on many challenging levels. 

Adaptive curriculum methods match the complexity of training levels to an agent’s current capabilities, and have been shown to produce more robust policies in fewer training steps than domain randomization. These methods can be viewed as a game between a teacher that designs challenging levels and a student that solves them. This game is potentially open-ended, leading to the co-evolution of generally-capable students. By tailoring the distribution of entire levels throughout training, adaptive curricula perform unsupervised environment design (UED). However, training an environment-designing teacher is difficult, and the prior state-of-the-art UED method, Prioritized Level Replay (PLR), simply finds challenging levels through random search, making it unable to build off of previously found structures that were useful for training agents in the past. We can also expect its performance to degrade as the size of the design space grows, limiting the potential for open-ended co-evolution between teacher and student. In contrast, the evolutionary processes between organisms and their environments, which UED resembles, efficiently search the design space by successively mutating a population and selecting the fittest individuals. 

We combine evolution with a principled regret-based environment designer in an algorithm called Adversarially Compounding Complexity by Editing Levels (ACCEL). As in PLR, our new method uses the difference between how well an agent did in an environment and how well it could have done (a metric known in decision theory as regret) to quantify the learning potential of revisiting this environment in the future. The important difference from PLR is that ACCEL evolves a curriculum by making small edits (e.g. mutations) to previously high regret levels, thus constantly producing new levels at the frontier of the student agent's capabilities. By compounding complexity over time, ACCEL harnesses the potential for efficient, open-ended search inherent to evolution. Our results show that ACCEL’s adaptive curricula lead to RL agents that outperform existing auto-curriculum learning methods. 

The rest of this article describes ACCEL in more technical detail. We first provide the necessary background on the UED formalism, followed by a comprehensive description of the ACCEL algorithm. We then present our experimental results in two challenging domains consisting of maze navigation and continuous-control bipedal locomotion, where ACCEL evolves levels with higher complexity and produces policies exhibiting significantly improved generalization compared to other adaptive curriculum methods. 

==> texs/theory.tex <==
% \section{Theoretical Analysis}
% \begin{thm}[Existence of Nash Equilibrium]
% Consider the two-player game between a prompt player $\pi_X$ and a policy player $\pi$, with compact strategy spaces $\Pi_X$ and $\Pi$ respectively. Let $\mathbb{P}(\cdot)$ be a continuous preference function. Define the payoff function:

% \begin{align}
%     J(\pi_X, \pi) = \mathbb{E}_{\pi_X \sim \Pi_X} \left[\max_{\pi^\prime \in \Pi} \mathbb{P}(\pi^\prime \succ \pi \mid \pi_X)\right].
% \end{align}

% % where $\mathbb{P}(\pi \succ \pi'|\vx) = \mathbb{E}_{\vtau \sim \pi(\cdot|\vx)} \mathbb{E}_{\vtau' \sim \pi'(\cdot|\vx)} [\mathbb{P}(\vtau \succ \vtau'|\vx)]$.

% Then, there exists a Nash equilibrium $(\pi_X^\star, \pi^\star)$ such that:

% \begin{align}
%     (\pi_X^\star, \pi^\star) \in \arg \max_{\pi_X \in \Pi_X} \min_{\pi \in \Pi} J(\pi_X, \pi).
% \end{align}
% \end{thm}


% TODO: update the Berk-Nash equilibrium analysis and justify the usage of regret gap as the selection metric.

==> texs_/analysis.tex <==
% \newpage
% \section{\textcolor{Gray}{[1\% Draft]} Theoretical Analysis}

% % \begin{thm}[Restated from Theorem 1 of~\citep{self-play-gu}] 
% % Assume the optimization problem is realizable in Eq.~\ref{eq:sppo-2}. Denote $\bar{\pi}_T=\frac{1}{T} \sum_{t=1}^T \pi_t$ as the average policy. By setting $\eta=\Theta(1 / \sqrt{T})$, the convergence rate of the average policy towards the Nash equilibrium is:
% % \begin{align}
% %     \max _\pi\left[\mathbb{P}\left(\pi \succ \bar{\pi}_T\right)\right]-\min _\pi\left[\mathbb{P}\left(\pi \prec \bar{\pi}_T\right)\right]=O(1 / \sqrt{T}) .
% % \end{align}
% % \end{thm}

% % The optimal policy is defined with regard to the initial $\calX_{\text{init}}$ and a pre-defined preference oracle $\sP(\cdot)$. Assuming there is a superset $\calX$ that $\mathcal{X}_{\text{init}} \subset \mathcal{X}$, we can show that the learned policy can be suboptimal under $\calX$. The interesting question is, that can we construct a sequence of $\{\calX_t\}_{t=0}^{\infty}$, such that the policy performance is monotonically improving?

% % The challenge here is, that unlike classical active learning, which mostly  cares about the \emph{sampling} issues, we care about \emph{generating} novel prompts from a fixed vocabulary.


% \begin{ftheo}[Policy Convergence with a Fixed Prompt Set, Restated from~\cite{self-play-gu}]

% Let $\mathcal{X}_{\text{init}}$ be a fixed prompt set and $\mathbb{P}(\cdot \succ \cdot)$ be a pre-defined preference oracle. Assume that the optimization problem is realizable in Eq.~\ref{eq:sppo-2}. Denote $\bar{\pi}_T=\frac{1}{T} \sum_{t=1}^T \pi_t$ as the average policy learned from $\mathcal{X}_{\text{init}}$. By setting $\eta=\Theta(1 / \sqrt{T})$, the convergence rate of the average policy towards the Nash equilibrium is:
% \begin{align}
%     \max_\pi\left[\mathbb{P}\left(\pi \succ \bar{\pi}_T\right)\right]-\min_\pi\left[\mathbb{P}\left(\pi \prec \bar{\pi}_T\right)\right]=O(1 / \sqrt{T}) .
% \end{align}
% \end{ftheo}
% % \begin{ftheo}

% Assuming a golden preference oracle, the convergence properties is established for a fixed prompt set $\mathcal{X}_{\text{init}}$. However, in real-world scenarios, we often encounter a broader range of prompts than initially anticipated. Let $\mathcal{X}$ be a superset representing the true distribution of prompts, where $\mathcal{X}_{\text{init}} \subset \mathcal{X}$. The policy $\pi^\star$ that is optimal with respect to $\mathcal{X}_{\text{init}}$ \emph{can be suboptimal} when evaluated on $\calX$.

% This observation motivates us to consider an evolving prompt set. The key question is: \emph{can we construct this sequence such that the performance of $\pi_t$ improves monotonically when evaluated on the full set $\mathcal{X}$?} This is just like mathematical conjecturing. Given a fixed set of known axioms or theorem statements, our goal is to navigate in the language space to iteratively create a new set which approximately covers all valid theorem statements. We formalize the idea below.

% \begin{mdframed}
% \begin{defn}[Prompt Set Sequence]
% A prompt set sequence is a series $\{\mathcal{X}_t\}_{t=0}^{\infty}$ where $\mathcal{X}_0 = \mathcal{X}_{\text{init}}$ and for all $t \geq 0$, $\mathcal{X}_t \subseteq \mathcal{X}_{t+1} \subseteq \mathcal{X}$, with $\mathcal{X}$ being a superset with all possible prompts.
% \end{defn}
% \end{mdframed}

% This question presents unique challenges distinct from classical active learning. While active learning primarily addresses sampling from a fixed set, our problem involves generating novel prompts from a fixed vocabulary. This generative aspect introduces additional complexity, as we must ensure that new prompts are both syntactically valid and semantically meaningful.



% \begin{mdframed}
% \begin{defn}[Policy Performance]
% Given a prompt set $\mathcal{X}$ and a preference oracle $\mathbb{P}(\cdot)$, the performance of a policy $\pi$ is defined as:
% \begin{align}
%     J(\pi, \mathcal{X}) = \mathbb{E}_{\mathbf{x} \sim \mathrm{Unif}(\mathcal{X})} \left[ \mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x})} [\mathbb{P}(\vtau \succ \pi_{\text{ref}} \mid \mathbf{x})] \right].
% \end{align}
% where $\pi_{\text{ref}}$ is any reference policy.
% \end{defn}
% \end{mdframed}

% The challenge lies in constructing each $\mathcal{X}_{t+1}$ such that $J(\pi_{t+1}, \mathcal{X}) \geq J(\pi_t, \mathcal{X})$. 

% %This is non-trivial because expanding the prompt set introduces new challenges for the policy, potentially leading to temporary decreases in performance. Moreover, the true set $\mathcal{X}$ is unknown, making direct optimization of $J(\pi_t, \mathcal{X})$ infeasible.

% \begin{mdframed}
% \begin{pro}[Prompt Generation]
% Given a fixed vocabulary $V$, a current prompt set $\mathcal{X}_t$, and a current policy $\pi_t$, find a function $g: V \times \mathcal{X}_t \times \Pi \rightarrow \mathcal{X}$ such that:
% \begin{enumerate}
%     \item $g(V, \mathcal{X}_t, \pi_t) \not\subseteq \mathcal{X}_t$.
%     \item $J(\pi_t, \mathcal{X}_t \cup g(V, \mathcal{X}_t, \pi_t)) \geq J(\pi_t, \mathcal{X}_t)$.
% \end{enumerate}

% where $\Pi$ is the space of all policies.
% \end{pro}
% \end{mdframed}












% % \subsection{Evolving Prompt Distribution}
% % \notes{To add more motivation here with formalized theoretical toy example. A simple intuition is, that assume the original prompt set contain an imbalanced set of easy and hard examples, and we should do dynamic upsampling and downsampling. Check the efficient exploration paper~\citep{efficient-llm}.}

% % In the SPPO framework, prompts are assumed to be sampled from a fixed distribution $\mathcal{X}$. However, in practice, we often work with a finite set of prompts that may not fully represent the true distribution of tasks the model will encounter. This mismatch can lead to poor generalization and inefficient learning. We formalize this issue in the following theorem:

% % \begin{lem}[Inefficiency of Static Prompt Set]
% % Let $\mathcal{X}$ be the true distribution of prompts, and let $\mathcal{X}_0 \subset \mathcal{X}$ be a finite subset used for training. Define the expected improvement for a prompt $\mathbf{x}$ at iteration $t$ as:
% % \begin{equation}
% % I_t(\mathbf{x}) = \mathbb{E}_{\vtau \sim \pi_t(\cdot|\mathbf{x})}[\max(0, \mathbb{P}(\vtau \succ \pi_t | \mathbf{x}) - 1/2)].
% % \end{equation}

% % For any $\epsilon > 0$, there exists a $T$ such that for all $t > T$:
% % \begin{equation}
% % \max_{\mathbf{x} \in \mathcal{X}_0} I_t(\mathbf{x}) < \epsilon,
% % \end{equation}

% % while there exists an $\mathbf{x}' \in \mathcal{X} \setminus \mathcal{X}_0$ such that:
% % \begin{equation}
% % I_t(\mathbf{x}') > \epsilon.
% % \end{equation}
% % \end{lem}

% % \notes{Re-state the lemma. The fundamental idea here is, that if we are sampling from a subset, the convergence will not be the Nash equilibrium, but rather the Berk-Nash equilibrium. We should thus build a sequence of $\calX_t$, so that we can converge.}

% % The intuition is that a static prompt set eventually becomes inefficient for learning, as the model's performance on these prompts plateaus while it remains poor on unseen prompts.

% % To address this issue, we propose a dynamic prompt set expansion strategy:

% % \begin{defn}[Dynamic Prompt Set]
% % Let $\mathcal{X}_t$ be the prompt set at iteration $t$. We update the prompt set according to:
% % \begin{equation}
% % \mathcal{X}_{t+1} = (1 - \alpha) \cdot \mathcal{X}_t \cup \alpha \cdot \calS_t
% % \end{equation}
% % where $\calS_t$ is a set of newly sampled prompts based on a criterion $C_t$ defined below, and $\alpha \in (0,1)$ is a mixing parameter.
% % \end{defn}

% % % The key challenge is defining an effective criterion $C_t$ for sampling new prompts. 

% % \begin{defn}[Uncertainty-based Prompt Sampling]
% % Let $U_t(\mathbf{x})$ be an uncertainty measure for prompt $\mathbf{x}$ at iteration $t$. We define:
% % \begin{equation}
% % C_t(\mathbf{x}) \propto U_t(\mathbf{x}) \cdot p(\mathbf{x})
% % \end{equation}

% % where $p(\mathbf{x})$ is an estimate of the true prompt distribution.
% % \end{defn}

% % There are different practical design choices to concertize the evolving prompt sets.

% % % -----------------------------------------
% % \subsection{Preference Model Refinement}
% % % -----------------------------------------

% % To address the limitations of a fixed preference oracle, we propose to \emph{distill} and \emph{refine} a preference (critic?) model alongside the policy. This approach allows us to distill knowledge from the oracle and potentially generalize beyond its limitations.

% % Let $p_\phi(\vtau \succ \vtau' | \mathbf{x})$ be a parameterized preference model (which could be trained with the network for the policy?). In the most naïve formulation, we can update this model using the beow objective:
% % \begin{equation}
% % \mathcal{L}_\text{pref}(\phi) = \mathbb{E}_{\mathbf{x}, \vtau, \vtau'}[(\mathbb{P}(\vtau \succ \vtau' | \mathbf{x}) - P_\phi(\vtau \succ \vtau' | \mathbf{x}))^2]
% % \end{equation}

% % We can then use this learned preference model in the SPPO update:
% % \begin{align}
% % \pi_{t+1}(\vtau | \mathbf{x}) \propto \pi_t(\vtau | \mathbf{x}) \exp(\eta \cdot p_\phi(\vtau \succ \pi_t | \mathbf{x})).
% % \end{align}

% % Intuitively, this approach allows the model to learn to discriminate at the same time.

% % Some other ideas:

% % \subsubsection{Online Preference Learning}

% % We can learn the preference model online, simultaneously with the policy. This approach is closer to the Berk-Nash equilibrium concept. The learned preference model represents the \emph{subjective belief} of the language models.

% % \begin{defn}[Online Preference Learning]
% % At each iteration $t$:
% % \begin{enumerate}
% %     \item Update preference model: $\theta_{t+1} = \arg\min_\theta L(\theta; \mathcal{D}_t)$
% %     where $\mathcal{D}_t$ is the observed preference data up to time $t$, and $L$ is a suitable loss function.
% %     \item Update policy: $\pi_{t+1}(\vtau|\mathbf{x}) \propto \pi_t(\vtau|\mathbf{x}) \exp(\eta P_{\theta_{t+1}}(\vtau \succ \pi_t | \mathbf{x}))$
% % \end{enumerate}
% % \end{defn}

% % This approach allows the preference model to adapt over time as more data is collected.

% % \subsubsection{Uncertainty-Aware Preference Modeling}

% % Instead of a point estimate, we maintain a distribution over preference models to capture uncertainty in our preference estimates.

% % \begin{defn}[Bayesian Preference Modeling]
% % We model the preference probability as:
% % \begin{align}
% % P(\vtau \succ \vtau' \mid \mathbf{x}) = \int P(\vtau \succ \vtau' \mid \mathbf{x}, \theta) p(\theta \mid \mathcal{D}_t) d\theta
% % \end{align}

% % where $p(\theta \mid \mathcal{D}_t)$ is the posterior  over preference model parameters given observed data $\mathcal{D}_t$.
% % \end{defn}

% % This Bayesian approach allows us to incorporate uncertainty into our policy updates and potentially make more informed decisions.

% % \begin{thm}[Convergence under Misspecified Preferences]
% % Under certain regularity conditions, if we use either the Online Preference Learning or Uncertainty-Aware Preference Modeling approach, the policy $\pi_t$ converges to a Berk-Nash equilibrium as $t \to \infty$.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows these key steps:
% % \begin{enumerate}
% %     \item The preference model converges to the best approximation within the model class, minimizing KL divergence to the true preference distribution.
% %     \item Given this converged preference model, the policy update converges to the optimal policy for this model.
% %     \item This combination of beliefs (represented by the converged preference model) and policy satisfies the definition of Berk-Nash equilibrium.
% % \end{enumerate}
% % A full proof would require specifying the regularity conditions and providing a more detailed analysis of the convergence properties.
% % \end{proof}

% % This theorem provides a theoretical foundation for our approach, showing that under appropriate conditions, our evolving self-play alignment framework can converge to a meaningful equilibrium even in the presence of misspecified preferences.



==> texs_/app-exp.tex <==
\newpage
\textbf{------------------- OLD OUTDATED STUFFS IGNORE --------------------}
\section{Comprehensive Evaluation Results on Alignment Benchmarks}

We here show evolving is helpful for alignment under different training settings.


\paragraph{Hyperparameter settings.} Unless otherwise specified, we use the hyperparameter setting below:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.66\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{IPO}    & \textbf{SimPO}  & \textbf{SPPO}    \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & 0.6    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ \bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-params}
\end{table}

\paragraph{Iterative Training Settings.} By default~\citep{self-play-gu}, we split data into equal-size subsets, then iterative train the model with different split at each iteration as:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_1$ : init with $\vtheta_0$; trained w/ the prompt split $D_1$ by self-generated responses.
    \item $\vtheta_2$ : init with $\vtheta_1$; trained w/ the prompt split $D_2$ via by self-generated responses.
    \item ...
\end{itemize}
\vspace{-5pt}
For the evolved models:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_1^{\text{evol}}$ : init with $\vtheta_1$; evolve $D_1$ to $D_1^{\text{evol}}$ by feedbacks from $\vtheta_1$; train with a mixture of $D_1$ and $D_1^{\text{evol}}$ by self-generated responses. 
    \item $\vtheta_2^{\text{evol}}$ : init with $\vtheta_1^{\text{evol}}$; train w/ $D_2$ by self-generated responses to get $\vtheta_2^{\text{evol}, \prime}$; evolve $D_2$ to $D_2^{\text{evol}}$ by feedbacks from $\vtheta_2^{\text{evol}, \prime}$; train w/ a mix of $D_2$ and $D_2^{\text{evol}}$ by self-generated responses. 
    \item ...
\end{itemize}



    % \item \textbf{Average Optimal Advantage}: This can be viewed as an approximation to the \emph{negative} \textbf{Bayesian regret}. Take $N$ as the total number of generated responses:
    % \begin{align}
    %     \hspace{-66pt} \emphblue{A^{\star}_{\text{avg}}(\rvx)} = r^{\star}(\rvx) - \frac{1}{N} \sum_{\rvy}r(\rvx, \rvy). \label{eq:avg-advantage}
    % \end{align}
    % \item \textbf{Leave-One-Out Advantage:} Excluding the current response from the average:
    % \begin{align}
    %     \emphblue{A_{\text{loo}}(\rvx)} = \frac{1}{N} \sum_{\rvy} \Bigr(r(\rvx, \rvy) - \frac{1}{N-1} \sum_{\rvy' \neq \rvy} r(\rvx, \rvy') \Bigr). \label{eq:loo-advantage}
    % \end{align}

% \begin{table}[!h]
% \centering
% \label{tab:lm-glossary}
% % \resizebox{1.0\columnwidth}{!}{%
% \begin{tabular}{ll}
%  &  \\
%  &  \\
% \end{tabular}%
% % }
% \end{table}


% \subsection{Setting 1: Iterative Training with 6 Splits}


% % In the default setting, we split the 60K UltraFeedback data into 6 splits. For each iteration, we use the exactly same hyperparameter setting, albeit different.

% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule

% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 9.01 & 8.32& 8.66& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-p}) } &  \textbf{9.04}& \textbf{8.75} & \textbf{8.90}& \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  \textbf{55.35} &    \textbf{55.53} \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 
% \midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  9.00 &  8.45 &  8.72 & \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{eva-p}) } &   &  &   &  &  &  &  & \\ 
% \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      &  9.03 &  8.21 &  8.62 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% \qquad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% \qquad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \qquad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{eva-p}) } & \textbf{9.11} &  \textbf{8.45} &  \textbf{8.78} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-1}
% \end{table}
% % --------------------------------------------------------

% \ziyu{It looks like IPO is sensitive to the hyperparameter setting. The previous setting uses n\_epoch=2}

% \subsection{Setting 2: Iterative Training with 3 Splits}
% % --------------------------------------------------------
% \ziyu{The DPO here is using gpt-4o-mini to evolve, and we observe a drop in the performance compared to Iter 1. Notice that existing literature~\citep{self-play-gu} also reports drop during multiple iterations. It is likely that we need to control the hyper-parameter setting (\eg decrease the learning rate for the new iteration) for better performance.}

% \ziyu{It is very likely that there is reward hacking, and the reward model per se may be much imperfect.}

% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}
% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule

% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule

% DPO \  \hspace{+3pt}   Iter 1 / 3    & 9.21 & 8.67& 8.94 &  56.6 \textcolor{gray}{{\tiny CI: (-2.1, 2.5)}} &  729&  \textbf{54.38} &  50.93 \textcolor{gray}{\tiny $\pm$ 1.76} & 1909  \\
% \qquad \ \ \ \hspace{+1pt} Iter 2 / 3      &   9.35 &  8.83 & 9.09 & &  & 41.98 & 40.75 \textcolor{gray}{\tiny $\pm$ 1.73} & 3505  \\
% \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       &  9.15 & 8.55 & 8.85 & & & 37.17 & 35.40 \textcolor{gray}{\tiny $\pm$ 1.68} & 2962 \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \  \hspace{+3pt}   Iter 1 / 3 (\texttt{eva-p}) } & 9.19 & 8.39 & 8.79& \textbf{59.5} \textcolor{gray}{{\tiny CI: (-2.0, 2.4)}} & 826   &  49.89 &    \textbf{51.61} \textcolor{gray}{\tiny $\pm$ 1.76} & 2394 \\ 

% % \midrule

% % IPO \ \hspace{+6pt}  Iter 1    &  &   &   \\
% % \qquad \ \ \ \hspace{+0.001pt} Iter 2        &   \\
% % \qquad \ \ \  \hspace{+0.001pt} Iter 3        &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO \ \hspace{+6pt}  Iter 1  (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 

% % \midrule

% % SimPO  Iter 1 / 3         &    \\
% % \qquad \ \ \ \hspace{+1pt} Iter 2 / 3        &   \\
% % \qquad \ \ \  \hspace{+1pt} Iter 3 / 3        &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{SimPO Iter 1 / 3 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% % \midrule

% % SPPO \hspace{+2pt}  Iter 1 / 3     &   \\
% % \qquad \ \ \ \hspace{+1pt} Iter 2 / 3       &   \\
% % \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       &    \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{SPPO \hspace{+2pt} Iter 1 / 3 (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 



% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-2}
% \end{table}
% % --------------------------------------------------------


% \subsection{Setting 3: Iterative Training with No Split}
% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}
% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & avg. score      & score (\%)  & avg. len     & LC (\%) & WR (\%) &  avg. len    \\ \midrule
% SFT Baseline       &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\
% \midrule
% DPO \hspace{+1pt}        &  \\
% \rowcolor[HTML]{e2fbe2} 

% \text{DPO (\texttt{eva-p}) } &  &  &   &  &  &  &  &  \\ 
% \midrule
% IPO \hspace{+1pt}      &  &   &   \\
% \rowcolor[HTML]{e2fbe2} 
% \text{IPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \midrule
% SPPO \hspace{+1pt}     &   \\



% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \midrule
% SimPO \hspace{+1pt}        &    \\
% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO (\texttt{eva-p}) } &  &  &   &  &  &  &  & \\ 
% \bottomrule
% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:app-alignment-3}
% \end{table}
% % --------------------------------------------------------


% \newpage
% \section{Ablation Studies}
% In this section, we present detailed analysis with ablation on:
% \begin{itemize}
%     \item Sampling setting:
%     \item Infomrativeness metric:
%     \item Prompt Evolving Strategy:
%     \item Prompt Generation Model:
% \end{itemize}

% % (i) sampling setting; (ii)

% For all the ablation study, we use DPO as the default loss function, and use 10K data (\ie the first split) from the UltraFeedback dataset as the training data.

% \subsection{Ablation Study on the Sampling Setting}
% We consider using filtering v.s. weighted sampling v.s. weighted sampling on a graph.

% \subsection{Ablation Study on the Informativeness Metric}
% Take one of the above setting, vary on the metric. We currently consider:
% \begin{itemize}
%     \item max-min advantage:
%     \item max-mean advantage:
%     \item leave-one-out advantage:
%     \item reward mean:
% \end{itemize}

% \subsection{Ablation Study on the Prompt Evolving Strategy}

% % \subsection{Ablation Study on the Mixup Ratio}

% \subsection{Ablation Study on the LLMs Used to Generate the Prompts}
% We consider to use different underlying models to generate new prompts.
% \textbf{---------- OLD STUFFS ----------}

==> texs_/app-lit.tex <==
% \newpage
% \section{Extended Literature Review}

% \paragraph{Open-ended learning.} 
% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{plr}:
%     \item \cite{paired}:
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% % \cite{poet, paired, accel, minimax-refine}
% % faster convergence and better generalization
% % incentivizing / guiding the learner to better basin of attraction



% % \paragraph{Open-ended learning.}

==> texs_/app-main-cp.tex <==
% \section{Reproducibility Statement}\label{app:settings}

% \paragraph{Hyperparameter settings.} We follow the hyperparameter setting stated in~\citep{orpo,simpo,self-play-gu}, default to be:

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \centering
% \resizebox{0.7\columnwidth}{!}{%
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
% learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
% learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
% $\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
% $\gamma$                                                      & /      & /      & 5      & /       \\
% $\lambda$                                                      & /      & 0.5      & /      & /       \\
% no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
% warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
% effective batch size                                          & 8      & 8      & 32     & 8       \\
% max length                                                    & 2048   & 2048   & 2048   & 1024    \\
% max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
% optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
% \bottomrule
% \end{tabular}%
% }
% % \caption{Hyper}
% \label{tab:app-main-params}
% \end{table}


% \paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-rewarding}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
% \vspace{-5pt}
% \begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
%     \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
%     % \item ...
% \end{itemize}

% For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this as well as other plug-in evolving methods.

% % \paragraph{Computation environments.} 

% \paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve OpenAI models and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. In general, our codebase is very simple to use and requires only a creator module addition within the \href{https://github.com/huggingface/alignment-handbook}{Alignment Handbook} pipeline.

%  \paragraph{Code release.} We currently put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\textcolor{black}{\texttt{\small anonymous.4open.science/r/eva-i/}}}, which we intend to as well release all the source code there, and all the datasets and models to HuggingFace, upon approval -- before then, we are happy to provide any additional clarification requested to help re-implement~\method~and replicate our results. 

% \paragraph{Evaluation settings.} If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge, and \texttt{gpt-4-0314} as the baseline when calculating the win rate for evaluating on the benchmarks.





% -------------------------------------------------------------
\section{Issues of Fixed Prompt Training Distributions}\label{app:prompts}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
    \caption{The initial prompt distribution of AlpacaEval (openly accessible on HuggingFace) obtained from zero-shot classification with \texttt{bart-large-mnli}, which is imbalanced. Additionally, looking at the reward distribution, the category with lowest average reward has the highest average reward gap (\ie our default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
\end{figure}


% \paragraph{\emphtext{\method~minimally impact downstream tasks.}} 




% \section{Extended Discussions on Open-Ended Learning}

% The design of our game-theoretic framework is inspired from many prior works in open-ended learning, which we encourage the LLM community to explore more.  The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but general enough to handle the diversity of complexity of future environments. In the curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively build more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case environments. It is not just about generalizing to novel environments but also about ensuring that the agent can handle the most challenging scenarios within those environments. This distinction highlights the value of minimax regret: while classical open-ended learning focuses on generalization through exposure to diverse environments, minimax regret ensures that the agent is robust even under the most adversarial conditions.


% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{paired}: using two agents to simulate the regret.
%     \item \cite{plr}: having a rolling buffer of high-regret levels.
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% \paragraph{Self-improving / self-training language models.} 
\section{Additional Experimental Results}
% \subsection{Evaluation on Downstream Tasks}\label{sec:ab-downstream}
In general,~\method~maintains the accuracy on downstream tasks and is robust on those reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to the training sources for such reward models~\citep{armorm}.
\input{tables/tab-ab-downstream}
\vspace{-8pt}

% \subsection{The Effect of Different Reward Models at Different Scales}\label{app:ab-rm}
% In general, \method~presents scaling behavior across different datasets. We notice that the performance on MT-Bench is less stable, which may be due to the limited evaluation scale (80 questions), as similarly reported in~\citep{simpo,ah}
% \notes{The experiment is running.}
\input{tables/tab-ab-rm-app}


% -------------------------------------------------------------
% \section{Limitations}\label{app:limit}
% Off-policy is one concern. Another concern is that the advantage-based framework does not inherently works for general preference (we first do pairwise comparison; after )

% \subsection{The On-Polcy Variant: \texttt{eva-o}}\label{app:eva-o}
% The iterative training approach is inherently an off-policy algorithm; while being efficient, the performance can get plateau when more iterations goes on. We hereby show our method can easily extend to be on-policy, as shown in Algorithm~\ref{alg:o-eva}, that draws inspiration from Iterative Machine Teaching~\citep{bo-mt} and Ordered SGD~\citep{ordered-sgd} in the informative pool set selection (Line 4, which can be achieved either by greedy or through weighted sampling), while adding the new evolving step (Line 5). 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}(\vx_i)\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \texttt{evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }





% \section{Prompt Examples and Distributions}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/example-prompt.png}
%     \caption{Prompts}
%     \label{fig:app-prompts}
% \end{figure}




==> texs_/app-main.tex <==
% \section{Reproducibility Statement}\label{app:settings}

% \paragraph{Hyperparameter settings.} We follow the hyperparameter setting stated in~\citep{orpo,simpo,self-play-gu}, default to be:

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[h]
% \centering
% \resizebox{0.7\columnwidth}{!}{%
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
% learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
% learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
% $\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
% $\gamma$                                                      & /      & /      & 5      & /       \\
% $\lambda$                                                      & /      & 0.5      & /      & /       \\
% no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
% warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
% effective batch size                                          & 8      & 8      & 32     & 8       \\
% max length                                                    & 2048   & 2048   & 2048   & 1024    \\
% max prompt length                                             & 1024   & 1024   & 1800   & 512     \\
% optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
% \bottomrule
% \end{tabular}%
% }
% % \caption{Hyper}
% \label{tab:app-main-params}
% \end{table}


% \paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-rewarding}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
% \vspace{-5pt}
% \begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
%     \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
%     % \item ...
% \end{itemize}

% For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this as well as other plug-in evolving methods.

% % \paragraph{Computation environments.} 

% \paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve OpenAI models and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. In general, our codebase is very simple to use and requires only a creator module addition within the \href{https://github.com/huggingface/alignment-handbook}{Alignment Handbook} pipeline.

%  \paragraph{Code release.} We currently put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\textcolor{black}{\texttt{\small anonymous.4open.science/r/eva-i/}}}, which we intend to as well release all the source code there, and all the datasets and models to HuggingFace, upon approval -- before then, we are happy to provide any additional clarification requested to help re-implement~\method~and replicate our results. 

% \paragraph{Evaluation settings.} If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge, and \texttt{gpt-4-0314} as the baseline when calculating the win rate for evaluating on the benchmarks.





% -------------------------------------------------------------
\section{Issues of Fixed Prompt Training Distributions}\label{app:prompts}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/example-prompt.png}
    \caption{The initial prompt distribution of AlpacaEval (openly accessible on HuggingFace) obtained from zero-shot classification with \texttt{bart-large-mnli}, which is imbalanced. Additionally, looking at the reward distribution, the category with lowest average reward has the highest average reward gap (\ie our default informativeness proxy), implying the potential to improve.}
    \label{fig:app-prompts}
\end{figure}


% \paragraph{\emphtext{\method~minimally impact downstream tasks.}} 




% \section{Extended Discussions on Open-Ended Learning}

% The design of our game-theoretic framework is inspired from many prior works in open-ended learning, which we encourage the LLM community to explore more.  The central idea of open-ended learning is \emph{not} to optimize for a \emph{specific, static} distribution, but to develop an agent that \emph{generalize} well across \emph{unseen, novel} environments, which are the environments that the agent has not been explicitly trained on. To achieve this, unsupervised environment design proposes to generate environments that present a curriculum of \emph{increasing complexity} for the agent to evolve, which ensures that the agent's learning is not \emph{narrow}, but general enough to handle the diversity of complexity of future environments. In the curriculum, as the agent solves simpler environments, it moves on to more difficult ones, thus progressively build more sophisticated strategies. Furthermore, by adopting a \emph{minimax regret} framework, this approach adds a layer of robustness by minimizing the agent’s performance gap in worst-case environments. It is not just about generalizing to novel environments but also about ensuring that the agent can handle the most challenging scenarios within those environments. This distinction highlights the value of minimax regret: while classical open-ended learning focuses on generalization through exposure to diverse environments, minimax regret ensures that the agent is robust even under the most adversarial conditions.


% \begin{itemize}
%     \item \cite{poet}:
%     \item \cite{paired}: using two agents to simulate the regret.
%     \item \cite{plr}: having a rolling buffer of high-regret levels.
%     \item \cite{accel}:
%     \item \cite{open-endedness}
% \end{itemize}

% \paragraph{Self-improving / self-training language models.} 
\section{Additional Experimental Results}

In general,~\method~maintains the accuracy on downstream tasks and is robust on those reasoning-heavy tasks, and the scaling with reward models is more prominent on AlpacaEval, possibly due to the training sources for such reward models~\citep{armorm}.
\input{tables/tab-ab-downstream}
\vspace{-8pt}

\input{tables/tab-ab-rm-app}

\begin{table}[H]
\centering

\resizebox{.8\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{6}{c}{{\textsc{Llama-3.2-3B-instruct}}} \\ \cmidrule(l){2-7}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{1}{c}{\textbf{Arena-Hard}} & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-2} \cmidrule(l){3-5} \cmidrule(l){6-7}



\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{WR} (\%)      & \textbf{avg. score}   & $1^{\text{st}}$ turn  & $2^{\text{nd}}$ turn & \textbf{LC-WR} (\%) & \textbf{WR} (\%)  \\ \midrule

$\vtheta_0$: SFT                & 9.7  & 7.24 & 7.60 & 6.88 & 27.15 & 29.94 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 11.4  &7.28  & 7.67 & 6.88 & 28.32 & 32.17 \\


\rowcolor{green!10} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  +  \texttt{\textbf{eva}} } & \textbf{13.0} & \textbf{7.37} & \textbf{7.71} & \textbf{7.03} & \textbf{29.54}  & \textbf{33.68} \\ 

\rowcolor[HTML]{f5f7fc} 
\tgray{$\vtheta_{1 \rightarrow 2}$: \quad +   \texttt{new human prompts}}      & \tgray{}  & \tgray{} & \tgray{} & \tgray{} & \tgray{\textbf{}}  & \tgray{\textbf{}}  \\



\bottomrule

\end{tabular}%
}
\caption{\textbf{Results with \text{Llama} models.}.}
\label{tab:main-10k-llama}
\end{table}
\vspace{-10pt}


% -------------------------------------------------------------
% \section{Limitations}\label{app:limit}
% Off-policy is one concern. Another concern is that the advantage-based framework does not inherently works for general preference (we first do pairwise comparison; after )

% \subsection{The On-Polcy Variant: \texttt{eva-o}}\label{app:eva-o}
% The iterative training approach is inherently an off-policy algorithm; while being efficient, the performance can get plateau when more iterations goes on. We hereby show our method can easily extend to be on-policy, as shown in Algorithm~\ref{alg:o-eva}, that draws inspiration from Iterative Machine Teaching~\citep{bo-mt} and Ordered SGD~\citep{ordered-sgd} in the informative pool set selection (Line 4, which can be achieved either by greedy or through weighted sampling), while adding the new evolving step (Line 5). 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}(\vx_i)\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \texttt{evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }





% \section{Prompt Examples and Distributions}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/example-prompt.png}
%     \caption{Prompts}
%     \label{fig:app-prompts}
% \end{figure}




==> texs_/app-notes.tex <==
\section{Temporary Notes}



% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% DPO \ \hspace{+3pt} Iter 2 / 6       & 8.64 & 8.88 & 8.39 & on h100-west \textcolor{gray}{{\tiny CI: (, )}} &  & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{d6fcf9}  
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-greedy}) } & 8.72 & \textbf{9.06} & 8.36 & on a100-cc & & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-iw}) } & \\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-greedy}) } & \\ 

% \rowcolor[HTML]{e9ebee}
% Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% % IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% % \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% % \quad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% % \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:notes}
% \end{table}
% % --------------------------------------------------------
% \footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
% \footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}



% --------------------------------------------------------
\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule

\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

$\vtheta_0$: SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


\midrule

$\vtheta_{0 \rightarrow 1}$: DPO     & 8.66 & 9.01 & 8.32& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\




\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad  + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.90} & \textbf{9.04}& \textbf{8.75} & \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  55.35 &    55.53 \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

\rowcolor[HTML]{e2fbe2}  
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{eva-greedy} } & 8.72 & \textbf{9.06} & 8.36 & 59.5 \textcolor{gray}{{\tiny CI: (-2.5, 2.2)}} & 736 & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K  \texttt{subset-iw} } & 8.69 & 9.00 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{dcf5fb} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + \ \ 2K   \texttt{subset-greedy} } & 8.68 & 8.98 & 8.38 & /\ & /\ & /\ & /\ & /\ \\ 

\rowcolor[HTML]{e9ebee} 
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}      & 8.64 & 8.88 & 8.39 & 59.8 \textcolor{gray}{{\tiny CI: (-3.0, 1.9)}} & 733 & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\






\rowcolor[HTML]{e9ebee}
Offline DPO w/ 60K Prompts\footnotemark       & 8.78 &   9.22 &   8.53  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  \textbf{56.46} & \textbf{58.07} \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

\midrule

% IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% \rowcolor[HTML]{e2fbe2} 
% \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% \midrule




$\vtheta_{0 \rightarrow 1}$: SPPO \hspace{+2pt}       & 8.62 &  9.03 &  8.21 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \Tilde{1}}$: \text{\quad + 10K  \texttt{\textbf{eva-iw}} } & \textbf{8.78} & \textbf{9.11} &  \textbf{8.45} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 

\rowcolor[HTML]{e9ebee}
$\vtheta_{1 \rightarrow 2}$: \quad + 10K   \texttt{new human prompts}    &  8.64 &  8.90 &  8.39 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 & 51.78 & 42.98 \textcolor{gray}{\tiny $\pm$ 1.74} & 1692 \\

\midrule

$\vtheta_{0 \rightarrow 1}$: IPO      & 8.72 & 9.00 & 8.45 & 45.2 \textcolor{gray}{{\tiny CI: (-2.4, 2.5)}} & 587 & 52.02 & 45.43 \textcolor{gray}{\tiny $\pm$ 1.75} & 1726 \\

\rowcolor[HTML]{e2fbe2} 
$\vtheta_{1 \rightarrow \tilde{1}}$: \quad + 10K  \texttt{\textbf{eva-iw}}  &  &  &  &  &  & 52.94  & 52.67 \textcolor{gray}{\tiny $\pm$ 1.76} & 2054 \\ 


% \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% \midrule





\bottomrule

\end{tabular}%
}
\vspace{+5pt}
\caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:notes-1}
\end{table}
% --------------------------------------------------------
\footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
\footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}











\begin{table}[ht]
\centering

\vspace{+5pt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}
\textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

\textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & \textbf{avg. score}      & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

SFT                &  8.57 &  8.81 &  8.32 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\

DPO + NLL$_{\text{LC}}$ \  \hspace{+3pt}   Iter 1 / 3    & 8.73 & 9.18 & 8.28 & 53.2 \textcolor{gray}{{\tiny CI: (-2.2, 3.2)}}  & 625 & 53.48 & 48.70 \textcolor{gray}{\tiny $\pm$ 1.76} & 1824 \\

\qquad \qquad \qquad \ \ \ \hspace{+1pt} Iter 2 / 3      &  8.75  & 9.25 & 8.24 & 47.0 \textcolor{gray}{{\tiny CI: (-2.0, 2.7)}} & 601 & 52.57 & 46.76 \textcolor{gray}{\tiny $\pm$ 1.76} & 1729   \\

\qquad \qquad \qquad \ \ \  \hspace{+1pt} Iter 3 / 3       & 8.66 & 9.13 & 8.19 & 46.8 \textcolor{gray}{{\tiny CI: (-2.2, 2.2)}} & 564 & 53.50 & 46.02 \textcolor{gray}{\tiny $\pm$ 1.76} & 1673  \\

\rowcolor[HTML]{e2fbe2} 
\text{DPO + NLL$_{\text{LC}}$  \  \hspace{+3pt}   Iter 1 / 3 (\texttt{eva-p}) } & \textbf{8.81} & 9.11 & \textbf{8.51} & \textbf{55.3} \textcolor{gray}{{\tiny CI: (-2.2, 2.4)}} &  871 & 52.37  &   52.92 \textcolor{gray}{\tiny $\pm$ 1.76} & 2300 \\ 

\bottomrule

\end{tabular}%
}
\vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
\label{tab:rpo}
\end{table}
% --------------------------------------------------------

% \begin{align}
%     \mathcal{L}_{\mathrm{DPO}+\mathrm{NLL}^{\mathrm{LC}}}\left(\pi_\vtheta ; \pi_{\text {\text{ref}}}\right)=-\mathbb{E}_{\left(\rvx, \rvy_{+}, \rvy_{-}\right) \sim \mathcal{D}}\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text {ref}}\left(\rvy_{+} \mid \rvx\right)}-\beta \log \frac{\pi_\vtheta\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text {ref}}\left(\rvy_{-} \mid \rvx\right)}\right)\right] - \alpha \frac{\log \pi_{\vtheta}(\rvy_{+} \mid \rvx)}{|\rvy_{+}|}. \nonumber
% \end{align}


\begin{minipage}{\linewidth}

\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{DPO}+\mathrm{NLL}_{\mathrm{LC}}}(\pi_\vtheta ; \pi_{\text{ref}}) = 
-\mathbb{E}
&\left[\log \sigma\left(\beta \log \frac{\pi_\vtheta(\rvy_{+} \mid \rvx)}{\pi_{\text{ref}}(\rvy_{+} \mid \rvx)}
-\beta \log \frac{\pi_\vtheta(\rvy_{-} \mid \rvx)}{\pi_{\text{ref}}(\rvy_{-} \mid \rvx)}\right)\right]- \alpha \frac{\log \pi_{\vtheta}(\rvy_{+} \mid \rvx)}{|\rvy_{+}|}. \nonumber
\end{split}
\end{equation}
\end{minipage}


% -------------------------------------------------------------
\subsubsection{The Effect of Different Initialization}\label{sec:ab-init}
\notes{This subsection can be put in the appendix section. In all our current setting, we start with a DPO checkpoint. We can test starting with the SFT checkpoint, and one-round BoN SFT checkpoint.}
\input{tables/tab-ab-init}
% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{Performance on the Downstream Tasks}\label{sec:ab-downstream}
% \input{tables/tab-ab-downstream}
% % -------------------------------------------------------------

\subsubsection{Other Preference Optimization Methods: BoN Finetuning and RLOO}\label{sec:ab-optim}
While in this work we focus on direct preference optimization, we also add ablation for other methods.
% In this section, we attempt the simplest setting. Instead of using contrastive methods like DPO, we directly use the chosen (\ie the response that achieves the best reward for each prompt)  


% \subsubsection{The Effect of Difficulty Aware Sampling}
% \notes{The idea is straightforward. For harder prompts, we just sample more responses. This is another way to utilize our informativeness metric, and making the response sampling more \emph{adaptive}.}

% % -------------------------------------------------------------
% \subsubsection{The Effect of Different Early Stopping Criteria}\label{sec:ab-stop}
% \notes{This subsection can be put in the appendix section.}
% \input{tables/tab-ab-stop}
% % -------------------------------------------------------------
% This is orthogonal to our contribution. Putting here just as a reference for tuning model performance in the later stages.


% \paragraph{Iterative training scheduling.} The base experiments test performance in one iteration. We now consider iterative training. Specifically, we define the models and the training data they use as follows:\begin{itemize}
%     \item $\vtheta_0$ : Base SFT model.
%     \item $\vtheta_1$ : init with $\vtheta_0$; trained w/ the $1^{\text{st}}$ prompt split $D_1$ by self-generated responses.
%     \item $\vtheta_2$ : init with $\vtheta_1$; trained w/ the $2^{\text{st}}$ prompt split $D_2$ via by self-generated responses.
%     \item ...
% \end{itemize}


% \paragraph{Self-rewarding mechanism.} In the base experiments, we assume preference comes from an external preference oracle. Following the setting of~\citep{self-reward}, we finetune the model for reward generation, then use the generated reward to replace the preference oracle for reward annotation.

% # saturated benchmark


























% % --------------------------------------------------------
% \begin{table}[ht]
% \centering

% \vspace{+5pt}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule

% \textbf{Model Family ($\rightarrow$)}          & \multicolumn{8}{c}{{\textsc{gemma-2-9b-it}}} \\ \cmidrule(l){2-9}

% \textbf{Benchmark ($\rightarrow$)}           & \multicolumn{3}{c}{\textbf{MT-Bench}} & \multicolumn{2}{c}{\textbf{Arena-Hard}} &\multicolumn{3}{c}{\textbf{AlpacaEval 2.0}}\\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-9}

% \textbf{Method ($\downarrow$) / Metric ($\rightarrow$)} & $1^{\text{st}}$ turn   & $2^{\text{nd}}$ turn  & \textbf{avg. score}      & \textbf{score} (\%)  & avg. len     & \textbf{LC} (\%) & \textbf{WR} (\%) &  avg. len    \\ \midrule

% SFT                &  8.81 &  8.32 &  8.57 &  41.3 \textcolor{gray}{{\tiny CI: (-2.6, 2.6)}} & 544 &  47.11 & 38.39 \textcolor{gray}{\tiny $\pm$ 1.71} & 1567 \\


% \midrule

% DPO \ \hspace{+3pt} Iter 1 / 6       & 9.01 & 8.32& 8.66& 51.6 \textcolor{gray}{{\tiny CI: (-2.5, 2.0)}} & 651 & 55.01 & 51.68 \textcolor{gray}{\tiny $\pm$ 1.76} & 1883  \\

% DPO \ \hspace{+3pt} Iter 2 / 6       & 8.88 & 8.39 & 8.64 & on h100-west \textcolor{gray}{{\tiny CI: (, )}} &  & 55.74 & 56.15 \textcolor{gray}{\tiny $\pm$ 1.75} & 2111  \\

% \rowcolor[HTML]{e2fbe2} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  \textbf{9.04}& \textbf{8.75} & \textbf{8.90}& \textbf{60.1} \textcolor{gray}{{\tiny CI: (-2.8, 2.3)}} &  725 &  \textbf{55.35} &    \textbf{55.53} \textcolor{gray}{\tiny $\pm$ 1.75} & 2089 \\ 

% \rowcolor[HTML]{d6fcf9}  
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{eva-greedy}) } & \textbf{9.06} & 8.36 & 8.72 & on a100-cc & & 54.52 & 55.22 \textcolor{gray}{\tiny $\pm$ 1.75} & 2091\\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-iw}) } & \\ 

% \rowcolor[HTML]{f6ebfd} 
% \text{DPO \ \hspace{+3pt}  Iter 1 / 6 (\texttt{subset-greedy}) } & \\ 

% \rowcolor[HTML]{e9ebee}
% Offline DPO w/ 60K Prompts\footnotemark       &   9.22 &   8.53 & 8.78  & 58.9\footnotemark  \textcolor{gray}{{\tiny CI: (-n/a, n/a)}} & 717 &  56.46 & 58.07 \textcolor{gray}{\tiny $\pm$ 1.74} &  2245 \\

% \midrule

% % IPO \ \hspace{+8pt}   Iter 1 / 6   &  8.58 &  8.36 &  8.47& \\

% % \rowcolor[HTML]{e2fbe2} 
% % \text{IPO  \ \hspace{+8pt}  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  8.74 & 8.31 &  8.53 &  &  &  &  & \\ 
% % \midrule


% SimPO Iter 1 / 6       &    \\

% \rowcolor[HTML]{e2fbe2} 
% \text{SimPO  Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } &  &  &   &  &  &  &  & \\ 

% \midrule

% SPPO \hspace{+2pt}  Iter 1 / 6      &  9.03 &  8.21 &  8.62 &  55.7 \textcolor{gray}{{\tiny CI: (-3.1, 1.9)}} & 560 & 51.58 & 42.17 \textcolor{gray}{\tiny $\pm$ 1.74} & 1636 \\

% % \quad \ \ \ \hspace{+1pt} Iter 2 / 6       &  8.90 &  8.39 &  8.64 &  57.7 \textcolor{gray}{{\tiny CI: (-2.3, 2.2)}} & 562 &   \\
% % \quad \ \ \  \hspace{+1pt} Iter 3 / 6       &  8.65 &  8.20 &  8.43 &  57.7 \textcolor{gray}{{\tiny CI: (-2.2, 2.5)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 4 / 6        &  8.95 &  8.38 &  8.66 &  57.5 \textcolor{gray}{{\tiny CI: (-2.4, 1.9)}} & 567 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 5 / 6      &  8.88 &  8.29 &  8.58 &  56.8 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 573 &  \\
% % \quad \ \ \  \hspace{+1pt} Iter 6 / 6       &  9.04 &  8.41 &  8.73 &  56.4 \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 582 &  \\

% % \midrule
% \rowcolor[HTML]{e2fbe2} 
% \text{SPPO \hspace{+2pt} Iter 1 / 6 (\texttt{\textbf{eva-iw}}) } & \textbf{9.11} &  \textbf{8.45} &  \textbf{8.78} &  \textbf{58.9} \textcolor{gray}{{\tiny CI: (-1.9, 1.9)}} & 567 & \textbf{51.86} & \textbf{43.04} \textcolor{gray}{\tiny $\pm$ 1.75} & 1665 \\ 


% \bottomrule

% \end{tabular}%
% }
% \vspace{+5pt}
% \caption{\textbf{Performance.} Evaluation results on general instruction-following alignment benchmarks.}
% \label{tab:notes}
% \end{table}
% % --------------------------------------------------------
% \footnotetext{We currently use the released model from \href{https://huggingface.co/princeton-nlp/gemma-2-9b-it-DPO}{\texttt{princeton-nlp/gemma-2-9b-it-DPO}}, which is trained from \href{https://huggingface.co/datasets/princeton-nlp/gemma2-ultrafeedback-armorm}{\texttt{princeton-nlp/gemma2-ultrafeedback-armorm}}.}
% \footnotetext{This number is directly taken from the reported result on this model's HuggingFace Page.}


==> texs_/app-settings.tex <==
\paragraph{Code release.} At the moment, we put supplementary materials and additional experiment results on \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}, where we intend to release all the source code there, and all the datasets (generated prompts and responses) and models (with other models beyond the current model family) \emph{anonymously} to HuggingFace, \text{upon approval} -- before then, we are happy to provide any clarification requested to help re-implement~\method~and replicate our results. 

In general, our codebase is made to be simple to use for practitioners, requiring \textbf{only a creator module addition} within the commonly adopted \href{https://github.com/huggingface/alignment-handbook}{\tb{\text{Alignment Handbook}}} pipeline.

\paragraph{Hyperparameter settings.} We follow the original hyperparameter settings as in~\citep{orpo,simpo,self-play-gu}, default to be:

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Hyperparameter ($\downarrow$) / Loss ($\rightarrow$)} & \textbf{DPO}    & \textbf{ORPO}    & \textbf{SimPO}  & \textbf{SPPO}     \\ \midrule
learning rate                                                 & 5e-7   & 5e-7   & 8e-7   & 5e-7    \\
learning rate scheduler                                       & cosine & cosine & cosine & linear  \\
$\beta$                                                       & 0.05   & /    & 10     & 0.001   \\
$\gamma$                                                      & /      & /      & 5      & /       \\
$\lambda$                                                      & /      & 0.5      & /      & /       \\
no. epochs per iter                                           & 2      & 1      & 1      & 6       \\
warmup ratio per iter                                         & 0.1    & 0.1    & 0.1    & 0.1     \\
effective batch size                                          & 8      & 8      & 32     & 8       \\
max length                                                    & 2048   & 2048   & 2048   & 1024    \\
max prompt length                                             & 1024   & 1024   & 1024   & 512     \\
optimizer                                                     & adamw  & adamw  & adamw  & rmsprop \\ 
\bottomrule
\end{tabular}%
}
% \caption{Hyper}
\label{tab:app-main-params}
\end{table}


\paragraph{Iterative Training Settings.} By default~\citep{snorkel,self-reward}, we train with equal-size prompt subset in each iteration. Unless otherwise specified, we use 10K prompts from the UltraFeedback dataset~\citep{ultrafeedback} per iteration. The incremental training proceeds as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\vtheta_0$ : Base SFT model.
    \item $\vtheta_{0 \rightarrow 1}$ : initialize with $\vtheta_0$; then train with the prompt split $\calX_1$ by self-generated responses from the initial model $\vtheta_0$.
    \item $\vtheta_{1 \rightarrow 2}$ : initialize with $\vtheta_{0 \rightarrow 1}$; trained with the prompt split $\calX_2$ via by self-generated responses from the initial model $\vtheta_{0 \rightarrow 1}$.
    % \item ...
\end{itemize}

For evolving prompts (\eg evolving $\calX_1$ to $\calX_{\tilde{1}}$), with the calculated informativeness metric for each prompt, we normalize them as the weight to do weighted sampling for a 25\% informative subset to get $\calX_1^{\texttt{\tiny info}}$. We then iterate over in $\calX_1^{\texttt{\tiny info}}$ and call \texttt{\small EvolInstrut}~\citep{wizardlm} as the plug-in evolving method (with the number of evolutions as 4) using the default mutation templates for (i) in-depth evolving  (\text{constraints}, \text{deepening}, \text{concretizing}, \text{increased reasoning steps}) and (ii) in-breadth evolving (extrapolation) as implemented in \href{https://github.com/argilla-io/distilabel/blob/main/src/distilabel/steps/tasks/evol_instruct/utils.py#L36}{\tb{\texttt{\small tasks/evol\_instruct/utils.py}}} of \texttt{\small distilabel==1.3.2}. Next we uniformly select $80\%$ prompts from this evolved dataset and $20\%$ from the original dataset (\ie the buffer) to form $\calX_{\tilde{1}}$. We do not seek extensive parameter search (\eg the number of evolutions, the evolving ratio) in this stage and encourage future works on exploring this and other plug-in evolving methods. For solver we generate 6 responses per prompt.

% \paragraph{Computation environments.} 

\paragraph{Software environments.} All our experiments are conducted on 8xNVIDIA H100 SXM GPUs. Our codebase primarily relies on \texttt{\small transformers==4.40.0}. For the response generation of \textsc{Gemma} models at the training stage, we use \texttt{\small vllm==0.5.4} with \texttt{\small flashinfer} backend for \texttt{\small CUDA 12.4} and \texttt{\small torch 2.4}.  For evolving prompts, we use \texttt{\small distilabel==1.3.2}, and use \texttt{\small LiteLLM} to serve Gemini, OpenAI (default to be \texttt{\small gpt-4o-mini}) and transformers models. For evaluation on all benchmarks, we use \texttt{\small sglang==0.2.10} and \texttt{\small openai==1.35.14}, with \texttt{\small gpt-4-1106-preview} as the judge model and \texttt{\small gpt-4-0314-preview} as the baseline model. Specifically for AlpacaEval 2.0, we use \texttt{\small alpaca\_eval\_gpt4\_turbo\_fn} as the annotator config. We use 42 as the random seed.

% We include main Appendix following references, also in \href{https://anonymous.4open.science/r/eva-i/}{\text{\texttt{\small anonymous.4open.science/r/eva-i/}}}.

==> texs_/conclusion-ckpt.tex <==
% \newpage
\section{\textcolor{Gray}{[Draft]} Conclusions, Limitations and Future Works}

\notes{Scratchpad. To refine later.}

\paragraph{Conclusions.} The primary implication of our work is: ....

Most post-training algorithms only consider how to provide a good answer (y | x); few consider how to teach the model to ask the right question (x). But an important property of intelligence is to actively ask questions.

This also brings a new perspective of ``generative'' exploration for RLHF, in the sense that we actively generate states for exploration and exploitation, which is typically undoable in classical contextual bandits and RL.

While \texttt{eva} standalone is self-contained, we also bring new perspective in classical literature. 
\begin{itemize}
    \item Compared to the self-training literature: (we are the first to self-training by jointly optimization $(\calX, \calY)$)
    \item Compared to the self-instruct literature: (we are the first to apply the method with contrastive preference optimization, and we also propose a new data selection metric.)
    \item Compared to the curriculum learning literature: (we incorporate generative data augmentation, instead of purely re-ordering the learning sequence.)
\end{itemize}

% Perhaps the primary implication of our work is: 

% Write some philosophical bits on robust, open-ended, sample efficient superintelligence.

% Write concrete future directions for people to follow based on our general framework.


\textbf{Limitation and future direction.}
\begin{itemize}
    \item Make the creator policy differentiable.
    \item Adding self-reward generation.
    \item Applying the method in reasoning tasks (combining with RPO~\citep{rpo}). 
    \begin{itemize}
        \item One way is on directly generating new problems or conjectures. 
        \item We may also combine with MCTS (add the theorem proving and auto conjecturing lines of work).
    \end{itemize}
    
    \item consider more players in the loop, \eg~the critic, the re-writer.
    \item extending to multi-turn.
    \item adding exploration bonus for diversity and coverage. (to cite the recent few papers on coverage guarantee.)
    \item explore more use of advantage function with other anchors
\end{itemize}

\notes{Some figures/tables to include in the main paper: prompt distribution (coverage and difficulty); also add the bar plot. and a pipeline, just like the self-rewarding paper.)}

% comparison with existing works (compared to rest-like paper, our generation happens in the joint space of x|y; compared to the self-instruct-like paper, our optimization is on contrastive optimization, instead of finetuning; we also have a specific data selection criteria; compared to curriculum learning paper, our data has generative augmentation, instead of purely re-ordering. 

\newpage

==> texs_/conclusion.tex <==
% \newpage
\section{Concluding Remarks}\label{sec:conclusion}
\vspace{-4pt}


% \vspace{-2pt}





% Perhaps the primary implication of our work is: 

% Write some philosophical bits on robust, open-ended, sample efficient superintelligence.

% Write concrete future directions for people to follow based on our general framework.

% also discuss the challenge of the evolving methods in the appendix

\textbf{Limitations and future directions.}
\ \ \method~defines a new paradigm for alignment, opening up many new directions, \eg (i) extending to differentiable creator policies, combining w/ other $\texttt{\small evolve}(\cdot)$ methods; (ii) evolving for more iterations w/ on-policy solvers like RLOO~\citep{rloo}; (iii) investigating exploration bonuses for distribution diversity and coverage, and the self-consuming loop~\citep{collapse}; (iv) extending the game with more players for full automation (\eg rewarders, critics, rewriters, verifiers, retrievers); (v) extending from alignment to reasoning (\eg auto-conjecturing for theorem proving~\citep{math-conjecture} can be cast as an asymmetric game), or from the bandits to the trajectories w/ process reward models and hierarchical tree search for creator and solver generations;  (vii) further scaling up w/ million-level prompts for post-training.
\vspace{-6pt}

% \paragraph{Conclusions.} \method~is a new and simple framework for aligning language models. We introduce the concept of open-ended RLHF, which seeks to jointly optimize the prompt distribution and the response
% policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks
% beyond the initial training prompt distribution for alignment. Our~\method~presents a practical algorithm by framing it as an asymmetric  game between a creator generating \emph{new \emph{and} learnable} prompts, quantified by our effective, regret-inspired informativeness metric, and a solver producing preferred responses. \method~can be easily plugged into any existing alignment pipeline, and shows universally strong gains with four preference optimization algorithms in public benchmarks. 
\paragraph{Conclusions.} \method~is a new, simple and scalable framework for aligning language models, and can be plugged into any existing alignment pipeline. The primary takeaway may be that RLHF can be made open-ended: (i) self-evolving joint data distributions can bring significant gain (as shown across various optimization algorithms), and (ii) reward advantage acts as an effective metric informing the collection and creation of \emph{future} prompts for alignment. \method~presents a new view of alignment by framing it as an asymmetric  game between a creator generating \emph{new \emph{and} learnable} prompts and a solver producing preferred responses. \method~also \emph{incentivizes agents to create problems} rather than to simply \emph{solve problems}, which is a key feature of intelligence, yet model trainers often neglect.
\vspace{+2pt}
\vspace{+2pt}


% First, making the creator policy differentiable could potentially lead to more efficient and effective prompt generation. Extending \method~to multi-turn interactions and exploring its application in reasoning tasks, possibly in combination with techniques like Monte Carlo Tree Search, could broaden its impact. Additionally, investigating the integration of exploration bonuses for diversity and coverage, as well as expanding the multi-agent framework for more players (\eg critics, rewriters, verifiers, retrievers) can lead to more robust self-improvement.

% \notes{Mention applying this in math or theorem proving. A particularly interesting one is~\citep{math-conjecture}, which conjectures and proves at the same time, just like our creator-solver game.}

% \notes{Limitation: (i) continuously evolving for more iterations, if resources permitted; (ii) other RLHF methods like PPO (in this work we focus on direct preference optimization) (iii) still we rely on a reward model - so two more directions - self-rewarding / using human preferences in an efficient way. (iv) we could add an additional data filtering process as done in~\citep{plr,accel} instead of uniformly using the evolved data for better precision. }


% \fix{reliance on external reward model - should be self-rewarding }
% \vspace{+5pt}
%Finally, further exploration of advantage functions with various anchors may yield additional insights into optimizing the alignment process.

% comparison with existing works (compared to rest-like paper, our generation happens in the joint space of x|y; compared to the self-instruct-like paper, our optimization is on contrastive optimization, instead of finetuning; we also have a specific data selection criteria; compared to curriculum learning paper, our data has generative augmentation, instead of purely re-ordering. 

\newpage

==> texs_/exp-fix.tex <==

\section{Experiments}\label{sec:exp}
% In this section, we present main results of our experiments, showing the remarkable performance gain from the additional creator step in~\method~on various benchmarks.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/arena-hard.png}
%         \caption{Caption for Arena Hard}
%         \label{fig:arena-hard}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/mt-bench.png}
%         \caption{Caption for MT Bench}
%         \label{fig:mt-bench}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/alpaca-eval.png}
%         \caption{Caption for Alpaca Eval}
%         \label{fig:alpaca-eval}
%     \end{subfigure}
%     \caption{Overall caption for the three figures}
%     \label{fig:three-figures}
% \end{figure} 


% \subsection{Experimental Settings}
\paragraph{Datasets and models for training.} We use  \textbf{UltraFeedback}~\citep{ultrafeedback} as the training dataset, which contains diverse high-quality prompts that are primarily human-generated. %Note that UltraFeedback contains some machine-generated prompts; however, it is primarily composed of high-quality human prompts (\eg~\cite{truthfulqa,sharegpt}), thus we use the shorthand notation.})
We use the instruction-finetuned \textsc{Gemma-2-9B}~\citep{gemma2} as the primary model, which is a strong baseline for models of its size.   Detailed experimental setting can be found in $\S$~\ref{app:reproduce}.

% \footnote{More models may be found in the anonymous repo: \href{https://anonymous.4open.science/r/eva-i/}{\textcolor{black}{\texttt{\small anonymous.4open.science/r/eva-i.}}}}

% and \textsc{Llama-3.1-8B}~\citep{llama3} 

% (\href{https://github.com/thunlp/UltraChat}{UltraChat}, \href{https://huggingface.co/datasets/RyokoAI/ShareGPT52K}{ShareGPT}, \href{https://github.com/nlpxucan/WizardLM}{Evol-Instruct}, \href{https://huggingface.co/datasets/truthfulqa/truthful_qa?row=10}{TruthfulQA}, \href{https://github.com/thunlp/FalseQA}{FalseQA}, and \href{https://huggingface.co/datasets/Muennighoff/flan}{FLAN})

% This dataset focuses on (i) instruction-following, (ii) truthfulness; (iii) honesty; and (iv) helpfulness.

% Each prompt is paired with 4 responses generated by different language models, where each response is rated from 1 to 5 according to the five dimensions by GPT-4.

\paragraph{Evaluation settings.} We choose:   (i) \textbf{AlpacaEval 2.0}~\citep{ae}, which assesses general instruction following with 805 questions; (ii) \textbf{MT-Bench}~\citep{llm-judge}, which evaluates multi-turn instruction following with 80 hard questions in 8 categories; (iii) \textbf{Arena-Hard}~\citep{ah}, which is derived from 200K user queries on Chatbot Arena with 500 challenging prompts across 250 topics.  We use \texttt{\small gpt-4-1106} as the judge and \texttt{\small gpt-4-0314} as the baseline for win rate.


% \vspace{-5pt}
% \begin{itemize}
% \item \textbf{MT-Bench}: This dataset evaluates multi-turn conversation and instruction-following. It contains 80 questions across 8 categories.\vspace{-0pt}
% \item \textbf{Arena-Hard}: This dataset is derived from 200K user queries on Chatbot Arena. It contains 500 high-quality  technical problem-solving prompts across 250 topics. \vspace{-0pt}
% \item \textbf{AlpacaEval 2.0}: This dataset assesses general instruction-following ability, and includes 805 questions from 5 datasets covering various tasks like creating, generating, and explaining.\vspace{-0pt}
% \end{itemize}

% \paragraph{Evaluation benchmarks.} We consider the following evaluation benchmarks\footnote{If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge model, and \texttt{gpt-4-0314} as the baseline model when calculating the win rate.}:
% % \vspace{-5pt}
% \begin{itemize}
% \item \textbf{MT-Bench}: This dataset evaluates multi-turn conversation and instruction-following. It contains 80 questions across 8 categories: writing, roleplay, extraction, reasoning, math, coding, STEM knowledge, humanities and social sciences knowledge.\vspace{-0pt}
% \item \textbf{Arena-Hard}: This dataset is derived from 200K user queries on Chatbot Arena. It contains 500 high-quality  technical problem-solving prompts across 250 topics. \vspace{-0pt}
% \item \textbf{AlpacaEval 2.0}: This dataset assesses general instruction-following ability, and includes 805 questions from 5 datasets covering various tasks like creating, generating, and explaining.\vspace{-0pt}
% \end{itemize}

% The benchmarks described below evaluate the  human preference on \emph{general} conversational ability and commonsense generation from language models by subjecting them to inquiries spanning multiple domains. All of them use external large language models as the judge to cheaply approximate human preferences.

% \begin{itemize}
%     \item  \href{https://arxiv.org/pdf/2306.05685}{\textbf{MT-Bench}}: This dataset focuses on the evaluation of (i) multi-turn conversation and (ii) instruction-following abilities of language models. It includes eight categories: (i) writing, (ii) roleplay, (iii) extraction, (iv) reasoning, (v) math, (vi) coding, (vii) knowledge I (STEM), and (viii) knowledge II (humanities / social sciences); each category features 10 carefully designed multi-turn questions, contributing to a total of 80 questions.
%     \item \href{https://tatsu-lab.github.io/alpaca_eval/}{\textbf{Alpaca-Eval}}. This dataset focuses on the evaluation of general instruction-following ability. It is built upon the 52K machine-generated instruction dataset~\citep{alpacafarm}, asking the language model to create, generate, suggest, design, construct, make, identify, calculate, convert, find, name, provide, summarize, classify, describe, edit, give, explain, write and re-write things\footnote{\href{https://github.com/tatsu-lab/stanford\_alpaca?tab=readme-ov-file\#data-generation-process}{\texttt{https://github.com/tatsu-lab/stanford\_alpaca}.}}. It consists of 805 questions from 5 datasets in total.
%     \item \href{https://lmsys.org/blog/2024-04-19-arena-hard/}{\textbf{Arena-Hard}}. Based on 200K diverse user queries collected via \href{https://arena.lmsys.org/}{Chatbot Arena}, the authors first cluster them into over 4K topics, then filter out low-quality prompts according to criteria including (i) complexity, (ii) creativity, (iii) technical accuracy, (iv) domain knowledge, (v) real-world application, (vi) specificity and (vii) problem solving. The resulting dataset contains 250 high-quality topic, where each topic corresponds to 2 randomly sampled prompts, contributing to 500 well-defined, technical problem-solving queries\footnote{\href{https://huggingface.co/spaces/lmsys/arena-hard-browser}{\texttt{https://huggingface.co/spaces/lmsys/arena-hard-browser}.}}. We use \texttt{gpt-4-1106-preview} as the judge model, and \texttt{gpt-4-0314} as the baseline model.
% \end{itemize}



 

 

 % We present a verbose review on existing preference optimization algorithms in Appendix~\ref{app:table}.
 % We consider DPO~\citep{dpo} as the default optimization algorithms, with ab

\paragraph{Optimization algorithms.} We focus on direct preference optimization and consider the following:
\vspace{-4pt}
\begin{itemize}
    \item \textbf{With reference policy}: DPO~\citep{dpo}, SPPO~\citep{self-play-gu}.\vspace{-1pt}
    \item \textbf{Without reference policy}: SimPO~\citep{simpo}, ORPO~\citep{orpo}.\vspace{-1pt}
\end{itemize}

\paragraph{Reward models as preference oracles.} We use \textsc{ArmoRM-8B}~\citep{armorm} as our default reward model as the human-preference proxy, and consider the following for ablation studies:
\vspace{-4pt}
\begin{itemize}
    \item \textbf{Pointwise}: \textsc{ArmoRM-8B}~\citep{armorm}, \textsc{SkyworkRM-27B}~\citep{skyworkrm}.\vspace{-1pt}
    \item \textbf{Pairwise}: \textsc{PairRM-0.4B}~\citep{pairrm}, \textsc{PairRM-8B}~\citep{pairrm8b}.\vspace{-1pt}
\end{itemize}

\subsection{Main Results}
\label{sec:main_results}
% For iterative training, we split the training set into equal-size partition and use one partition per iteration.


In general, \method~brings notable gains in alignment without relying on any human-crafted data, thus offering more efficiency. In the base setup, building on the one-iteration finetuned model ($\vtheta_{0 \rightarrow 1}$), \method~adds a creator to self-evolve the prompt set of the initial iteration and uses any preference optimization algorithm  for an additional open-ended RLHF iteration, resulting in  $\vtheta_{1 \rightarrow \tilde{1}}$\footnote{Unless stated otherwise, each iteration uses 10K prompts (\ie 1/6 partition from UltraFeedback in classical training). We denote $\vtheta_{t \rightarrow t+1}$ as the model trained with new human prompts based on the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the model trained with evolved prompts from the $t$-th checkpoint w/o adding any new human prompts.}.

% \footnotetext{We observe that the performance improvement in AlpacaEval is less pronounced compared to Arena-Hard, which may be due to the focus of~\method~on the most informative prompts; we encourage future works to explore effective coverage and diversity constraints into prompt generation to bring further gain.}
% \subsubsection{\textnormal{\textbf{\texttt{eva-i}}}: Main Results with the Iterative Training Setting}
\vspace{-3pt}
\paragraph{\method~achieves self-improvement.}  As shown in red rows in Table~\ref{tab:main-10k}, \method~yields notable performance improvement over $\vtheta_{0 \rightarrow 1}$ across different optimization algorithms, especially on the harder Arena-Hard benchmark, which is recognized to be more challenging and distinguishable among others due to the complexity of its prompts and its fairer scoring system~\citep{ah,simpo}. Specifically, \method~brings $8.4\%$ gain with SimPO as the solver, and $8.5\%$ gain with DPO as the solver, surpassing its 27B version and matching \texttt{\small claude-3-opus-240229} as reported on the \href{https://github.com/lm-sys/arena-hard-auto/tree/efc012e192b88024a5203f5a28ec8fc0342946df?tab=readme-ov-file#full-leaderboard-updated-0831}{\textcolor{gblue}{AH leaderboard}}, while using fully self-automated prompt generation for alignment. Interestingly, \method~brings the least gains on AlpacaEval 2.0, a simpler evaluation benchmark. This indicates \method~improves the most for challenging tasks.
% \notes{Also add one sentence saying that eva notably improves the performance on the second-turn results of MT-bench, without being explicitly trained for them. We conjecture that the self-discovered hard prompts by eva might include such property (\eg asking follow-up questions), and thus eva improves the performance by reinforcing those prompts.}
\vspace{-3pt}
\paragraph{\method~can surpass human-crafted prompts.}  We further show that \method-prompt-trained models ($\vtheta_{1 \rightarrow \tilde{1}}$) can match and even outperform those trained on additional new prompts from UltraFeedback ($\vtheta_{1 \rightarrow 2}$) (which we denoted as human prompts), while being much cheaper and more efficient. Additionally, on MT-Bench, training with new human prompts typically show decreased performance in the first turn and only modest gains in the second turn. In contrast,~\method~notably enhances second-turn performance. We hypothesize that~\method~evolves novel, learnable prompts that include characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions.
\input{tables/tab-main-10k}
% Additionally, on MT-Bench, we found that human prompts generally exhibit performance recession in first turn with modest gain in the second turn -- \method~fixes this while remarkably improves the second-turn performance without explicit training for it; we hypothesize that the novel, learnable prompts evolved from~\method~may incorporate characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions more effectively.


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: Main Results with the Online Training Setting}
% \input{tables/tab-main-10k-o}

% \subsection{Subsections}





% -------------------------------------------------------------


% \newpage
\vspace{-10pt}
\subsection{Ablation Studies}
% \notes{For now, we use tables to record results. We can shift to other illustrations later (\eg performance plot, pareto circle, prompt distribution w.r.t. metric, etc).}
We conduct in-depth ablation studies on \texttt{\textbf{eva}}, with findings below to be elaborated on later: 

% \setlength{\leftmargini}{9pt}
\vspace{-4pt}
\begin{itemize}
    \item $\S$~\ref{sec:ab-metric} - \textbf{informativeness metric}: our \emph{regret}-based metric outperforms other alternatives.
    \item $\S$~\ref{sec:ab-procedure} - \textbf{sample-then-evolve procedure}: our method outperforms greedy selection.
    \item $\S$~\ref{sec:ab-rm} - \textbf{scaling w/ reward models}: the alignment gain of~\method~scales with reward models.
    \item $\S$~\ref{sec:ab-cont} - \textbf{continual training }: our method has monotonic gain with incremental training;  the \emph{evolved data and schedule} by~\method~serves as an \emph{implicit regularizer} for better local minima.
\end{itemize}
\vspace{-4pt}
% In the appendix, we show~\method~has little performance regression on a range of downstream tasks.

% \footnotetext{Some works~\citep{active-pl,plr} considered Shannon entropy, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage future studies into this.}

% incremental training with informative prompts is comparable to scratch training, and outperforms incremental training with raw prompts from the wild world, effective serving as a regularizer for better local minima. \notes{to revise later}

% \method~can bring monotonic gain


% (i) \textbf{informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives. (ii) \textbf{scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method. (iii) \textbf{continual training schedule}: incremental training with informative prompts is comparable to scratch training, and outperforms incremental training with raw prompts from the wild world, effective serving as a regularizer for better local minima. 
% \begin{itemize}
%     \item \textbf{Informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives.\vspace{-2pt}
%     \item \textbf{Scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method.\vspace{-2pt}
%     \item \textbf{Continual training schedule}: incremental training with informative prompts can be comparable to scratch training, effective serving as a regularizer.  \vspace{-2pt}
%     % \item \textbf{Iterative evolving schedule}: we can obtain monotonic gain from iterative evolving.\vspace{-0pt}
%     % \item \textbf{Base creator LLMs}: self-instruct is effective, and we can benefit from stronger LLMs.\vspace{-0pt}
%     % \item number of examples per iteration
% \end{itemize}

% We conduct serveral ablation studies on \texttt{\textbf{eva-i}}, with the following findings:\vspace{-5pt}
% \begin{itemize}
%     \item \textbf{Informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives.\vspace{-2pt}
%     \item \textbf{Scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method.\vspace{-2pt}
%     \item \textbf{Continual training schedule}: incremental training with informative prompts can be comparable to scratch training, effective serving as a regularizer.  \vspace{-2pt}
%     % \item \textbf{Iterative evolving schedule}: we can obtain monotonic gain from iterative evolving.\vspace{-0pt}
%     % \item \textbf{Base creator LLMs}: self-instruct is effective, and we can benefit from stronger LLMs.\vspace{-0pt}
%     % \item number of examples per iteration
% \end{itemize}

% -------------------------------------------------------------
\subsubsection{The Choice of Informativeness Metrics: \texttt{info(\textperiodcentered)}}\label{sec:ab-metric}
\vspace{-4pt}
% \notes{To make a table on all metrics in Section~\ref{sec:ab-metric}, similar to~\citep{plr}.}
\input{tables/tab-info-metric}
\vspace{-8pt}
\input{tables/tab-ab-metric}
\vspace{-12pt}
% (\textit{cf}., the principle of insufficient reason~\citep{key,dr})
\paragraph{Advantage as the informativeness metric outperforms baselines.} \hspace{-5pt}As in Table~\ref{tab:ab-metric}, \textbf{\texttt{eva}} offers an effective curriculum by the advantage-based proxy as the informativeness metric (bottom row):
\vspace{-4pt}
\begin{itemize}
    \item Comparing w/ \emph{uniform evolving} (brown): Existing baselines generate prompts in a uniform manner~\citep{self-reward} w/o informativeness measure (\textit{cf}., the principle of insufficient reason~\citep{key,dr}). \method~concretely outperforms, corroborating~\cite{active-rlhf} that uniform learners can suffer sub-optimality gaps.
    \item Comparing w/ \emph{other heuristics} (blue): Prior practices~\citep{team-1} tried heuristics like prioritizing prompts w/ the most variance in its  rewards or w/ the lowest/highest average. We find our advantage based methods (red) outperforms those heuristics; see $\S$~\ref{app:metric} for more.
    \item Comparing w/ the \emph{inverse advantage} (purple): Contrary to curriculum learning, a line of works conjecture that examples w/ higher losses may be prioritized~\citep{hard-losers,ordered-sgd}, which can be done by inverting our metric. We find it significantly \emph{hurt} the alignment gain, corroborating~\cite{rho-loss} that those examples are often noisy, unlearnable or irrelevant, meaning our curriculum is effective and practical. 
    \item Among our \emph{advantage variants} (red): We  designed variants of our default advantage-based metric, as in Table~\ref{tab:info-metric}; the default $A^{\star}_{\min}$ remains competitive among its peers. Together, the advantage-based principle provides a robust guideline for prompt sampling and evolving.
\end{itemize}
\vspace{-4pt}
The lesson is that we must be selective about which are the promising to evolve, otherwise unlearnable, noisy or naïve prompts may hinder learning. Our regret-inspired metric represents a solid baseline. 

% \notes{Compare a star min with the uniform (no ordering), then compare it with its inverse (from hard to easy).}

% \paragraph{\emphtext{\method~is better other metric.}}  

% \notes{compare eva with other advantage variants, and other common choices that people have been using (choosing variance or mean) probably cite~\citep{active-pl,active-rlhf,selm} and emphasize our reliance on reward model. then cite~\cite{self-improving} in the footnote.}

% \paragraph{\emphtext{\method~.}}  \notes{compare eva with other advantage variants.}
% -------------------------------------------------------------

\vspace{-2pt}
% -------------------------------------------------------------
\subsubsection{The Effect of the sample-then-evolve procedure}\label{sec:ab-procedure}
\input{tables/tab-ab-procedure}
% \vspace{-5pt}
% : \texttt{sample(\textperiodcentered)}, \texttt{evolve(\textperiodcentered)}
\vspace{+8pt}
% \paragraph{\emphtext{Both designs of \texttt{sample(\textperiodcentered)} and \texttt{evolve(\textperiodcentered)} in~\method~is effective.}} As in Table~\ref{tab:ab-procedure}, we show:
\paragraph{The design of \texttt{\small evolve(\textperiodcentered)} in~\method~is effective.} As in Table~\ref{tab:ab-procedure}, we show:
\vspace{-4pt}
\begin{itemize}
    \item Removing the $\texttt{\small evolve}(\cdot)$ step: if we only do subset sampling or ordered selection, we still have gain, but not as much as w/ evolving (\eg \method~brings $4.8\%$ additional wins on AH).
    \item Altering the $\texttt{\small sample}(\cdot)$ step: if we greedily select prompts by the metric instead of using them as weights for importance sampling, the performance will be weaker as we evolve.
    % \footnote{When there is only subset selection, however, being greedy is slightly better on the Arena-Hard benchmark, but as we evolve more prompts such gain disappears.}. 
\end{itemize}
\vspace{-4pt}

% The lesson is that simply active learning on fixed prompts is unsatisfactory~\notes{To find a better description. AL is more about budget}; the open-ended RLHF with \emph{generative} prompt exploration we present brings a substantial headroom for self-improvement.
This shows that simply adaptive training within a fixed prompt distribution is unsatisfactory; our open-ended RLHF with \emph{generative} prompt exploration gives a substantial headroom for self-improvement.
% -------------------------------------------------------------




% -------------------------------------------------------------
\vspace{-40pt}
\subsubsection{Scaling Pointwise and Pairwise Reward Models}\label{sec:ab-rm}

\begin{figure}[H]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
        \end{subfigure}
        \vspace{-8pt}
        \caption{\textbf{\method\ scales with quality of reward models}, under pointwise RMs w/ DPO (\emph{left}) and pairwise RMs w/ SPPO (\emph{right}).  Note SPPO handles general preferences thus requires pairwise RMs, and DPO relies on the Bradley-Terry assumption, for which pointwise RMs are suitable.}
        \label{fig:ab-rm}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\textwidth}
        Figure~\ref{fig:ab-rm} presents the length-controlled win rate of \method~on  AlpacaEval  using pointwise and pairwise reward models of varying scales.
        %and types. We compare pointwise reward models w/ DPO, and pairwise reward models w/ SPPO\footnotemark.  
        The results give a clear trend: as the quality of reward models improve, \method~brings higher alignment gain. The scaling observation shows the effectiveness of~\method~in exploiting more accurate reward signals to choose informative prompts for better alignment.  One takeaway is interaction w/ the external world is essential for intelligence. The more accurate reward signals observed, the better the agent incentivize themself to improve (\textit{cf.},~\cite{silver2021reward}).
    \end{minipage}
\end{figure}
\vspace{-8pt}


% \footnotetext{We note that when there is only subset selection, being greedy is slightly better on the Arena-Hard benchmark. However, as we evolve more prompts, this discrepancy reverses.}

% \begin{figure}[!ht]
%     \centering
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
%         \end{subfigure}
%         \vspace{+0.1pt}
%         \caption{\textbf{Scaling with reward models.} Benchmark evaluation shows~\method~scales with reward models under both pointwise (\emph{left}) and pairwise (\emph{right}) setting.}
%         \label{fig:ab-rm}
%     \end{minipage}
% \end{figure}
% \vspace{-3pt}

% \paragraph{\emphtext{\method~scales with reward models.}} Figure~\ref{fig:ab-rm} presents the performance of \method~on the AlpacaEval benchmark using reward models of varying scales and types. We compare pointwise reward models with DPO~\citep{dpo} with pairwise reward models with SPPO~\citep{self-play-gu}\footnote{SPPO handles general preferences and thus requires pairwise reward models, whereas DPO relies on the Bradley-Terry model, for which pointwise reward models are suitable.}.  The results demonstrate a clear trend: as the quality of the reward model improves, \method~brings higher performance gain. The scaling observation shows the effectiveness of~\method~in leveraging more accurate reward signals to select informative prompts for better alignment. More results are in $\S$~\ref{app:ab-rm}.


% % \notes{The experiment is running.}
% \input{tables/tab-ab-rm}





% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{\method~Improves Both Sample Efficiency and Generalization}\label{sec:ab-cont}
We then continuously run the default \emph{incremental training} (\ie trainining from the last checkpoint w/ the evolved set in each iteration), as in Fig~\ref{fig:sad}, \method~presents \emphtext{\it monotonic performance gain} over iterations, and surpasses that trained w/ new human prompts, implying the generalization benefit\footnote{Behaviors of the dashed/dotted lines relate to \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat}.  Classical works resolve it by the optimization view (\eg weight perturbing), whereas~\method~provides a fresh data view, potentially mimicing an \textbf{implicit regularizer for better generalization}.}.
\vspace{-3pt}

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% \notes{Finished running. Waiting for evaluation.}



% A prominent line of research is on the loss of plasticity for continual (incremental) training~\citep{cont-critical,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm,cont-warm}; prior works all try to solve this via the optimization perspective, while our \eva method provides a fresh data perspective to solve the issue, operating like adding a regularizer to find better local minima.

\vspace{-5pt}
\begin{figure}[h!]
\centering

% \begin{minipage}{0.34\textwidth}
% \includegraphics[width=.8\textwidth]{figs/sad.png}
% % \caption{Iterative incremental training in different settings. } \label{fig:sad}
% \vspace{+2pt}
% \caption{\textbf{Continual training.} Our method stays robust w/ more iterations in incremental training. } \label{fig:sad}
% \end{minipage}
\begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=.86\textwidth]{figs/dpo-it.pdf} % First figure
    % \vspace{10pt} % Adjust spacing between figures if needed
    \includegraphics[width=.86\textwidth]{figs/sppo-it.pdf} % Second figure
    \vspace{-6pt}
    \caption{\textbf{Continual training.} \method~stays robust w/ more iterations in incremental training.}
    \label{fig:sad}
\end{minipage}
\hfill
\begin{minipage}{0.64\textwidth} 
% \setlength{\parindent}{1em} % Adjust as needed for indentation
The solutions found by~\method~cannot be recovered by training longer w/ a fixed distribution (the dashed), nor by naïvely sourcing new prompts w/o examining informativeness (the gray dotted),  thus our generative data schedule is effective.\vspace{+6pt}

In Table~\ref{tab:ab-cont}, we ablate~\method~in \textit{scratch training}, \ie training w/ the full set (the evolved and the original data). \method~is competitive in incremental training, thus \emphtext{\emph{learns more effective} with \emph{less data}} -- a nice bonus via minimax regret~\citep{dcd}.

% , as in $\S$~\ref{sec:int}


% Next, we consider two different continual procedures:
% \begin{itemize}
%     \item \textbf{Incremental training}\footnotemark: train with only the evolved data on the finetuned checkpoint $\vtheta_{0 \rightarrow 1}$.\vspace{-1pt}
%     \item \textbf{Scratch training}: combine the evolved data with the full initial prompt set, train from scratch with $\vtheta_0$.
% \end{itemize}
% \vspace{+4pt}

\vspace{-6pt}
\input{tables/tab-ab-cont}


% We then iteratively run incremental training, as in Figure~\ref{fig:sad}, \method~presents monotonic performance gain.\vspace{+4pt}

% A prominent line of research is on the difficulty of continual (incremental) training, and prior works all try to solve this via the explicit regularizer perspective~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}, while \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

\end{minipage}

\end{figure}
\vspace{-9pt}


% cont-rewarm
% acting like an implicit regularizer for better local minima

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% Furthermore, the open-ended nature of~\method~naturally aligns with the continual learning literature; one of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better generalization.

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% The open-ended nature of~\method~naturally aligns with the continual learning literature.
% One of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima, 
% ~\notes{To update the figure; having DPO+SPPO.}
% \vspace{+6pt}


% \footnotetext{This is the default training strategy that we are using as it is computational efficient.}



% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{The Effect of Iteratively Evolving}\label{sec:ab-iter}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% \input{tables/tab-ab-iter}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of the Base LLM for the Creator}\label{sec:ab-gen-lm}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% % \notes{Experiments running in process. Mostly finished training. }
% \input{tables/tab-ab-gen-lm}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of The Number of Training Examples}\label{sec:ab-scale}
% \input{tables/tab-ab-scale}
% % -------------------------------------------------------------

% \notes{We may need to add additional compute resources usage discussions to illustrate efficiency.}














==> texs_/exp.tex <==
\newpage
\section{Experiments}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/arena-hard.png}
%         \caption{Caption for Arena Hard}
%         \label{fig:arena-hard}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/mt-bench.png}
%         \caption{Caption for MT Bench}
%         \label{fig:mt-bench}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/alpaca-eval.png}
%         \caption{Caption for Alpaca Eval}
%         \label{fig:alpaca-eval}
%     \end{subfigure}
%     \caption{Overall caption for the three figures}
%     \label{fig:three-figures}
% \end{figure} 


\subsection{Experimental Settings}

\paragraph{Datasets and Models for Training.} We use  \text{UltraFeedback}~\citep{ultrafeedback} as the training dataset.  It contains 64K prompts from six different datasets. We use the instruction-finetuned version of \textsc{Gemma-2-9B}~\citep{gemma2} and \textsc{Llama-3.1-8B}~\citep{llama3} as the baseline model.

% (\href{https://github.com/thunlp/UltraChat}{UltraChat}, \href{https://huggingface.co/datasets/RyokoAI/ShareGPT52K}{ShareGPT}, \href{https://github.com/nlpxucan/WizardLM}{Evol-Instruct}, \href{https://huggingface.co/datasets/truthfulqa/truthful_qa?row=10}{TruthfulQA}, \href{https://github.com/thunlp/FalseQA}{FalseQA}, and \href{https://huggingface.co/datasets/Muennighoff/flan}{FLAN})

% This dataset focuses on (i) instruction-following, (ii) truthfulness; (iii) honesty; and (iv) helpfulness.

% Each prompt is paired with 4 responses generated by different language models, where each response is rated from 1 to 5 according to the five dimensions by GPT-4.

\paragraph{Evaluation benchmarks.} We consider: (i) \text{MT-Bench}~\citep{llm-judge}: this dataset evaluates multi-turn instruction-following, with 80 questions from 8 categories. (ii) \text{Arena-Hard}~\citep{ah}: this dataset is derived from 200K user queries on Chatbot Arena, with 500 hard technical prompts across 250 topics. (iii) \text{AlpacaEval 2.0}~\citep{ae}: This dataset assesses general instruction-following ability, and includes 805 questions.
% \footnote{If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge model, and \texttt{gpt-4-0314} as the baseline model when calculating the win rate.}
% \vspace{-5pt}
% \begin{itemize}
% \item \textbf{MT-Bench}: This dataset evaluates multi-turn conversation and instruction-following. It contains 80 questions across 8 categories.\vspace{-0pt}
% \item \textbf{Arena-Hard}: This dataset is derived from 200K user queries on Chatbot Arena. It contains 500 high-quality  technical problem-solving prompts across 250 topics. \vspace{-0pt}
% \item \textbf{AlpacaEval 2.0}: This dataset assesses general instruction-following ability, and includes 805 questions from 5 datasets covering various tasks like creating, generating, and explaining.\vspace{-0pt}
% \end{itemize}

% \paragraph{Evaluation benchmarks.} We consider the following evaluation benchmarks\footnote{If not otherwise specified, we use \texttt{gpt-4-1106-preview} as the judge model, and \texttt{gpt-4-0314} as the baseline model when calculating the win rate.}:
% % \vspace{-5pt}
% \begin{itemize}
% \item \textbf{MT-Bench}: This dataset evaluates multi-turn conversation and instruction-following. It contains 80 questions across 8 categories: writing, roleplay, extraction, reasoning, math, coding, STEM knowledge, humanities and social sciences knowledge.\vspace{-0pt}
% \item \textbf{Arena-Hard}: This dataset is derived from 200K user queries on Chatbot Arena. It contains 500 high-quality  technical problem-solving prompts across 250 topics. \vspace{-0pt}
% \item \textbf{AlpacaEval 2.0}: This dataset assesses general instruction-following ability, and includes 805 questions from 5 datasets covering various tasks like creating, generating, and explaining.\vspace{-0pt}
% \end{itemize}

% The benchmarks described below evaluate the  human preference on \emph{general} conversational ability and commonsense generation from language models by subjecting them to inquiries spanning multiple domains. All of them use external large language models as the judge to cheaply approximate human preferences.

% \begin{itemize}
%     \item  \href{https://arxiv.org/pdf/2306.05685}{\textbf{MT-Bench}}: This dataset focuses on the evaluation of (i) multi-turn conversation and (ii) instruction-following abilities of language models. It includes eight categories: (i) writing, (ii) roleplay, (iii) extraction, (iv) reasoning, (v) math, (vi) coding, (vii) knowledge I (STEM), and (viii) knowledge II (humanities / social sciences); each category features 10 carefully designed multi-turn questions, contributing to a total of 80 questions.
%     \item \href{https://tatsu-lab.github.io/alpaca_eval/}{\textbf{Alpaca-Eval}}. This dataset focuses on the evaluation of general instruction-following ability. It is built upon the 52K machine-generated instruction dataset~\citep{alpacafarm}, asking the language model to create, generate, suggest, design, construct, make, identify, calculate, convert, find, name, provide, summarize, classify, describe, edit, give, explain, write and re-write things\footnote{\href{https://github.com/tatsu-lab/stanford\_alpaca?tab=readme-ov-file\#data-generation-process}{\texttt{https://github.com/tatsu-lab/stanford\_alpaca}.}}. It consists of 805 questions from 5 datasets in total.
%     \item \href{https://lmsys.org/blog/2024-04-19-arena-hard/}{\textbf{Arena-Hard}}. Based on 200K diverse user queries collected via \href{https://arena.lmsys.org/}{Chatbot Arena}, the authors first cluster them into over 4K topics, then filter out low-quality prompts according to criteria including (i) complexity, (ii) creativity, (iii) technical accuracy, (iv) domain knowledge, (v) real-world application, (vi) specificity and (vii) problem solving. The resulting dataset contains 250 high-quality topic, where each topic corresponds to 2 randomly sampled prompts, contributing to 500 well-defined, technical problem-solving queries\footnote{\href{https://huggingface.co/spaces/lmsys/arena-hard-browser}{\texttt{https://huggingface.co/spaces/lmsys/arena-hard-browser}.}}. We use \texttt{gpt-4-1106-preview} as the judge model, and \texttt{gpt-4-0314} as the baseline model.
% \end{itemize}



 

 

 % We present a verbose review on existing preference optimization algorithms in Appendix~\ref{app:table}.
 % We consider DPO~\citep{dpo} as the default optimization algorithms, with ab

\paragraph{Preference optimization algorithms.} We consider the following algorithms:
\vspace{-2pt}
\begin{itemize}
    \item \textbf{w/ the reference model}: DPO~\citep{dpo}, SPPO~\citep{self-play-gu}.\vspace{-1pt}
    \item \textbf{w/o the reference model}: SimPO~\citep{simpo}, ORPO~\citep{orpo}.\vspace{-1pt}
\end{itemize}

\paragraph{Reward Models as preference oracles.} We use \textsc{ArmoRM-8B}~\citep{armorm} as the default off-the-shelf reward model as the preference proxy, and consider the following for ablation studies:
\vspace{-2pt}
\begin{itemize}
    \item \textbf{Pairwise}: \textsc{PairRM-0.4B}~\citep{pairrm}, \textsc{PairRM-8B}~\citep{pairrm8b}.\vspace{-1pt}
    \item \textbf{Absolute}: \textsc{ArmoRM-8B}~\citep{armorm}, \textsc{SkyworkRM-27B}~\citep{skyworkrm}.\vspace{-1pt}
\end{itemize}


\subsection{Main Results}

In general, \method~brings concrete improvement in alignment without any additional human prompts.

\subsubsection{\textnormal{\textbf{\texttt{eva-i}}}: Main Results with the Iterative Training Setting}
\input{tables/tab-main-10k}

\subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: Main Results with the Online Training Setting}
\input{tables/tab-main-10k-o}

% \subsection{Subsections}





% -------------------------------------------------------------


% \newpage
\subsection{Ablation Studies}
% \notes{For now, we use tables to record results. We can shift to other illustrations later (\eg performance plot, pareto circle, prompt distribution w.r.t. metric, etc).}
We conduct serveral ablation studies on \texttt{\textbf{eva-i}}, with the following findings: (i) textbf{Informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives. (ii) \textbf{Scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method. (iii) \textbf{Continual training schedule}: incremental training with informative prompts is comparable to scratch training, effective serving as a regularizer. 
% \begin{itemize}
%     \item \textbf{Informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives.\vspace{-2pt}
%     \item \textbf{Scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method.\vspace{-2pt}
%     \item \textbf{Continual training schedule}: incremental training with informative prompts can be comparable to scratch training, effective serving as a regularizer.  \vspace{-2pt}
%     % \item \textbf{Iterative evolving schedule}: we can obtain monotonic gain from iterative evolving.\vspace{-0pt}
%     % \item \textbf{Base creator LLMs}: self-instruct is effective, and we can benefit from stronger LLMs.\vspace{-0pt}
%     % \item number of examples per iteration
% \end{itemize}

% We conduct serveral ablation studies on \texttt{\textbf{eva-i}}, with the following findings:\vspace{-5pt}
% \begin{itemize}
%     \item \textbf{Informativeness metric}: the proposed informativeness metric based on \emph{advantage} is effective and outperforms other alternatives.\vspace{-2pt}
%     \item \textbf{Scaling w/ reward models}: the more accurate the reward model, the better the alignment improvement brought by our method.\vspace{-2pt}
%     \item \textbf{Continual training schedule}: incremental training with informative prompts can be comparable to scratch training, effective serving as a regularizer.  \vspace{-2pt}
%     % \item \textbf{Iterative evolving schedule}: we can obtain monotonic gain from iterative evolving.\vspace{-0pt}
%     % \item \textbf{Base creator LLMs}: self-instruct is effective, and we can benefit from stronger LLMs.\vspace{-0pt}
%     % \item number of examples per iteration
% \end{itemize}

% -------------------------------------------------------------
\subsubsection{The Effect of Different Informativeness Metrics}\label{sec:ab-metric}
% \notes{To make a table on all metrics in Section~\ref{sec:ab-metric}, similar to~\citep{plr}.}
\input{tables/tab-ab-metric}
% -------------------------------------------------------------



% -------------------------------------------------------------
\subsubsection{The Effect of Different Reward Models at Different Scales}\label{sec:ab-rm}
% \notes{The experiment is running.}
\input{tables/tab-ab-rm}
% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{The Effect of Different Continual Training Procedures}\label{sec:ab-cont}
% \notes{Finished running. Waiting for evaluation.}



% A prominent line of research is on the loss of plasticity for continual (incremental) training~\citep{cont-critical,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm,cont-warm}; prior works all try to solve this via the optimization perspective, while our \eva method provides a fresh data perspective to solve the issue, operating like adding a regularizer to find better local minima.
\input{tables/tab-ab-cont}
\vspace{-5pt}
\begin{figure}[h!]
\centering

\begin{minipage}{0.34\textwidth}
\includegraphics[width=\textwidth]{figs/sad.png}
\caption{Iterative incremental training in different settings. } \label{fig:sad}
\end{minipage}
\hfill
\begin{minipage}{0.62\textwidth} 
% \setlength{\parindent}{1em} % Adjust as needed for indentation

We consider two different continual training procedure:
\begin{itemize}
    \item \textbf{Incremental training}\footnotemark: train with only new data on the last finetuned checkpoint.\vspace{-1pt}
    \item \textbf{Scratch training}: combining new data with the initial training set, then train with the augmented dataset with the initial checkpoint.
\end{itemize}

The results is in Table~\ref{tab:ab-cont}, showing that \method~is comparable or better than scratch training, while being much more efficient.

We then iteratively run incremental training, as in Figure~\ref{fig:sad}, \method~presents monotonic performance gain.\vspace{+4pt}

A prominent line of research is on the difficulty of continual (incremental) training, and prior works all try to solve this via the explicit regularizer perspective~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}, while \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

\end{minipage}

\end{figure}
\vspace{-5pt}
\footnotetext{This is the default training strategy that we are using as it is computational efficient.}


% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{The Effect of Iteratively Evolving}\label{sec:ab-iter}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% \input{tables/tab-ab-iter}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of the Base LLM for the Creator}\label{sec:ab-gen-lm}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% % \notes{Experiments running in process. Mostly finished training. }
% \input{tables/tab-ab-gen-lm}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of The Number of Training Examples}\label{sec:ab-scale}
% \input{tables/tab-ab-scale}
% % -------------------------------------------------------------

% \notes{We may need to add additional compute resources usage discussions to illustrate efficiency.}














==> texs_/intro-cache.tex <==


% \textcolor{red}{[Expected to have a complete draft by tonight (Mon Sep 23.); the introduction section will be revised in the last after we have a good draft of Section~\ref{sec:method}.]}





% \begin{figure}[hb]
%     \centering
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/mt-bench.png}
%         \caption{Alpaca Eval}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/arena-hard.png}
%         \caption{Arena Hard}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/alpaca-eval.png}
%         \caption{MT Bench}
%     \end{subfigure}
%     \caption{Placeholder plot on evaluation results.}
%     \label{fig:three_benchmarks}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
%     \caption{Placeholder plot on pipeline.}
% \end{figure}


%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
\section {Introduction}
Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
High quality human data, crucial for scaling large language model (LLM) based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as LLMs become more capable, they need to solve increasingly complex challenges, requiring training data beyond abilities of humans to create. This necessitates a new fundamental mechanism for self-improving, where models is able to continuously self-generate and self-solve harder problems. We thereby investigates the research question below:\vspace{+6pt}
\begin{minipage}{1.\textwidth}
% \footnotesize
\centering
\textit{Can language models \emph{self-create} new, learnable tasks to work on,\\}
\textit{to \emph{self-improve} to \emph{generalize} better for human preferences alignment?}
\end{minipage}
%or higher intelligence.


% \notes{One way to write the motivation part may be to follow ~\citep{poet,bengio2009curriculum,accel,paired}. Discuss how we incentivize the agent to generate prompt distribution with increasing complexity, promoting the models to solve harder problems.}

% \notes{Additional motivation/intuition/background paragraphs need to be added here. Motivate why we need to jointly optimize for both.}

% We aim to develop language agents capable of surpassing even superior intelligence, enabling them to solve increasingly complex problems.

\begin{figure}[ht]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{0.258\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline.png}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.732\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/creator.png}
            % \caption{Arena Hard}
        \end{subfigure}
        \caption{\textbf{Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our proposed~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with an easy-to-implement \emph{estimate, sample then evolve} procedure; specifically, it estimates the informativeness for each prompt by how contrastive the self-generated responses are to the prompt, from the reward signals it receives. The creator evolves new prompts  from highly informative prompts, which the solver uses for continual training. Both the solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective design in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}
\vspace{-6pt}

% (\eg rewriting the prompts for in-depth/breadth variations)

\vspace{+2pt}



% at the same time as
% Given a fixed training set,
%to generalize well on new, unseen tasks?
% on \fix{to fix: some target domain}

% \notes{Add more intuition. Motivating why we are doing so.}

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

\vspace{-6pt}
To go beyond the fixed training paradigm, we propose to evolve the training distribution for aligning LLMs. Our method, which we call~\method,  alternates between two steps: (i) \tb{creating tasks} (or prompts), and (ii) \tb{solving them}.  As shown in Figure~\ref{fig:game}, these two steps are as follows:
\vspace{-3pt}
\begin{itemize}
    \item $\emphredd{\text{\bf \tc{Creator}}}$ \hspace{+1pt}: generates increasingly informative prompts.
    \item $\emphgreenn{\text{\bf \tg{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}}$ \hspace{+1pt}: produces responses to prompts and optimize for alignment.
\end{itemize}

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% One of the key challenges in open-ended learning is ensuring that an agent can generalize to unseen, novel environments, rather than overfitting to a fixed distribution. 

Typical preference optimization algorithms~\citep{dpo,self-play-gu,simpo} rely on a static set of training prompts, which can be viewed as a single \tb{solver step}. By adding the \tb{creator step}, ~\method\ can identify and generate a set of most informative prompts for the current policy to most efficiently learn from. This allow going beyond a static prompt set during training in the typical preference learning setting, and creating an evolving training curriculum that's most fit to the current policy and help generalize to the real-world tasks. Specifically, we implement the creator step by: (i) \textbf{estimate} the informativeness of each prompt, given an existing prompt distribution; (ii) \textbf{sample} an informative subset from those prompts, weighted by the informativeness score; (iii) \textbf{evolve} the informative subset by synthetically generating similar prompts in its \emph{proximal region}, and combine with a buffer of previous prompts, which forms a new prompt distribution. This can be flexibly plugged into any existing alignment pipeline, as shown in  Fig~\ref{fig:pipeline} and Algo~\ref{alg:i-eva}.

% \footnote{The informativeness measure we use is %related to the advantage function, which is empirically 
% estimated by sampling multiple responses from the prompt and take the difference between the maximal reward $r_{\max}$ and the minimal reward $r_{\min}$ received for the responses.}

% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 

% RA.24.9: Discuss and summarize empirical results here.

%% RA.24.9: This seemed quite repetitive, so merged it with previous para.
% In Algorithm~\ref{alg:i-eva}, we illustrate a practical algorithm for~\method. Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{dpo,simpo}.

% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.


% \notes{To write it differently. Instead of motivating by the iterative training issue, we should directly focus on our method per se. First introduce the underlying principle of generative state exploration; then discuss the classical literature on instruction generation (mostly uniform). Then discuss the practical design of our method. Our main table would focus on 1-iteration improvement with our method. We can then move to the iterative setting . In the literature part, we can mention other concurrent works.}

% Our setup is iterative preference optimization with self-generated responses\footnote{This approach has become increasingly common in recent literature~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}.}. It is important that we choose to initilize using the solution of the previous iteration\footnote{See more discussion on efficiency issues forthcoming}, rather than initilizing from scratch. The baseline setting is that there is only a fixed prompt set, and we iteratively train models with the fixed prompt set with newly self-generated response. We can show that there is a performance drop or plateau as more iterations go, if we only evolve in the $\rvy \mid \rvx$ distribution for the new iterations. We propose that we must adapt the $\rvx$ distribution as well, and propose a new principle as well as an practical algorithm.
  
% \begin{center}
% \emph{Starting from a fixed training prompt set, can we continuously improve alignment on the target domain?}
% \end{center}

% \method~generates the next training batch of prompts, by evolving prompts (\ie~making edits or variations) with higher estimated learning potential.

% Our method, \method, evolves the prompt distribution by generating prompts with high learning potential, incentivizing the language agents to solve increasingly informative prompts. 



Our main contributions are summarized as:
\begin{itemize}
\vspace{-3pt}
    % \item \textbf{A phenomenon}: We show that classical iterative preference optimization algorithms exhibit the \emph{reverse scaling trap}, where continual training with more data can \emph{hurts}  alignment. 

    \item \textbf{A new principle}: We propose \method, a generalized \textbf{open-ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment.
    % \fix{add generalization, and say that also generalize classical RLHF}
% \begin{align}
% % \max_{\phi, \theta} &\mathbb{E}_{\textcolor{red}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{Green}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] \nonumber \\
% % &- D_{\text{KL}}(\textcolor{red}{p_{\phi}(x)} \cdot \pi_{\theta}(y \mid x) \mid\mid \textcolor{red}{p_{\text{true}}(x)}\cdot \pi_{\text{ref}}(y \mid x)) \nonumber \\
% \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \emphred{\textcolor{cred}{\pi_{\vphi}(\rvx)}} \cdot \emphgreen{ \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)}} \ \| \ \emphgray{\tb{\pi_{\text{ref}}(\rvx, \rvy)}}\ \Biggr]\nonumber 
% % \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{black}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\ \Biggr]\nonumber 
% % \\
% % &= \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})]   - \mathbb{E}_{\textcolor{red}{\mathbf{x} \sim p_{\phi}(\cdot)}}[\textcolor{black}{D_{\text{KL}}(\textcolor{cgreen}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx))}] \nonumber \\
% % & \qquad \quad \ - \textcolor{cred}{D_{\text{KL}}(\pi_{\phi}(\rvx) \mid\mid p_{\text{true}}(\rvx))} \nonumber
% \end{align} 

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline.

    % \item \textbf{A new continual training procedure}: We first formally identify the \textbf{inverse scaling trap} in iterative alignment. Combining with explicit regularization, we present an efficient continual training procedure with our method. \ziyu{This part needs more tuning.}
    
    \item \textbf{State-of-the-art performance}: We empirically validate our method on public alignment benchmarks and present universally strong performance improvement when plugged in with different preference optimization algorithms (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide additional insights on the choice of informativeness metric, reward model, and training schedules. 
    % \notes{To mention impact on downstream tasks, as the original RLHF paper did~\citep{rlhf}.}
\end{itemize}

% [TODO: a paragraph that explains our method in the simplest form.] Our approach is very simple: given any existing prompt set, the creator sample prompts that are most informative for preference aligning, then evolve a new set upon the previous set; the solver will generate responses, which will in turn be used for preference optimization. Central to our approach is the informativeness metric, which we use the reward gap (contrastive ratio). 


% \notes{consider adding the metric (reward advantage / contrastive ratio) for prompt informativeness as a new contribution (useful beyond our work); also provide an intuitive example with bandits.}

% \notes{Also discuss the regret-based curriculum and the open-endedness literature~\citep{accel} }

% \notes{TODO: providing an intuitive example using bandits to illustrate that our perspective is new (This also brings a new perspective of ``\emph{generative exploration}'' for RL, in the sense that we actively generate states during the learning process, which is typically undoable in classical contextual bandits/RL.). }

% Having a distribution that covers all the complexity of the real world is very challenging~\citep{paired}.

% \fix{The creator step is straight-forward.}



\method~is simple to implement. We hope it can serve as a scalable starting point to build \text{open-ended} self-improving language agents that align with human values and co-evolve with human intelligence.

% \notes{producing learnable but novel artifacts~\citep{open-endedness}}\notes{maybe somewhere differentiate mention intrinsic motivation and incentivizing } 
% \fix{See App~\ref{sec:temporary notes} for some revision notes (\eg adding literature discussion; structured motivation; most importantly, highlight on the usage of reward model; improve clarity; etc.). We can improve a lot.}

% \textcolor{red}{[Introduction needs some work and should state that the creator step relies on the computation of a notion of informativeness and on a method that evolves prompts. This needs to be stated asap so the reader understands the method and the algorithm. ]}

% \notes{Also adding a figure to illustrate the joint distribution perspective. One figure is on standard alignment, and the other figure is on eva.}

% Line 6 – 8 is a practical plug-in implementation to mimic the adversarial prompt player:
% evaluating the informativeness for each prompt
% e.g., max_reward - min_reward
% using the above metric as the weight for adaptive sampling to create an informative subset
% generating new prompts via a prompt generation policy 


% are many human values really worth to align?

% Central to our method is the informativeness measure 

% TODO: add plots of algo pipeline and performance.

% Two motivations: (i) the size of the prompt set is a bottleneck on existing alignment performance, and we need a robust way to continuously improve the alignment performance; (ii) naïvely training with more data could hurt the performance - this happens in both training from scratch  

% In~\citep{warm}, ``conventional intuition suggests that when solving a sequence of related optimization problem of this from, it should be possible to initialize using the solution of the previous iterate to ``warm start'' the optimization rather than ``initialize from scratch''. However, in practice this warm-starting seems to yield poorer generalization performance than models that have fresh random initialization.''

% Adding discussions on the re-warming and loss of plasticity literature; comparing with them.

% Adding discussions in the exploration literature of bandit and RL.



% We cast the preference alignment problem as an two-player asymmetric self-play game, while one player learns to propose the most informative prompt set, and the other player learns to best respond to the proposed prompt set. At the equilibrium, we expect to have the optimal policy of language generation for both players.

% % The simplifying assumptions underlying Bradley-Terry model cannot capture real-world human preferences, which are often intransitive.

% Self-play preference optimization~\citep{nlhf,rlhf-more-diff,self-play-gu} casts the alignment problem as a two-player, general-sum game, where each player is a policy, parameterized by the language model, that aims to optimize the probability of its responses to be preferred against the other player's. Existing works iteratively update the policy network for it to converge to the optimal policy characterizing by the Nash equilibrium, empirically showing it as a promising framework.

% However, a fundamental issue, which is often neglected by current algorithms, is that the initial prompt set may not adequately represent the full range of scenarios the model will encounter in the real world. This limitation can lead to policies that are optimal within the confined space of the initial prompts but suboptimal or even poorly performing when faced with a broader distribution of inputs.  
% %\notes{The reasoning gap could be one example.}
% %Moreover, as language models continue to evolve and improve, the nature and complexity of prompts that can effectively challenge and improve these models also change. This dynamic landscape necessitates a more adaptive approach to prompt selection and generation throughout the finetuning process. 

% % \notes{Rewrite this paragraph, and put emphasis only on the prompt set optimization part.}
% % However, several fundamental challenges arise when applying self-play alignment in the real world:
% % \begin{itemize}
% %     \item \textbf{Prompt Distribution Mismatch:} The assumption of sampling from a fixed prompt distribution $\mathcal{X}$ may lead to generalization issues. \notes{i.e., exploration in $p(x)$?}
% %     \item \textbf{Preference Uncertainty:} The preference oracle $\mathbb{P}(\cdot)$ may be noisy, biased, or limited in its capacity to judge all types of responses.\notes{This is like having two nested equilibriums; policy v. policy; generator v. discriminator.}
% %     \item \textbf{Response Space Constraints:} The model's ability to generate responses may not sufficiently cover the space of optimal responses. \notes{to rephrase; simply exploration for $p(y|x)$}
% % \end{itemize}

% % A useful prompt is often a \emph{surprising} prompt~\citep{ai-mathematician}.

% To address these challenges, we propose an \emph{evolving alignment} framework, with an \emph{asymmetric self-play} mechanism.

% Simply put, we consider to grow $\calX, \calY$, while existing work mostly care about $\calY \mid \calX$ with a fixed $\calX$.


    

    

==> texs_/intro-fix.tex <==
\section{\textcolor{Gray}{[Draft]} Introduction}



% \begin{figure}[hb]
%     \centering
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/mt-bench.png}
%         \caption{Alpaca Eval}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/arena-hard.png}
%         \caption{Arena Hard}
%     \end{subfigure}
%     \hspace{0.02\textwidth} % Small space between the subfigures
%     \begin{subfigure}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/alpaca-eval.png}
%         \caption{MT Bench}
%     \end{subfigure}
%     \caption{Placeholder plot on evaluation results.}
%     \label{fig:three_benchmarks}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
%     \caption{Placeholder plot on pipeline.}
% \end{figure}


%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
Long-lived language agents must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
The human-generated data, crucial for scaling language models, is projected to run out in the next few years \citep{run-out-of-data}. This limitation necessitates new framework for continual model improvement.

% Some motivation statements:
% The key thing here is that learning is not a ``train-once'' thing; it should be open-ended and self-improving. Just like humans, we start with some basic knowledge, then we develop the whole modern science. The central things for  learning is about: (i) identifying the informative spaces (states \emph{and} actions) to explore; (ii) receiving useful feedback on such exploration. In this way we can continuously improve. 

% then motivate with 

% maybe providing a simple bandit example.

% revealed preference theory

% ~\citep{poet}: ``as compelling as this narrative may be, it is not the only conceivable path forward.  ... only rarely discussed, the job of the algorithm could be to conveive both the challenges and the solutions at the same time.'' increased complexity
% relation of self-play to co-evolution

Our research question is:

\begin{minipage}{1.0\textwidth}
% \footnotesize
\centering
\textit{Starting from a given training prompt set,\\}
\textit{can we continuously improve the alignment performance on a target domain?}
\end{minipage}


%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.


% \notes{To write it differently. Instead of motivating by the iterative training issue, we should directly focus on our method per se. First introduce the underlying principle of generative state exploration; then discuss the classical literature on instruction generation (mostly uniform). Then discuss the practical design of our method. Our main table would focus on 1-iteration improvement with our method. We can then move to the iterative setting . In the literature part, we can mention other concurrent works.}

% Our setup is iterative preference optimization with self-generated responses\footnote{This approach has become increasingly common in recent literature~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}.}. It is important that we choose to initilize using the solution of the previous iteration\footnote{See more discussion on efficiency issues forthcoming}, rather than initilizing from scratch. The baseline setting is that there is only a fixed prompt set, and we iteratively train models with the fixed prompt set with newly self-generated response. We can show that there is a performance drop or plateau as more iterations go, if we only evolve in the $\rvy \mid \rvx$ distribution for the new iterations. We propose that we must adapt the $\rvx$ distribution as well, and propose a new principle as well as an practical algorithm.
  
% \begin{center}
% \emph{Starting from a fixed training prompt set, can we continuously improve alignment on the target domain?}
% \end{center}




Our main contributions are summarized as:
\begin{itemize}
    % \item \textbf{A phenomenon}: We show that classical iterative preference optimization algorithms exhibit the \emph{reverse scaling trap}, where continual training with more data can \emph{hurts}  alignment. 

    \item \textbf{A new principle}: We propose \method, a general \textit{open-ended self-improving} \textbf{RLHF principle}:
\begin{align}
% \max_{\phi, \theta} &\mathbb{E}_{\textcolor{red}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{Green}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] \nonumber \\
% &- D_{\text{KL}}(\textcolor{red}{p_{\phi}(x)} \cdot \pi_{\theta}(y \mid x) \mid\mid \textcolor{red}{p_{\text{true}}(x)}\cdot \pi_{\text{ref}}(y \mid x)) \nonumber \\
\hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \emphred{\textcolor{cred}{\pi_{\vphi}(\rvx)}} \cdot \emphgreen{ \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)}} \ \| \ \emphgray{\tb{\pi_{\text{target}}(\rvx, \rvy)}}\ \Biggr]\nonumber 
% \hspace{-16pt}&\quad \max _{\vphi, \vtheta}  \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi(\cdot)}}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}\Biggr[\ r(\mathbf{x}, \mathbf{y}) \ \Biggr] - D_{\text{KL}}\Biggr[\ \textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{cgreen}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{black}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\ \Biggr]\nonumber 
% \\
% &= \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{cgreen}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})]   - \mathbb{E}_{\textcolor{red}{\mathbf{x} \sim p_{\phi}(\cdot)}}[\textcolor{black}{D_{\text{KL}}(\textcolor{cgreen}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx))}] \nonumber \\
% & \qquad \quad \ - \textcolor{cred}{D_{\text{KL}}(\pi_{\phi}(\rvx) \mid\mid p_{\text{true}}(\rvx))} \nonumber
\end{align} 

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, implemented through alternating optimization in a \textbf{creator \emph{v.s.} solver game}\footnote{In the language space, the creator refers to the prompt generation policy $\pi_X$ and the solver refers to the response generation policy $\pi_{Y|X}$.}. We develop a simple and flexible algorithm that can be easily plugged into any existing alignment pipeline, with both off-policy (\texttt{eva-i}) and on-policy (\texttt{eva-o}) variants.

    % \item \textbf{A new continual training procedure}: We first formally identify the \textbf{inverse scaling trap} in iterative alignment. Combining with explicit regularization, we present an efficient continual training procedure with our method. \ziyu{This part needs more tuning.}
    
    \item \textbf{State-of-the-art performance}: We empirically validate our method on popular alignment benchmarks and present strong performance improvement with extensive ablation studies.
\end{itemize}

% [TODO: a paragraph that explains our method in the simplest form.] Our approach is very simple: given any existing prompt set, the creator sample prompts that are most informative for preference aligning, then evolve a new set upon the previous set; the solver will generate responses, which will in turn be used for preference optimization. Central to our approach is the informativeness metric, which we use the reward gap (contrastive ratio). 


% \notes{consider adding the metric (reward advantage / contrastive ratio) for prompt informativeness as a new contribution (useful beyond our work); also provide an intuitive example with bandits.}

% \notes{Also discuss the regret-based curriculum and the open-endedness literature~\citep{accel} }

% \notes{TODO: providing an intuitive example using bandits to illustrate that our perspective is new (This also brings a new perspective of ``\emph{generative exploration}'' for RL, in the sense that we actively generate states during the learning process, which is typically undoable in classical contextual bandits/RL.). }



We envision \texttt{eva}~as a foundational and scalable starting point to build open-ended self-improving language agents that aligns with human values. \fix{See Appendix~\ref{sec:temporary notes} for revision notes.}

% \notes{Also adding a figure to illustrate the joint distribution perspective. One figure is on standard alignment, and the other figure is on eva.}

% Line 6 – 8 is a practical plug-in implementation to mimic the adversarial prompt player:
% evaluating the informativeness for each prompt
% e.g., max_reward - min_reward
% using the above metric as the weight for adaptive sampling to create an informative subset
% generating new prompts via a prompt generation policy 


% are many human values really worth to align?

% Central to our method is the informativeness measure 

% TODO: add plots of algo pipeline and performance.

% Two motivations: (i) the size of the prompt set is a bottleneck on existing alignment performance, and we need a robust way to continuously improve the alignment performance; (ii) naïvely training with more data could hurt the performance - this happens in both training from scratch  

% In~\citep{warm}, ``conventional intuition suggests that when solving a sequence of related optimization problem of this from, it should be possible to initialize using the solution of the previous iterate to ``warm start'' the optimization rather than ``initialize from scratch''. However, in practice this warm-starting seems to yield poorer generalization performance than models that have fresh random initialization.''

% Adding discussions on the re-warming and loss of plasticity literature; comparing with them.

% Adding discussions in the exploration literature of bandit and RL.



% We cast the preference alignment problem as an two-player asymmetric self-play game, while one player learns to propose the most informative prompt set, and the other player learns to best respond to the proposed prompt set. At the equilibrium, we expect to have the optimal policy of language generation for both players.

% % The simplifying assumptions underlying Bradley-Terry model cannot capture real-world human preferences, which are often intransitive.

% Self-play preference optimization~\citep{nlhf,rlhf-more-diff,self-play-gu} casts the alignment problem as a two-player, general-sum game, where each player is a policy, parameterized by the language model, that aims to optimize the probability of its responses to be preferred against the other player's. Existing works iteratively update the policy network for it to converge to the optimal policy characterizing by the Nash equilibrium, empirically showing it as a promising framework.

% However, a fundamental issue, which is often neglected by current algorithms, is that the initial prompt set may not adequately represent the full range of scenarios the model will encounter in the real world. This limitation can lead to policies that are optimal within the confined space of the initial prompts but suboptimal or even poorly performing when faced with a broader distribution of inputs.  
% %\notes{The reasoning gap could be one example.}
% %Moreover, as language models continue to evolve and improve, the nature and complexity of prompts that can effectively challenge and improve these models also change. This dynamic landscape necessitates a more adaptive approach to prompt selection and generation throughout the finetuning process. 

% % \notes{Rewrite this paragraph, and put emphasis only on the prompt set optimization part.}
% % However, several fundamental challenges arise when applying self-play alignment in the real world:
% % \begin{itemize}
% %     \item \textbf{Prompt Distribution Mismatch:} The assumption of sampling from a fixed prompt distribution $\mathcal{X}$ may lead to generalization issues. \notes{i.e., exploration in $p(x)$?}
% %     \item \textbf{Preference Uncertainty:} The preference oracle $\mathbb{P}(\cdot)$ may be noisy, biased, or limited in its capacity to judge all types of responses.\notes{This is like having two nested equilibriums; policy v. policy; generator v. discriminator.}
% %     \item \textbf{Response Space Constraints:} The model's ability to generate responses may not sufficiently cover the space of optimal responses. \notes{to rephrase; simply exploration for $p(y|x)$}
% % \end{itemize}

% % A useful prompt is often a \emph{surprising} prompt~\citep{ai-mathematician}.

% To address these challenges, we propose an \emph{evolving alignment} framework, with an \emph{asymmetric self-play} mechanism.

% Simply put, we consider to grow $\calX, \calY$, while existing work mostly care about $\calY \mid \calX$ with a fixed $\calX$.


    

    

==> texs_/intro.tex <==


%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
\vspace{+3.pt}
\section {Introduction}\label{sec:intro}\vspace{-5pt}
Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
High quality human data, crucial for scaling large language model (LLM) based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as LLMs become more capable, they need to solve increasingly complex or new challenges, requiring training data beyond abilities of humans to create. This necessitates a new fundamental mechanism for self-improving, where models can continuously self-generate and self-solve harder problems. We thereby investigate the research question below:
\begin{minipage}{1.\textwidth}
% \footnotesize
\centering\vspace{+4.5pt}
\textit{Can language models \emph{self-create} new, learnable tasks to work on,\\}
\textit{to \emph{self-improve} to \emph{generalize} better for human preferences alignment?}
\vspace{+2.5pt}
\end{minipage}
%or higher intelligence.


% \notes{One way to write the motivation part may be to follow ~\citep{poet,bengio2009curriculum,accel,paired}. Discuss how we incentivize the agent to generate prompt distribution with increasing complexity, promoting the models to solve harder problems.}

% \notes{Additional motivation/intuition/background paragraphs need to be added here. Motivate why we need to jointly optimize for both.}

% We aim to develop language agents capable of surpassing even superior intelligence, enabling them to solve increasingly complex problems.


% \vspace{-6pt}


% \vspace{+2pt}







% \vspace{-6pt}

\newpage
\vspace{-30pt}
Many preference optimization algorithms~\citep{rlhf,dpo,slic, self-play-gu,liu2023statistical, dpo-ai-feedback} have been proposed to improve the alignment of language models, however, they all default to  fixed prompt training distributions. Such fixed training paradigm inevitably leads to: (i) \emph{generalization issues} (models may underperform or hack on instructions that are insufficiently represented within the fixed set) and (ii) \emph{efficiency issues} (data annotation and model training are costly, however not all prompt provide the same utility; it is wasteful to invest in sub-optimal fixed set, while identifying informative prompts through human efforts is expensive and time-consuming)~\citep{team-1,gemma2,llama3}. 

The objective thereby should not only be to optimize over a specific, static distribution of prompts, yet to develop an agent that can autonomously evolve the training data distribution for self-improvement, to align well across unseen, novel environments or tasks (instantiated by prompts).

% rely on a static set of training prompts.

% , which can be viewed as a single \tb{solver step}. 

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.


Thus, we develop~\method~(\underline{E}volving Alignment \emph{\underline{v}ia} \underline{A}symmetric Self-Play), as illustrated in Figure~\ref{fig:game}. Central to our approach is a game with the minimax-regret objective, achieved through alternating optimization between \tb{creating prompts} and  \tb{solving them}. The interplay encourages evolving curricula~\citep{accel}, potentially benefits both generalization and efficiency (see also $\S$~\ref{sec:int}). Orthogonal to many recent self-play studies in LLM alignment~\citep{nlhf,srpo,self-play-gu}, \method~is \emph{asymmetric}~\citep{intrinsic}, with two policies of different goals:
\vspace{-3pt}
\begin{itemize}
    \item \textbf{Creator}: evolves the prompt distribution for alignment.
    \item \textbf{Solver}: produces responses and optimizes  alignment based on the evolving prompts.
\end{itemize}


% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 



% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.





Our main contributions are summarized as:
\begin{itemize}
\vspace{-3pt}
    \item \textbf{A new principle}: We propose a generalized \textbf{Open-Ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment, as in Definition~\ref{eq:rlhf-joint}.

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline, as in Algorithm~\ref{alg:i-eva}.
    
    \item \textbf{State-of-the-art performance}: We empirically validate our method on public alignment benchmarks and present general strong performance improvement when plugged in with different preference optimization algorithms (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide additional insights on the choice of informativeness metric, reward model, and training schedules, as in $\S$~\ref{sec:exp}.

\end{itemize}

\begin{figure}[t]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \caption{\textbf{Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our proposed~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with an easy-to-implement \emph{estimate, sample then evolve} procedure; specifically, it estimates the informativeness for each prompt by how contrastive the self-generated responses are to the prompt, from the reward signals it receives. The creator evolves new prompts  from highly informative prompts, which the solver uses for continual training. Both the solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective that drives the above design in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \vspace{-8pt}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure}



\method~\textbf{is easy to implement}. We hope it can serve as a scalable method for the research community to build \text{open-ended}, robust, and self-improving language agents, that align with human values.




==> texs_/lit-fix.tex <==
% \newpage
\section{\textcolor{Gray}{[Draft]} Related Works}

% to read: curriculum learning, trpo, self-rewarding llm.

% We here cite major relevant works and highlight the difference from our work. More detailed discussions can be found in the Appendix \textcolor{Maroon}{?}.

% We hereby cite the most relevant works and highlight the distinctions between them and our framework. A more comprehensive discussion is provided in the Appendix \textcolor{Maroon}{?}.

\paragraph{Self-improving algorithms and iterative optimization.} This line of work focuses on iteratively generating samples from the response policy and continuously re-training the policy by selected self-generated samples. Major works include ReST~\citep{rest, rest_em}, STaR~\citep{star}, RFT~\citep{rft}, RAFT~\citep{raft}, self-improving LLMs~\citep{llm-can-self-improve, self-reward}; in the context of preference optimization, iterative DPO~\citep{dpo-iterative,dpo-on-policy,snorkel,xiong2024iterative,rpo} has proven effective. Most works focus on self-training by improving in the $\calY \mid \calX$ space, we are the first to \emph{jointly optimize} both responses and prompts through generative exploration in the $(\calX, \calY)$ space. 
% \notes{We may add detailed comparison with~\cite{self-reward} on the usage of instructions.}
% Maybe we can explain this in a more clear way in the appendix. Check the self-play finetuning review in the sppo paper.

\paragraph{Prompt synthesis for language models.}  Existing works, such as Self-Instruct~\citep{self-instruct}, WizardLM~\citep{wizardlm,wizardmath}, Self-Align~\citep{self-align}, Glan~\citep{glan}, EvoPrompt~\citep{evoprompt}, Magpie~\citep{magpie} and others~\citep{survey-data}, primarily rely on supervised fine-tuning (\ie the SFT phase) to optimize language models. In contrast, our work (i) presents a new reward-driven metric to endow prompt the notion of informativenss; (ii) focuses on preference optimization (\ie the RLHF phase), and (iii) is supported by solid theoretical foundations.



% \notes{Most existing works consider to (i) uniformly evolve prompts, (ii) using the evolved prompts for SFT. Our works differ by proposing a prompt selection metric elicited from rewards, and utilizing the prompts for alignment.}

\paragraph{Self-play and curriculum RL.} Any agent trained on a fixed data distribution is often brittle and may struggle to adapt to the real world~\citep{open}. Self-play~\citep{checker,gan,alphago} addresses this by having the agent learn through self-interaction, thus creating more diverse experiences and automatic curricula. In asymmetric self-play, the paradigm centers on ``\emph{Alice proposing a task, and Bob doing it}''~\citep{intrinsic,maestro,minimax-refine,paired}. We\hide{are among the first to} rejuvenate the classical asymmetric self-play principle~\citep{horde} in optimizing language models. Unlike traditional curriculum RL~\citep{accel}, which usually renders environments from specified settings~\citep{paired}, our approach is \emph{generative} by nature, as we directly generate contexts (prompts) from the auto-regressive language models, guided by informativeness signals elicited from preferences.

% \paragraph{Self-play in RLHF.} There is a growing line of research that frame RLHF as two-player constant game, where both players are the response player compete to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between the response players, they still assume a fixed prompt distribution, while the most important thing of our approach is that we enable a dynamic prompt distribution useful for training. One similar concurrent work to ours is GPO~\citep{gpo}, however it is (i) designed for defend adversarial attack instead of general alignment; (ii) using PPO instead of direct preference optimization. We additionally present a summary table on other alignment algorithms in Appendix~\ref{app:table}.

\paragraph{Self-play in RLHF.} A growing line of research frames RLHF as a symmetric two-player game, where both players are the  response players competing to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between response players, these methods still rely on a fixed prompt distribution thus is sub-optimal. In contrast, our method  integrates evolving prompt distributions \textit{via} the asymmetric game setting\footnote{We notice one concurrent work adopting the asymmetric two-player setup~\citep{gpo}, however (i) it focuses on adversarial defense rather than general alignment, (ii) it uses PPO instead of direct preference optimization, and (iii) it uses the maxmin principle (which is known to be producing unlearnable environments~\citep{paired} and is not incentivized to guide the learning agents) instead of minimax \emph{regret} principle~\citep{fan1953minimax,savage1951theory} as we do.}.
% Additionally, our approach is more flexible and can be easily integrated into existing alignment pipelines. 

% \paragraph{Curriculum learning, active learning and evolution strategies.} Curriculum learning~\citep{bengio2009curriculum}; ordered SGD~\citep{ordered-sgd}, Active Preference Learning~\citep{active-pl}, Curry-DPO~\citep{curry-dpo},  Selective Reflection-Tuning~\citep{selective-rt}; . \notes{Existing works consider only \emph{re-weighting} or \emph{re-ordering} the data presented in training, while we propose to \emph{generate} new data based on, this resembles evolution strategies~\citep{es-openai}. }

\paragraph{Curriculum learning, active learning, and evolution strategies.} Existing methods, such as curriculum learning~\citep{bengio2009curriculum}, ordered SGD~\citep{ordered-sgd}, active preference optimization~\citep{active-pl,curry-dpo},  and selective finetuning~\citep{selective-rt}, focus on \emph{re-weighting} or \emph{re-ordering} the training data. In contrast, we propose a method that \emph{generates} new data based on preference signals, with similarities to evolution strategies~\citep{es-openai}. 





% \paragraph{Iterative (preference) optimization.} Self-improving LLMs~\citep{llm-can-self-improve},  self-rewarding LLMs~\citep{self-reward}, \citep{xiong2024iterative}, SRPO~\citep{srpo}, reasoning preference optimization~\citep{rpo}, ReST~\citep{rest}, Iterative DPO~\citep{snorkel}.

% \paragraph{Self-play LLMs.} Self-Reine, STaR, ReST, SPPO, SRPO.
% ~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}

% (Some somewhat relevant concurrent works: GPO~\citep{gpo}, SEAS~\citep{seas}, , )



% % \paragraph{Data Synthesis with LLMs.} EvoPrompt~\citep{evoprompt}, Self-Instruct~\citep{self-instruct}

% \paragraph{Self-improving algorithms.} General: \citep{def-open,open-endedness,continual-rl}. For LLMs: self-instruct~\citep{camel,self-instruct,evoprompt}, self-critique~\citep{camel}, self-debug~\citep{self-debug}. 

% \paragraph{Self-play and automatic curriculum generation.} \citep{checker,silver2017mastering}

% % \paragraph{Self-training.} 

% \paragraph{Online (contrastive) alignment algorithms.} 
% % Generating in the X space presents a fundamentally different challenge.

% % \paragraph{Evolving instructions for language model post-training.} 


==> texs_/lit.tex <==
\newpage
\section{Related Works}\label{sec:lit}
\vspace{-4pt}

% to read: curriculum learning, trpo, self-rewarding llm.

% We here cite major relevant works and highlight the difference from our work. More detailed discussions can be found in the Appendix \textcolor{Maroon}{?}.

% We hereby cite the most relevant works and highlight the distinctions between them and our framework. A more comprehensive discussion is provided in the Appendix \textcolor{Maroon}{?}.

\paragraph{Self-improving algorithms and iterative optimization.} This line of work focuses on iteratively generating samples from the response policy and continuously re-training the policy by selected self-generated samples. Major works include ReST~\citep{rest, rest_em}, STaR~\citep{star}, RFT~\citep{rft}, RAFT~\citep{raft}, self-improving LLMs~\citep{llm-can-self-improve, self-reward}; in the context of preference optimization, iterative DPO~\citep{dpo-iterative,dpo-on-policy,snorkel,xiong2024iterative,rpo} has proven effective. Most works focus on self-training by improving in $\calY \mid \calX$, while we \emph{jointly optimize} both responses and prompts via generative exploration in the $(\calX, \calY)$ space. Among them, we also distinctly present a game-theoretic framework with the minimax-regret principle  as the guidance. 
\vspace{-6pt}
% \notes{We may add detailed comparison with~\cite{self-reward} on the usage of instructions.}
% Maybe we can explain this in a more clear way in the appendix. Check the self-play finetuning review in the sppo paper.

\paragraph{Prompt synthesis for language models.}  Existing works include Self-Instruct~\citep{self-instruct}, WizardLM~\citep{wizardlm,wizardmath}, Self-Align~\citep{self-align}, Glan~\citep{glan}, EvoPrompt~\citep{evoprompt}, Magpie~\citep{magpie} and others~\citep{survey-data}. \method~is an orthogonal contribution since any synthesis method can be plugged in as the $\texttt{\small evolve}(\cdot)$ for the creator. Importantly, our work presents a new reward-related metric to endow prompt the notion of informativeness, with new implications as in $\S$~\ref{sec:int}. We also focus on preference optimization algorithms, while those existing works  primarily use synthesized prompts in an SFT-only way.
% supervised fine-tuning (\ie the SFT phase).
 
\vspace{-6pt}
% \notes{Mention that our work is an orthogonal contribution to this since we can plug in any prompt synthesis method -- just editting in the high-regret levels.}
% , and (iii) is supported by solid theoretical foundations.
% (\ie the RLHF phase)



% \notes{Most existing works consider to (i) uniformly evolve prompts, (ii) using the evolved prompts for SFT. Our works differ by proposing a prompt selection metric elicited from rewards, and utilizing the prompts for alignment.}

\paragraph{Self-play and curriculum RL.} Agents trained on a fixed data distribution are often brittle and may struggle to adapt to the real world~\citep{open}. Self-play~\citep{checker,gan,alphago} addresses this by having the agent learn through self-interaction, thus creating more diverse experiences and automatic curricula. In asymmetric self-play, the paradigm centers on ``\emph{Alice proposing a task, and Bob doing it}''~\citep{intrinsic,maestro,minimax-refine,paired}. We\hide{are among the first to} revive the classical asymmetric self-play principle~\citep{horde} in optimizing language models. Unlike traditional curriculum RL~\citep{accel}, which usually renders environments from specified levels~\citep{paired}, our approach is \emph{generative} by nature, as we directly generate contexts from the auto-regressive language models.
\vspace{-6pt}
% guided by informativeness signals elicited from preferences.

% \paragraph{Self-play in RLHF.} There is a growing line of research that frame RLHF as two-player constant game, where both players are the response player compete to generate more preferred responses~\citep{nlhf,self-play-gu,srpo,dno}. However, since the game is between the response players, they still assume a fixed prompt distribution, while the most important thing of our approach is that we enable a dynamic prompt distribution useful for training. One similar concurrent work to ours is GPO~\citep{gpo}, however it is (i) designed for defend adversarial attack instead of general alignment; (ii) using PPO instead of direct preference optimization. We additionally present a summary table on other alignment algorithms in Appendix~\ref{app:table}.
 % competing to generate more preferred responses
\paragraph{Self-play in RLHF.} A growing line of research frames RLHF as a \emph{symmetric} self-play game, where both players are response players~\citep{nlhf,self-play-gu,srpo,dno}. However,  these methods still rely on a fixed prompt distribution thus is sub-optimal. In contrast, we solve this by \emph{asymmetric} self-play, enabling evolving prompt distributions for more generalizable language agents. During our work, we notice one concurrent paper adopting the asymmetric two-player setup~\citep{gpo}, however (i) it applies to adversarial attack tasks instead of general alignment benchmarks, (ii) it is incompatible w/ direct preference optimization, and (iii) it relies on the maxmin principle (which is known to be producing unlearnable environments~\citep{paired}) instead of the minimax \emph{regret} principle~\citep{fan1953minimax,savage1951theory} as we do. We also first precisely defined the new problem of open-ended RLHF, which generalizes over classical RLHF.
\vspace{-6pt}
 % and is not incentivized to guide the learning agents
% Additionally, our approach is more flexible and can be easily integrated into existing alignment pipelines. 

% \paragraph{Curriculum learning, active learning and evolution strategies.} Curriculum learning~\citep{bengio2009curriculum}; ordered SGD~\citep{ordered-sgd}, Active Preference Learning~\citep{active-pl}, Curry-DPO~\citep{curry-dpo},  Selective Reflection-Tuning~\citep{selective-rt}; . \notes{Existing works consider only \emph{re-weighting} or \emph{re-ordering} the data presented in training, while we propose to \emph{generate} new data based on, this resembles evolution strategies~\citep{es-openai}. }

% \paragraph{Curriculum learning, active learning, and evolution strategies.} Existing methods, such as curriculum learning~\citep{bengio2009curriculum}, ordered SGD~\citep{ordered-sgd}, active preference optimization~\citep{active-pl,curry-dpo},  and selective finetuning~\citep{selective-rt}, focus on \emph{re-weighting} or \emph{re-ordering} the training data. In contrast, we propose a method that \emph{generates} new data based on preference signals, with similarities to evolution strategies~\citep{es-openai}. 





% \paragraph{Iterative (preference) optimization.} Self-improving LLMs~\citep{llm-can-self-improve},  self-rewarding LLMs~\citep{self-reward}, \citep{xiong2024iterative}, SRPO~\citep{srpo}, reasoning preference optimization~\citep{rpo}, ReST~\citep{rest}, Iterative DPO~\citep{snorkel}.

% \paragraph{Self-play LLMs.} Self-Reine, STaR, ReST, SPPO, SRPO.
% ~\citep{self-play-gu,xiong2024iterative,simpo,srpo,self-reward,rpo,snorkel,rest,rest_em}

% (Some somewhat relevant concurrent works: GPO~\citep{gpo}, SEAS~\citep{seas}, , )



% % \paragraph{Data Synthesis with LLMs.} EvoPrompt~\citep{evoprompt}, Self-Instruct~\citep{self-instruct}

% \paragraph{Self-improving algorithms.} General: \citep{def-open,open-endedness,continual-rl}. For LLMs: self-instruct~\citep{camel,self-instruct,evoprompt}, self-critique~\citep{camel}, self-debug~\citep{self-debug}. 

% \paragraph{Self-play and automatic curriculum generation.} \citep{checker,silver2017mastering}

% % \paragraph{Self-training.} 

% \paragraph{Online (contrastive) alignment algorithms.} 
% % Generating in the X space presents a fundamentally different challenge.

% % \paragraph{Evolving instructions for language model post-training.} 


==> texs_/method-cache.tex <==
\newpage
\section{Method}\label{sec:method}
Our objective is to develop LLMs that can \emph{self-improve  to generalize well on new, unseen tasks} beyond the initial training prompt distribution for alignment. 
In $\S$\ref{sec:principle}, we motivate by the limitations of existing RLHF frameworks and formally define the new objective of open-ended RLHF. Next in $\S$\ref{sec:mechanism}, we introduce the creator-solver game to tractably optimize the objective. Later in $\S$\ref{sec:algo}, we detail the practical algorithm compatible with any preference optimization method as the solver, with a creator in the loop. Lastly in $\S$\ref{sec:int}, we present further interpretations on the nice properties of~\method.

% We frame this as a creator-solver game: starting from a given prompt distribution, the creator identifies the region with the most learning potential using reward signals, then evolves prompts in those regions via proximal modifications; the solver then generates multiple responses to each of the evolved prompts and performs preference optimization based on reward annotation. We will precisely define the terminology used here as follows.

% The creator LLM and the solver LLM can share the same or different parameters. % maybe make this a footnote
% ~\notes{Revise this paragraph for intuitive motivation.}


% \textcolor{red}{[The method and algorithm section should be merged together and go directly to the point. The reader needs to wait for page 5 before having a clear understanding of what is the proposed method. Bring the presentation of the method sooner. Explaining that the method consists of two steps, creating prompts and solving them. Needs to appear asap in the presentation. Especially the choice of what is the creator optimising.]}

% to add more discussions. the initial RLHF fixed in a training set~\citep{rlhf}; we want the process to be open-ended (there are many informal or formal definitions of open-endedness~\citep{open-endedness}); two crucial characteristics are that 


% Our goal is to achieve high rewards on the unknown target distribution for prompts in the wild $\pi_{\text{target}}(\rvx)$, while maintaining the proximity of the response policy to the reference policy. Here, the newly introduced $\pi_{\text{target}}(\rvx)$  can be seen as an \emph{unspecified environment}~\citep{paired}.

% \tc{Discuss the issue of traditional RLHF, then lead to that we need a framework that can discover novel and learnable prompts to further improve the performance. In open-ended RLHF, we want to generate a distribution of prompts to continue to train the policy for preference optimization;}
%% RA.21.9: Before showing any math, probably worth motivating what we want to do -- the role of  theory is formalize things, which should be intutitive. 

% TODO: introducing the asymmetric self-play mechanism for language models.
% Essentially there are two 
\subsection{The Principle: Open-edned RLHF for Joint Self-Improvement}~\label{sec:principle}
\hspace{-6pt}\textbf{Intuition.} \ \ Classical RLHF (\textit{cf}., Eq.~\ref{eq:rlhf-cls}) optimizes over a static distribution, meaning that the agent is only aligned to a fixed reference point, making the agent brittle when it encounters new tasks or is evaluated on new benchmarks in the ever-changing real world, \ie \emph{the static optimization fails to adapt}. The idea behind our Open-Ended RLHF is to break away from this static framework, with the objective of developing an agent that generalizes well across \emph{unseen, novel} environments, where the prompts (tasks) may not have been explicitly encountered during training. To achieve this, we must design a new objective that moves beyond optimizing over a fixed dataset $\mathcal{D}$, allowing $\rvx$ to come from a dynamic, ever-changing distribution that co-evolves with the agent's ability to solve tasks.




\vspace{-4pt}
\paragraph{Formalization.} We formally define this by introducing an \emph{optimizable} prompt generation policy $\pi_{\vphi}(\rvx)$, which is \emph{jointly} optimized with the response policy $\pi_{\vtheta}(\rvy \mid \rvx)$, as follows:

\vspace{+1pt}


% \notes{First mention the limit of traditional RLHF here, then discuss why we need open-ended RLHF}
% \hspace{-8pt}The goal is to train a language agent that can perform well across the unknown target prompt distribution. We formalize the idea below.
% \vspace{-0.35cm}
\begin{mdframed}
\begin{defn}[Open-ended RLHF]\label{eq:rlhf-joint}
We define \emph{evolving alignment} as the open-ended joint optimization\footnote{\textcolor{black}{Classical RLHF (Eq.~\ref{eq:rlhf-cls}) is a special case when $\pi_{\phi}$ is  static as $p_{\text{ref}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint-}:}
\begin{align}
\max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\bigr[\ r(\mathbf{x}, \mathbf{y}) \ \bigr]   &- \textcolor{cred}{\sE}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cred}{\bigr[ \ }\textcolor{black}{\sD_{\text{KL}}\bigr[\textcolor{black}{\pi_{\theta}(\rvy | \rvx)} \| \pi_{\text{ref}}(\rvy | \rvx)\bigr]}\ \textcolor{cred}{\bigr]} 
- \textcolor{cred}{\sD_{\text{KL}}\bigr[\ \pi_{\phi}(\rvx) \| p_{\text{ref}}(\rvx)\ \bigr]}. \nonumber 
\end{align}}  on the prompt and response policy for alignment w.r.t the joint reference policy:
\begin{align}
    \max_{\vphi, \vtheta} \  J_{\vphi, \vtheta}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\emphinlinered{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}} \ , \ \emphinlinegreen{\textcolor{cgreen}{\rvy \sim \pi_{\vtheta}(\rvy|\rvx)}} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
    - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vphi, \vtheta}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)  } \ \Biggl], \label{eq:rlhf-joint-} \vspace{-5pt}
\end{align}
where $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ and $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$.
% denotes the training joint distribution and the reference joint distribution, respectively.
\end{defn}
\end{mdframed}
Here, $p_{\text{ref}}(\rvx)$ represents an idealized, potentially intractable probability measure over all possible tasks (instantiated \emph{via} prompts) in the wild. This is a conceptual reference  that encompasses the full diversity and complexity of tasks agents may encounter, serving as a guiding target for alignment. Additionally, the \emph{joint optimization} ensures that the task distribution and the agent’s response policy are updated in tandem, enabling adaptation to increasingly complex tasks, thereby promoting generalization.
 % or directly optimizable

% \begin{itemize}
%     \vspace{-4pt}
%     \item $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ is the joint policy for prompts and responses.
%     % \item $\tc{\emphred{\pi_{\vphi, \vtheta}(\rvx, \rvy) }} := \tc{\emphred{\pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}$ is the joint policy for prompts and responses.
%     \item $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$ is the reference joint distribution.
% \end{itemize}

% \begin{defn}[Evolving Alignment]
% Evolving alignment is the open-ended joint optimization\footnote{Classical RLHF is a special case when $\pi_{\phi}$ is a static distribution as $\pi_{\text{target}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint}:
% \begin{align}
% \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]   &- \textcolor{black}{\sE}_{\textcolor{black}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{black}{\Bigr[}\textcolor{black}{\sD_{\text{KL}}\Bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx)\Bigr]}\textcolor{black}{\Bigr]} 
% - \textcolor{black}{\sD_{\text{KL}}\Bigr[\pi_{\phi}(\rvx) \mid\mid \pi_{\text{target}}(\rvx)\Bigr]}. \nonumber
% \end{align}}  of the prompt distribution and response policy for alignment w.r.t the joint reference distribution, that is:
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\emphinlinered{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}} \ , \ \emphinlinegreen{\textcolor{cgreen}{\rvy \sim \pi_{\vtheta}(\rvy|\rvx)}} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vpsi}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
% \end{align}
% where $\vpsi = (\vphi, \vtheta)$ represents all parameters of the joint policy such that:
% \begin{itemize}
%     \item $\tc{\emphred{\pi_{\vpsi}(\rvx, \rvy) }} := \tc{\emphred{\pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}$ is the joint policy distribution for prompts and responses.
%     \item $\pi_{\text{ref}}(\rvx, \rvy) := \pi_{\text{target}}(\rvx) \cdot \pi_{\text{ref}}(\rvy \mid \rvx)$ is the reference joint distribution.
% \end{itemize}
% \end{defn}

% \notes{Revise the definition for more rigor and clarity.}


% We generalize the classical RLHF objective to jointly optimize over contexts and responses\footnote{Classical RLHF is a special case when $\pi_{\phi}$ is a static distribution as $\pi_{\text{target}}$. To see this, expanding Eq.~\ref{eq:rlhf-joint}:
% \begin{align}
% \max_{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}}\Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr]   &- \textcolor{cred}{\sE}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\phi}(\cdot)}}\textcolor{cred}{\Bigr[}\textcolor{black}{\sD_{\text{KL}}\Bigr[\textcolor{black}{\pi_{\theta}(\rvy \mid \rvx)} \mid\mid \pi_{\text{ref}}(\rvy \mid \rvx)\Bigr]}\textcolor{cred}{\Bigr]} 
% - \textcolor{cred}{\sD_{\text{KL}}\Bigr[\pi_{\phi}(\rvx) \mid\mid \pi_{\text{target}}(\rvx)\Bigr]}. \nonumber
% \end{align}}:
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{target}})\ := \ \mathbb{E}_{\textcolor{cred}{(\rvx,\, \rvy) \sim \pi_{\vpsi}(\rvx, \rvy)}}\Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \underbrace{\tc{\emphred{ \hspace{+5pt} \pi_{\vpsi}(\rvx, \rvy) \hspace{+5pt} }  }}_{  \tc{\emphred{  \pi_{\vphi}(\rvx)}} \cdot \tg{\emphgreen{\pi_{\vtheta}(\rvy \mid \rvx)}}   } \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
%     % \\ \underbrace{a}_{b}
% \end{align}
% \begin{align}
%     \max_{\vpsi} \  J_{\vpsi}(\pi_{\text{ref}})\ := \ \mathbb{E}_{\textcolor{cred}{\rvx\sim \pi_{\vphi}(\rvx)}, \tg{\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)}}\Biggr[ \ r(\rvx, \rvy) \ \Biggr]
%     - \beta \cdot  \sD_{\text{KL}}\Biggl[\  \emphred{ \tc{\pi_{\vpsi}(}\tc{\rvx}\tc{, \ } \tc{\rvy}\tc{)}} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)} \ \Biggl], \label{eq:rlhf-joint}
% \end{align}
% which can be equivalently written in the \emph{regret minimization form}, and we have:








% \begin{defn}[Evolving Alignment]
% Evolving Alignment describes the optimization process of the prompt distribution $\pi_{\vphi}(\rvx)$ and response policy $\pi_{\vtheta}(\rvy \mid \rvx)$ for alignment improvement with regard to the target distribution $\pi_{\text{target}}(\rvx)$.
% \end{defn}





% We propose a new objective:
% \begin{align}
% &\quad \max _{\vphi, \vtheta} \ \mathbb{E}_{\textcolor{cred}{\mathbf{x} \sim \pi_{\vphi}(\cdot)}, \textcolor{black}{\mathbf{y} \sim \pi_\vtheta(\cdot \mid \mathbf{x})}}[r(\mathbf{x}, \mathbf{y})] - \beta \cdot \sD_{\text{KL}}\Bigr[\textcolor{cred}{\pi_{\vphi}(\rvx)} \cdot \textcolor{black}{\pi_{\vtheta}(\rvy \mid \rvx)} \ \| \ \textcolor{cred}{\pi_{\text{target}}(\rvx)}\cdot \pi_{\text{ref}}(\rvy \mid \rvx))\Bigr],
% \end{align} 



\subsection{The Mechanism: Asymmetric Self-Play \emph{via} the Creator v.s. Solver Game}~\label{sec:mechanism}
% \notes{TODO: add explanation texts on how we could optimize this through alternating optimization, which naturally gives rise to the asymmetric self-play view.}
\hspace{-6pt}\textbf{Motivation.}\quad  It is challenging to directly optimize the objective in Eq.~\ref{eq:rlhf-joint-}, due to (i) the \textbf{intractability} of the unspecified target environment~\citep{paired}; (ii) the \textbf{instability} of joint differentiable optimization~\citep{gan}. We hereby propose an \textit{alternating optimization} solution by formulating evolving alignment as an asymmetric game between a creator and the solver. Mathematically, this is similar to RL optimization based on expectation-maximization~\citep{hinton-em, rest_em}, where the parameter $\vphi$ for the prompt distribution is fixed at each step.


% Instead of directly optimizing Eq.~\ref{eq:rlhf-joint}, we seek to optimize the performance in the worst-case scenario.  

% This motivate us to formulate the above self-improving alignment problem as an asymmetric self-play game with the minimax regret objective.



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.48\linewidth]{texs_/game.png}
%     % \caption{Game}
%     \label{fig:game}
% \end{figure}


% \subsubsection{The High Level: {Solver v.s. Creator}}\label{sec:high-level}
% \notes{In preliminaries, discuss the regret-based preference learning paradigm~\citep{cpl,regret-knox,regret-knox-0,open-problems}.}
% \notes{The upcoming subsections still needs lots of re-writing.}

% To start with, we first define the regret of a policy with regard to a prompt as follows\footnote{For simplicity, we here omit the KL divergence term and present a detailed discussion in Section~\ref{sec:int-dpo}.}:
% \begin{align}
%     \operatorname{Regret}(\rvx, \pi)=\max _{\pi^{\prime} \in \Pi_{\calX}}\Bigr[\ r\left(\rvx, \pi^{\prime}\right)-r(\rvx, \pi) \ \Bigr]
% \end{align}

% Instead of directly optimize for~\ref{eq:rlhf-joint}, we seek a minimax regret objective.

\textbf{Formalization.}\quad We formalize the alternating optimization as an asymmetric game as follows:
\vspace{-5pt}
\begin{itemize}
    \item $\emphredd{\text{\bf \tc{Creator}}}$ \hspace{+1pt}: the prompt player \textcolor{cred}{$\emphredd{\pi_\calX}$} that generates prompts for the solver to solve.
    \item  $\emphgreenn{\text{\bf \tg{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}}$ \hspace{+1pt}: the response player \textcolor{cgreen}{$\emphgreenn{\pi_{\calY \mid \calX}}$} (denoted as \textcolor{cgreen}{$\pi$} occasionally for simplicity).
    % , whose goal is to identify areas where the solver can improve and propose increasingly informative prompts for the solver to learn.
\end{itemize}

 
% Note the regularized \emph{reward maximization} in Eq.~\ref{eq:rlhf-cls} can be cast as \emph{regret minimization}~\citep{rl-maxent}.

We now illustrate objectives for both players. A proper goal for the \tg{solver} is to minimize regret~\citep{cpl}, \ie the difference in the reward of the current policy and the optimal policy:
\begin{align}
    \operatorname{Regret}(\rvx, \pi) = \mathbb{E}_{\rvy' \sim \pi(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr] - \mathbb{E}_{\rvy' \sim \pi^{\star}(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr].\label{eq:regret-pi}
\end{align}


Similar to unsupervised environment design~\citep{accel}, the \tc{creator} agent seeks to produce a series of prompt distributions that form a curriculum for the solver agent to improve its generalization across the vast target prompt distribution space and to solve even harder problems unseen in the initial distribution. This is often characterized by maximizing the regret for the solver,
which leads to the following result~\citep{cpl,regret-knox,regret-knox-0,open-problems}:
\vspace{+1pt}
\begin{mdframed}
\begin{rem}[Minimax Regret]
    If the solver-creator game reaches an equilibrium, the solver follows a minimax regret strategy, \ie it can produce preferred responses in all scenarios:
\begin{align}
    \textcolor{cgreen}{\pi^{\star}} \in \arg \min _{\tg{\pi \in \Pi_{\calY | \calX}}} \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}}  \ \mathbb{E} _{\tc{\rvx \sim \pi_{\calX}}}\Bigr[\ \operatorname{Regret}(\rvx, \tg{\pi}) \ \Bigr].\label{eq:minimax-regret}
\end{align}
\end{rem}
\end{mdframed}

% \begin{mdframed}
% \begin{rem}
%     When the solver-creator game reaches a Nash equilibrium, the solver follows a minimax regret strategy, \ie it is able to generate preferred responses for all solvable prompts.
% \begin{align}
%     \left(\textcolor{cgreen}{\pi^{\star}}, \textcolor{cred}{\pi_{\mathcal{X}}^{\star}}\right) \in \arg \min _{\tg{\pi \in \Pi_{\calY | \calX}}} \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}}  \ \mathbb{E} _{\tc{\rvx \sim \pi_{\calX}}}\Bigr[\ \operatorname{Regret}(\rvx, \tg{\pi}) \ \Bigr].\label{eq:minimax-regret}
% \end{align}
% \end{rem}
% \end{mdframed}


% \begin{align}
%     \left( \textcolor{cred}{\pi_{\mathcal{X}}^{\star}}, \textcolor{cgreen}{\pi^{\star}}\right) \in \arg \max _{\textcolor{cred}{\pi_{\mathcal{X}}} \tc{\in \Pi_{\mathcal{X}}}} \min _{\tg{\pi \in \Pi}} \ \mathbb{E}_{\tc{\rvx \sim \pi_{\calX}}}\left[\operatorname{Regret}(\rvx, \tg{\pi})\right]
% \end{align}


% TODO: change the sequence and add the KL terms


% \subsubsection{The low Level: Solver v.s. Solver}\label{sec:low-level}
% Without direct access to the optimal policy, we choose to approximate the regret via the value obtained by two competing solvers: 
% \begin{align}
% \left(\tg{\pi^{\star}}, \tg{\pi^{\prime\star}}\right)=\arg \max _{\pi \in \Pi} \min _{\pi^{\prime} \in \Pi^{\prime}} \mathbb{E}_{\rvx\sim \mathcal{X}}\left[\mathbb{E}_{\rvy \sim \pi(\cdot \mid \mathbf{x}), \rvy^{\prime} \sim \pi^{\prime}(\cdot \mid \rvx)} \left[\mathbb{P}\left(\rvy \succ \rvy^{\prime} \mid \rvx\right)\right]\right]
% \end{align}

% \notes{We might need to revise this to make it more aligned with our setting; \ie sample multiple responses (actions), then using the reward discrepancy between the best and the worst (or the average) as the \emph{regret proxy}.}

% \subsubsection{Putting Together: The Dual Minimax Regret and Automatic Curricular}
% The overall objective can thus be expressed as:
% \begin{align}
%     \left(\tc{\pi_{\mathcal{X}}^{\star}}, \tg{\pi^{\star}}, \tg{\pi^{\prime \star}}\right)=\arg \max _{\pi_{\mathcal{X}} \in \Pi_{\mathcal{X}}} \max _{\pi \in \Pi} \min _{\pi^{\prime} \in \Pi^{\prime}} \mathbb{E}_{\rvx \sim \pi_{\mathcal{X}}}\left[\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \rvx\right)\right]
% \end{align}


Without access to the true optimal policy, we must approximate the regret. We choose to use variants of advantage functions for the approximation, as shown in Table~\ref{tab:info-metric}, which we also refer as the informativeness proxy\footnote{Note that some works~\citep{plr,active-pl} had tested using Shannon entropy as the informativeness metric, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage more future studies into this.}, with $A^{\star}_{\min}$ as the default proxy due to its relation to minimax regret in Eq.~\ref{eq:minimax-regret}.
\vspace{+1pt}
\begin{mdframed}
\begin{defn}[Informativeness Proxy]
    We use the minimax regret as the proxy for the informativeness metric of the prompt, approximated by the (absolute) worst-case optimal advantage:
\begin{align}
    \text{info}(\rvx) \gets A_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | 
\end{align}
\end{defn}
\end{mdframed}


To calculate the empirical value of $A^{\star}_{\min}$ for  each prompt, we first sample multiple responses from the prompt, where we label each response with its reward, then we use the difference between the highest reward $r_{\max}$ and the lowest reward $r_{\min}$ to represent the informativeness proxy. This proxy enjoys many nice properties, which we present an in-depth discussion in $\S$~\ref{sec:int}.


\subsection{The Practical Algorithm}~\label{sec:algo}
\hspace{-6pt}Next, we illustrate \method~of Algorithm~\ref{alg:i-eva} in details, with  implementation specifications in Appendix~\ref{app:settings}.

The full pipeline is that we combine the creator and solver step in an iterative preference optimization pipeline.

\subsubsection{\tb{\emphtextred{The Creator Step}}:  Estimate, Sample then Evolve}\label{sec:creator-step}
\textbf{Intuition.}\quad We find prompts with the most learning potential and generatively evolve them. This is similar to curriculum RL~\citep{accel} which finds environments with high-regret levels and edit within some distance, or the evolution strategies~\citep{schwefel1977evolutionsstrategien} which find the most promising species then mutate and crossover. As in Section~\ref{sec:mechanism}, we do not seek a differentiable creator for optimization in this work. The creator is implemented in three steps as in Figure~\ref{fig:pipeline}. 
\vspace{-5pt}

% \textbf{$\emphgray{\texttt{sample}(\cdot)}$ -- weighted sampling for an informative subset.}
% We then sample a prompt set with high learning potential. This is achieved by weighted sampling using the informativeness metric as the weight.

% \textbf{$\emphgray{\texttt{evolve}(\cdot)}$ -- evolving for a proximal region of high-advantage prompts.}

% This gives a simple heuristic: sampling multiple responses from the LLM, then using the maximal reward minus the minimal reward, $r_{\max} - r_{\min}$ as the reward for the creator, thus incentivizing the creator to generate more such prompts.

\paragraph{Step 1: $\emphgray{\texttt{\small info}(\cdot)}$ -- estimate the informativeness.} For each prompt $\rvx$ in the initial prompt set $\calX_t$, we generate responses, annotate rewards and calculate a informativeness metric to $\rvx$ as in Table~\ref{tab:info-metric}.\vspace{-3pt}

\paragraph{Step 2: $\emphgray{\texttt{\small sample}(\cdot)}$ -- weighted sampling for an informative subset.} Using the informativeness metric as the weight,
we sample a smaller informative prompt set $\calX_t^{\texttt{\tiny info}}$ (\eg 20\% of the original). \vspace{-3pt}

\paragraph{Step 3: $\emphgray{\texttt{\small evolve}(\cdot)}$ -- evolving for a proximal region of high-advantage prompts.} Our method does not rely on any specific evolving method. We take \text{EvolInstruct}~\citep{wizardlm} as an off-the-shelf baseline evolving method, which conducts in-depth (\ie, adding constraints, deepening, concretising, complicating) and in-breadth evolving (\ie mutation) by meta-instruction (\ie using an LLM to re-write the original prompts with the aforementioned evolving directions). Specifically, we iterate over each prompt in the $\calX_t^{\texttt{\tiny info}}$, where each prompt is evolved to multiple (\eg 4) variations, then mix the newly generated prompts with a uniformly sampled buffer from $\calX_t$ to create $\calX_{t+1}$.


\subsubsection{\tb{\emphtextgreen{The Solver Step}}: Solve then Optimize}
This step is the classical preference optimization algorithm~\citep{dpo,simpo}, where responses are generated and the gradient descent is performed, as shown in Algorithm~\ref{alg:i-eva}.



% \paragraph{Further Interpretations on the Informativeness Proxy.} \tc{[Discuss further interpretations.]}
\subsection{Further Interpretation on the Informativeness Proxy}\label{sec:int}
\tc{An important contribution of our work is proposing the metric for preference optimization; so worth having a subsection somewhere on this.}
\paragraph{Learning potential.} Finding the prompts where the agent is weak, but still solvable.

\paragraph{Worst-case guarantees.}

\paragraph{Auto-curricula for the creator.}
the advantage can be generalized as the reward difference between a base solver and a reference solver, where the creator is incentivized to produce new prompts that are just out of the comfort zone of solvers~\citep{zone-promximal}:
\vspace{-4pt}
\begin{itemize}
    \item For very complex prompts, both solutions may perform poorly, leading to low regret proxy.\vspace{-2pt}
    \item For very simple prompts, the base solution already performs well, giving low regret proxy.\vspace{-2pt}
    \item The optimal strategy is to find prompts that are just beyond the solvers’ current capability.
\end{itemize}


\paragraph{Auto-curricula for the \textnormal{\textit{contrastive}} solver.} 
Another nice property of our informativeness metric (\eg $A^{\star}_{\min}$) is that it matches the curriculum learning property with the DPO loss. In the specific case of contrastive preference optimization~\citep{cpl,dpo}, the loss is monotonically smaller as $\bdlog$ gets larger. This justifies our use of $r_{\max} - r_{\min}$ as the informativeness metric to prioritize the training examples according to the curriculum learning literature~\citep{easy-bengio2009curriculum}\footnote{We follow the curriculum learning literature that prioritizes examples with smaller losses for improvement in convergence and generalization. There is another line of work in optimization that claims examples with higher losses should be prioritized~\citep{hard-losers,hard-obs,hard-osgd,ordered-sgd}; however, \cite{rho-loss} conjecture that those example are often noisy (not learnable) or irrelevant thus are impractical. Our empirical results in Section~\ref{sec:ab-metric} on confirms this.}, which is essentially the reward of the chosen response ($r_{\max}$) minus the reward of the rejected response ($r_{\min}$), that is:
\begin{align}
    \emphgray{A^{\star}_{\min}(\rvx)}  = \beta \cdot \textcolor{black}{\emphgray{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}}}  \ \approx \ \emphgray{r_{\max} - r_{\min}}.
\end{align}
In this way, we incentivize the creator to generate prompts that \emph{bring the most contrastive responses}\footnote{One direction that worth to explore could be to directly use $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ instead of the reward proxy.}, that improves the convergence and generalization of the solver, formalized as below:
\begin{hypo}[Contrastive Curriculum Hypothesis]
    In direct preference optimization, prioritizing prompts w/ \emph{higher contrastive ratio} improves sample efficiency and generalization.
\end{hypo}




% \begin{itemize}
%     \item \textbf{Worst-case guarantee} for generally capable agents:
%     \item \textbf{Curriculum effect for the creator}: This is analogous to the solver \emph{v.s.} solver game~\citep{paired,dcd}, where the advantage can be generalized as the reward difference between a base solver and a reference solver. This naturally induce a curriculum effect, where the creator is incentivized to produce new prompts that are just out of the comfort zone of the solver~\citep{zone-promximal}.
%     \item \textbf{Curriculum effect for the solver}: 
%     \item \textbf{Learning potential}:
% \end{itemize}

% \notes{Maybe move the interpretation on the informativeness metric upward here. including: (i) \textbf{worst-case guarantee} for generally capable agents; (ii) \textbf{curriculum effect for the creator}; (iii) \textbf{curriculum effect for the contrastive solver}; (iv) learning potential. }














% \subsection{Further Interpretation via Contrastive Preference Optimization}\label{sec:int-dpo}

% \textcolor{red}{[How do compute rmax and rmin in practice? This needs to be explained more clearly.]}

% \textcolor{red}{[More time needs to be spent on explaining how the informativeness measure is computed in practice and how the prompts are evolved. Those are the two major steps in the algorithm and it is quite important for readability and reproducibility that the presentation focuses on those.]}





% -------------------------

% \subsubsection{Further Interpretation from Continual Deep Learning}\label{sec:int-cont}
% {\color{red} RA.9.26: This sounds like a para for related work possibly along with the footnote}


% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------
% , which accelerates the learning.

% \footnote{While we may directly select data with $\bdlog$, the usage of $r_{\max} - r_{\min}$ provides a fast approximation to the empirical contrastive ratio.}.



% \footnote{This presents another message on adaptively adjusting the , we should adaptively choose the informativeness metric when we use different optimization algorithms.}




% The overall objective can be expressed as:
% \begin{align}
%     (\emphtactic{\pi_\mathcal{X}^\star}, \emphgoal{\pi^{\prime\star}}, \emphgoal{\pi^{\star}}) \in \arg \emphtactic{\max_{\pi_\mathcal{X} \in \Pi_\mathcal{X}}} \ \emphgoal{\max_{\pi^{\prime} \in \Pi^{\prime}}} \ \emphgoal{\min_{\pi \in \Pi}} \ \mathbb{E}_{\vx \sim \pi_\mathcal{X}} \left[ \emphgold{\mathbb{P}\left(\pi^{\prime} \succ \pi \mid \vx \right)} \right].
% \end{align}

% TODO: introducing the new loss design. We may leave this as a theoretical version.

% \subsubsection{The New Loss Design}
% (TODO: make this general then use different inner-loop derivation)
% \begin{align}
%     \nabla_\theta \mathcal{L}\left(\pi_\theta ; \pi_{\text {ref}}\right)= 
%     -\beta \mathbb{E}_{\rvx \sim \pi_\theta(\rvx), (\rvy_w, \rvy_l) \sim \pi_\theta(\rvy|\rvx)}[&\sigma\left(\hat{r}_\theta\left(\rvx, \rvy_l\right)-\hat{r}_\theta\left(\rvx, \rvy_w\right)\right) \nonumber \\
%     &[\nabla_\theta \log \pi_\theta(\rvx) + \nabla_\theta \log \pi_\theta\left(\rvy_w \mid \rvx\right)-\nabla_\theta \log \pi_\theta\left(\rvy_l \mid \rvx\right)]]. \nonumber
% \end{align}


% \begin{figure}[H]
% \centering
% \begin{minipage}{0.46\textwidth}
%     \includegraphics[width=\textwidth]{texs_/mechanism.png}
%     \caption{\text{The creator step of Algorithm~\ref{alg:i-eva}.} }
%     \label{fig:mechanism}
% \end{minipage}
% \hfill
% \begin{minipage}{0.49\textwidth} 
% In Algorithm~\ref{alg:i-eva}, we illustrate a practical algorithm for~\method. Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{simpo}.
% \end{minipage}
% \end{figure}
% \vspace{-10pt}


% Specifically, we introduce a new \text{\tc{creator step}} for evolving the prompt distribution during preference optimization, which can be plugged on top of any existing alignment algorithm. These existing algorithms can be seen as containing only the \tg{solver step}, where responses are generated, and gradient descent is performed. By adding the \tc{creator step}, we introduce dynamic prompt generation, extending the optimization process beyond the static prompts used in conventional methods~\citep{simpo}.



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.48\linewidth]{texs_/mechanism.png}
%     \caption{\text{The creator step of Algorithm~\ref{alg:i-eva}.} }
%     \label{fig:mechanism}
% \end{figure}

% We illustrate a practical algorithm for~\method~in Algorithm~\ref{alg:i-eva}. We introduce an additional \text{\tc{creator step}} for  an evolving prompt distribution during preference optimization, which can be plugged on top of any alignment algorithms (which can be seen come with only the \tg{solver step} that generates responses.).

% \newpage
% \notes{Re-writing this part to make the evolving part more clear. Essentially, this is a bit like~\citep{accel}, which we make edits at the proximal region of the prompts which have high learning potential.}
% As shown in Fig~\ref{fig:pipeline}, the \tc{creator step} can be practically implemented by three steps:
% \begin{enumerate}
%     \item \textbf{Estimate} the informativeness for each prompt.

%     \begin{itemize}
%         \item Under the minimax regret game, we use the worst-case optimal advantage for each prompt $\rvx$, that is $\widehat{A}^{\star}_{\min}(\rvx)=r_{\max}(\rvx)-r_{\min}(\rvx)$, to measure their informativeness.
%     \end{itemize}
    
%     \item \textbf{Sample} an subset of prompts by the informativeness weight.
    
%     \item \textbf{Evolve} a new prompt set from the subset, mix with a buffer of the seed prompts.
% \end{enumerate}

% \notes{Add a table or color code to illustrate the difference from existing works.}

% \subsection{The Informativeness Measure by Reward Models}
% The non-trivial part here is leveraging the reward model to elicit informativeness of prompts.

% \subsubsection{\textnormal{\textbf{\texttt{eva-i}}}: The Iterative Off-Policy EVA Algorithm}\label{sec:eva-i}

% For simplicity, we remove subscripts and the superscripts for sets.
% We introduce an additional creator step that can be plugged into any alignment algorithms.

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% % -------------------------------------------
% \subsection{The Practical Algorithm}~\label{sec:algo}
% \hspace{-6pt}In Algorithm~\ref{alg:i-eva}, we illustrate a simple practical algorithm for~\method, where the details of $\texttt{info}(\cdot)$, $\texttt{sample}(\cdot)$ and $\texttt{evolve}(\cdot)$ are shown in Section~\ref{sec:creator-step}.  We use iterative off-policy (\method\texttt{\textbf{-i}}) training as our baseline setting, which is popularly adopted in recent works~\citep{dpo-iterative,snorkel,self-play-gu}. In this setup, the prompt set $\calX$ represents the full or a partition of the full dataset, with each iteration corresponding to a complete pass over this set\footnote{Our algorithm can be easily made on-policy, where the prompt set $\calX_t$ is essentially a mini-batch or a mini-pool (from which we sample mini-batches). We present the algorithm in Appendix~\ref{app:eva-o}.}.
% % ------------------------------------

% {
% \noindent
% \centering
% \begin{minipage}{.8\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
%     % , sample size of responses per prompt $n$ 
%     \Statex

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{{creator step}}}
%         \State \tb{\emph{self-generate responses}:} \hspace{+25pt}\tb{$\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ }
%         %\Comment{self-generate $\rvy$}
%         % \vspace{+2.5pt}
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$
%         \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{ ({\vy^{(j)}_i}, {r^{(j)}_i})\}$}

%         % \Statex \hspace{+11pt}   \tb{\emph{annotate rewards}:} \hspace{+47pt}\tb{$\calX_{t} \gets \calX_t \cup \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}\}$} 
%         %\Comment{annotate reward}
%         % \vspace{+0.1pt}
        
%         \vspace{+5pt}
%         \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \calX_t \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}$ 
        
%         % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\calX_{t} \gets \{(\rvx_i, \tb{\texttt{info}(\rvx_i)}\}$ 
%         % where $\texttt{info}_i = f(\calD_{t}[i])$ 
%         %\Comment{estimate information}
%         \vspace{+2pt}
        

%         \Statex \hspace{+11pt}  \tb{\emph{sample subset}:} \hspace{+60pt}$\calX_{t}^{{ {\texttt{info}}}} \gets \tb{{\textbf{\texttt{sample}}}(\mathcal{X}_{t})}$ 
%         %\Comment{sample the informative subset}
%         \vspace{+2.5pt}

%         \Statex \hspace{+11pt} \tb{\emph{self-evolve prompts}:} \hspace{+40pt}$\mathcal{X}_{t}^{\prime} \leftarrow \tb{\textbf{\texttt{evolve}}(\calX_{t}^{\texttt{info}})}$ 
%         %\Comment{self-evolve $\rvx$}

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
        
%         \State \tb{\emph{self-generate responses}:} \hspace{+26pt} $\forall$ $\vx_i \in \mathcal{X}_{t}^{\prime}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 
%         %\Comment{self-generate $\rvy$}
        
%         \Statex \hspace{+11pt} \tb{\emph{annotate rewards}:} \hspace{+48pt} $\calX_{t}^{\prime} \gets \calX_{t}^{\prime} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 
%         %\Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \vspace{+2.5pt}
        
%         \State \tb{\emph{preference optimization}:}$ \hspace{+32pt} \boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calX'_t}(\boldsymbol{\theta})$ 
%         %\Comment{preference optimization}

%         \Statex

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }


% It is easy to see that this algorithm can be made on-policy, or off-policy (which is faster). To illustrate:
% \vspace{-5pt}
% \begin{itemize}
%     \item \texttt{eva-o}: for the on-policy version, the seed prompt set $\calX_t$ is essentially a mini-batch or a mini-pool (from which we sample mini-batches), and each episode is one optimization step.

    
%     \item \texttt{eva-i}: for the off-policy version, the seed prompt set is the full dataset; and each episode is one full iteration over the dataset, containing multiple optimization steps.\vspace{-5pt}
%     %This resembles~\citep{dpo-iterative}.
% \end{itemize}
% By removing the creator step, we can recover the classical  (iterative) preference optimization algorithm~\citep{cringe,snorkel,dpo-iterative}.



% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Iterative \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-i})}} }\label{alg:i-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{episode} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State $\forall$ $\vx_i \in \mathcal{X}_{t-1}$,  sample $\{{\vy^{(j)}_i}\}^{n}_{j=1} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ \Comment{self-generate $\rvy$}
%         % \vspace{+2.5pt}
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$

%         \State $\mathcal{D}_{t-1} \gets \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{n}_{j=1}\}_{i = 1 }^{|\calX_{t-1}|}$ \Comment{annotate reward}
%         % \vspace{+0.1pt}

%         \Statex \hspace{+11pt} $\calI_{t-1} \gets \{(\rvx_i, \texttt{info}_i)\}_{i = 1 }^{|\calX_{t-1}|}$ where $\texttt{info}_i = f(\calD_{t-1}[i])$ \Comment{estimate information}
%         \vspace{+2.5pt}

%         \State $\calX_{t-1}^{\texttt{info}} \gets \textsc{Sample}(\mathcal{X}_{t-1} \mid \calI_{t-1})$ \Comment{sample the informative subset}

%         \Statex \hspace{+11pt} $\mathcal{X}_{t} \leftarrow \textsc{Evolve}(\calX_{t-1}^{\texttt{info}})$ \Comment{self-evolve $\rvx$}

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{X}_{t}$,  sample $\{{\vy^{(j)}_i}\}^{n}_{j=1} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ \Comment{self-generate $\rvy$}
%         \State  $\mathcal{D}_{t} \gets \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{n}_{j=1}\}_{i \in |\calX_{t}|}$ \Comment{reward annotation}
%         % \State update $\vtheta_{t-1}$ to $\vtheta_{t}$ by preference optimization on $\mathcal{D}_{t}$
%         \State $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calD_t}(\boldsymbol{\theta})$ \Comment{preference optimization}

%         \Statex

%         % \LineComment{\textcolor{Black}{Response generator step}}

%         % \State $\vtheta_{t} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: The On-Policy EVA Algorithm}\label{sec:eva-o}
% % ~\citep{ordered-sgd}
% % Naïvely, this can also be considered as a variant of ordered gradient descent with generative data augmentation. At each step, we first uniformly select a pool (e,g., with 8 examples) from the original; then form a subset (e.g., with 2 examples) and evolve a new batch (e.g., each evolving 2), then train with 2 (top original) + 2 (random original) + 4 (evolved). In this way, we create an online data curriculum with newly generated data. 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{Online \underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play (\texttt{eva-o})}} }\label{alg:o-eva}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, initial prompt set $\mathcal{X}_0$, informative subset size $n_{\calI}$, pool size $n_{\calP} \geq n_{\calI}$, mini-batch size $n_{\calB}$, sample size of responses per prompt $n$
%     \Statex

%     \For{\textbf{step} $t = 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{\textcolor{cred}{creator step}}
%         \State sample a input data pool $\calP_t$ of size $n_{\calP}$ from $\calX_0$
        
%         \State $\forall \vx_i \in \calP_t$, generate responses and annotate rewards, then compute its informativeness
        
%         \State Choose $\calP_t^{\texttt{info}} \leftarrow\left\{\left(\boldsymbol{x}_i, \texttt{info}_i\right)\right\}_{i=1}^{n_{\calI}}$, the \textbf{top}-$n_{\calI}$ samples in $\calP_t$ in terms of informativeness

%         \State Obtain $\calB_t = \textsc{Evolve}(\calP_t^{\texttt{info}})$

%         \Statex
        
%         \LineComment{\textcolor{cgreen}{solver step}}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\forall$ $\vx_i \in \mathcal{B}_{t}$, generate responses and annotate rewards
        
%         \State  $\boldsymbol{\theta}^{t} \leftarrow \boldsymbol{\theta}^{t-1}-\eta \nabla_{\boldsymbol{\theta}} \mathcal{L}_{\calB_t}(\boldsymbol{\theta})$, do mini-batch preference optimization

%         \Statex
        
%     \EndFor
%     \State \Return final solver policy $\pi_{\vtheta_T}(\cdot \mid \cdot)$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }



% \newpage
% \section{\textcolor{Gray}{[1\% Draft]} Method}


% % Essentially there are two 

% {
% \noindent
% \centering
% \begin{minipage}{.96\linewidth}
%   \begin{algorithm}[H]
%     \small
    
%     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
%     \begin{algorithmic}[1]
%     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$, preference oracle $\mathbb{P}$, learning rate $\eta$, number of generated samples $K$, initial prompt set $\mathcal{X}_0$
%     \Statex

%     \For{$t = 0, 1, 2, \ldots$}
%         \Statex 
        
%         \LineComment{prepare the training dataset}
%         \State for all $\vx_i \in \mathcal{X}_t$,  sample $\{{\vy^{(j)}_i}\}^{K}_{j=1} \sim \pi_{\vtheta_t}(\cdot \mid \mathbf{x})$
        
%         % \State annotate the win-rate $\mathbb{P}(\vy_k \succ \vy_{k'} \mid \mathbf{x})$, $\forall k, k' \in [K]$

%         \State annotate the preference and form the dataset $\mathcal{D}_t = \{(\mathbf{x}_i, \{{\vy^{(j)}_i}, {r^{(j)}_i}\}^{K}_{j=1}\}_{i \in [N]}$

%         \Statex
        
%         \LineComment{update policy (any other loss can be plug-in as well)}
%         % \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \mathbb{E}_{(\mathbf{x}, \vtau, \widehat{P}) \sim \mathcal{D}_t} \left(\log \frac{\pi_{\vtheta}(\vtau \mid \mathbf{x})}{\pi_{\vtheta_t}(\vtau \mid \mathbf{x})} - \eta(\widehat{P}(\vtau \succ \pi_{\vtheta_t} \mid \mathbf{x}) - \frac{1}{2})\right)^2$
%         \State $\vtheta_{t+1} \leftarrow \arg\min_{\vtheta} \calL_{\vtheta}(\cdot)$

%         \Statex
        
%         \LineComment{evolve the prompt distribution from learned metric}
%         \State $\calI_t(\mathbf{x}) \leftarrow \textsc{Assess}(\pi_{\vtheta_{t+1}}, \mathbf{x})$, $\forall \mathbf{x} \in \mathcal{X}_t$
        
%         \State $S_t \leftarrow \textsc{Evolve}(\pi_{\vtheta_{t+1}}, \calI_t, \mathcal{X}_t)$
        
%         \State $\mathcal{X}_{t+1} \leftarrow \textsc{Update}(\mathcal{X}_t, S_t)$

%         \Statex
%     \EndFor
%     \State \Return Final policy $\pi_{\vtheta_T}$
%     \end{algorithmic}
%   \end{algorithm}
% \end{minipage}
% \par
% }

% % \subsection{Regret and Minimax Framework}

% % Our goal is to design a self-improving agent that continually expands its capabilities through generative exploration. We formulate this using a minimax regret objective, which provides performance guarantees across an evolving distribution of prompts.

% % Let $\mathcal{X}$ be the space of prompts, $\mathcal{Y}$ the space of responses, and $\Pi$ the space of policies. We define regret as:

% % \begin{align}
% %     \text{Regret}(\vx, \pi) &= \max_{\pi^\star \in \Pi} [V(\vx, \pi^\star) - V(\vx, \pi)]
% % \end{align}

% % where $V(\vx, \pi) = \mathbb{E}_{\vy \sim \pi(\cdot \mid \vx)}[r(\vx, \vy)]$ is the value function, with $r(\vx, \vy)$ being the reward for response $\vy$ to prompt $\vx$. This formulation quantifies the difference in performance between a given policy $\pi$ and the best possible policy $\pi^\star$ for a given prompt $\vx$.

% % We then introduce a prompt player $\pi_X: \mathcal{H} \rightarrow \Delta(\mathcal{X})$, where $\mathcal{H}$ represents the interaction history. The minimax regret objective is:

% % \begin{align}
% %     J^\star &= \min_{\pi \in \Pi} \max_{\pi_X} \mathbb{E}_{\vx \sim \pi_X} [\text{Regret}(\vx, \pi)]
% % \end{align}

% % This formulation aims to find a policy $\pi$ that minimizes the worst-case regret across all possible prompt distributions. At equilibrium, this guarantees that the chosen policy $\pi$ performs robustly across the entire prompt space $\mathcal{X}$.

% % \subsection{Proxy for Regret Computation}

% % Computing the regret directly is infeasible as we lack access to the optimal policy $\pi^\star$. We therefore introduce a proxy using two policies: a base policy $\pi$ and an improvement policy $\pi_\dagger$. The regret proxy is defined as:

% % \begin{align}
% %     \text{Regret}_\text{proxy}(\vx, \pi, \pi_\dagger) = \max_{\pi_\dagger} \min_\pi [\emphgoal{p(\vy_2 \succ \vy_1 \mid \vx)} - \beta D_\text{KL}(\pi_\dagger \parallel \pi_\text{ref} \mid \vy_1, \vx) + \beta D_\text{KL}(\pi \parallel \pi_\text{ref} \mid \vx)] \nonumber
% % \end{align}

% % where $\vy_1 \sim \pi(\cdot \mid \vx)$, $\vy_2 \sim \pi_\dagger(\cdot \mid \vy_1, \vx)$, and $p(\vy_2 \succ \vy_1 \mid \vx)$ is the probability that $\vy_2$ is preferred to $\vy_1$ given $\vx$.

% % This proxy serves as an approximation of the true regret for several reasons:

% % \begin{itemize}
% %     \item The term $p(\vy_2 \succ \vy_1 \mid \vx)$ captures the improvement of $\pi_\dagger$ over $\pi$, analogous to the value difference in the true regret.
% %     \item The KL divergence terms encourage exploration of the policy space while maintaining proximity to a reference policy, mimicking the search for the optimal policy in the true regret.
% %     \item The max-min formulation reflects the adversarial nature of finding the largest possible improvement, similar to finding the optimal policy in the true regret.
% % \end{itemize}

% \subsection{Combined Objective}

% Incorporating this proxy into our original objective, we obtain:

% \begin{align}
%     J^\star = \min_\pi \max_{\pi_\dagger} \min_{\pi_X} \mathbb{E}_{\vx \sim \pi_X, \vy_1 \sim \pi, \vy_2 \sim \pi_\dagger} [\text{Regret}_\text{proxy}(\vx, \pi, \pi_\dagger)]
% \end{align}

% \subsection{Curriculum Effect}

% This formulation naturally induces a curriculum effect. The prompt player $\pi_X$ is incentivized to generate prompts that maximize the regret proxy, leading to a progression of challenges:

% \begin{itemize}
%     \item For prompts where $\pi$ performs poorly but $\pi_\dagger$ can improve, $p(\vy_2 \succ \vy_1 \mid \vx)$ will be high, increasing the regret proxy.
%     \item The KL divergence term $D_\text{KL}(\pi \parallel \pi_\text{ref} \mid \vx)$ will be larger for prompts that challenge $\pi$, further increasing the regret proxy.
%     \item As $\pi$ improves on certain prompts, $\pi_X$ must generate new, more challenging prompts to maintain a high regret proxy.
% \end{itemize}

% This mechanism ensures that $\pi_X$ continuously generates prompts just out of the comfort zone of $\pi$'s capabilities. The regret proxy is maximized when $\pi_X$ generates the simplest prompts that $\pi$ cannot yet solve but $\pi_\dagger$ can improve upon:

% \begin{itemize}
%     \item For very complex prompts, both $\pi$ and $\pi_\dagger$ may perform poorly, leading to low $p(\vy_2 \succ \vy_1 \mid \vx)$ and thus low regret proxy.
%     \item For very simple prompts, $\pi$ may already perform well, again leading to low regret proxy.
%     \item The optimal strategy for $\pi_X$ is to find prompts just beyond $\pi$'s current capabilities, where $\pi_\dagger$ can still demonstrate improvement.
% \end{itemize}

% This property ensures a smooth progression of the curriculum, always challenging $\pi$ with prompts that are neither too easy nor impossibly difficult.


% % As a naive baseline, we can use the preference advantage to evaluate the value of the prompt. We can set a threshold to select the prompts.

% % Next, we can adopt a combination of different practical prompting methods to grow the chosen prompt set:
% % \begin{itemize}
% %     \item Contrastive prompting
% %     \item Interpolating prompting
% %     \item Extrapolating prompting
% %     \item Adversarial prompting (like the camel paper)
% % \end{itemize}

% % \notes{TODO: provide concrete examples; check literature on similar synthetic data generation works.}

% % \notes{As an ablation study, we can add adversarial training loss in the original loss.}

% % One relevant baseline could be EvoPrompt~\citep{evoprompt}.

% % Essentially this is just like evolutionary algorithms as it is about population optimization. However, we don't need to confine ourselves in the rigid setting of classical evolution strategies.


% \newpage

% IGNORE THE OLD STUFFS

% \textbf{Stackelberg Game Formulation for Self-Improving Language Models}

% \begin{enumerate}
%     \item \textbf{Players:}
%     \begin{itemize}
%         \item Prompt Player: $$\textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)}$$
%         \item Response Player: $$\textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')}$$
%     \end{itemize}

%     \item \textbf{Definitions:}
%     \begin{itemize}
%         \item $\rvx \in \mathcal{X}$: Base prompts from a distribution $\mathcal{X}$
%         \item $\rvx' \in \mathcal{X}'$: Generated prompts
%         \item $\rvy \in \mathcal{Y}$: Responses
%         \item $\rvh \in \mathcal{H}$: Historical information
%         \item $\vtheta \in \Theta$: Shared parameters of the prompt and response generators
%     \end{itemize}

%     \item \textbf{Objective Functions:}
%     \begin{equation*}
%     \overbrace{\max_{\vtheta} \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}}}})}^{\text{prompt player}}, \qquad 
%     \overbrace{\max_{\vtheta} \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}}^{\text{response player}}
%     \end{equation*}
    
%     where
%     \begin{align*}
%        \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}, \rvy\sim p^{\text{response}}_{\vtheta}}\left[D(\rvx', \rvx) + \lambda U(\rvx', \vtheta)\right] \\
%         \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}}\left[R(p^{\text{response}}_{\vtheta}(\cdot \mid \rvx'), \rvx')\right]
%     \end{align*}

%     And:
%     \begin{itemize}
%         \item $D: \mathcal{X}' \times \mathcal{X} \to \mathbb{R}_+$ is a diversity measure
%         \item $U: \mathcal{X}' \times \Theta \to \mathbb{R}_+$ is an uncertainty measure
%         \item $R: (\mathcal{Y} \to [0,1]) \times \mathcal{X}' \to \mathbb{R}$ is a reward function
%         \item $\lambda \in \mathbb{R}_+$ is a hyperparameter
%     \end{itemize}

%     \item \textbf{Game Formulation:}
%     \begin{align*}
%         &\vtheta^\star = \arg\max_{\vtheta}\emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} \\
%         \text{s.t. } &\vtheta \in \arg\max_{\vtheta'} \ \   \emphgoal{J_R(\vtheta', \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}
%     \end{align*}

%     \item \textbf{Induced Distributions:}
%     \begin{align*}
%         \mu_{\vtheta}(\rvx', \rvy) &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \cdot \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')} \ \right] \\
%         \nu_{\vtheta}(\rvx') &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \ \right]
%     \end{align*}
% \end{enumerate}

% \textbf{Game Formulation Explanation:}

% The Stackelberg game formulation captures the interaction between the prompt generator (leader) and the response generator (follower). The prompt generator aims to maximize $J_P$, which encourages the generation of diverse and uncertain prompts. The response generator, in turn, maximizes $J_R$, which rewards high-quality responses to the generated prompts.

% % The game is asymmetric, with the prompt generator acting first. This allows the prompt generator to anticipate the response generator's behavior and generate prompts that will lead to overall improvement in the language model's capabilities.

% The constraint $\vtheta \in \arg\max_{\vtheta'} J_R(\vtheta', p^{\text{prompt}}_{\vtheta})$ ensures that the response generator is optimal with respect to the current prompt distribution. This captures the idea that the response generator quickly adapts to the prompts generated by the prompt generator.

% \textbf{Induced Distributions Explanation:}

% The induced distributions $\mu_{\vtheta}$ and $\nu_{\vtheta}$ characterize the behavior of the language model under the current parameters $\vtheta$:

% 1. $\mu_{\vtheta}(\rvx', \rvy)$ is the joint distribution of generated prompts and responses. It captures the overall behavior of the language model, including both prompt generation and response generation.

% 2. $\nu_{\vtheta}(\rvx')$ is the marginal distribution of generated prompts. This distribution is crucial for understanding the diversity and coverage of the prompt space achieved by the prompt generator.

% % These distributions play a key role in analyzing the equilibrium properties of the game and in proving theoretical guarantees about the language model's performance.
% \newpage

% \textbf{Equilibrium Properties and Theoretical Guarantees}

% \begin{itemize}
%     \setcounter{enumi}{5}
%     \item \textbf{Stackelberg Equilibrium:}
%     A Stackelberg equilibrium $\vtheta^\star$ satisfies:
%     \begin{align*}
%         \vtheta^\star &\in \arg\max_{\vtheta} J_P(\vtheta, \textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}) \\
%         \vtheta^\star &\in \arg\max_{\vtheta} J_R(\vtheta, \textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}})
%     \end{align*}

%     At this equilibrium:
%     \begin{enumerate}
%         \item $\textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}}$ generates diverse prompts that effectively explore the prompt space and target areas of model uncertainty.
%         \item $\textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}$ produces high-quality responses across the range of generated prompts.
%     \end{enumerate}

%     \item \textbf{Theorem (Performance Guarantee):} 
%     At the Stackelberg equilibrium $\vtheta^\star$:
%     \begin{equation*}
%         \mathbb{E}_{\rvx'\sim\nu_{\vtheta^\star}}[R(p^{\text{response}}_{\vtheta^\star}(\cdot \mid \rvx'), \rvx')] \geq R^\star - (\varepsilon_D + \varepsilon_U + \varepsilon_T)
%     \end{equation*}

%     Where:
%     \begin{itemize}
%         \item $R^*$ is the optimal achievable reward
%         \item $\varepsilon_D \geq 0$ is the suboptimality in prompt diversity
%         \item $\varepsilon_U \geq 0$ is the suboptimality in uncertainty targeting
%         \item $\varepsilon_T \geq 0$ is a transfer error term
%     \end{itemize}

%     \item \textbf{Proof Sketch:}
%     \begin{enumerate}
%         \item Let $p^{\text{prompt}*}$ and $p^{\text{response}*}$ be the optimal prompt and response generators, respectively.
%         \item By the optimality of $\vtheta^*$ for the response player:
%         \begin{equation*}
%             \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}}_{\vtheta^*}(\cdot \mid \rvx'), \rvx')] \geq \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \varepsilon_R
%         \end{equation*}
%         where $\varepsilon_R \geq 0$ is the suboptimality of the response generator.
        
%         \item The diversity and uncertainty terms in $J_P$ ensure:
%         \begin{equation*}
%             D_{KL}(\nu_{\vtheta^*} \parallel \nu^*) \leq \varepsilon_D + \varepsilon_U
%         \end{equation*}
%         where $\nu^*$ is the optimal prompt distribution and $D_{KL}$ is the Kullback-Leibler divergence.
        
%         \item Using Pinsker's inequality and the properties of the reward function:
%         \begin{equation*}
%             |\mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')]| \leq \varepsilon_T
%         \end{equation*}
        
%         \item Combining these inequalities and noting that $\mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] = R^*$, we obtain the desired result.
%     \end{enumerate}

%     \item \textbf{Corollary (Convergence):}
%     Under mild conditions on the learning dynamics and function approximators, the iterative algorithm converges to a Stackelberg equilibrium as $T \to \infty$.
% \end{itemize}

% \textbf{Stackelberg Game Variants}

% \begin{itemize}
%     \setcounter{enumi}{9}
%     \item \textbf{Prompt as Leader (PaL):} 
%     Choosing the prompt player as leader results in the following optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_P\left(\vtheta, p^{\text{response}*}_{\vtheta}\right) \text{ s.t. } p^{\text{response}*}_{\vtheta} \in \arg \max_{p^{\text{response}}} J_R\left(\vtheta, p^{\text{prompt}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     We solve this nested optimization using the first-order gradient approximation, resulting in updates:
%     \begin{align*}
%     p^{\text{response}}_{k+1} &\approx \arg \max_{p^{\text{response}}} J_R\left(\vtheta_k, p^{\text{prompt}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \alpha_k \nabla_{\vtheta} J_P\left(\vtheta, p^{\text{response}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Response as Leader (RaL):} 
%     Conversely, choosing the response player as leader results in the optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_R\left(\vtheta, p^{\text{prompt}*}_{\vtheta}\right) \text{ s.t. } p^{\text{prompt}*}_{\vtheta} \in \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta, p^{\text{response}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     Similarly, we solve this using the first-order gradient approximation:
%     \begin{align*}
%     p^{\text{prompt}}_{k+1} &\approx \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta_k, p^{\text{response}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \beta_k \nabla_{\vtheta} J_R\left(\vtheta, p^{\text{prompt}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Comparison:} 
%     \begin{itemize}
%         \item PaL prioritizes the generation of diverse and uncertain prompts, potentially leading to more exploratory behavior.
%         \item RaL focuses on optimizing responses, which may result in more stable learning but potentially less exploration.
%         \item The choice between PaL and RaL depends on the specific requirements of the task and the desired balance between exploration and exploitation.
%     \end{itemize}

%     \item \textbf{Convergence Properties:}
%     Under suitable regularity conditions on $J_P$, $J_R$, and the function approximators:
%     \begin{itemize}
%         \item Both PaL and RaL converge to local Stackelberg equilibria as $k \to \infty$.
%         \item The rate of convergence and the quality of the equilibrium may differ between PaL and RaL, depending on the landscape of $J_P$ and $J_R$.
%     \end{itemize}
% \end{itemize}


% \newpage
% \section{Experiments}

% \notes{TODO: add experimental details in this section. In general, we can consider two types of tasks, one is the general alignment task, where the preference comes from human values; the other can be math/coding task, where the preference oracle is the environment, signaling true or false for the correctness.}

% % \section{Evolutionary Prompt Set Optimization}

% % We formulate the problem of evolving the prompt set as a population-based optimization algorithm. Let $\mathcal{X}$ be the space of all possible prompts, and $\mathcal{X}_t \subset \mathcal{X}$ be our prompt set at iteration $t$.

% % \subsection{Fitness Function}

% % Define a fitness function $f: \mathcal{X} \times \Pi \rightarrow \mathbb{R}$, where $\Pi$ is the space of policies. For a prompt $\mathbf{x} \in \mathcal{X}$ and policy $\pi \in \Pi$, $f(\mathbf{x}, \pi)$ measures the "fitness" of $\mathbf{x}$ with respect to $\pi$. This could be defined in various ways, such as:

% % \begin{equation}
% % f(\mathbf{x}, \pi) = \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[\mathbb{P}(\vtau \succ \pi | \mathbf{x})] - \frac{1}{2}
% % \end{equation}

% % where $\mathbb{P}(\vtau \succ \pi | \mathbf{x})$ is the probability that response $\vtau$ is preferred over $\pi$'s typical response to $\mathbf{x}$.

% % \subsection{Population Dynamics}

% % Let $P_t = \{(\mathbf{x}_i, w_i)\}_{i=1}^N$ be the population at time $t$, where $\mathbf{x}_i \in \mathcal{X}_t$ and $w_i \in \mathbb{R}^+$ is a weight associated with $\mathbf{x}_i$. The evolution of the population follows these steps:

% % 1. \textbf{Selection}: Select a subset $S_t \subset P_t$ based on fitness values.
% % 2. \textbf{Variation}: Generate new prompts $V_t$ through mutation and crossover operations on $S_t$.
% % 3. \textbf{Evaluation}: Compute fitness for new prompts in $V_t$.
% % 4. \textbf{Replacement}: Update $P_{t+1}$ by combining $P_t$ and $V_t$.

% % \subsection{Information-Theoretic Approach}

% % We can incorporate information theory to guide the evolution process. Define the information content of a prompt $\mathbf{x}$ with respect to policy $\pi$ as:

% % \begin{equation}
% % I(\mathbf{x}, \pi) = H(\pi(\cdot|\mathbf{x})) - \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[H(\mathbb{P}(\cdot|\mathbf{x}, \vtau))]
% % \end{equation}

% % where $H(\cdot)$ is the Shannon entropy and $\mathbb{P}(\cdot|\mathbf{x}, \vtau)$ is the distribution over preferences given prompt $\mathbf{x}$ and response $\vtau$.

% % We can then define a composite fitness function:

% % \begin{equation}
% % F(\mathbf{x}, \pi) = \alpha f(\mathbf{x}, \pi) + (1-\alpha) I(\mathbf{x}, \pi)
% % \end{equation}

% % where $\alpha \in [0,1]$ balances between preference improvement and information gain.

% % \subsection{Variation Operators}

% % 1. \textbf{Mutation}: For $\mathbf{x} \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \mathbf{x} + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% %    \end{equation}
% %    where $\sigma^2$ is the mutation strength.

% % 2. \textbf{Crossover}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \lambda \mathbf{x}_1 + (1-\lambda) \mathbf{x}_2, \quad \lambda \sim \text{Beta}(a, b)
% %    \end{equation}

% % 3. \textbf{Information Exchange}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$ from different topics, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \textsc{Combine}(\mathbf{x}_1, \mathbf{x}_2)
% %    \end{equation}
% %    where \textsc{Combine} is a function that merges aspects of $\mathbf{x}_1$ and $\mathbf{x}_2$.

% % \subsection{Convergence Analysis}

% % Under certain conditions, we can prove convergence properties of this evolutionary algorithm:

% % \begin{thm}[Convergence of Evolutionary Prompt Optimization]
% % Let $\{\mathcal{X}_t\}_{t=0}^\infty$ be the sequence of prompt sets generated by the evolutionary algorithm. Assume:
% % \begin{enumerate}
% %     \item $f(\mathbf{x}, \pi)$ is continuous in $\mathbf{x}$ for all $\pi \in \Pi$.
% %     \item The variation operators are ergodic.
% %     \item The selection operator retains the best prompt with non-zero probability.
% % \end{enumerate}
% % Then, with probability 1:
% % \begin{equation}
% % \lim_{t \to \infty} \max_{\mathbf{x} \in \mathcal{X}_t} f(\mathbf{x}, \pi_t) = \sup_{\mathbf{x} \in \mathcal{X}} f(\mathbf{x}, \pi^*)
% % \end{equation}
% % where $\pi^*$ is the optimal policy.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows from the theory of evolutionary algorithms with elitist selection. The key steps are:
% % 1. Show that the best fitness in the population is non-decreasing.
% % 2. Use the ergodicity of variation operators to show that any point in $\mathcal{X}$ can be reached with non-zero probability.
% % 3. Apply the Borel-Cantelli lemma to show that the global optimum will be found in the limit.
% % \end{proof}



% % Essentially for the prompt evolving, we care about two things:
% % \begin{itemize}
% %     \item When the coverage is sufficient: we want to make sure the distribution is balanced.
% %     \item When the coverage is insufficient: we want to generate more \emph{novel} prompts.
% % \end{itemize}

% % {
% % \noindent
% % \centering
% % \begin{minipage}{.96\linewidth}
% %   \begin{algorithm}[H]
% %     \small
    
% %     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
% %     \begin{algorithmic}[1]
% %     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$
% %     \Statex

% %     \Repeat

% %     \Until 
% %     \State
% %     \Return 
% %     \end{algorithmic}
% %   \end{algorithm}
% % \end{minipage}
% % \par
% % }

% %self-improving robust optimization

==> texs_/method.tex <==
\newpage
% \section{Method}\label{sec:method}
\paragraph{Section overview.} We aim to develop language models that can \emph{self-improve to generalize well on new, unseen tasks} beyond the initial training prompt distribution for alignment. 
In $\S$\ref{sec:principle}, we present the limitations of classical RLHF and generalize it to the new objective of open-ended RLHF. In $\S$\ref{sec:mechanism}, we introduce the creator-solver game to tractably optimize the objective. In $\S$\ref{sec:algo}, we detail the practical algorithm, compatible with any preference optimization method as the solver, with our designed creator in the loop. Lastly in $\S$\ref{sec:int}, we present various interpretations for~\method.

%% RA.21.9: Before showing any math, probably worth motivating what we want to do -- the role of  theory is formalize things, which should be intutitive. 

\subsection{The Principle: Open-Ended RLHF for Joint Self-Improvement}~\label{sec:principle}
\hspace{-6pt}\textbf{Intuition.} \ \ Classical RLHF (\textit{cf}., Eq.~\ref{eq:rlhf-cls}) optimizes over a \emph{static} prompt distribution, meaning that the agent is only aligned to a fixed prompt set $\mathcal{D}$, making it brittle when it is evaluated on new problems from the ever-changing real world. Our Open-Ended RLHF breaks away from this static framework, with the goal to develop an agent that \emph{generalizes} well across \emph{unseen, novel} environments (where the tasks entailed in prompts may not have been explicitly encountered during training). To achieve this, we must design a new objective that agents can generate its own problems for self-improvement.
% , allowing $\rvx$ to come from a dynamic, ever-changing distribution that co-evolves with the agent's ability to solve tasks.
 % \ie \emph{the static optimization fails to adapt}.


\vspace{-4pt}
\paragraph{Formalization.} We introduce an \emph{open-ended} reference distribution $p_{\text{ref}}(\rvx)$, which is conceptually approached by a prompt  policy $\pi_{\vphi}(\rvx)$, co-evolving with the response policy for alignment:

% We introduce an \emph{optimizable} prompt generation policy $\pi_{\vphi}(\rvx)$, which is conceptually optimized towards an \emph{open-ended reference distribution} $p_{\text{ref}}(\rvx)$, jointly with the response policy optimization for preference alignment, formalized as:

\vspace{+3pt}

\begin{mdframed}
\begin{defn}[Open-Ended RLHF]\label{eq:rlhf-joint}
We define \emph{evolving alignment} as the open-ended joint optimization  on the prompt and response policy for alignment w.r.t the joint reference policy:
\vspace{-3pt}
\begin{align}
    \max_{\vphi, \vtheta}  \ \mathbb{E}_{\tg{\rvx\sim \pi_{\vphi}(\cdot)}  , \  \tc{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
- \beta \cdot  \sD_{\text{KL}}\Biggl[\ \tb{\pi_{\vphi, \vtheta}(}\tb{\rvx}\tb{, \ } \tb{\rvy}\tb{)} \ \| \ \tb{ \pi_{\text{ref}}(\rvx, \rvy)  } \ \Biggl], \label{eq:rlhf-joint-} \vspace{-5pt}
\end{align}
where $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy \mid \rvx)}$ and $\pi_{\text{ref}}(\rvx, \rvy) := p_{\text{ref}}(\rvx) \cdot \pi_{\text{SFT}}(\rvy \mid \rvx)$\footnote{\textcolor{black}{This generalizes  classical RLHF (Eq.~\ref{eq:rlhf-cls}). One may extend the above and rewrite coefficients to be:}
\vspace{-6pt}
\begin{align}
\scalebox{0.9}{$ 
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[  }} \emphred{\tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \bigr[ r(\mathbf{x}, \mathbf{y})  \bigr] - \beta_1 {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy | \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy | \rvx)\bigr]}}} \textcolor{cgreen}{\Bigr]} 
- \beta_2  \emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx) \Bigr]}}.
$}\label{eq:rlhf-expand}
\end{align} \vspace{-14pt}}.
% denotes the training joint distribution and the reference joint distribution, respectively.
\end{defn}
\end{mdframed}
\vspace{-2pt}
Here, $p_{\text{ref}}(\rvx)$ represents an \emph{underspecified}, potentially intractable probability distribution over possible tasks (instantiated \emph{via} prompts) in the wild, as a realizable \textbf{open-ended reference} that covers the full diversity and complexity of tasks agents may encounter, \emph{not} the initial static prompt set $\calD$. The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts, while being close to the SFT policy $\pi_{\text{SFT}}(\rvy | \rvx)$. 
% The joint optimization formalizes the setting that task distributions and the agent’s response policy are both updated, for the agent to be well-aligned in the broader prompt space of the open world.
\vspace{-3pt}



\subsection{The Mechanism: Asymmetric Self-Play \emph{via} the Creator v.s. Solver Game}~\label{sec:mechanism}
\hspace{-6pt}\textbf{Intuition.}\quad  It can be hard to directly solve  Eq.~\ref{eq:rlhf-joint-}, due to (i) the \textbf{intractability} of the underspecified reference~\citep{paired}, (ii) the  \textbf{instability} of joint differentiation~\citep{gan}. We present a heuristic of iterative alternating optimization by casting it as an \textbf{asymmetric creator-solver game}, that \textbf{implicitly achieves} the conceptual probability matching of $\sD_{\text{KL}}[\pi_{\phi}(\rvx) \ \| \ p_{\text{ref}}(\rvx) ]$ by iteratively creating a \emph{sequence} of prompt distributions to expand over the task space. 
\vspace{-3pt}
\begin{itemize}
    \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{${\pi_{\phi}(\rvx)}$} that strategically generate new prompt distributions.
    \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
\end{itemize}
This game serves as one potential choice to implicitly achieve the Open-Ended RLHF principle.
\vspace{-3pt}
\begin{itemize}
    \item By design, the creator can guide the solver with an \emph{informative prompt curriculum}, for it to develop more general capabilities to handle complexities in the wild~\citep{jiang-thesis}. 
    \item Intuitively, this resembles RL optimization \emph{via} expectation-maximization~\citep{hinton-em, rest_em}, where $\vphi$ for the prompt distribution is fixed at each step.
\end{itemize}



% \quad We formalize the alternating optimization as an asymmetric game as follows:
% \vspace{-3pt}
% \begin{itemize}
%     \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{$\pi_{\phi}(\rvx)$} that strategically generate new prompt distributions.
%     \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
% \end{itemize}

% This asymmetric game is one potential modeling choice to implicitly achieve the open-ended RLHF principle. We look forward to exploring more principled solutions in the future.

\textbf{Formalization.} We consider the \emph{minimax regret} strategy~\citep{savage1951theory},  where the \tb{solver} minimizes and the \tb{creator}  maximizes regret\footnote{Please see $\S$~\ref{app:theory} and Eq.~\ref{eq:KL-regret} for details on the KL-optimal policy $\pi^{\star}_{\text{KL}}(\rvy \mid \rvx)$. }, \ie the reward difference of the current and KL-optimal policy:
\begin{align}
    \operatorname{Regret}(\pi_{\phi}, \pi_{\vtheta}) = \sE_{\rvx \sim \pi_{\phi}(\cdot)} \Bigr[ \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] - \mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] \Bigr].\label{eq:regret-pi}
\end{align}
\newpage
% , \ie it can produce preferred responses in all scenarios
% \begin{align}
%     \tc{\pi^{\star}_{\calY \mid \calX}} \in \underset{ \tc{\pi_{\calY \mid \calX}} }{\arg \min} \  \underset{\tg{\pi_\calX}}{\max} \ \sE_{\rvx \sim \pi_{\calX}}  \ \Bigr[\ \operatorname{Regret}(\rvx, \tc{\pi_{\calY \mid \calX}}) \ \Bigr].\label{eq:minimax-regret}
% \end{align}

At the equilibrium~\citep{nash}, prior works~\citep{paired} have shown:
\vspace{+1pt}
\begin{mdframed}
\begin{rem}[Minimax Regret]
    If the above solver-creator game reaches an equilibrium, the solver follows a minimax regret policy, \ie the worst-case regret is bounded:
\begin{align}
    \tb{\pi^{\star}_{\calY \mid \calX}} \in \underset{ \tb{\pi_{\calY \mid \calX}} }{\arg \min} \  \underset{\tb{\pi_\calX}}{\max} \ \sE_{\rvx \sim \pi_{\calX}}  \ \Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\calY \mid \calX}}) \ \Bigr].\label{eq:minimax-regret}
\end{align}
\end{rem}
\end{mdframed}
\vspace{-6pt}
To illustrate, open-ended RLHF allows for the creation of evolving prompt distributions that challenge the agent progressively for better generalization; the introduced minimax regret objective further adds \emph{robustness} on top of such evolving curricula by \emph{incentivizing agents to perform well in all cases}. 

% \begin{align}
%     \text{info}(\rvx) \gets \widehat{A}_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') |, \label{eq:info-proxy}
% \end{align}


However, while it is often straightforward for the \textbf{solver} to minimize the regret (\eg by direct policy optimization), the optimal policy remains unknown during optimization, thus regret as the decision signal is often intractable to the \textbf{creator} -- regret approximation is needed. We design the proxy below for creator's  regret approximation (see  $\S$~\ref{app:theory} for more), also as a metric for prompt informativeness:
\vspace{+0.6pt}
\begin{mdframed}
\begin{defn}[Informativeness]\label{def:info-proxy}
    We estimate the informativeness of a prompt $\rvx$ in preference optimization by the (absolute) worst-case optimal advantage, approximating regret in Eq.~\ref{eq:regret_definition}:
\begin{align}
    | \hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta}) | \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{-}) , \label{eq:info-proxy}
\end{align}
\vspace{-5pt}
where\vspace{-5pt}
\begin{align}
\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \quad \mathbf{y}_{-} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}
and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle.
% which is estimated by sampling multiple responses for $\rvx$ from the solver and calculating  gap between the maximal reward (from the best $\rvy$) and the minimal reward (from the worst $\rvy$).
\end{defn}
\end{mdframed}
\vspace{-4pt}
We use the informativeness proxy to guide the creator for prompt distribution adaptation, which has a few useful properties under different interpretations, as in $\S$~\ref{sec:int}. In this way, we define a mechanism that the solver learns to improve, as the creator keeps challenging the solver on its weaknesses.

% \footnote{Some works~\citep{plr,active-pl} tested Shannon entropy, which is empirically found to underperform reward-based metric. We encourage future studies into this.}

% \fix{Add one sentence comment on the implications on the mimax regret; for example: To iterate, our open-ended RLHF objective does not focus on a fixed distribution of prompts, but rather allow for the creation of an evolving distribution that challenges the agent progressively, to ensure it generalize well under unseen, novel scenarios. The minimax regret framework adds a layer of robustness by minimizing the agent's performance gap in worst cases. It is not just about generalizing to novel prompted tasks, but also ..} Without access to the true optimal policy, we must approximate the regret. We design the advantage-based proxy as follows:

% We choose to use variants of advantage functions for the approximation, as shown in Table~\ref{tab:info-metric}, which we also refer as the informativeness proxy\footnote{Note that some works~\citep{plr,active-pl} had tested using Shannon entropy as the informativeness metric, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage more future studies into this.}, with $A^{\star}_{\min}$ as the default proxy due to its relation to minimax regret in Eq.~\ref{eq:minimax-regret}.
% \vspace{+1pt}
% \begin{mdframed}
% \begin{defn}[Informativeness Proxy]
%     We use the minimax regret as the proxy for the informativeness metric of the prompt, approximated by the (absolute) worst-case optimal advantage:
% \begin{align}
%     \text{info}(\rvx) \gets A_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | 
% \end{align}
% \end{defn}
% \end{mdframed}
% This proxy enjoys many nice properties under various interpretations, which we illustrate in $\S$~\ref{sec:int}.

\vspace{-4pt}
\subsection{The Practical Algorithm}~\label{sec:algo}\vspace{-4pt}
\hspace{-4pt}We now illustrate~\method~of Algorithm~\ref{alg:i-eva}, with practical implementations specified in $\S$~\ref{app:reproduce}. 

% The full pipeline is that we combine the creator and solver step in an iterative preference optimization pipeline.

\subsubsection{The Creator Step:  Estimate, Sample then Evolve}\label{sec:creator-step}\vspace{-2pt}
Plainly, the creator finds most useful prompts and generate variants of them for preference optimization. One may relate this to \emph{evolution strategies}~\citep{schwefel1977evolutionsstrategien} which find the most promising species, then mutate and crossover, or to \emph{curriculum RL}~\citep{accel} which finds environments with high-regret levels, then edits within some distance. As in Section~\ref{sec:mechanism}, we do not seek a differentiable creator in this work. The creator is implemented in three steps as in Figure~\ref{fig:pipeline}. 
\vspace{-6pt}

\paragraph{Step 1: $\texttt{\small info}(\cdot)$ -- \textnormal{\it estimate the informativeness}.} For each $\rvx$ in the  prompt set $\calX_t$, we generate responses, annotate rewards and estimate a informativeness metric to $\rvx$ by Eq.~\ref{eq:info-proxy} (see also Table~\ref{tab:info-metric}). \vspace{-6pt}
% To calculate the empirical value of $A^{\star}_{\min}$ for  each prompt, we first sample multiple responses from the prompt, where we label each response with its reward, then we use the difference between the highest reward $r_{\max}$ and the lowest reward $r_{\min}$ to represent the informativeness proxy.

\paragraph{Step 2: $\texttt{\small sample}(\cdot)$ -- \textnormal{\it weighted sampling for an informative subset}.} By using the informativeness metric as the weight,
we sample an informative prompt subset $\calX_t^{\texttt{\tiny info}}$ to be evolved later. This is similar to finding high-regret levels in curriculum RL.\vspace{-6pt}

\paragraph{Step 3: $\texttt{\small evolve}(\cdot)$ -- \textnormal{\it evolving for a proximal region of high-advantage prompts}.} Our algorithm is agnostic to and does not rely on any specific evolving method. We take \text{EvolInstruct}~\citep{wizardlm} as an off-the-shelf method, which conducts in-depth (\ie adding constraints, deepening, concretising, complicating) and in-breadth evolving (\ie mutation) for prompts. Specifically, we iterate over each prompt in the $\calX_t^{\texttt{\tiny info}}$, where each one is evolved to multiple variations, then optionally mix the newly generated prompts with a uniformly sampled buffer from $\calX_t$ to create $\calX_{t}^\prime$.

 % (\eg 20\% of the original)

 % by meta-instruction (\ie using an LLM to re-write the original prompts with the aforementioned evolving directions)


\subsubsection{The Solver Step: Solve then Optimize}\label{sec:solver-step}\vspace{-2pt}
This step is the classical preference optimization~\citep{dpo}, where responses are generated and the gradient descent is performed. Take the pointwise reward model setting as an example, for every prompt, we sample $n$ responses with reward annotated for each; we take the responses with the maximal and the minimal reward to construct the preference pairs, then optimize upon. This implicitly minimizes the regret to the KL-optimal policy, which we present in more details at $\S$~\ref{app:theory}.

Put together, \method~can unify existing iterative optimization pipeline~\citep{snorkel} with a new creator module, which can either share the same network as the solver policy or operate independently.

% \tc{An important contribution of our work is proposing the metric for preference optimization; so worth having a subsection somewhere on this.}
% (probably point to the appendix on the prompt distribution when we have it).


% \paragraph{Learning potential.} Our metric intuitively captures prompts with high learning potential by distinguishing between those that elicit both high-reward and low-reward responses. This contrast highlights areas where the agent can improve.

\subsection{Understanding the Informativeness Proxy in Different Intuitive Ways}\label{sec:int}

\paragraph{Learning potential.} Our metric intuitively identifies the learning potential of a prompt by measuring the gap between the best and worst response to it from the solver. We reason, that prompts eliciting \emph{both} high-reward and low-reward outcomes, reflect \emph{learnable} tasks where the model is capable of improving but has not yet mastered, thereby implying learning potential (\textit{cf.}, \cite{plr}). 
% The evolving step then generates similar prompts with increased diversity to further promote generalization.
\vspace{-2pt}



\paragraph{Worst-case guarantees.} The minimax-regret objective, by design, leads to solvers that  perform robustly across the prompt space, thus gives the worst-case guarantee. While exact equilibrium may not be attainable with approximation,  our empirical results in  $\S$~\ref{sec:ab-metric} demonstrate robustness.
\vspace{-2pt}

\paragraph{Auto-curricula for the players.}
We visualize curriculum induced by~\method~in $\S$~\ref{app:curr}. With the stochastic policy, the advantage may be heuristically understood as the reward difference between \emph{a base solver} and \emph{a reference solver}. Rather than optimizing separate solvers~\citep{paired}, we sample multiple times from the same policy to create the pair. In this way, the creator is incentivized to produce new prompts that are just out of the comfort zone of solvers~\citep{zone-promximal}:
\vspace{-6pt}
\begin{itemize}
    \item For overly challenging prompts, both solutions perform poorly, leading to a low  proxy.\vspace{-2pt}
    \item For overly easy prompts, the base solution already performs well, again giving a low proxy.\vspace{-2pt}
    \item The optimal strategy is to find prompts that are just beyond the solver's current capability.
\end{itemize}
\vspace{-2pt}
% , where the loss is monotonically smaller as the contrastive ratio $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ gets larger.

% \paragraph{Auto-curricula inherent to  \textnormal{\textit{Contrastive Optimization}}.} 
% \paragraph{Auto-curricula inherent to Contrastive Optimization.} 
% Another nice property of our informativeness metric is that it matches the curriculum learning property~\citep{easy-bengio2009curriculum}\footnote{We follow the curriculum learning literature that prioritizes examples with smaller losses for improvement in convergence and generalization. There is another line of work in optimization that claims examples with higher losses should be prioritized~\citep{hard-losers,hard-obs,hard-osgd,ordered-sgd}; however, \cite{rho-loss} conjecture that those example are often noisy (not learnable) or irrelevant thus are impractical. Our empirical results in Section~\ref{sec:ab-metric} on confirms this.} with contrastive preference optimization~\citep{cpl,dpo}, which generalizes DPO and a family of losses (\textit{c.f.}, Appendix~\ref{app:table}). In this way, we emphasize examples with smaller losses, thus enhancing convergence and generalization, by \emph{generatively} prioritize training examples w.r.t. our informativeness proxy:
% \begin{align}
%     \emphgray{A^{\star}_{\min}(\rvx)}  = \beta \cdot \textcolor{black}{\emphgray{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}}}  \ \approx \ \emphgray{r_{\max} - r_{\min}}.
% \end{align}
% Thus, we incentivize the creator to generate prompts that \emph{bring the most contrastive responses}. We hereby suggest the \emph{Contrastive Curriculum Hypothesis}: in contrastive preference optimization, prioritizing prompts w/ higher contrastive ratio improves sample efficiency and generalization. We show some initial empirical results on this in $\S$~\ref{sec:ab-cont}.


\paragraph{Auto-curricula inherent to Contrastive Optimization.} Contrastive preference optimization generalizes DPO and a family of algorithms (\textit{c.f.}, \cite{cpl,dpo,tang2024generalized}), many of whose losses monotonically decrease as the contrastive ratio increases. Here, by Eq.~\ref{eq:reward-re} and Eq.~\ref{eq:contrastive-ratio-main}, the \emph{contrastive ratio} can be written via the \emph{advantage-based proxy}:
\begin{align}
    A^{\star}_{\min}(\rvx)  = \beta \cdot \textcolor{black}{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}} .
\end{align}
By our proxy, we implicitly incentivize the creator to generate prompts that \emph{bring the most contrastive responses}, which decrease the loss the most. This matches the curriculum learning literature, which prioritizes (in~\method, \emph{generatively} prioritizes) examples with smaller losses for better convergence and generalization~\citep{easy-bengio2009curriculum}. We hence suggest the \emphtext{\textit{Contrastive Curriculum Hypothesis}}: in contrastive preference optimization, prioritizing prompts with higher contrastive ratio improves sample efficiency and generalization. We show initial empirical results on this in $\S$~\ref{sec:ab-metric} and $\S$~\ref{sec:ab-cont}.
% \begin{hypo}[Contrastive Curriculum Hypothesis]
%     In contrastive preference optimization, prioritizing prompts w/ \emph{higher contrastive ratio} improves sample efficiency and generalization.
% \end{hypo}

% footnote{One direction that worth to explore could be to directly use $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ instead of the reward proxy.}















% {\color{red} RA.9.26: This sounds like a para for related work possibly along with the footnote}

% % This formulation aims to find a policy $\pi$ that minimizes the worst-case regret across all possible prompt distributions. At equilibrium, this guarantees that the chosen policy $\pi$ performs robustly across the entire prompt space $\mathcal{X}$.

% This property ensures a smooth progression of the curriculum, always challenging $\pi$ with prompts that are neither too easy nor impossibly difficult.


% \textbf{Stackelberg Game Formulation for Self-Improving Language Models}

% \begin{enumerate}
%     \item \textbf{Players:}
%     \begin{itemize}
%         \item Prompt Player: $$\textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)}$$
%         \item Response Player: $$\textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')}$$
%     \end{itemize}

%     \item \textbf{Definitions:}
%     \begin{itemize}
%         \item $\rvx \in \mathcal{X}$: Base prompts from a distribution $\mathcal{X}$
%         \item $\rvx' \in \mathcal{X}'$: Generated prompts
%         \item $\rvy \in \mathcal{Y}$: Responses
%         \item $\rvh \in \mathcal{H}$: Historical information
%         \item $\vtheta \in \Theta$: Shared parameters of the prompt and response generators
%     \end{itemize}

%     \item \textbf{Objective Functions:}
%     \begin{equation*}
%     \overbrace{\max_{\vtheta} \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}}}})}^{\text{prompt player}}, \qquad 
%     \overbrace{\max_{\vtheta} \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}}^{\text{response player}}
%     \end{equation*}
    
%     where
%     \begin{align*}
%        \emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}, \rvy\sim p^{\text{response}}_{\vtheta}}\left[D(\rvx', \rvx) + \lambda U(\rvx', \vtheta)\right] \\
%         \emphgoal{J_R(\vtheta, \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})} &= \mathbb{E}_{\rvx\sim\mathcal{X}, \rvx'\sim p^{\text{prompt}}_{\vtheta}}\left[R(p^{\text{response}}_{\vtheta}(\cdot \mid \rvx'), \rvx')\right]
%     \end{align*}

%     And:
%     \begin{itemize}
%         \item $D: \mathcal{X}' \times \mathcal{X} \to \mathbb{R}_+$ is a diversity measure
%         \item $U: \mathcal{X}' \times \Theta \to \mathbb{R}_+$ is an uncertainty measure
%         \item $R: (\mathcal{Y} \to [0,1]) \times \mathcal{X}' \to \mathbb{R}$ is a reward function
%         \item $\lambda \in \mathbb{R}_+$ is a hyperparameter
%     \end{itemize}

%     \item \textbf{Game Formulation:}
%     \begin{align*}
%         &\vtheta^\star = \arg\max_{\vtheta}\emphtactic{{J_P(\vtheta, \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}})}} \\
%         \text{s.t. } &\vtheta \in \arg\max_{\vtheta'} \ \   \emphgoal{J_R(\vtheta', \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}})}
%     \end{align*}

%     \item \textbf{Induced Distributions:}
%     \begin{align*}
%         \mu_{\vtheta}(\rvx', \rvy) &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \cdot \textcolor{RoyalBlue1}{p^{\text{response}}_{\vtheta}(\rvy \mid \rvx')} \ \right] \\
%         \nu_{\vtheta}(\rvx') &= \mathbb{E}_{\rvx\sim\mathcal{X}}\left[ \ \textcolor{Orange3}{p^{\text{prompt}}_{\vtheta}(\rvx' \mid \rvx, \rvh)} \ \right]
%     \end{align*}
% \end{enumerate}

% \textbf{Game Formulation Explanation:}

% The Stackelberg game formulation captures the interaction between the prompt generator (leader) and the response generator (follower). The prompt generator aims to maximize $J_P$, which encourages the generation of diverse and uncertain prompts. The response generator, in turn, maximizes $J_R$, which rewards high-quality responses to the generated prompts.

% % The game is asymmetric, with the prompt generator acting first. This allows the prompt generator to anticipate the response generator's behavior and generate prompts that will lead to overall improvement in the language model's capabilities.

% The constraint $\vtheta \in \arg\max_{\vtheta'} J_R(\vtheta', p^{\text{prompt}}_{\vtheta})$ ensures that the response generator is optimal with respect to the current prompt distribution. This captures the idea that the response generator quickly adapts to the prompts generated by the prompt generator.

% \textbf{Induced Distributions Explanation:}

% The induced distributions $\mu_{\vtheta}$ and $\nu_{\vtheta}$ characterize the behavior of the language model under the current parameters $\vtheta$:

% 1. $\mu_{\vtheta}(\rvx', \rvy)$ is the joint distribution of generated prompts and responses. It captures the overall behavior of the language model, including both prompt generation and response generation.

% 2. $\nu_{\vtheta}(\rvx')$ is the marginal distribution of generated prompts. This distribution is crucial for understanding the diversity and coverage of the prompt space achieved by the prompt generator.

% % These distributions play a key role in analyzing the equilibrium properties of the game and in proving theoretical guarantees about the language model's performance.
% \newpage

% \textbf{Equilibrium Properties and Theoretical Guarantees}

% \begin{itemize}
%     \setcounter{enumi}{5}
%     \item \textbf{Stackelberg Equilibrium:}
%     A Stackelberg equilibrium $\vtheta^\star$ satisfies:
%     \begin{align*}
%         \vtheta^\star &\in \arg\max_{\vtheta} J_P(\vtheta, \textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}) \\
%         \vtheta^\star &\in \arg\max_{\vtheta} J_R(\vtheta, \textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}})
%     \end{align*}

%     At this equilibrium:
%     \begin{enumerate}
%         \item $\textcolor{RoyalBlue1}{p^{\text{prompt}}_{\vtheta^\star}}$ generates diverse prompts that effectively explore the prompt space and target areas of model uncertainty.
%         \item $\textcolor{Orange3}{p^{\text{response}}_{\vtheta^\star}}$ produces high-quality responses across the range of generated prompts.
%     \end{enumerate}

%     \item \textbf{Theorem (Performance Guarantee):} 
%     At the Stackelberg equilibrium $\vtheta^\star$:
%     \begin{equation*}
%         \mathbb{E}_{\rvx'\sim\nu_{\vtheta^\star}}[R(p^{\text{response}}_{\vtheta^\star}(\cdot \mid \rvx'), \rvx')] \geq R^\star - (\varepsilon_D + \varepsilon_U + \varepsilon_T)
%     \end{equation*}

%     Where:
%     \begin{itemize}
%         \item $R^*$ is the optimal achievable reward
%         \item $\varepsilon_D \geq 0$ is the suboptimality in prompt diversity
%         \item $\varepsilon_U \geq 0$ is the suboptimality in uncertainty targeting
%         \item $\varepsilon_T \geq 0$ is a transfer error term
%     \end{itemize}

%     \item \textbf{Proof Sketch:}
%     \begin{enumerate}
%         \item Let $p^{\text{prompt}*}$ and $p^{\text{response}*}$ be the optimal prompt and response generators, respectively.
%         \item By the optimality of $\vtheta^*$ for the response player:
%         \begin{equation*}
%             \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}}_{\vtheta^*}(\cdot \mid \rvx'), \rvx')] \geq \mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \varepsilon_R
%         \end{equation*}
%         where $\varepsilon_R \geq 0$ is the suboptimality of the response generator.
        
%         \item The diversity and uncertainty terms in $J_P$ ensure:
%         \begin{equation*}
%             D_{KL}(\nu_{\vtheta^*} \parallel \nu^*) \leq \varepsilon_D + \varepsilon_U
%         \end{equation*}
%         where $\nu^*$ is the optimal prompt distribution and $D_{KL}$ is the Kullback-Leibler divergence.
        
%         \item Using Pinsker's inequality and the properties of the reward function:
%         \begin{equation*}
%             |\mathbb{E}_{\rvx'\sim\nu_{\vtheta^*}}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] - \mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')]| \leq \varepsilon_T
%         \end{equation*}
        
%         \item Combining these inequalities and noting that $\mathbb{E}_{\rvx'\sim\nu^*}[R(p^{\text{response}*}(\cdot \mid \rvx'), \rvx')] = R^*$, we obtain the desired result.
%     \end{enumerate}

%     \item \textbf{Corollary (Convergence):}
%     Under mild conditions on the learning dynamics and function approximators, the iterative algorithm converges to a Stackelberg equilibrium as $T \to \infty$.
% \end{itemize}

% \textbf{Stackelberg Game Variants}

% \begin{itemize}
%     \setcounter{enumi}{9}
%     \item \textbf{Prompt as Leader (PaL):} 
%     Choosing the prompt player as leader results in the following optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_P\left(\vtheta, p^{\text{response}*}_{\vtheta}\right) \text{ s.t. } p^{\text{response}*}_{\vtheta} \in \arg \max_{p^{\text{response}}} J_R\left(\vtheta, p^{\text{prompt}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     We solve this nested optimization using the first-order gradient approximation, resulting in updates:
%     \begin{align*}
%     p^{\text{response}}_{k+1} &\approx \arg \max_{p^{\text{response}}} J_R\left(\vtheta_k, p^{\text{prompt}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \alpha_k \nabla_{\vtheta} J_P\left(\vtheta, p^{\text{response}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Response as Leader (RaL):} 
%     Conversely, choosing the response player as leader results in the optimization:
%     \begin{equation*}
%     \max_{\vtheta} \left\{J_R\left(\vtheta, p^{\text{prompt}*}_{\vtheta}\right) \text{ s.t. } p^{\text{prompt}*}_{\vtheta} \in \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta, p^{\text{response}}_{\vtheta}\right)\right\}
%     \end{equation*}

%     Similarly, we solve this using the first-order gradient approximation:
%     \begin{align*}
%     p^{\text{prompt}}_{k+1} &\approx \arg \max_{p^{\text{prompt}}} J_P\left(\vtheta_k, p^{\text{response}}_{\vtheta_k}\right) \\
%     \vtheta_{k+1} &= \vtheta_k + \beta_k \nabla_{\vtheta} J_R\left(\vtheta, p^{\text{prompt}}_{k+1}\right)
%     \end{align*}

%     \item \textbf{Comparison:} 
%     \begin{itemize}
%         \item PaL prioritizes the generation of diverse and uncertain prompts, potentially leading to more exploratory behavior.
%         \item RaL focuses on optimizing responses, which may result in more stable learning but potentially less exploration.
%         \item The choice between PaL and RaL depends on the specific requirements of the task and the desired balance between exploration and exploitation.
%     \end{itemize}

%     \item \textbf{Convergence Properties:}
%     Under suitable regularity conditions on $J_P$, $J_R$, and the function approximators:
%     \begin{itemize}
%         \item Both PaL and RaL converge to local Stackelberg equilibria as $k \to \infty$.
%         \item The rate of convergence and the quality of the equilibrium may differ between PaL and RaL, depending on the landscape of $J_P$ and $J_R$.
%     \end{itemize}
% \end{itemize}


% \newpage
% \section{Experiments}

% \notes{TODO: add experimental details in this section. In general, we can consider two types of tasks, one is the general alignment task, where the preference comes from human values; the other can be math/coding task, where the preference oracle is the environment, signaling true or false for the correctness.}

% % \section{Evolutionary Prompt Set Optimization}

% % We formulate the problem of evolving the prompt set as a population-based optimization algorithm. Let $\mathcal{X}$ be the space of all possible prompts, and $\mathcal{X}_t \subset \mathcal{X}$ be our prompt set at iteration $t$.

% % \subsection{Fitness Function}

% % Define a fitness function $f: \mathcal{X} \times \Pi \rightarrow \mathbb{R}$, where $\Pi$ is the space of policies. For a prompt $\mathbf{x} \in \mathcal{X}$ and policy $\pi \in \Pi$, $f(\mathbf{x}, \pi)$ measures the "fitness" of $\mathbf{x}$ with respect to $\pi$. This could be defined in various ways, such as:

% % \begin{equation}
% % f(\mathbf{x}, \pi) = \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[\mathbb{P}(\vtau \succ \pi | \mathbf{x})] - \frac{1}{2}
% % \end{equation}

% % where $\mathbb{P}(\vtau \succ \pi | \mathbf{x})$ is the probability that response $\vtau$ is preferred over $\pi$'s typical response to $\mathbf{x}$.

% % \subsection{Population Dynamics}

% % Let $P_t = \{(\mathbf{x}_i, w_i)\}_{i=1}^N$ be the population at time $t$, where $\mathbf{x}_i \in \mathcal{X}_t$ and $w_i \in \mathbb{R}^+$ is a weight associated with $\mathbf{x}_i$. The evolution of the population follows these steps:

% % 1. \textbf{Selection}: Select a subset $S_t \subset P_t$ based on fitness values.
% % 2. \textbf{Variation}: Generate new prompts $V_t$ through mutation and crossover operations on $S_t$.
% % 3. \textbf{Evaluation}: Compute fitness for new prompts in $V_t$.
% % 4. \textbf{Replacement}: Update $P_{t+1}$ by combining $P_t$ and $V_t$.

% % \subsection{Information-Theoretic Approach}

% % We can incorporate information theory to guide the evolution process. Define the information content of a prompt $\mathbf{x}$ with respect to policy $\pi$ as:

% % \begin{equation}
% % I(\mathbf{x}, \pi) = H(\pi(\cdot|\mathbf{x})) - \mathbb{E}_{\vtau \sim \pi(\cdot|\mathbf{x})}[H(\mathbb{P}(\cdot|\mathbf{x}, \vtau))]
% % \end{equation}

% % where $H(\cdot)$ is the Shannon entropy and $\mathbb{P}(\cdot|\mathbf{x}, \vtau)$ is the distribution over preferences given prompt $\mathbf{x}$ and response $\vtau$.

% % We can then define a composite fitness function:

% % \begin{equation}
% % F(\mathbf{x}, \pi) = \alpha f(\mathbf{x}, \pi) + (1-\alpha) I(\mathbf{x}, \pi)
% % \end{equation}

% % where $\alpha \in [0,1]$ balances between preference improvement and information gain.

% % \subsection{Variation Operators}

% % 1. \textbf{Mutation}: For $\mathbf{x} \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \mathbf{x} + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2 I)
% %    \end{equation}
% %    where $\sigma^2$ is the mutation strength.

% % 2. \textbf{Crossover}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \lambda \mathbf{x}_1 + (1-\lambda) \mathbf{x}_2, \quad \lambda \sim \text{Beta}(a, b)
% %    \end{equation}

% % 3. \textbf{Information Exchange}: For $\mathbf{x}_1, \mathbf{x}_2 \in S_t$ from different topics, generate $\mathbf{x}'$ as:
% %    \begin{equation}
% %    \mathbf{x}' = \textsc{Combine}(\mathbf{x}_1, \mathbf{x}_2)
% %    \end{equation}
% %    where \textsc{Combine} is a function that merges aspects of $\mathbf{x}_1$ and $\mathbf{x}_2$.

% % \subsection{Convergence Analysis}

% % Under certain conditions, we can prove convergence properties of this evolutionary algorithm:

% % \begin{thm}[Convergence of Evolutionary Prompt Optimization]
% % Let $\{\mathcal{X}_t\}_{t=0}^\infty$ be the sequence of prompt sets generated by the evolutionary algorithm. Assume:
% % \begin{enumerate}
% %     \item $f(\mathbf{x}, \pi)$ is continuous in $\mathbf{x}$ for all $\pi \in \Pi$.
% %     \item The variation operators are ergodic.
% %     \item The selection operator retains the best prompt with non-zero probability.
% % \end{enumerate}
% % Then, with probability 1:
% % \begin{equation}
% % \lim_{t \to \infty} \max_{\mathbf{x} \in \mathcal{X}_t} f(\mathbf{x}, \pi_t) = \sup_{\mathbf{x} \in \mathcal{X}} f(\mathbf{x}, \pi^*)
% % \end{equation}
% % where $\pi^*$ is the optimal policy.
% % \end{thm}

% % \begin{proof}[Proof Sketch]
% % The proof follows from the theory of evolutionary algorithms with elitist selection. The key steps are:
% % 1. Show that the best fitness in the population is non-decreasing.
% % 2. Use the ergodicity of variation operators to show that any point in $\mathcal{X}$ can be reached with non-zero probability.
% % 3. Apply the Borel-Cantelli lemma to show that the global optimum will be found in the limit.
% % \end{proof}



% % Essentially for the prompt evolving, we care about two things:
% % \begin{itemize}
% %     \item When the coverage is sufficient: we want to make sure the distribution is balanced.
% %     \item When the coverage is insufficient: we want to generate more \emph{novel} prompts.
% % \end{itemize}

% % {
% % \noindent
% % \centering
% % \begin{minipage}{.96\linewidth}
% %   \begin{algorithm}[H]
% %     \small
    
% %     \caption{{\small\textbf{\underline{Ev}olving Self-Play \underline{A}lignment (\texttt{\underline{EVA}})} } }\label{alg:tree-in-tree}
% %     \begin{algorithmic}[1]
% %     \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$
% %     \Statex

% %     \Repeat

% %     \Until 
% %     \State
% %     \Return 
% %     \end{algorithmic}
% %   \end{algorithm}
% % \end{minipage}
% % \par
% % }

% %self-improving robust optimization

==> texs_/pre.tex <==
\newpage
\section{Preliminaries}
We hereby review major concepts, which we later in $\S$~\ref{sec:method} use  \emphtext{\emph{regret}}  and the proxy by  \emphtext{\emph{advantage}} to identify informative prompts, leading to learning curricular implicitly maximizing \emphtext{\emph{contrastive ratio}}.
% in preference optimization. 
% We then present the algorithm overview, which we will elaborate on in $\S$\ref{sec:method}.
% We hereby briefly review main concepts in RLHF, which we will later use the concept of \textbf{{regret}}  and the approximation by the \textbf{advantage} function to identify informative prompts, that leads to a learning curriculum through maximizing \textbf{contrastive ratio} in direct preference optimization algorithms. We then present the algorithm overview, which we will elaborate on in $\S$\ref{sec:method}.

\paragraph{Alignment by RLHF.} Classical RLHF~\citep{ouyang2022training} optimizes on a fixed distribution $\calD$:
\begin{align}
    \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Biggl[\ r(\rvx, \rvy) \ \Biggl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Biggl[ \beta \cdot \mathbb{D}_{\text{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \Bigl] \Biggl],\label{eq:rlhf-cls}
\end{align}
where $\rvx$ and $\rvy$ denote the prompts and responses, and $r(\cdot, \cdot)$ is the reward function.


\paragraph{Reward.} Let the \emph{optimal policy} of Eq.~\ref{eq:rlhf-cls} be $\pi^{\star}(\cdot)$ and $Z(\cdot)$ be the partition function, we have:
% \begin{align}
%     \hspace{+24pt} \emphgray{\pi^{\star}(\rvy \mid \rvx)} =\textcolor{black}{ \frac{1}{Z(\rvx)} \pi_{\text{ref}}(\rvy \mid \rvx)} \exp \left(\frac{1}{\beta} \cdot \emphgray{r(\rvx, \rvy)}\right), 
% \end{align}
% LightSteelBlue3
% \begin{align}
%     \pi^{\star}(\rvy | \rvx) \propto  \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right).\nonumber
% \end{align}
% and $\textcolor{black}{Z(\rvx) = \sum_{\rvy} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} r(\rvx, \rvy)\right)}$, thus 
% the reward function can be re-parameterized as:
\begin{align}
    \hspace{+5pt}r(\rvx, \rvy)=\beta \cdot \log \frac{ \pi^{\star}(\rvy \mid \rvx)} {\pi_{\text {\text{SFT}}}(\rvy \mid \rvx)}\textcolor{black}{ \ + \ \beta \cdot \log Z(\rvx)}. \label{eq:reward-re}
\end{align}

\paragraph{Regret.} Given the optimal policy \( \pi^\star \), the \emph{regret} of a policy \( \pi_{\boldsymbol{\theta}} \) at \( \mathbf{x} \) is:
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\mathbf{y} \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\mathbf{y} \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr]. \label{eq:regret_definition}
\end{align}


% \paragraph{Regret.} Let $r^\star(\rvx) = \max_{\rvy'} r(\rvx, \rvy')$ be the optimal reward achievable at $\rvx$, the \emph{regret} to take $\rvy$ is:\vspace{+3pt}
% \begin{align}
%     \hspace{-40pt} \operatorname{Regret}(\rvx, \rvy) = r^\star(\rvx) - r(\rvx, \rvy).\label{eq:regret_definition}
% \end{align}
% Define 

% \begin{align}
%     \min _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\rvy \mid \rvx)}\Bigl[\ \operatorname{Regret}(\rvx, \rvy) \ \Bigl] + \beta \cdot \mathbb{D}_{\mathrm{KL}}\Bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\mathrm{ref}}(\rvy \mid \rvx) \ \Bigl].\label{eq:rlhf-regret}
% \end{align}

\paragraph{Advantage.} The \emph{advantage} function quantifies how much better a response $\rvy$ is w.r.t. a baseline:
\begin{align}
    \hspace{+8pt}A(\rvx, \rvy) = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi(\rvy' \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \label{eq:advantage-definition}
\end{align}
% where $\pi(\rvy \mid \rvx)$ is any policy under consideration.
%% RA.21.9: Do we need to define these variants for the main paper? Probably can be moved to appendix.
Variants of advantage (\eg the worst-case advantage $A^{\star}_{\min}$) are related to regret, as shown in Table~\ref{tab:info-metric}.
% The worst-case optimal advantage $A^{\star}_{\min}$ is equivalent to negative regret, as in Table~\ref{tab:info-metric}.


% \begin{itemize}
%     \item \textbf{Worst-case Optimal Advantage}: This is equivalent to the \emph{negative} \textbf{worst-case regret}, by taking the worst-case reward as $r_{\min}(\rvx) = \min_{\rvy'} r(\rvx, \rvy')$ and using $r^{\star}$ as the baseline:
%     \begin{align}
%        \hspace{-90pt} \emphgray{A^{\star}_{\min}(\rvx)} = r_{\min}(\rvx) - r^{\star}(\rvx). \label{eq:worst-advantage}
%     \end{align}
%     % \item \textbf{Average Optimal Advantage}: This can be viewed as an approximation to the \emph{negative} \textbf{Bayesian regret}. Take $N$ as the total number of generated responses:
%     % \begin{align}
%     %     \hspace{-66pt} \emphgray{A^{\star}_{\text{avg}}(\rvx)} = r^{\star}(\rvx) - \frac{1}{N} \sum_{\rvy}r(\rvx, \rvy). \label{eq:avg-advantage}
%     % \end{align}
%     % \item \textbf{Leave-One-Out Advantage:} Excluding the current response from the average:
%     % \begin{align}
%     %     \emphgray{A_{\text{loo}}(\rvx)} = \frac{1}{N} \sum_{\rvy} \Bigr(r(\rvx, \rvy) - \frac{1}{N-1} \sum_{\rvy' \neq \rvy} r(\rvx, \rvy') \Bigr). \label{eq:loo-advantage}
%     % \end{align}
% \end{itemize}



\paragraph{Direct preference optimization.} The DPO~\citep{dpo} objective for RLHF is:
% \begin{align}
%     \calL_{\beta}^{\text{DPO}}(\pi_\vtheta) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}} - \log \Biggr[\sigma \Bigr(\beta \cdot  \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right) \Bigr)\Biggr],
% \end{align}
\begin{align}
    \hspace{+16pt}\calL_{\beta}^{\text{DPO}}(\pi_\vtheta) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}} - \log \Bigr[\sigma \Bigr(\beta \cdot  \Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx} \Bigr)\Bigr],
\end{align}
where we use $+, -$ to denote chosen and rejected responses, and denote the \textbf{contrastive ratio} as:
\begin{align}
\hspace{+16pt}\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}:=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}. \label{eq:contrastive-ratio-main}
\end{align}
By reward reparameterization with Eq.~\ref{eq:reward-re},  advantage also relates to contrastive ratio, as in $\S$~\ref{sec:int}.

% \footnote{Many preference optimization algorithms can be generalized w.r.t. the contrastive ratio -- see  Appendix~\ref{app:table}.}

% It is easy to see that by Eq.~\ref{eq:reward-re}, the  advantage is related to the contrastive ratio, \ie $\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx} =  A^{\star}_{\min}(\rvx) $.
% \begin{align}
%     \emphgray{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}} =  \emphgray{A^{\star}_{\min}(\rvx)} 
% \end{align}

% , and further discuss the relationship of the \emph{contrastive ratio} and the \emph{advantage} through the \emph{reward} in Section~\ref{sec:int-dpo}.

% \paragraph{Algorithm overview.} Our~\method~requires tiny changes to existing alignment pipeline \emph{via} a creator that adapts prompt distributions for \emph{open-ended RLHF} by the \emph{estimate, sample then evolve} procedure, which mimics the \emph{minimax-regret} policy in the asymmetric self-play game, that will be detailed in $\S$\ref{sec:method}.
\section{Method}\label{sec:method}
\paragraph{Algorithm overview.} On a high level, \method~extends classical RLHF to open-ended  RLHF \emph{via} a creator that adapts prompt distributions with an easy-to-implement \emphtext{\emph{estimate, sample then evolve}} procedure, mimicing the \emphtext{\emph{minimax-regret}} policy of asymmetric self-play games, as detailed in $\S$\ref{sec:algo}.
% \paragraph{Algorithm overview.} Motivated by the \emph{minimax-regret} principle for open-ended learning, our~\method~introduces a creator that adapts prompt distributions through an \emph{estimate, sample, then evolve} procedure. This requires only minor modifications to the existing alignment pipeline. Further details are provided in $\S$\ref{sec
% }.

\vspace{-5pt}
\input{tables/algo-eva}


% We now present a verbose description of our method~\method, which we will revisit later in different ways. Our overall procedure trains a series of models $\vtheta_1, \cdots, \vtheta_T$ from the initial model $\vtheta_0$. For the creator step, starting from the initial prompt set $\calX_t$ where $t=0$, for each prompt $\vx_i$ in the prompt set, we generate $n$ responses $\vy_i^{(j)}$ with the current $\vtheta_t$, then each response receives a reward $r_i^{(j)}$ from an external preference oracle. We then evaluate the informativeness of the prompt by signals elicited from rewards, say the worst-case reward advantage, such that $\text{info}(\rvx_i) = \widehat{A}^{\star}_{\min}(\rvx) = \max(\{ r_i^{(j)}\}_{j=1}^n) - \min(\{ r_i^{(j)}\}_{j=1}^n)$. Next, we conduct weighted sampling on the original set $\calX_t$ using $\text{info}(\rvx_i)$ as the weight to obtain a informative subset $\calX_t^{\text{info}}$. This step is similar to finding the high-regret level among all levels in classical open-ended learning~\citep{accel}. We then evolve a new set  based on $\calX_t^{\text{info}}$; the evolving process (\eg adding constraints to or concretizing the original prompts as in~\citep{wizardlm}) is similar to making small edits on the high-regret levels; we then combine the evolved new set with a buffer of original prompts from $\calX_t$ to obtain $\calX_{t+1}$. This will be used as the training prompt distribution to train $\vtheta_t$ to $\vtheta_{t+1}$, which we term as the solver step. We then repeat the process to continuously grow the prompt distribution and optimize the parameter.

% , where each current model $\vtheta_t$ is trained 

% \paragraph{Creator step.}

% \paragraph{Solver step.}


% In the next, we will illustrate that a useful strategy for open-ended learning is to continuously generate \emph{high regret} environments. In our context, this is equivalent to generating prompts with \emph{high absolute advantage}. This can also be interpreted as generating prompts with \emph{high contrastive ratio}. Informally, the notion of the contrastive ratio $\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}$ captures captures how much \emph{surprise} we have about the $\rvx$ by sampling responses from $\pi_{\vtheta}$, and we use it as a proxy for the informativeness of a prompt.


% Together this brings an automatic curriculum that helps the learning agent generalize better.

% (\log \frac{\pi_{\vtheta}\left(\rvy_{+} \mid \rvx \right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx \right)}- \log \frac{\pi_{\vtheta}\left(\rvy_{-} \mid \rvx \right)}{\pi_{\mathrm{ref}}\left(\rvy_{-} \mid \rvx \right)}) 
% \begin{align}
% \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot   \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right)\right)\right],
% \end{align}
% where we define the \textcolor{black}{\emph{contrastive ratio}} as:
% \begin{align}
%     \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right):=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \label{eq:contrastive-ratio-main}
% \end{align}

% Essentially, the loss function of most preference optimization algorithms can be generalized as a convex function of the contrastive ratio, \ie~$f_{\beta}(\Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right))$\footnote{A concurrent work~\citep{tang2024generalized} discusses about this generalization as well.}.




% \begin{align}
%     \min_{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}} \left[ \mathbb{E}_{\rvy \sim \pi_\vtheta(\rvy \mid \rvx)} \left[ \operatorname{Regret}(\rvx, \rvy) \right] \right]
%     + \beta \cdot \mathbb{D}_{\mathrm{KL}}\left[ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\mathrm{ref}}(\rvy \mid \rvx) \right]. \label{eq:regret_minimization}
% \end{align}


% the optimal policy is also proportional to the optimal advantage function, which is the negated regret:
% \begin{align}
%     \pi^{\star}(\rvy | \rvx) \propto  
% \end{align}


% The optimal solution is:
% \begin{align}
%     \pi^{\star}(\rvy | \rvx) = \textcolor{lightgray}{\frac{1}{Z(\rvx)}} \pi_{\text{ref}}(\rvy \mid \rvx) \exp \left(\frac{1}{\beta} \cdot r(\rvx, \rvy)\right). 
% \end{align}

% By re-parameterization, we have:
% \begin{align}
%     r(\rvx, \rvy)=\beta \cdot \log \frac{\pi^{\star}(\rvy \mid \rvx)}{\pi_{\text {\text{ref}}}(\rvy \mid \rvx)} + \textcolor{lightgray}{\beta \cdot \log Z(\rvx)}.
% \end{align}


% The RLHF objective is to maximize:
% \begin{align}
%     J_{\beta}(\pi) &= J(\pi) - \beta \cdot \mathbb{D}_{\mathrm{KL}}\left[\pi(\vtau) \| \pi_{\mathrm{ref}}(\vtau)\right] \\
%     &= \sE_{\vtau \sim \pi(\vtau)} \left[ r(\vtau) - \beta \cdot \log \frac{\pi(\vtau)}{\pi_{\text{ref}}(\vtau)}\right] \label{eq:rlhf-2} \\
%     &= \sE_{\rva_h \sim \pi(\cdot \mid \rvs_h)} \left[ \sum_{h=1}^{H} \left( r(\rvs_h, \rva_h) -\beta \log \frac{\pi\left(\rva_h \mid \rvs_h\right)}{\pi_{\mathrm{ref}}\left(\rva_h \mid \rvs_h\right)} \right)  \mid \rvs_0 \sim \rho(\rvs_0)\right]. 
%     %= \underset{\rva_h \sim \pi(\cdot \mid \rvs_h)}{\sE}
% \end{align}









% \paragraph{Direct preference optimization (DPO).} The DPO objective~\citep{dpo} is to minimize:
% \begin{align}
%     \calL_{\beta}^{\text{DPO}}(\pi) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}_{\text {pref}}} - \log \left[\sigma\left(\beta \cdot  \log \frac{\pi\left(\rvy_{+} \mid \rvx \right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx \right)}-\beta \cdot \log \frac{\pi\left(\rvy_{-} \mid \rvx \right)}{\pi_{\mathrm{ref}}\left(\rvy_{-} \mid \rvx \right)}\right)\right],
% \end{align}
% where $\sigma(\cdot)$ is the sigmoid function. We denote the loss function as:
% % \begin{align}
% % \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot  \emphgray{\dlog} \right)\right],
% % \end{align}
% \begin{align}
% \ell_{\beta}^{\text{DPO}}(\pi_{\vtheta}) = - \log \left[\sigma\left(\beta \cdot   \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right)\right)\right],
% \end{align}
% where we define the \textcolor{black}{\emph{contrastive ratio}} as:
% \begin{align}
%     \Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right):=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)} \label{eq:contrastive-ratio-main}
% \end{align}

% Essentially, the loss function of most preference optimization algorithms can be generalized as a convex function of the contrastive ratio, \ie~$f_{\beta}(\Delta_{\log }\left(\pi_{\boldsymbol{\theta}} \| \pi_{\text{ref}}\right))$\footnote{A concurrent work~\citep{tang2024generalized} discusses about this generalization as well.}.

% We present a summary table on other preference alignment algorithms in Appendix~\ref{app:table}.

















% \paragraph{No-regret learning.}

% \notes{TODO: Move the following part to Section~\ref{sec:mechanism} as a sub-sub-section, that illustrate that our objective has a specific meaning for DPO objective.}

% In the specific case of DPO, the loss is monotonically smaller as $\dlog$ gets larger. This justifies our use of $r_{\max} - r_{\min}$ as the informativeness metric to prioritize the training examples according to the curriculum learning literature~\citep{easy-bengio2009curriculum}\footnote{In general, the curriculum learning literature prioritizes examples with lower losses and claims improvement in both convergence and generalization. There is also another line of literature in optimization that claims examples with higher losses can be prioritized~\citep{hard-losers,hard-obs,hard-osgd,ordered-sgd}; however, \cite{rho-loss} conjecture that those example are often noisy (not learnable) or task-irrelevant, and are impractical. Our empirical results in Section~\ref{sec:ab-metric} confirms this. We hereby follow the curriculum learning literature.}, which is essentially the reward of the chosen response ($r_{\max}$) minus the reward of the rejected response ($r_{\min}$), that is:
% \begin{align}
%     r_{\max} - r_{\min} = \beta \cdot \textcolor{SlateBlue4}{\Delta_{\log}(\pi ^\star \| \pi_{\text{ref}})}.
% \end{align}

% While we may directly select data with $\dlog$, the usage of $r_{\max} - r_{\min}$ provides a fast approximation to this term.

% Another message is that, we should adaptively choose the informativeness metric when we use different optimization algorithms.

% \notes{A issue might be that, as the contrastive ratio becomes larger, the gradient update will decrease. We may want to adaptively adjust the learning rate.}
% \notes{To generalize all the online RLHF algorithms in the game-theoretic framework.}

% \paragraph{Alignment with Reward Modeling.} Classical preference optimization methods consider to first learn a reward model explicitly~\citep{rlhf} or implicitly~\citep{nash} using the Bradley-Terry model~\citep{bt}. Given a triplet $(\rvx, \vtau^+, \vtau^-)$ where $\rvx$ is the prompt and $\vtau$ is the response, the Bradley-Terry model specifies the probability of preferring $\vtau^+$ over $\vtau^-$ as:
% \begin{align}
%     \sP_{\text{BT}}\left(\vtau^+ \succeq \mathbf{\vtau}^- \mid \rvx \right) &=\frac{\exp (r\left(\vtau^+, \rvx\right)) }{\exp (r\left(\vtau^+, \rvx\right)) +\exp( r\left(\vtau^-, \rvx\right))} \nonumber \\
%     % &= \frac{1}{1 + \exp \left(- (r\left(\mathbf{x}, \vtau^+\right) - r\left(\mathbf{x}, \vtau^-\right))\right)} \\
%     &= \sigma \left(r\left(\vtau^+, \rvx\right) - r\left(\vtau^-, \rvx\right)\right). \label{eq:bt}
% \end{align}
% Classical RLHF~\citep{rlhf} first learn a reward model $r_{\phi}(\cdot, \cdot)$ by maximizing the log likelihood of the above, then optimize the following objective:
% \begin{align}
%     \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \calX, \vtau \sim \pi_\theta(\cdot \mid \rvx)}\left[r_\phi(\rvx, \vtau)\right]-\eta ^{-1} \cdot \mathbb{D}_{\mathrm{KL}}\left[\pi_\vtheta(\vtau \mid \rvx) \ \| \ \pi_{\mathrm{ref}}(\vtau \mid \rvx)\right].\label{eq:rlhf-cls}
% \end{align}
% The optimization problem has a closed-form solution~\citep{dpo} as:
% \begin{align}
%     \pi^{\star}(\vtau \mid \rvx) &= \textcolor{gray}{\frac{1}{Z(\rvx)}}\cdot \pi_{\text{ref}}(\vtau \mid \rvx) \cdot \exp \left(\eta \cdot \emphgray{r(\vtau, \rvx)}\right) \label{eq:rlhf-1} \\
%     &\propto \pi_{\mathrm{ref}}(\vtau \mid \mathbf{x}) \cdot \exp (\eta \cdot r(\vtau, \rvx)). \label{eq:rlhf-2}
% \end{align}
% This leads to the implicit optimal reward formulation:
% \begin{align}
%     r^{\star}(\vtau, \rvx)=\eta^{-1} \cdot \log \frac{\pi^{\star}(\vtau \mid \rvx)}{\pi_{\text {\text{ref}}}(\vtau \mid \rvx)}+\textcolor{gray}{\eta^{-1} \cdot \log Z(\rvx)}.
% \end{align}

% Taken it back to the Bradley Terry model, we have:
% \begin{align}
%       \sP_{\text{BT}}\left(\vtau^+ \succeq \mathbf{\vtau}^- \mid \rvx \right) &= \sigma\left(\eta^{-1} \log \frac{\pi^{\star}\left(\vtau^+ \mid \rvx\right)}{\pi_{\text{ref}}\left(\vtau^+ \mid \rvx\right)}-\eta^{-1} \log \frac{\pi^{\star}\left(\vtau^- \mid \rvx\right)}{\pi_{\text{ref}}\left(\vtau^- \mid \rvx\right)}\right).
% \end{align}
% The direct preference optimization (DPO) loss thus is:
% \begin{align}
%     \mathcal{L}_{\mathrm{DPO}}\left(\pi_\vtheta ; \pi_{\text {\text{ref}}}\right)=-\mathbb{E}_{\left(\rvx, \vtau^+, \vtau^-\right) \sim \mathcal{D}}\left[\log \sigma\left(\eta^{-1} \log \frac{\pi_\vtheta\left(\vtau^+ \mid \rvx\right)}{\pi_{\text {ref}}\left(\vtau^+ \mid \rvx\right)}-\eta^{-1} \log \frac{\pi_\vtheta\left(\vtau^- \mid \rvx\right)}{\pi_{\text {ref}}\left(\vtau^- \mid \rvx\right)}\right)\right].
% \end{align}

% % \notes{Double check IPO on the preference modeling part.}


% \paragraph{Alignment with General Preferences.} This line of works~\citep{nlhf,self-play-gu} consider to learn the general preference $\sP\left(\vtau \succeq \mathbf{\vtau}^\prime \mid \rvx \right)$ \emph{without reward modeling}, by casting the problem as a two-player constant-sum game, where optimal policy is assumed to be identified by the minimax winner or the Nash equilibrium~\citep{nash}:
% \begin{align}
%     \left(\pi^\star, \pi^\star\right)=\arg \max _\pi \min _{\pi^{\prime}} \mathbb{E}_{\mathbf{x} \sim \mathcal{X}}\left[\mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x}), \vtau^{\prime} \sim \pi^{\prime}(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right]\right].
% \end{align}
% Define the preference over policies as:
% \begin{align}
%     &\mathbb{P}(\vtau \succ \pi \mid \mathbf{x})=\mathbb{E}_{\vtau^{\prime} \sim \pi(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right], \\
%     &\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \mathbf{x}\right)=\mathbb{E}_{\vtau \sim \pi(\cdot \mid \mathbf{x})} \mathbb{E}_{\vtau^{\prime} \sim \pi^{\prime}(\cdot \mid \mathbf{x})}\left[\mathbb{P}\left(\vtau \succ \vtau^{\prime} \mid \mathbf{x}\right)\right], \\
%     &\mathbb{P}\left(\pi \succ \pi^{\prime}\right)=\mathbb{E}_{\mathbf{x} \sim \mathcal{X}}\left[\mathbb{P}\left(\pi \succ \pi^{\prime} \mid \mathbf{x}\right)\right].
% \end{align}
% The Nash equilibrium can then be expressed as:
% \begin{align}
%     \left(\pi^\star, \pi^\star\right)=\arg \max _\pi \min _{\pi^{\prime}} \mathbb{P}\left(\pi \succ \pi^{\prime}\right) .
% \end{align}

% \paragraph{Self-Play Preference Optimization (SPPO).} We hereby provide a brief intro on SPPO~\citep{self-play-gu}. The high-level idea is to iteratively update the policy with the multiplicative weight for it to asymptotically converge to the optimal policy. The iterative framework is:
% \begin{align}
%     \pi_{t+1}(\vtau \mid \rvx) = \textcolor{gray}{\frac{1}{Z_{\pi_t}(\rvx)}} \cdot \pi_t(\vtau \mid \rvx) \cdot \exp \left(\eta \cdot \emphgray{\mathbb{P}(\vtau \succ \pi_t \mid \mathbf{x})} \right). \label{eq:sppo-1}
% \end{align}
% Notice how this differs from Eq.~\ref{eq:rlhf-1}. The DPO-alike loss considers to re-parameterize the reward model and cancel out the normalizing factor $Z(\cdot)$. Alternatively, SPPO considers to directly approximate the policy update raio, in terms of $L_2$ distance:
% \begin{align}
% \pi_{t+1}=\underset{\pi}{\arg \min} \ \mathbb{E}_{\mathbf{x} \sim \mathcal{X}, \vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left(\underbrace{\log \left(\frac{\pi(\vtau \mid \mathbf{x})}{\pi_t(\vtau \mid \mathbf{x})}\right)}_{\text{Policy Update Ratio}} - \underbrace{\left(\eta \cdot \emphgray{\mathbb{P}\left(\vtau \succ \pi_t \mid \mathbf{x}\right)}-\log Z_{\pi_t}(\mathbf{x})\right)}_{\text{Preference Advantage Term}}\right)^2. \label{eq:sppo-2}
% \end{align}
% The finite-sample optimization problem is written as:
% \begin{align}
% \pi_{t+1}=\underset{\pi}{\arg \min} \ \mathbb{E}_{\mathbf{x} \sim \mathcal{X}, \vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left(\underbrace{\log \left(\frac{\pi(\vtau \mid \mathbf{x})}{\pi_t(\vtau \mid \mathbf{x})}\right)}_{\text{Policy Update Ratio}} - \underbrace{\left(\eta \cdot \emphorange{\mathbb{P}\left(\vtau \succ \widehat{\pi}^K_t \mid \mathbf{x}\right)}-\log Z_{\widehat{\pi}^K_t}(\mathbf{x})\right)}_{\text{Preference Advantage Term}}\right)^2,
% \end{align}
% where the preference is approximated by $K$ samples of responses with the oracle $\sP(\cdot)$:
% \begin{align}
%     \emphorange{\mathbb{P}\left(\vtau \succ \widehat{\pi}_t^K \mid \mathbf{x}\right)} = \frac{1}{K} \cdot \sum_{k=1}^K \mathbb{P}\left(\vtau \succ \vtau_k \mid \mathbf{x}\right),
% \end{align}
% and the normalizing factor is:
% \begin{align}
%     Z_{\widehat{\pi}_t^K}(\mathbf{x})=\mathbb{E}_{\vtau \sim \pi_t(\cdot \mid \mathbf{x})}\left[\exp \left(\eta \cdot \mathbb{P}\left(\vtau \succ \widehat{\pi}_t^K \mid \mathbf{x}\right)\right)\right],
% \end{align}
% where the expectation can be approximated by $M$ samples from the policy $\pi_t$. In~\citep{self-play-gu}, the term is replaced by a constant $1/2$, meaning the model will not be updated when there is a tie.


% % \paragraph{Nash Equilibrium.}





==> texs_/quotes.tex <==
% QUOTES from the accel~\citep{accel} paper

% --------------------
Deep reinforcement learning (RL) has seen tremendous success over the past decade. However, agents trained on fixed environments are brittle, often failing the moment the environment changes even slightly, thus limiting the real-world applicability of current RL methods. A common remedy is to introduce more training data diversity by randomizing the environment’s parameters in every episode—a process called domain randomization (DR). For example, these parameters might control the friction coefficient and lighting conditions in a robotic arm simulation or the position of obstacles in a maze (we call each such environment variation a level). Procedurally generating training levels to expose RL agents to more diverse experiences has quickly become a common method for improving the robustness of RL agents. However, DR is often not enough to train robust agents in domains where the agent struggles to make progress on many challenging levels. 

Adaptive curriculum methods match the complexity of training levels to an agent’s current capabilities, and have been shown to produce more robust policies in fewer training steps than domain randomization. These methods can be viewed as a game between a teacher that designs challenging levels and a student that solves them. This game is potentially open-ended, leading to the co-evolution of generally-capable students. By tailoring the distribution of entire levels throughout training, adaptive curricula perform unsupervised environment design (UED). However, training an environment-designing teacher is difficult, and the prior state-of-the-art UED method, Prioritized Level Replay (PLR), simply finds challenging levels through random search, making it unable to build off of previously found structures that were useful for training agents in the past. We can also expect its performance to degrade as the size of the design space grows, limiting the potential for open-ended co-evolution between teacher and student. In contrast, the evolutionary processes between organisms and their environments, which UED resembles, efficiently search the design space by successively mutating a population and selecting the fittest individuals. 

We combine evolution with a principled regret-based environment designer in an algorithm called Adversarially Compounding Complexity by Editing Levels (ACCEL). As in PLR, our new method uses the difference between how well an agent did in an environment and how well it could have done (a metric known in decision theory as regret) to quantify the learning potential of revisiting this environment in the future. The important difference from PLR is that ACCEL evolves a curriculum by making small edits (e.g. mutations) to previously high regret levels, thus constantly producing new levels at the frontier of the student agent's capabilities. By compounding complexity over time, ACCEL harnesses the potential for efficient, open-ended search inherent to evolution. Our results show that ACCEL’s adaptive curricula lead to RL agents that outperform existing auto-curriculum learning methods. 

The rest of this article describes ACCEL in more technical detail. We first provide the necessary background on the UED formalism, followed by a comprehensive description of the ACCEL algorithm. We then present our experimental results in two challenging domains consisting of maze navigation and continuous-control bipedal locomotion, where ACCEL evolves levels with higher complexity and produces policies exhibiting significantly improved generalization compared to other adaptive curriculum methods. 

==> texs_/theory.tex <==
% \section{Theoretical Analysis}
% \begin{thm}[Existence of Nash Equilibrium]
% Consider the two-player game between a prompt player $\pi_X$ and a policy player $\pi$, with compact strategy spaces $\Pi_X$ and $\Pi$ respectively. Let $\mathbb{P}(\cdot)$ be a continuous preference function. Define the payoff function:

% \begin{align}
%     J(\pi_X, \pi) = \mathbb{E}_{\pi_X \sim \Pi_X} \left[\max_{\pi^\prime \in \Pi} \mathbb{P}(\pi^\prime \succ \pi \mid \pi_X)\right].
% \end{align}

% % where $\mathbb{P}(\pi \succ \pi'|\vx) = \mathbb{E}_{\vtau \sim \pi(\cdot|\vx)} \mathbb{E}_{\vtau' \sim \pi'(\cdot|\vx)} [\mathbb{P}(\vtau \succ \vtau'|\vx)]$.

% Then, there exists a Nash equilibrium $(\pi_X^\star, \pi^\star)$ such that:

% \begin{align}
%     (\pi_X^\star, \pi^\star) \in \arg \max_{\pi_X \in \Pi_X} \min_{\pi \in \Pi} J(\pi_X, \pi).
% \end{align}
% \end{thm}


% TODO: update the Berk-Nash equilibrium analysis and justify the usage of regret gap as the selection metric.

==> texs_icml/exp-cache.tex <==
\newpage
\section{Experiments}\label{sec:exp}
% In this section, we present main results of our experiments, showing the remarkable performance gain from the additional creator step in~\method~on various benchmarks.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/arena-hard.png}
%         \caption{Caption for Arena Hard}
%         \label{fig:arena-hard}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/mt-bench.png}
%         \caption{Caption for MT Bench}
%         \label{fig:mt-bench}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/alpaca-eval.png}
%         \caption{Caption for Alpaca Eval}
%         \label{fig:alpaca-eval}
%     \end{subfigure}
%     \caption{Overall caption for the three figures}
%     \label{fig:three-figures}
% \end{figure} 


% \subsection{Experimental Settings}
\paragraph{Datasets and models for training.} We use  \textbf{UltraFeedback}~\citep{ultrafeedback} as the training dataset, which contains diverse high-quality prompts that are primarily human-generated. We use the instruction-finetuned \textsc{Gemma-2-9B}~\citep{gemma2} as the primary model, which is a strong baseline for models of its size.   Detailed experimental setting can be found in $\S$~\ref{app:reproduce}.
\vspace{-10pt}
\paragraph{Evaluation settings.} We choose:   (i) \textbf{AlpacaEval 2.0}~\citep{ae}, which assesses general instruction following with 805 questions; (ii) \textbf{MT-Bench}~\citep{llm-judge}, which evaluates multi-turn instruction following with 80 hard questions in 8 categories; (iii) \textbf{Arena-Hard}~\citep{ah}, which is derived from 200K user queries on Chatbot Arena with 500 challenging prompts across 250 topics.  We use \texttt{\small gpt-4-1106} as the judge and \texttt{\small gpt-4-0314} as the baseline for win rate.
\vspace{-10pt}
\paragraph{Optimization algorithms.} We focus on direct preference optimization and consider the following:
\vspace{-6pt}
\begin{itemize}
    \item \textbf{With reference policy}: DPO~\citep{dpo}, SPPO~\citep{self-play-gu}.\vspace{+1pt}
    \item \textbf{Without reference policy}: SimPO~\citep{simpo}, ORPO~\citep{orpo}.
\end{itemize}
\vspace{-10pt}
\paragraph{Reward models as preference oracles.} We use \textsc{ArmoRM-8B}~\citep{armorm} as our default reward model as the human-preference proxy, and consider the following for ablation studies:
\vspace{-6pt}
\begin{itemize}
    \item \textbf{Pointwise}: \textsc{ArmoRM-8B}~\citep{armorm}, \textsc{SkyworkRM-27B}~\citep{skyworkrm}.\vspace{+1pt}
    \item \textbf{Pairwise}: \textsc{PairRM-0.4B}~\citep{pairrm}, \textsc{PairRM-8B}~\citep{pairrm8b}.
\end{itemize}

\subsection{Main Results}
\label{sec:main_results}
% For iterative training, we split the training set into equal-size partition and use one partition per iteration.

% \footnote{\vspace{-2pt}Unless stated otherwise, each iteration uses 10K prompts (\ie 1/6 partition from UltraFeedback in classical training). We denote \vspace{-16pt}$\vtheta_{t \rightarrow t+1}$ as the model trained with new human prompts based on the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the model trained with evolved prompts \vspace{-56pt}from the $t$-th checkpoint w/o adding any new human prompts.}
In general, \method~brings notable gains in alignment without relying on any human-crafted data, thus offering more efficiency. In the base setup, building on the one-iteration finetuned model ($\vtheta_{0 \rightarrow 1}$), \method~adds a creator to self-evolve the prompt set of the initial iteration and uses any preference optimization algorithm  for an additional open-ended RLHF iteration, resulting in  $\vtheta_{1 \rightarrow \tilde{1}}$\footnote{\vspace{-0pt}Unless stated otherwise, each training iteration uses 10K prompts; we denote $\vtheta_{t \rightarrow t+1}$ as the one trained w/ new human prompts \\\vspace{-49pt}from the $t$-th checkpoint, and $\vtheta_{t \rightarrow \tilde{t}}$ as the one trained w/ evolved prompts from the $t$-th checkpoint w/o any new human prompts.}.
\vspace{-10pt}
\paragraph{\method~achieves self-improvement.}  As shown in red rows in Table~\ref{tab:main-10k}, \method~yields notable performance improvement over $\vtheta_{0 \rightarrow 1}$ across different optimization algorithms, especially on the harder Arena-Hard benchmark, which is recognized to be more challenging and distinguishable among others due to the complexity of its prompts and its fairer scoring system~\citep{ah,simpo}. Specifically, \method~brings $8.4\%$ gain with SimPO as the solver, and $8.5\%$ gain with DPO as the solver, surpassing its 27B version and matching \texttt{\small claude-3-opus-240229} as reported on the \href{https://github.com/lm-sys/arena-hard-auto/tree/efc012e192b88024a5203f5a28ec8fc0342946df?tab=readme-ov-file#full-leaderboard-updated-0831}{\textcolor{gblue}{AH leaderboard}}, while using fully self-automated prompt generation for alignment. Interestingly, \method~brings the least gains on AlpacaEval 2.0, a simpler evaluation benchmark. This indicates \method~improves the most for challenging tasks.
\vspace{-10pt}
\paragraph{\method~can surpass human-crafted prompts.}  We further show that \method-prompt-trained models ($\vtheta_{1 \rightarrow \tilde{1}}$) can match and even outperform those trained on additional new prompts from UltraFeedback ($\vtheta_{1 \rightarrow 2}$) (which we denoted as human prompts), while being much cheaper and more efficient. Additionally, on MT-Bench, training with new human prompts typically show decreased performance in the first turn and only modest gains in the second turn. In contrast,~\method~notably enhances second-turn performance. We hypothesize that~\method~evolves novel, learnable prompts that include characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions.
\input{tabs/tab-main-10k}
% Additionally, on MT-Bench, we found that human prompts generally exhibit performance recession in first turn with modest gain in the second turn -- \method~fixes this while remarkably improves the second-turn performance without explicit training for it; we hypothesize that the novel, learnable prompts evolved from~\method~may incorporate characteristics of second-turn questions, reflecting emergent skills like handling follow-up interactions more effectively.


% \subsubsection{\textnormal{\textbf{\texttt{eva-o}}}: Main Results with the Online Training Setting}
% \input{tabs/tab-main-10k-o}

% \subsection{Subsections}





% -------------------------------------------------------------


% \newpage
\vspace{-10pt}
\subsection{Ablation Studies}
% \notes{For now, we use tables to record results. We can shift to other illustrations later (\eg performance plot, pareto circle, prompt distribution w.r.t. metric, etc).}
We conduct in-depth ablation studies on \texttt{\textbf{eva}}, with findings below to be elaborated on later: 

% \setlength{\leftmargini}{9pt}
\vspace{-5pt}
\begin{itemize}
    \item $\S$~\ref{sec:ab-metric} - \textbf{informativeness metric}: our \emph{regret}-based metric outperforms other alternatives.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-procedure} - \textbf{sample-then-evolve procedure}: our method outperforms greedy selection.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-rm} - \textbf{scaling w/ reward models}: the alignment gain of~\method~scales with reward models.\vspace{+1.5pt}
    \item $\S$~\ref{sec:ab-cont} - \textbf{continual training }: our method has monotonic gain with incremental training;  the \emph{evolved data and schedule} by~\method~serves as an \emph{implicit regularizer} for better local minima.
\end{itemize}
\vspace{-4pt}

%-------------------------------------------------------------
\vspace{-10pt}
\subsubsection{The Choice of Informativeness Metrics: \texttt{info(\textperiodcentered)}}\label{sec:ab-metric}
\vspace{-4pt}
% \notes{To make a table on all metrics in Section~\ref{sec:ab-metric}, similar to~\citep{plr}.}
\input{tabs/tab-info-metric}
\vspace{-8pt}
\input{tabs/tab-ab-metric}
\vspace{-12pt}
% (\textit{cf}., the principle of insufficient reason~\citep{key,dr})
\paragraph{Advantage as the informativeness metric outperforms baselines.} \hspace{-5pt}As in Table~\ref{tab:ab-metric}, \textbf{\texttt{eva}} offers an effective curriculum by the advantage-based proxy as the informativeness metric (bottom row):
\vspace{-6pt}
\begin{itemize}
    \item \emph{Comparing w/ uniform evolving} (\textcolor{brown!85}{brown}): Existing baselines generate prompts in a uniform manner~\citep{self-reward}  (\textit{cf}., the principle of insufficient reason~\citep{key,dr}). \method~concretely outperforms, corroborating~\cite{active-rlhf} that uniform learners can suffer from sub-optimality gaps.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ other heuristics} (\textcolor{dmblue200}{blue}): Prior practices~\citep{team-1} tried heuristics like prioritizing prompts w/ the most variance in its  rewards or w/ the lowest/highest average. We find our advantage based methods (red) outperforms those heuristics; see $\S$~\ref{app:metric} for more.\vspace{+1.5pt}
    
    \item \emph{Comparing w/ the inverse advantage} (\textcolor{dmpurple500}{purple}): Contrary to curriculum learning, a line of works conjecture that examples w/ higher losses may be prioritized~\citep{hard-losers,ordered-sgd}, which can be done by inverting our metric. We find it significantly \emph{hurt} the alignment gain, corroborating~\cite{rho-loss} that those examples can be unlearnable or irrelevant, meaning our curriculum is effective and practical. \vspace{+1.5pt}
    
    \item \emph{Among our advantage variants} (\textcolor{dmgreen900}{green}): We  designed variants of our default advantage-based metric, as in Table~\ref{tab:info-metric}; the default $A^{\star}_{\min}$ remains competitive among its peers. Together, the advantage-based principle provides a robust guideline for prompt sampling and evolving.
\end{itemize}
\vspace{-6pt}
The lesson is that we must be selective about which are the promising to evolve, otherwise unlearnable, noisy or naïve prompts may hinder learning. Our regret-inspired metric represents a solid baseline. 
\vspace{-6pt}


% \notes{Compare a star min with the uniform (no ordering), then compare it with its inverse (from hard to easy).}

% \paragraph{\emphtext{\method~is better other metric.}}  

% \notes{compare eva with other advantage variants, and other common choices that people have been using (choosing variance or mean) probably cite~\citep{active-pl,active-rlhf,selm} and emphasize our reliance on reward model. then cite~\cite{self-improving} in the footnote.}

% \paragraph{\emphtext{\method~.}}  \notes{compare eva with other advantage variants.}
% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{The Effect of the Sample-then-Evolve Procedure}\label{sec:ab-procedure}
\input{tabs/tab-ab-procedure}

\paragraph{The design of \texttt{\small evolve(\textperiodcentered)} in~\method~is effective.} As in Table~\ref{tab:ab-procedure}, we show:
\vspace{-6pt}
\begin{itemize}
    \item Removing the $\texttt{\small evolve}(\cdot)$ step: if we only do subset sampling or ordered selection, we still have gain, but not as much as w/ evolving (\eg \method~brings $4.8\%$ additional wins on AH).\vspace{+1.5pt}
    \item Altering the $\texttt{\small sample}(\cdot)$ step: if we greedily select prompts by the metric instead of using them as weights for importance sampling, the performance will be weaker as we evolve.
    % \footnote{When there is only subset selection, however, being greedy is slightly better on the Arena-Hard benchmark, but as we evolve more prompts such gain disappears.}. 
\end{itemize}
\vspace{-4pt}

% The lesson is that simply active learning on fixed prompts is unsatisfactory~\notes{To find a better description. AL is more about budget}; the open-ended RLHF with \emph{generative} prompt exploration we present brings a substantial headroom for self-improvement.
This shows that simply adaptive training within a fixed prompt distribution is unsatisfactory; our open-ended RLHF with \emph{generative} prompt exploration gives a substantial headroom for self-improvement.
% -------------------------------------------------------------




% -------------------------------------------------------------
\subsubsection{Scaling Pointwise and Pairwise Reward Models}\label{sec:ab-rm}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
        \end{subfigure}
        \vspace{-8pt}
        \caption{\textbf{\method\ scales with quality of reward models}, under pointwise RMs w/ DPO (\emph{left}) and pairwise RMs w/ SPPO (\emph{right}).  Note SPPO handles general preferences thus requires pairwise RMs, and DPO relies on the Bradley-Terry assumption, for which pointwise RMs are suitable.}
        \label{fig:ab-rm}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\textwidth}
        Figure~\ref{fig:ab-rm} presents the length-controlled win rate of \method~on  AlpacaEval  using pointwise and pairwise reward models of varying scales.
        %and types. We compare pointwise reward models w/ DPO, and pairwise reward models w/ SPPO\footnotemark.  
        The results give a clear trend: as the quality of reward models improve, \method~brings higher alignment gain. The scaling observation shows the effectiveness of~\method~in exploiting more accurate reward signals to choose informative prompts for better alignment.  One takeaway is interaction w/ the external world is essential for intelligence. The more accurate reward signals observed, the better the agent incentivize themself to improve (\textit{cf.},~\cite{silver2021reward}).
    \end{minipage}
\end{figure}
\vspace{-8pt}


% \footnotetext{We note that when there is only subset selection, being greedy is slightly better on the Arena-Hard benchmark. However, as we evolve more prompts, this discrepancy reverses.}

% \begin{figure}[!ht]
%     \centering
%     \begin{minipage}{0.5\textwidth}
%         \centering
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/dpo-rm-ae.pdf}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}{0.46\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{figs/sppo-rm-ae.pdf}
%         \end{subfigure}
%         \vspace{+0.1pt}
%         \caption{\textbf{Scaling with reward models.} Benchmark evaluation shows~\method~scales with reward models under both pointwise (\emph{left}) and pairwise (\emph{right}) setting.}
%         \label{fig:ab-rm}
%     \end{minipage}
% \end{figure}
% \vspace{-3pt}

% \paragraph{\emphtext{\method~scales with reward models.}} Figure~\ref{fig:ab-rm} presents the performance of \method~on the AlpacaEval benchmark using reward models of varying scales and types. We compare pointwise reward models with DPO~\citep{dpo} with pairwise reward models with SPPO~\citep{self-play-gu}\footnote{SPPO handles general preferences and thus requires pairwise reward models, whereas DPO relies on the Bradley-Terry model, for which pointwise reward models are suitable.}.  The results demonstrate a clear trend: as the quality of the reward model improves, \method~brings higher performance gain. The scaling observation shows the effectiveness of~\method~in leveraging more accurate reward signals to select informative prompts for better alignment. More results are in $\S$~\ref{app:ab-rm}.


% % \notes{The experiment is running.}
% \input{tabs/tab-ab-rm}





% -------------------------------------------------------------


% -------------------------------------------------------------
\subsubsection{\method~Improves Both Sample Efficiency and Generalization}\label{sec:ab-cont}
We continuously run the default \emph{incremental training} (\ie trainining from the last checkpoint w/ the evolved set in each iteration), as in Fig~\ref{fig:sad} and~\secref{app:exp-iter}, \method~presents \emphtext{\it monotonic performance gain} over iterations, and surpasses that trained w/ new human prompts, implying the generalization benefit. 

We conjecture that behaviors of the dashed/dotted lines relate to \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-primary-bias,cont-loss-rl,cont-repeat}.  Classical works resolve it by the \emph{optimization} perspective (\eg weight perturbing), whereas~\method~provides a new \emph{data} perspective, potentially mimicing an \textbf{implicit regularizer for better generalization}.
\vspace{-3pt}

% -------------------------
% The open-ended nature of our method naturally aligns with continual learning literature.
% One of the primary challenge of the field is that learning agents tends to lose their momentum to generalize well as the training goes on, a phenomenon often termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. while , \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

% \notes{First present the figure, show that eva is better at incremental training. Then present the table, show that eva is performant in both training schedules.}
% -------------------------


% \notes{Finished running. Waiting for evaluation.}



% A prominent line of research is on the loss of plasticity for continual (incremental) training~\citep{cont-critical,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm,cont-warm}; prior works all try to solve this via the optimization perspective, while our \eva method provides a fresh data perspective to solve the issue, operating like adding a regularizer to find better local minima.

\vspace{-5pt}
\begin{figure}[!ht]
\centering
\begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=.86\textwidth]{figs/dpo-it.pdf} % First figure
    % \vspace{10pt} % Adjust spacing between figures if needed
    \includegraphics[width=.86\textwidth]{figs/sppo-it.pdf} % Second figure
    \vspace{-6pt}
    \caption{\textbf{Continual training.} \method~stays robust w/ more iterations in incremental training.}
    \label{fig:sad}
\end{minipage}
\hfill
\begin{minipage}{0.64\textwidth} 
% \setlength{\parindent}{1em} % Adjust as needed for indentation
The solutions found by~\method~cannot be recovered by training longer w/ a fixed distribution (the dashed), nor by naïvely sourcing new prompts w/o examining informativeness (the gray dotted),  thus our generative data schedule is effective.\vspace{+6pt}

In Table~\ref{tab:ab-cont}, we ablate~\method~in \textit{scratch training}, \ie training w/ the full set (the evolved and the original data). \method~is competitive in incremental training, thus \emphtext{\emph{learns more effective} with \emph{less data}} -- a nice bonus via minimax regret~\citep{dcd}.

% , as in $\S$~\ref{sec:int}


% Next, we consider two different continual procedures:
% \begin{itemize}
%     \item \textbf{Incremental training}\footnotemark: train with only the evolved data on the finetuned checkpoint $\vtheta_{0 \rightarrow 1}$.\vspace{-1pt}
%     \item \textbf{Scratch training}: combine the evolved data with the full initial prompt set, train from scratch with $\vtheta_0$.
% \end{itemize}
% \vspace{+4pt}

\vspace{-6pt}
\input{tabs/tab-ab-cont}


% We then iteratively run incremental training, as in Figure~\ref{fig:sad}, \method~presents monotonic performance gain.\vspace{+4pt}

% A prominent line of research is on the difficulty of continual (incremental) training, and prior works all try to solve this via the explicit regularizer perspective~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}, while \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima.

\end{minipage}

\end{figure}
\vspace{-9pt}


% cont-rewarm
% acting like an implicit regularizer for better local minima

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% Furthermore, the open-ended nature of~\method~naturally aligns with the continual learning literature; one of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better generalization.

% From the perspective of continual learning~\citep{cont-loss}, \method~present a new solution to loss of plasticity during \emph{via} its generative data schedule, potentially acting as a regularizer for better generalization.

% The open-ended nature of~\method~naturally aligns with the continual learning literature.
% One of the primary challenges of the field is that  agents tends to lose their momentum to generalize well as the training goes on, a phenomenon termed as \emph{loss of plasticity}~\citep{cont-warm,cont-loss,cont-loss-rl,cont-repeat,cont-rewarm}. While classical works all try to solve this from the optimization perspective (\eg adding weight randomization), \method~provides a fresh data perspective, acting like an implicit regularizer for better local minima, 
% ~\notes{To update the figure; having DPO+SPPO.}
% \vspace{+6pt}


% \footnotetext{This is the default training strategy that we are using as it is computational efficient.}



% -------------------------------------------------------------



% % -------------------------------------------------------------
% \subsubsection{The Effect of Iteratively Evolving}\label{sec:ab-iter}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% \input{tabs/tab-ab-iter}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of the Base LLM for the Creator}\label{sec:ab-gen-lm}
% % \notes{This subsection can be put in the appendix section. We just continuously evolving based on the dataset from the last iteration.}
% % \notes{Experiments running in process. Mostly finished training. }
% \input{tabs/tab-ab-gen-lm}
% % -------------------------------------------------------------

% % -------------------------------------------------------------
% \subsubsection{The Effect of The Number of Training Examples}\label{sec:ab-scale}
% \input{tabs/tab-ab-scale}
% % -------------------------------------------------------------

% \notes{We may need to add additional compute resources usage discussions to illustrate efficiency.}














==> texs_icml/intro-cache-cache.tex <==
%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
% \vspace{+3.pt}
% \section {Introduction}\label{sec:intro}\vspace{-5pt}

\begin{figure}[htbp]
    \centering
    \hypbox{The Evolving Alignment Objective}{
    Language models shall generatively adapt their training prompt distribution for ever-evolving RL post-training.}
    \includegraphics[width=0.78\linewidth]{figs/front-fig.pdf}
    \caption{\textbf{Illustration on evolving alignment.} 
    Conventional RLHF is restricted to static prompt distributions. We show that adapting the prompt distribution during training is crucial, and further design a method allowing LLMs to robustly \emph{create} new prompts with improved \emph{coverage} and \emph{complexity} for \textbf{continual RL post-training}, offering remarkable gains (\secref{sec:exp}). This echoes \citet{continual-rl} in viewing learning as not just \emph{finding a solution}  but \emph{endless adaptation}, while offering a brand new training paradigm.
    }
    \label{fig:placeholder}
\end{figure}



\section{Introduction}\label{sec:intro}

\begin{figure*}[t]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline-icml.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \caption{\textbf{Asymmetric Self-Play Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with a simple \emph{estimate, sample then evolve} procedure; specifically, the informativeness for each prompt is elicited from reward signals. This leads to an infinite game where the creator evolves new prompts and the solver solves for continual RL training. The solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective that drives the game design \& different practical implementations in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \vspace{-6pt}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure*}

Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet the current training stage tends to be fairly short-lived and static.

% Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
% High-quality human data, crucial for scaling large language model based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as those large models become more capable, they need to identify and solve new and increasingly complex challenges, requiring training data beyond the capabilities of humans to create. This necessitates a new fundamental training mechanism, where models can continue to self-improve by generatively exploring and solving new problems. We thereby investigate the research question below:
% The fundamental issue arises from the finite data regime, specifically, the finite prompt regime.

LLM training is typically done with two stages, imitation (or supervised fine-tuning) and reinforcement learning , and in this paper we focus on the RL phase. The fundamental issue in all existing practices is, that they restrict themselves within a \emph{pre-curated}, \emph{static} prompt distribution throughout the training. This is sub-optimal, in terms of training efficiency and model generalizability. \notes{Another way to phrase, is that,  ``We are entering an era where compute is not primarily for training; it's for creating better data.'' (add cite). Scaling up in the $\calY | \calX$ space has achieved lots of success, but the model's performance can still plateau. What is the next right thing to scale? We suggest to look at the prompt space $\calX$.}

 % If we only optimize LLMs over a fixed prompt set, they will likely be brittle in front of new challenges, and it may be hard for the model to \emph{think out of the box}.

This leads to two subsequent research questions:
\begin{enumerate}
    \item \emph{Which prompts are actually useful during RL training?}
    \item \emph{How can we get more of those helpful prompts, and leverage them to keep LLMs self-improving?}
\end{enumerate}

% \notes{This paragraph is reserved to explain our method. For the first question, the key insight is to use reward signals. For the second question, the key insight is to self-create with meta instructions, and we propose online eva and iterative eva to achieve self-improvement.}


% More broadly, our work argues for a paradigm shift from conventional RL training, which can be seen as in a \textbf{finite game}~\citep{dogma}, where there is a fixed world is given, and \emph{learning is for purely solving} -- we only optimize a ``solver'' policy $\pi_{\vtheta}(\cdot | \rvx)$ which find solutions in a fixed environment or dataset from which $\rvx$ is sampled, then stop learning. 


% We argue for a paradigm shift, that RL training should be viewed as an \textbf{infinite game}, where \emph{learning is for jointly creating and solving}. Instead of optimizing the performance over a static dataset, we should also incentivize the models to create new environments/tasks, then continuously self-improve in the infinite data regime.







% \vspace{-6pt}


% Many preference optimization algorithms~\citep{rlhf,dpo,slic, liu2023statistical, dpo-ai-feedback} have been proposed to improve the alignment of language models, however, they all default to  fixed prompt training distributions. Such fixed training paradigm inevitably leads to: (i) \emph{generalization issues} (models may underperform or hack on instructions that are insufficiently represented in the fixed set) and (ii) \emph{efficiency issues} (data annotation and model training are costly, however not all prompt provide the same utility; it is wasteful to invest in sub-optimal fixed set, while identifying informative prompts through human efforts is expensive and time-consuming)~\citep{team-1,gemma2,llama3}. 

% The objective thereby should not only be to optimize over a specific, static distribution of prompts, yet to develop an agent that can autonomously evolve the training data distribution for self-improvement, to align well across unseen, novel environments or tasks (instantiated by prompts).



% rely on a static set of training prompts.

% , which can be viewed as a single \tb{solver step}. 

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.


% Thus, we develop~\method~(\underline{E}volving Alignment \emph{\underline{v}ia} \underline{A}symmetric Self-Play), as illustrated in Figure~\ref{fig:game}. Central to our approach is a game with the minimax-regret objective, achieved through alternating optimization between \tb{creating prompts} and  \tb{solving them}. The interplay encourages evolving curricula~\citep{accel}, potentially benefits both generalization and efficiency (see also $\S$~\ref{sec:int}). Orthogonal to many recent self-play studies in LLM alignment~\citep{nlhf,srpo,self-play-gu}, \method~is \emph{asymmetric}~\citep{intrinsic}, with two policies of different goals:
% \vspace{-5pt}
% \begin{itemize}
%     \item \textbf{Creator}: evolves the prompt distribution for alignment.\vspace{+1.5pt}
%     \item \textbf{Solver}: produces responses and optimizes  alignment based on the evolving prompts.
% \end{itemize}


% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 



% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.
% \notes{add a note on the difference compared to related work is in intro.}

We detail the uniqueness and novelty of this work \emph{w.r.t.} literature in \secref{sec:lit}, and summarize main contributions as follows:
\begin{enumerate}


    % (Learning a better curriculum and adapt it on the fly during training).

    % Specifically, 

    \item \textbf{We propose the first open-ended RLHF objective.}

    As in Definition~\ref{eq:rlhf-joint}, our new objective \emph{jointly} optimizes the prompt and response policy, and allows continual self-training beyond initial static prompts, improving (i) training \emph{efficiency} and (ii) model \emph{generalizability}.

    \item \textbf{We introduce and verify effective signals for LLMs to identify useful prompts in RL post-training.}

    In $\S$~\ref{sec:method}, we use variants of reward advantage (as proxies for regret) as effective signals in identifying learnable and worth-learning prompts, which can guide the prioritization of prompts during RL post-training.

    
    
    \item \textbf{We design~\method, the first method to our knowledge that allows LLMs to adaptively creates useful prompts and evolves in continual RL post-training.}

    In $\S$~\ref{sec:method}, to optimize the intractable open-ended RLHF objective, we further design a practical algorithm \emph{via} an infinite creator-solver game, incentivizing LLMs to create new prompts for  better \emph{learning curricula} (evidenced in $\S$~\ref{sec:ab-curr}) and adapt it on the fly for endless continual RL post-training.

    \item \textbf{\method\ is made to be easy-to-implement by everyone.}

    As in Algorithm~\ref{alg:i-eva}, \method\ can be easily plugged into \emph{any} RLHF pipeline, with an extensible creator module.
    
    \item \textbf{\method~leads to SOTA on challenging alignment benchmarks, with almost universal improvement across a variety of RL post-training algorithms.}

    In~$\S$ \ref{sec:exp}, we run \emph{extensive experiments} showing\ \method\ gives strong gains in  both online RL (\eg RLOO, OAIF) and offline RL (\eg DPO, SPPO, SimPO, ORPO).
\end{enumerate}

Lastly, as we enter the new epoch where compute is moving from training to data synthesis, the question on ``\emph{how to put more compute in generating better data}''~\citep{nishihara2025} is more critical than ever in AI research. While existing works~\citep{star,rest,bon-training} primarily focus on the \textbf{exploration in $\calY \mid \calX$} (\ie the solution space), we perform, to our knowledge, the first systematic study in \textbf{exploration in} $\calX$ (\ie the problem space)\footnote{More precisely, \method~explores the joint space, $(\calX, \calY)$. Note, \textbf{exploration} in RL can fall into \textbf{data generation} in common sense.} for RL post-training of LLMs. Such exploration is non-trivial, and relates to carefully designed \emph{reward signals}, as we show in $\S$~\ref{sec:ab-metric}.  We hope \method\ can be a starting point for researchers to push further along this new direction and discover the next right thing to scale~\citep{sutskever2024}.




% Our main contributions are summarized as:
% \begin{itemize}
%     \item \textbf{A new principle}: We propose a generalized \textbf{Open-Ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment, as in Definition~\ref{eq:rlhf-joint}.\vspace{+1.5pt}

%     \item \textbf{A new algorithm}: We propose what is, to our knowledge, the \emph{first} practical algorithm to allow \emph{infinite continual RL training for LLMs}. To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline, as in Algorithm~\ref{alg:i-eva}.\vspace{+1.5pt}
    
%     \item \textbf{A new start of the art}: We empirically validate~\method~on public alignment benchmarks and present general strong performance improvement when plugged in with \emph{both} online RL (\ie RLOO, OAIF) and offline RLHF (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide further insights on choices of informativeness metrics, reward models and training schedules, as in $\S$~\ref{sec:exp}.

% \end{itemize}

% We believe it can serve as a starting point for practitioners to work on open-ended RL post-training for language models. 






==> texs_icml/intro-cache.tex <==
%% RA.21.9: maybe start more strongly by stating how things are currently done for language models and why that's a problem? running out of human data, using a bounded set despite tasks / open-endedness is evolving
% Long-lived language agents 
% Agents based on large language models~(LLMs) 
% \vspace{+3.pt}
% \section {Introduction}\label{sec:intro}\vspace{-5pt}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth,height=0.2\textheight]{example-image-a}
    \caption{A placeholder figure on open-ended rlhf; and the joint RLHF (with creator and solver) definition, like the front figure in~\cite{platonic}.}
    \label{fig:placeholder}
\end{figure}

\section{Introduction}\label{sec:intro}
Long-lived artificial intelligence must deal with an ever-evolving, open-ended world, yet currently face constraints in both the \emph{scale} and \emph{quality} of available data, and the \emph{growth rate} at which new, useful information is created. 
High-quality human data, crucial for scaling large language model based intelligence, is projected to run out in the next few years \citep{run-out-of-data}; the quality of such data is also expected to stagnate: as those large models become more capable, they need to identify and solve new and increasingly complex challenges, requiring training data beyond the capabilities of humans to create. This necessitates a new fundamental training mechanism, where models can continue to self-improve by generatively exploring and solving new problems. We thereby investigate the research question below:

\begin{minipage}{.5\textwidth}
% \footnotesize
\centering
\textit{Can language models identify and \emph{self-create} new, learnable tasks to work on, to \emph{self-improve} to \emph{generalize} better for human preferences alignment?}
\end{minipage}
%or higher intelligence.


% \notes{One way to write the motivation part may be to follow ~\citep{poet,bengio2009curriculum,accel,paired}. Discuss how we incentivize the agent to generate prompt distribution with increasing complexity, promoting the models to solve harder problems.}

% \notes{Additional motivation/intuition/background paragraphs need to be added here. Motivate why we need to jointly optimize for both.}

% We aim to develop language agents capable of surpassing even superior intelligence, enabling them to solve increasingly complex problems.


% \vspace{-6pt}


% \vspace{+2pt}







% \vspace{-6pt}
\begin{figure*}[t]
    \centering
    \begin{minipage}{1\textwidth} % Adjust width to fit both figures in the same line
        \centering
        \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/pipeline.pdf}
            % \caption{Alpaca Eval}
        \end{subfigure}
        \caption{\textbf{Pipeline}: We generalize classical RLHF with open-ended RLHF, optimized with a creator-solver game for self-improving language models. Our proposed~\method~strategically evolves prompt distributions with a creator policy, which synthesizes prompts with an easy-to-implement \emph{estimate, sample then evolve} procedure; specifically, it estimates the informativeness for each prompt by how contrastive the self-generated responses are to the prompt, from the reward signals it receives. The creator evolves new prompts  from highly informative prompts, which the solver uses for continual training. The solver and creator policy can share the same network or operate independently. See more on our minimax-regret objective that drives the above design in $\S$~\ref{sec:method}.}
        \label{fig:pipeline}
    \vspace{-6pt}
    \end{minipage}
    \hspace{0.05\textwidth} % Space between the two main figures
\end{figure*}

Many preference optimization algorithms~\citep{rlhf,dpo,slic, liu2023statistical, dpo-ai-feedback} have been proposed to improve the alignment of language models, however, they all default to  fixed prompt training distributions. Such fixed training paradigm inevitably leads to: (i) \emph{generalization issues} (models may underperform or hack on instructions that are insufficiently represented in the fixed set) and (ii) \emph{efficiency issues} (data annotation and model training are costly, however not all prompt provide the same utility; it is wasteful to invest in sub-optimal fixed set, while identifying informative prompts through human efforts is expensive and time-consuming)~\citep{team-1,gemma2,llama3}. 

The objective thereby should not only be to optimize over a specific, static distribution of prompts, yet to develop an agent that can autonomously evolve the training data distribution for self-improvement, to align well across unseen, novel environments or tasks (instantiated by prompts).



% rely on a static set of training prompts.

% , which can be viewed as a single \tb{solver step}. 

% \fix{Need to add a paragraph discussing. Why existing works (to cite classcal RLHF) is insufficient. what are the prompts (new and learnable) to evolve. Why do we use the advantage-based proxy.}

% This process is akin to adaptively generating task curricula to train more generally-capable agents, and the job of the agents is to conceive both the challenges and solutions simultaneously~\citep{poet}.

% The goal is to train a open-ended self-improving language agent. Intuitively, this can be likened to starting with a fixed set of elementary math problems; as the agent becomes better at solving these problems, the distribution of prompts evolves to include more advanced topics, such as college-level and even more challenging problems. This dynamic progression embodies a co-evolution between a creator, which generates increasingly difficult prompts to maximize the agent's learning potential, and a solver, which adapts its response policy to effectively address the presented prompts. Through this iterative interaction, the agent continuously enhances its capabilities, ensuring robust performance across a broad and evolving range of prompts.


Thus, we develop~\method~(\underline{E}volving Alignment \emph{\underline{v}ia} \underline{A}symmetric Self-Play), as illustrated in Figure~\ref{fig:game}. Central to our approach is a game with the minimax-regret objective, achieved through alternating optimization between \tb{creating prompts} and  \tb{solving them}. The interplay encourages evolving curricula~\citep{accel}, potentially benefits both generalization and efficiency (see also $\S$~\ref{sec:int}). Orthogonal to many recent self-play studies in LLM alignment~\citep{nlhf,srpo,self-play-gu}, \method~is \emph{asymmetric}~\citep{intrinsic}, with two policies of different goals:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Creator}: evolves the prompt distribution for alignment.\vspace{+1.5pt}
    \item \textbf{Solver}: produces responses and optimizes  alignment based on the evolving prompts.
\end{itemize}


% ~\fix{YW: ``Dynamic prompt generation'' sounds too general for this idea (and sounds not very exciting). It's more about finding the most promising tasks to work on and improve learning efficiency (and generalization).} 



% \fix{Central to our approach is the usage of informativeness metric, and the method that evolves the prompts.}

% \fix{Mention the co-evolution literature.}

%% The research question in POET~\citep{poet} as a reference: Can we ignite a process that on its own \emph{unboundedly produces increasingly diverse and complex challenges at the same time as solving them? And, assuming computation is sufficient, can it last (in principle) forever?}

%%\cite{poet}: ``by evolving a set of diverse and increasingly complex environmental challenges at the same time as collectively optimizing their solutions.''




%% RA.21.9: Now, we should motivate what we are doing to do this -- key insight is that we can use the reward model as a learning signal on synthetic prompts -- but what synthetic prompts are useful? This leads the principle we have in the paper.




Our main contributions are summarized as:
\begin{itemize}
    \item \textbf{A new principle}: We propose a generalized \textbf{Open-Ended RLHF} objective for aligning language models, which seeks to jointly optimize the prompt distribution and the response policy, thus incentivizes models to self-improve to generalize well on new, unseen tasks beyond the initial training prompt distribution for alignment, as in Definition~\ref{eq:rlhf-joint}.\vspace{+1.5pt}

    \item \textbf{A new algorithm}: To optimize the objective, we design a practical algorithm \textit{via} asymmetric self-play, which is implemented through alternating optimization in a \textbf{creator}-\textbf{solver game}, and  can be easily plugged into any existing alignment pipeline, as in Algorithm~\ref{alg:i-eva}.\vspace{+1.5pt}
    
    \item \textbf{State-of-the-art performance}: We empirically validate~\method~on public alignment benchmarks and present general strong performance improvement when plugged in with different preference optimization algorithms (\ie DPO, SPPO, SimPO, ORPO). We also conduct extensive ablation studies that provide further insights on choices of informativeness metrics, reward models and training schedules, as in $\S$~\ref{sec:exp}.

\end{itemize}

\method~\textbf{is easy to implement}. We hope it can serve as a scalable method for the research community to build \text{open-ended}, robust, and self-improving language agents, that align with human values.




==> texs_icml/method-cache.tex <==


\newpage
\section{Method}\label{sec:method}
\paragraph{Algorithm overview.} On a high level, \method~extends classical RLHF to open-ended  RLHF \emph{via} a creator that adapts prompt distributions with an easy-to-implement \emphtext{\emph{estimate, sample then evolve}} procedure, mimicing the \emphtext{\emph{minimax-regret}} policy of asymmetric self-play games, as detailed in $\S$~\ref{sec:algo}.
% \paragraph{Algorithm overview.} Motivated by the \emph{minimax-regret} principle for open-ended learning, our~\method~introduces a creator that adapts prompt distributions through an \emph{estimate, sample, then evolve} procedure. This requires only minor modifications to the existing alignment pipeline. Further details are provided in $\S$\ref{sec
% }.

{
\noindent
\centering
\begin{minipage}{1\linewidth}
  \begin{algorithm}[H]
    \small
    
    \caption{{\small\textbf{\method:~\underline{E}volving Alignment \textnormal{\textit{\underline{v}ia}} \underline{A}symmetric Self-Play}}}\label{alg:i-eva}
    \begin{algorithmic}[1]
    \Statex \textbf{Input:} initial policy $\pi_{\vtheta_0}$,  initial prompt set $\mathcal{X}_0$
    % , sample size of responses per prompt $n$ 
    \vspace{+3pt}

    \For{\textbf{iteration} $t = 1, 2, \ldots$}
        \vspace{+5pt}
        
        \LineComment{\textcolor{cgreen}{{\textbf{\texttt{creator step}}}}}
        
        \vspace{+5pt}
        % \State  \tb{\emph{estimate informativeness}:} \hspace{+20pt}$\tb{\calX_{t-1} \gets \calX_{t-1} \cup \{\tb{\textbf{\texttt{info}}(\rvx_i)}\}}_i$ 
        \State  \tb{\emph{estimate}:}  $\mathcal{X}_{t-1} \gets \{ (\rvx_i, {\mathsf{\footnotesize info}}(\rvx_i)) | \rvx_i \in \mathcal{X}_{t-1} \}$

        
        \vspace{+2pt}
        

        \Statex \hspace{+12pt}  
        \tb{\emph{sample}:} \hspace{+60pt}$\tb{\calX_{t-1}^{{ {\mathsf{info}}}} \gets \tb{{{\mathsf{\footnotesize sample}}}(\mathcal{X}_{t-1})}}$ 
        \vspace{+2.5pt}

        \Statex  \hspace{+12pt}
        \tb{\emph{evolve}:} \hspace{+40pt}$\tb{\mathcal{X}_{t} \leftarrow \tb{{\mathsf{\footnotesize evolve}}(\calX_{t-1}^{\texttt{info}})}}$ 

        \vspace{+8pt}
        
        \LineComment{\textcolor{cred}{ \textbf{ \texttt{solver step} } }}
        
        \State 
        \tb{\emph{generate}:}  $\forall$ $\vx_i \in \mathcal{X}_{t}$,  generate $\{{\vy^{(j)}_i}\} \sim \pi_{\vtheta_{t-1}}(\cdot \mid \vx_i)$ 

        \Statex  \hspace{+12pt}
        \tb{\emph{annotate rewards}:} \hspace{+10pt} $\calX_{t}^{\prime} \gets \calX_{t} \cup \{{(\vy^{(j)}_i}, {r^{(j)}_i})\}$ 

        \vspace{+2.5pt}
        
        \Statex  \hspace{+12pt}
        \tb{\emph{optimization}:}$ \hspace{+32pt} \tb{\boldsymbol{\theta}_{t} \leftarrow \boldsymbol{\theta}_{t-1} + \eta \nabla_{\boldsymbol{\theta}} \mathcal{J}_{\calX'_t}(\boldsymbol{\theta})}$ 
        \vspace{+5pt}
        
    \EndFor 
    \State \Return final solver policy $\pi_{\vtheta_T}$
    \end{algorithmic}
  \end{algorithm}
\end{minipage}
\par
}

\paragraph{Section overview.} We aim to develop language models that can \emph{self-improve to generalize well on new, unseen tasks} beyond the initial training prompt distribution. 
In $\S$~\ref{sec:principle}, we show the limitations of classical RLHF and generalize it to the new objective of open-ended RLHF. In $\S$~\ref{sec:mechanism}, we introduce creator-solver games to tractably achieve the objective. In $\S$~\ref{sec:algo}, we detail a practical algorithm with a plug-in creator, compatible with any preference optimization algorithm as the solver. Lastly in $\S$~\ref{sec:int}, we discuss various interpretations for~\method.
%% RA.21.9: Before showing any math, probably worth motivating what we want to do -- the role of  theory is formalize things, which should be intutitive. 
\vspace{-10pt}
\subsection{The Principle: Open-Ended RLHF for Joint Self-Improvement}~\label{sec:principle}
\hspace{-6pt}\textbf{Intuition.} \ \ Classical RLHF (\textit{cf}., Eq.~\ref{eq:rlhf-cls}) optimizes over a \emph{static} prompt distribution, meaning that the agent is only aligned to a fixed prompt set $\mathcal{D}$, making it brittle when it is evaluated on new problems from the ever-changing real world. Our Open-Ended RLHF breaks away from this static framework, with the goal to develop an agent that \emph{generalizes} well across \emph{unseen, novel} environments (where the tasks entailed in prompts may not have been explicitly encountered during training). To achieve this, we must design a new objective that agents can generate its own problems for self-improvement.
% , allowing $\rvx$ to come from a dynamic, ever-changing distribution that co-evolves with the agent's ability to solve tasks.
 % \ie \emph{the static optimization fails to adapt}.


\vspace{-10pt}
\paragraph{Formalization.} We introduce an \emph{open-ended} reference distribution $p_{\text{ref}}(\rvx)$, which is conceptually approached by a prompt  policy $\pi_{\vphi}(\rvx)$, co-evolving with the response policy for alignment:

% We introduce an \emph{optimizable} prompt generation policy $\pi_{\vphi}(\rvx)$, which is conceptually optimized towards an \emph{open-ended reference distribution} $p_{\text{ref}}(\rvx)$, jointly with the response policy optimization for preference alignment, formalized as:


Here, $p_{\text{ref}}(\rvx)$ represents an \emph{underspecified}, potentially intractable probability distribution over possible tasks (instantiated \emph{via} prompts) in the wild, as a realizable \textbf{open-ended reference} that covers the full diversity and complexity of tasks agents may encounter, \emph{not} the initial static prompt set $\calD$. The joint regularization towards $\pi_{\text{ref}}(\rvx, \rvy)$ captures the objective for agents to generalize on alignment in $p_{\text{ref}}(\rvx)$ with broader open-ended prompts, while being close to the SFT policy $\pi_{\text{SFT}}(\rvy | \rvx)$. 
% The joint optimization formalizes the setting that task distributions and the agent’s response policy are both updated, for the agent to be well-aligned in the broader prompt space of the open world.
\vspace{-3pt}



\subsection{The Mechanism: Asymmetric Self-Play \emph{via} Creator-Solver Games}~\label{sec:mechanism}
\hspace{-6pt}\textbf{Intuition.}\quad  It can be hard to directly solve  Eq.~\ref{eq:rlhf-joint-}, due to (i) the \textbf{intractability} of the underspecified reference~\citep{paired}, (ii) the  \textbf{instability} of joint differentiation~\citep{gan}. We present a heuristic of iterative alternating optimization by casting it as an \textbf{asymmetric creator-solver game}, that \textbf{implicitly achieves} the conceptual probability matching of $\sD_{\text{KL}}[\pi_{\phi}(\rvx) \ \| \ p_{\text{ref}}(\rvx) ]$ by iteratively creating a \emph{sequence} of prompt distributions to expand over the task space. 
\vspace{-5pt}
\begin{itemize}
    \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{${\pi_{\phi}(\rvx)}$} that strategically generate new prompt distributions.
    \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
\end{itemize}
\vspace{-10pt}
This game serves as one potential choice to implicitly achieve the Open-Ended RLHF principle.
\vspace{-5pt}
\begin{itemize}
    \item By design, the creator can guide the solver with an \emph{informative prompt curriculum}, for it to develop more general capabilities to handle complexities in the wild~\citep{jiang-thesis}. 
    \item Intuitively, this resembles RL optimization \emph{via} expectation-maximization~\citep{hinton-em, rest_em}, where $\vphi$ for the prompt distribution is fixed at each step.
\end{itemize}



% \quad We formalize the alternating optimization as an asymmetric game as follows:
% \vspace{-3pt}
% \begin{itemize}
%     \item $\text{\bf \tb{Creator}}$ \hspace{+1pt}: the prompt player \tg{$\pi_{\phi}(\rvx)$} that strategically generate new prompt distributions.
%     \item  $\text{\bf \tb{\hspace{+0.6pt} Solver \hspace{+0.6pt}}}$ \hspace{+1pt}: the response player \tc{$\pi_{\vtheta}(\rvy \mid \rvx)$} that learns to optimize for preference alignment.
% \end{itemize}

% This asymmetric game is one potential modeling choice to implicitly achieve the open-ended RLHF principle. We look forward to exploring more principled solutions in the future.

\textbf{Formalization.} We consider the \emph{minimax regret} strategy~\citep{savage1951theory},  where the \tb{solver} minimizes and the \tb{creator}  maximizes regret\footnote{Please see $\S$~\ref{app:theory} and Eq.~\ref{eq:KL-regret} for details on the KL-optimal policy $\pi^{\star}_{\text{KL}}(\rvy \mid \rvx)$. }, \ie the reward difference of the current and KL-optimal policy:
\vspace{-12pt}

\begin{minipage}{1\linewidth}
\small
\begin{align}
    \operatorname{Regret}(\pi_{\phi}, \pi_{\vtheta}) = &\sE_{\rvx \sim \pi_{\phi}(\cdot)} \Bigr[ \mathbb{E}_{\rvy \sim \pi_{\vtheta}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] \nonumber \\
    - &\mathbb{E}_{\rvy \sim \pi^{\star}_{\text{KL}}(\rvy \mid \rvx)} \bigr[ \ r(\rvx, \rvy) \ \bigr] \Bigr].\label{eq:regret-pi}
\end{align}
\end{minipage}

At the equilibrium~\citep{nash}, prior works~\citep{paired} have shown:

% \begin{mdframed}
\begin{rem}[Minimax Regret]
    If the above solver-creator game reaches an equilibrium, the solver follows a minimax regret policy, \ie the worst-case regret is bounded:
\begin{align}
    \tb{\pi^{\star}_{\calY \mid \calX}} \in \underset{ \tb{\pi_{\calY \mid \calX}} }{\arg \min} \  \underset{\tb{\pi_\calX}}{\max} \ \sE_{\rvx \sim \pi_{\calX}}  \ \Bigr[\ \operatorname{Regret}(\rvx, \tb{\pi_{\calY \mid \calX}}) \ \Bigr].\label{eq:minimax-regret}
\end{align}
\end{rem}
% \end{mdframed}
% \vspace{-6pt}
To illustrate, open-ended RLHF allows for the creation of evolving prompt distributions that challenge the agent progressively for better generalization; the introduced minimax regret objective further adds \emph{robustness} on  such evolving curricula by \emph{incentivizing agents to perform well in all cases}. 

% \begin{align}
%     \text{info}(\rvx) \gets \widehat{A}_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') |, \label{eq:info-proxy}
% \end{align}

\paragraph{Regret Minimization for the Solver.} It is rather straightforward to understand the objective of the solver $\pi_{\vtheta}(\cdot \mid \rvx)$ as regret minimization, since the goal is to align the policy $\pi_{\vtheta}(\cdot \mid \rvx)$ with the KL-optimal solution $\pi^{\star}_{\text{KL}}(\cdot \mid \rvx)$, which directly minimizes the KL-regularized regret by design. This formulation allows flexibility in the plug-in preference optimization algorithms for the solver's step in Algorithm~\ref{alg:i-eva}, and ensures the alignment problem is well-defined. In practice, we use variants of REINFORCE~\citep{rloo} for online~\method~and DPO~\citep{dpo} for offline~\method~as the solvers, detailed in $\S$~\ref{sec:exp}.
%by using an oracle preference model for the labeling on the preference pairs. The detailed specifications can be found in $\S$~\ref{sec:exp}.

% \text{info}_{\vtheta}(\rvx) :=

\paragraph{Regret Maximization for the Creator.} As discussed previously, while it is often trivial for the solver to minimize the regret through direct policy optimization, the optimal policy remains unknown during the optimization process, thus we cannot directly calculate the regret -- we must approximate it when using it as the utility for the creator. Similarly to heuristics proposed by prior works~\citep{plr,dcd,accel}, we use the advantage-based estimate:
\begin{align}
    \hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta}) \gets     r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{\text{baseline}}) , 
\end{align}
where
\begin{align}
&\mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \\ \quad &\mathbf{y}_{\text{baseline}} := \operatorname{avg}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}) \text{ or }  {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
\end{align}

and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle. We use ${\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y})$ by default due to its simplicity and efficiency (see also $\S$~\ref{sec:int} for additional interpretation) and consistent strong empirical gains we observed in vast experiments. As the policy optimizes, the proxy should approximate the true regret better. We leave exploration of other informativeness proxy designs in~\method~to future work.


% However, while it is often straightforward for the \textbf{solver} to minimize the regret (\eg by direct policy optimization), the optimal policy remains unknown during optimization, thus regret as the decision signal is often intractable to the \textbf{creator} -- regret approximation is needed. We design the proxy below for creator's  regret approximation (see  $\S$~\ref{app:theory} for further illustration), also as a metric for prompt informativeness:
% \vspace{+0.6pt}
% \begin{mdframed}
% \begin{defn}[Informativeness]\label{def:info-proxy}
%     We estimate the informativeness of a prompt $\rvx$ in preference optimization by the (absolute) worst-case optimal advantage, approximating regret in Eq.~\ref{eq:regret_definition}:
% \begin{align}
%     | \hat{\operatorname{Regret}}(\rvx, \pi_{\vtheta}) | \gets  \text{info}_{\vtheta}(\rvx) :=   r(\rvx, \rvy_{+}) - r(\rvx, \rvy_{-}) , \label{eq:info-proxy}
% \end{align}
% \vspace{-5pt}
% where\vspace{-5pt}
% \begin{align}
% \mathbf{y}_{+} := {\operatorname{arg\,max}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}), \quad \mathbf{y}_{-} := {\operatorname{arg\,min}}_{\mathbf{y}_i} \, r(\mathbf{x}, \mathbf{y}),    
% \end{align}
% and $\{\mathbf{y}_i\}_{i=1}$ is a set of responses sampled from $\pi_{\vtheta}(\cdot \mid \rvx)$ and $r(\cdot, \cdot)$ is the reward oracle.
% % which is estimated by sampling multiple responses for $\rvx$ from the solver and calculating  gap between the maximal reward (from the best $\rvy$) and the minimal reward (from the worst $\rvy$).
% \end{defn}
% \end{mdframed}
% \vspace{-4pt}
% We use the informativeness proxy to guide the creator for prompt distribution adaptation, which has a few useful properties under different interpretations, as in $\S$~\ref{sec:int}. In this way, we define a mechanism that the solver learns to improve, as the creator keeps challenging the solver on its weaknesses.

% \footnote{Some works~\citep{plr,active-pl} tested Shannon entropy, which is empirically found to underperform reward-based metric. We encourage future studies into this.}

% \fix{Add one sentence comment on the implications on the mimax regret; for example: To iterate, our open-ended RLHF objective does not focus on a fixed distribution of prompts, but rather allow for the creation of an evolving distribution that challenges the agent progressively, to ensure it generalize well under unseen, novel scenarios. The minimax regret framework adds a layer of robustness by minimizing the agent's performance gap in worst cases. It is not just about generalizing to novel prompted tasks, but also ..} Without access to the true optimal policy, we must approximate the regret. We design the advantage-based proxy as follows:

% We choose to use variants of advantage functions for the approximation, as shown in Table~\ref{tab:info-metric}, which we also refer as the informativeness proxy\footnote{Note that some works~\citep{plr,active-pl} had tested using Shannon entropy as the informativeness metric, which is known to be hard to precisely estimate and empirically found to underperform reward-based metric. We encourage more future studies into this.}, with $A^{\star}_{\min}$ as the default proxy due to its relation to minimax regret in Eq.~\ref{eq:minimax-regret}.
% \vspace{+1pt}
% \begin{mdframed}
% \begin{defn}[Informativeness Proxy]
%     We use the minimax regret as the proxy for the informativeness metric of the prompt, approximated by the (absolute) worst-case optimal advantage:
% \begin{align}
%     \text{info}(\rvx) \gets A_{\min}^{\star} := | \min_{\rvy} r(\rvx, \rvy) - \max_{\rvy'} r(\rvx, \rvy') | 
% \end{align}
% \end{defn}
% \end{mdframed}
% This proxy enjoys many nice properties under various interpretations, which we illustrate in $\S$~\ref{sec:int}.


\subsection{The Practical Algorithm}~\label{sec:algo}
We now illustrate~\method~of Algorithm~\ref{alg:i-eva}, with practical implementations specified in $\S$~\ref{app:reproduce}. 

% The full pipeline is that we combine the creator and solver step in an iterative preference optimization pipeline.

\subsubsection{The Creator Step:  Estimate, Sample then Evolve}\label{sec:creator-step}\vspace{-2pt}
Plainly, the creator finds most useful prompts and generate variants of them for preference optimization. One may relate this to \emph{evolution strategies}~\citep{schwefel1977evolutionsstrategien} which find the most promising species, then mutate and crossover, or to \emph{curriculum RL}~\citep{accel} which finds environments with high-regret levels, then edits within some distance. In this work, we do not seek a differentiable creator in this work; the creator is implemented in three steps as in Figure~\ref{fig:pipeline} to approximate regret maximization. See more in $\S$~\ref{app:theory}.
\vspace{-6pt}

\paragraph{Step 1: $\texttt{\small info}(\cdot)$ -- \textnormal{\it estimate the informativeness}.} For each $\rvx$ in the  prompt set $\calX_t$, we generate responses, annotate rewards and estimate a informativeness metric to $\rvx$ by Eq.~\ref{eq:info-proxy} (see also Table~\ref{tab:info-metric}). \vspace{-6pt}
% To calculate the empirical value of $A^{\star}_{\min}$ for  each prompt, we first sample multiple responses from the prompt, where we label each response with its reward, then we use the difference between the highest reward $r_{\max}$ and the lowest reward $r_{\min}$ to represent the informativeness proxy.

\paragraph{Step 2: $\texttt{\small sample}(\cdot)$ -- \textnormal{\it weighted sampling for an informative subset}.} By using the informativeness metric as the weight,
we sample an informative prompt subset $\calX_t^{\texttt{\tiny info}}$ to be evolved later. This is similar to finding high-regret levels in curriculum RL~\citep{accel}.\vspace{-6pt}

\paragraph{Step 3: $\texttt{\small evolve}(\cdot)$ -- \textnormal{\it evolving for a proximal region of high-advantage prompts}.} Our algorithm is agnostic to and does not rely on any specific evolving method (see empirical evidence in~\secref{app:exp-evol}). We take \text{EvolInstruct}~\citep{wizardlm} as a default off-the-shelf method, which conducts in-depth (\ie adding constraints, deepening, concretising, complicating) and in-breadth evolving (\ie mutation) for prompts. Specifically, we iterate over each prompt in the $\calX_t^{\texttt{\tiny info}}$, where each one is evolved to multiple variations, then optionally mix the newly generated prompts with a uniformly sampled buffer from $\calX_t$ to create $\calX_{t+1}$.

 % (\eg 20\% of the original)

 % by meta-instruction (\ie using an LLM to re-write the original prompts with the aforementioned evolving directions)


\subsubsection{The Solver Step: Solve then Optimize}\label{sec:solver-step}\vspace{-2pt}
This step is the classical preference optimization~\citep{dpo}, where responses are generated and the gradient descent is performed. Take the pointwise reward model setting as an example, for every prompt, we sample $n$ responses with reward annotated for each; we take the responses with the maximal and the minimal reward to construct the preference pairs, then optimize upon. This implicitly minimizes the regret to the KL-optimal policy, which we present in more details at $\S$~\ref{app:theory}.

% Put together, \method~can unify existing iterative optimization pipeline~\citep{snorkel} with a new creator module, which can either share the same network as the solver policy or operate independently.

% \tc{An important contribution of our work is proposing the metric for preference optimization; so worth having a subsection somewhere on this.}
% (probably point to the appendix on the prompt distribution when we have it).


% \paragraph{Learning potential.} Our metric intuitively captures prompts with high learning potential by distinguishing between those that elicit both high-reward and low-reward responses. This contrast highlights areas where the agent can improve.

% \subsection{Understanding the Informativeness Proxy in Different Intuitive Ways}\label{sec:int}

% \paragraph{Learning potential.} Our metric intuitively identifies the learning potential of a prompt by measuring the gap between the best and worst response to it from the solver. We reason, that prompts eliciting \emph{both} high-reward and low-reward outcomes, reflect \emph{learnable} tasks where the model is capable of improving but has not yet mastered, thereby implying learning potential (\textit{cf.}, \cite{plr}). 
% % The evolving step then generates similar prompts with increased diversity to further promote generalization.
% \vspace{-10pt}
% \paragraph{Worst-case guarantees.} The minimax-regret objective, by design, leads to solvers that  perform robustly across the prompt space, thus gives the worst-case guarantee. While exact equilibrium may not be attainable with approximation,  our empirical results in  $\S$~\ref{sec:ab-metric} demonstrate robustness.
% \vspace{-10pt}
% \paragraph{Auto-curricula for the players.}
% We visualize the curriculum induced by~\method~in $\S$~\ref{app:curr}. With the stochastic policy, the advantage may be heuristically understood as the reward difference between \emph{a base solver} and \emph{a reference solver}. Rather than optimizing separate solvers~\citep{paired}, we sample multiple times from the same policy to create the pair. In this way, the creator is incentivized to produce new prompts that are just out of the comfort zone of solvers~\citep{zone-promximal}:
% \vspace{-6pt}
% \begin{itemize}
%     \item For overly challenging prompts, both solutions perform poorly, leading to a low  proxy.\vspace{+1pt}
%     \item For overly easy prompts, the base solution already performs well, again giving a low proxy.\vspace{+1pt}
%     \item The optimal strategy is to find prompts that are just beyond the solver's current capability.
% \end{itemize}
% \vspace{-2pt}
% \vspace{-10pt}
% \paragraph{Auto-curricula inherent to Contrastive Optimization.} Contrastive preference optimization generalizes DPO and a family of algorithms (\textit{c.f.}, \cite{cpl,dpo,tang2024generalized}), many of whose losses monotonically decrease as the contrastive ratio increases. Here, by Eq.~\ref{eq:reward-re} and Eq.~\ref{eq:contrastive-ratio-main}, the \emph{contrastive ratio} can be written via the \emph{advantage-based proxy}:
% \begin{align}
%     A^{\star}_{\min}(\rvx)  = \beta \cdot \textcolor{black}{\Delta_{{\boldsymbol{\theta}^{\star}};  {\text{ ref}}}^{\rvx}} .
% \end{align}
% By our proxy, we implicitly incentivize the creator to generate prompts that \emph{bring the most contrastive responses}, which decrease the loss the most. This matches the curriculum learning literature, which prioritizes (in~\method, \emph{generatively} prioritizes) examples with smaller losses for better convergence and generalization~\citep{easy-bengio2009curriculum}. We hence suggest the \emphtext{\textit{Contrastive Curriculum Hypothesis}}: in contrastive preference optimization, prioritizing prompts with higher contrastive ratio improves sample efficiency and generalization. We show initial empirical results on this in $\S$~\ref{sec:ab-metric} and $\S$~\ref{sec:ab-cont}.




==> texs_icml/pre-cache-cache.tex <==
% \newpage
\section{Preliminaries}

Classical RL post-training~\citep{ouyang2022training} solves regularized optimization for a \textbf{fixed prompt distribution} $\calD$:
\vspace{-20pt}

\begin{minipage}{1\linewidth}
\small
\begin{align}
    \max_{\pi_\vtheta} \ & \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}
    \Bigl[ r(\rvx, \rvy) \Bigl] \notag \\
     - \ &\mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ 
    \beta \cdot \mathbb{D}_{\mathsf{KL}}\bigl[ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\mathsf{base}}(\rvy \mid \rvx) \bigl] \Bigl], \label{eq:rlhf-cls}
\end{align}
\end{minipage}

where $\pi_{\mathsf{base}}(\rvy | \rvx)$ is a base reference policy, $\rvx$ and $\rvy$ are the prompts and responses, $r(\cdot, \cdot)$ is the reward that is assumed to be from an oracle, effectively $r^{\star}(\cdot, \cdot)$, in this paper.

In practice, depending on how $\rvy$ is generated, RLHF methods can be framed as: (i) \textbf{online}, where $\rvy$ are generated on-policy, \ie $\vy_{(1)}, \ldots, \vy_{(k)} \sim \pi_\vtheta(\cdot | \rvx)$~\citep{rloo}; and (ii) \textbf{offline}, where $\rvy$ are \textit{pre-generated} by human experts or previous model checkpoints~\citep{xiong2024iterative}. 

These methods naturally serve as the \textbf{solver} in \method, which adapts to both under the same principle: in online RL, we evolve prompts at each mini-batch, while in offline RL, we construct new prompt sets after each full iteration.  


% RLHF methods fall into two practices: \textbf{online RL} and \textbf{offline RL}, differing in how $\rvy$ is generated. In online setting~\citep{rloo}, $\rvy$ are generated on-policy, \ie $\rvy_{(1)}, \ldots, \rvy_{(k)} \sim \pi_\vtheta(\cdot | \rvx)$. In offline setting~\citep{xiong2024iterative}, $\rvy$ are \textit{pre-generated} by human experts or its previous iteration. A reward oracle provides feedback on these responses, which is then used to update the policy.

% \begin{itemize}
%     \item \textbf{Online RL (stepwise $\rvy$ generation):} At each optimization step, responses $\rvy_{(1)}, \ldots, \rvy_{(k)} \stackrel{\text{i.i.d.}}{\sim} \pi_\theta(\cdot \mid \rvx)$ on-policy. A reward oracle provides feedback on these responses, which is then used to update the policy (e.g., RLOO).
    
%     \item \textbf{Offline RL (iteration-wise $\rvy$ generation):} Responses are \textit{pre-generated} using a fixed model checkpoint—often from a previous iteration of itself~\citep{sppo, iterative-dpo}. The reward oracle assigns scores to these responses, and optimization is conducted over multiple epochs using the fixed dataset (e.g., DPO).
% \end{itemize}


% Further details are in the Appendix.


% \notes{TODO: discuss RLOO and DPO as representative online and offline RL post-training methods, then finalize preliminary at this page.}



\begin{figure*}[t]
\begin{mdframed}
\begin{defn}[Open-Ended RLHF]\label{eq:rlhf-joint}
We define \emph{evolving alignment} as the open-ended joint optimization  on the prompt and response policy for alignment w.r.t the joint reference policy:
\vspace{-3pt}
\begin{align}
    \max_{\vphi, \vtheta} \  \calJ(\vphi, \vtheta) := \ \mathbb{E}_{\tg{\rvx\sim \pi_{\vphi}(\cdot)}  , \  \tc{\rvy \sim \pi_{\vtheta}(\cdot|\rvx)} \  }    \Biggr[ \ r(\rvx, \rvy) \ \Biggr]
    - \beta \cdot  \sD_{\text{KL}}\Biggl[\ \tb{\pi_{\vphi, \vtheta}(}\tb{\rvx}\tb{, \ } \tb{\rvy}\tb{)} \ \| \ \tb{ \pi_{\mathsf{ref}}(\rvx, \rvy)  } \ \Biggl], \label{eq:rlhf-joint-} \vspace{-5pt}
\end{align}
where $\tb{\pi_{\vphi, \vtheta}(\rvx, \rvy) } := \tb{\pi_{\vphi}(\rvx)} \cdot \tb{\pi_{\vtheta}(\rvy | \rvx)}$ and $\pi_{\mathsf{ref}}(\rvx, \rvy) := p_{\mathsf{ref}}(\rvx) \cdot \pi_{\mathsf{base}}(\rvy | \rvx)$\footnote{\textcolor{black}{This generalizes  classical RLHF (Eq.~\ref{eq:rlhf-cls}). One may extend the above and rewrite coefficients to be:}
\vspace{-6pt}
\begin{align}
\scalebox{0.9}{$ 
\max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbracket{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\mathsf{base}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
- \beta_2 \cdot \tg{\underbracket{\emphgreen{\textcolor{cgreen}{\sD_{\mathsf{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\mathsf{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}.
$}\label{eq:rlhf-expand}
\end{align} \vspace{-10pt}}, and $p_{\mathsf{ref}}(\rvx)$ is an open-ended reference.

\notes{Another way to make this more clear -- remove this joint part, directly use Eq.~\ref{eq:rlhf-expand}, however, removing $p_{\mathsf{ref}}(\rvx)$, instead we put a regularization there. Then the question will be: starting from the initial seed prompt, what would a good $\phi$? or what would be a good sequence of $\phi$? }
% denotes the training joint distribution and the reference joint distribution, respectively.
\end{defn}
\end{mdframed}
\end{figure*}
\vspace{-20pt}

% \resizebox{\textwidth}{!}{$
% \max_{\tb{\vphi}, \tb{\vtheta}} \     \tg{\sE_{\mathbf{x} \sim \pi_{\phi}(\cdot)}}{\tg{\Bigr[ \ }} \tc{\underbrace{\emphred{ \tc{\mathbb{E}_{ {\mathbf{y} \sim \pi_\theta(\cdot \mid \mathbf{x})}} \Bigr[\ r(\mathbf{x}, \mathbf{y}) \ \Bigr] - \beta_1 \cdot {\sD_{\text{KL}}\bigr[{\pi_{\theta}(\rvy \mid \rvx)} \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx)\bigr]}}}}_{\text{\small solver}} }\ \textcolor{cgreen}{\Bigr]} 
% - \beta_2 \cdot \tg{\underbrace{\emphgreen{\textcolor{cgreen}{\sD_{\text{KL}}\Bigr[\ \pi_{\phi}(\rvx) \ \| \  p_{\text{ref}}(\rvx)\ \Bigr]}}}_{\text{\small creator}}}. \nonumber 
% $}

==> texs_icml/pre-cache.tex <==
\newpage
\section{Preliminaries}
We hereby review major concepts, which we later in $\S$~\ref{sec:method} use  \emphtext{\emph{regret}}  and the proxy by  \emphtext{\emph{advantage}} to identify informative prompts, leading to learning curricular implicitly maximizing \emphtext{\emph{contrastive ratio}}.

\vspace{-10pt}
\paragraph{Alignment by RLHF.} Classical RLHF~\citep{ouyang2022training} optimizes on a fixed distribution $\calD$:
% \begin{align}
%     \max _{\pi_\vtheta} \ \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}\Bigl[\ r(\rvx, \rvy) \ \Bigl]- \mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ \beta \cdot \mathbb{D}_{\text{KL}}\bigl[\ \pi_\vtheta(\rvy \mid \rvx) \ \| \ \pi_{\text{SFT}}(\rvy \mid \rvx) \ \bigl] \Bigl],\label{eq:rlhf-cls}
% \end{align}
\begin{minipage}{1\linewidth}
\small
\begin{align}
    \max_{\pi_\vtheta} \ & \mathbb{E}_{\rvx \sim \mathcal{D}, \rvy \sim \pi_\vtheta(\cdot \mid \rvx)}
    \Bigl[ r(\rvx, \rvy) \Bigl] \notag \\
     - \ &\mathbb{E}_{\rvx \sim \mathcal{D}} \Bigl[ 
    \beta \cdot \mathbb{D}_{\text{KL}}\bigl[ \pi_\vtheta(\rvy \mid \rvx) \| \pi_{\text{SFT}}(\rvy \mid \rvx) \bigl] \Bigl],
\end{align}
\end{minipage}

where $\rvx$ and $\rvy$ denote the prompts and responses, and $r(\cdot, \cdot)$ is the reward function.


\paragraph{Reward.} Let the \emph{optimal policy} of Eq.~\ref{eq:rlhf-cls} be $\pi^{\star}(\cdot)$ and $Z(\cdot)$ be the partition function, we have:

\begin{minipage}{1\linewidth}
\small
\begin{align}
    \hspace{+5pt}r(\rvx, \rvy)=\beta \cdot \log \frac{ \pi^{\star}(\rvy \mid \rvx)} {\pi_{\text {\text{SFT}}}(\rvy \mid \rvx)}\textcolor{black}{ \ + \ \beta \cdot \log Z(\rvx)}. \label{eq:reward-re}\vspace{-10pt}
\end{align}
\end{minipage}

\paragraph{Regret and advantage.} Given the optimal policy \( \pi^\star \), the \emph{regret} of a policy \( \pi_{\boldsymbol{\theta}} \) at \( \mathbf{x} \) is:
\vspace{-10pt}
\begin{minipage}{1\linewidth}
\small
\begin{align}
    \operatorname{Regret}(\mathbf{x}, \pi_{\boldsymbol{\theta}}) = \mathbb{E}_{\mathbf{y} \sim \pi^\star(\cdot \mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr] - \mathbb{E}_{\mathbf{y} \sim \pi_{\boldsymbol{\theta}}(\cdot\mid \mathbf{x})} \Bigr[ r(\mathbf{x}, \mathbf{y}) \Bigr]. \nonumber
    % \label{eq:regret_definition}
\end{align}
\end{minipage}

The \emph{advantage} function quantifies how much better a response $\rvy$ is \emph{w.r.t.} a baseline:
\begin{align}
    \hspace{+8pt}A(\rvx, \rvy) = r(\rvx, \rvy) - \mathbb{E}_{\rvy' \sim \pi(\cdot \mid \rvx)} \Bigr[ \ r(\rvx, \rvy') \ \Bigr]. \label{eq:advantage-definition}
\end{align}
Variants of advantage (\eg the worst-case advantage $A^{\star}_{\min}$) are related to regret, as shown in Table~\ref{tab:info-metric}.



\vspace{-10pt}
\paragraph{Direct preference optimization.} The DPO~\citep{dpo} objective for RLHF is:
\begin{align}
    \hspace{+16pt}\calL_{\beta}^{\text{DPO}}(\pi_\vtheta) = \sum_{\left(\rvy_{+} , \rvy_{-}, \rvx \right) \in \mathcal{D}} - \log \Bigr[\sigma \bigr(\beta \cdot  \Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx} \bigr)\Bigr],
\end{align}
where we use $+, -$ to denote chosen and rejected responses, and denote the \textbf{contrastive ratio} as:
\begin{align}
\hspace{+16pt}\Delta_{{\boldsymbol{\theta}};  {\text{ ref}}}^{\rvx}:=\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{+} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{+} \mid \rvx\right)}-\log \frac{\pi_{\boldsymbol{\theta}}\left(\rvy_{-} \mid \rvx\right)}{\pi_{\text{ref}}\left(\rvy_{-} \mid \rvx\right)}. \label{eq:contrastive-ratio-main}
\end{align}
By reward reparameterization with Eq.~\ref{eq:reward-re},  variants of advantage also relate to contrastive ratio, as in $\S$~\ref{sec:int}.




